A review of UAV Visual Detection and Tracking Methods

This paper presents a review of techniques used for the detection and tracking of UAVs or drones. There are different techniques that depend on collecting measurements of the position, velocity, and image of the UAV and then using them in detection and tracking. Hybrid detection techniques are also presented. The paper is a quick reference for a wide spectrum of methods that are used in the drone detection process.

==> 01_Intro.tex <==
\section{Introduction} 
\label{sec:Intro}



==> 02_Background.tex <==
\section{Background}\label{sec:Background}

\subsection{UAV fundamentals}
\subsection{UAV types}


==> All_UAV_doc_Scopus.tex <==

@ARTICLE{Zhao2022,
author={Zhao, M. and Fang, Z. and Yang, H. and Cheng, L. and Chen, J. and Xie, C.},
title={Uavc: A new method for correcting lidar overlap factors based on unmanned aerial vehicle vertical detection},
journal={Applied Sciences (Switzerland)},
year={2022},
volume={12},
number={1},
art_number={184},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85121697130&doi=10.3390\%2fapp12010184&partnerID=40&md5=6c2bf7c5822242d099be51677cc3dd62},
abstract={A method to calibrate the overlap factor of Lidar is proposed, named unmanned aerial vehicle correction (UAVC), which uses unmanned aerial vehicles (UAVs) to detect the vertical distribution of particle concentrations. The conversion relationship between the particulate matter concentration and the aerosol extinction coefficient is inverted by the high-altitude coincidence of the vertical detection profiles of the UAV and Lidar. Using this conversion relationship, the Lidar signal without the influence of the overlap factor can be inverted. Then, the overlap factor profile is obtained by comparing the signal with the original Lidar signal. A 355 nm Raman-Mie Lidar and UAV were used to measure overlap factors under different weather conditions. After comparison with the Raman method, it is found that the overlap factors calculated by the two methods are in good agreement. The changing trend of the extinction coefficient at each height is relatively consistent, after comparing the inversion result of the corrected Lidar signal with the ground data. The results show that after the continuously measured Lidar signal is corrected by the overlap factor measured by this method, low-altitude aerosol information can be effectively obtained. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@ARTICLE{Bouguettaya2022,
author={Bouguettaya, A. and Zarzour, H. and Taberkit, A.M. and Kechida, A.},
title={A review on early wildfire detection from unmanned aerial vehicles using deep learning-based computer vision algorithms},
journal={Signal Processing},
year={2022},
volume={190},
art_number={108309},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85114741439&doi=10.1016%2fj.sigpro.2021.108309&partnerID=40&md5=c698f5a42a16439b5201e0379c5cea87},
abstract={Wildfire is one of the most critical natural disasters that threaten wildlands and forest resources. Traditional firefighting systems, which are based on ground crew inspection, have several limits and can expose firefighters’ lives to danger. Thus, remote sensing technologies have become one of the most demanded strategies to fight against wildfires, especially UAV-based remote sensing technologies. They have been adopted to detect forest fires at their early stages, before becoming uncontrollable. Autonomous wildfire early detection from UAV-based visual data using different deep learning algorithms has attracted significant interest in the last few years. To this end, in this paper, we focused on wildfires detection at their early stages in forest and wildland areas, using deep learning-based computer vision algorithms to prevent and then reduce disastrous losses in terms of human lives and forest resources. © 2021 Elsevier B.V.},
}

@ARTICLE{Idhis2022429,
author={Idhis, S.M. and Dawdi, T. and Nasir, Q. and Talib, M.A. and Omran, Y.},
title={Detection and Localization of Unmanned Aerial Vehicles Based on Radar Technology},
journal={Lecture Notes in Networks and Systems},
year={2022},
volume={218},
pages={429-452},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113369662&doi=10.1007%2f978-981-16-2164-2_34&partnerID=40&md5=f33f1a4667a115535f1a9a7c598a8920},
abstract={Ever since unmanned aerial vehicles (UAV), also known as drones, became available for civilian use, their risks increased. Along with that, the need to control and monitor them increased rapidly. In the literature, many researchers explored different techniques and developed genuine and hybrid systems to counter UAVs. These systems are not only found in academia, but different commercial options are also available. In this paper, the detection and localization using radar systems method are addressed. This method is one way to thwart drones. Other approaches are briefed in the background of this research study. Different radar technologies exist, and consequently different approaches to apply UAV detection and localization using radars. These approaches that are addressed in academia and the industry are surveyed in this research paper. Furthermore, the different possible radar categories are detailed to help the reader understand radar technology and thus its applications. In addition to commonly used localization algorithms for UAVs, the software and hardware implementation methods are also surveyed in this paper. © 2022, The Author(s), under exclusive license to Springer Nature Singapore Pte Ltd.},
}

@ARTICLE{Wang2022946,
author={Wang, R. and Zou, J.},
title={Vision-Based Landing Site Detection for Unmanned Aerial Vehicle: A Review},
journal={Lecture Notes on Data Engineering and Communications Technologies},
year={2022},
volume={80},
pages={946-954},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85111899878&doi=10.1007%2f978-3-030-81007-8_108&partnerID=40&md5=2d76d90da7c23d9a115d993a949c831a},
abstract={Autonomous landing technique for Unmanned Aerial Vehicle (UAV) is a well-studied problem, for most flight accidents happened during this stage. This survey aims to provide an extensive overview for a guide for vision-based autonomous landing site detection development. According to whether an auxiliary marker is set, the detection tactics can be categorized as marker-aided and markerless ones. Marker-aided tactics usually employ an elaborate and distinctive geometric design to achieve robust detection efficiently. While the markerless tactics can be further decomposed into two main steps: pattern recognition and flat site detection. Moreover, the computational optics theory and deep learning are now showing extraordinary talents in mobile platforms including UAV, thus we elaborate monocular depth estimation with different supervision methods for flatness analysis in markless tactics. We hope our comprehensive overview may possibly be helpful in the analysis and improving the vision-based autonomous landing technique for UAV. © 2022, The Author(s), under exclusive license to Springer Nature Switzerland AG.},
}

@ARTICLE{Zheng2022936,
author={Zheng, Y. and Zhang, X. and Liu, H. and Xing, K.},
title={A Fast Position Estimation Method of Near-Surface Targets Detection for Unmanned Aerial Vehicle Magnetic Surveys},
journal={Lecture Notes on Data Engineering and Communications Technologies},
year={2022},
volume={80},
pages={936-945},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85111799155&doi=10.1007%2f978-3-030-81007-8_107&partnerID=40&md5=44369d4a219049509a18af75197b76bc},
abstract={In recent years, unmanned aerial vehicle magnetic survey system has been widely used in geophysical exploration and other fields because of its high efficiency and low cost. However, the lack of effective data interpretation methods limits its development. In this paper, the magnetic field distribution of the near-surface targets was analyzed, and the locations of the targets were estimated by using the characteristic points of the magnetic anomaly profiles. The relationship between the location and buried depth of the target and the characteristic points of the anomaly profile was established by multiple regression. Field experiments have been carried out, the positioning deviation of the results obtained by the proposed method was less than 0.25 m, and the location accuracy was higher than the traditional Euler deconvolution method. The results showed that this simple method can provide a preliminary estimation of the locations of near-surface targets without losing effectiveness. © 2022, The Author(s), under exclusive license to Springer Nature Switzerland AG.},
}

@ARTICLE{Merlino2021,
author={Merlino, S. and Paterni, M. and Locritani, M. and Andriolo, U. and Gonçalves, G. and Massetti, L.},
title={Citizen science for marine litter detection and classification on unmanned aerial vehicle images},
journal={Water (Switzerland)},
year={2021},
volume={13},
number={23},
art_number={3349},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85120155768&doi=10.3390%2fw13233349&partnerID=40&md5=4bc1b2ba0cd0d549c4f0b1452fc47611},
abstract={Unmanned aerial vehicles (UAV, aka drones) are being used for mapping macro-litter in the environment. As drone images require a manual processing task for detecting marine litter, it is of interest to evaluate the accuracy of non-expert citizen science operators (CSO) in performing this task. Students from Italian secondary schools (in this work, the CSO) were invited to identify, mark, and classify stranded litter items on a UAV orthophoto collected on an Italian beach. A specific training program and working tools were developed for the aim. The comparison with the standard in situ visual census survey returned a general underestimation (50%) of items. However, marine litter bulk categorisation was fairly in agreement with the in situ survey, especially for sources classification. The concordance level among CSO ranged between 60% and 91%, depending on the item properties considered (type, material, and colour). As the assessment accuracy was in line with previous works developed by experts, remote detection of marine litter on UAV images can be improved through citizen science programs, upon an appropriate training plan and provision of specific tools. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@ARTICLE{Wang2021,
author={Wang, Z. and Zhang, X. and Li, J. and Luan, K.},
title={A yolo-based target detection model for offshore unmanned aerial vehicle data},
journal={Sustainability (Switzerland)},
year={2021},
volume={13},
number={23},
art_number={12980},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85119983856&doi=10.3390%2fsu132312980&partnerID=40&md5=ebdf5d8483a48c795db626da214b39d4},
abstract={Target detection in offshore unmanned aerial vehicle data is still a challenge due to the complex characteristics of targets, such as multi-sizes, alterable orientation, and complex backgrounds. Herein, a YOLO-based detection model (YOLO-D) was proposed for target detection in offshore unmanned aerial vehicle data. Based on the YOLOv3 network, the residual module was improved by establishing dense connections and adding a dual-attention mechanism (CBAM) to enhance the use of features and global information. Then, the loss function of the YOLO-D model was added to the weight coefficients to increase detection accuracy for small-size targets. Finally, the feature pyramid network (FPN) was replaced by the secondary recursive feature pyramid network to reduce the impacts of a complicated environment. Taking the car, boat, and deposit near the coastline as the targets, the proposed YOLO-D model was compared against other models, including the faster R-CNN, SSD, YOLOv3, and YOLOv5, to evaluate its detection performance. The results showed that the evaluation metrics of the YOLO-D model, including precision (Pr), recall (Re), average precision (AP), and the mean of average precision (mAP), had the highest values. The mAP of the YOLO-D model increased by 37.95%, 39.44%, 28.46%, and 5.08% compared to the faster R-CNN, SSD, YOLOv3, and YOLOv5, respectively. The AP of the car, boat, and deposit reached 96.24%, 93.70%, and 96.79% respectively. Moreover, the YOLO-D model had a higher detection accuracy than other models, especially in the detection of small-size targets. Collectively, the proposed YOLO-D model is a suitable model for target detection in offshore unmanned aerial vehicle data. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@ARTICLE{Zhu2021,
author={Zhu, H. and Liu, C. and Li, M. and Shang, B. and Liu, M.},
title={Unmanned aerial vehicle passive detection for Internet of Space Things},
journal={Physical Communication},
year={2021},
volume={49},
art_number={101474},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85117908654&doi=10.1016%2fj.phycom.2021.101474&partnerID=40&md5=9da8eb20221598f10df0aafe4edcc9dc},
abstract={Unmanned aerial vehicle (UAV) passive detection is an essential part of intelligent surveillance in the Internet of Space Things (IoST). The satellite has the potential to play a vital role in many applications of IoST. This paper proposes a novel UAV passive detection using multiple satellites. Specifically, we consider target detection in the ground dual receiver system, which is divided into reference channel and monitoring channel. The reference channel receives the direct wave signals from multiple external emitters, and the monitoring channel receives the echo signals reflected by the UAV. We propose a multiple satellite joint target detection method based on a generalized likelihood ratio test (GLRT). This detection algorithm is robust to the reference channel noise. According to the known or unknown noise variance and interference targets, the conditions are divided into three types, where we use GLRT to design the detectors under different conditions. Extensive simulations are conducted to evaluate the performance of the algorithm under various parameter settings. © 2021 Elsevier B.V.},
}

@ARTICLE{Zhang20211436,
author={Zhang, L.-G. and Jiang, Y.-X. and Tian, G.-J.},
title={Research on Unmanned Aerial Vehicle to Ground Vehicle Target Detection Algorithm Based on Multiscale Fusion Method [基于多尺度融合方法的无人机对地车辆目标检测算法研究]},
journal={Jiliang Xuebao/Acta Metrologica Sinica},
year={2021},
volume={42},
number={11},
pages={1436-1442},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85121828182&doi=10.3969%2fj.issn.1000-1158.2021.11.05&partnerID=40&md5=788e9a76a8f54986c6e47badba99ab5a},
abstract={With the development of drone technology, the use of drone images for ground vehicle target recognition is of great significance both in rescue and disaster relief and in traffic management. However, in actual use, due to the flight height and other reasons, the target in the image is generally small in size and the feature information is not obvious. It is difficult to detect the target using existing algorithms. Therefore, an image multi-target detection method based on multi-scale fusion is proposed. Using Faster R-CNN as the basic framework, the feature information of different levels is fused, and the context information is combined to realize the detection of small targets in unmanned aerial vehicle images. The VisDrone dataset is used to perform ground inspection on ground vehicles. Experiments have shown that the detection of ground vehicle targets by drones has achieved good results. The accuracy of the algorithm used has reached 88%, which is an increase of 3.8% compared with other algorithms the above. © 2021, Acta Metrologica Sinica Press. All right reserved.},
}

@ARTICLE{Bravo2021,
author={Bravo, D.T. and Lima, G.A. and Alves, W.A.L. and Colombo, V.P. and Djogbénou, L. and Pamboukian, S.V.D. and Quaresma, C.C. and Araujo, S.A.D.},
title={Automatic detection of potential mosquito breeding sites from aerial images acquired by unmanned aerial vehicles},
journal={Computers, Environment and Urban Systems},
year={2021},
volume={90},
art_number={101692},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85112357688&doi=10.1016%2fj.compenvurbsys.2021.101692&partnerID=40&md5=bf8c2e3300a303d3b41603cfdfe418c7},
abstract={The World Health Organization (WHO) has stated that effective vector control measures are critical to achieving and sustaining reduction of vector-borne infectious disease incidence. Unmanned aerial vehicles (UAVs), popularly known as drones, can be an important technological tool for health surveillance teams to locate and eliminate mosquito breeding sites in areas where vector-borne diseases such as dengue, zika, chikungunya or malaria are endemic, since they allow the acquisition of aerial images with high spatial and temporal resolution. Currently, though, such images are often analyzed through manual processes that are excessively time-consuming when implementing vector control interventions. In this work we propose computational approaches for the automatic identification of objects and scenarios suspected of being potential mosquito breeding sites from aerial images acquired by drones. These approaches were developed using convolutional neural networks (CNN) and Bag of Visual Words combined with the Support Vector Machine classifier (BoVW + SVM), and their performances were evaluated in terms of mean Average Precision - mAP-50. In the detection of objects using a CNN YOLOv3 model the rate of 0.9651 was obtained for the mAP-50. In the detection of scenarios, in which the performances of BoVW+SVM and a CNN YOLOv3 were compared, the respective rates of 0.6453 and 0.9028 were obtained. These findings indicate that the proposed CNN-based approaches can be used to identify potential mosquito breeding sites from images acquired by UAVs, providing substantial improvements in vector control programs aiming the reduction of mosquito-breeding sources in the environment. © 2021 Elsevier Ltd},
}

@CONFERENCE{Evita2021,
author={Evita, M. and Seno, S. and Zakiyyatuddin, A. and Muid, A. and Djamal, M.},
title={Application of UAV (Unmanned Aerial Vehicle) Photogrammetry for Forest Fire Early Detection System},
journal={IOP Conference Series: Earth and Environmental Science},
year={2021},
volume={830},
number={1},
art_number={012025},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85117408529&doi=10.1088%2f1755-1315%2f830%2f1%2f012025&partnerID=40&md5=6e9e36b9866f5f6fd2e1ee464b256555},
abstract={Indonesia has 15 big potential forest fires locations which destroyed twice the area annually. Moreover, there are almost 20 fire points for each location which increase gradually according to the satellite images of LAPAN (Lembaga Penerbangan dan Antariksa Nasional - National Institute of Aeronautics and Space of Indonesia). Therefore, some monitoring and early warning system for this disaster are needed to minimize the loss and damage of forest ecosystem, smoke exposure to human respiratory system, aviation business, and some forest related industries. Unmanned Aerial Vehicle (UAV) technology could be proposed as the alternative to solve this problem. The forest is monitored by an UAV, in other hand it could be used for image data acquisition to construct 2D and 3D maps for further analysis of the early warning system. The images of sampling location had been taken by an UAV - DJI Phantom 4 Pro which automatically controlled by a flight plan using Pix4D Capture and processed by Pix4D Mapper. The sampling location took place in different areas: near a building, few km squares of campus area consists of building-vegetation combination, and three forest locations in two active volcanoes. The maps with Ground Sample Distance (GSD) under 3 cm/pixel result in under 1% error for X, Y and Z of 2D and 3D constructed maps. The maps also show an important finding where the movement object could be detected, which potential to be applied for fire evolution detection of a forest fire early warning system. © Published under licence by IOP Publishing Ltd.},
}

@CONFERENCE{Vu2021,
author={Vu, H.N. and Nguyen, H.M. and Pham, C.D. and Tran, A.D. and Trong, K.N. and Pham, C. and Nguyen, V.H.},
title={Landslide Detection with Unmanned Aerial Vehicles},
journal={2021 International Conference on Multimedia Analysis and Pattern Recognition, MAPR 2021 - Proceedings},
year={2021},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85119275621&doi=10.1109%2fMAPR53640.2021.9585261&partnerID=40&md5=506f93dfdf8c22d62305f61aeee31844},
abstract={Landslide is one of the most dangerous disasters, especially for countries with large mountainous terrain. It causes a great damage to lives, infrastructure and environments, such as traffic congestion and high accidents. Therefore, automated landslide detection is an important task for warning and reducing its consequences such as blocked traffic or traffic accidents. For instance, people approaching the disaster area can adjust their routes to avoid blocked roads, or dangerous traffic signs can be positioned in time to warn the traffic participants to avoid the interrupted road ahead. This paper proposes a method to detect blocked roads caused by landslide by utilizing images captured from Unmanned Aerial Vehicles (UAV). The proposed method comprises of three components: road segmentation, blocked road candidate extraction, and blocked road classification, which is leveraged by a multi-stage convolutional neural network model. Our experiments demonstrate that the proposed method can surpass over several state-of-the art methods on our self-collected dataset of 400 images captured with an UAV. © 2021 IEEE.},
}

@ARTICLE{Alkinani2021,
author={Alkinani, M.H. and Almazroi, A.A. and Jhanjhi, N.Z. and Khan, N.A.},
title={5g and iot based reporting and accident detection (Rad) system to deliver first aid box using unmanned aerial vehicle},
journal={Sensors},
year={2021},
volume={21},
number={20},
art_number={6905},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85117100453&doi=10.3390%2fs21206905&partnerID=40&md5=ccf15f1e7ba56418b41d6d82c37ff163},
abstract={Internet of Things (IoT) and 5G are enabling intelligent transportation systems (ITSs). ITSs promise to improve road safety in smart cities. Therefore, ITSs are gaining earnest devotion in the industry as well as in academics. Due to the rapid increase in population, vehicle numbers are increasing, resulting in a large number of road accidents. The majority of the time, casualties are not appropriately discovered and reported to hospitals and relatives. This lack of rapid care and first aid might result in life loss in a matter of minutes. To address all of these challenges, an intelligent system is necessary. Although several information communication technologies (ICT)-based solutions for accident detection and rescue operations have been proposed, these solutions are not compatible with all vehicles and are also costly. Therefore, we proposed a reporting and accident detection system (RAD) for a smart city that is compatible with any vehicle and less expensive. Our strategy aims to improve the transportation system at a low cost. In this context, we developed an android application that collects data related to sound, gravitational force, pressure, speed, and location of the accident from the smartphone. The value of speed helps to improve the accident detection accuracy. The collected information is further processed for accident identification. Additionally, a navigation system is designed to inform the relatives, police station, and the nearest hospital. The hospital dispatches UAV (i.e., drone with first aid box) and ambulance to the accident spot. The actual dataset from the Road Safety Open Repository is used for results generation through simulation. The proposed scheme shows promising results in terms of accuracy and response time as compared to existing techniques. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@ARTICLE{Zhu2021,
author={Zhu, H. and Liu, C. and Li, M. and Shang, B. and Liu, M.},
title={Passive detection of unmanned aerial vehicle in space-air-ground integrated networks},
journal={Physical Communication},
year={2021},
volume={48},
art_number={101439},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85112345292&doi=10.1016%2fj.phycom.2021.101439&partnerID=40&md5=0af0f44ed5fe4e3931fbd251a6549b5b},
abstract={Passive detection of unmanned aerial vehicle (UAV) is an important part of surveillance. Satellite has the potential to play a key role in many applications of space-air-ground integrated networks (SAGIN). In this paper, we propose a novel passive detection method for UAV based on Rao detection. Two hypotheses of UAV detection features are proposed when constructing the signal model. Under this condition, the Rao detection method is extended to weak echo signal detection in a multi-satellite scene. When the noise variance is unknown, two different Rao detectors are designed according to the existence of an interfering target. Moreover, the two detectors’ detection thresholds are obtained given the false alarm probability, respectively. Then, the detection performance of the two detectors is analyzed. Finally, we evaluate the Rao detection performance in different situations with extensive simulations. © 2021 Elsevier B.V.},
}

@ARTICLE{ShahAlam2021,
author={Shah Alam, M. and Oluoch, J.},
title={A survey of safe landing zone detection techniques for autonomous unmanned aerial vehicles (UAVs)},
journal={Expert Systems with Applications},
year={2021},
volume={179},
art_number={115091},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85105319161&doi=10.1016%2fj.eswa.2021.115091&partnerID=40&md5=d797f532741a57dccad2d1a757a4f9a2},
abstract={The age of automation is upon us. Few decades earlier, nearly all the flying vehicles were human-controlled. Nowadays, almost every air vehicle is partially automated or getting closer to full automation. This race towards full automation has led to the introduction of features like autopilot. Unmanned aerial vehicles (UAVs) are the tiniest version of all types of air vehicles. The widespread usage of autonomous UAVs has spawned the need for safe landing zone (SLZ) detection techniques for UAV landing. A SLZ detection becomes an important face of a mission when the UAV needs emergency landing due to the technical difficulties or adverse weather conditions on the way of its operation. Before directly proceeding for landing, a UAV has to decide whether the landing zones are safe or not. On-board visual sensors provide potential information of the ground surface in the form of image or signal. Different image processing and safe landing area detection (SLAD) algorithms are then used to identify the best possible landing sites from the input data. In this survey, we discuss indoor and outdoor landing zone detection techniques. We further classify outdoor landing zones as either static or dynamic and discuss existing literature in the specific categories. We critique the shortcomings of existing SLZ detection techniques while also acknowledging their contributions. Further, we point to potential areas of improvement and future directions of the safe landing zone detection algorithms we surveyed. This survey paper may be a useful tutorial for understanding the types of landing zones and landing zone detection techniques for the UAVs, the strengths of zone detection algorithms, and the open areas for future improvement and research. © 2021 Elsevier Ltd},
}

@ARTICLE{Niwa2021541,
author={Niwa, H.},
title={Detection of organic tea farms based on the density of spider webs using aerial photography with an unmanned aerial vehicle (UAV)},
journal={Landscape and Ecological Engineering},
year={2021},
volume={17},
number={4},
pages={541-546},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85102733341&doi=10.1007%2fs11355-021-00454-x&partnerID=40&md5=e91c857f446b131fb597fc1b09920388},
abstract={Organic tea farms promote biodiversity and perform important ecological functions that benefit the environment and supply safe and secure products to consumers. The study of organic farming requires field study to identify and collect species on site. I proposed the use of aerial photography obtained by an unmanned aerial vehicle (UAV) to identify tea farms that provided a habitat for spiders. In this study, two locations were selected in tea farms near the town of Wazuka, in Kyoto Prefecture, Japan. Aerial photographs were taken after confirming conditions on the ground were right for maximum contrast because the spider webs appearing white when the right atmospheric conditions highlight fine water droplets adhering to the strands in the webs. This occurs when the temperature and humidity combine in such a way as to cause moisture to condense from the atmosphere, also known as the dew point. When this occurs, the webs appear white in daylight and are easily identified by visual orthomosaic images obtained from the UAV. The spatial distribution of spider webs varied as a function of farming method used in different sections of the farms. The results of the visual analysis showed that the density of spider webs correlates with the type of farming method. Sections in which organic farming methods were practiced showed the highest density of webs, followed by sections of conventional farming (extensive cultivation), and lastly, sections using conventional farming methods had the lowest density of webs. The density was easily estimated from orthomosaic images constructed from aerial photographs and demonstrated that organic tea farms can be distinguished from farms employing conventional farming methods based on this criterion. © 2021, International Consortium of Landscape and Ecological Engineering.},
}

@CONFERENCE{Karreddula202150,
author={Karreddula, K.S. and Deb, A.K.},
title={Detection of Normal and Abnormal Conditions for Boundary Surveillance using Unmanned Aerial Vehicle},
journal={2021 International Symposium of Asian Control Association on Intelligent Robotics and Industrial Automation, IRIA 2021},
year={2021},
pages={50-56},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85119092233&doi=10.1109%2fIRIA53009.2021.9588734&partnerID=40&md5=a640a30b60ac3855c72740d35db291ec},
abstract={There are several advanced methods to detect objects, humans, etc., which requires large dataset for training. In this paper, a difference of difference (DoD) technique has been proposed to detect normal and abnormal conditions with minimal dataset during surveillance. This dataset has been used for setting a threshold value to detect condition without training. Captured images have been compared with created dataset toget net difference value and this value has been compared with the threshold value to detect normal and abnormal conditions. This technique can be used at no-man zone areas, boundaries and security borders, and also it can be used as a front-liner along with any advanced technique for surveillance application. This method has been simulated on real images using MATLAB and conducted practical experiment using quad rotor, RPi and ROS. © 2021 IEEE.},
}

@ARTICLE{Lee2021,
author={Lee, D. and Park, W. and Nam, W.},
title={Autonomous landing of micro unmanned aerial vehicles with landing-assistive platform and robust spherical object detection},
journal={Applied Sciences (Switzerland)},
year={2021},
volume={11},
number={18},
art_number={8555},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85115245628&doi=10.3390%2fapp11188555&partnerID=40&md5=8c5ce958e21542b4a1aab83226a64841},
abstract={Autonomous unmanned aerial vehicle (UAV) landing can be useful in multiple applications. Precise landing is a difficult task because of the significant navigation errors of the global positioning system (GPS). To overcome these errors and to realize precise landing control, various sensors have been installed on UAVs. However, this approach can be challenging for micro UAVs (MAVs) because strong thrust forces are required to carry multiple sensors. In this study, a new autonomous MAV landing system is proposed, in which a landing platform actively assists vehicle landing. In addition to the vision system of the UAV, a camera was installed on the platform to precisely control the MAV near the landing area. The platform was also designed with various types of equipment to assist the MAV in searching, approaching, alignment, and landing. Furthermore, a novel algorithm was developed for robust spherical object detection under different illumination conditions. To validate the proposed landing system and detection algorithm, 80 flight experiments were conducted using a DJI TELLO drone, which successfully landed on the platform in every trial with a small landing position average error of 2.7 cm. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@ARTICLE{Xu2021,
author={Xu, D. and Zhao, Y. and Jiang, Y. and Zhang, C. and Sun, B. and He, X.},
title={Using improved edge detection method to detect mining-induced ground fissures identified by unmanned aerial vehicle remote sensing},
journal={Remote Sensing},
year={2021},
volume={13},
number={18},
art_number={3652},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85115101864&doi=10.3390%2frs13183652&partnerID=40&md5=0834d18f8216e884737b8af5d1066c1a},
abstract={Information on the ground fissures induced by coal mining is important to the safety of coal mine production and the management of environment in the mining area. In order to identify these fissures timely and accurately, a new method was proposed in the present paper, which is based on an unmanned aerial vehicle (UAV) equipped with a visible light camera and an infrared camera. According to such equipment, edge detection technology was used to detect mining-induced ground fissures. Field experiments show high efficiency of the UAV in monitoring the mining-induced ground fissures. Furthermore, a reasonable time period between 3:00 am and 5:00 am under the studied conditions helps UAV infrared remote sensing identify fissures preferably. The Roberts operator, Sobel operator, Prewitt operator, Canny operator and Laplacian operator were tested to detect the fissures in the visible image, infrared image and fused image. An improved edge detection method was proposed which based on the Laplacian of Gaussian, Canny and mathematical morphology operators. The peak signal-to-noise rate, effective edge rate, Pratt’s figure of merit and F-measure indicated that the proposed method was superior to the other methods. In addition, the fissures in infrared images at different times can be accurately detected by the proposed method except at 7:00 am, 1:00 pm and 3:00 pm. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@ARTICLE{Xia2021,
author={Xia, L. and Zhang, R. and Chen, L. and Li, L. and Yi, T. and Wen, Y. and Ding, C. and Xie, C.},
title={Evaluation of deep learning segmentation models for detection of pine wilt disease in unmanned aerial vehicle images},
journal={Remote Sensing},
year={2021},
volume={13},
number={18},
art_number={3594},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85114685703&doi=10.3390%2frs13183594&partnerID=40&md5=df6976f62fd8816e931e72015fe87af6},
abstract={Pine wilt disease (PWD) is a serious threat to pine forests. Combining unmanned aerial vehicle (UAV) images and deep learning (DL) techniques to identify infected pines is the most efficient method to determine the potential spread of PWD over a large area. In particular, image segmentation using DL obtains the detailed shape and size of infected pines to assess the disease’s degree of damage. However, the performance of such segmentation models has not been thoroughly studied. We used a fixed-wing UAV to collect images from a pine forest in Laoshan, Qingdao, China, and conducted a ground survey to collect samples of infected pines and construct prior knowledge to interpret the images. Then, training and test sets were annotated on selected images, and we obtained 2352 samples of infected pines annotated over different backgrounds. Finally, high-performance DL models (e.g., fully convolutional networks for semantic segmentation, DeepLabv3+, and PSPNet) were trained and evaluated. The results demonstrated that focal loss provided a higher accuracy and a finer boundary than Dice loss, with the average intersection over union (IoU) for all models increasing from 0.656 to 0.701. From the evaluated models, DeepLLabv3+ achieved the highest IoU and an F1 score of 0.720 and 0.832, respectively. Also, an atrous spatial pyramid pooling module encoded multiscale context information, and the encoder–decoder architecture recovered location/spatial information, being the best architecture for segmenting trees infected by the PWD. Furthermore, segmentation accuracy did not improve as the depth of the backbone network increased, and neither ResNet34 nor ResNet50 was the appropriate backbone for most segmentation models. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@ARTICLE{Chen2021,
author={Chen, P. and Ma, X. and Wang, F. and Li, J.},
title={A new method for crop row detection using unmanned aerial vehicle images},
journal={Remote Sensing},
year={2021},
volume={13},
number={17},
art_number={3526},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85114556111&doi=10.3390%2frs13173526&partnerID=40&md5=b58698ff494a48450a4b38b72ca0b16e},
abstract={Crop row detection using unmanned aerial vehicle (UAV) images is very helpful for precision agriculture, enabling one to delineate site-specific management zones and to perform precision weeding. For crop row detection in UAV images, the commonly used Hough transform-based method is not sufficiently accurate. Thus, the purpose of this study is to design a new method for crop row detection in orthomosaic UAV images. For this purpose, nitrogen field experiments involving cotton and nitrogen and water field experiments involving wheat were conducted to create different scenarios for crop rows. During the peak square growth stage of cotton and the jointing growth stage of wheat, multispectral UAV images were acquired. Based on these data, a new crop detection method based on least squares fitting was proposed and compared with a Hough transform-based method that uses the same strategy to preprocess images. The crop row detection accuracy (CRDA) was used to evaluate the performance of the different methods. The results showed that the newly proposed method had CRDA values between 0.99 and 1.00 for different nitrogen levels of cotton and CRDA values between 0.66 and 0.82 for different nitrogen and water levels of wheat. In contrast, the Hough transform method had CRDA values between 0.93 and 0.98 for different nitrogen levels of cotton and CRDA values between 0.31 and 0.53 for different nitrogen and water levels of wheat. Thus, the newly proposed method outperforms the Hough transform method. An effective tool for crop row detection using orthomosaic UAV images is proposed herein. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@CONFERENCE{Wang2021,
author={Wang, Z. and Yu, Z. and Liu, Y. and Song, H.},
title={Abnormal Data Detection of Unmanned Aerial Vehicles Based on Double Shortcuts ZB-ResNet},
journal={Proceedings of 2021 IEEE International Conference on Signal Processing, Communications and Computing, ICSPCC 2021},
year={2021},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85118455652&doi=10.1109%2fICSPCC52875.2021.9564996&partnerID=40&md5=ab265db10a633461810d2be2ebfda843},
abstract={Unmanned aerial vehicles (UAVs) are unmanned aircrafts operated by radio remote control and programmed control equipment. Due to their small size, low cost, and high flexibility, UAV s are widely used in military and civilian fields. Along with the broad applications of UAVs and the significant advancement of information technologies, they also face cyber threats. Among them, false spoofing is a typical cyber-Attack. If this attack hits UAV s, it could result in damage to property and the release of private data or classified documents. In this paper, we propose the Double Shortcuts Zero-Bias Residual Network (Double Shortcuts ZB-ResNet) with small storage capacity and low time complexity for abnormal data detection of UAVs. It is designed by combining double shortcuts residual blocks and Zero-Bias (ZB) fully connected layer to anomaly detections. By comparing with the experimental results of the improved Convolutional Neural Networks with ZB layer, the detection accuracy of the Double Shortcuts ZB-ResNet model is improved by nearly two percentage points. © 2021 IEEE.},
}

@ARTICLE{Tony2021506,
author={Tony, L.A. and Ghose, D. and Chakravarthy, A.},
title={Unmanned aerial vehicle mid-air collision detection and resolution using avoidance maps},
journal={Journal of Aerospace Information Systems},
year={2021},
volume={18},
number={8},
pages={506-529},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85114640728&doi=10.2514%2f1.I010900&partnerID=40&md5=424a79a82b468776f59461b6d05d27fb},
abstract={Collision avoidance for fixed-wing unmanned aerial vehicles (UAVs), using a novel methodology of avoidance map, is addressed in this work. Avoidance map is defined as a mapping in the control input space of a pair of UAVs, which partitions the control space into avoidance and collision regions, respectively. The choice of maneuvers to execute successful avoidance can be effectively obtained by using the avoidance map. The duration of control application is determined by a simple method that is time optimal and computationally efficient. Different versions of the map portraying the evolution of the concept are also given. Precision control, defined as a gradual reduction in control, is discussed to reduce the control input demand for the entire duration of avoidance. The concept is extended to multiple UAVs, and the additional requirement of the UAVs to return to nominal trajectory after avoidance, using Dubins paths, is also addressed. Finally, simulation results using realistic UAV models are considered, and some needed modifications to the basic avoidance strategy, made necessary by realistic maneuver models, are discussed. Several illustrative simulation results are given to support the applicability of the proposed method. Copyright © 2021 by Lima Agnel Tony, Debasish Ghose, and Animesh Chakravarty. Published by the American Institute of Aeronautics and Astronautics, Inc., with permission.},
}

@ARTICLE{Yan2021,
author={Yan, Y. and Mao, Z. and Wu, J. and Padir, T. and Hajjar, J.F.},
title={Towards automated detection and quantification of concrete cracks using integrated images and lidar data from unmanned aerial vehicles},
journal={Structural Control and Health Monitoring},
year={2021},
volume={28},
number={8},
art_number={e2757},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85109056730&doi=10.1002%2fstc.2757&partnerID=40&md5=9260e94d175cdd5fdd8c217d28983559},
abstract={Recent advances in visual sensing technology and unmanned aerial vehicle (UAV) provide an effective tool to capture the as-is conditions of infrastructure and thus have gained their popularity in infrastructure inspection and documentation. To facilitate this process, several recent studies have proposed automated methods for detecting concrete cracks from UAV-based images. This study is aimed at proposing a new method for automating both the detection and quantification of concrete cracks. The proposed method advances state-of-the-art image-based concrete crack detection methods by integrating the RGB images with the lidar data collected by UAV. The key innovations focus on two aspects: (1) by recognizing objects of interest in the lidar data, regions of interest can be extracted automatically from the images; (2) by retrieving the depth information through the lidar data, the actual pixel sizes can be estimated to facilitate both the detection and quantification of concrete cracks. In order to validate the proposed method, a customized UAV platform that was equipped with a high-resolution camera and a Velodyne VLP-16 lidar scanner was developed to scan the substructure elements of an in-service bridge where multiple concrete cracks can be observed. The effectiveness of the proposed method in recognizing and quantifying concrete cracks is validated quantitively against manually annotated images and physical measurements. The results indicate that the proposed approach can recognize crack pixels with an accuracy of 85% on average as well as quantify the recognized concrete cracks with an error less than 10%. © 2021 John Wiley & Sons, Ltd.},
}

@CONFERENCE{Alqudsi2021,
author={Alqudsi, Y.S. and Alsharafi, A.S. and Mohamed, A.},
title={A Review of Airborne Landmine Detection Technologies: Unmanned Aerial Vehicle-Based Approach},
journal={2021 International Congress of Advanced Technology and Engineering, ICOTEN 2021},
year={2021},
art_number={9493528},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85112392772&doi=10.1109%2fICOTEN52080.2021.9493528&partnerID=40&md5=c576d35ecc1ddc40b820b90d2a4820cc},
abstract={The rapid development of Unmanned Aerial Vehicles (UAVs) leads to expand the application of such technologies in various fields. The detection and mapping of landmines are one of the challenging and critical areas. The provision of efficient airborne detection technologies will save the lives of thousands of civilians and even workers involved in such dangerous missions. The objective of this paper is to provide a brief review of the state-of-the-art airborne landmine detection studies for researchers to further explore. We have also proposed a promising direction for future research towards a reliable, efficient, and integrated UAV-based landmine detection system. © 2021 IEEE.},
}

@ARTICLE{Zheng20215059,
author={Zheng, J. and Yang, T. and Liu, H. and Su, T. and Wan, L.},
title={Accurate Detection and Localization of Unmanned Aerial Vehicle Swarms-Enabled Mobile Edge Computing System},
journal={IEEE Transactions on Industrial Informatics},
year={2021},
volume={17},
number={7},
pages={5059-5067},
art_number={9165125},
note={cited By 29},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85104186701&doi=10.1109%2fTII.2020.3015730&partnerID=40&md5=ee5ca70869fdf1c7d860d2cc260e369b},
abstract={Unmanned aerial vehicle (UAV) swarms-enabled mobile edge computing system can be deployed in critical industrial zones for monitoring. Meanwhile, its malicious use may bring great threat to the security, and the accurate detection, and localization are important. UAV swarms show characteristics of the high density, small radar cross section, far range, and time-varying motion, and have posed formidable challenges to the accurate detection and localization. In this article, the accurate detection and localization of UAV swarms are investigated, and an effective method is proposed based on the Dechirp-keystone transform, and frequency-selective reweighted trace minimization. It inherits high robustness of the coherent long-time integration technique and superresolution of the gridless sparse technique. Mathematical analyzes and numerical simulations validate its superiorities in accurate detection and localization of UAV swarms. © 2005-2012 IEEE.},
}

@ARTICLE{Miao20214531,
author={Miao, Y. and Tang, Y. and Alzahrani, B.A. and Barnawi, A. and Alafif, T. and Hu, L.},
title={Airborne LiDAR Assisted Obstacle Recognition and Intrusion Detection towards Unmanned Aerial Vehicle: Architecture, Modeling and Evaluation},
journal={IEEE Transactions on Intelligent Transportation Systems},
year={2021},
volume={22},
number={7},
pages={4531-4540},
art_number={9210562},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85101720818&doi=10.1109%2fTITS.2020.3023189&partnerID=40&md5=de5ea37ceae5e92c93d84d97f984327d},
abstract={With the rapid development of wireless communication and flight control technologies, the unmanned aerial vehicles (UAVs) have been widely used in multiple application scenarios. A typical scenario is massive crowd management of the multi-millions annual Hajj Pilgrimage to Mecca where UAVs are widely utilized to conduct crowd monitoring by carrying sensory devices. The safe flight of a UAV is crucial for ensuring the successful execution of missions. With the aim to overcome the disadvantage caused by the ground station intrusion detection, the combination of UAV and airborne LiDAR has been widely studied in the field of UAV obstacle recognition. This article studies the UAV network architecture under a common scenario and proposes an obstacle recognition and intrusion detection algorithm for UAV based on an airborne LiDAR (ALORID). First, the preprocessing of the data obtained by a LiDAR, i.e., the coordinate conversion of LiDAR data in combination with UAV motion parameters, is completed. Then, the LiDAR data graph at the current moment is generated by the image noisy point filtering algorithm. After that, the improved density-based spatial clustering of applications with noise (DBSCAN) algorithm is used for image clustering of intrusions to obtain the LiDAR time-domain cumulative graph in a certain detection time. Finally, the motion recognition and location detection of each cluster are completed. The experiment results verify the effectiveness of the proposed algorithm in identifying the moving state of the intrusions. © 2000-2011 IEEE.},
}

@ARTICLE{Yoon20211462,
author={Yoon, S. and Gwon, G.-H. and Lee, J.-H. and Jung, H.-J.},
title={Three-dimensional image coordinate-based missing region of interest area detection and damage localization for bridge visual inspection using unmanned aerial vehicles},
journal={Structural Health Monitoring},
year={2021},
volume={20},
number={4},
pages={1462-1475},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85085327303&doi=10.1177%2f1475921720918675&partnerID=40&md5=ffcdccf79edfb5009fafda5e5aea22da},
abstract={In this study, the three-phase missing region of interest area detection and damage localization methodology based on three-dimensional image coordinates was proposed. In Phase 1, the coordinate transformation is performed by the position and attitude information of the unmanned aerial vehicles and camera, and the coordinates of the center point of each acquired image are obtained with the distance information between the camera and the target surface. For Phase 2, the size of the field of view of every acquired image is calculated using the focal length and working distance of the camera. Finally, in Phase 3, the missing part of the region of interest area can be identified and any damage detected at the individual image level can also be localized on the whole inspection region using information about the sizes of the field of view in all images calculated in the previous phase. In order to demonstrate the proposed methodology, experimental validation was performed on the actual bridge pier and deck as well as the lab-scale concrete shear wall. In the tests, the missing area detection and damage localization results were compared with image stitching and human visual inspection results, respectively. Experimental validation results have shown that the proposed methodology identifies missing areas and damage locations within reasonable accuracy of 10 cm. © The Author(s) 2020.},
}

@ARTICLE{Kim202116159,
author={Kim, J.-S. and Lee, M.J. and Nam, H. and Do, S. and Lee, J.H. and Park, M.K. and Park, B.H.},
title={Indoor and Outdoor Tests for a Chemi-capacitance Carbon Nanotube Sensor Installed on a Quadrotor Unmanned Aerial Vehicle for Dimethyl Methylphosphonate Detection and Mapping},
journal={ACS Omega},
year={2021},
volume={6},
number={24},
pages={16159-16164},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85110427113&doi=10.1021%2facsomega.1c02104&partnerID=40&md5=79339fc57e678fdab605580dd8b27bb9},
abstract={Unmanned aerial vehicles (UAVs) have been used as a new chemical reconnaissance platform in chemical, biological, radiological, and nuclear detection and in industrial monitoring and environmental research, owing to their mobility, unconventional accessibility, and safety. Based on the UAV's payload and operational time considerations, the ultralight chip-sized chemical sensor is the most promising candidate for chemical reconnaissance among various chemical sensors. To optimize the UAV's chip-sensor performance, realistic outdoor tests of chemical sensors during UAV flights have to be conducted to verify their performances. In this study, indoor and outdoor experiments were conducted with a carbon nanotube (CNT)-based chip sensor installed on the UAV to detect dimethyl methylphosphonates (DMMPs), commonly used as chemical warfare agent simulants. Based on the indoor tests, DMMP concentrations and the position/direction of the CNT sensor were analyzed to optimize the sensing performances during UAV operations. Based on outdoor tests, we confirmed that the chemical sensor mounted on the UAV could detect DMMP gases by moving designated pathways in realistic conditions. © 2021 The Authors. Published by American Chemical Society.},
}

@CONFERENCE{Swinney20211494,
author={Swinney, C.J. and Woods, J.C.},
title={RF Detection and Classification of Unmanned Aerial Vehicles in Environments with Wireless Interference},
journal={2021 International Conference on Unmanned Aircraft Systems, ICUAS 2021},
year={2021},
pages={1494-1498},
art_number={9476867},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85111412134&doi=10.1109%2fICUAS51884.2021.9476867&partnerID=40&md5=e777570c3680bf1a46e5e3abb7eeb6cf},
abstract={Unmanned Aerial Vehicle (UAV) detection and classification methods include the use of audio, video, thermal, RADAR and radio frequency (RF) signals. RF signals have the ability to detect UAVs at longer ranges but interference from other signals in the same frequency band such as Bluetooth and Wi-Fi at 2.4GHz is a known limitation. The experiments in this paper evaluate the effect of real world Bluetooth and Wi-Fi signal interference on UAV detection and classification, using transfer learning via Convolutional Neural Network (CNN) feature extraction and machine learning classifiers Logistic Regression (LR) and k Nearest Neighbour (kNN). 2 class UAV detection, 4 class UAV type and 10 class flight mode classification are evaluated with graphical representation from the time and frequency domain. Flight modes evaluated included mode 1 - switched on and connected to the controller, mode 2 - hovering and mode 3 - flying. Results show that Bluetooth signals are more likely to interfere with detection and classification accuracy than Wi-Fi signals but that accuracy can be maintained at over 96% by using frequency domain features with LR as the classifier. Time domain features were shown to be less robust than frequency domain features when interefence signals were introduced. In the presence of Bluetooth or Wi-Fi signals, 2 class UAV detection produced 100% accuracy, 4 class UAV type classification produced 99.9% (+/- 0.1%) and 10 class UAV flight mode classification produced 96.4% (+/- 0.5%) accuracy. Overall we have shown frequency domain features extracted from a CNN to be more robust than time domain features in the presence of interference and that high accuracy can be maintained using LR as a classifier with CNN derived features. © 2021 IEEE.},
}

@CONFERENCE{Bayhan2021,
author={Bayhan, E. and Ozkan, Z. and Namdar, M. and Basgumus, A.},
title={Deep Learning Based Object Detection and Recognition of Unmanned Aerial Vehicles [Insansiz Hava Ara5larmm Derin Ogrenme Temelli Nesne Tespiti ve Tanimasi]},
journal={HORA 2021 - 3rd International Congress on Human-Computer Interaction, Optimization and Robotic Applications, Proceedings},
year={2021},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85114494685&doi=10.1109%2fHORA52670.2021.9461279&partnerID=40&md5=12169587cad72235deee5f35eba6eade},
abstract={In this study, the methods of deep learning-based detection and recognition of the threats, evaluated in terms of military and defense industry, by unmanned aerial vehicles (UAV) are presented. In the proposed approach, firstly, the training for machine learning on the objects is carried out using convolutional neural networks, which is one of the deep learning algorithms. By choosing the Faster-RCNN and YoloV4 architectures of the deep learning method, it is aimed to compare the achievements of the accuracy in the training process. In order to be used in the training and testing stages of the recommended methods, data sets containing images selected from different weather, land conditions and different time periods of the day are determined. The model for the detection and recognition of the threatening elements is trained, using 2595 images. The method of detecting and recognizing the objects is tested with military operation images and records taken by the UAVs. While an accuracy rate of 93% has been achieved in the Faster-RCNN architecture in object detection and recognition, this rate has been observed as 88% in the YoloV4 architecture. © 2021 IEEE.},
}

@ARTICLE{Kim2021367,
author={Kim, N.-K. and Park, M.-S. and Jeong, M.-J. and Hwang, D.-H. and Yoon, H.-J.},
title={A study on field compost detection by using unmanned aerial vehicle image and semantic segmentation technique based deep learning},
journal={Korean Journal of Remote Sensing},
year={2021},
volume={37},
number={3},
pages={367-378},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85111167054&doi=10.7780%2fkjrs.2020.37.3.1&partnerID=40&md5=0c6c823207ba7a27baab99a09884c819},
abstract={Field compost is a representative non-point pollution source for livestock. If the field compost flows into the water system due to rainfall, nutrients such as phosphorus and nitrogen contained in the field compost can adversely affect the water quality of the river. In this paper, we propose a method for detecting field compost using unmanned aerial vehicle images and deep learning-based semantic segmentation. Based on 39 ortho images acquired in the study area, about 30,000 data were obtained through data augmentation. Then, the accuracy was evaluated by applying the semantic segmentation algorithm developed based on U-net and the filtering technique of Open CV. As a result of the accuracy evaluation, the pixel accuracy was 99.97%, the precision was 83.80%, the recall rate was 60.95%, and the F1-Score was 70.57%. The low recall compared to precision is due to the underestimation of compost pixels when there is a small proportion of compost pixels at the edges of the image. After, It seems that accuracy can be improved by combining additional data sets with additional bands other than the RGB band. © 2021 Korean Journal of Remote Sensing. All rights reserved.},
}

@CONFERENCE{Rauch2021,
author={Rauch, J. and Doer, C. and Trommer, G.F.},
title={Object Detection on Thermal Images for Unmanned Aerial Vehicles Using Domain Adaption through Fine-Tuning},
journal={28th Saint Petersburg International Conference on Integrated Navigation Systems, ICINS 2021},
year={2021},
art_number={9470420},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113240150&partnerID=40&md5=0c2156f1b69a7197190497f719118f9c},
abstract={This work addresses state-of-the-art object detection methods using deep learning on thermal images for application on Unmanned Aerial Vehicles (UAVs). For this purpose, fine-tuning is performed using a custom dataset. Special focus is given to the generation of this dataset, as the annotations for the thermal images are automatically generated from simultaneously acquired visual images. The bounding boxes found on visual images using state-of-the-art object detection methods are applied as annotations to the thermal images. Furthermore, it is shown how the fine-tuned models can be executed in real-time on the drone's embedded PC, which is limited in its computing power, by using additional accelerator hardware. © 2021 Concern CSRI Elektropribor, JSC.},
}

@CONFERENCE{Averyanov2021,
author={Averyanov, V.S. and Kartsan, I.N. and Efremova, S.V.},
title={Methods of automated detection of anomalies and nonlinear transitions by autonomous unmanned aerial vehicles},
journal={Journal of Physics: Conference Series},
year={2021},
volume={1889},
number={4},
art_number={042001},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85107398176&doi=10.1088%2f1742-6596%2f1889%2f4%2f042001&partnerID=40&md5=1ceb36bc8da2d8073095c1b51c8cb9f1},
abstract={The paper considers the possibility of automating the recognition of anomalies and nonlinear properties of objects in different environments by assembling the UAV payload in the form of a nonlinear locator with a minimum participation of the operator in the processes of probing influence. The process of selecting the main flight platform has a number of requirements that meet the required mission, and by its tactics and technical characteristics it is able to fully implement monitoring algorithms. The theoretical basis of the model construction is given and the main parameters for the standard operation of the model in terms of height, speed and required payload set are defined. The regression model of the interval of scanning of terrain areas depending on the speed of the device and the load of the main processor is compiled. The results of the calculations are summarized and reduced to the method of automated detection of anomalies and nonlinear transitions of objects detected as a result of terrain scanning missions. The main operating properties and optimal conditions of external technological impacts of the developed mathematical model are described. © Published under licence by IOP Publishing Ltd.},
}

@ARTICLE{Loureiro2021,
author={Loureiro, G. and Dias, A. and Martins, A. and Almeida, J.},
title={Emergency landing spot detection algorithm for unmanned aerial vehicles},
journal={Remote Sensing},
year={2021},
volume={13},
number={10},
art_number={1930},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85106641855&doi=10.3390%2frs13101930&partnerID=40&md5=c25613ef03e65624dd10374f41fabc8b},
abstract={The use and research of Unmanned Aerial Vehicle (UAV) have been increasing over the years due to the applicability in several operations such as search and rescue, delivery, surveillance, and others. Considering the increased presence of these vehicles in the airspace, it becomes necessary to reflect on the safety issues or failures that the UAVs may have and the appropriate action. Moreover, in many missions, the vehicle will not return to its original location. If it fails to arrive at the landing spot, it needs to have the onboard capability to estimate the best area to safely land. This paper addresses the scenario of detecting a safe landing spot during operation. The algorithm classifies the incoming Light Detection and Ranging (LiDAR) data and store the location of suitable areas. The developed method analyses geometric features on point cloud data and detects potential right spots. The algorithm uses the Principal Component Analysis (PCA) to find planes in point cloud clusters. The areas that have a slope less than a threshold are considered potential landing spots. These spots are evaluated regarding ground and vehicle conditions such as the distance to the UAV, the presence of obstacles, the area’s roughness, and the spot’s slope. Finally, the output of the algorithm is the optimum spot to land and can vary during operation. The proposed approach evaluates the algorithm in simulated scenarios and an experimental dataset presenting suitability to be applied in real-time operations. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@ARTICLE{Bao2021,
author={Bao, M. and Chala Urgessa, G. and Xing, M. and Han, L. and Chen, R.},
title={Toward more robust and real-time unmanned aerial vehicle detection and tracking via cross-scale feature aggregation based on the center keypoint},
journal={Remote Sensing},
year={2021},
volume={13},
number={8},
art_number={1416},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85104229178&doi=10.3390%2frs13081416&partnerID=40&md5=7da37628036e3b5d6500647ecba60e33},
abstract={Unmanned aerial vehicles (UAVs) play an essential role in various applications, such as transportation and intelligent environmental sensing. However, due to camera motion and complex environments, it can be difficult to recognize the UAV from its surroundings thus, traditional methods often miss detection of UAVs and generate false alarms. To address these issues, we propose a novel method for detecting and tracking UAVs. First, a cross-scale feature aggregation CenterNet (CFACN) is constructed to recognize the UAVs. CFACN is a free anchor-based center point estimation method that can effectively decrease the false alarm rate, the misdetection of small targets, and computational complexity. Secondly, the region of interest-scale-crop-resize (RSCR) method is utilized to merge CFACN and region-of-interest (ROI) CFACN (ROI-CFACN) further, in order to improve the accuracy at a lower computational cost. Finally, the Kalman filter is adopted to track the UAV. The effectiveness of our method is validated using a collected UAV dataset. The experimental results demonstrate that our methods can achieve higher accuracy with lower computational cost, being superior to BiFPN, CenterNet, YoLo, and their variants on the same dataset. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@ARTICLE{Han2021,
author={Han, D. and Lee, S.B. and Song, M. and Cho, J.S.},
title={Change detection in unmanned aerial vehicle images for progress monitoring of road construction},
journal={Buildings},
year={2021},
volume={11},
number={4},
art_number={150},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85104192478&doi=10.3390%2fbuildings11040150&partnerID=40&md5=74fb716a29d89cc530cb23e8ca334622},
abstract={Currently, unmanned aerial vehicles are increasingly being used in various construction projects such as housing developments, road construction, and bridge maintenance. If a drone is used at a road construction site, elevation information and orthoimages can be generated to acquire the construction status quantitatively. However, the detection of detailed changes in the site owing to construction depends on visual video interpretation. This study develops a method for automatic detection of the construction area using multitemporal images and a deep learning method. First, a deep learning model was trained using images of the changing area as reference. Second, we obtained an effective application method by applying various parameters to the deep learning process. The application of the time-series images of a construction site to the selected deep learning model enabled more effective identification of the changed areas than the existing pixel-based change detection. The proposed method is expected to be very helpful in construction management by aiding in the development of smart construction technology. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@ARTICLE{Escobar-Flores2021,
author={Escobar-Flores, J.G. and Sandoval, S.},
title={Unmanned aerial vehicle (UAV) for sea turtle skeleton detection in the Mexican Pacific},
journal={Remote Sensing Applications: Society and Environment},
year={2021},
volume={22},
art_number={100501},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85103338380&doi=10.1016%2fj.rsase.2021.100501&partnerID=40&md5=bf28489ccbff933256c87f088a1858d6},
abstract={By means of a Parrot ANAFI UAV, we obtained 8000 images with a spatial resolution of 1.40 cm along 30 km of a nesting beach of Lepidochelys olivacea. The images were used to construct orthomosaics for the detection of turtle shells using object-based image analysis. Four attributes describing the shapes of the shells were obtained from the processes of segmenting the images: compactness, convexity, roundness and elongation. A total of 54 sea turtle skeletons were quantified in the field, 51 were detected by object-based image algorithm, two records turned out to be 20-L plastic bottles and one not detected because it was very old and covered by sand. The value of the coefficient and its 95% confidence interval was kappa = 0.787 (0.015), indicating considerable agreement. The shape attributes of roundness were consistent with values for circular shapes, and the convexity values were greater than 1, indicating that they were convex, which is consistent with the shape of marine turtle shells. The advantages of using the Parrot ANAFI to detect skeletons on the beach is that it can survey a visual image field from a nadir angle of 90, which enables all skeletons to be detected regardless of the slope of the berm, as well as its affordable price. © 2021 Elsevier B.V.},
}

@ARTICLE{Zeng20215385,
author={Zeng, Y. and Duan, Q. and Chen, X. and Peng, D. and Mao, Y. and Yang, K.},
title={UAVData: A dataset for unmanned aerial vehicle detection},
journal={Soft Computing},
year={2021},
volume={25},
number={7},
pages={5385-5393},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85100183583&doi=10.1007%2fs00500-020-05537-9&partnerID=40&md5=d44fdef689a1aa4a932f5d8e2b0870f6},
abstract={The unmanned aerial vehicles (UAVs) significantly contribute to the convenience and intelligence of life. However, the large use of UAVs also leads to high security risk. Only detecting the small and flying UAVs can prevent the safety accidents. UAV detection task could be regarded as a branch of object detection in flied of image processing. The advanced object detection models are mainly data driven, which depend on large-scale databases. The well-labeled datasets have proved to be of profound value for the effectiveness and accuracy in various object detection tasks. Thus, the first step of detecting UAVs is to build up a dataset of UAVs. In this study, we collect and release a dataset for UAV detection, called UAVData. To maintain the universality and robustness of the trained models, balloons and 6 types of UAVs are recorded in the dataset which totally consists of 13,803 well-labeled and recognizable images. We further conduct strong benchmarks using several advanced deep detection models, including faster R-CNN, SSD, YOLOv3. In addition, we utilize 4 different convolutional neural network models as the backbone models of these object detection methods to learn UAV-related features in images. By providing this dataset and baselines, we hope to gather researchers in both UAVs detection and machine learning field to advance toward the application. © 2021, The Author(s), under exclusive licence to Springer-Verlag GmbH, DE part of Springer Nature.},
}

@ARTICLE{Chen20213604,
author={Chen, W. and Zhao, Y. and You, T. and Wang, H. and Yang, Y. and Yang, K.},
title={Automatic Detection of Scattered Garbage Regions Using Small Unmanned Aerial Vehicle Low-Altitude Remote Sensing Images for High-Altitude Natural Reserve Environmental Protection},
journal={Environmental Science and Technology},
year={2021},
volume={55},
number={6},
pages={3604-3611},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85102964542&doi=10.1021%2facs.est.0c04068&partnerID=40&md5=b069e25aa478a35ed68fb5799b626ff9},
abstract={Recently, some famous high-altitude nature reserves have been shut down due to tourist garbage pollution. In order to clean up such garbage more conveniently and quickly, a novel detection framework is proposed to automatically detect scattered garbage regions using low-altitude remote sensing of small unmanned aerial vehicles (SUAVs), and it contains the following steps. First, high-resolution, low-altitude, multitemporal remote sensing images containing scattered garbage regions are collected by SUAVs, and two data augmentation methods are proposed to expand the training samples. Second, low-altitude remote sensing image registration and target-level image change detection are used to extract the candidate regions of garbage. Finally, a deep learning detection network is adopted to classify the scattered garbage regions. Experimental results show that the proposed detection framework achieves a mean accuracy of 96.94% and provides better performances on the real dataset compared with state-of-the-art methods. © 2021 American Chemical Society.},
}

@ARTICLE{Park20211,
author={Park, K.H. and Park, E. and Kim, H.K.},
title={Unsupervised fault detection on unmanned aerial vehicles: Encoding and thresholding approach},
journal={Sensors},
year={2021},
volume={21},
number={6},
pages={1-17},
art_number={2208},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85102773469&doi=10.3390%2fs21062208&partnerID=40&md5=2c5e5600f8a8751ad36d3ac45040ec07},
abstract={Unmanned Aerial Vehicles are expected to create enormous benefits to society, but there are safety concerns in recognizing faults at the vehicle’s control component. Prior studies proposed various fault detection approaches leveraging heuristics-based rules and supervised learning-based models, but there were several drawbacks. The rule-based approaches required an engineer to update the rules on every type of fault, and the supervised learning-based approaches necessitated the acquisition of a finely-labeled training dataset. Moreover, both prior approaches commonly include a limit that the detection model can identify the trained type of faults only, but fail to recognize the unseen type of faults. In pursuit of resolving the aforementioned drawbacks, we proposed a fault detection model utilizing a stacked autoencoder that lies under unsupervised learning. The autoencoder was trained with data from safe UAV states, and its reconstruction loss was examined to distinguish the safe states and faulty states. The key contributions of our study are, as follows. First, we presented a series of analyses to extract essential features from raw UAV flight logs. Second, we designed a fault detection model consisting of the stacked autoencoder and the classifier. Lastly, we validated our approach’s fault detection performance with two datasets consisting of different types of UAV faults. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@ARTICLE{Yang2021509,
author={Yang, Y. and Wang, X. and Zhang, B.},
title={Radar Detection of Unmanned Aerial Vehicles Based on Time-frequency Detection and Polarization Matching [基于时频检测与极化匹配的雷达无人机检测方法]},
journal={Dianzi Yu Xinxi Xuebao/Journal of Electronics and Information Technology},
year={2021},
volume={43},
number={3},
pages={509-515},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85103101908&doi=10.11999%2fJEIT200768&partnerID=40&md5=b9b5a2cc7cd4a98779aad1c0c8c539ee},
abstract={Radar detection of Unmanned Aerial Vehicle (UAV) is a big problem. To address this problem, a detection method with dual polarization radar is proposed. First, radar reduces the detection threshold to make the UAV be detected by using the traditional two dimensional cell averaging constant false alarm probability detector in two polarization channels respectively. However, some false targets caused by clutter are also detected by radar at the same time. To eliminate these false targets, the detection results are integrated and the second detection is carried out for the integrated results in two polarization channels respectively. Then, the second detection results in two polarization channels are matched to further eliminate the false targets. Outdoor experiment is carried out. The processing results for the real data demonstrate that the second types of UAV can be effectively detected and the false targets caused by clutter can be eliminated at the same time with the proposed method. © 2021, Science Press. All right reserved.},
}

@ARTICLE{Kraft20211,
author={Kraft, M. and Piechocki, M. and Ptak, B. and Walas, K.},
title={Autonomous, onboard vision-based trash and litter detection in low altitude aerial images collected by an unmanned aerial vehicle},
journal={Remote Sensing},
year={2021},
volume={13},
number={5},
pages={1-17},
art_number={965},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85102660880&doi=10.3390%2frs13050965&partnerID=40&md5=f1da5b24b81c4c427bffc79d76be11e3},
abstract={Public littering and discarded trash are, despite the effort being put to limit it, still a serious ecological, aesthetic, and social problem. The problematic waste is usually localised and picked up by designated personnel, which is a tiresome, time-consuming task. This paper proposes a low-cost solution enabling the localisation of trash and litter objects in low altitude imagery collected by an unmanned aerial vehicle (UAV) during an autonomous patrol mission. The objects of interest are detected in the acquired images and put on the global map using a set of onboard sensors commonly found in typical UAV autopilots. The core object detection algorithm is based on deep, convolutional neural networks. Since the task is domain-specific, a dedicated dataset of images containing objects of interest was collected and annotated. The dataset is made publicly available, and its description is contained in the paper. The dataset was used to test a range of embedded devices enabling the deployment of deep neural networks for inference onboard the UAV. The results of measurements in terms of detection accuracy and processing speed are enclosed, and recommendations for the neural network model and hardware platform are given based on the obtained values. The complete system can be put together using inexpensive, off-the-shelf components, and perform autonomous localisation of discarded trash, relieving human personnel of this burdensome task, and enabling automated pickup planning. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@ARTICLE{Matczak20211,
author={Matczak, G. and Mazurek, P.},
title={Comparative monte carlo analysis of background estimation algorithms for unmanned aerial vehicle detection},
journal={Remote Sensing},
year={2021},
volume={13},
number={5},
pages={1-20},
art_number={870},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85102113484&doi=10.3390%2frs13050870&partnerID=40&md5=f7272b1bb5c72123ab0bb1ef2a37278b},
abstract={Background estimation algorithms are important in UAV (Unmanned Aerial Vehicle) vision tracking systems. Incorrect selection of an algorithm and its parameters leads to false detections that must be filtered by the tracking algorithm of objects, even if there is only one UAV within the visibility range. This paper shows that, with the use of genetic optimization, it is possible to select an algorithm and its parameters automatically. Background estimation algorithms (CNT (CouNT), GMG (Godbehere-Matsukawa-Goldberg), GSOC (Google Summer of Code 2017), MOG (Mixture of Gaussian), KNN (K-Nearest Neighbor-based Background/Foreground Segmentation Algorithm), MOG2 (Mixture of Gaussian version 2), and MEDIAN) and the reference algorithm of thresholding were tested. Monte Carlo studies were carried out showing the advantages of the MOG2 algorithm for UAV detection. An empirical sensitivity analysis was presented that rejected the MEDIAN algorithm. © 2021 by the authors.},
}

@ARTICLE{Iannace202177,
author={Iannace, G. and Ciaburro, G. and Trematerra, A.},
title={Acoustical unmanned aerial vehicle detection in indoor scenarios using logistic regression model},
journal={Building Acoustics},
year={2021},
volume={28},
number={1},
pages={77-96},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85084564915&doi=10.1177%2f1351010X20917856&partnerID=40&md5=400e82e54358d4cc9d68803946393897},
abstract={In this study, the data obtained from the acoustic measurements were used to train a model based on logistic regression in order to detect a quadrotor’s vehicle in indoor environment. To simulate a real environment, we made sound recordings in a shopping center. The sounds related to two scenarios were recorded: only anthropic noise and anthropic noise with background music. Later, we reproduced these sounds in an indoor environment of the same size and characteristics as the shopping center. During the simulation test, a drone placed at different distances from the sound level meter was turned on at different speeds to identify their presence in complex acoustic scenarios. Subsequently, these measurements were used to implement a model based on logistic regression for the automatic detection of the unmanned aerial vehicle. Logistic regression is widely used in pattern recognition of the binary dependent variable. This model returns high value of accuracy (0.994), indicating a high number of correct detections. The results obtained in this study suggest the use of this tool for unmanned aerial vehicle detection applications. © The Author(s) 2020.},
}

@CONFERENCE{Kuznetcov2021,
author={Kuznetcov, I.E. and Kuznetcov, A.A. and Baklanov, I.O. and Strashko, O.V.},
title={The probabilistic model of search and detection of ground objects using unmanned aerial vehicles in difficult weather conditions},
journal={Journal of Physics: Conference Series},
year={2021},
volume={1745},
number={1},
art_number={012048},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85102394874&doi=10.1088%2f1742-6596%2f1745%2f1%2f012048&partnerID=40&md5=8d37bafa6fdfba2c5d9454751d1855d5},
abstract={The paper proposes the model of search and detection of ground objects in difficult weather conditions with the use of unmanned aerial vehicles. The model is based on the probabilistic approach and allows assessing the quality of reconnaissance missions taking into account the influence of the most significant meteorological values and weather phenomena. © Published under licence by IOP Publishing Ltd.},
}

@CONFERENCE{Goncharenko2021,
author={Goncharenko, V.I. and Lebedev, G.N. and Mikhailin, D.A.},
title={Pre-flight and Operational Planning of Surveillance by a Group of Unmanned Aerial Vehicles of Separated Parts of Launch Vehicles during Their Search and Detection},
journal={AIP Conference Proceedings},
year={2021},
volume={2318},
art_number={100011},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85101699446&doi=10.1063%2f5.0035858&partnerID=40&md5=53039861a03895ba8eee7f81fc42d2ba},
abstract={This paper proposes a new approach to tacking problems of preflight and operational planning of UAV group actions. In contrast to the accepted cases in practice, this paper deals with the maintenance processes of a special class of dynamic objects, whose schedules require prior assignment in order to serve these objects "at the right time and in the right place". The goal of this work is to achieve the maximum effectiveness of group actions of unmanned aerial vehicles in a single flight, in order to find the separating parts of launch vehicles in the territory with the maximum speed. The main difference between the problem being solved and the known problem of a traveling salesman is the consideration of the required service schedule. The essence of the proposed approach is that the entire planned route is divided into several sections, the boundaries of which are dynamic objects that need to be served in the specified schedule. In each of these sections, one or two particular criteria are dominant - either timeliness is important, or cost-effectiveness, etc.the Developed software-algorithmic planning automation device allows increasing the efficiency of measures to detect separating parts of launch vehicles using a group of unmanned aerial vehicles. Consequently, of computer modeling, it turned out that a successful combination of individual sections of routes with each other by crossing and mutation, when each of the sections is formed using its own private two-parameter criterion, provides an increase in planning efficiency by 10-15% compared to known heuristic algorithms. © 2021 American Institute of Physics Inc.. All rights reserved.},
}

@ARTICLE{Bhoi2021,
author={Bhoi, S.K. and Jena, K.K. and Panda, S.K. and Long, H.V. and Kumar, R. and Subbulakshmi, P. and Jebreen, H.B.},
title={An Internet of Things assisted Unmanned Aerial Vehicle based artificial intelligence model for rice pest detection},
journal={Microprocessors and Microsystems},
year={2021},
volume={80},
art_number={103607},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85097332927&doi=10.1016%2fj.micpro.2020.103607&partnerID=40&md5=97a76003225d3c125de33801c2605947},
abstract={Rice is a very essential food for the survival of human society. Most of the people focus on production of rice for their financial gain as well as their survival in the society. Rice production means a lot, not only for the farmers, but also for the entire human society However, it is very difficult to protect the rice during and after the production due to several reasons, such as natural calamities, heavy rain fall, flood, earthquakes, damage of rice due to pests, etc. Damage of rice can occur during production and after the production due to several pests. So, it is very much essential to identify the pests in the rice so that preventive measures can be taken for its protection. In this paper, an Internet of Things (IoT) assisted Unmanned Aerial Vehicle (UAV) based rice pest detection model using Imagga cloud is proposed to identify the pests in the rice during its production in the field. The IoT assisted UAV focuses on artificial intelligence (AI) mechanism and Python programming paradigm for sending the rice pest images to the Imagga cloud and providing the pest information. The Imagga cloud detects the pest by finding the confidence values with the tags. The tag represents the object in that image. The tag with maximum confidence value and beyond threshold is selected as the target tag to identify the pest. If pest is detected then the information is sent to the owner for further actions. The proposed method can able to identify any kind of the pest that affects the rice during production. Alternatively, this paper attempts to minimize the wastage of rice during its production by monitoring the pests at regular intervals. © 2020 Elsevier B.V.},
}

@CONFERENCE{Maqsood2021486,
author={Maqsood, H. and Taimoor, M. and Ullah, Z. and Ali, N. and Sohail, M.},
title={Novel Sensor Fault Detection and Isolation for an Unmanned Aerial Vehicle},
journal={Proceedings of 18th International Bhurban Conference on Applied Sciences and Technologies, IBCAST 2021},
year={2021},
pages={486-493},
art_number={9393247},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85104683935&doi=10.1109%2fIBCAST51254.2021.9393247&partnerID=40&md5=f9b130a85f76aba49828442c383c9b1c},
abstract={To avoid adverse impacts on humans and the environment and upon the system itself, early detection and isolation of faults and failures in the flight control system are crucial. This paper focuses on designing a novel detection and isolation (FDI) of sensor faults in quadrotors. The traditional nonlinear fault detection techniques including integral chain differentiator and high gain observer are incorporated to realize the accurate reconstruction of the sensor faults. However, the proposed approach based on the improved high gain observer is employed that offers fast detection of sensor faults with improved detection accuracy and lower gain requirement than the traditional observer. Various simulation results validate the superiority of the proposed FDI method and prove its efficacy under the influence of different fault scenarios. © 2021 IEEE.},
}

@ARTICLE{Chen2021106,
author={Chen, S. and Liang, D. and Ying, B. and Zhu, W. and Zhou, G. and Wang, Y.},
title={Assessment of an improved individual tree detection method based on local-maximum algorithm from unmanned aerial vehicle RGB imagery in overlapping canopy mountain forests},
journal={International Journal of Remote Sensing},
year={2021},
volume={42},
number={1},
pages={106-125},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85092934219&doi=10.1080%2f01431161.2020.1809024&partnerID=40&md5=b7be6d199c6f24bd9f31d8c389e9b66f},
abstract={Low consumer-grade cameras attached to small unmanned aerial vehicles (UAV) can easily acquire high spatial resolution images, leading to convenient forest monitoring at small-scales for forest managers. However, most studies were carried out in the low canopy density and flat ground plantations to detect individual trees. We selected overlapping canopy plantation in mountainous area in the eastern of China and acquired high spatial resolution UAV RGB images to detect individual trees. A total of 402 reference trees were located in three rectangle plots (900 m2). To enhance the confidence of the tested individual tree detection method, clear-cutting and Real-Time Kinematic (RTK) were used to obtain the truth values in the plots. A novel method for semi-automatic individual tree detection was proposed based on a local-maximum algorithm and UAV-derived DSM data (LAD) in this study. The detection accuracy of LAD was compared with commonly used methods based on UAV-derived orthophoto images, local-maximum algorithm (LAO), object-oriented feature segmentation (OFS), multiscale segmentation technique (MST) and manual visual interpretation (MVI). The overall accuracy (OA (%) decreased in the order of LAD (84.5%) &gt; MST (69.1%) &gt; OFS (65.1%) &gt; MVI (64.1%) &gt; LAO (59.1%). LAD had only 15.5%s omission errors (OM (%), which was less than half of the other four methods in comparison. It was noteworthy that MVI had 35.9% OM %, which revealed that MVI should be used carefully as the truth value. LAD showed similar repeated detection error (RP (%) and completely wrong detection (CW (%), while the other four methods had obviously higher CW % than the RP %. From our results, it can be concluded that the proposed LAD method may help improving the accuracy of individual tree detection to an acceptable accuracy (&gt;80%) in dense mountain forests, and has practical advantages in future research direction to assess tree attributes from UAV RGB image. © 2020 Informa UK Limited, trading as Taylor & Francis Group.},
}

@ARTICLE{Na2021,
author={Na, L. and Kuangang, F. and Yahui, L. and Qinghua, O.},
title={Unmanned aerial vehicle detection based on ASRPCA fused with five-frame difference [基于 ASRPCA 和五帧差分融合的无人机检测研究]},
journal={Laser and Optoelectronics Progress},
year={2021},
volume={58},
number={20},
art_number={2015007},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85119987868&doi=10.3788%2fLOP202158.2015007&partnerID=40&md5=3acfb4741deba570297b428784efcce6},
abstract={The popularization of unmanned aerial vehicle UAV has brought great security risks to people A UAV video detection algorithm based on the active subspace robust principal component analysis ASRPCA fused with the five-frame difference is designed to solve this problem. First an alternating iteration method combined with the augmented Lagrange multiplier method is used to optimize and solve the ASRPCA model thereby obtaining the background image of the current frame of the video sequence. Second the background image replaces the intermediate frame of the five-frame difference. Finally differential binarization operation is performed simultaneously on the intermediate frames previous two frames and subsequent two frames. This makes UAV have a better detection result and a denoising ability. The experimental results show that under different backgrounds compared with the algorithm of total variation regularized RPCA TVRPCA the average of recall rate precision rate and comprehensive performance of the proposed algorithm is increased by 5 percent 4.8 percent and 5 percent respectively The running time is approximately 0.51 s per frame which meets the offline real-time requirements of the target algorithms. © 2021 Universitat zu Koln. All rights reserved.},
}

@ARTICLE{Yu2021,
author={Yu, J. and Gao, H. and Sun, J. and Zhou, D. and Ju, Z.},
title={Spatial Cognition-driven Deep Learning for Car Detection in Unmanned Aerial Vehicle Imagery},
journal={IEEE Transactions on Cognitive and Developmental Systems},
year={2021},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85118655708&doi=10.1109%2fTCDS.2021.3124764&partnerID=40&md5=fb7d4d4bb8815f54e4863502e1731fe5},
abstract={Small object detection is the main challenge for image detection of unmanned aerial vehicles (UAVs), especially with small pixel ratios and blurred boundaries. In this paper, a one-stage detector (SF-SSD) is proposed with a new spatial cognition algorithm. The deconvolution operation is introduced to a feature fusion module, which enhances the representation of shallow features. These more representative features prove effective for small-scale object detection. Empowered by a spatial cognition method, the deep model can re-detect objects with less-reliable confidence scores. This enables the detector to improve detection accuracy significantly. Both between-class similarity and within-class similarity are fully exploited to suppress useless background information. This motivates the proposed model to take full use of semantic features in the detection process of multi-class small objects. A simplified network structure can improve the speed of object detection. The experiments are conducted on a newly collected dataset (SY-UAV) and the benchmark datasets (CARPK and PUCPR+). To further demonstrate the effectiveness of the spatial cognition module, a multi-class object detection experiment is conducted on the Stanford Drone dataset (SDD). The results show that the proposed model achieves high frame rates and better detection accuracies than the state-of-the-art methods, which are 90.1% (CAPPK), 90.8% (PUCPR+), and 91.2% (SDD). IEEE},
}

@ARTICLE{Wu2021,
author={Wu, X. and Li, W. and Hong, D. and Tao, R. and Du, Q.},
title={Deep Learning for Unmanned Aerial Vehicle-Based Object Detection and Tracking: A Survey},
journal={IEEE Geoscience and Remote Sensing Magazine},
year={2021},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85118621887&doi=10.1109%2fMGRS.2021.3115137&partnerID=40&md5=a8272bf63f97596dbdc02e3532c4f401},
}

@ARTICLE{SegoviaRamírez2021,
author={Segovia Ramírez, I. and Das, B. and García Márquez, F.P.},
title={Fault detection and diagnosis in photovoltaic panels by radiometric sensors embedded in unmanned aerial vehicles},
journal={Progress in Photovoltaics: Research and Applications},
year={2021},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85116274189&doi=10.1002%2fpip.3479&partnerID=40&md5=d7725c19d94f917617db441d9d070185},
abstract={Photovoltaic solar energy is increasing its capacity in the global electric market due to its lower operating costs and higher efficiency, together with the support of the governments. Photovoltaic solar panels require high initial investments, and it is necessary to use advanced and efficient methods that lead to the maintainability and reliability of these systems, extending their life cycle and productivity. New condition monitoring systems are being applied to reduce the cost of inspections and ensure efficient data collection. The main contribution of this paper is a new efficient and low-cost condition monitoring system based on radiometric sensors. The thermal patterns of the main photovoltaic faults (hot spot, fault cell, open circuit, bypass diode, and polarization) are studied in real photovoltaic panels. Different scenarios are considered, analyzing online the main patterns of the faults by Internet of Things. The accuracies of the results are statistically analyzed and compared with fault-free scenarios. The validation of the approach is done by thermographic analysis of the experiments and employing a different radiometric sensor. The detection of faults with statistical analysis is achieved in 100% of the cases, and the identification of the specific fault in 96% of the scenarios. An artificial neural network and classification learner algorithms are employed to validate the results, obtaining similar results for fault identification, 95% and 94%, respectively, and 100% for fault detection. © 2021 The Authors. Progress in Photovoltaics: Research and Applications published by John Wiley & Sons Ltd.},
}

@ARTICLE{Guan20211,
author={Guan, R. and Yu, J. and Li, M. and Yan, J. and Liu, Z.},
title={Preparation of electrochemical sensor assisted unmanned aerial vehicles system for SO2, O3, NO2, CO and PM2.5/PM10 detection in air},
journal={International Journal of Electrochemical Science},
year={2021},
volume={16},
pages={1-9},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85115645821&doi=10.20964%2f2021.10.28&partnerID=40&md5=ca65f8a981540b84bdf65b6067ad1352},
abstract={The spatial and especially vertical monitoring of atmospheric pollutants is of great significance to the analysis and prevention of air pollution. It is also a useful supplement to the current monitoring method which is mainly based on ground monitoring stations. Small UAVs offer a new way of vertical monitoring of air pollution. In this study, an electrochemical sensor incorporated unmanned aerial vehicles (UAV) platform was proposed, which can detect pollution at vertical heights, and has been used for PM2.5, PM10 and 4 pollutants (SO2, O3, NO2, CO) at different heights. Based on this monitoring data, the vertical distribution characteristics as well as the statistical correlation of PM2.5 and its pollutants were analyzed. The experimental results show that PM2.5 concentration increases with height in the larger integrated industrial areas, while it decreases and then increases near the small-scale industrial and residential areas. The trends of PM10 and PM2.5 are basically consistent. In the vertical direction, the maximum values of CO and SO2 always appear near the ground and then start to decrease, and NO2 increases with the height © 2021 The Authors. Published by ESG (www.electrochemsci.org). This article is an open access article distributed under the terms and conditions of the Creative Commons Attribution license (http://creativecommons.org/licenses/by/4.0/).},
}

@ARTICLE{Qiang20211,
author={Qiang, C. and Yuan-Yuan, L. and Zi-Yi, J. and Qian-Hao, C.},
title={3D change detection of urban construction waste accumulations using unmanned aerial vehicle photogrammetry},
journal={Sensors and Materials},
year={2021},
volume={33},
pages={1-23},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113714341&doi=10.18494%2fSAM.2021.3447&partnerID=40&md5=961bd5474e405f7e109cb5126ecddb6e},
abstract={Due to the large annual production of construction waste in China, the rapid changes in construction waste materials, and the need to quickly obtain high-precision 3D change information for construction waste, we have used a rapid monitoring method for construction waste accumulations, which uses unmanned aerial vehicle (UAV) photogrammetry to obtain a digital surface model (DSM) and a digital orthophoto map (DOM) of two study areas located in Pingdingshan City, China. Then, we built 3D models of waste accumulations in 2019 and 2020 for the two study areas. We also proposed a 3D change detection model combined with self-adaptive roughness quantification and supervised classification based on the elevation threshold to extract construction waste accumulations, and the extraction accuracies in 2019 and 2020 were 84.9% and 85.6%, respectively. Also, we used the adaptive threshold method and the discrete integral method to calculate the changes in areas and volumes of the accumulations. The calculation accuracy of the volume of construction waste reached 88%. This study provides a method for quickly obtaining 3D change information for construction waste accumulations. © MYU K.K.},
}

@ARTICLE{Peng20218858,
author={Peng, X. and Chen, Z. and Chen, Y. and Chen, Q. and Liu, H. and Wang, J. and Li, H.},
title={Modelling of the biodiversity of tropical forests in China based on unmanned aerial vehicle multispectral and light detection and ranging data},
journal={International Journal of Remote Sensing},
year={2021},
volume={42},
number={23},
pages={8858-8877},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113537742&doi=10.1080%2f01431161.2021.1954714&partnerID=40&md5=533190aafe25f5c7be50c3aa7a6741ae},
abstract={Rapid and accurate monitoring of biodiversity is a major challenge in biodiversity conservation. Obtaining data using unmanned aerial vehicles (UAV) provides a new direction for biodiversity monitoring. However, studies on the relationship between UAV data and biodiversity are limited. In this study, we used a machine learning algorithm to evaluate the effectiveness of UAV-light detection and ranging (LiDAR) and UAV multispectral data for estimating three α-diversity indices in tropical forests located in Hainan, China. We obtained 126 biodiversity-related metrics (68 from multispectral and 58 from LiDAR) based on the UAV data and three α-diversity indices from 62 sample plots at two sites. We used the recursive feature elimination algorithm to filter significant metrics. We found that both multispectral and LiDAR data can be used to predict α-diversity. The coefficient of determination (R 2) values of multispectral data (LiDAR data) for the species richness, Shannon index, and Simpson index were 0.69, 0.70, and 0.57 (0.72, 0.63, 0.44), respectively. LiDAR data were more accurate than multispectral data for predicting species richness, whereas multispectral data were more accurate than LiDAR data for predicting the Shannon and Simpson indices. Given the best result obtained with a single datum, the accuracy (R 2) of the combination of the two data types for species richness and Shannon and Simpson indices increased by 0.05, 0.05, and 0.06, respectively, indicating that the prediction accuracy of the α-diversity index can be improved by integrating different remote sensing data. Additionally, the most important multispectral metrics used to predict α-diversity were related to vegetation index and texture metrics, whereas the most important LiDAR metrics were related to canopy height characteristics. Our research results indicate that UAV data are effective for predicting the α-diversity index of Hainan tropical forest on a fine scale. UAV data may help local biodiversity workers to identify vulnerable areas. © 2021 Informa UK Limited, trading as Taylor & Francis Group.},
}

@ARTICLE{Quan202136,
author={Quan, X. and Doluschitz, R.},
title={Unmanned aerial vehicle (UAV) technical applications, standard workflow, and future developments in maize production -water stress detection, weed mapping, nutritional status monitoring and yield prediction},
journal={Landtechnik},
year={2021},
volume={76},
number={1},
pages={36-51},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85111493718&doi=10.15150%2flt.2021.3263&partnerID=40&md5=b7b45489ed7dd9431808e2ff9ccc3115},
abstract={As a consequence of rapid ongoing technological developments and increasing integration into agricultural mechanization and agricultural intelligence, UAVs are gradually starting to play an increasingly important role in field crop management and monitoring. This review introduces and covers the development in four major applications of UAVs in maize production: (i) water stress detection, (ii) weed mapping, (iii) nutrient status monitoring and (iv) yield prediction. In addition, this review summarizes UAV data management methods, explains how expert systems work in UAV systems, and provides standardized workflow data for farmers in maize production. In addition, the strengths, weaknesses, opportunities, and threats of UAV use in maize production are analyzed. Based on more than eighty publications and our own research, the discussion and conclusions point out key issues in UAV usage in maize cropping and research gaps that need to be filled, along with a number of recommendations for the development of UAVs in maize production in the future. © 2021 by the authors. This is an open access},
}

@ARTICLE{Yahia2021,
author={Yahia, C.N. and Scott, S.E. and Boyles, S.D. and Claudel, C.G.},
title={Unmanned aerial vehicle path planning for trafﬁc estimation and detection of non-recurrent congestion},
journal={Transportation Letters},
year={2021},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85111436526&doi=10.1080%2f19427867.2021.1951524&partnerID=40&md5=d0ca32c98f51ed1a9f3aa3b1301d28c1},
abstract={Unmanned aerial vehicles (UAVs) provide a novel means of extracting road and traffic information from video data. In particular, by analyzing objects in a video frame, UAVs can detect traffic characteristics and road incidents. Leveraging the mobility and detection capabilities of UAVs, we investigate a navigation algorithm that seeks to maximize information on the road/traffic state under non-recurrent congestion. We propose an active exploration framework that (1) assimilates UAV observations with speed-density sensor data, (2) quantifies uncertainty on the road/traffic state, and (3) adaptively navigates the UAV to minimize this uncertainty. The navigation algorithm uses the A-optimal information measure (mean uncertainty), and it depends on covariance matrices generated by a dual state ensemble Kalman filter (EnKF). Our results indicate that targeted UAV observations aid in the detection of incidents under congested conditions where speed-density data are not informative. © 2021 Informa UK Limited, trading as Taylor & Francis Group.},
}

@ARTICLE{Hensel2021254,
author={Hensel, S. and Marinov, M.B. and Schmitt, M.},
title={Object Detection and Mapping with Unmanned Aerial Vehicles Using Convolutional Neural Networks},
journal={Lecture Notes of the Institute for Computer Sciences, Social-Informatics and Telecommunications Engineering, LNICST},
year={2021},
volume={382},
pages={254-267},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85111423702&doi=10.1007%2f978-3-030-78459-1_19&partnerID=40&md5=be1a94d8ac5d899a19a1fe1a41917f4b},
abstract={Significant progress has been made in the field of deep learning through intensive research over the last decade. So-called convolutional neural networks are an essential component of this research. In this type of neural network, the mathematical convolution operator is used to extract characteristics or anomalies. The purpose of this work is to investigate the extent to which it is possible in certain initial settings to input aerial recordings and flight data of Unmanned Aerial Vehicles (UAVs) in the architecture of a neural network and to detect and map an object. Using the calculated contours or dimensions of the so-called bounding boxes, the position of the objects can be determined relative to the current UAV location. © 2021, ICST Institute for Computer Sciences, Social Informatics and Telecommunications Engineering.},
}

@ARTICLE{Ji202199995,
author={Ji, G. and Song, C. and Huo, H.},
title={Detection and Identification of Low-Slow-Small Rotor Unmanned Aerial Vehicle Using Micro-Doppler Information},
journal={IEEE Access},
year={2021},
volume={9},
pages={99995-100008},
art_number={9481096},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85110863197&doi=10.1109%2fACCESS.2021.3096264&partnerID=40&md5=45cf8fb16619f0e28f1451f4749009a8},
abstract={The capability of a radar system to detect and identify the low-slow-small rotor unmanned aerial vehicle (UAV) is intensely important for management and control in low altitude, and it can be enhanced by the characteristics of UAV, which inherently carries micro-Doppler information. In this paper, we establish a micro-motion model of rotor UAV, and analyze the range walking and Doppler broadening caused by micro-motion. Hence, based on the characteristics of micro-Doppler of the rotors apart from the main body for the moving UAV, a micro-motion target detection and micro-Doppler parameters estimation method is proposed. Firstly, a method based on datashift in range dimension is used to compensate the translational component of the main body. Secondly, for the echo after translation compensation, a parameter estimation method of micro-Doppler based on the optimal demodulation operator is proposed. The operator contents the maximum likelihood criterion, which strengthens the difference between the micro-Doppler signal and the background clutters, so that more signal energy can be accumulated while the clutter is suppressed. Subsequently, the micro-Doppler parameters of the micro-motion component are obtained by the optimal demodulator, so that the detection and identification of the target are realized. Additionally, the performance of proposed method, including parameter estimation, signal-to-noise ratio (SNR) improvement and the calculation efficiency is analyzed. Finally, the simulation and experimental results reveal that the proposed method does possess the capability to improve the performance of detection and recognition of rotor UAV. © 2013 IEEE.},
}

@ARTICLE{Zhao2021,
author={Zhao, Z. and Han, J. and Song, L.},
title={YOLO-Highway: An Improved Highway Center Marking Detection Model for Unmanned Aerial Vehicle Autonomous Flight},
journal={Mathematical Problems in Engineering},
year={2021},
volume={2021},
art_number={1205153},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85108459434&doi=10.1155%2f2021%2f1205153&partnerID=40&md5=119dc1402e4ee7d4b06eae085e041275},
abstract={Automatic visual navigation flight of an unmanned aerial vehicle (UAV) plays an important role in the highway maintenance field. Automatic highway center marking detection is the most important part of the visual navigation flight of a UAV. In this study, the UAV-viewed highway data are collected from the UAV perspective. This paper proposes a model named the YOLO-Highway that uses an improved form of the You Only Look Once (YOLO) model to enhance the real-time detection of highway marking problems. The proposed model is mainly designed by optimizing the network structure and the loss function of the original YOLOv3 model. The proposed model is verified by the experiments using the highway center marking dataset, and the results show that the average precision (AP) of the trained model is 82.79%, and the frames per second (FPS) is 25.71 f/s. In comparison with the original YOLOv3 model, the detection accuracy of the proposed model is improved by 7.05%, and its speed is improved by 5.29 f/s. Moreover, the proposed model had stronger environmental adaptability and better detection precision and speed than the original model in complex highway scenarios. The experimental results show that the proposed YOLO-Highway model can accurately detect the highway center markings in real-time and has high robustness to changes in different environmental conditions. Therefore, the YOLO-Highway model can meet the real-time requirements of the highway center marking detection. © 2021 Zhiwei Zhao et al.},
}

@ARTICLE{Song2021,
author={Song, B. and Park, K.},
title={Comparison of outdoor compost pile detection using unmanned aerial vehicle images and various machine learning techniques},
journal={Drones},
year={2021},
volume={5},
number={2},
art_number={31},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85106753028&doi=10.3390%2fdrones5020031&partnerID=40&md5=d9e5044138e652790fd55e3a72341b86},
abstract={Since outdoor compost piles (OCPs) contain large amounts of nitrogen and phosphorus, they act as a major pollutant that deteriorates water quality, such as eutrophication and green algae, when the OCPs enter the river during rainfall. In South Korea, OCPs are frequently used, but there is a limitation that a lot of manpower and budget are consumed to investigate the current situation, so it is necessary to efficiently investigate the OCPs. This study compared the accuracy of various machine learning techniques for the efficient detection and management of outdoor compost piles (OCPs), a non-point pollution source in agricultural areas in South Korea, using unmanned aerial vehicle (UAV) images. RGB, multispectral, and thermal infrared UAV images were taken in August and October 2019. Additionally, vegetation indices (NDVI, NDRE, ENDVI, and GNDVI) and surface temperature were also considered. Four machine learning techniques, including support vector machine (SVM), decision tree (DT), random forest (RF), and k-NN, were implemented, and the machine learning technique with the highest accuracy was identified by adjusting several variables. The accuracy of all machine learning techniques was very high, reaching values of up to 0.96. Particularly, the accuracy of the RF method with the number of estimators set to 10 was highest, reaching 0.989 in August and 0.987 in October. The proposed method allows for the prediction of OCP location and area over large regions, thereby foregoing the need for OCP field measurements. Therefore, our findings provide highly useful data for the improvement of OCP management strategies and water quality. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@ARTICLE{Zhu2021,
author={Zhu, H. and Wang, L. and Liu, M.},
title={Using DTMB-Based Passive Radar for Small Unmanned Aerial Vehicle Detection},
journal={Wireless Communications and Mobile Computing},
year={2021},
volume={2021},
art_number={9987992},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85106376272&doi=10.1155%2f2021%2f9987992&partnerID=40&md5=68455d1e7486cf25bbbc55dccb95f6bc},
abstract={There is inevitable polarization angle deviation between the target echo signal and the direct path signal of illuminator of opportunity (IO) in passive radar. In order to investigate the potential performance loss in target detection induced by the random deviation, small unmanned aerial vehicle (UAV) detection experiments with digital television terrestrial multimedia broadcasting-(DTMB-) based passive radar are conducted in this paper. Experimental results show that the polarization angles of the clutter signal and target echo signal are inconsistent. When the polarization diversity technology is used to suppress the clutter signal, the processing performance of the target echo signal may be reduced. On the premise that clutter is effectively suppressed by the processing algorithm, polarization synthesis can maximize the target echo signal processing gain. The effectiveness of the target localization algorithm combining time difference of arrival (TDOA) and direction of arrival (DOA) is also verified with polarization diversity reception in this paper. © 2021 Huijie Zhu et al.},
}

@ARTICLE{Liu2021,
author={Liu, X. and Zhang, Z.},
title={A Vision-Based Target Detection, Tracking, and Positioning Algorithm for Unmanned Aerial Vehicle},
journal={Wireless Communications and Mobile Computing},
year={2021},
volume={2021},
art_number={5565589},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85105762417&doi=10.1155%2f2021%2f5565589&partnerID=40&md5=a1036b5775241698abaa783cc4d91c1e},
abstract={Unmanned aerial vehicles (UAV) play a pivotal role in the field of security owing to their flexibility, efficiency, and low cost. The realization of vehicle target detection, tracking, and positioning from the perspective of a UAV can effectively improve the efficiency of urban intelligent traffic monitoring. In this work, by fusing the target detection network, YOLO v4, with the detection-based multitarget tracking algorithm, DeepSORT, a method based on deep learning for automatic vehicle detection and tracking in urban environments, has been designed. With the aim of addressing the problem of UAV positioning a vehicle target, the state equation and measurement equation of the system have been constructed, and a particle filter based on interactive multimodel has been employed for realizing the state estimation of the maneuvering target in the nonlinear system. Results of the simulation show that the algorithm proposed in this work can detect and track vehicles automatically in urban environments. In addition, the particle filter algorithm based on an interactive multimodel significantly improves the performance of the UAV in terms of positioning the maneuvering targets, and this has good engineering application value. © 2021 Xin Liu and Zhanyue Zhang.},
}

@ARTICLE{Kuzmin2021,
author={Kuzmin, A. and Korhonen, L. and Kivinen, S. and Hurskainen, P. and Korpelainen, P. and Tanhuanpää, T. and Maltamo, M. and Vihervaara, P. and Kumpula, T.},
title={Detection of european aspen (populus tremula L.) based on an unmanned aerial vehicle approach in boreal forests},
journal={Remote Sensing},
year={2021},
volume={13},
number={9},
art_number={1723},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85105586543&doi=10.3390%2frs13091723&partnerID=40&md5=ebc2e4600ac363d550b77a27f7eea7d4},
abstract={European aspen (Populus tremula L.) is a keystone species for biodiversity of boreal forests. Large-diameter aspens maintain the diversity of hundreds of species, many of which are threatened in Fennoscandia. Due to a low economic value and relatively sparse and scattered occurrence of aspen in boreal forests, there is a lack of information of the spatial and temporal distribution of aspen, which hampers efficient planning and implementation of sustainable forest management practices and conservation efforts. Our objective was to assess identification of European aspen at the individual tree level in a southern boreal forest using high-resolution photogrammetric point cloud (PPC) and multispectral (MSP) orthomosaics acquired with an unmanned aerial vehicle (UAV). The structure-from-motion approach was applied to generate RGB imagery-based PPC to be used for individual tree-crown delineation. Multispectral data were collected using two UAV cameras: Parrot Sequoia and MicaSense RedEdge-M. Tree-crown outlines were obtained from watershed segmentation of PPC data and intersected with multispectral mosaics to extract and calculate spectral metrics for individual trees. We assessed the role of spectral data features extracted from PPC and multispectral mosaics and a combination of it, using a machine learning classifier-Support Vector Machine (SVM) to perform two different classifications: discrimination of aspen from the other species combined into one class and classification of all four species (aspen, birch, pine, spruce) simultaneously. In the first scenario, the highest classification accuracy of 84% (F1-score) for aspen and overall accuracy of 90.1% was achieved using only RGB features from PPC, whereas in the second scenario, the highest classification accuracy of 86 % (F1-score) for aspen and overall accuracy of 83.3% was achieved using the combination of RGB and MSP features. The proposed method provides a new possibility for the rapid assessment of aspen occurrence to enable more efficient forest management as well as contribute to biodiversity monitoring and conservation efforts in boreal forests. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@ARTICLE{Dutta2021,
author={Dutta, T. and Soni, A. and Gona, P. and Gupta, H.P.},
title={Real Testbed for Autonomous Anomaly Detection in Power Grid using low-cost Unmanned Aerial Vehicles and Aerial Imaging},
journal={IEEE Multimedia},
year={2021},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85104659906&doi=10.1109%2fMMUL.2021.3075295&partnerID=40&md5=874d60328a3beb4ff183ec1297f53199},
abstract={Critical utility infrastructure like power grid is vast (in hundreds of kilometers), linear, and operated 24x7 throughout the year. Maintenance inspections using low-cost unmanned aerial vehicles and aerial imaging, are therefore gaining popularity. To have low-cost framework, the quality of camera used is not of high quality or a stereo-rig one. Also, the sensors used are limited in variety and efficiency. 3D reconstruction of a power grid will help to improve access, detect anomalies (damages), and reduce projection error. The depth estimation of wiry objects, like powerlines, in a cluttered background is challenging. The background clutter includes trees, pavement, greenery patches, and man-made objects. In this paper, we propose an efficient framework for 3D anomaly detection in power grid using UAV-based aerial images. The framework uses context information to become adaptive with different nonlinear movements that are unavoidable in aerial imaging. The proposed work is tested on real-data captured using a low-cost framework consisting of a non-stereo-rig aerial camera and a mini-UAV. IEEE},
}

@ARTICLE{Hong2021,
author={Hong, H. and He, K. and Gan, Z. and Jiang, G.},
title={Stability Precision Error Correction of Photoelectric Detection by Unmanned Aerial Vehicle},
journal={Journal of Sensors},
year={2021},
volume={2021},
art_number={5564448},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85104463050&doi=10.1155%2f2021%2f5564448&partnerID=40&md5=8b585c47c9e9dc1cd8300585395906ab},
abstract={For getting clear images and overcoming shaking caused by various disturbances, real-time compensation of pointing errors will improve the overall stability performance of photoelectric detection by unmanned aerial vehicle. However, the compensation will be greatly deteriorated by error-causing sources, and the error correction process is of great importance. In this research, the problem of stability precision error correction is comprehensively studied. First, by modeling overall kinematics, error-causing sources, and error compensation, the error correction process is mathematically modeled and simulated. Then, by using simulation data regression, error correction models including the global function model and parametric model are established. The models are validated by carrying out both simulations and validation experiments. At last, the performances of the error correction models are compared and analyzed, which concerns the factors of parameter identification, model simplicity, and final improvement effect. Results show that the final stability precision can be greatly improved over 20%, and the parametric model outperforms the global function model comprehensively. It can be concluded that, either in simulation environment or real application scenarios, the obtained models and related analysis results are effective in improving the system stability performance. © 2021 Huajie Hong et al.},
}

@ARTICLE{Arantes2021,
author={Arantes, B.H.T. and Moraes, V.H. and Geraldine, A.M. and Alves, T.M. and Albert, A.M. and da Silva, G.J. and Castoldi, G.},
title={Spectral detection of nematodes in soybean at flowering growth stage using unmanned aerial vehicles [Detecção espectral de nematóides na soja em estádio de florescimento por meio de veículos aéreos não-tripulados]},
journal={Ciencia Rural},
year={2021},
volume={51},
number={5},
art_number={e20200283},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85103882760&doi=10.1590%2f0103-8478cr20200283&partnerID=40&md5=33e5b329ba99a509d36d97889ae29d7d},
abstract={Soybean is one of the main crop species grown in the world. However, there is a decline in productivity due to the various types of stress, including the nematodes Heterodera glycines and Pratylenchus brachyurus. The objectives were to determine the best spectral band for detecting H. glycines and P. brachyurus at the beginning of flowering (R1). Soil and root sampling was conducted at nine sampling sites in each of the five nematode-infested regions, totaling 45 sampling points. Flights were made at all regions using Phantom 4 Advanced, Sequoia and 14-band customized Sentera. For H. glycines, the red spectral band best explained the variability on soil and root nematode counts as well as the second stage of juveniles in soil. For P. brachyurus, Sentera RedEdge best explained the variability in root nematode counts and Sequoia NIR best explained soil juveniles. A multiple linear regression model using spectral data for detecting P. brachyurus and H. glycines improved R² compared to simple linear regressions. At flowering growth stage (R1), soybean spectral reflectance was associated with the number of H. glycines and P. brachyurus on soil and roots using low-cost and multispectral sensors. © 2021, Universidade Federal de Santa Maria. All rights reserved.},
}

@ARTICLE{López-Estrada2021254,
author={López-Estrada, F.R. and Méndez-López, A. and Santos-Ruiz, I. and Valencia-Palomo, G. and Escobar-Gómez, E.},
title={Fault detection in unmanned aerial vehicles via orientation signals and machine learning [Detección de fallas en vehículos aéreos no tripulados mediante señales de orientación y técnicas de aprendizaje de máquina]},
journal={RIAI - Revista Iberoamericana de Automatica e Informatica Industrial},
year={2021},
volume={18},
number={3},
pages={254-264},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85101420541&doi=10.4995%2fRIAI.2020.14031&partnerID=40&md5=8bc2022371a286a78ba664be8b542837},
abstract={This work proposes an actuator fault detection and isolation scheme for a quadrotor unmanned aerial vehicle (UAV) under a data-driven approach using machine learning techniques. In this approach, an implicit model of the system is built through the information provided by the onboard sensors of the UAV. First, using a tailored flying platform, vibrations corresponding to the orientation, angular position and linear acceleration were captured with the UAV flying in hover mode under nominal conditions. This data is processed by Principal Component Analysis (PCA) for feature extraction. Subsequently, faults in the actuators are induced through a cut in each of the UAV propellers which generate a reduction in the thrust of the rotors. These data are also projected into the PCA subspace and compared to the nominal data. Hotelling’s T 2 statistic is used to discern between nominal data and data when the vehicle exhibits an actuator fault. Finally, the developed algorithms were complemented with k-nearest neighbors (k-NN) and support vector machine (SVM) classification algorithms. The results show a correct classification rate of 89.6 % (k-NN) and 92.4 % (SVM) respectively for 423 validation datasets. © 2021 Universitat Politecnica de Valencia. All rights reserved.},
}

@ARTICLE{Gbopa202141,
author={Gbopa, A.O. and Ayodele, E.G. and Okolie, C.J. and Ajayi, A.O. and Iheaturu, C.J.},
title={Unmanned aerial vehicles for three-dimensional mapping and change detection analysis6},
journal={Geomatics and Environmental Engineering},
year={2021},
volume={15},
number={1},
pages={41-61},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85101068425&doi=10.7494%2fgeom.2021.15.1.41&partnerID=40&md5=191f62f54163696edd8f0cca2ff7896a},
abstract={Unmanned Aerial Vehicles (UAVs), commonly known as drones are increas-ingly being used for three-dimensional (3D) mapping of the environment. This study utilised UAV technology to produce a revised 3D map of the University of Lagos as well as land cover change detection analysis. A DJI Phantom 4 UAV was used to collect digital images at a flying height of 90 m, and 75% fore and 65% side overlaps. Ground control points (GCPs) for orthophoto rectifica-tion were coordinated with a Trimble R8 Global Navigation Satellite System. Pix4D Mapper was used to produce a digital terrain model and an orthophoto at a ground sampling distance of 4.36 cm. The change detection analysis, using the 2015 base map as reference, revealed a significant change in the land cover such as an increase of 16,306.7 m2 in buildings between 2015 and 2019. The root mean square error analysis performed using 7 GCPs showed a horizontal and vertical accuracy of 0.183 m and 0.157 m respectively. This suggests a high level of accuracy, which is adequate for 3D mapping and change detection analysis at a sustainable cost. © 2020 Authors.},
}

@CONFERENCE{Saeed2021624,
author={Saeed, M.S.},
title={Unmanned Aerial Vehicle for Automatic Detection of Concrete Crack using Deep Learning},
journal={International Conference on Robotics, Electrical and Signal Processing Techniques},
year={2021},
pages={624-628},
art_number={9331177},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85100818701&doi=10.1109%2fICREST51555.2021.9331177&partnerID=40&md5=368882be20bd58764a0d603927dcfe8d},
abstract={Cracks in concrete structure can lead to catastrophic damage if not addressed correctly at the right time. Although crack close to ground surfaces are easily addressable, however cracks on the surface of pillars of bridges, high-rise buildings and tall concrete structures are difficult to notice due to their heights and if left unaddressed can be risky and may lead to massive damage. Visual inspection is normally done to identify the cracks but it is time consuming and costly, it is also dangerous for specialists, and improper environments can cause evaluation errors. This paper proposes an efficient method of automatically detecting cracks by using Convolutional Neural Network with the help of an unmanned aerial vehicle. The crack detection model was developed and trained from scratch and achieved a training accuracy of 98.60% and validation accuracy of 96.84% before transferring it to a raspberry pi 4 mounted on an Unmanned Arial Vehicle which was developed and tested with the model. © 2021 IEEE.},
}

@ARTICLE{Liu20212236,
author={Liu, W. and Xu, J. and Guo, Z. and Li, E. and Li, X. and Zhang, L. and Liu, W.},
title={Building Footprint Extraction from Unmanned Aerial Vehicle Images Via PRU-Net: Application to Change Detection},
journal={IEEE Journal of Selected Topics in Applied Earth Observations and Remote Sensing},
year={2021},
volume={14},
pages={2236-2248},
art_number={9327466},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85099724210&doi=10.1109%2fJSTARS.2021.3052495&partnerID=40&md5=35209de803b1515c20a60e5b02b41768},
abstract={As the manual detection of building footprint is inefficient and labor-intensive, this study proposed a method of building footprint extraction and change detection based on deep convolutional neural networks. The study modified the existing U-Net model to develop the 'PRU-Net' model. PRU-Net incorporates pyramid scene parsing (PSP) to allow multiscale scene parsing, a residual block (RB) in ResNet for feature extraction, and focal loss to address sample imbalance. Within the proposed method, building footprint extraction is conducted as follows: 1) unmanned aerial vehicle images are cropped, denoised, and semantically marked, and datasets are created (including training/validation and prediction datasets); 2) the training/validation and prediction datasets are input into the full convolutional neural network PRU-Net for model training/validation and prediction. Compared with the U-Net, PSP+U-Net (PU-Net), and U-Net++ models, PRU-Net offers improved footprint extraction of buildings with a range of sizes and shapes. The large-scale experimental results demonstrated the effectiveness of the PSP module for multiscale scene analysis and the RB module for feature extraction. After demonstrating the improvements in building extraction offered by PRU-Net, the building footprint results were further processed to generate a building change map. © 2008-2012 IEEE.},
}

@ARTICLE{Golcarenarenji20212440,
author={Golcarenarenji, G. and Martinez-Alpiste, I. and Wang, Q. and Alcaraz-Calero, J.M.},
title={Efficient Real-Time Human Detection Using Unmanned Aerial Vehicles Optical Imagery},
journal={International Journal of Remote Sensing},
year={2021},
volume={42},
number={7},
pages={2440-2462},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85098663237&doi=10.1080%2f01431161.2020.1862435&partnerID=40&md5=0e2069f834f62272ed5a9732459b1b98},
abstract={Unmanned Aerial Vehicles (UAVs) are promising technologies within many different application scenarios including human detection in search and rescue and surveillance use cases, which have received considerable attention worldwide. However, adverse conditions, such as varying altitude, overhead camera placement, changing illumination and moving platform, impose challenges for high-performance yet cost-efficient human detection. To overcome these challenges, we propose a novel combination of dilated convolutions with Path Aggregation Network (PAN) as a new deep neural network-based human detection algorithm in real time. Furthermore, we establish a comprehensive human detection dataset with varying backgrounds, illuminations, and contrast and train the proposed machine-learning model on the collected dataset. Our approach achieves both high precision (88.0% mean Average Precision (mAP)) and real time (67.0 Frames Per Second (FPS)) on a commercial off-the-shelf PC platform. In terms of accuracy, the result is comparable to the standard You Only Look Once v3 (YOLOv3). However, the speed is twice as that of the standard YOLOv3. YOLOv4 is slightly more accurate (89.8%) than our approach. However, it is slower (38.0 versus 67.0 FPS) and has more Billion Floating-Point Operations (BFLOPS). The proposed algorithm has also trained with the VisDrone2019 dataset and compared with seven studies using this dataset. The results have further validated the effectiveness of the proposed approach. Moreover, the algorithm has been evaluated on an embedded system (Jetson AGX Xavier), which demonstrates the usefulness of this method on power-constrained devices. The proposed algorithm is fast, memory efficient, and computationally less expensive to achieve high detection performance. It is expected to contribute significantly to the wider use of UAV applications including search and rescue missions to locate missing people, and surveillance particularly for applications running on resource-constrained platforms, like smartphones or tablets. This proposed system is now being used in aerial drone system of Police of Scotland to help them locate and find missing and vulnerable people. The results of the project were broadcasted by BBC Scotland. © 2020 Informa UK Limited, trading as Taylor & Francis Group.},
}

@ARTICLE{Vergura2021124,
author={Vergura, S.},
title={Correct Settings of a Joint Unmanned Aerial Vehicle and Infrared Camera System for the Detection of Faulty Photovoltaic Modules},
journal={IEEE Journal of Photovoltaics},
year={2021},
volume={11},
number={1},
pages={124-130},
art_number={9252969},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85098260322&doi=10.1109%2fJPHOTOV.2020.3033777&partnerID=40&md5=bda011c84087b253f2b17061a2af1827},
abstract={The technological development of photovoltaic (PV) devices (perovskite-based or bifacial modules, etc.) has progressed considerably, but the commercial PV modules do not show analogous improvements and their efficiency is still low. Therefore, a diagnostic tool that can check the current operation of installed PV modules and their aging is important. In this scenario, an unmanned aerial vehicle (UAV), equipped with a camera, infrared (IR) camera, or both, represents a new avenue for the fast evaluation of faults for large or not easily accessible PV plants and the discovery of defective PV modules. Thermography has the advantage of not disconnecting the PV system during the inspection. Nevertheless, some specific parameters, such as the emissivity, the reflected temperature, and the resolution, are fixed during the acquisition, even if their values are dependent on the mutual position (distance and angle) between the IR camera and the PV modules. The movement of the UAV, equipped with an IR camera, modifies the position of the IR camera, and due to this movement, the values of the parameters can be incorrect during acquisition, which also results in errors in the radiometric map. In this article, we explore these issues and provide suggestions to ensure the correct acquisition and reading of thermal images of PV modules. © 2011-2012 IEEE.},
}

@ARTICLE{Ruiz20211099,
author={Ruiz, R.D.B. and Lordsleem Júnior, A.C. and Fernandes, B.J.T. and Oliveira, S.C.},
title={Unmanned Aerial Vehicles and Digital Image Processing with Deep Learning for the Detection of Pathological Manifestations on Facades},
journal={Lecture Notes in Civil Engineering},
year={2021},
volume={98},
pages={1099-1112},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85088447369&doi=10.1007%2f978-3-030-51295-8_76&partnerID=40&md5=4feb38614b0b55256780cb4fd2d16158},
abstract={In the diagnosis phase of pathological manifestations in facades, the visual inspection stage deserves special attention due to its inherent complexity (height, size, access difficulties and exposure conditions). In recent years, the use of deep learning techniques to detect and classify specific features in images and videos has been increasing, which when combined with the use of Unmanned Aerial Vehicles (UAVs) for capturing images, is a potential useful tool that can assist and automate the visual inspection procedure of facades. This paper aimed to perform the analysis of Digital Image Processing (DIP) for automatic detection of cracks in building ceramic tiles, associated with UAV, which would potentially result in benefits (time, cost and safety) with respect to diagnosis. Thus, the research results showed the technical feasibility of detection of cracks by DIP techniques, however, the main limitation for this purpose is the lack of a dataset of images of pathological manifestations in facades publicly available, restricting the computer learning process and consequently compromising the recognition capacity. Still, the project was able to develop a simple and efficient methodology to what was proposed. © 2021, The Editor(s) (if applicable) and The Author(s), under exclusive license to Springer Nature Switzerland AG.},
}

@ARTICLE{Mawrence20201,
author={Mawrence, R. and Munniks, S. and Valente, J.},
title={Calibration of electrochemical sensors for nitrogen dioxide gas detection using unmanned aerial vehicles},
journal={Sensors (Switzerland)},
year={2020},
volume={20},
number={24},
pages={1-13},
art_number={7332},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85098105745&doi=10.3390%2fs20247332&partnerID=40&md5=a1f6d960a628144115a1d78f166bf974},
abstract={For years, urban air quality networks have been set up by private organizations and governments to monitor toxic gases like NO2. However, these networks can be very expensive to maintain, so their distribution is usually widely spaced, leaving gaps in the spatial resolution of the resulting air quality data. Recently, electrochemical sensors and their integration with unmanned aerial vehicles (UAVs) have attempted to fill these gaps through various experiments, none of which have considered the influence of a UAV when calibrating the sensors. Accordingly, this research attempts to improve the reliability of NO2 measurements detected from electrochemical sensors while on board an UAV by introducing rotor speed as part of the calibration model. This is done using a DJI Matrice 100 quadcopter and Alphasense sensors, which are calibrated using regression calculations in different environments. This produces a predictive r-squared up to 0.97. The sensors are then calibrated with rotor speed as an additional variable while on board the UAV and flown in a series of flights to evaluate the performance of the model, which produces a predictive r-squared up to 0.80. This methodological approach can be used to obtain more reliable NO2 measurements in future outdoor experiments that include electrochemical sensor integration with UAV’s. © 2020 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@CONFERENCE{Meng2020280,
author={Meng, W. and Tia, M.},
title={Unmanned aerial vehicle classification and detection based on deep transfer learning},
journal={Proceedings - 2020 International Conference on Intelligent Computing and Human-Computer Interaction, ICHCI 2020},
year={2020},
pages={280-285},
art_number={9424778},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85106408656&doi=10.1109%2fICHCI51889.2020.00067&partnerID=40&md5=2cc214b83f15aa98cd47c4ef17861d91},
abstract={Currently, major security incidents caused by the 'unlicensed flying' of Unmanned Aerial Vehicle (UAV) have emerged one after another, which poses a grave threat to the security issues of public facilities and sensitive areas. Whether it can timely detect and prevent 'unlicensed flying' of UAV has become a social concern. In response to this demand, the transfer learning method is adopted in this paper to conduct twoclassification and detection on UAV images. Image recognition technology based on transfer learning is an effective method to improve recognition accuracy by applying deep learning models to small samples. Different from the large number of training samples required by deep learning, transfer learning transfers the weights of the pre-trained deep neural network, and uses only small sample data to obtain good results in UAV image recognition. First of all, this paper proposes to construct a UAV data set according to different types of UAV shape structures, to perfect the classification and detection effect and the generalization ability of the model. Then, based on the transfer learning method, experimental comparison is made between three classic deep convolutional neural network classification models (Inception V3, ResNet 101 and VGG16) and two classic deep convolutional neural network detection models (Faster RCNN and SSD). Finally, an experimental evaluation is conducted on the collected UAV test data set. Compared with the traditional recognition model, the image classification model based on transfer learning employed in this paper has achieved important improvements in accuracy, recall and precision. Especially in the InceptionV3 model of transfer training, the recall reaches 96.98%. In addition, the image detection model based on transfer learning has achieved good detection results in accuracy, recall and F1-score. © 2020 IEEE.},
}

@CONFERENCE{Utomo2020234,
author={Utomo, W. and Bhaskara, P.W. and Kurniawan, A. and Juniastuti, S. and Yuniarno, E.M.},
title={Traffic Congestion Detection Using Fixed-Wing Unmanned Aerial Vehicle (UAV) Video Streaming Based on Deep Learning},
journal={CENIM 2020 - Proceeding: International Conference on Computer Engineering, Network, and Intelligent Multimedia 2020},
year={2020},
pages={234-238},
art_number={9297921},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85099642027&doi=10.1109%2fCENIM51130.2020.9297921&partnerID=40&md5=51c5c2a21762c1ea3267205cabbfc8fe},
abstract={Population growth in the region has led to increased use of roads that causes traffic congestion. Traffic congestion also occurs during long weekend in outsides city. The roads in the area are usually smooth traffic flow, it becomes very congested. One method of the smart road monitoring system is a fixed camera sensor as input and artificial intelligent as the analysis. However, these methods require a great infrastructure on highways such as: power supply, protective CPU, good power supply and stable computer network connections. This will be difficult to fulfill if applied on roads outside the city. To overcome the problem, we propose a system of vehicles detection and road density classification using Fixed-Wing Unmanned Aerial Vehicle (UAV) video streaming. We chose Fixed-Wing UAV for its advantages: wide range and fast flight speed. The proposed system detects and classifies vehicles. Vehicles are detected and calcified using CNN's Deep Learning which uses the YOLO architecture. The level of traffic density is determined by the area of the road covered by vehicles to road area. We tested the proposed system using YouTube video and UAV video streaming. Both experimental scenarios have almost the same results. Precisions of recording video UAV and streaming video are: 90.75% and 90%, respectively. © 2020 IEEE.},
}

@CONFERENCE{Whelan202023,
author={Whelan, J. and Sangarapillai, T. and Minawi, O. and Almehmadi, A. and El-Khatib, K.},
title={Novelty-based Intrusion Detection of Sensor Attacks on Unmanned Aerial Vehicles},
journal={Q2SWinet 2020 - Proceedings of the 16th ACM Symposium on QoS and Security for Wireless and Mobile Networks},
year={2020},
pages={23-28},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85097649377&doi=10.1145%2f3416013.3426446&partnerID=40&md5=cafd94dcce96eb7daeee4e8265aecf2f},
abstract={Unmanned Aerial Vehicles (UAVs) have proven to be a useful technology in numerous industries including industrial control systems surveillance, law enforcement, and military operations. Due to their heavy reliance on wireless protocols and hostile operating environments, UAVs face a large threat landscape. As attacks against UAVs increase, an intelligent intrusion detection system (IDS) is needed to aid the UAV in identifying attacks. The UAV domain presents unique challenges for intelligent IDS development, such as the variety of sensors, communication protocols, UAV platforms, control configurations, and dataset availability. In this paper, we propose a novelty-based approach to intrusion detection in UAVs by using one-class classifiers. One-class classifiers require only non-anomalous data to exist in the training set. This allows for the use of flight logs as training data, which are created by most UAVs during flight by default. Principal Component Analysis is applied to sensor logs for dimensionality reduction, and one-class classifier models are generated per sensor. A number of one-class classifiers are selected: One-Class Support Vector Machine, Autoencoder Neural Network, and Local Outlier Factor. The pre-processing, feature selection, training, and tuning of the selected algorithms is discussed. GPS spoofing is used throughout the paper as a common example of an external sensor-based attack. This approach shows to be effective across multiple UAV platforms with platform-specific F1 scores up to 99.56% and 99.73% for benign and malicious sensor readings respectively. © 2020 ACM.},
}

@CONFERENCE{Martinez-Alpiste20209,
author={Martinez-Alpiste, I. and Golcarenarenji, G. and Wang, Q. and Alcaraz-Calero, J.M.},
title={Real-Time Low-Pixel Infrared Human Detection from Unmanned Aerial Vehicles},
journal={DIVANet 2020 - Proceedings of the 10th ACM Symposium on Design and Analysis of Intelligent Vehicular Networks and Applications},
year={2020},
pages={9-15},
art_number={3424600},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85096978925&doi=10.1145%2f3416014.3424600&partnerID=40&md5=8ec4081c45044656a04f23bbbd0ee9dc},
abstract={To improve the speed and accuracy in human detection in Search and Rescue (SAR) operations, this paper presents a novel and highly efficient machine learning empowered system by extending the You Only Look Once (YOLO) algorithm, which is designed and deployed on an embedded system. The proposed approach has been evaluated under real-world conditions on a Jetson AGX Xavier platform and the results have shown a well-balanced system in terms of accuracy, speed and portability. Moreover, the system demonstrates its resilience to perform low-pixel human detection on infrared images received from an Unmanned Aerial Vehicle (UAV) at low-light conditions, different altitudes and postures such as sitting, walking and running. The proposed approach has achieved in a constrained environment a total of 89.26% of accuracy and 24.6 FPS, surpassing the barrier of real-time object recognition. © 2020 ACM.},
}

@ARTICLE{Liu20201,
author={Liu, T. and Shi, T. and Zhang, H. and Wu, C.},
title={Detection of rise damage by leaf folder (Cnaphalocrocis medinalis) using unmanned aerial vehicle based hyperspectral data},
journal={Sustainability (Switzerland)},
year={2020},
volume={12},
number={22},
pages={1-15},
art_number={9343},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85096015604&doi=10.3390%2fsu12229343&partnerID=40&md5=07e030962166d2b71832579c70ceb36d},
abstract={Crop pests and diseases are key factors that damage crop production and threaten food security. Remote sensing techniques may provide an objective and effective alternative for automatic detection of crop pests and diseases. However, ground-based spectroscopic or imaging sensors may be limited in practically guiding the precision application and reduction of pesticide. Therefore, this study developed an unmanned aerial vehicle (UAV)-based remote sensing system to detect leaf folder (Cnaphalocrocis medinalis). Rice canopy reflectance spectra were obtained in the booting growth stage by using the UAV-based hyperspectral remote sensor. Newly developed and published multivariate spectral indices were initially calculated to estimate leaf-roll rates. The newly developed two-band spectral index (R490−R470), three-band spectral index (R400−R470)/(R400−R490), and published spectral index photochemical reflectance index (R550−R531)/(R550+R531) showed good applicability for estimating leaf-roll rates. The newly developed UAV-based micro hyperspectral system had potential in detecting rice stress induced by leaf folder. The newly developed spectral index (R490−R470) and (R400−R470)/(R400−R490) might be recommended as an indicator for estimating leaf-roll rates in the study area, and (R550−R531)/(R550+R531) might serve as a universal spectral index for monitoring leaf folder. © 2020 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@ARTICLE{Tao20208238,
author={Tao, H. and Li, C. and Zhao, D. and Deng, S. and Hu, H. and Xu, X. and Jing, W.},
title={Deep learning-based dead pine tree detection from unmanned aerial vehicle images},
journal={International Journal of Remote Sensing},
year={2020},
volume={41},
number={21},
pages={8238-8255},
note={cited By 7},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85089183153&doi=10.1080%2f01431161.2020.1766145&partnerID=40&md5=c9b1a895c865954d6f17090895cb23a0},
abstract={Understanding the spatial distribution of dead pine trees (DPTs) in mountainous areas is vital for diseased wood cleanup and the prediction of pine wilt disease. The study induced a deep learning (DL) model of convolutional neural networks (CNNs) for the DPT detection using unmanned aerial vehicle images. Two thousand manually labelled DPT and Non-DPT samples were collected to train (80%) and optimize (20%) the CNNs of AlexNet and GoogLeNet, and 768 samples from other three areas were used to predict the categories in Jinjiang, Fujian, southeastern China. The same dataset was used to compare the classification accuracy between CNNs and the traditional template matching (TM) method. In addition, the potential factors influencing the overall accuracy of the DL model for DPT detection were evaluated. Training results of AlexNet and GoogLeNet showed an accuracy of over 93.30% and 97.38% respectively for the top-1 test after the final training iteration. For the DPT classification in the prediction areas of pure forests, the TM method showed the 56–65% of overall accuracy while CNNs showed 65–80%. CNNs-based DPT detection was more accurate than the traditional TM method. Terrains and red broadleaf trees influence the CNNs-based DPT detection from aerial visible-images in mixed artificial forest and peaks areas. © 2020 Informa UK Limited, trading as Taylor & Francis Group.},
}

@CONFERENCE{Wang2020137,
author={Wang, G. and Hong, H. and Zhang, Y. and Wu, J. and Wang, Y. and Li, S.},
title={Realization of Detection Algorithms for Key Parts of Unmanned Aerial Vehicle Based on Deep Learning},
journal={12th International Conference on Wireless Communications and Signal Processing, WCSP 2020},
year={2020},
pages={137-142},
art_number={9299682},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85099480291&doi=10.1109%2fWCSP49889.2020.9299682&partnerID=40&md5=1596218bb817d3e8a150af3804dc6404},
abstract={Fixed-point attack on the key parts of small aerial vehicles is one of the important means of UAV (Unmanned Aerial Vehicle) countermeasure. Fixed-wing aircraft flying in the air has two characteristics: fast speed and fast attitude change of aircraft. However, the traditional detection method of key parts of fixed-wing aircraft in infrared images is not only slow in speed but also low in accuracy. This paper presents an improved target detection and motion tracking algorithm based on deep learning method. The algorithm uses a deeper neural network to enhance the feature extraction capabilities of CNN and obtain richer feature information. The detection algorithm obtains the position and motion direction of the key points of the target. Experimental results show that the detection algorithm proposed in this paper is up to 30 frame/s, with an average accuracy of 91.5%/. The method achieved good results in the experiment. © 2020 IEEE.},
}

@CONFERENCE{Rahman2020,
author={Rahman, M.A. and Rahman, M.T. and Kisacikoglu, M. and Akkaya, K.},
title={Intrusion Detection Systems-Enabled Power Electronics for Unmanned Aerial Vehicles},
journal={2020 IEEE CyberPELS, CyberPELS 2020},
year={2020},
art_number={9311545},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85100254808&doi=10.1109%2fCyberPELS49534.2020.9311545&partnerID=40&md5=d75427509c8648563b5460f8d0333fb0},
abstract={Compromised power electronics, due to firmware attacks and hardware Trojans, in a flight computer can jeopardize the safety and security of an Unmanned Aerial Vehicle (UAV). They can maliciously alter sensor measurements or control commands to make a UAV to take disastrous moves. Unfortunately, most of these attacks are difficult to detect before deploying components in the system. Therefore, detecting compromised behavior run-time is important, while it is challenging at the same time. In this work, we propose to build machine learning-based intrusion detection systems (IDSs) to be deployed at the power electronics/microcontorller level such that it can deal with malicious data/control commands initiated due to hardware attacks. © 2020 IEEE.},
}

@CONFERENCE{Kantue2020336,
author={Kantue, P. and Pedro, J.O.},
title={Integrated Fault Detection and Diagnosis of an Unmanned Aerial Vehicle using Time Difference of Arrival},
journal={2020 24th International Conference on System Theory, Control and Computing, ICSTCC 2020 - Proceedings},
year={2020},
pages={336-342},
art_number={9259777},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85097983956&doi=10.1109%2fICSTCC50638.2020.9259777&partnerID=40&md5=c11f0ba994fb9f255bf866f106ffd3f9},
abstract={An integrated approach to the fault detection and diagnosis (FDD) of an unmanned aerial vehicle is presented. A novel approach using the Time Difference Of Arrival (TDOA) principle has been developed to detect, isolate and identify an incipient fault condition in the rotor dynamics. The requirements of a reconfigurable controller (RC) has been taken into account through the real-time implementation of a continuous forward algorithm (CFA) with a golden section search (GSS) combined with a meta-heuristic global optimization technique. The training and testing data for Radial Basis Function Neural Networks (RBF-NN) learning and prediction were supplied in discrete-time and its integration capacity validated through a Hardware-in-the-loop simulation (HILS) using a Teensy 3.6 microcontroller. The Pseudo real-time desktop simulation showed that the FDD algorithm was able to detect and isolate an incipient rotor fault and supply the RC a post-fault model and associated fault uncertainties. This method showed robustness towards prediction errors (bias and variance) and can be used in an integrated fault-tolerant control framework. © 2020 IEEE.},
}

@CONFERENCE{Asri2020,
author={Asri, N.A.M. and Sakidin, H. and Othman, M. and Matori, A.N. and Ahmad, A.},
title={Analysis of the hydrocarbon seepage detection in oil palm vegetation stress using unmanned aerial vehicle (UAV) multispectral data},
journal={AIP Conference Proceedings},
year={2020},
volume={2266},
art_number={050007},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85094574504&doi=10.1063%2f5.0018054&partnerID=40&md5=e75077b2bf8463ce66e9ccb1bc1b9b4d},
abstract={Due to difference pressure beneath the earth, oil and gas or known as hydrocarbon most probably rises to the surface. This presence of oil and gas can be identified through their seepage. The hydrocarbon seepage can lead to an abnormality of soil and dynamism of vegetation health on land surface. This phenomenon can be act as indicator for detecting potential onshore of oil and gas reservoir. Through remote sensing spectral reflectance vegetation index, the abnormality and dynamism of plant growth can be detected. In this study, spectral reflectance data originating from Unmanned Aerial Vehicle (UAV) Multispectral is used to monitor and determine the hydrocarbon seepage detection in oil palm vegetation stress. Based on the experimental design, 12 oil palm trees were simulated with crude oil and remaining three trees were left as control sample which these trees are divided into five sample. The spectra acquisition was taken on the first day, 30th day, 60th day and 90th day of experiment. From the data, the potential visible region and Near - Infrared (NIR) reflectance region being investigated by exerted the statistical analysis to vegetation index which is Normalised Difference Vegetation Index (NDVI) data trends to study the impact of hydrocarbon seepage towards oil palm tree. Detecting hydrocarbon seepage using vegetation reflectance is very useful in oil and gas field as this can be one of the alternative approaches in exploring new oil and gas resources. © 2020 Author(s).},
}

@ARTICLE{Chen2020803,
author={Chen, X. and Chen, W. and Rao, Y. and Huang, Y. and Guan, J. and Dong, Y.},
title={Progress and prospects of radar target detection and recognition technology for flying birds and unmanned aerial vehicles (in English)},
journal={Journal of Radars},
year={2020},
volume={9},
number={5},
pages={803-827},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85101760475&doi=10.12000%2fJR20068&partnerID=40&md5=b4afb5d9e10eb9242f4b85d6bc947faf},
abstract={Flying birds and Unmanned Aerial Vehicles (UAVs) are typical "low, slow, and small" targets with low observability. The need for effective monitoring and identification of these two targets has become urgent and must be solved to ensure the safety of air routes and urban areas. There are many types of flying birds and UAVs that are characterized by low flying heights, strong maneuverability, small radar cross-sectional areas, and complicated detection environments, which are posing great challenges in target detection worldwide. "Visible (high detection ability) and clear-cut (high recognition probability)" methods and technologies must be developed that can finely describe and recognize UAVs, flying birds, and "low-slow-small" targets. This paper reviews the recent progress in research on detection and recognition technologies for rotor UAVs and flying birds in complex scenes and discusses effective detection and recognition methods for the detection of birds and drones, including echo modeling and recognition of fretting characteristics, the enhancement and extraction of maneuvering features in ubiquitous observation mode, distributed multi-view features fusion, differences in motion trajectories, and intelligent classification via deep learning. Lastly, the problems of existing research approaches are summarized, and we consider the future development prospects of target detection and recognition technologies for flying birds and UAVs in complex scenarios. © 2020 Institute of Electronics Chinese Academy of Sciences. All rights reserved.},
}

@ARTICLE{Chen2020,
author={Chen, T. and Yang, W. and Zhang, H. and Zhu, B. and Zeng, R. and Wang, X. and Wang, S. and Wang, L. and Qi, H. and Lan, Y. and Zhang, L.},
title={Early detection of bacterial wilt in peanut plants through leaf-level hyperspectral and unmanned aerial vehicle data},
journal={Computers and Electronics in Agriculture},
year={2020},
volume={177},
art_number={105708},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85089341225&doi=10.1016%2fj.compag.2020.105708&partnerID=40&md5=6daa7873d415b494ae34590c1ed2b041},
abstract={Bacterial wilt (BW) caused by Ralstonia solanacearum is the most serious peanut diseases in South China. Its timely and accurate detection is important to opportunely implement disease management practices. This study aimed to establish and select the most appropriate leaf-level reflectance-based vegetation indices for BW detection and to determine whether these new indices can be used in UAV multispectral imaging for peanut BW detection. ANOVA, multilayer perception, and the reduced sampling method were used to analyze the spectral data. The most effective detection wavelengths, 730 nm and 790 nm, were used for developing new peanut BW detection indices. The 15 hyperspectral indices with highest correlation coefficients (R > 0.80) were obtained based on 46 hyperspectral indices and the BW severity results from Experiment 1. By testing the above vegetation indices at the leaf level and in UAV images using different methods and the results from Experiment 2, it was found that four of the developed indices (BWI1, BWI3, BWI4, and BWI6) performed appropriately (P < 0.01, M > 1.0), as they could distinguish between healthy and BW infected peanut plants, even if the plant presented minimal external symptoms. Our findings confirmed the potential of hyperspectral remote sensing including leaf-level and UAV images for peanut BW detection at early disease stages and discrimination of different BW severity levels based on vegetation indices derived from leaf-level reflectance. Timely BW severity determination based on our results could provide farmers with useful information to control peanut BW disease. © 2020},
}

@CONFERENCE{Kinaneva2020133,
author={Kinaneva, D. and Hristov, G. and Georgiev, G. and Kyuchukov, P. and Zahariev, P.},
title={An artificial intelligence approach to real-time automatic smoke detection by unmanned aerial vehicles and forest observation systems},
journal={Proceedings of the International Conference on Biomedical Innovations and Applications, BIA 2020},
year={2020},
pages={133-138},
art_number={9244498},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85096785864&doi=10.1109%2fBIA50171.2020.9244498&partnerID=40&md5=aa41b33fe885f35d8808c9099b391eea},
abstract={Natural disaster events, like volcanic eruptions and earthquakes, usually cause serious havoc and result in property losses for millions of Euro and unfortunately sometimes in loss of human life. These events are very hard to predict and are out of human control. Much like them, wildfires can be devastating and can lead to significant destructions, but fortunately they can be detected, controlled and prevented from spreading. The evolution of the wildfire detection and prevention technologies is long. The traditional methods rely on human involvement and include the use of manned fire watchtowers and piloted fire observation aircrafts. These solutions are very effective, but they are also very costly and sometimes can be extremely dangerous. With the technological advancements in the different engineering areas, safer and cheaper solutions for early forest fire detection were slowly developed - fire detection satellites, fire and lightning detectors, wireless sensor networks, as well as static optical or thermal cameras. Nevertheless, all of these solutions have disadvantages, which calls for their constant improvement, as well as for the development of more advanced and reliable systems. In this paper we present our experience in the area of the systems for early forest fire and smoke detection. Following the introduction section, we analyse in details an artificial intelligence (AI) approach to real-time automatic smoke detection, which is suitable for use in camera-based static forest observation systems and unmanned aerial vehicles. The paper concludes with discussions on the capability of the presented approach and with directions for further work. © 2020 IEEE.},
}

@CONFERENCE{Kartashov202035,
author={Kartashov, V. and Oleynikov, V. and Koryttsev, I. and Sheiko, S. and Zubkov, O. and Babkin, S.},
title={Processing of Wide Band Acoustic Signals during Detection of Unmanned Aerial Vehicles},
journal={2020 IEEE Ukrainian Microwave Week, UkrMW 2020 - Proceedings},
year={2020},
pages={35-39},
art_number={9252626},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85097721877&doi=10.1109%2fUkrMW49653.2020.9252626&partnerID=40&md5=2dc417541d2192fb703ca3a626788b07},
abstract={The problem of space-time processing of the received acoustic signal of an unmanned aerial vehicle, which is performed according to the criterion of the maximum of the ratio of useful signal/interference at the output of the adaptive antenna array, is considered. Mathematical relations are given that determine the operation of the space-time filter of the acoustic signal broadband in the space-time sense. The effectiveness of the considered signal processing method is shown using the computer simulation method in the Matlab environment. © 2020 IEEE.},
}

@CONFERENCE{Ipek202074,
author={Ipek, B. and Akpinar, M.},
title={Application of deep learning based object detection on unmanned aerial vehicle},
journal={5th International Conference on Computer Science and Engineering, UBMK 2020},
year={2020},
pages={74-78},
art_number={9219462},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85095688016&doi=10.1109%2fUBMK50275.2020.9219462&partnerID=40&md5=6d9a0b56264340f2e23bd07d07adc0dd},
abstract={Object recognition can be seen in every field thanks to today's high computation power. It has become possible to extract information from the images with high accuracy in different areas such as human, animal, vehicle, traffic signs and MR images. In this study, plastic water bottle detection was applied by using Inception v2, MobileNet v2 and ResNet50 architectures to be used in the Scientific and Technological Research Council of Turkey (TUBITAK) International Unmanned Aerial Vehicle Competition. Cloud based training applied to locate very small objects from up to 5 meters high. In the present study, the Single Shot Detector (SSD) ResNet50 model yielded the best results for mAP@0.75 and final loss. It was also determined that SSD Inception v2 model gave better results than SSD MobileNet v2 model. When the processing times were considered, it was determined that models could not work at Raspberry Pi 3 Model B+ equipment at sufficient speed. However, these results have shown that the Jetson Nano card can be operated correctly on a drone. In the next stage of this study, the aim will be determining environmental pollution level by detecting objects such as plastic bags, bottles and fruits on the streets. © 2020 IEEE.},
}

@ARTICLE{Dang20201,
author={Dang, L.M. and Wang, H. and Li, Y. and Min, K. and Kwak, J.T. and Lee, O.N. and Park, H. and Moon, H.},
title={Fusarium wilt of radish detection using rgb and near infrared images from unmanned aerial vehicles},
journal={Remote Sensing},
year={2020},
volume={12},
number={17},
pages={1-21},
art_number={2863},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85095435688&doi=10.3390%2frs12172863&partnerID=40&md5=99ee8c165c19aa4cb7f273ec43a8a305},
abstract={The radish is a delicious, healthy vegetable and an important ingredient to many side dishes and main recipes. However, climate change, pollinator decline, and especially Fusarium wilt cause a significant reduction in the cultivation area and the quality of the radish yield. Previous studies on plant disease identification have relied heavily on extracting features manually from images, which is time-consuming and inefficient. In addition to Red-Green-Blue (RGB) images, the development of near-infrared (NIR) sensors has enabled a more effective way to monitor the diseases and evaluate plant health based on multispectral imagery. Thus, this study compares two distinct approaches in detecting radish wilt using RGB images and NIR images taken by unmanned aerial vehicles (UAV). The main research contributions include (1) a high-resolution RGB and NIR radish field dataset captured by drone from low to high altitudes, which can serve several research purposes; (2) implementation of a superpixel segmentation method to segment captured radish field images into separated segments; (3) a customized deep learning-based radish identification framework for the extracted segmented images, which achieved remarkable performance in terms of accuracy and robustness with the highest accuracy of 96%; (4) the proposal for a disease severity analysis that can detect different stages of the wilt disease; (5) showing that the approach based on NIR images is more straightforward and effective in detecting wilt disease than the learning approach based on the RGB dataset. © 2020 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@CONFERENCE{McGee2020883,
author={McGee, J. and Mathew, S.J. and Gonzalez, F.},
title={Unmanned Aerial Vehicle and Artificial Intelligence for Thermal Target Detection in Search and Rescue Applications},
journal={2020 International Conference on Unmanned Aircraft Systems, ICUAS 2020},
year={2020},
pages={883-891},
art_number={9213849},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85094952073&doi=10.1109%2fICUAS48674.2020.9213849&partnerID=40&md5=97b785aca828f50a768aadec2427c72f},
abstract={Abstract- Recent developments in unmanned aerial vehicles (UAV), artificial intelligence and miniaturized thermal imaging systems represent a new opportunity for search and rescue (SAR) experts to survey relatively large areas. The system presented in this paper includes thermal image acquisition, the video processing pipeline that performs object detection and classification of people in need of SAR in outdoor environments. The system is tested on thermal video data from ground based and test flight footage and is found to be able to detect all the target people located in the surveyed area. The training dataset is a combination of gathered data and internet sourced data. The initial data procurement utilised online academic thermal databases and also the simulation of the UAV mounted camera environment. Ground based data was collected at Kangaroo Point cliffs in Brisbane, Australia, giving an approximate elevation of 26m. Airborne datasets were collected at South Bribie Island in Queensland, Australia, at a range of heights and vegetation density. These datasets where collected at different times of the day, allowing for a range of contrast levels between background and intended target. Once all data was collected, individual frames where extracted from each image and augmentation and annotation was completed. The images were gaussian blurred, lightened and darkened, once all annotation were completed. A total of 2751 original images were annotated, with the augmented dataset comprising of 10380 images. The YOLOV3 algorithm was selected as the neural network (NN) to be used for this experiment throughout training and classification. The 'Experiencor' GitHub pipeline was also used throughout the entirety of this project for data output and analysis purposes. The algorithm training was implemented on the Queensland University of Technology (QUT) High Performance Computing (HPC) cluster. Two main models were trained using different hyperparameters for comparison purposes. The first model had a loss of 3.81, AP of 98.6 after ~88 hours of training, with model two having a loss of 4.73, AP of 97.7 after ~184 hours of training. The comparison shows the importance of the chosen parameters when training detection algorithms of this nature, as minor changes can be the difference between an efficiently trained model and an inefficient failed training attempt. The prediction testing was completed on the test data sets that were not included in the training of the two models. This was done to remove any bias from the system, although it is noted that due to the shared environments of two of the test sets with the training sets, a small amount of bias will exist. Predictions made on the two data sets sharing environmental conditions with the training data, showed good prediction results for both trained models, with very limited false positive and missed detections. The system is flexible in that the user can readily define the types of objects to classify and the object characteristics that should be considered during training. © 2020 IEEE.},
}

@ARTICLE{Izzuddin2020497,
author={Izzuddin, M.A. and Hamzah, A. and Nisfariza, M.N. and Idris, A.S.},
title={Analysis of multispectral imagery from unmanned aerial vehicle (UAV) using object-based image analysis for detection of ganoderma disease in oil palm},
journal={Journal of Oil Palm Research},
year={2020},
volume={32},
number={3},
pages={497-508},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85094566580&doi=10.21894%2fjopr.2020.0035&partnerID=40&md5=801289068d9933394d1b1413108635cb},
abstract={Ganoderma disease that affects oil palms has caused huge losses to the palm oil industry in Malaysia. To curb widespread infection and mitigate further losses, attempts have been made to detect infected oil palms automatically so that they can be treated or destroyed. The multispectral remote sensing technology can be employed to this effect efficiently. From the aerial images, infected oil palms can be detected and classified according to the Ganoderma Disease Severity Index (GDSI). In this study, object-based image analysis (OBIA) was performed to classify oil palms in a selected area into three classes namely; healthy (T0), moderately infected (T2) and severely infected (T3). It would be desirable if lightly infected oil palms could also be categorised as a class. However, it was extremely difficult to discriminate lightly infected oil palms from the healthy ones just by analysing the aerial images since symptoms of early infection were not evident in the fronds yet. Images of each individual band as well as those obtained by combining two, three or four bands of the available spectra were analysed. The OBIA was conducted using example-based feature extraction procedure and various OBIA settings were tested to achieve a number of classification results. The accuracies of the results are quantified by comparing the results with the ground truth data. The results suggest that the combination of Edge-based segmentation and merge algorithm using Full-Lambda Schedule (FLS), Support Vector Machine (SVM) classifier and three-band data of (G_R_NIR) scores the highest accuracy of (91.8%). When data of individual bands were tested using the same algorithm and classifier, they obtained moderate accuracies ranging from 65.5%-76.2%. However, when data of two, three and four bands were combined, better results with classification accuracies from 70%-90% were recorded. These results show that the OBIA can be used to analyse multispectral images of oil palms to detect moderate and severe infection of Ganoderma disease. Detection of early infection of Ganoderma is feasible if more advanced algorithms and classifiers can be used with multispectral and hyperspectral aerial images. © 2020 Lembaga Minyak Sawit Malaysia. All rights reserved.},
}

@ARTICLE{Yang2020,
author={Yang, B. and Qiu, Q. and Yang, F. and Guan, H.},
title={A Framework of Linear Sensor Networks with Unmanned Aerial Vehicle for Rainfall-Induced Landslides Detection},
journal={International Journal of Structural Stability and Dynamics},
year={2020},
volume={20},
number={10},
art_number={2042017},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85093360228&doi=10.1142%2fS0219455420420171&partnerID=40&md5=ed9454b52ca42cd75865fc82b7b1031f},
abstract={This paper proposes a real-time monitoring framework for a landslide susceptibility area based on wireless sensor network using multiple Unmanned Aerial Vehicles (UAVs). Many researchers have considered building a landslide susceptibility map to distinguish different levels of landslide susceptible zones. However, to prevent damage from landslides, it is more important for the disaster control center to identify the time and location of the landslide occurrence in those highly susceptible areas. Hence, a rain-triggered landslide monitoring system is proposed herein for local mountain areas. First, a wireless sensor network framework is constructed to inform the control center as immediately as possible when landslides occur. Second, multiple UAV sensors will be responsible for collecting the stereo images of the slope in highly sensitive zones on schedule. Based on the stereo images and the binocular model, in-depth information can be obtained. With the depth information and Speeded Up Robust Features (SURF) detection, the key point characteristic information is constructed as the input data for Support Vector Machine (SVM). An SVM algorithm is designed with Python program language and executed in real time. Using this algorithm, the real-time images collected by UAVs and the landslide warning information will be sent to the control center for further analysis. Finally, a field experiment is conducted to demonstrate the effectiveness of the proposed method. © 2020 World Scientific Publishing Company.},
}

@ARTICLE{Fernández2020,
author={Fernández, A. and Usamentiaga, R. and de Arquer, P. and Fernández, M.Á. and Fernández, D. and Carús, J.L. and Fernández, M.},
title={Robust detection, classification and localization of defects in large photovoltaic plants based on unmanned aerial vehicles and infrared thermography},
journal={Applied Sciences (Switzerland)},
year={2020},
volume={10},
number={17},
art_number={5948},
note={cited By 6},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85090221450&doi=10.3390%2fapp10175948&partnerID=40&md5=6634f6697a24314a8c414ad7925574e7},
abstract={The efficiency and profitability of photovoltaic (PV) plants are highly controlled by their operation and maintenance (O&M) procedures. Today, the effective diagnosis of any possible fault of PV plants remains a technical and economic challenge, especially when dealing with large-scale PV plants. Currently, PV plant monitoring is carried out by either electrical performance measurements or image processing. The first approach presents limited fault detection ability, it is costly and time-consuming, and it is incapable of fast identification of the physical location of the fault. In the second approach, Infrared Thermography (IRT) imaging has been used for the characterization of PV module failures, but their setup and processing are rather complex and an experienced technician is required. The use of Unmanned Aerial Vehicles (UAVs) for IRT imaging of PV plants for health status monitoring of PV modules has been identified as a cost-effective approach that offers 10-15 fold lower inspection times than conventional techniques. However, previous works have not performed a comprehensive approach in the context of automated UAV inspection using IRT. This work provides a fully automated approach for the: (a) detection, (b) classification, and (c) geopositioning of the thermal defects in the PV modules. The system has been tested on a real PV plant in Spain. The obtained results indicate that an autonomous solution can be implemented for a full characterization of the thermal defects. © 2020 by the authors.},
}

@CONFERENCE{Mayr2020765,
author={Mayr, A. and Bremer, M. and Rutzinger, M.},
title={3D Point Errors and Change Detection Accuracy of Unmanned Aerial Vehicle Laser Scanning Data},
journal={ISPRS Annals of the Photogrammetry, Remote Sensing and Spatial Information Sciences},
year={2020},
volume={5},
number={2},
pages={765-772},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85091072839&doi=10.5194%2fisprs-annals-V-2-2020-765-2020&partnerID=40&md5=5d14799764466d2317736e03af90c9f3},
abstract={Unmanned aerial vehicle laser scanning (ULS) has recently become available for operational mapping and monitoring (e.g. for forestry applications or erosion studies). It combines advantages of terrestrial and airborne laser scanning, but there is still little proof of ULS accuracy. For the detection and monitoring of small-magnitude surfaces changes with multitemporal point clouds, an estimate of the level of detection (LOD) is required. The LOD is a threshold applied on distance measurements to separate real surface change (e.g. due to erosion or deposition by geomorphic processes) from errors. This paper investigates key components of the error budget for two ULS point clouds acquired for erosion monitoring at a grassland site in the Alps. In addition to the registration error and effects of the local surface roughness, we assess the positional uncertainties of each point that result from laser footprint effects, which are a function of the scanning geometry (including range, incidence angle and beam divergence). By removing erroneous points with an increasingly stricter point error criterion, we illustrate that the positional point errors strongly affect the LOD and discuss how this type of error can be mitigated. Moreover, our experimental results with three different surface classes (<i>bare earth and rock, buildings and grassland</i>) show that the level of detection tends to be slightly better for areas with bare earth and rock than for grass-covered areas (due to their roughness). For all these surface types reliable distance measurements are possible with sub-decimetre levels of detection. © 2020 Copernicus GmbH. All rights reserved.},
}

@ARTICLE{Yang2020575,
author={Yang, X. and Smith, A.M. and Bourchier, R.S. and Hodge, K. and Ostrander, D.},
title={Flowering leafy spurge (Euphorbia esula) detection using unmanned aerial vehicle imagery in biological control sites: Impacts of flight height, flight time and detection method},
journal={Weed Technology},
year={2020},
volume={34},
number={4},
pages={575-588},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85091650747&doi=10.1017%2fwet.2020.8&partnerID=40&md5=8623296f51cf2ce73bc5af8feaa5d05a},
abstract={Leafy spurge, a noxious perennial weed, is a major threat to the prairie ecosystem in North America. Strategic planning to control leafy spurge requires monitoring its spatial distribution and spread. The ability to detect flowering leafy spurge at two biological control sites in southern Saskatchewan, Canada, was investigated using an unmanned aerial vehicle (UAV) system. Three flight missions were conducted on June 30, 2016, during the leafy spurge flowering period. Imagery was acquired at four flight heights and one or two acquisition times, depending on the site. The sites were reflown on June 28, 2017, to evaluate the change in flowering leafy spurge over time. Mixture tuned matched filtering (MTMF) and hue, intensity, and saturation (HIS) threshold analyses were used to determine flowering leafy spurge cover. Flight height of 30 m was optimal; the strongest relationships between UAV and ground estimates of leafy spurge cover (r= 0.76 to 0.90; normalized root mean square error [NRMSE] = 0.10 to 0.13) and stem density (r= 0.72 to 0.75) were observed. Detection was not significantly affected by the image analysis method (P > 0.05). Flowering leafy spurge cover estimates were similar using HIS (1.9% to 14.8%) and MTMF (2.1% to 10.3%) and agreed with the ground estimates (using HIS: r= 0.64 to 0.93, NRMSE = 0.08 to 0.25; using MTMF: r= 0.64 to 0.90, NRMSE = 0.10 to 0.27). The reduction in flowering leafy spurge cover between 2016 and 2017 detected using UAV images and HIS (8.1% at site 1 and 2.7% at site 2) was consistent with that based on ground digital photographs (10% at site 1 and 1.8% at site 2). UAV imagery is a useful tool for accurately detecting flowering leafy spurge and could be used for routine monitoring purposes in a biological control program. © 2020 Cambridge University Press. All rights reserved.},
}

@ARTICLE{Kaye2020890,
author={Kaye, T.G. and Pittman, M.},
title={Fluorescence-based detection of field targets using an autonomous unmanned aerial vehicle system},
journal={Methods in Ecology and Evolution},
year={2020},
volume={11},
number={8},
pages={890-898},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85087312968&doi=10.1111%2f2041-210X.13402&partnerID=40&md5=69f9327f64fc78e5d1a221682bea287d},
abstract={Here we describe a proof-of-concept autonomous unmanned aerial vehicle (UAV) system that utilizes the fluorescence characteristics unique to different materials to scan and acquire targets in the field that includes fossils, rocks and minerals, organisms and archaeological artefacts. This is possible because these targets are often highly fluorescent against lower fluorescence backgrounds and may exhibit different colours. To detect these targets from a moving UAV, we utilize laser-stimulated fluorescence. This involves an intense laser beam that—unlike regular UV light—can project greater distances and generate sufficient fluorescence for targets to be detected on the UAV camera many metres above the ground. The system involves a lightweight UAV programmed to fly a waypoint pattern autonomously at night over the area of interest. LIDAR maintains its height above the terrain. A near-UV laser is projected across the ground as a horizontal line directly below the UAV. Co-mounted with the laser is a small highly sensitive video camera stabilized on a motion-controlled gimbal that records the laser line during the flight. An intermittent, powerful white light strobe flashes during the flight to record the UAV's ground position in the scanned area. The UAV returns with the laser video at the end of each autonomous mission. This video is post-processed, extracting the laser line data into a long continuous scan image showing the fluorescing ground targets. Initial analysis determines what colour the targets fluoresce so that a specific colour range can be extracted from the image to identify the locations of the detected targets. The white light strobe images are then used to quickly follow-up on the detections. This system holds the promise of becoming the lowest ‘ground truth’ layer in the mix of high-altitude map data produced by satellite- and airplane-based Geographic Information Systems. With centimetre resolution and the geochemical differences shown via fluorescence, this system will increase the scale and efficiency of data collection involving fossils, rocks and minerals including mineable materials, fluorescent organisms including biogenic mineral producers like shellfish as well as archaeological artefacts. Thus, the fields of evolution, ecology, Earth and planetary science, archaeology and other subjects involving fluorescent targets would all benefit from this new system. © 2020 The Authors. Methods in Ecology and Evolution published by John Wiley & Sons Ltd on behalf of British Ecological Society},
}

@ARTICLE{Zhang2020555,
author={Zhang, J. and Liang, X. and Wang, M. and Yang, L. and Zhuo, L.},
title={Coarse-to-fine object detection in unmanned aerial vehicle imagery using lightweight convolutional neural network and deep motion saliency},
journal={Neurocomputing},
year={2020},
volume={398},
pages={555-565},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85085863614&doi=10.1016%2fj.neucom.2019.03.102&partnerID=40&md5=63e9a267ea9b42059533908175d6eb20},
abstract={Unmanned aerial vehicles (UAVs) have been widely applied to various fields, facing mass imagery data, object detection in UAV imagery is under extensive research for its significant status in both theoretical study and practical applications. In order to achieve the accurate object detection in UAV imagery on the premise of real-time processing, a coarse-to-fine object detection method for UAV imagery using lightweight convolutional neural network (CNN) and deep motion saliency is proposed in this paper. The proposed method includes three steps: (1) Key frame extraction using image similarity measurement is performed on the UAV imagery to accelerate the successive object detection procedure; (2) Deep features are extracted by PeleeNet, a lightweight CNN, to achieve the coarse object detection on the key frames; (3) LiteFlowNet and objects prior knowledge is utilized to analyze the deep motion saliency map, which further helps to refine the detection results. The detection results on key frames propagate to the temporally nearest non-key frames to achieve the fine detection. Five experiments are conducted to verify the effectiveness of the proposed method on Stanford drone dataset (SDD). The experimental results demonstrate that the proposed method can achieve comparable detection speed but superior accuracy to six state-of-the-art methods. © 2019 Elsevier B.V.},
}

@ARTICLE{Ponte20201,
author={Ponte, S. and Ariante, G. and Papa, U. and Core, G.D.},
title={An embedded platform for positioning and obstacle detection for small unmanned aerial vehicles},
journal={Electronics (Switzerland)},
year={2020},
volume={9},
number={7},
pages={1-18},
art_number={1175},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85088250983&doi=10.3390%2felectronics9071175&partnerID=40&md5=a824b3d8caa3fb63cb82b91ea5d0cb7e},
abstract={Unmanned Aerial Vehicles (UAV) with on-board augmentation systems (UAS, Unmanned Aircraft System) have penetrated into civil and general-purpose applications, due to advances in battery technology, control components, avionics and rapidly falling prices. This paper describes the conceptual design and the validation campaigns performed for an embedded precision Positioning, field mapping, Obstacle Detection and Avoiding (PODA) platform, which uses commercial-off-the-shelf sensors, i.e., a 10-Degrees-of-Freedom Inertial Measurement Unit (10-DoF IMU) and a Light Detection and Ranging (LiDAR), managed by an Arduino Mega 2560 microcontroller with Wi-Fi capabilities. The PODA system, designed and tested for a commercial small quadcopter (Parrot Drones SAS Ar.Drone 2.0, Paris, France), estimates position, attitude and distance of the rotorcraft from an obstacle or a landing area, sending data to a PC-based ground station. The main design issues are presented, such as the necessary corrections of the IMU data (i.e., biases and measurement noise), and Kalman filtering techniques for attitude estimation, data fusion and position estimation from accelerometer data. The real-time multiple-sensor optimal state estimation algorithm, developed for the PODA platform and implemented on the Arduino, has been tested in typical aerospace application scenarios, such as General Visual Inspection (GVI), automatic landing and obstacle detection. Experimental results and simulations of various missions show the effectiveness of the approach. © 2020 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@CONFERENCE{Titouna2020469,
author={Titouna, C. and Nait-Abdesselam, F. and Moungla, H.},
title={An Online Anomaly Detection Approach for Unmanned Aerial Vehicles},
journal={2020 International Wireless Communications and Mobile Computing, IWCMC 2020},
year={2020},
pages={469-474},
art_number={9148073},
note={cited By 6},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85089654324&doi=10.1109%2fIWCMC48107.2020.9148073&partnerID=40&md5=075a32d3d5f540b3d2c25a6754c3f273},
abstract={A non-predicted and transient malfunctioning of one or multiple unmanned aerial vehicles (UAVs) is something that may happen over a course of their deployment. Therefore, it is very important to have means to detect these events and take actions for ensuring a high level of reliability, security, and safety of the flight for the predefined mission. In this research, we propose algorithms aiming at the detection and isolation of any faulty UAV so that the performance of the UAVs application is kept at its highest level. To this end, we propose the use of Kullback-Leiler Divergence (KLD) and Artificial Neural Network (ANN) to build algorithms that detect and isolate any faulty UAV. The proposed methods are declined in these two directions: (1) we compute a difference between the internal and external data, use KLD to compute dissimilarities, and detect the UAV that transmits erroneous measurements. (2) Then, we identify the faulty UAV using an ANN model to classify the sensed data using the internal sensed data. The proposed approaches are validated using a real dataset, provided by the Air Lab Failure and Anomaly (ALFA) for UAV fault detection research, and show promising performance. © 2020 IEEE.},
}

@ARTICLE{Syrotenko20202798,
author={Syrotenko, A. and Shchypanskyi, P. and Savchenko, V. and Krashchenko, D. and Yerhidzei, K. and Havryliuk, I.},
title={Evaluation of quality of hidden transmitters detection by a group of coordinated unmanned aerial vehicles on the basis of entropy decrease dynamics},
journal={International Journal of Emerging Trends in Engineering Research},
year={2020},
volume={8},
number={6},
pages={2798-2804},
art_number={93},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85087386465&doi=10.30534%2fijeter%2f2020%2f93862020&partnerID=40&md5=4ff831328583473fd771af5c1dd9ccc4},
}

@ARTICLE{Liang20201758,
author={Liang, X. and Zhang, J. and Zhuo, L. and Li, Y. and Tian, Q.},
title={Small Object Detection in Unmanned Aerial Vehicle Images Using Feature Fusion and Scaling-Based Single Shot Detector with Spatial Context Analysis},
journal={IEEE Transactions on Circuits and Systems for Video Technology},
year={2020},
volume={30},
number={6},
pages={1758-1770},
art_number={8672115},
note={cited By 20},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85086308643&doi=10.1109%2fTCSVT.2019.2905881&partnerID=40&md5=7f317ad8395a69d1f48b2494d085f68d},
abstract={Objects in unmanned aerial vehicle (UAV) images are generally small due to the high-photography altitude. Although many efforts have been made in object detection, how to accurately and quickly detect small objects is still one of the remaining open challenges. In this paper, we propose a feature fusion and scaling-based single shot detector (FS-SSD) for small object detection in the UAV images. The FS-SSD is an enhancement based on FSSD, a variety of the original single shot multibox detector (SSD). We add an extra scaling branch of the deconvolution module with an average pooling operation to form a feature pyramid. The original feature fusion branch is adjusted to be better suited to the small object detection task. The two feature pyramids generated by the deconvolution module and feature fusion module are utilized to make predictions together. In addition to the deep features learned by the FS-SSD, to further improve the detection accuracy, spatial context analysis is proposed to incorporate the object spatial relationships into object redetection. The interclass and intraclass distances between different object instances are computed as a spatial context, which proves effective for multiclass small object detection. Six experiments are conducted on the PASCAL VOC dataset and the two UAV image datasets. The experimental results demonstrate that the proposed method can achieve a comparable detection speed but an accuracy superior to those of the six state-of-the-art methods. © 1991-2012 IEEE.},
}

@ARTICLE{Xiong2020261,
author={Xiong, J. and Liu, Z. and Chen, S. and Liu, B. and Zheng, Z. and Zhong, Z. and Yang, Z. and Peng, H.},
title={Visual detection of green mangoes by an unmanned aerial vehicle in orchards based on a deep learning method},
journal={Biosystems Engineering},
year={2020},
volume={194},
pages={261-272},
note={cited By 12},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85084043112&doi=10.1016%2fj.biosystemseng.2020.04.006&partnerID=40&md5=228f4a605dae998f71cc90e2363944eb},
abstract={In this paper, a visual detection method by a UAV (unmanned aerial vehicle) was proposed to detect green mangoes on the surface of the tree crown rapidly and meet the need of estimating the number of mango fruits in orchards. The YOLOv2 model was used for quick detection of mango images captured by a UAV. First, mango images were collected by a UAV. These images were marked manually and used to build a training set and a test set. The parameters of the model were determined by experiments. The resolution of the images was 544 × 544 pixels. The batch size was 64, and the initial learning rate was 0.01. The mAP (mean average precision) of the trained model on the training set was 86.4%. Good detection results were achieved on images containing different fruit numbers and different lighting conditions with a precision of 96.1% and a recall rate of 89.0%. Finally, an experiment was conducted to estimate the actual number of green mango fruits. A method of generating an image of the whole mango tree was designed. The fruit numbers estimation model for green mango was obtained by linear fitting between the actual number and the detected number of mangoes. From the comparison of the fruit numbers of 10 mango trees determined by manual calculation and model prediction, an estimation error rate of 1.1% was achieved. The result demonstrated that the algorithm was effective for green mango detection and provided a methodological reference for quick estimation of the number of green mango fruits in orchards. © 2020 IAgrE},
}

@CONFERENCE{Sadhu20205255,
author={Sadhu, V. and Zonouz, S. and Pompili, D.},
title={On-board Deep-learning-based Unmanned Aerial Vehicle Fault Cause Detection and Identification},
journal={Proceedings - IEEE International Conference on Robotics and Automation},
year={2020},
pages={5255-5261},
art_number={9197071},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85092743339&doi=10.1109%2fICRA40945.2020.9197071&partnerID=40&md5=8017925cf1e437e6c7a7ea0acbda6bb2},
abstract={With the increase in use of Unmanned Aerial Vehicles (UAVs)/drones, it is important to detect and identify causes of failure in real time for proper recovery from a potential crash-like scenario or post incident forensics analysis. The cause of crash could be either a fault in the sensor/actuator system, a physical damage/attack, or a cyber attack on the drone's software. In this paper, we propose novel architectures based on deep Convolutional and Long Short-Term Memory Neural Networks (CNNs and LSTMs) to detect (via Autoencoder) and classify drone mis-operations based on real-time sensor data. The proposed architectures are able to learn high-level features automatically from the raw sensor data and learn the spatial and temporal dynamics in the sensor data. We validate the proposed deep-learning architectures via simulations and realworld experiments on a drone. Empirical results show that our solution is able to detect (with over 90% accuracy) and classify various types of drone mis-operations (with about 99% accuracy (simulation data) and upto 85% accuracy (experimental data)). © 2020 IEEE.},
}

@ARTICLE{Yi2020,
author={Yi, W. and Jing, Z. and Shuang, G.},
title={Hue–saturation–intensity and texture feature-based cloud detection algorithm for unmanned aerial vehicle images},
journal={International Journal of Advanced Robotic Systems},
year={2020},
volume={17},
number={3},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85086067552&doi=10.1177%2f1729881420903532&partnerID=40&md5=30f6a227522ba563ae2583380864da03},
abstract={There are a large number of cloud-covered areas in most unmanned aerial vehicle images and lead to the loss of information in the image and affect image post procession such as image fusion and target identification. Finding the cloud-occluded area in an image is a key step in image processing. Based on the differences of color and texture characteristics between cloud and ground, a cloud detection algorithm for the unmanned aerial vehicle images is proposed. Simulation results show that the proposed algorithm is better than the classical cloud detection algorithms in accuracy rate, false-positive rate, and kappa coefficient. © The Author(s) 2020.},
}

@ARTICLE{Yu20201141,
author={Yu, H. and Li, G. and Zhang, W. and Huang, Q. and Du, D. and Tian, Q. and Sebe, N.},
title={The Unmanned Aerial Vehicle Benchmark: Object Detection, Tracking and Baseline},
journal={International Journal of Computer Vision},
year={2020},
volume={128},
number={5},
pages={1141-1159},
note={cited By 31},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85076021121&doi=10.1007%2fs11263-019-01266-1&partnerID=40&md5=a866176966771af53bd08128f85a76a6},
abstract={With the increasing popularity of Unmanned Aerial Vehicles (UAVs) in computer vision-related applications, intelligent UAV video analysis has recently attracted the attention of an increasing number of researchers. To facilitate research in the UAV field, this paper presents a UAV dataset with 100 videos featuring approximately 2700 vehicles recorded under unconstrained conditions and 840k manually annotated bounding boxes. These UAV videos were recorded in complex real-world scenarios and pose significant new challenges, such as complex scenes, high density, small objects, and large camera motion, to the existing object detection and tracking methods. These challenges have encouraged us to define a benchmark for three fundamental computer vision tasks, namely, object detection, single object tracking (SOT) and multiple object tracking (MOT), on our UAV dataset. Specifically, our UAV benchmark facilitates evaluation and detailed analysis of state-of-the-art detection and tracking methods on the proposed UAV dataset. Furthermore, we propose a novel approach based on the so-called Context-aware Multi-task Siamese Network (CMSN) model that explores new cues in UAV videos by judging the consistency degree between objects and contexts and that can be used for SOT and MOT. The experimental results demonstrate that our model could make tracking results more robust in both SOT and MOT, showing that the current tracking and detection methods have limitations in dealing with the proposed UAV benchmark and that further research is indeed needed. © 2019, Springer Science+Business Media, LLC, part of Springer Nature.},
}

@ARTICLE{Marston2020779,
author={Marston, Z.P.D. and Cira, T.M. and Hodgson, E.W. and Knight, J.F. and MacRae, I.V. and Koch, R.L. and Rondon, S.},
title={Detection of Stress Induced by Soybean Aphid (Hemiptera: Aphididae) Using Multispectral Imagery from Unmanned Aerial Vehicles},
journal={Journal of Economic Entomology},
year={2020},
volume={113},
number={2},
pages={779-786},
note={cited By 9},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85084408370&doi=10.1093%2fjee%2ftoz306&partnerID=40&md5=ef13a1afb7629df70d8b71056a3cfd73},
abstract={Soybean aphid, Aphis glycines Matsumura (Hemiptera: Aphididae), is a common pest of soybean, Glycine max (L.) Merrill (Fabales: Fabaceae), in North America requiring frequent scouting as part of an integrated pest management plan. Current scouting methods are time consuming and provide incomplete coverage of soybean. Unmanned aerial vehicles (UAVs) are capable of collecting high-resolution imagery that offer more detailed coverage in agricultural fields than traditional scouting methods. Recently, it was documented that changes to the spectral reflectance of soybean canopies caused by aphid-induced stress could be detected from ground-based sensors; however, it remained unknown whether these changes could also be detected from UAV-based sensors. Small-plot trials were conducted in 2017 and 2018 where cages were used to manipulate aphid populations. Additional open-field trials were conducted in 2018 where insecticides were used to create a gradient of aphid pressure. Whole-plant soybean aphid densities were recorded along with UAV-based multispectral imagery. Simple linear regressions were used to determine whether UAV-based multispectral reflectance was associated with aphid populations. Our findings indicate that near-infrared reflectance decreased with increasing soybean aphid populations in caged trials when cumulative aphid days surpassed the economic injury level, and in open-field trials when soybean aphid populations were above the economic threshold. These findings provide the first documentation of soybean aphid-induced stress being detected from UAV-based multispectral imagery and advance the use of UAVs for remote scouting of soybean aphid and other field crop pests. © 2019 The Author(s) 2019. Published by Oxford University Press on behalf of Entomological Society of America. All rights reserved.},
}

@ARTICLE{Liu2020,
author={Liu, M. and Wang, X. and Zhou, A. and Fu, X. and Ma, Y. and Piao, C.},
title={Uav-yolo: Small object detection on unmanned aerial vehicle perspective},
journal={Sensors (Switzerland)},
year={2020},
volume={20},
number={8},
art_number={2238},
note={cited By 34},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85083426750&doi=10.3390%2fs20082238&partnerID=40&md5=c6ad292cfb69aff68efea62a189929c2},
abstract={Object detection, as a fundamental task in computer vision, has been developed enormously, but is still challenging work, especially for Unmanned Aerial Vehicle (UAV) perspective due to small scale of the target. In this study, the authors develop a special detection method for small objects in UAV perspective. Based on YOLOv3, the Resblock in darknet is first optimized by concatenating two ResNet units that have the same width and height. Then, the entire darknet structure is improved by increasing convolution operation at an early layer to enrich spatial information. Both these two optimizations can enlarge the receptive filed. Furthermore, UAV-viewed dataset is collected to UAV perspective or small object detection. An optimized training method is also proposed based on collected UAV-viewed dataset. The experimental results on public dataset and our collected UAV-viewed dataset show distinct performance improvement on small object detection with keeping the same level performance on normal dataset, which means our proposed method adapts to different kinds of conditions. © 2020 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@ARTICLE{Sun2020,
author={Sun, Y. and Li, H. and Sun, L.},
title={Window detection employing a global regularity level set from oblique unmanned aerial vehicle images and point clouds},
journal={Journal of Applied Remote Sensing},
year={2020},
volume={14},
number={2},
art_number={024513},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85088519275&doi=10.1117%2f1.JRS.14.024513&partnerID=40&md5=60af7a68af077fcbdd0f47e30bd06fce},
abstract={Detailed building façade structures are significant parts of three-dimensional building models. A photogrammetric point cloud, generated from oblique unmanned aerial system imagery, is a type of data applied in building reconstruction. Its positive characteristics, alongside its challenging qualities, have provoked discussions related to our study. To obtain highly accurate window detection results, we propose a regular window detection method using a global regularity level set. Our method first detects the window boundaries from point clouds using a hole-based boundary extraction method. The minimum bounding rectangle of each boundary point cloud is then used specifically to represent the window. Next, façade partitioning is applied to subdivide the rectified façade images into a series of slices followed by cells. Each cell contains only one window rectangle after the processing. Finally, a global regularity level set algorithm is developed to optimize rectangular windows in horizontal and vertical slices using façade images. The proposed method was validated through a comparison with the slicing method on data from two façades. The accuracy of the window sizes in height and width was also discussed. The experiment results indicate that our method can obtain regular window locations and shapes from photogrammetric point clouds. © 2020 Society of Photo-Optical Instrumentation Engineers (SPIE).},
}

@ARTICLE{He2020,
author={He, K. and Hong, H. and Jiang, G. and Gu, H.},
title={Analysis of assembly error effect on stability accuracy of unmanned aerial vehicle photoelectric detection system},
journal={Applied Sciences (Switzerland)},
year={2020},
volume={10},
number={7},
art_number={2311},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85083579048&doi=10.3390%2fapp10072311&partnerID=40&md5=54bf711f6f43c3633c65907a3b00145f},
abstract={A photoelectric detection system is a typical type of device widely used for detecting purposes based on unmanned aerial vehicles (UAV). Stability accuracy is the key performance index. Compared to traditional analysis methods aimed at unpredictable error-causing sources, assembly errors can be easily controlled during the manufacturing processes. In this research, an analysis method of assembly error effect on stability accuracy is proposed. First, by using kinematics analysis of homogeneous coordinate transformation, stability accuracy is comprehensively modeled and simulated. Then, by analyzing the manufacturing process, assembly errors of axis perpendicularities, run-outs and gyroscopes are defined and modeled. By simulating different carrier movements, the effects caused by assembly errors under various environments are studied. Finally, error sensitivity is proposed by using standard deviation analysis. Results show that the most sensitive assembly errors are identified, and ranked in order of sensitivity as follows: x-component of pitch axis perpendicularity, y-component of the azimuth gyroscope assembly, and z-component of the pitch gyroscope assembly. In conclusion, the results can be used as standards of manufacturing process improvements, and the proposed methods can be used to provide valuable references for real application scenarios. © 2020 by the authors.},
}

@CONFERENCE{Xie2020,
author={Xie, X. and Wei, X. and Wang, X. and Guo, X. and Li, J. and Cheng, Z.},
title={Photovoltaic panel anomaly detection system based on Unmanned Aerial Vehicle platform},
journal={IOP Conference Series: Materials Science and Engineering},
year={2020},
volume={768},
number={7},
art_number={072061},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85083005204&doi=10.1088%2f1757-899X%2f768%2f7%2f072061&partnerID=40&md5=4dd0e5ee00c6299566cee100b1c40f3d},
abstract={The emergence and rapid development of the Unmanned Aerial Vehicle (UAV) Photovoltaic inspection system have become an effective means of solving the operation and maintenance of photovoltaic power plants. In order to cooperate with the current UAV platform for photovoltaic panel anomaly detection, this paper proposes a photovoltaic infrared target anomaly detection system. In this paper, the Sobel operator is used to extract the photovoltaic slab area of the image, and the canny operator is used to obtain the photovoltaic small plate area to realize the complementary advantages. At the same time, the deep learning is applied to the algorithm to learn the discriminative characteristics of the image, and the brightness statistics are used. The method is supplemented by the method to achieve anomaly detection of the photovoltaic panel area. The effectiveness of the proposed algorithm is proved by a large number of experiments. © Published under licence by IOP Publishing Ltd.},
}

@CONFERENCE{Fakhrulddin2020,
author={Fakhrulddin, S.S. and Gharghan, S.K.},
title={An Elderly First Aid System Based-Fall Detection and Unmanned Aerial Vehicle},
journal={IOP Conference Series: Materials Science and Engineering},
year={2020},
volume={745},
number={1},
art_number={012096},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85082933527&doi=10.1088%2f1757-899X%2f745%2f1%2f012096&partnerID=40&md5=f93f9efeb00f4632c4cac1f495ad27e4},
abstract={A first-aid system is proposed for monitoring elderly patients who risk falling based on fall detection system (FDs) and for providing the first aid kit from an emergency call centre (ECC) to them by using an unmanned aerial vehicle (UAV). In previous studies, the measurement accuracy of falls and heart rate was not sufficiently accurate. In addition, determination of UAV delivery time is also crucial and can save lives. In this work, the proposed system aims to determine patient falls and accurately measure heart rate and reduce UAV delivery time to patients. The FDs was practically implemented based on heartbeat and accelerometer sensors, a microcontroller, a GSM module, and GPS. While, a UAV, a first aid kit, and Smartphone were adopted in an ECC. Falls were accurately detected based on elderly fall detection (EFD) algorithm. The result showed that the proposed FDs was succeeded in monitoring elderly patients' vital signs with a fall detection accuracy of 99.11%. In addition, the UAV succeeded in all missions and arrived at the patient's locations before the ambulance in urban areas, with an average time saving of 1.75 min. The proposed elderly first aid system outperformed previous systems presented in terms of fall detection and UAV arrival time. © 2020 IOP Publishing Ltd.},
}

@ARTICLE{Ponce-Corona202082,
author={Ponce-Corona, E. and Guadalupe Sánchez, M. and Fajardo-Delgado, D. and Acevedo-Juárez, B. and De-La-Torre, M. and Avila-George, H. and Castro, W.},
title={A systematic review of the literature focused on the use of unmanned aerial vehicles during the vegetation detection process [Una revisión sistemática de la literatura enfocada al uso de vehículos aéreos no tripulados durante el proceso de detección de vegetación]},
journal={RISTI - Revista Iberica de Sistemas e Tecnologias de Informacao},
year={2020},
volume={2020},
number={36},
pages={82-101},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85085320941&doi=10.17013%2fristi.36.82-101&partnerID=40&md5=29c27be7c736f5ab03300bb1bac0cac4},
abstract={In recent years, the use of unmanned aerial vehicles has become popular in the development of agricultural and forestry applications. Due to the importance of plants in both rural and urban environments, the extraction of information from remote sensing data is a relevant research area; such information is fundamental for urban and rural planning, establishing sustainable ecological niches, estimating crop yields, conducting forest inventories, monitoring agricultural management systems and some other agricultural applications. In this article, a systematic review of the literature concerning the use of unmanned aerial vehicles in applications related to vegetation detection and plant inventory is presented. Likewise, an analysis of the main computational and statistical techniques used for processing unmanned aerial vehicles images is also made. © 2020, Associacao Iberica de Sistemas e Tecnologias de Informacao. All rights reserved.},
}

@ARTICLE{Nguyen2020,
author={Nguyen, T.L. and Han, D.Y.},
title={Detection of road surface changes from multi-temporal unmanned aerial vehicle images using a convolutional siamese network},
journal={Sustainability (Switzerland)},
year={2020},
volume={12},
number={6},
art_number={2482},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85082876471&doi=10.3390%2fsu12062482&partnerID=40&md5=52e30fdf99e8bd137d4ed0e4ddd8def2},
abstract={Road quality commonly decreases due to aging and deterioration of road surfaces. As the number of roads that need to be surveyed increases, general maintenance-particularly surveillance-can be quite costly if carried out using traditional methods. Therefore, using unmanned aerial vehicles (UAVs) and deep learning to detect changes via surveys is a promising strategy. This study proposes a method for detecting changes on road surfaces using pairs of UAV images captured at different times. First, a convolutional Siamese network is introduced to extract the features of an image pair and a Euclidean distance function is applied to calculate the distance between two features. Then, a contrastive loss function is used to enlarge the distance between changed feature pairs and reduce the distance between unchanged feature pairs. Finally, the initial change map is improved based on the preliminary differences between the two input images. Our experimental results confirm the effectiveness of this approach. © 2020 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@ARTICLE{Tanut2020,
author={Tanut, B. and Riyamongkol, P.},
title={The development of a defect detection model from the high-resolution images of a sugarcane plantation using an unmanned aerial vehicle},
journal={Information (Switzerland)},
year={2020},
volume={11},
number={3},
art_number={136},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85082444699&doi=10.3390%2finfo11030136&partnerID=40&md5=ba05953d2af0478b673f76cc1c7cf3b0},
abstract={This article presents a defect detection model of sugarcane plantation images. The objective is to assess the defect areas occurring in the sugarcane plantation before the harvesting seasons. The defect areas in the sugarcane are usually caused by storms and weeds. This defect detection algorithm uses high-resolution sugarcane plantations and image processing techniques. The algorithm for defect detection consists of four processes: (1) data collection, (2) image preprocessing, (3) defect detection model creation, and (4) application program creation. For feature extraction, the researchers used image segmentation and convolution filtering by 13 masks together with mean and standard deviation. The feature extraction methods generated 26 features. The K-nearest neighbors algorithm was selected to develop a model for the classification of the sugarcane areas. The color selection method was also chosen to detect defect areas. The results show that the model can recognize and classify the characteristics of the objects in sugarcane plantation images with an accuracy of 96.75%. After the comparison with the expert surveyor's assessment, the accurate relevance obtained was 92.95%. Therefore, the proposed model can be used as a tool to calculate the percentage of defect areas and solve the problem of evaluating errors of yields in the future. © 2020 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@ARTICLE{Picos2020,
author={Picos, J. and Bastos, G. and Míguez, D. and Alonso, L. and Armesto, J.},
title={Individual tree detection in a eucalyptus plantation using unmanned aerial vehicle (UAV)-LiDAR},
journal={Remote Sensing},
year={2020},
volume={12},
number={5},
art_number={885},
note={cited By 22},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85081894763&doi=10.3390%2frs12050885&partnerID=40&md5=f394609faa9e06bf8f53eeb9b34f8371},
abstract={The present study addresses the tree counting of a Eucalyptus plantation, the most widely planted hardwood in the world. Unmanned aerial vehicle (UAV) light detection and ranging (LiDAR) was used for the estimation of Eucalyptus trees. LiDAR-based estimation of Eucalyptus is a challenge due to the irregular shape and multiple trunks. To overcome this difficulty, the layer of the point cloud containing the stems was automatically classified and extracted according to the height thresholds, and those points were horizontally projected. Two different procedures were applied on these points. One is based on creating a buffer around each single point and combining the overlapping resulting polygons. The other one consists of a two-dimensional raster calculated from a kernel density estimation with an axis-aligned bivariate quartic kernel. Results were assessed against the manual interpretation of the LiDAR point cloud. Both methods yielded a detection rate (DR) of 103.7% and 113.6%, respectively. Results of the application of the local maxima filter to the canopy height model (CHM) intensely depends on the algorithm and the CHM pixel size. Additionally, the height of each tree was calculated from the CHM. Estimates of tree height produced from the CHM was sensitive to spatial resolution. A resolution of 2.0 m produced a R2 and a root mean square error (RMSE) of 0.99 m and 0.34 m, respectively. A finer resolution of 0.5 m produced a more accurate height estimation, with a R2 and a RMSE of 0.99 and 0.44 m, respectively. The quality of the results is a step toward precision forestry in eucalypt plantations. © 2020 by the author. Licensee MDPI, Basel, Switzerland.},
}

@ARTICLE{Silva2020531,
author={Silva, A. and Mendonça, R. and Santana, P.},
title={Monocular Trail Detection and Tracking Aided by Visual SLAM for Small Unmanned Aerial Vehicles},
journal={Journal of Intelligent and Robotic Systems: Theory and Applications},
year={2020},
volume={97},
number={3-4},
pages={531-551},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85066022268&doi=10.1007%2fs10846-019-01033-x&partnerID=40&md5=cd52a495f6df04af3ef17a937216e095},
abstract={This article addresses the navigation problem of small and medium-sized unmanned aerial vehicles (UAVs) built to perform missions in forest environments (e.g., search and rescue) by exploiting the presence of natural or man-made paths, typically present in this type of environments. The proposed system extends a previous monocular-based technique for trail detection and tracking so as to take into account volumetric data acquired from a Visual SLAM algorithm and, as a result, to increase its sturdiness upon challenging trails. The experimental results, obtained via a set of 12 videos recorded with a camera installed in a tele-operated, unmanned small-sized aerial vehicle, show the ability of the proposed system to overcome some of the difficulties of the original detector, attaining a success rate of 97.8%. © 2019, Springer Nature B.V.},
}

@CONFERENCE{Kovbasiuk2020267,
author={Kovbasiuk, S. and Kanevskyy, L. and Chernyshuk, S. and Romanchuk, M.},
title={Detection of vehicles on images obtained from unmanned aerial vehicles using instance segmentation},
journal={Proceedings - 15th International Conference on Advanced Trends in Radioelectronics, Telecommunications and Computer Engineering, TCSET 2020},
year={2020},
pages={267-271},
art_number={9088601},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85086305339&doi=10.1109%2fTCSET49122.2020.235437&partnerID=40&md5=cc9578c46ab16e1e7a91db2b62dabd1a},
abstract={In recent years, developing and improving of methods for automatic processing of imagery pictures taken from air with unmanned aerial vehicles (UAV) for ground vehicles detection have received priority. One of the most perspective approach in this direction is application of neural networks. However, UAV imagery has some distinctive features compared to normal images namely high resolution, complex image background, unequal distribution by size and quantity of training data, image bending due to flight-performance changes caused by air environment conditions. These factors compromise and make much more complicated detection of fine-graded objects by standard models of neural networks and in some cases renders automated processing of such images impossible. For the purpose of automatic detection of vehicles in images taken from UAV the analysis of existing methods of automated images processing and models of neural networks as the basis for these methods was conducted. The results of analysis allowed to highlight a multistage pipeline of aerial image, that combines approaches to detection, instance and semantic segmentation. The model of segmentation cascade was improved through considering objects geometrical dimensions and their ratio as well as scale changing and survey conditions. Application of suggested model of segmentation cascade for automated vehicle detection on aerial images allows to increase the accuracy of localization and detection of such objects. © 2020 IEEE.},
}

@CONFERENCE{Kartashov2020377,
author={Kartashov, V. and Oleynikov, V. and Koryttsev, I. and Sheiko, S. and Zubkov, O. and Babkin, S. and Selieznov, I.},
title={Use of Acoustic Signature for Detection, Recognition and Direction Finding of Small Unmanned Aerial Vehicles},
journal={Proceedings - 15th International Conference on Advanced Trends in Radioelectronics, Telecommunications and Computer Engineering, TCSET 2020},
year={2020},
pages={377-380},
art_number={9088621},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85086304495&doi=10.1109%2fTCSET49122.2020.235458&partnerID=40&md5=58b62ddff0684820d7007bdf318cb75d},
abstract={Unmanned aerial vehicles can fly in an autonomic flight mode without any active radio control or passive radio navigation and they are almost invisible for radars. Only engines and propellers acoustic emission (AE) may give lots of information for their detection, recognition and location. This paper discusses the experimental results of testing the classical detection and direction finding methods by Bartlett, Capeon and cross-correlation function method with the use of microphone array. Experiments include physical investigations of the UAV acoustic emission presented with two signal models - harmonic signal and broadband signal and for two conditions, namely, indoor and in the open area. Detection and recognition the UAV on a noisy background by spectral signs give the same quality as the Mel-Frequency cepstral coefficients method, but don't need to make acoustic portraits. The cross-correlation function method gives the best results in direction finding of the UAV. © 2020 IEEE.},
}

@ARTICLE{Mu2020,
author={Mu, Y. and Zhang, X. and Xie, W. and Zheng, Y.},
title={Automatic detection of near-surface targets for unmanned aerial vehicle (UAV) magnetic survey},
journal={Remote Sensing},
year={2020},
volume={12},
number={3},
art_number={452},
note={cited By 14},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85080860804&doi=10.3390%2frs12030452&partnerID=40&md5=7bb759820079aa394a39b204f9902ff9},
abstract={Great progress has been made in the integration of Unmanned Aerial Vehicle (UAV) magnetic measurement systems, but the interpretation of UAV magnetic data is facing serious challenges. This paper presents a complete workflow for the detection of the subsurface objects, like Unexploded Ordnance (UXO), by the UAV-borne magnetic survey. The elimination of interference field generated by the drone and an improved Euler deconvolution are emphasized. The quality of UAV magnetic data is limited by the UAV interference field. A compensation method based on the signal correlation is proposed to remove the UAV interference field, which lays the foundation for the subsequent interpretation of UAV magnetic data. An improved Euler deconvolution is developed to estimate the location of underground targets automatically, which is the combination of YOLOv3 (You Only Look Once version 3) and Euler deconvolution. YOLOv3 is a deep convolutional neural network (DCNN)-based image and video detector and it is applied in the context of magnetic survey for the first time, replacing the traditional sliding window. The improved algorithm is more satisfactory for the large-scale UAV-borne magnetic survey because of the simpler and faster workflow, compared with the traditional sliding window (SW)-based Euler method. The field test is conducted and the experimental results show that all procedures in the designed routine is reasonable and effective. The UAV interference field is suppressed significantly with root mean square error 0.5391 nT and the improved Euler deconvolution outperforms the SW Euler deconvolution in terms of positioning accuracy and reducing false targets. © 2020 by the authors.},
}

@ARTICLE{Nagarani2020463,
author={Nagarani, N. and Venkatakrishnan, P. and Balaji, N.},
title={Unmanned Aerial vehicle's runway landing system with efficient target detection by using morphological fusion for military surveillance system},
journal={Computer Communications},
year={2020},
volume={151},
pages={463-472},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85077949049&doi=10.1016%2fj.comcom.2019.12.039&partnerID=40&md5=122408f95bf09df75f793d992c3e4cb3},
abstract={In the surveillance of military system Unmanned Ariel vehicles (UAV's) offers a remarkable service. Software Defined Network (SDN) is one of approach for UAV for improving target localization with surveillance for many applications. One of the critical issues for an Unmanned Ariel vehicles (UAV's) landing is the detection of runway in a low visibility conditions with computer vision. Also, the key problem is the accurate and robust detection of runway. A method of runway detection for fixed wing UAVs with a forward-looking camera is uses sensor based communication in network framework between source (UAV'S) and destination (runway sensor). Yet, this depends on the technical experience for landing an UAV's safely. Nowadays, highly advanced equipments are being developed for improving safety and transportation system to handle the problem of landing under low visibility conditions. However, natural or habitual vision could be reduced during low visibility situations. This may be due to many meteorological factors like haze, darkness, fog etc. From the discussion made in this paper, the authors mainly concentrate on managing an aircraft system under low luminosity condition during the landing. In this research, effective Morphological fusion method is employed for the prediction of virtual runway imagery to avoid accident landing process. For this, fusion of sensor data for DEM (Digital Elevation Map) Data, infrared image (IR) and navigation parameter are used. The performance of this research using Morphological fusion method gives a fused image of the runway prediction for UAV's under poor visibility condition. After obtaining the fused image, it is involved in ROI (Region of Interest) contour tracing process to get the clear location of landing of an UAV's without harm. The virtual imaginary model can be produced through contour tracing to predict runway. By this method, a less prediction time or setting time is achieved and maximum accuracy is obtained through simulation using MATLAB tool. Finally, the proposed experimental outcomes are compared with the existing technology. The proposed approach will be use in aircraft sensor based communication between the network (source to destination) to detect the target and to provide a better surveillance for military applications. © 2019 Elsevier B.V.},
}

@ARTICLE{Zheng2020,
author={Zheng, H. and Zhou, X. and He, J. and Yao, X. and Cheng, T. and Zhu, Y. and Cao, W. and Tian, Y.},
title={Early season detection of rice plants using RGB, NIR-G-B and multispectral images from unmanned aerial vehicle (UAV)},
journal={Computers and Electronics in Agriculture},
year={2020},
volume={169},
art_number={105223},
note={cited By 21},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85077797429&doi=10.1016%2fj.compag.2020.105223&partnerID=40&md5=0f26109c5cc7e126aa90e79b6bf76af5},
abstract={Crop plant detection is vital for mapping crop planting area and extracting pure crop canopy information. In this study, three cameras (RGB, color infrared (NIR-G-B) and multispectral (MS) camera) were mounted on a multi-rotor unmanned aerial vehicle (UAV) to obtain images of rice canopy at the early growth stages (tillering, jointing and initial booting stages). We proposed a new decision tree (DT) combining texture features (mean and variance (C.V)) and spectral features (TS-DT) for rice plants detection within UAV images. First, the image was classified into the pure class and the mixed class based on the C.V value. Then the pure class was classified into rice plants and road by the DN or reflectance value in red band. The mixed class was classified into rice plants and background (soil, water and duckweed) through comparing each pixel value to the mean value within the moving window. The results showed that TS-DT exhibited an averaged high classification accuracy with overall accuracy (OA) and kappa coefficient (KC) of 91.25%, 0.86, 92.88%, 0.86 and 93.53%, 0.88 for RGB, NIR and MS image among the early three growth stages, respectively. The highest estimation accuracy was obtained at booting stage and the lowest was at tillering stage. Compared with the traditional classification methods, the TS-DT method achieved an improved estimation accuracy of 5.2–26.71% in OA and 0.06–0.40 in KC. Therefore, this TS-DT method is a reliable approach for crop plants detection using UAV imagery. © 2020},
}

@CONFERENCE{Wang20201937,
author={Wang, R. and Zhang, S. and Chen, B. and Xu, J. and Zhong, L.},
title={Unmanned aerial vehicle (UAV) vision-based detection and location of power towers for transmission line maintenance},
journal={IET Conference Publications},
year={2020},
volume={2020},
number={CP775},
pages={1937-1941},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85116480628&doi=10.1049%2ficp.2020.0328&partnerID=40&md5=9bb06245990004d064475fe59310a8e6},
abstract={With the rapid development of technology in unmanned aerial vehicles (UAV), more and more UAVs are used by power supply companies for power line inspection and maintenance. However, a large quantity of aerial images captured by UAVs are processed manually at present, which relies on prior knowledge of power towers and is not only time-consuming but also inefficient. Worse still, the geographical positions of abnormal power towers are difficult to be obtained so that the maintenance team has no direction to proceed. In this work, we propose a deep learning-based method for detecting and locating abnormal power towers from the aerial images captured by UAVs. In this method, an objection detection algorithm based on deep convolutional neural network (CNN) is firstly designed to identify and detect abnormal power towers from aerial images. Secondly, the geographical positions of the detected abnormal power towers are approximated by UAV metadata recorded in aerial images (e.g. pixel size, altitude, pitch angle, roll angle, yaw angle, et al.) and several coordinate transformations. Compared with the classical image processing methods, the present method is automatic and end-to-end, and can be easily applied in the UAV based inspection of power transmission lines. © 2020 Institution of Engineering and Technology. All rights reserved.},
}

@BOOK{Cristofaro202067,
author={Cristofaro, A. and Rotondo, D. and Johansen, T.A.},
title={An unknown input observer-based framework for fault and icing detection and accommodation in overactuated unmanned aerial vehicles},
journal={Fault Diagnosis and Fault-Tolerant Control of Robotic and Autonomous Systems},
year={2020},
pages={67-92},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85115713423&doi=10.1049%2fPBCE126E_ch4&partnerID=40&md5=2107667515208cea067ee230e521d37d},
abstract={The use of unmanned aerial vehicles (UAVs) as support to operations in remote areas and harsh environments, such as marine operations in the Arctic, is becoming more and more crucial. These systems are expected to face very critical weather conditions, and for this reason they are naturally prone to the occurrence of icing. The formation of ice layers on airfoils decreases the lift and, simultaneously, increases the drag and the mass of the vehicle, thus requiring additional engine power and implying a premature stall angle. By adopting some tools from the control allocation framework, this chapter aims at presenting an unknown input observer (UIO) approach for fault and icing diagnosis and accommodation in UAVs equipped with a redundant suite of effectors and actuators. The chapter is structured as follows. At first, the UAV model and the basic setups are given, and then the fault and icing effects on the UAV dynamics are discussed. A short overview on the design ofUIOs is proposed, and a main section is dedicated to present the icing diagnosis and accommodation tasks. Furthermore, by means of appropriate scheduling parameters, the UIO-based diagnosis scheme can be extended to the nonlinear aircraft dynamics by considering the framework of linear parameter varying (LPV) systems. A collection of simulation examples concludes the chapter and illustrates the practical application of the proposed architecture. © The Institution of Engineering and Technology 2020.},
}

@ARTICLE{Pawełczyk2020174394,
author={Pawełczyk, M.Ł. and Wojtyra, M.},
title={Real world object detection dataset for quadcopter unmanned aerial vehicle detection},
journal={IEEE Access},
year={2020},
volume={8},
pages={174394-174409},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85102729789&doi=10.1109%2fACCESS.2020.3026192&partnerID=40&md5=69842a2cc079bf76c2d1ac3bc078d7b1},
abstract={Recent years have shown a noticeable rise in the number of incidents with drones, related to both civilian and military installations. While drone neutralization techniques have become increasingly effective, detection most often relies on professional equipment, which is too expensive to be used for all critical nodes and applications. Therefore, there is a need for drone detection systems that could work on low performance hardware. Its critical component consists of an object detection system. In this article, we introduce a new object detection dataset, built entirely to train computer vision based object detection machine learning algorithms for a task of binary object detection to enable automated, industrial camera based detection of multiple drone objects using camera feed. The dataset expands existing multiclass image classification and object detection datasets (ImageNet, MS-COCO, PASCAL VOC, anti-UAV) with a diversified dataset of drone images. In order to maximize the effectiveness of the model, real world footage was utilized, transformed into images and hand-labelled to create a custom set of 56821 images and 55539 bounding boxes. Additionally, semi-automated labelling was proposed, tested and proved to be very useful for object detection applications. The dataset was divided into train and test subsets for further processing and used to generate 603 easily deployable Haar Cascades as well as 819 high performing Deep Neural Networks based models. They were used to test different object detection methods to determine the long term feasibility of a large scale drone detection system utilizing machine learning algorithms. The study has shown that Haar Cascade can be used as the Minimum Viable Product model for mediocre performance but fails to scale up effectively for a larger dataset compared to the Deep Neural Network model. © 2021},
}

@ARTICLE{Abramov202036,
author={Abramov, S. and Abramova, V. and Abramov, K. and Lukin, V. and Bondar, V. and Kaluzhinov, I.},
title={TECHNIQUE OF DETECTION FIELD ESTIMATING FOR UNMANNED AERIAL VEHICLES BY A GROUND OBSERVER},
journal={Radioelectronic and Computer Systems},
year={2020},
number={3-95},
pages={36-42},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85101538977&doi=10.32620%2freks.2020.3.04&partnerID=40&md5=0386858b9ba30f373d2f3e8259c6cebf},
abstract={The widespread use of small-sized unmanned aerial vehicles (UAVs) makes it urgent to control their use in the airspace over strategic infrastructure facilities. The design features of UAVs provide them with low visibility in all existing observation ranges: radar, visual, thermal, and acoustic. In this regard, for the reliable detection of such aircraft, it is necessary to use complex systems that conduct simultaneous observations in all available ranges. To optimize the location of such systems, the problem arises of determining the fields of reliable detection of UAVs for each of the means included in the system. To solve this problem for the means of visual and thermal detection based on the previously developed technique for determining the indications of the detection range based on the determination of the visually visible area of the UAV, calculated from the existing three-dimensional model of the vehicle, a new method is proposed for analyzing the characteristics of the UAV visibility for the ground observer. The application of the proposed technique is demonstrated by the example of two UAV models: ECO – with an internal combustion engine, and ELECTRA – with an electric motor. The concept of the indicatrix of the detection field is introduced, as an indicatrix of the maximum detection range, transferred from the UAV coordinate system to the observer's coordinate system by simple geometric transformations. Based on the indications of the detection field, it is possible to carry out both a direct comparative analysis of the visual visibility of UAVs and to obtain additional information from them, useful for making recommendations on the parameters of the UAV flight, in particular, the flight altitude and the direction of approach to the location of a potential observer. If there is an indicatrix of the detection field for the analyzed UAV, the calculation of the detection zone boundary can be performed automatically for any given height. This allows you to visualize information about the limits within which the UAV detection range can change depending on the direction and altitude of its flight. © С. К. Абрамов, В. В. Абрамова, К. Д. Абрамов, В. В. Лукин, В. В. Бондарь, И. В. Калужинов, 2020},
}

@ARTICLE{Ham2020553,
author={Ham, S.W. and Park, H.-C. and Kim, E.-J. and Kho, S.-Y. and Kim, D.-K.},
title={Investigating the influential factors for practical application of multi-class vehicle detection for images from unmanned aerial vehicle using deep learning models},
journal={Transportation Research Record},
year={2020},
volume={2674},
number={12},
pages={553-567},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85099447130&doi=10.1177%2f0361198120954187&partnerID=40&md5=4775311d74619618636af7578a20ac61},
abstract={Traffic density, which is a critical measure in traffic operations, should be collected precisely at various locations and times to reflect site-specific spatiotemporal characteristics. For detailed analysis, heavy vehicles have to be separated from ordinary vehicles, since heavy vehicles have a significant effect on traffic flow as well as traffic safety. With unmanned aerial vehicles (UAVs), it is easy to acquire video for vehicle detection by collecting images from above the traffic without any disturbances. Despite previous studies on vehicle detection, there is still a lack of research on real-world applications in estimating traffic density. This study investigates the effects of several influential factors: the size of objects, the number of samples, and a combination of datasets, on detecting multi-class vehicles using deep learning models in various UAV images. Three detection models are compared: faster region-based convolutional neural networks (faster R-CNN), region-based fully convolutional network (R-FCN), and single-shot detector (SSD), to suggest guidelines for model selection. The results provided several findings: (i) vehicle detection from UAV images showed sufficient performance with a small number of samples and small objects; (ii) deep learning-based multi-class vehicle detectors can have advantages compared with single-class detectors; (iii) among all the models, SSD showed the best performance because of its algorithmic structure; (iv) simply combining datasets in different environments cannot guarantee performance improvement. Based on these findings, practical guidelines are offered for estimating multi-class traffic density using UAV. © National Academy of Sciences: Transportation Research Board 2020.},
}

@ARTICLE{Hu2020,
author={Hu, G. and Zhu, Y. and Wan, M. and Bao, W. and Zhang, Y. and Liang, D. and Yin, C.},
title={Detection of diseased pine trees in unmanned aerial vehicle images by using deep convolutional neural networks},
journal={Geocarto International},
year={2020},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85098869503&doi=10.1080%2f10106049.2020.1864025&partnerID=40&md5=7f3320890cc4046741e97cf153da15c6},
abstract={This study presents a method that uses high-resolution remote sensing images collected by an unmanned aerial vehicle (UAV) and combines MobileNet and Faster R-CNN for detecting diseased pine trees. MobileNet is used to remove backgrounds to reduce the interference of background information. Faster R-CNN is adopted to distinguish between diseased and healthy pine trees. The number of training samples is expanded due to the insufficient number of available UAV images. Experimental results show that the proposed method is better than traditional machine learning approaches, such as support vector machine and AdaBoost, and methods of DCNN, such as Alexnet, Inception and Faster R-CNN. Through sample expansion and background removal, the proposed method achieves effective detection of diseased pine trees in UAV images by using deep learning technology. © 2021 Informa UK Limited, trading as Taylor & Francis Group.},
}

@ARTICLE{Park202045,
author={Park, K.H. and Park, E. and Kim, H.K.},
title={Unsupervised intrusion detection system for unmanned aerial vehicle with less labeling effort},
journal={Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
year={2020},
volume={12583 LNCS},
pages={45-58},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85098269536&doi=10.1007%2f978-3-030-65299-9_4&partnerID=40&md5=4140709d61e50bd724488c86a8af51b3},
abstract={Along with the importance of safety, an IDS has become a significant task in the real world. Prior studies proposed various intrusion detection models for the UAV. Past rule-based approaches provided a concrete baseline IDS model, and the machine learning-based method achieved a precise intrusion detection performance on the UAV with supervised learning models. However, previous methods have room for improvement to be implemented in the real world. Prior methods required a large labeling effort on the dataset, and the model could not identify attacks that were not trained before. To jump over these hurdles, we propose an IDS with unsupervised learning. As unsupervised learning does not require labeling, our model let the practitioner not to label every type of attack from the flight data. Moreover, the model can identify an abnormal status of the UAV regardless of the type of attack. We trained an autoencoder with the benign flight data only and checked the model provides a different reconstruction loss at the benign flight and the flight under attack. We discovered that the model produces much higher reconstruction loss with the flight under attack than the benign flight; thus, this reconstruction loss can be utilized to recognize an intrusion to the UAV. With consideration of the computation overhead and the detection performance in the wild, we expect our model can be a concrete and practical baseline IDS on the UAV. © Springer Nature Switzerland AG 2020.},
}

@CONFERENCE{Mao2020,
author={Mao, Z. and Zhao, C. and Zheng, Y. and Mao, Y. and Li, H. and Hua, L. and Liu, Y.},
title={Research on detection method of pavement diseases based on Unmanned Aerial Vehicle (UAV)},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2020},
volume={11584},
art_number={115840L},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85097199870&doi=10.1117%2f12.2580285&partnerID=40&md5=419d17ad68b87f91d355cf3247583df6},
abstract={In order to improve the accuracy of road surface disease detection, the development technology of unmanned aerial vehicle (UAV) in the intelligent transportation field are analyzed. Firstly, the framework of pavement disease recognition and perception system based on UAV is constructed; Secondly, the pavement image data collection experiment is carried out with Yuneec H520 UAV, and the pavement disease image preprocessing technology based on wavelet threshold transform is analyzed; Thirdly, the pavement disease image preprocessing technology based on the DPM is studied, and the recognition method of pavement disease based on VGG-16 neural net-work model is proposed. Theoretical analysis and experimental results show that the method of pavement disease identification based on VGG-16 neural network model has high classification accuracy, and its classification accuracy is better than 90ï1/4. © COPYRIGHT SPIE. Downloading of the abstract is permitted for personal use only.},
}

@CONFERENCE{Golyak2020,
author={Golyak, I.S. and Anfimov, D.R. and Fufurin, I.L. and Nazolin, A.L. and Bashkin, S.V. and Glushkov, V.L. and Morozov, A.N.},
title={Optical multi-band detection of unmanned aerial vehicles with YOLO v4 convolutional neural network},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2020},
volume={11525},
art_number={115250Y},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85097171427&doi=10.1117%2f12.2584591&partnerID=40&md5=02fc740765044f4f6bd990289a392892},
abstract={The paper presents a method for optical detection drones using the YOLO v4 neural network. Recognition performs simultaneously in the visible (Vis) and long-wave infrared (LWIR) ranges. The results of UAV detection on various types of urban background environment at day and night conditions, as well as at different distances from cameras, are presented. An algorithm for detecting of unmanned vehicles in the video cameras field of view of the Vis and LWIR ranges is described. This algorithm takes as input the outputs of two neural networks that recognize the drone in two ranges and estimates the probability of detection. Its shown that the YOLO v4 neural network recognizes unmanned objects on various background substrates with a minimum temperature difference of 0.4 degrees on the NEC 2640 thermal imager. Copyright © 2020 SPIE.},
}

@ARTICLE{Cazzato2020,
author={Cazzato, D. and Cimarelli, C. and Sanchez-Lopez, J.L. and Voos, H. and Leo, M.},
title={A survey of computer vision methods for 2d object detection from unmanned aerial vehicles},
journal={Journal of Imaging},
year={2020},
volume={6},
number={8},
art_number={78},
note={cited By 10},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85091995725&doi=10.3390%2fJIMAGING6080078&partnerID=40&md5=2da1234b79a9085870cf8fa29d34a5e8},
abstract={The spread of Unmanned Aerial Vehicles (UAVs) in the last decade revolutionized many applications fields. Most investigated research topics focus on increasing autonomy during operational campaigns, environmental monitoring, surveillance, maps, and labeling. To achieve such complex goals, a high-level module is exploited to build semantic knowledge leveraging the outputs of the low-level module that takes data acquired from multiple sensors and extracts information concerning what is sensed. All in all, the detection of the objects is undoubtedly the most important low-level task, and the most employed sensors to accomplish it are by far RGB cameras due to costs, dimensions, and the wide literature on RGB-based object detection. This survey presents recent advancements in 2D object detection for the case of UAVs, focusing on the differences, strategies, and trade-offs between the generic problem of object detection, and the adaptation of such solutions for operations of the UAV. Moreover, a new taxonomy that considers different heights intervals and driven by the methodological approaches introduced by the works in the state of the art instead of hardware, physical and/or technological constraints is proposed. © 2020 by the authors. Licensee MDPI, Basel, Switzerland. This article is an open access article distributed under the terms and conditions of the Creative Commons Attribution (CC BY) license (http://creativecommons.org/licenses/by/4.0/).},
}

@CONFERENCE{Esposito20201,
author={Esposito, N. and Fontana, U. and D’autilia, G. and Bianchi, L. and Alibani, M. and Pollini, L.},
title={A hybrid approach to detection and tracking of unmanned aerial vehicles},
journal={AIAA Scitech 2020 Forum},
year={2020},
volume={1 PartF},
pages={1-10},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85091897676&doi=10.2514%2f6.2020-1345&partnerID=40&md5=3e75365b57da0196509cd14387487233},
abstract={This paper proposes a novel, hybrid vision-based system to autonomously detect and track a specific moving target, in our case an evader UAV (Unmanned Aerial Vehicles), with a moving camera. The framework is based on a detection stage which exploits a Faster Region-based Convolutional Neural Network (Faster R-CNN) designed to detect the Region Of Interest (ROI) associated to the UAV’s position in the image plane. The moving target is tracked by using an Optical Flow-based tracking system and a Kalman Filter is used to give temporal consistency between consecutive measurements. The tracking system is designed to be able to achieve real-time image processing on embedded systems, for this reason a lag compensation algorithm for the delay due to the Faster R-CNN computation time is implemented. Algorithm’s performance is evaluated by computing the error between the true UAV position in the image plane and the estimated position resulting from the tracking system. © 2020, American Institute of Aeronautics and Astronautics Inc, AIAA. All rights reserved.},
}

@CONFERENCE{Loureiro2020129,
author={Loureiro, G. and Dias, A. and Martins, A.},
title={Survey of approaches for emergency landing spot detection with unmanned aerial vehicles},
journal={Robots in Human Life- Proceedings of the 23rd International Conference on Climbing and Walking Robots and the Support Technologies for Mobile Machines, CLAWAR 2020},
year={2020},
pages={129-136},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85091310506&doi=10.13180%2fclawar.2020.24-26.08.52&partnerID=40&md5=90ea63c344838efed6931b3dd34f8e90},
abstract={For the past years, the interest in the use of Unmanned Aerial Vehicles (UAVs) has been increasing due to the multiple research topics provided by the field of aerial robotics. Conversely, vehicles are susceptible to failures or malfunctions. Consequently, one main emergent research topic is the detection of a safe landing spot in these emergency scenarios. Therefore, this paper exposes and details the multiple techniques that attempt to solve the problem of landing site detection. This paper aims to present the current literature with several sensors that can be used to solve the aforementioned problem. Finally, the paper presents our proposed approach with some preliminary results in simulation. © CLAWAR Association Ltd.},
}

@ARTICLE{Gao2020,
author={Gao, J. and Zhang, Q. and Chen, J.},
title={EKF-Based Actuator Fault Detection and Diagnosis Method for Tilt-Rotor Unmanned Aerial Vehicles},
journal={Mathematical Problems in Engineering},
year={2020},
volume={2020},
art_number={8019017},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85090767852&doi=10.1155%2f2020%2f8019017&partnerID=40&md5=e4cb22a7b8e8d17021af99a05ff5e6a8},
abstract={Flight safety is of vital importance for tilt-rotor unmanned aerial vehicles (UAVs), which can take off and land vertically as well as cruise at high speed, especially in different kinds of complex environment. As being the executor of the flight control, the actuator failure will directly affect the controllability of the tilt-rotor UAV, and it has high probability of causing fatal personal injury and financial loss. However, due to the limitation of weight and cost, small UAVs cannot be equipped with redundant actuators. Therefore, there is an urgent need of fault detection and diagnosis method for the actuators. In this paper, an actuator fault detection and diagnosis (FDD) method based on the extended Kalman filter (EKF) and multiple-model adaptive estimation (MMAE) is proposed. The actuator deflections are added to the state vector and estimated using EKF. The fault diagnosis algorithm of MMAE could assign a conditional probability to each faulty actuator according to the residual of EKF and diagnose the fault. This paper is structured as follows: first, the structure and model of tilt-rotor UAV actuator are established. Then, EKF observers are introduced to estimate the state vector and to calculate residual sequences caused by different faulty actuators. The residuals from EKFs are used by fault diagnosis algorithm to assign a conditional probability to each failure condition, and fault type can be diagnosed according to the probabilities. The FDD method is verified by simulations, and the results demonstrate that the FDD algorithm could accurately and efficiently diagnose actuator fault without any additional sensor. © 2020 Jiaxin Gao et al.},
}

@ARTICLE{Liang2020,
author={Liang, C. and Miao, M. and Ma, J. and Yan, H. and Zhang, Q. and Li, X.},
title={Detection of global positioning system spoofing attack on unmanned aerial vehicle system},
journal={Concurrency Computation},
year={2020},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85088312463&doi=10.1002%2fcpe.5925&partnerID=40&md5=b26fa5588b2159625ea21aed4b644632},
abstract={Most of the existing global positioning system (GPS) spoofing detection schemes are vulnerable to the generative GPS spoofing attack, or require additional auxiliary equipment and extensive signal processing capabilities, leading to defects such as low real-time performance and large communication overhead which are not available for the unmanned aerial vehicle (UAV, also known as drone) system. Therefore, we propose a novel solution which employs information fusion based on the GPS receiver and inertial measurement unit. We use a real-time model of tracking and calculating to derive the current position of the drones which are then contrasted with the position information received by the receiver to verify whether the presence or absence of spoofing attack. Subsequent experimental work shows that, the proposed method can accurately detect the spoof within 8 seconds, with a detection rate (DR) of 98.6%. Compared with the existing schemes, the performance of real-time detecting is improved while the DR is ensured. Even in our worst-case, we detect the spoof within 28 seconds after the UAV system starts its mission. © 2020 John Wiley & Sons Ltd},
}

@ARTICLE{Yamazaki2020101398,
author={Yamazaki, Y. and Premachandra, C. and Perea, C.J.},
title={Audio-Processing-Based Human Detection at Disaster Sites with Unmanned Aerial Vehicle},
journal={IEEE Access},
year={2020},
volume={8},
pages={101398-101405},
art_number={9104665},
note={cited By 7},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85086626642&doi=10.1109%2fACCESS.2020.2998776&partnerID=40&md5=071685ef90f3df9585b6e1a4c95efffd},
abstract={This paper describes a human search system that uses an unmanned aerial vehicle (UAV). The use of robots to search for people is expected to become an auxiliary tool for saving lives during a disaster. In particular, because UAVs can collect information from the air, there has been much research into human search using UAVs equipped with cameras. However, the disadvantage of cameras is that they struggle to detect people who are hidden in shadows. To solve this problem, we mounted an array microphone on a UAV and to detect the human voice as a means of finding people that cameras cannot. Also a search method is proposed that combines voice and camera human detection to compensate for their respective shortcomings. The rate and accuracy of human detection by the proposed method are assessed experimentally. © 2020 IEEE.},
}

@ARTICLE{Doukhi2020295,
author={Doukhi, O. and Hossain, S. and Lee, D.-J.},
title={Real-time deep learning for moving target detection and tracking using unmanned aerial vehicle},
journal={Journal of Institute of Control, Robotics and Systems},
year={2020},
volume={26},
number={5},
pages={295-301},
note={cited By 9},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85085090612&doi=10.5302%2fJ.ICROS.2020.20.0027&partnerID=40&md5=1c178a6622bd9c2e29e5b89dec532985},
abstract={Real-timeand-rescue. object detection and tracking are crucial for many applications such as observation and surveillance, and search-There have been many advancements in deep learning techniques for object detection and tracking due to the successful development of computing devices. Based on these ideas, the YOLO deep learning visual object detection algorithm was utilized to visually guide the UAV to track the detected target. The detected target bounding box and the image frame center were the main parameters that were used to control the forward motion, heading, and altitude of the vehicle. The proposed control system approach consisted of two PID controllers that managed the heading and altitude rates. For a real-time computing device a Nvidia Jetson TX2 based edge-computing module is used, whichh takes the input data from onboard sensors such as camera. A navigation system operated entirely onboard the UAV in the absence of external localization sensors or a GPS signal is introduced, and it uses a fisheye camera to perform a visual SLAM for localization. The robustness and effectiveness of the proposed deep-learning based target detection and tracking algorithms were verified through various simulation and real-time flight experiments. © ICROS 2020.},
}

@CONFERENCE{Sanyal202073,
author={Sanyal, S. and Bhushan, S. and Sivayazi, K.},
title={Detection and location estimation of object in unmanned aerial vehicle using single camera and GPS},
journal={2020 1st International Conference on Power, Control and Computing Technologies, ICPC2T 2020},
year={2020},
pages={73-78},
art_number={9071439},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85084324248&doi=10.1109%2fICPC2T48082.2020.9071439&partnerID=40&md5=c3df658bf8d714e89b49c19637a353ee},
abstract={It is important for an Unmanned Aerial Vehicle (UAV) to detect any object in its view. This enables the UAV to locate the object with respect to itself and is required for locking and tracking the object. Object detection and location estimation makes the UAV capable of manipulating the environment as well as to follow the target. In the present work, object detection has been carried out using You Only Look Once (YOLO) to detect the object in the image stream of the Robot Operating System (ROS) bag file. The GPS information of the UAV is used to further calculate the GPS coordinates of the object. The images are acquired using a single monocular camera. © 2020 IEEE.},
}

@ARTICLE{Lozano2020855,
author={Lozano, V. and Brundu, G. and Ghiani, L. and Piccirilli, D. and Sassu, A. and Tiloca, M.T. and Ledda, L. and Gambella, F.},
title={Detection and Monitoring of Alien Weeds Using Unmanned Aerial Vehicle in Agricultural Systems in Sardinia (Italy)},
journal={Lecture Notes in Civil Engineering},
year={2020},
volume={67},
pages={855-862},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85083990384&doi=10.1007%2f978-3-030-39299-4_92&partnerID=40&md5=7e68c2369b3b086472c5d536925a8f72},
abstract={Emerging technologies such as high-resolution Unmanned Aerial Vehicles (UAVs) surveys combined with object-based image analysis, and field surveys could represent a reliable, precise, and effective tool to support land management in agricultural systems. The technological advances of UAVs can also promote the detection and regular monitoring of invasive alien plants and agricultural weeds. The objective of the study has been to identify, map and monitor alien weed species in agricultural systems to provide an overview of the future applications and challenges of precision farming. In particular, we evaluated how UAV imagery can be used to assess the cover of Oxalis pes-caprae, present in several crops in Sardinia as an alien invasive weed, with negative direct and indirect effects on the affected crops. Our core assumption is that the most reliable species discrimination can be achieved by targeting flights during flowering to allow easier detection due to species-specific spectral differences. Therefore, O. pes-caprae infestation was acquired using RGB camera installed on board a Phantom 4 pro. As a result, we presented the mapping of O. pes-caprae, highlighting the cost-effectiveness and replicability of this approach to detect the presence of this alien weed in agricultural fields. © Springer Nature Switzerland AG 2020.},
}

@ARTICLE{Meng2020,
author={Meng, L. and Peng, Z. and Zhou, J. and Zhang, J. and Lu, Z. and Baumann, A. and Du, Y.},
title={Real-time detection of ground objects based on unmanned aerial vehicle remote sensing with deep learning: Application in excavator detection for pipeline safety},
journal={Remote Sensing},
year={2020},
volume={12},
number={1},
art_number={182},
note={cited By 17},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85081888375&doi=10.3390%2fRS12010182&partnerID=40&md5=61c67b9da93afb5644704e79ec1e21e3},
abstract={Unmanned aerial vehicle (UAV) remote sensing and deep learning provide a practical approach to object detection. However, most of the current approaches for processing UAV remote-sensing data cannot carry out object detection in real time for emergencies, such as firefighting. This study proposes a new approach for integrating UAV remote sensing and deep learning for the real-time detection of ground objects. Excavators, which usually threaten pipeline safety, are selected as the target object. A widely used deep-learning algorithm, namely You Only Look Once V3, is first used to train the excavator detection model on a workstation and then deployed on an embedded board that is carried by a UAV. The recall rate of the trained excavator detection model is 99.4%, demonstrating that the trained model has a very high accuracy. Then, the UAV for an excavator detection system (UAV-ED) is further constructed for operational application. UAV-ED is composed of a UAV Control Module, a UAV Module, and a Warning Module. A UAV experiment with different scenarios was conducted to evaluate the performance of the UAV-ED. The whole process from the UAV observation of an excavator to theWarning Module (350 km away from the testing area) receiving the detection results only lasted about 1.15 s. Thus, the UAV-ED system has good performance and would benefit the management of pipeline safety. © 2020 by the authors.},
}

@CONFERENCE{Wang2020,
author={Wang, W. and Hong, H. and Zhang, Y. and Li, S. and Shi, J.},
title={Realization of real-time detection algorithms for key parts of unmanned aerial vehicle based on support vector machine},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2020},
volume={11429},
art_number={114290N},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85081337150&doi=10.1117%2f12.2538213&partnerID=40&md5=7acca340570255ee3fa7d1550005db65},
abstract={Fixed-point attack on the key parts of small aerial vehicles is an important means of UAV (Unmanned Aerial Vehicle) countermeasure. Because of the fast speed and flexible attitude of fixed-wing aircraft, the detection accuracy of key points of fixed-wing aircraft in infrared images is low and the speed is slow. This paper presents an improved detection and tracking algorithm based on SVM. Firstly, the detection module extracts the fixed-wing aircraft area by image segmentation, then extracts the characteristics of the fixed-wing aircraft, then uses SVM to judge the flight direction of the fixed-wing aircraft, and then locates the key points according to the direction. The experimental results show that the proposed detection algorithm can process 30 frames per second on the platform of DSP (TSM320C6678), and still achieve a high detection rate (<93%) with very high practical value. © 2020 SPIE.},
}

@ARTICLE{Loureiro2020122,
author={Loureiro, G. and Soares, L. and Dias, A. and Martins, A.},
title={Emergency Landing Spot Detection for Unmanned Aerial Vehicle},
journal={Advances in Intelligent Systems and Computing},
year={2020},
volume={1093 AISC},
pages={122-133},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85079102815&doi=10.1007%2f978-3-030-36150-1_11&partnerID=40&md5=1c0be99d0d6285c08b0473c7ce798a17},
abstract={This paper addresses the topic of emergency landing spot detection for Unmanned Aerial Vehicles (UAVs). During operation, the vehicle is susceptible to faults and must be able to predict the land spot able to ensure that the UAV will be able to land without damages and injuries to humans and structures. A method was developed, based on geometric features extracted from Light Detection And Ranging (LIDAR) data. A simulation environment was developed in order to validate the effectiveness and the robustness of the proposed method. © 2020, Springer Nature Switzerland AG.},
}

@ARTICLE{Sun2020755,
author={Sun, J. and Wu, Y. and Lu, X. and Feng, Y.},
title={Cascade Improved Visual Detection and Distance Estimation in Formation of Micro Unmanned Aerial Vehicles},
journal={Lecture Notes in Electrical Engineering},
year={2020},
volume={582},
pages={755-765},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85076835606&doi=10.1007%2f978-981-15-0474-7_71&partnerID=40&md5=abb609dc11776f83fb9e55ac9127bd8f},
abstract={According to the localization of UAVs in formation, this paper has proposed a visual based method using cascade classifiers of LBP and Haar-like features to realize UAVs’ detection and distance estimation. Since the phenomenon of overlapping in formation has an obvious influence on the performance of detection, this paper adopts the method of integrating two classifiers with different features (LBP and Haar) to improve the performance of detector. For the purpose of enhancing the precision of distance estimation, an optimized method is proposed based on the prediction of UAV’s attitude. The description of coordination is deducted to obtain accurately relative position from visual information. The results of test videos verify the performance of proposed method on the application of UAVs formation. © 2020, Springer Nature Singapore Pte Ltd.},
}

@ARTICLE{Cao20201107,
author={Cao, H. and Cheng, L. and Wu, B. and Gao, G.Q.},
title={Research on Unmanned Aerial Vehicle Water Combined Quality Detection and Early-Warning System},
journal={Lecture Notes in Electrical Engineering},
year={2020},
volume={582},
pages={1107-1117},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85076826801&doi=10.1007%2f978-981-15-0474-7_104&partnerID=40&md5=c1f42ca305d3182df700e12f0f6ed9b4},
abstract={Many lands in China are close to rivers and oceans and they are very suitable for developing fisheries. Water quality monitoring is indispensable to the development of fisheries. Therefore, a method of detecting fishery water quality by using unmanned aerial vehicle (UAV) electrode sensor array, evaluating and predicting the data transmission back to the background, and feeding back the evaluation and prediction results in time is proposed. The results show that this method can timely monitor fishery water quality and predict the future trend of water quality, and improve the detection efficiency. © 2020, Springer Nature Singapore Pte Ltd.},
}

@ARTICLE{Srinivas2020646,
author={Srinivas, K. and Dua, M.},
title={Fog Computing and Deep CNN Based Efficient Approach to Early Forest Fire Detection with Unmanned Aerial Vehicles},
journal={Lecture Notes in Networks and Systems},
year={2020},
volume={98},
pages={646-652},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85075056956&doi=10.1007%2f978-3-030-33846-6_69&partnerID=40&md5=4026859c9c87ff5f408ad9a7ee5f1bc3},
abstract={Fog computing assits the development of distributed real-time systems. This offers solutions to a quicker response systems for developing disaster monitoring, prevention and detection models into existence. This paper proposes the integration of Fog computing and Convolutional Neural Networks (CNN) with Unmanned Aerial Vehicles (UAV) to detect the forest fire at an early stage. A highly efficient CNN model has been used for fire image recognition due to its proven ability for such recognition tasks. By using AlexNet and other architectures in the proposed model, image recognition tasks have become more capable, to an extent that a pre-trained model has an ability equal to a primate. Using these architectures, we trained our model and deployed the same on a Fog device, which has resulted in achieving higher accuracy and response time. © Springer Nature Switzerland AG 2020.},
}

@ARTICLE{Sudhakar20201,
author={Sudhakar, S. and Vijayakumar, V. and Sathiya Kumar, C. and Priya, V. and Ravi, L. and Subramaniyaswamy, V.},
title={Unmanned Aerial Vehicle (UAV) based Forest Fire Detection and monitoring for reducing false alarms in forest-fires},
journal={Computer Communications},
year={2020},
volume={149},
pages={1-16},
note={cited By 61},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85072979773&doi=10.1016%2fj.comcom.2019.10.007&partnerID=40&md5=6606cd6a3e9fca293f853c3fae4a7323},
abstract={The primary sources for ecological degradation currently are the Forest Fires (FF). The present observation frameworks for FF absence need supporting in constant checking of each purpose of the location at all time and prime location of the fire dangers. This approach gives works on preparing UAV (Unmanned Aerial Vehicle) aeronautical picture information as indicated by the prerequisites of ranger service territory application on a UAV stage. It provides a continuous and remote watch on a flame in forests and mountains, all the while the UAV is flying and getting the elevated information, helping clients maintain the number and area of flame focuses. Observing programming spreads capacities, including Fire: source identification, area, choice estimation, and LCD module. This paper proposed includes (1) Color Code Identification, (2) Smoke Motion Recognition, and (3) Fire Classification algorithms. Strikingly, the use of a helicopter with visual cameras portrayed. The paper introduces the strategies utilized for flame division invisible cameras, and the systems to meld the information acquired the following: Correctly, the current FF location stays testing, given profoundly convoluted and non-organized conditions of the forest, smoke hindering the flame, the movement of cameras mounted on UAVs, and analogs of fire attributes. These unfavorable impacts can truly purpose either false alert. This work focuses on the improvement of trustworthy and exact FF recognition algorithms which apply to UAVs. To effectively execute missions and meet their relating execution criteria examinations on the best way to diminish false caution rates, increment the possibility of profitable recognition, and upgrade versatile abilities to different conditions are firmly requested to improve the unwavering quality and precision of FF location framework. © 2019 Elsevier B.V.},
}

@ARTICLE{Li2020230,
author={Li, K.W. and Chang, S.J. and Peng, L. and Zhao, C.},
title={Visual Detection of Trespassing of a Small Unmanned Aerial Vehicle into an Airspace},
journal={Advances in Intelligent Systems and Computing},
year={2020},
volume={962},
pages={230-237},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85067878609&doi=10.1007%2f978-3-030-20467-9_21&partnerID=40&md5=68dd154c4066393574bfa3927ec463da},
abstract={Small unmanned aerial vehicles (sUAV) have becoming widespread both in commercial and for entertainment usages. They have been used in both business and entertainment purposes. There are sUAV-induced problems. sUAV trespassing into prohibited areas has been the major one of them. A sUAV was guided using a remote controller to suspending in the air. The sUAV may enter a prohibited public area. It may also enter private areas unwelcomed. We conducted a study to quantify human subjects&#x2019; sensitivity in discovering the trespassing of a sUAV into a specific area. Twenty human subjects were requested to determine whether the sUAV has trespassed in the test field or not by answering the question &#x201C;whether the sUAV is inside the test field?&#x201D; by replying a score from 1- definitely yes to 5- definitely no. The conditional probabilities of finding trespassing of the sUAV were calculated. A receivers&#x2019; operating characteristics curve was plotted. The P(A) was calculated and was adopted to represent the sensitivity of the subjects in detecting the trespassing of the drone. The outcomes of the analysis of variance testing the effects of the direction on the probabilities of replying &#x201C;definitely yes&#x201D; and &#x201C;definitely or probably yes&#x201D; were both insignificant. Neither were the effects of direction on the P(A) significant. &#x00A9; 2020, Springer Nature Switzerland AG.},
}

@ARTICLE{Guo2020273,
author={Guo, Q. and Li, Y. and Wang, D.},
title={Pedestrian Detection in Unmanned Aerial Vehicle Scene},
journal={Studies in Computational Intelligence},
year={2020},
volume={810},
pages={273-278},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85062917693&doi=10.1007%2f978-3-030-04946-1_26&partnerID=40&md5=e2531b5602abdfcbff5b5228e5c41f6f},
abstract={With the increasing adoption of unmanned aerial vehicles (UAVs), pedestrian detection with use of such vehicles has been attracting attention. Object detection algorithms based on deep learning have considerably progressed in recent years, but applying existing research results directly to the UAV perspective is difficult. Therefore, in this study, we present a new dataset called UAVs-Pedestrian, which contains various scenes and angles, for improving test results. To validate our dataset, we use the classical detection algorithms SSD, YOLO, and Faster-RCNN. Findings indicate that our dataset is challenging and conducive to the study of pedestrian detection using UAVs. © 2020, Springer Nature Switzerland AG.},
}

@ARTICLE{Ma2019,
author={Ma, Q. and Zhu, B. and Cheng, Z. and Zhang, Y.},
title={Detection and Recognition Method of Fast Low-Altitude Unmanned Aerial Vehicle Based on Dual Channel [基于双通道的快速低空无人机检测识别方法]},
journal={Guangxue Xuebao/Acta Optica Sinica},
year={2019},
volume={39},
number={12},
art_number={1210002},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85078060072&doi=10.3788%2fAOS201939.1210002&partnerID=40&md5=5a6c00423bab2385da347310d6cab7af},
abstract={Using the YOLOv3 architecture, we propose a recognition method for fast low-altitude unmanned aerial vehicle (UAV) detection based on the dual channel (Dual-YOLOv3). In this method, the infrared and visible UAV images are simultaneously input into the deep residual network for feature extraction, and the extracted feature maps are fused to enhance the expression ability of the features. Then, the multi-scale prediction network is used to determine the classification and the position regression of the UAV targets. Finally, we obtain the detection and recognition results. Comparison experiments are conducted on the real collected dataset of dual-band UAVs. The results show that the mAP (mean of average precision) of Dual-YOLOv3-D with average fusion is improved by 6.1% as compared with that of YOLOv3 with the single data source; the detection speed is approximately 27 s-1. © 2019, Chinese Lasers Press. All right reserved.},
}

@ARTICLE{Cong20191634,
author={Cong, M. and Han, L. and Ding, M. and Xu, M. and Tao, Y.},
title={Salient man-made object detection based on saliency potential energy for unmanned aerial vehicles remote sensing image},
journal={Geocarto International},
year={2019},
volume={34},
number={14},
pages={1634-1647},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85055589490&doi=10.1080%2f10106049.2018.1497095&partnerID=40&md5=f86b0708cc37db2dd0c2c985ff97e690},
abstract={It is difficult to automatically recognize complex ground objects, and massive data images with the super-high ground resolution in images captured by unmanned aerial vehicles (UAVs). In order to directly identify the salient man-made ground objects from the UAV remote sensing (RS) image, a saliency detection method based on saliency potential energy (SPE) is proposed. With a detection, filtration and backtracking strategy, the texture, shape and colour of the UAV RS image are comprehensively and numerally analysed by the SPE to detect the salient man-made objects. Both qualitative and quantitative evaluations have indicated that, compared to the state-of-art saliency detection methods, our method could achieve better performance with better accuracy and less errors, which prove that our method has great application potential in UAV RS image understanding. © 2018, © 2018 Informa UK Limited, trading as Taylor & Francis Group.},
}

@ARTICLE{Liu2019,
author={Liu, M. and Gai, M. and Lai, S.},
title={Simulating unmanned aerial vehicle flight control and collision detection},
journal={Visual Computing for Industry, Biomedicine, and Art},
year={2019},
volume={2},
number={1},
art_number={5},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85100665651&doi=10.1186%2fs42492-019-0014-9&partnerID=40&md5=32799a06ffbd8551dcde3e6c25d20557},
abstract={An unmanned aerial vehicle (UAV) is a small, fast aircraft with many useful features. It is widely used in military reconnaissance, aerial photography, searches, and other fields; it also has very good practical-application and development prospects. Since the UAV’s flight orientation is easily changeable, its orientation and flight path are difficult to control, leading to its high damage rate. Therefore, UAV flight-control technology has become the focus of attention. This study focuses on simulating a UAV’s flight and orientation control, and detecting collisions between a UAV and objects in a complex virtual environment. The proportional-integral-derivative control algorithm is used to control the orientation and position of the UAV in a virtual environment. A version of the bounding-box method that combines a grid with a k-dimensional tree is adopted in this paper, to improve the system performance and accelerate the collision-detection process. This provides a practical method for future studies on UAV flight position and orientation control, collision detection, etc. © 2019, The Author(s).},
}

@CONFERENCE{Luo2019421,
author={Luo, Y. and Shen, J. and Zhang, Y. and Guo, C. and Lv, H.},
title={Health Detection Technology Used on Unmanned Aerial Vehicle Based on Optical Fiber},
journal={2019 16th International Computer Conference on Wavelet Active Media Technology and Information Processing, ICCWAMTIP 2019},
year={2019},
pages={421-424},
art_number={9067610},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85084322767&doi=10.1109%2fICCWAMTIP47768.2019.9067610&partnerID=40&md5=bde833cc36b458336f7d9e75b0d0387b},
abstract={At present, many flight tests of the new aircraft must be carried out by means of structural strength test. The method of resistance strain gauge is the effective method to measure strain in the flight test. However, the resistance strain gauge is used to measure strain, some questions occur. The workload of patch, welding line and sealing sheet is large and the efficiency is relatively low. When there are a large number of test points, the number of sensors and power supply wiring is relatively large, and the number of test channels is inevitably increased, resulting in the increase of the volume and weight of the test system. In addition, the resistance strain measurement method is greatly affected by environmental conditions, which affect the measurement accuracy and reliability. These problems are not well solved in the flight test. In the work, fiber Bragg grating sensors and resistance strain gauge are used to jointly monitor and compare the body strain in the loading process of unmanned aerial vehicle loading. The test shows that the fiber Bragg grating sensors can accurately monitor the strain of the unmanned aerial vehicle body with small errors, which demonstrate great potential in combat missions. © 2019 IEEE.},
}

@CONFERENCE{Jena2019284,
author={Jena, K.K. and Mishra, S. and Mishra, S. and Bhoi, S.K.},
title={Unmanned Aerial Vehicle Assisted Bridge Crack Severity Inspection Using Edge Detection Methods},
journal={Proceedings of the 3rd International Conference on I-SMAC IoT in Social, Mobile, Analytics and Cloud, I-SMAC 2019},
year={2019},
pages={284-289},
art_number={9032510},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85083031393&doi=10.1109%2fI-SMAC47947.2019.9032510&partnerID=40&md5=932ade4e3077fe5b7177b1fe5dcaa54e},
abstract={Currently, cracks in bridge is a major problem for the existence of human life. Bridge accident increases due to lack of the surveillance of bridges. The cracks are common in bridges due to frequent running of heavy motor vehicles, natural calamities, etc. However, if the crack width increases it may create problem in transportation system. So, it is essential to regularly monitor the critical positions of bridge by capturing their images through unmanned aerial vehicles (UAVs), surveillance camera, vibration sensors, etc. The captured images are processed to monitor the cracks. In this paper, a UAV based bridge crack inspection model focusing on edge detection (ED) mechanisms is proposed to support the Internet of Things (IoTs) applications. ED refers to the process of identification of edge pixels in an image. The images after taken from the UAVs are transmitted to an Information Center (IC) through internet for processing using ED methods to identify the crack. If the crack width is greater than a threshold then actions are taken for bridge crack (BC) repair or bridge reconstruction. In this methodology, the main work is focused on several BCs using different existing standard ED methods such as sobel, prewitt, roberts, Laplacian of Gaussian (LoG), morphological and canny methods. These methods are implemented in MATLAB R2015b and evaluated using Peak Signal to Noise Ratio (PSNR) and Signal to Noise Ratio (SNR). © 2019 IEEE.},
}

@CONFERENCE{Jena2019324,
author={Jena, K.K. and Bhoi, S.K. and Behera, B.D. and Panda, S. and Sahu, B. and Sahu, R.},
title={A Trust Based False Message Detection Model for Multi-Unmanned Aerial Vehicle Network},
journal={Proceedings of the 3rd International Conference on I-SMAC IoT in Social, Mobile, Analytics and Cloud, I-SMAC 2019},
year={2019},
pages={324-329},
art_number={9032550},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85083030974&doi=10.1109%2fI-SMAC47947.2019.9032550&partnerID=40&md5=735bad9abeb34dbca5440a0a731a14fb},
abstract={Unmanned Aerial Vehicles (UAVs) are increasing in number all over the world as they are very useful as well as effective for the society. UAVs are commonly known as drones, which are being used by different sectors like military, commercial, scientific, recreational, and many more. In order to perform different tasks and responsibilities, communication is considered as an important aspect. A multi-UAV network exchanges real-time messages using UAV-to-UAV (U2U) communication and UAV-to-Infrastructure (U2I) communication. However, a false message will impact navigation, monitoring, and tracking of other drones. In this paper, an event-based reputation model is proposed to filter false event messages. This solution considers two different roles for the same event. A dynamic role-development, reputation, and evaluation mechanism is determined, whether an incoming message is true and trustworthy to other UAVs. By using this, the spreading of false event messages can be prevented in multi-UAV network. Simulation results show that this model performs better in filtering the false event messages. © 2019 IEEE.},
}

@CONFERENCE{Bhoi2019257,
author={Bhoi, S.K. and Jena, K.K. and Jena, A. and Panda, B.C. and Singh, S. and Behera, P.},
title={A reputation deterministic framework for true event detection in unmanned aerial vehicle network (UAVN)},
journal={Proceedings - 2019 International Conference on Information Technology, ICIT 2019},
year={2019},
pages={257-262},
art_number={9031881},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85082868548&doi=10.1109%2fICIT48102.2019.00052&partnerID=40&md5=fbc542176ed271ffe2c3408efbacd104},
abstract={UAVs have enormous application possibilities in In-ternet of Things (IoTs). UAVs provide IoT services to the users by using its sensors, cameras, GPS receivers, etc. for various applications like event detection, mili-tary, security, medicine, and surveillance. These ser-vices need trusted and reliable communication among the nodes. UAVs have a dynamic and distributed archi-tecture because of which they are prone to malicious attacks. Two factors that provide basic security and control to network traffic congestion and network fil-ter are trust and reputation. In this paper, a reputation management framework is proposed. This framework presents a message-node model which checks the real-ness of event messages generated in a network after encountering an event, and it also checks the genuine-ness of the UAV node which reports the event message. This model uses majority voting protocol for deter-mining the truthfulness of event messages. Based on that, reputation is calculated for a message producer. A central hub is introduced which keeps record of all the UAV nodes. Reputation from different recom-menders and a global reputation value is used to calcu-late the node's recommendation bound reputation. Simulation results show that proposed model outper-forms the similarity mining model in terms of reputation value analysis. © 2019 IEEE.},
}

@CONFERENCE{Bhoi2019222,
author={Bhoi, S.K. and Jena, K.K. and Maniharika, G.V. and Muduli, S. and Sahoo, R. and Bhol, D.},
title={Detection of intended and unintended misbehaviors in unmanned aerial vehicle network (UAVN)},
journal={Proceedings - 2019 International Conference on Information Technology, ICIT 2019},
year={2019},
pages={222-227},
art_number={9031886},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85082866199&doi=10.1109%2fICIT48102.2019.00046&partnerID=40&md5=b3c079c041b576c44e9308556b99a39e},
abstract={UAV has enormous applications in civil and military domain. Ensuring high level of security in inter UAV communication in a wireless medium is a challenging task. The UAVs participating in the communication network have limited energy and computational power. A UAV can drop a packet showing either it's intended or unintended misbehavior, where intended misbehavior can be observed when a UAV node gets attacked by an attacker or unintended misbehavior can be observed due to the system obligations respectively. In this paper, a trust model is proposed for detecting intended and unintended misbehavior in communication among UAVs. In this model, three factors are considered in order to detect the malicious or bad nodes such as buffer size of each UAV, energy of each UAV and the stability of link between two nodes. This model also includes a method which focuses on the path of a packet from source to destination by using the weight value of each UAV. Simulation is performed on python environment to analyze the performance of the network. It is witnessed that the proposed model has a detection ratio of 94% by outperforming the previously proposed UNION model. © 2019 IEEE.},
}

@CONFERENCE{Liu2019381,
author={Liu, K. and Han, X. and Chen, B.M.},
title={Deep learning based automatic crack detection and segmentation for unmanned aerial vehicle inspections},
journal={IEEE International Conference on Robotics and Biomimetics, ROBIO 2019},
year={2019},
pages={381-387},
art_number={8961534},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85079048568&doi=10.1109%2fROBIO49542.2019.8961534&partnerID=40&md5=9c6a03f0a4738fbaa4258a02fcbe002b},
abstract={Automatic crack detection and segmentation plays a significant role in the whole system of unmanned aerial vehicle inspections. In this paper, we have implemented a deep learning framework for crack detection based on classical network architectures including Alexnet, VGG and Resnet. Moreover, inspired by the feature pyramid network architecture, a hierarchical convolutional neural network (CNN) deep learning framework which is efficient in crack segmentation is also proposed, and the performance of it is compared with other state of the art network architecture. We have summarized the existing crack detection and segmentation datasets and established the largest existing benchmark-dataset on the internet for crack detection and segmentation, which is open-sourced for the research community. Our feature pyramid crack segmentation network is tested on the benchmark-dataset and gives satisfactory segmentation results. A framework for automatic unmanned aerial vehicle inspections is also proposed for the crack inspection tasks of various concrete structures. © 2019 IEEE.},
}

@CONFERENCE{Ambata2019,
author={Ambata, L. and Chavez, A.F. and Devnani, N. and Ingeniero, J. and Paggabao, A.K.},
title={Three-Dimensional Mapping System for Environment and Object Detection on an Unmanned Aerial Vehicle},
journal={2019 IEEE 11th International Conference on Humanoid, Nanotechnology, Information Technology, Communication and Control, Environment, and Management, HNICEM 2019},
year={2019},
art_number={9072891},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85084746787&doi=10.1109%2fHNICEM48295.2019.9072891&partnerID=40&md5=24f495fed7dee213f434a36b824bf666},
abstract={This study aims to solve the problem of multiple devices and methods used in surveying as well as a low-cost alternative to 3D mapping using a LiDAR; which would be used for surveying post-disaster areas. To solve this problem, a system composed of 2D stitching, object detection, 3D mapping, and LiDAR point cloud data processing is created. The study includes utilizing a camera-equipped unmanned aerial vehicle for data gathering of the system. © 2019 IEEE.},
}

@CONFERENCE{Li20193305,
author={Li, C. and Xie, X. and Luo, F.},
title={Obstacle Detection and Path Planning Based on Monocular Vision for Unmanned Aerial Vehicles},
journal={Proceedings - 2019 Chinese Automation Congress, CAC 2019},
year={2019},
pages={3305-3309},
art_number={8996752},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85080099842&doi=10.1109%2fCAC48633.2019.8996752&partnerID=40&md5=bdd1679bb666e2ad664173f576f226ad},
abstract={This article mainly introduces the algorithm design and simulation process of unmanned aerial vehicle obstacle detection and path planning based on monocular vision. In this article, we will first explain the basics of image processing, with focus on the design algorithms and the operations and principles that will be used in simulation experiments in the second half of the article. The subject is the obstacle detection and path planning of drones, so the article divides this topic into two sub-topics. Subtask 1 focuses on solving obstacle detection problems for drones. This paper will use the method of contour detection. Subtask 2 focuses on solving the problem of path planning after unmanned aerial vehicles detect obstacles. This paper uses A∗ path search algorithm. The simulation results show that the algorithm has a good degree of completion, and all the materials used can basically avoid obstacles accurately and plan the relatively safe and shortest optimal path. © 2019 IEEE.},
}

@ARTICLE{Zhao20192296,
author={Zhao, T.-F. and Li, H.-C. and Zhang, G.},
title={Ultraviolet detection and positioning method for unmanned aerial vehicle patrol of power line discharge [无人机巡检电力线放电的紫外探测及定位]},
journal={Guangxue Jingmi Gongcheng/Optics and Precision Engineering},
year={2019},
volume={27},
number={11},
pages={2296-2304},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85076692564&doi=10.3788%2fOPE.20192711.2296&partnerID=40&md5=90d7d3f5aff528195f85af88fb08b1d9},
abstract={As discharge failures caused by problems such as pollution and cracking of transmission facilities have constantly threatened the safety of the transmission network, in this paper, discharge ultraviolet detection technology was first studied. Then, the Photomultiplier Tube (PMT) was used as the detector to design the discharge ultraviolet detection scheme. An ultraviolet detection and localization method for the Unmanned Aerial Vehicle (UAV) inspection of power line discharge was proposed. The PMT was driven by the steering of the steering gear to perform multi-angle detection, the current detection position and detection angle were recorded, and the preliminary positioning coordinates of the discharge point were obtained using the direction-finding cross-positioning method. In order to accurately locate the discharge point, n sets of data were solved to obtain the preliminary positioning coordinates of n(n-1)/2 discharge points. The preliminary positioning coordinates of the discharge point were then removed from the abnormal point and imported into the K-means clustering algorithm. A second solution was applied to obtain the exact coordinates of the discharge point. In the experiment, to test the relationship between the PMT detection angle and discharge ultraviolet signal, θ=90° was selected as the steering angle of the steering gear. Conducting discharge patrol experiments at 18 m, 30 m, and 50 m showed that the positioning error of discharge point are within 9.0%. The experimental results show that the method can meet the need for rapid location of the discharge point when the UAV patrols the power line. © 2019, Science Press. All right reserved.},
}

@ARTICLE{Guzmán-Rabasa20191228,
author={Guzmán-Rabasa, J.A. and López-Estrada, F.R. and González-Contreras, B.M. and Valencia-Palomo, G. and Chadli, M. and Pérez-Patricio, M.},
title={Actuator fault detection and isolation on a quadrotor unmanned aerial vehicle modeled as a linear parameter-varying system},
journal={Measurement and Control (United Kingdom)},
year={2019},
volume={52},
number={9-10},
pages={1228-1239},
note={cited By 22},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85068234843&doi=10.1177%2f0020294018824764&partnerID=40&md5=ec90a118249188eb2f89ef5aa6a0a825},
abstract={This paper presents the design of a fault detection and diagnosis system for a quadrotor unmanned aerial vehicle under partial or total actuator fault. In order to control the quadrotor, the dynamic system is divided in two subsystems driven by the translational and the rotational dynamics, where the rotational subsystem is based on a linear parameter-varying model. A robust linear parameter-varying observer applied to the rotational subsystem is considered to detect actuator faults, which can occur as total failures (loss of a propeller or a motor) or partial faults (degradation). Furthermore, fault diagnosis is done by analyzing the displacements of the roll and pitch angles. Numerical experiments are carried out in order to illustrate the effectiveness of the proposed methodology. © The Author(s) 2019.},
}

@ARTICLE{Sharma2019159,
author={Sharma, A. and Kiragi, V.},
title={An enhanced deep learning & artificial intelligence vehicle detection method from unmanned aerial vehicles imagery},
journal={International Journal of Advanced Science and Technology},
year={2019},
volume={28},
number={12},
pages={159-168},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85080133797&partnerID=40&md5=0c2e8ff8a6c718eeda5331620718d17e},
abstract={For the use in many applications like civil, recreational and commercial areas, military due to indoor and outdoor use, vertical takeoff and vertical landing and high maneuverability the unmanned aerial vehicles are becoming popular platform for research. It has been developing very powerful, light and small embedding systems in recent innovations. For detecting the vehicles by integrating these types of embedding systems many real time applications can run on platform of unmanned aerial vehicle [1]. In this paper it studies the Deep Learning method for detecting the vehicles from unmanned aerial vehicle imaginary. © 2019 SERSC.},
}

@ARTICLE{GarcíaRubio2019,
author={García Rubio, V. and Rodrigo Ferrán, J.A. and Menéndez García, J.M. and Sánchez Almodóvar, N. and Lalueza Mayordomo, J.M. and Álvarez, F.},
title={Automatic Change Detection System over Unmanned Aerial Vehicle Video Sequences Based on Convolutional Neural Networks},
journal={Sensors (Basel, Switzerland)},
year={2019},
volume={19},
number={20},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85073630005&doi=10.3390%2fs19204484&partnerID=40&md5=026e2de4e98350fdd01e1cc701f354af},
abstract={In recent years, the use of unmanned aerial vehicles (UAVs) for surveillance tasks has increased considerably. This technology provides a versatile and innovative approach to the field. However, the automation of tasks such as object recognition or change detection usually requires image processing techniques. In this paper we present a system for change detection in video sequences acquired by moving cameras. It is based on the combination of image alignment techniques with a deep learning model based on convolutional neural networks (CNNs). This approach covers two important topics. Firstly, the capability of our system to be adaptable to variations in the UAV flight. In particular, the difference of height between flights, and a slight modification of the camera's position or movement of the UAV because of natural conditions such as the effect of wind. These modifications can be produced by multiple factors, such as weather conditions, security requirements or human errors. Secondly, the precision of our model to detect changes in diverse environments, which has been compared with state-of-the-art methods in change detection. This has been measured using the Change Detection 2014 dataset, which provides a selection of labelled images from different scenarios for training change detection algorithms. We have used images from dynamic background, intermittent object motion and bad weather sections. These sections have been selected to test our algorithm's robustness to changes in the background, as in real flight conditions. Our system provides a precise solution for these scenarios, as the mean F-measure score from the image analysis surpasses 97%, and a significant precision in the intermittent object motion category, where the score is above 99%.},
}

@ARTICLE{Rubio2019,
author={Rubio, V.G. and Ferrán, J.A.R. and García, J.M.M. and Almodóvar, N.S. and Mayordomo, J.M.L. and Álvarez, F.},
title={Automatic change detection system over unmanned aerial vehicle video sequences based on convolutional neural networks},
journal={Sensors (Switzerland)},
year={2019},
volume={19},
number={20},
art_number={4484},
note={cited By 6},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85073684832&doi=10.3390%2fs19204484&partnerID=40&md5=e4508c3fe736e2d5437e95d16421a707},
abstract={In recent years, the use of unmanned aerial vehicles (UAVs) for surveillance tasks has increased considerably. This technology provides a versatile and innovative approach to the field. However, the automation of tasks such as object recognition or change detection usually requires image processing techniques. In this paper we present a system for change detection in video sequences acquired by moving cameras. It is based on the combination of image alignment techniques with a deep learning model based on convolutional neural networks (CNNs). This approach covers two important topics. Firstly, the capability of our system to be adaptable to variations in the UAV flight. In particular, the difference of height between flights, and a slight modification of the camera’s position or movement of the UAV because of natural conditions such as the effect of wind. These modifications can be produced by multiple factors, such as weather conditions, security requirements or human errors. Secondly, the precision of our model to detect changes in diverse environments, which has been compared with state-of-the-art methods in change detection. This has been measured using the Change Detection 2014 dataset, which provides a selection of labelled images from different scenarios for training change detection algorithms. We have used images from dynamic background, intermittent object motion and bad weather sections. These sections have been selected to test our algorithm’s robustness to changes in the background, as in real flight conditions. Our system provides a precise solution for these scenarios, as the mean F-measure score from the image analysis surpasses 97%, and a significant precision in the intermittent object motion category, where the score is above 99%. © 2019 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@CONFERENCE{Ponce-Corona2019,
author={Ponce-Corona, E. and Sanchez, M.G. and Fajardo-Delgado, D. and Castro, W. and De-La-Torre, M. and Avila-George, H.},
title={Detection of vegetation using unmanned aerial vehicles images: A systematic review},
journal={2019 8th International Conference on Software Process Improvement, CIMPS 2019 - Applications in Software Engineering},
year={2019},
art_number={9082434},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85084973486&doi=10.1109%2fCIMPS49236.2019.9082434&partnerID=40&md5=829ffdec53af4fb156b064c98b21690e},
abstract={In recent years, the use of unmanned aerial vehicles for the development of agricultural and forestry applications has become popular. Given the importance of plants in both rural and urban environments, the extraction of information from data obtained by remote sensing is a highly relevant area of research. Such information is vital in urban and rural planning activities, the establishment of sustainable ecological niches, estimation of crop yields, the realization of forest inventories, the supervision of agricultural management systems, and some other agricultural applications. In this paper, we present a systematic review of the literature regarding the use of unmanned aerial vehicles in applications related to the detection of vegetation and plants inventory. Likewise, an analysis of the software used and the main computational and statistical techniques for the processing of images taken from unmanned aerial vehicles is made. © 2019 IEEE.},
}

@CONFERENCE{Wu20191201,
author={Wu, Z. and Suresh, K. and Narayanan, P. and Xu, H. and Kwon, H. and Wang, Z.},
title={Delving into robust object detection from unmanned aerial vehicles: A deep nuisance disentanglement approach},
journal={Proceedings of the IEEE International Conference on Computer Vision},
year={2019},
volume={2019-October},
pages={1201-1210},
art_number={9008566},
note={cited By 16},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85081552827&doi=10.1109%2fICCV.2019.00129&partnerID=40&md5=ae79d36af723ba62ac094b6bb6a8bb76},
abstract={Object detection from images captured by Unmanned Aerial Vehicles (UAVs) is becoming increasingly useful. Despite the great success of the generic object detection methods trained on ground-to-ground images, a huge performance drop is observed when they are directly applied to images captured by UAVs. The unsatisfactory performance is owing to many UAV-specific nuisances, such as varying flying altitudes, adverse weather conditions, dynamically changing viewing angles, etc. Those nuisances constitute a large number of fine-grained domains, across which the detection model has to stay robust. Fortunately, UAVs will record meta-data that depict those varying attributes, which are either freely available along with the UAV images, or can be easily obtained. We propose to utilize those free meta-data in conjunction with associated UAV images to learn domain-robust features via an adversarial training framework dubbed Nuisance Disentangled Feature Transform (NDFT), for the specific challenging problem of object detection in UAV images, achieving a substantial gain in robustness to those nuisances. We demonstrate the effectiveness of our proposed algorithm, by showing state-of-the- art performance (single model) on two existing UAV-based object detection benchmarks. The code is available at https://github.com/TAMU-VITA/UAV-NDFT. © 2019 IEEE.},
}

@CONFERENCE{Qi2019,
author={Qi, Y. and Shi, H. and Li, N. and Li, Y. and Zhou, H.},
title={Vehicle Detection Under Unmanned Aerial Vehicle Based on Improved YOLOv3},
journal={Proceedings - 2019 12th International Congress on Image and Signal Processing, BioMedical Engineering and Informatics, CISP-BMEI 2019},
year={2019},
art_number={8966013},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85079198776&doi=10.1109%2fCISP-BMEI48845.2019.8966013&partnerID=40&md5=c58d72d5d09854d93eac262c495902e9},
abstract={Under the unmanned aerial vehicle (UAV), the ground vehicle target is generally small in size, and the background information is more prominent. Therefore, we propose an improved detection model based on YOLOv3. First, in order to make full use of network feature information, we add connections between the front and back layers of the network to improve the information flow in the deep network. These layers are constructed as a loop and alternately updated structure, which reduces the depth of the network and improve the reuse of features. In addition, on the one hand, considering that the vehicle target is small in the UAV scene, the imbalance between the foreground and the background category is extremely serious. We improve the loss function and reduce the weight of the easily discernible background confidence loss, so that the model pays more attention to the hard samples. On the other hand, the improved IoU index is used as the loss function of regression task to improve the accuracy of small target detection. Experiments on the vehicle dataset of UAV show that the detection accuracy of the proposed algorithm is improved without reducing the rate. © 2019 IEEE.},
}

@CONFERENCE{Xiang2019,
author={Xiang, C. and Shi, H. and Li, N. and Ding, M. and Zhou, H.},
title={Pedestrian Detection Under Unmanned Aerial Vehicle an Improved Single-Stage Detector Based on RetinaNet},
journal={Proceedings - 2019 12th International Congress on Image and Signal Processing, BioMedical Engineering and Informatics, CISP-BMEI 2019},
year={2019},
art_number={8965666},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85079123531&doi=10.1109%2fCISP-BMEI48845.2019.8965666&partnerID=40&md5=ebd7f13cc576c2e9c205a6c07d14cfe5},
abstract={As a kind of single-stage detection network, RetinaNet has excellent performance in object detection, but it still has some difficulties in small object detection in unmanned aerial vehicle (UAV) images. Based on RetinaNet, this paper uses improved ResNet50 as backbone to extract features. We increase the number of anchor ratios, but reduce the number of anchor scales so that the number of anchors won't increase too much. We add the shallower features to predict smaller targets. We also add Receptive Field Block after each predicted feature to increase the receptive field. We have changed the values of parameters in the loss function for better detection performance. The improved model effectively increases the detection rate of small targets so that it can be applied to pedestrian detection under UAV. In our UAV pedestrian dataset, the improved model increases average precision (AP) from 51.29% to 84.05%. © 2019 IEEE.},
}

@CONFERENCE{Chen2019,
author={Chen, S. and Lu, X. and Li, Y. and Wu, R.},
title={A Convolutional Neural Network for Real-Time Vehicle Detection Under the Unmanned Aerial Vehicle Platform},
journal={Proceedings - 2019 12th International Congress on Image and Signal Processing, BioMedical Engineering and Informatics, CISP-BMEI 2019},
year={2019},
art_number={8965752},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85079115094&doi=10.1109%2fCISP-BMEI48845.2019.8965752&partnerID=40&md5=890e2d15b44b40031deca82546dd2f0e},
abstract={The detection of vehicles under the unmanned aerial vehicle platform has several technical challenges. Compared with surveillance videos, aerial videos have more complex background and broader range which lead to larger space for searching. It is also difficult to build a effective background model due to the movement of the unmanned aerial vehicle. The low performance of development board on the aerial vehicle also make it difficult to perform real-time detection. We proposes a convolutional neural network to carry out real-time detection of vehicles under the unmanned aerial vehicle platform. Multi-scale anchor design is carried out to improve the adaptability to different vehicles and the algorithm is time optimized based on the binary weight network. As a consequence, our algorithm runs at 28.8 FPS with average precision of 91.2% under the unmanned aerial vehicle platform. © 2019 IEEE.},
}

@CONFERENCE{Kharchenko201971,
author={Kharchenko, V. and Kuzmenko, N. and Kukush, A. and Ostroumov, I.},
title={Kernel Density Estimation for Foreground Detection in Dynamic Video Processing for Unmanned Aerial Vehicle Application},
journal={2019 IEEE 5th International Conference Actual Problems of Unmanned Aerial Vehicles Developments, APUAVD 2019 - Proceedings},
year={2019},
pages={71-74},
art_number={8943857},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85078252451&doi=10.1109%2fAPUAVD47061.2019.8943857&partnerID=40&md5=19f828b27918fcc5914723e894c56ed2},
abstract={The paper considers aspects of Unmanned Aerial Vehicle video stream foreground detection based on computer vision and artificial intelligence. Nonparametric approach for background subtraction based on kernel model was used as the most appropriate for usage in dynamic environment. One of the key elements of the kernel density estimation is bandwidth selection that significantly effects results of image segmentation and object detection. Several approaches of bandwidth selection and their impact on object detection performance is investigated in the paper. Otsu's method was used for threshold selection for image segmentation. © 2019 IEEE.},
}

@ARTICLE{Jurecka2019,
author={Jurecka, M. and Miziński, B. and Niedzielski, T.},
title={Impact of boosting saturation on automatic human detection in imagery acquired by unmanned aerial vehicles},
journal={Journal of Applied Remote Sensing},
year={2019},
volume={13},
number={4},
art_number={044525},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85077773367&doi=10.1117%2f1.JRS.13.044525&partnerID=40&md5=18fa63ee906e24bc2bc11d19fb9f6c18},
abstract={We aim to investigate a potential impact of boosting saturation of aerial imagery on the performance of unsupervised human detection algorithms. The study is empirical since it is based on processing photographs taken during a full year experiment in the Izerskie Mountains (southwestern Poland) by a consumer-grade Canon S110 camera mounted onboard eBee, a fixed-wing micro-unmanned aerial vehicle (UAV). In the preliminary analysis, we used a few basic color adjustments (sharpening, hue-saturation-luminance, contrast, saturation, and vibrance) to process UAV-taken photographs prior to the automated human detection with the nested k-means algorithm. We found that saturation boost is an image preprocessing method that may potentially improve the performance of human detection. In the actual analysis, we investigate only the saturation effect by employing four saturation modification schemes (two versions of enhancements of unusual colors, additive boost of saturation, and multiplicative boost of saturation) and three human detection algorithms [three-dimensional (3-D) nested k-means on RGB, two-dimensional nested k-means on hue-saturation-value, morphological operations of erosion, and dilation with thresholding]. All the studied saturation boost techniques increase detection rates of the 3-D nested k-means on RGB, with particularly meaningful improvement for images acquired in the spring. Morphological operations of erosion and dilation are not found to be skillful in detecting persons. However, their performance is improved after the initial preprocessing by the original or modified enhancement of unusual colors. © 2019 Society of Photo-Optical Instrumentation Engineers (SPIE).},
}

@ARTICLE{Neupane2019,
author={Neupane, B. and Horanont, T. and Hung, N.D.},
title={Deep learning based banana plant detection and counting using high-resolution red-green-blue (RGB) images collected from unmanned aerial vehicle (UAV)},
journal={PLoS ONE},
year={2019},
volume={14},
number={10},
art_number={e0223906},
note={cited By 35},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85073625556&doi=10.1371%2fjournal.pone.0223906&partnerID=40&md5=65a6293b4ad9bc22b9bf4e021d145600},
abstract={The production of banana—one of the highly consumed fruits—is highly affected due to loss of certain number of banana plants in an early phase of vegetation. This affects the ability of farmers to forecast and estimate the production of banana. In this paper, we propose a deep learning (DL) based method to precisely detect and count banana plants on a farm exclusive of other plants, using high resolution RGB aerial images collected from Unmanned Aerial Vehicle (UAV). An attempt to detect the plants on the normal RGB images resulted less than 78.8% recall for our sample images of a commercial banana farm in Thailand. To improve this result, we use three image processing methods—Linear Contrast Stretch, Synthetic Color Transform and Triangular Greenness Index—to enhance the vegetative properties of orthomosaic, generating multiple variants of orthomosaic. Then we separately train a parameter-optimized Convolutional Neural Network (CNN) on manually interpreted banana plant samples seen on each image variants, to produce multiple results of detection on our region of interest. 96.4%, 85.1% and 75.8% of plants were correctly detected on three of our dataset collected from multiple altitude of 40, 50 and 60 meters, of same farm. Further discussion on results obtained from combination of multiple altitude variants are also discussed later in the research, in an attempt to find better altitude combination for data collection from UAV for the detection of banana plants. The results showed that merging the detection results of 40 and 50 meter dataset could detect the plants missed by each other, increasing recall upto 99%. © 2019 Neupane et al. This is an open access article distributed under the terms of the Creative Commons Attribution License, which permits unrestricted use, distribution, and reproduction in any medium, provided the original author and source are credited.},
}

@ARTICLE{Khan2019,
author={Khan, S. and Liew, C.F. and Yairi, T. and McWilliam, R.},
title={Unsupervised anomaly detection in unmanned aerial vehicles},
journal={Applied Soft Computing Journal},
year={2019},
volume={83},
art_number={105650},
note={cited By 14},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85069952423&doi=10.1016%2fj.asoc.2019.105650&partnerID=40&md5=e0a2f3c30ed10e3a6d0508adda42068f},
abstract={A real-time anomaly detection solution indicates a continuous stream of operational and labelled data that must satisfy several resources and latency requirements. Traditional solutions to the problem rely heavily on well-defined features and prior supervised knowledge, where most techniques refer to hand-crafted rules derived from known conditions. While successful in controlled situations, these rules assume that good data is available for them to detect anomalies; indicating that these rules will fail to generalise beyond known scenarios. To investigate these issues, current literature is examined for solutions that can be used to detect known and unknown anomalous instances whilst functioning as an out-of-the-box approach for efficient decision-making. The applicability of the isolation forest is discussed for engineering applications using the Aero-Propulsion System Simulation dataset as a benchmark where it is shown to outperform other unsupervised distance-based approaches. Also, the authors have carried out real-time experiments on an unmanned aerial vehicle to highlight further applications of the method. Finally, some conclusions are drawn concerning its simplicity and robustness in handling diagnostic problems. © 2019},
}

@ARTICLE{Han2019,
author={Han, S. and Yoo, J. and Kwon, S.},
title={Real-time vehicle-detection method in bird-view unmanned-aerial-vehicle imagery},
journal={Sensors (Switzerland)},
year={2019},
volume={19},
number={18},
art_number={3958},
note={cited By 6},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85072540941&doi=10.3390%2fs19183958&partnerID=40&md5=360ed993cfdf0563b92674eab26f727e},
abstract={Vehicle detection is an important research area that provides background information for the diversity of unmanned-aerial-vehicle (UAV) applications. In this paper, we propose a vehicle-detection method using a convolutional-neural-network (CNN)-based object detector. We design our method, DRFBNet300, with a Deeper Receptive Field Block (DRFB) module that enhances the expressiveness of feature maps to detect small objects in the UAV imagery. We also propose the UAV-cars dataset that includes the composition and angular distortion of vehicles in UAV imagery to train our DRFBNet300. Lastly, we propose a Split Image Processing (SIP) method to improve the accuracy of the detection model. Our DRFBNet300 achieves 21 mAP with 45 FPS in the MS COCO metric, which is the highest score compared to other lightweight single-stage methods running in real time. In addition, DRFBNet300, trained on the UAV-cars dataset, obtains the highest AP score at altitudes of 20-50 m. The gap of accuracy improvement by applying the SIP method became larger when the altitude increases. The DRFBNet300 trained on the UAV-cars dataset with SIP method operates at 33 FPS, enabling real-time vehicle detection. © 2019 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@CONFERENCE{D'Apolito2019,
author={D'Apolito, F. and Sulzbachner, C. and Bruckmueller, F.},
title={A Multiple Hypothesis Tracking Approach to Collision Detection for Unmanned Aerial Vehicles},
journal={AIAA/IEEE Digital Avionics Systems Conference - Proceedings},
year={2019},
volume={2019-September},
art_number={9081705},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85084730942&doi=10.1109%2fDASC43569.2019.9081705&partnerID=40&md5=82be393cd65fb27e31d082718aff803e},
abstract={It is obvious that future unmanned aerial vehicle (UAV) applications will have a high degree of automation, up to autonomy, and will be integrated into civil airspace to go beyond line of sight. To ensure the safe operation of these systems, new technologies are required. Currently, the regulatory and technological frameworks are insufficient. For instance, there are no standards for sensors required to detect obstacles and avoid possible collisions. It is evident that data from several sensors need to be combined to obtain a robust environmental map in order to cope with the high standards of aviation. This paper aims to introduce a Multiple Hypothesis Tracking (MHT) approach to multi-sensor data fusion for future collision avoidance systems. The data from several sensors are merged to obtain new and more accurate measurement data to capture the environment more robustly. The sensors consist of several optical and thermal sensors, radar and transponder systems. This combined measurement data is processed by an avoidance algorithm to calculate avoidance maneuvers. So far, simulations and ground based tests have shown that the implemented MHT approach provides qualitatively better results than conventional probabilistic data fusion approaches. In a next step, test flights will be performed to evaluate the proposed MHT data fusion approach in an airborne environment. © 2019 IEEE.},
}

@ARTICLE{Buters20191,
author={Buters, T. and Belton, D. and Cross, A.},
title={Seed and seedling detection using unmanned aerial vehicles and automated image classification in the monitoring of ecological recovery},
journal={Drones},
year={2019},
volume={3},
number={3},
pages={1-16},
art_number={53},
note={cited By 12},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85082749769&doi=10.3390%2fdrones3030053&partnerID=40&md5=0a2cf1aa52b9e2581fad51890facc269},
abstract={Monitoring is a crucial component of ecological recovery projects, yet it can be challenging to achieve at scale and during the formative stages of plant establishment. The monitoring of seeds and seedlings, which represent extremely vulnerable stages in the plant life cycle, is particularly challenging due to their diminutive size and lack of distinctive morphological characteristics. Counting and classifying seedlings to species level can be time-consuming and extremely difficult, and there is a need for technological approaches offering restoration practitioners with fine-resolution, rapid and scalable plant-based monitoring solutions. Unmanned aerial vehicles (UAVs) offer a novel approach to seed and seedling monitoring, as the combination of high-resolution sensors and low flight altitudes allow for the detection and monitoring of small objects, even in challenging terrain and in remote areas. This study utilized low-altitude UAV imagery and an automated object-based image analysis software to detect and count target seeds and seedlings from a matrix of non-target grasses across a variety of substrates reflective of local restoration substrates. Automated classification of target seeds and target seedlings was achieved at accuracies exceeding 90% and 80%, respectively, although the classification accuracy decreased with increasing flight altitude (i.e., decreasing image resolution) and increasing background surface complexity (increasing percentage cover of non-target grasses and substrate surface texture). Results represent the first empirical evidence that small objects such as seeds and seedlings can be classified from complex ecological backgrounds using automated processes from UAV-imagery with high levels of accuracy. We suggest that this novel application of UAV use in ecological monitoring offers restoration practitioners an excellent tool for rapid, reliable and non-destructive early restoration trajectory assessment. © 2019 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@ARTICLE{Wang2019,
author={Wang, J. and Simeonova, S. and Shahbazi, M.},
title={Orientation- and scale-invariant multi-vehicle detection and tracking from unmanned aerial videos},
journal={Remote Sensing},
year={2019},
volume={11},
number={18},
art_number={2155},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85072641252&doi=10.3390%2frs11182155&partnerID=40&md5=a91be4a1d1bb20f9382bba94da653c20},
abstract={Along with the advancement of light-weight sensing and processing technologies, unmanned aerial vehicles (UAVs) have recently become popular platforms for intelligent traffic monitoring and control. UAV-mounted cameras can capture traffic-flow videos from various perspectives providing a comprehensive insight into road conditions. To analyze the traffic flow from remotely captured videos, a reliable and accurate vehicle detection-and-tracking approach is required. In this paper, we propose a deep-learning framework for vehicle detection and tracking from UAV videos for monitoring traffic flow in complex road structures. This approach is designed to be invariant to significant orientation and scale variations in the videos. The detection procedure is performed by fine-tuning a state-of-the-art object detector, You Only Look Once (YOLOv3), using several custom-labeled traffic datasets. Vehicle tracking is conducted following a tracking-by-detection paradigm, where deep appearance features are used for vehicle re-identification, and Kalman filtering is used for motion estimation. The proposed methodology is tested on a variety of real videos collected by UAVs under various conditions, e.g., in late afternoons with long vehicle shadows, in dawn with vehicles lights being on, over roundabouts and interchange roads where vehicle directions change considerably, and from various viewpoints where vehicles' appearance undergo substantial perspective distortions. The proposed tracking-by-detection approach performs efficiently at 11 frames per second on color videos of 2720p resolution. Experiments demonstrated that high detection accuracy could be achieved with an average F1-score of 92.1%. Besides, the tracking technique performs accurately, with an average multiple-object tracking accuracy (MOTA) of 81.3%. The proposed approach also addressed the shortcomings of the state-of-the-art in multi-object tracking regarding frequent identity switching, resulting in a total of only one identity switch over every 305 tracked vehicles. © 2019 by the authors.},
}

@ARTICLE{Lee2019,
author={Lee, W.Y. and Park, M. and Hyun, C.-U.},
title={Detection of two Arctic birds in Greenland and an endangered bird in Korea using RGB and thermal cameras with an unmanned aerial vehicle (UAV)},
journal={PLoS ONE},
year={2019},
volume={14},
number={9},
art_number={e0222088},
note={cited By 6},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85071741874&doi=10.1371%2fjournal.pone.0222088&partnerID=40&md5=e40fa041905530823a5f086c04d8d659},
abstract={Unmanned aerial vehicles (UAVs), so-called ‘drones’, have been widely used to monitor wild animals. Here, we tested a UAV with red, green, and blue (RGB) and thermal cameras to detect free-living birds in a high Arctic region in North Greenland and in a restricted area in the Republic of Korea. Small flocks of molting pink-footed geese (Anser brachyrhynchus) near sea ice and incubating common ringed plovers (Charadrius hiaticula) in the Arctic environment were chosen for the RGB and thermal image studies. From the acquired images, we built mosaicked RGB images and coregistered thermal images, and estimated the animal shapes. Our results showed that geese were discriminated in both RGB and thermal images with water and sea ice backgrounds. Incubating plover bodies were not distinguished in RGB images due to their cryptic coloration, but they were detected in thermal images with cold background areas in the Arctic environment. We further conducted a blind survey in a restricted area under military control in Korea near the breeding sites of black-faced spoonbill (Platalea minor), which is an endangered species. From UAV flights with RGB and thermal cameras operated out of the restricted area, we acquired images of white objects in the mudflats and verified that the objects were resting spoonbills by watching the birds. We suggest that thermal cameras and UAVs can be applied to monitor animals in extreme environments and in restricted areas and help researchers find cryptic wader nests. © 2019 Lee et al. This is an open access article distributed under the terms of the Creative Commons Attribution License, which permits unrestricted use, distribution, and reproduction in any medium, provided the original author and source are credited.},
}

@ARTICLE{Esfahlani201942,
author={Esfahlani, S.S.},
title={Mixed reality and remote sensing application of unmanned aerial vehicle in fire and smoke detection},
journal={Journal of Industrial Information Integration},
year={2019},
volume={15},
pages={42-49},
note={cited By 19},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85064892700&doi=10.1016%2fj.jii.2019.04.006&partnerID=40&md5=c2698a35439578d79c4052ec7f3293da},
abstract={This paper proposes the development of a system incorporating inertial measurement unit (IMU), a consumer-grade digital camera and a fire detection algorithm simultaneously with a nano Unmanned Aerial Vehicle (UAV) for inspection purposes. The video streams are collected through the monocular camera and navigation relied on the state-of-the-art indoor/outdoor Simultaneous Localisation and Mapping (SLAM) system. It implements the robotic operating system (ROS) and computer vision algorithm to provide a robust, accurate and unique inter-frame motion estimation. The collected onboard data are communicated to the ground station and used the SLAM system to generate a map of the environment. A robust and efficient re-localization was performed to recover from tracking failure, motion blur, and frame lost in the data received. The fire detection algorithm was deployed based on the color, movement attributes, temporal variation of fire intensity and its accumulation around a point. The cumulative time derivative matrix was utilized to analyze the frame-by-frame changes and to detect areas with high-frequency luminance flicker (random characteristic). Color, surface coarseness, boundary roughness, and skewness features were perceived as the quadrotor flew autonomously within the clutter and congested area. Mixed Reality system was adopted to visualize and test the proposed system in a physical environment, and the virtual simulation was conducted through the Unity game engine. The results showed that the UAV could successfully detect fire and flame, autonomously fly towards and hover around it, communicate with the ground station and simultaneously generate a map of the environment. There was a slight error between the real and virtual UAV calibration due to the ground truth data and the correlation complexity of tracking real and virtual camera coordinate frames. © 2019},
}

@ARTICLE{Jiao20191300,
author={Jiao, Z. and Jia, G. and Cai, Y.},
title={A new approach to oil spill detection that combines deep learning with unmanned aerial vehicles},
journal={Computers and Industrial Engineering},
year={2019},
volume={135},
pages={1300-1311},
note={cited By 22},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85056668357&doi=10.1016%2fj.cie.2018.11.008&partnerID=40&md5=f9de9231e870bbff79fbedceb7da6df0},
abstract={This study presents a novel approach to automatic oil spill detection, using unmanned aerial vehicle (UAV) images to realize intelligent control in oil production. Despite considerable effort, oil spills still cannot be detected automatically and effectively due to the complexity of the real production environment, which forces oil enterprises to manually inspect facilities and detect oil spills. To solve the problem, we propose an approach consisting of UAVs, deep learning and traditional algorithms—an approach which divides the oil spill detection task into three independent sub-tasks. First, we constructed a model based on the deep convolutional neural network, which can quickly detect the suspected oil spill area in images to ensure there are no omissions. Second, to remove other obstacles in the images, we adjusted the Otsu algorithm to filter the detection results, which improves precision while not affecting the recall rate. Third, the Maximally Stable Extremal Regions algorithm was used to obtain the detail polygon region from the detection box, thus automatically evaluating the severity of the oil spill. Experiments showed that our method could solve problems effectively, reducing the cost of oil spill detection by 57.2% when compared with the traditional manual inspection process. © 2018 Elsevier Ltd},
}

@CONFERENCE{Zhao2019,
author={Zhao, X. and Zhao, J. and Zheng, X. and Cheng, J. and Yi, Z.},
title={Feasibility analysis of laser detection and positioning for unmanned aerial vehicles},
journal={IOP Conference Series: Materials Science and Engineering},
year={2019},
volume={569},
number={3},
art_number={032010},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85071871276&doi=10.1088%2f1757-899X%2f569%2f3%2f032010&partnerID=40&md5=1efefc92407e361fd63bdf7ed429b732},
abstract={In order to carry out effective anti-reconnaissance for unmanned aerial vehicles (UAV), the feasibility of effective monitoring of UAV by laser detection system has been analyzed. The models of laser transmitting and receiving system and the photoelectric imaging system on UAV are established. The characteristics of specular scattering and focal plane reflection of UAV imaging lens are simulated. Taking the UAV located at a height of 10,000 m as an example, the feasibility of the application of two detection systems under reflected light has been analyzed. The range of incident angle of the detection laser, the distribution characteristics of light intensity on the photosensitive surface of the detection system and the variation characteristics of return light of the detection laser during dynamic scanning have been obtained respectively. The results show that the focal plane reflected light intensity of the UAV imaging lens is much higher than that of the specular scattered light intensity, and has a good return characteristic. Within the field coverage of the UAV imaging system, the focus plane reflected light can be used to effectively detect and locate the UAV target. © Published under licence by IOP Publishing Ltd.},
}

@ARTICLE{Bae2019354,
author={Bae, S. and Yu, J. and Wang, L. and Kim, J. and Park, C.},
title={Experiments on unmanned aerial vehicle survey for detection of micro beach features},
journal={Journal of Coastal Research},
year={2019},
volume={90},
number={sp1},
pages={354-361},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85087153081&doi=10.2112%2fSI90-045.1&partnerID=40&md5=61c38165584fc767c51f8c1198588840},
abstract={This study tested the effectiveness of using UAV point clouds at different densities to delineate micro beach features. A profile-based method was applied to three different types of geometric patterns of ripples: featureless, regular pattern, and irregular pattern. A terrestrial laser scanner (TLS) based profile was used as the baseline. In general, the overall RMSE between TLS-based profile and UAV-based profiles increased with UAV flight altitude. For the featureless test zone, the UAV beach profile matched the TLS profile with acceptable errors for all three test flight altitudes. In the irregular ripple area, UAV profiles showed much lower RMSE than the regular ripple area. Furthermore, in the irregular ripple area, the UAV profiles captured more extreme elevation points than in the regular ripple area. The results suggest that in beach areas with an irregular spatial pattern of features, UAV surveys could take higher flight altitudes to achieve the same level of accuracy as in an area with a regular pattern of features. This study proved that UAV-based elevation surveys could achieve high-level accuracy with controlled flight heights and could replace the costly TLS-based surveys. © Coastal Education and Research Foundation, Inc. 2019.},
}

@ARTICLE{Ficapal2019,
author={Ficapal, A. and Mutis, I.},
title={Framework for the detection, diagnosis, and evaluation of thermal bridges using infrared thermography and unmanned aerial vehicles},
journal={Buildings},
year={2019},
volume={9},
number={8},
art_number={179},
note={cited By 9},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85071173189&doi=10.3390%2fbuildings9080179&partnerID=40&md5=dbc0570b4c0d8a365813fd414b85fde9},
abstract={The glass curtain wall system is an architectural, functional innovation where failures of insulation systems create areas of reduced resistance to heat transfer-thermal bridges-during a building's operational lifetime. These failures enable energy flows that trigger unanticipated temperature changes and increased energy consumption, ultimately damaging the façade structure and directly impacting occupants. Our study aims to design and test an innovative method for rapidly identifying thermal bridges in façade systems, with minimum or no occupant disturbance. The research focus is in the classification of damage as either a local failure or as being related to a poor systematic construction/assembly. A nontraditional approach is adopted to survey an entire fully operational building using infrared thermography and an unmanned aerial vehicle (UAV) using a noncontact infrared camera mounted on and operated from theUAV. The system records the emissivity of the façade materials and calculates the thermal radiation to estimate localized temperatures. The system records thermal radiation readings which are analyzed using graphs to be compared with the American Society of Heating, Refrigerating and Air Conditioning Engineers (ASHRAE) standards, under ideal conditions using the THERM software. The results enable discussion relating to the most common failure areas for existing structures, facilitating the identification of focus areas for the improvement of construction methods through improved processes. © 2019 by the authors.},
}

@ARTICLE{Yeom2019,
author={Yeom, S. and Cho, I.-J.},
title={Detection and tracking of moving pedestrians with a small unmanned aerial vehicle},
journal={Applied Sciences (Switzerland)},
year={2019},
volume={9},
number={16},
art_number={3359},
note={cited By 12},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85070917674&doi=10.3390%2fapp9163359&partnerID=40&md5=240979260de3ddd4ff04823f6d3cd754},
abstract={Small unmanned aircraft vehicles (SUAVs) or drones are very useful for visual detection and tracking due to their efficiency in capturing scenes. This paper addresses the detection and tracking of moving pedestrians with an SUAV. The detection step consists of frame subtraction, followed by thresholding, morphological filter, and false alarm reduction, taking into consideration the true size of targets. The center of the detected area is input to the next tracking stage. Interacting multiple model (IMM) filtering estimates the state of vectors and covariance matrices, using multiple modes of Kalman filtering. In the experiments, a dozen people and one car are captured by a stationary drone above the road. The Kalman filter and the IMM filter with two or three modes are compared in the accuracy of the state estimation. The root-mean squared errors (RMSE) of position and velocity are obtained for each target and show the good accuracy in detecting and tracking the target position-the average detection rate is 96.5%. When the two-mode IMM filter is used, the minimum average position and velocity RMSE obtained are around 0.8 m and 0.59 m/s, respectively. © 2019 by the authors.},
}

@CONFERENCE{Zhang20191630,
author={Zhang, S. and Chen, B. and Wang, R. and Wang, J. and Zhong, L. and Gao, B.},
title={Unmanned Aerial Vehicle (UAV) Vision-based Detection of Power Line Poles by CPU-based Deep Learning Method},
journal={9th IEEE International Conference on Cyber Technology in Automation, Control and Intelligent Systems, CYBER 2019},
year={2019},
pages={1630-1634},
art_number={9066764},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85084291683&doi=10.1109%2fCYBER46603.2019.9066764&partnerID=40&md5=677677c6078db84a6bf5437ab2b99c7b},
abstract={More and more power supply companies use Unmanned Aerial Vehicles (UAV) for power line inspection. UAVs allow almost immediate inspection of power lines after extreme weather events. However, the current UAV vision based damage assessments have still been performed manually, which is time-consuming, poor efficient, and low accurate. In this work, a fast CPU-based detection model is presented for detecting normal and abnormal power line poles from the UAV vision data after typhoon striking. Three types of poles including two types of normal poles and one type of abnormal poles are considered. The detection process is designed in two stages. The first stage is to generate candidate boxes of poles based on the YOLO-Lite model, and the second stage is to filter the background candidate boxes based on the classification model of the SPP (Spatial Pyramid Pooling) network structure. The combined model achieves a detection precision of 75.80%, an increase of 26.85% compared to the YOLO-Lite model alone, and reaches a recall of 57.33%. The combined poles detection model runs at 9 FPS (Frames Per Second) on a CPU-only computer. © 2019 IEEE.},
}

@ARTICLE{Buatik2019132,
author={Buatik, A. and Ali, L. and Chaiyasarn, K.},
title={3D model-based image registration for change detection in historical structures via unmanned aerial vehicle},
journal={International Journal of GEOMATE},
year={2019},
volume={16},
number={58},
pages={132-138},
art_number={8218},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85067613768&doi=10.21660%2f2019.58.8218&partnerID=40&md5=e47a8b740f3f502ebe43c38ae3a99b79},
abstract={Visual inspection is a common technique to detect and examine the state of health of the structural system. Periodic inspection is carried out to determine if anomalies, such as cracks and surface paint, found in previous visits have changed in appearance over time. The image-based change detection techniques require accurate geometrical and photometrical corrections in pre-processing steps to minimize errors. Although several techniques have been proposed to remove geometrical errors, they still fail to align image correctly, which often results in inaccuracy in a change detection system. In this paper, a change detection system is proposed to tackle this problem. The system acquired images via an unmanned aerial vehicle. Then, the acquired images were manually processed to identify damages, such as cracks, which were used to guide a drone to obtain more images of damage areas for monitoring purpose. The images were then used to obtain a 3D surface model and camera calibration through Structure from Motion (SfM), which were used in the image synthesis technique to obtain an image with identical camera parameters as a queried image for accurate geometrical adjustment. The synthesized images were used to compare with the queried image to see if there were changes between them. In this research project, it was showed that the drone can be used to monitor problematic areas and the image synthetic technique via 3D modeling can be used in geometrical registration to improve a change detection system. © Int. J. of GEOMATE. All rights reserved.},
}

@CONFERENCE{Kim2019626,
author={Kim, S. and Kwon, D. and Ji, Y.},
title={CNN based human detection for unmanned aerial vehicle},
journal={MobiSys 2019 - Proceedings of the 17th Annual International Conference on Mobile Systems, Applications, and Services},
year={2019},
pages={626-627},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85069218463&doi=10.1145%2f3307334.3328659&partnerID=40&md5=a3ea13159b302002d330b31cc7c4843e},
abstract={In order to utilize a unmanned aerial device such as a drone in terms of reconnaissance, surveillance and disaster management, a technique capable of performing real-time human detection is needed. In this study, we introduce a method of human detection by constructing environment similar to a drone by installing wide angle lens camera on the ceiling. Tiny-Yolo, which is a kind of Convolutional Neural Network, was used as recognition technology. Camera sensors were installed on ceilings in various places inside the building to collect training data for human detection. The Training was performed based on 4,000 pieces of collected data, and the accuracy of recognition was measured. As a result, 95.37% precision and 96.60% recall were obtained. © 2019 Copyright held by the owner/author(s).},
}

@ARTICLE{Parrott20191,
author={Parrott, E. and Panter, H. and Morrissey, J. and Bezombes, F.},
title={A low cost approach to disturbed soil detection using low altitude digital imagery from an unmanned aerial vehicle},
journal={Drones},
year={2019},
volume={3},
number={2},
pages={1-12},
art_number={50},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85088049052&doi=10.3390%2fdrones3020050&partnerID=40&md5=969b2b6f0bc0f43d55fed716a2881414},
abstract={Until recently, clandestine burial investigations relied upon witness statements to determine target search areas of soil and vegetation disturbance. Due to this, remote sensing technologies are increasingly used to detect fresh clandestine graves. However, despite the increased capabilities of remote sensing, clandestine burial searches remain resourcefully intensive as the police have little access to the technology when it is required. In contrast to this, Unmanned Aerial Vehicle (UAV) technology is increasingly popular amongst law enforcement worldwide. As such, this paper explores the use of digital imagery collected from a low cost UAV for the aided detection of disturbed soil sites indicative of fresh clandestine graves. This is done by assessing the unaltered UAV video output using image processing tools to detect sites of disturbance, therefore highlighting previously unrecognised capabilities of police UAVs. This preliminary investigation provides a low cost rapid approach to detecting fresh clandestine graves, further supporting the use of UAV technology by UK police. © 2019 by the authors.},
}

@CONFERENCE{Huang2019,
author={Huang, X. and Yan, K. and Wu, H.-C. and Wu, Y.},
title={Unmanned Aerial Vehicle Hub Detection Using Software-Defined Radio},
journal={IEEE International Symposium on Broadband Multimedia Systems and Broadcasting, BMSB},
year={2019},
volume={2019-June},
art_number={8971851},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85079341624&doi=10.1109%2fBMSB47279.2019.8971851&partnerID=40&md5=30d01d28d4da589425eec17ad26ee418},
abstract={The applications of unmanned aerial vehicles (UAVs) have increased dramatically in the past decade. Meanwhile, close-range UAV detection has been intriguing by many researchers for its great importance in privacy, security, and safety control. Positioning of the UAV controller (hub) is quite challenging but still difficult. In order to combat this emerging problem for public interest, we propose to utilize a software-defined radio (SDR) platform, namely HackRF One, to enable the UAV hub detection and localization. The SDR receiver can acquire the UAV source signals. The theoretical path-loss propagation model is adopted to predict the signal strength attenuation. Thus, the UAV hub location can be estimated using the modified multilateration approach by only three or more SDR receivers. © 2019 IEEE.},
}

@CONFERENCE{Cidronali2019438,
author={Cidronali, A. and Traverso, P. and Passafiume, M. and Colantonio, P. and Collodi, G. and Florian, C. and Leuzzi, G. and Pirola, M. and Ramella, C. and Santarelli, A.},
title={System Level Analysis of Millimetre-wave GaN-based MIMO Radar for Detection of Micro Unmanned Aerial Vehicles},
journal={Progress in Electromagnetics Research Symposium},
year={2019},
volume={2019-June},
pages={438-450},
art_number={9017681},
note={cited By 9},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85078913436&doi=10.1109%2fPIERS-Spring46901.2019.9017681&partnerID=40&md5=930d2173f596b78fba724aea35029f30},
abstract={The detection of Unmanned Aerial Vehicles (UAVs) of micro/nano dimensions, is becoming a hot topic, due to their large diffusion, and represents a challenging task from both the system architecture and components point of view. The Frequency Modulated Continuous Wave (FMCW) radar architecture in a Multi-Input Multi-Output configuration has been identified as the most suitable solution for this purpose, due to both its inherent short-range detection capability and compact implementation. This paper describes the operation and technology challenges inherent to the development of a millimeter-wave FMCW MIMO radar for small UAVs detection. In particular it analyzes the sub-systems specifications and the expected system performance with respect to a chip set designed and developed in GaN at 37.5 GHz applications. © 2019 IEEE.},
}

@CONFERENCE{Wu2019608,
author={Wu, Q. and Zhou, Y.},
title={Multi-pose moving human detection based on unmanned aerial vehicle in real-time},
journal={Proceedings of the 14th IEEE Conference on Industrial Electronics and Applications, ICIEA 2019},
year={2019},
pages={608-613},
art_number={8833758},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85073070170&doi=10.1109%2fICIEA.2019.8833758&partnerID=40&md5=2f2d2f42e76a576e6f75fd6e4b04c22b},
abstract={In this paper, a multi-pose human detection system is presented based on Unmanned Aerial Vehicle (UAV) imageries in real-time. A satisfying detection accuracy of multipose human detection in complex outdoor environments can be achieved with no accelerating hardware like graphics processing unit. First, 30,000 positive samples with various appearances are selected manually from different shooting angles and are used to train the convolutional neural network (CNN) classifier. Second, optical flow of the two successive frames taken by onboard camera is used to extract region of interests and a series of post-processing methods, i.e., average filtering, morphological operation and extraction of outer contour are applied to meet the real-time requirement. Then a two-stream CNN combining the appearance and motion information are applied to reduce the false detection accuracy. Field experiments in complex outdoor environments have been performed to verify that the proposed system can be used to detect multi-pose humans with high detection accuracy in real-time. © 2019 IEEE.},
}

@ARTICLE{Seo2019814,
author={Seo, C.},
title={Vehicle Detection and Car Type Identification System using Deep Learning and Unmanned Aerial Vehicle},
journal={International Journal of Innovative Technology and Exploring Engineering},
year={2019},
volume={8},
number={8},
pages={814-819},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85068704863&partnerID=40&md5=6ceb81f7c1ba1ff28654edf7a675076c},
abstract={Background/Objectives: UAV (unmanned aerial vehicle) based traffic measurement system has various advantages than the traditional traffic monitoring systems using fixed loop sensors. This paper proposes the designing and implementing method of vehicle detection and type identification using Deep Learning and UAV in UHD (ultra-high definition) 4K video images. Methods/Statistical analysis: The present study proposes the implementation method of detection and classification system that can be accomplished vehicle classification according to AUSTROADS�s plan. The proposed system has designed two primary processes: detection and classification. This paper introduces the method that vehicle data training, detection, and classification method by applying a Darknet-53 for vehicles found in UHD images. Also, we propose the variable classification method due to parked and stopped cars for traffic flow monitoring. So, we considered the three conditions of driving, stopping, and parking. Findings: The results of the experiment show that the proposed approach resulted in errors that were twice as low as conventional methods that are using a fixed search area. Improvements/Applications: The proposed study can be applied to traffic flow monitoring system, ITS (intelligent transport system), vehicle detection and classification system. © BEIESP.},
}

@ARTICLE{Lee2019794,
author={Lee, J. and Seo, C.},
title={Deep Learning based Pedestrian Detection and Tracking System using Unmanned Aerial Vehicle and Prediction Method},
journal={International Journal of Innovative Technology and Exploring Engineering},
year={2019},
volume={8},
number={8},
pages={794-799},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85068687408&partnerID=40&md5=b9032dd6135009db4db9bd9eb7d83c83},
abstract={Pedestrian detection and tracking system have become an essential field in the object detection and target tracking research area. This study proposes for developing and implementing the fast pedestrian detection and tracking system using Deep learning (YOLOv3), UAV (Unmanned Aerial Vehicle) and prediction method that is the Kalman Filter. Methods/Statistical analysis: The performance of the object detection and tracking system is decided by the performance time and the accuracy of object detection and tracking algorithms. So we applied to the YOLOv3 which is the fast detection method recent at our proposed system and also proposed the Kalman Filter algorithm with a variable detection area as the pedestrian tracking system. Findings: In the experiments, the proposed method successfully detected and tracked pedestrians who move at 53 FPS maximum and 38-43 FPS on average each test videos. The proposed way with variable search ranges made much fewer errors than the traditional object detector with fixed search ranges. Improvements/Applications: This research result can be applied pedestrian moving monitoring system, ITS (intelligent transport system) and security surveillance system. © BEIESP.},
}

@ARTICLE{Xu2019,
author={Xu, F. and Hong, T. and Zhao, J. and Yang, T.},
title={Detection and identification technology of rotor unmanned aerial vehicles in 5G scene},
journal={International Journal of Distributed Sensor Networks},
year={2019},
volume={15},
number={6},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85066991832&doi=10.1177%2f1550147719853990&partnerID=40&md5=e83fdc70f9cf1549bc9dc7cae5ceb88c},
abstract={In the 5G era, integration between different networks is required to realize a new world of Internet of things, the most typical model is Space–Air–Ground Internet of things. In the Space–Air–Ground Internet of things, unmanned aerial vehicle network is widely used as the representative of air-based networks. Therefore, a lot of unmanned aerial vehicle “black flying” incidents have occurred. UAVs are a kind of “low, slow and small” artificial targets, which face enormous challenges in detecting, identifying, and managing them. In order to identify the “black flying” unmanned aerial vehicle, combined with the advantages of 5G millimeter wave radar and machine learning methods, the following methods are adopted in this article. For a one-rotor unmanned aerial vehicle, the radar echo data are a single-component sinusoidal frequency modulation signal. The echo signal is conjugated first and then is subjected to a short-time Fourier transform, while the micro-Doppler has a double effect. For a multi-rotor unmanned aerial vehicle, the radar echo data are a multi-component sinusoidal frequency modulation signal, the k-order Bessel function base and the signal are used for integral projection processing, which better identifies the micro-Doppler characteristics such as the number of rotors or the rotational speed of each rotor. The noise interference is added to verify that the algorithm has better robustness. The micro-Doppler characteristics of rotor unmanned aerial vehicles are extracted by the above algorithm, and the data sets are built to train the model. Finally, the classification of unmanned aerial vehicle is realized, and the classification results are given. The research in this article provides an effective solution to solve the problem of detecting and identifying unmanned aerial vehicle by 5G millimeter wave radar in the Internet of Things, which has high practical application value. © The Author(s) 2019.},
}

@ARTICLE{Gallego2019782,
author={Gallego, A.-J. and Pertusa, A. and Gil, P. and Fisher, R.B.},
title={Detection of bodies in maritime rescue operations using unmanned aerial vehicles with multispectral cameras},
journal={Journal of Field Robotics},
year={2019},
volume={36},
number={4},
pages={782-796},
note={cited By 12},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85057729270&doi=10.1002%2frob.21849&partnerID=40&md5=7ef6359e47b83b2c20295059b3f42984},
abstract={In this study, we use unmanned aerial vehicles equipped with multispectral cameras to search for bodies in maritime rescue operations. A series of flights were performed in open-water scenarios in the northwest of Spain, using a certified aquatic rescue dummy in dangerous areas and real people when the weather conditions allowed it. The multispectral images were aligned and used to train a convolutional neural network for body detection. An exhaustive evaluation was performed to assess the best combination of spectral channels for this task. Three approaches based on a MobileNet topology were evaluated, using (a) the full image, (b) a sliding window, and (c) a precise localization method. The first method classifies an input image as containing a body or not, the second uses a sliding window to yield a class for each subimage, and the third uses transposed convolutions returning a binary output in which the body pixels are marked. In all cases, the MobileNet architecture was modified by adding custom layers and preprocessing the input to align the multispectral camera channels. Evaluation shows that the proposed methods yield reliable results, obtaining the best classification performance when combining green, red-edge, and near-infrared channels. We conclude that the precise localization approach is the most suitable method, obtaining a similar accuracy as the sliding window but achieving a spatial localization close to 1 m. The presented system is about to be implemented for real maritime rescue operations carried out by Babcock Mission Critical Services Spain. © 2018 Wiley Periodicals, Inc.},
}

@CONFERENCE{Wu2019574,
author={Wu, Q. and Zhou, Y.},
title={Real-time object detection based on unmanned aerial vehicle},
journal={Proceedings of 2019 IEEE 8th Data Driven Control and Learning Systems Conference, DDCLS 2019},
year={2019},
pages={574-579},
art_number={8908984},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85076430328&doi=10.1109%2fDDCLS.2019.8908984&partnerID=40&md5=44e80c5f9fc16670e8b19d4ed74c8ab0},
abstract={In this paper, a real-time image detection system for unmanned aerial vehicle (UAV) is presented. First, the You Only Look Once (YOLO) detector is retrained to detect and recognize objects in UAV images fast and accurately. The retrained YOLO detector possesses a tradeoff between quickly objects identification and precisely objects localization, accounting for 4 general moving objects (i.e., car, bus, truck and pedestrian) in UAV images. Second, extra 4, 000 UAV images shot by the embedded UAV camera are fed into the YOLO which is used to predict bounding-box with label probabilities from a full image. The YOLO is compared with the Faster Region Convolutional Neural Network, as well as other deep-learning frameworks for object detection. Field experiments on UAV videos shot in various backgrounds are performed to testify that the proposed system can detect objects in UAV images effectively and robustly, achieving a real-time detection speed at 15 frames per second and a satisfying accuracy on the wild test set of 400 UAV images with a Graphic Processing Unit (GPU) acceleration. © 2019 IEEE.},
}

@CONFERENCE{Parfiryev2019,
author={Parfiryev, A.V. and Dushkin, A.V. and Dubrovin, A.S. and Stepanov, L.V.},
title={Control of unmanned aerial vehicles based on the detection algorithm},
journal={Journal of Physics: Conference Series},
year={2019},
volume={1202},
number={1},
art_number={12014},
note={cited By 13},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85065727875&doi=10.1088%2f1742-6596%2f1202%2f1%2f012014&partnerID=40&md5=4dc50d1da77c040f4b748c638498869c},
abstract={The work analyzes the current tasks of unmanned aircraft, which showed the need to develop algorithms and systems for automatic tracking of objects operating in real-time mode, in the tasks of conducting reconnaissance flights and targeting precision weapons. An algorithm for detecting objects in the image by correlation filtration based on a two-dimensional discrete Fourier transform for control problems of unmanned aerial vehicles is developed. A software implementation of the detection algorithm using the OpenCV/C ++ computer vision library (EmguCV/C #) is obtained. A number of methods of computer libraries used for constructing program code are presented. Time schedules and recommendations for using the algorithm in different shooting conditions are given. © Published under licence by IOP Publishing Ltd.},
}

@CONFERENCE{Surinta2019206,
author={Surinta, O. and Khruahong, S.},
title={Tracking people and objects with an autonomous unmanned aerial vehicle using face and color detection},
journal={ECTI DAMT-NCON 2019 - 4th International Conference on Digital Arts, Media and Technology and 2nd ECTI Northern Section Conference on Electrical, Electronics, Computer and Telecommunications Engineering},
year={2019},
pages={206-210},
art_number={8692269},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85065092724&doi=10.1109%2fECTI-NCON.2019.8692269&partnerID=40&md5=ae8d400520e0bf8e3235dc80526b48e4},
abstract={We propose a people and object tracking algorithm for an autonomous unmanned aerial vehicle (UAV). It uses as a surveillance camera and can move anywhere. The camera from UAV is not fixed l ocation a s c losed-circuit t elevision. T he face detection and objection detection are applied to support our proposed. In this research, the UAV model for this paper was AR-Drone 2.0. It has a constraint on the front camera because it has fixed the position of view and cannot change the view during flight. W e d esigned t wo e xperiments. F irst, t he f ace detection using images and applied to the popularity of the face detection, is a Haar-cascade classifier and max-margin object detection with convolutional neural network based features because they have high precision in analysis. Second, color detection system, which only focuses on the color of objects which can developed as an obstacle detection system. The results of the experiment can be accepted to adapt to tracking people and objects in the smart-city. © 2019 IEEE.},
}

@ARTICLE{Dell201979,
author={Dell, M. and Stone, C. and Osborn, J. and Glen, M. and McCoull, C. and Rimbawanto, A. and Tjahyono, B. and Mohammed, C.},
title={Detection of necrotic foliage in a young Eucalyptus pellita plantation using unmanned aerial vehicle RGB photography–a demonstration of concept},
journal={Australian Forestry},
year={2019},
volume={82},
number={2},
pages={79-88},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85067552465&doi=10.1080%2f00049158.2019.1621588&partnerID=40&md5=9245019ae73f71a9d0b6a3e7b7f24b82},
abstract={Recent advances and commercialisation of unmanned aerial vehicle/red blue green (RGB) camera systems and digital photogrammetric techniques now provide a cheap and flexible alternative to higher-cost airborne platforms for routine monitoring of canopy health in timber plantations. Structure-from-Motion photogrammetry produces very dense three-dimensional (3D) point clouds which can be used to derive metrics for inventory estimation. Unmanned aerial vehicle RGB photography also captures data that can relate to tree health. In contrast to the more common use of orthorectified RGB photography to extract this spectral information, we used the software package Agisoft Photoscan to assign a simple Vegetation Index value directly to each point in the 3D point cloud. Using data acquired by a DJI Phantom 4 Pro, we present a simple processing and photogrammetric workflow solution for detecting dead and dying trees in a young Eucalyptus pellita plantation located in the provenance of Riau, Sumatra. Trees affected by the bacterial wilt Ralstonia sp. present symptoms of necrotic foliage on individual branches or the whole crown. Assigning the Visible Atmospheric Resistant Index Vegetation Index colour-coded values to individual points in the 3D point cloud significantly enhanced visualisation of necrotic foliage on individual trees in both the point cloud and the associated orthophoto compared to the RGB equivalent images. This approach could easily be operationally deployed for the rapid detection and mapping of unhealthy trees with symptoms of necrotic foliage. © 2019, © 2019 The Author(s). Published by Informa UK Limited, trading as Taylor & Francis Group.},
}

@ARTICLE{Azevedo2019,
author={Azevedo, F. and Dias, A. and Almeida, J. and Oliveira, A. and Ferreira, A. and Santos, T. and Martins, A. and Silva, E.},
title={LiDAR-based real-time detection and modeling of power lines for unmanned aerial vehicles},
journal={Sensors (Switzerland)},
year={2019},
volume={19},
number={8},
art_number={1812},
note={cited By 27},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85065117235&doi=10.3390%2fs19081812&partnerID=40&md5=2d584d5c67fadac0c04b8a59000b3feb},
abstract={The effective monitoring and maintenance of power lines are becoming increasingly important due to a global growing dependence on electricity. The costs and risks associated with the traditional foot patrol and helicopter-based inspections can be reduced by using UAVs with the appropriate sensors. However, this implies developing algorithms to make the power line inspection process reliable and autonomous. In order to overcome the limitations of visual methods in the presence of poor light and noisy backgrounds, we propose to address the problem of power line detection and modeling based on LiDAR. The PL2DM, Power Line LiDAR-based Detection and Modeling, is a novel approach to detect power lines. Its basis is a scan-by-scan adaptive neighbor minimalist comparison for all the points in a point cloud. The power line final model is obtained by matching and grouping several line segments, using their collinearity properties. Horizontally, the power lines are modeled as a straight line, and vertically as a catenary curve. Using a real dataset, the algorithm showed promising results both in terms of outputs and processing time, adding real-time object-based perception capabilities for other layers of processing. © 2019 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@CONFERENCE{Uzun2019,
author={Uzun, B. and Eker, O. and Saribas, H. and Cevikalp, H.},
title={Detection based tracking of unmanned aerial vehicles [Insansiz Hava Araclarinin Konumlandirilarak Takip Edilmesi]},
journal={27th Signal Processing and Communications Applications Conference, SIU 2019},
year={2019},
art_number={8806391},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85071983195&doi=10.1109%2fSIU.2019.8806391&partnerID=40&md5=33ac4e23d43e7c699336c286f8975861},
abstract={Object tracking is one of the fundamental problems of computer vision, which has many difficulties such as fast camera motion, occlusion and similar objects. Today, small and lightweight single board computers with very high processing power have been developed. Real-time processing of the computer vision applications on unmanned aerial vehicles has become possible with the integration of such single board computers within UAVs. In this study, a hybrid method is developed to detect and track UAVs by another UAV. A deep learning based approach which is one of the fastest and most accurate method in the literature, YOLOv3 and YOLOv3-Tiny (You Only Look Once), are utilized to detect the UAV at the beginning of the video and when tracking of the UAV is failed. Kernelized Correlation Filter (KCF) is used for real time tracking purpose of the detected UAVs. A dataset is created that consists different UAVs to train and test YOLOv3. Performance of the proposed methods are evaluated on this dataset. © 2019 IEEE.},
}

@CONFERENCE{Lishchenko2019559,
author={Lishchenko, V. and Khudov, H. and Tiutiunnyk, V. and Kuprii, V. and Zots, F. and Misiyuk, G.},
title={The Method of Increasing the Detection Range of Unmanned Aerial Vehicles in Multiradar Systems Based on Surveillance Radars},
journal={2019 IEEE 39th International Conference on Electronics and Nanotechnology, ELNANO 2019 - Proceedings},
year={2019},
pages={559-562},
art_number={8783263},
note={cited By 17},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85070867685&doi=10.1109%2fELNANO.2019.8783263&partnerID=40&md5=1cd4c95558f8bbdbb4d0a5c1a48ec3b3},
abstract={The paper analyses a model of a small base synchronous multiradar system on the basis of two-coordinate surveillance radar, which will enable to increase the detection range of unmanned aerial vehicles. Separate positions of elements of such systems are spacious apart from each other, but the processing of radar information is carried out in a single point. A special feature will be the using of radars with mechanical rotation in the azimuth plane as elements of the system. It will increase the efficiency of detection due to the using of radar information contained in the structure of the electromagnetic field more efficiently than the monostatic two-coordinate radars. The advantage will be an increasing in the energy potential of the system as a result of the addition of the power of the pulses of individual radars and an increasing in the gain of the antenna array due to the more directional properties of the antenna array compared to single antenna. Calculations of the multiradar system parameters are carried out by the method of mathematical modelling. © 2019 IEEE.},
}

@CONFERENCE{Azevedo2019,
author={Azevedo, F. and Dias, A. and Almeida, J. and Oliveira, A. and Ferreira, A. and Santos, T. and Martins, A. and Silva, E.},
title={Real- Time LiDAR-based Power Lines Detection for Unmanned Aerial Vehicles},
journal={19th IEEE International Conference on Autonomous Robot Systems and Competitions, ICARSC 2019},
year={2019},
art_number={8733646},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85068440790&doi=10.1109%2fICARSC.2019.8733646&partnerID=40&md5=ced8d553c3507ae53e5f2b12970c05fd},
abstract={The growing dependence of modern-day societies on electricity increases the importance of effective monitoring and maintenance of power lines. Endowing UAVs with the appropriate sensors for inspecting power lines, the costs and risks associated with the traditional foot patrol and helicopter-based inspections can be reduced. However, this implies the development of algorithms to make the inspection process reliable and autonomous. Visual methods are usually applied to locate the power lines and their components, but poor light conditions or a background rich in edges may compromise their results. To overcome those limitations, we propose to address the problem of power line detection and modeling based on LiDAR. A novel approach to the power line detection was developed, the PL2DM - Power Line LiDAR-based Detection and Modeling. It is based in a scan-by-scan adaptive neighbor minimalist comparison for all the points in a point cloud. The power line final model is obtained by matching and grouping several line segments, using their collinearity properties. Horizontally, the power lines are modeled as a straight line, and vertically as a catenary curve. The algorithm was validated with a real dataset, showing promising results both in terms of outputs and processing time, adding real-time object-based perception capabilities for other layers of processing. © 2019 IEEE.},
}

@ARTICLE{Wu2019,
author={Wu, X. and Shen, X. and Cao, L. and Wang, G. and Cao, F.},
title={Assessment of individual tree detection and canopy cover estimation using unmanned aerial vehicle based light detection and ranging (UAV-LiDAR) data in planted forests},
journal={Remote Sensing},
year={2019},
volume={11},
number={8},
art_number={908},
note={cited By 45},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85065031707&doi=10.3390%2frs11080975&partnerID=40&md5=5a6f11e385db1277cb4b85550c0e78ad},
abstract={Canopy cover is a key forest structural parameter that is commonly used in forest inventory, sustainable forest management and maintaining ecosystem services. Recently, much attention has been paid to the use of unmanned aerial vehicle (UAV)-based light detection and ranging (LiDAR) due to the flexibility, convenience, and high point density advantages of this method. In this study, we used UAV-based LiDAR data with individual tree segmentation-based method (ITSM), canopy height model-based method (CHMM), and a statistical model method (SMM) with LiDAR metrics to estimate the canopy cover of a pure ginkgo (Ginkgo biloba L.) planted forest in China. First, each individual tree within the plot was segmented using watershed, polynomial fitting, individual tree crown segmentation (ITCS) and point cloud segmentation (PCS) algorithms, and the canopy cover was calculated using the segmented individual tree crown (ITSM). Second, the CHM-based method, which was based on the CHM height threshold, was used to estimate the canopy cover in each plot. Third, the canopy cover was estimated using the multiple linear regression (MLR) model and assessed by leave-one-out cross validation. Finally, the performance of three canopy cover estimation methods was evaluated and compared by the canopy cover from the field data. The results demonstrated that, the PCS algorithm had the highest accuracy (F = 0.83), followed by the ITCS (F = 0.82) and watershed (F = 0.79) algorithms; the polynomial fitting algorithm had the lowest accuracy (F = 0.77). In the sensitivity analysis, the three CHM-based algorithms (i.e., watershed, polynomial fitting and ITCS) had the highest accuracy when the CHM resolution was 0.5 m, and the PCS algorithm had the highest accuracy when the distance threshold was 2 m. In addition, the ITSM had the highest accuracy in estimation of canopy cover (R2 = 0.92, rRMSE = 3.5%), followed by the CHMM (R2 = 0.94, rRMSE = 5.4%), and the SMM had a relative low accuracy (R2 = 0.80, rRMSE = 5.9%). The UAV-based LiDAR data can be effectively used in individual tree crown segmentation and canopy cover estimation at plot-level, and CC estimation methods can provide references for forest inventory, sustainable management and ecosystem assessment. © 2019 by the authors.},
}

@ARTICLE{Hong2019,
author={Hong, S.-J. and Han, Y. and Kim, S.-Y. and Lee, A.-Y. and Kim, G.},
title={Application of deep-learning methods to bird detection using unmanned aerial vehicle imagery},
journal={Sensors (Switzerland)},
year={2019},
volume={19},
number={7},
art_number={1651},
note={cited By 45},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85064572639&doi=10.3390%2fs19071651&partnerID=40&md5=7d96da0847298c134dd400bb4997e612},
abstract={Wild birds are monitored with the important objectives of identifying their habitats and estimating the size of their populations. Especially in the case of migratory bird, they are significantly recorded during specific periods of time to forecast any possible spread of animal disease such as avian influenza. This study led to the construction of deep-learning-based object-detection models with the aid of aerial photographs collected by an unmanned aerial vehicle (UAV). The dataset containing the aerial photographs includes diverse images of birds in various bird habitats and in the vicinity of lakes and on farmland. In addition, aerial images of bird decoys are captured to achieve various bird patterns and more accurate bird information. Bird detection models such as Faster Region-based Convolutional Neural Network (R-CNN), Region-based Fully Convolutional Network (R-FCN), Single Shot MultiBox Detector (SSD), Retinanet, and You Only Look Once (YOLO) were created and the performance of all models was estimated by comparing their computing speed and average precision. The test results show Faster R-CNN to be the most accurate and YOLO to be the fastest among the models. The combined results demonstrate that the use of deep-learning-based detection methods in combination with UAV aerial imagery is fairly suitable for bird detection in various environments. © 2019 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@ARTICLE{Farlik2019,
author={Farlik, J. and Kratky, M. and Casar, J. and Stary, V.},
title={Multispectral detection of commercial unmanned aerial vehicles},
journal={Sensors (Switzerland)},
year={2019},
volume={19},
number={7},
art_number={1517},
note={cited By 14},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85063929253&doi=10.3390%2fs19071517&partnerID=40&md5=2a7f3d727bc25e2cbc54a84f4e81d286},
abstract={The fight against unmanned vehicles is nothing new; however, especially with the arrival of new technologies that are easily accessible for the wider population, new problems are arising. The deployment of small unmanned aerial vehicles (UAVs) by paramilitary organizations during conflicts around the world has become a reality, non-lethal “paparazzi” actions have become a common practice, and it is only a matter of time until the population faces lethal attacks. The basic prerequisite for direct defense against attacking UAVs is their detection. The authors of this paper analysed the possibility of detecting flying aircraft in several different electro-magnetic spectrum bands. Firstly, methods based on calculations and simulations were chosen, and experiments in laboratories and measurements of the exterior were subsequently performed. As a result, values of the radar cross section (RCS), the noise level, the surface temperature, and optical as well as acoustic traces of tested devices were quantified. The outputs obtained from calculated, simulated, and experimentally detected values were found via UAV detection distances using specific sensors working in corresponding parts of the frequency spectrum. © 2019 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@CONFERENCE{Korki2019,
author={Korki, M. and Shankar, N.D. and Shah, R.N. and Waseem, S.M. and Hodges, S.},
title={Automatic Fault Detection of Power Lines using Unmanned Aerial Vehicle (UAV)},
journal={2019 1st International Conference on Unmanned Vehicle Systems-Oman, UVS 2019},
year={2019},
art_number={8658283},
note={cited By 8},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85063947565&doi=10.1109%2fUVS.2019.8658283&partnerID=40&md5=4817fbb36dad85e0d6f772f8b6d982d4},
abstract={Safety and automation are the two major challenges in the application of Unmanned Aerial Vehicle (UAV), commonly known as drone, to the power lines inspection and fault detection. While current state-of-the-art UAVs are equipped with collision avoidance features, there is less attention to the automatic and real-time fault detection of power lines using UAVs. This paper presents the architecture of three drone-oriented concept designs for automatic and real-time fault detection of power lines using UAVs. The proposed systems could be potential candidates for replacing traditional inspection methods of power lines, which are risky and costly. By incorporating a robust neural network, i.e., Artificial Intelligence (AI), and using appropriate and efficient sensors, the systems can automatically detect various faults and defects on power lines with high precision. We propose three concept design options comprised of different hardware/software components and their feasibility factors. For instance, FLIR Duo Pro R as a thermal sensor and Zenmuse XT for thermal vision have been proposed to be used in the concept designs. For data communication, the proposed designs use cloud-based virtual private network (VPN) for a secure connection between remote control (RC) of the UAV and the server. Based on the advantages and disadvantages of the three proposed design options, the most efficient design is also discussed. This design proposes a system with lightweight sensors, which could increase the flight time of the UAV. Further, the AI interface is coded on to the RC, making it economical, without any database for big data storage. The back-end of the neural network is stored in a cloud server. With the help of GSM antenna, the AI can run on the tablet if there is an available cellular network. © 2019 IEEE.},
}

@CONFERENCE{Benjdira2019,
author={Benjdira, B. and Khursheed, T. and Koubaa, A. and Ammar, A. and Ouni, K.},
title={Car Detection using Unmanned Aerial Vehicles: Comparison between Faster R-CNN and YOLOv3},
journal={2019 1st International Conference on Unmanned Vehicle Systems-Oman, UVS 2019},
year={2019},
art_number={8658300},
note={cited By 112},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85063932058&doi=10.1109%2fUVS.2019.8658300&partnerID=40&md5=7edcf3211e52741d7f163b4a627a0e65},
abstract={Unmanned Aerial Vehicles are increasingly being used in surveillance and traffic monitoring thanks to their high mobility and ability to cover areas at different altitudes and locations. One of the major challenges is to use aerial images to accurately detect cars and count-them in real-time for traffic monitoring purposes. Several deep learning techniques were recently proposed based on convolution neural network (CNN) for real-time classification and recognition in computer vision. However, their performance depends on the scenarios where they are used. In this paper, we investigate the performance of two state-of-the art CNN algorithms, namely Faster R-CNN and YOLOv3, in the context of car detection from aerial images. We trained and tested these two models on a large car dataset taken from UAVs. We demonstrated in this paper that YOLOv3 outperforms Faster R-CNN in sensitivity and processing time, although they are comparable in the precision metric. © 2019 IEEE.},
}

@ARTICLE{Safonova2019,
author={Safonova, A. and Tabik, S. and Alcaraz-Segura, D. and Rubtsov, A. and Maglinets, Y. and Herrera, F.},
title={Detection of fir trees (Abies sibirica) damaged by the bark beetle in unmanned aerial vehicle images with deep learning},
journal={Remote Sensing},
year={2019},
volume={11},
number={6},
art_number={643},
note={cited By 57},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85115775394&doi=10.3390%2frs11060643&partnerID=40&md5=70d9b33eeed153342e7e1ea09a85a429},
abstract={Invasion of the Polygraphus proximus Blandford bark beetle causes catastrophic damage to forests with firs (Abies sibirica Ledeb) in Russia, especially in Central Siberia. Determining tree damage stage based on the shape, texture and colour of tree crown in unmanned aerial vehicle (UAV) images could help to assess forest health in a faster and cheaper way. However, this task is challenging since (i) fir trees at different damage stages coexist and overlap in the canopy, (ii) the distribution of fir trees in nature is irregular and hence distinguishing between different crowns is hard, even for the human eye. Motivated by the latest advances in computer vision and machine learning, this work proposes a two-stage solution: In a first stage, we built a detection strategy that finds the regions of the input UAV image that are more likely to contain a crown, in the second stage, we developed a new convolutional neural network (CNN) architecture that predicts the fir tree damage stage in each candidate region. Our experiments show that the proposed approach shows satisfactory results on UAV Red, Green, Blue (RGB) images of forest areas in the state nature reserve “Stolby” (Krasnoyarsk, Russia). © 2019 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@ARTICLE{Zhang20192170,
author={Zhang, Q. and Wang, X. and Xiao, X. and Pei, C.},
title={Design of a fault detection and diagnose system for intelligent unmanned aerial vehicle navigation system},
journal={Proceedings of the Institution of Mechanical Engineers, Part C: Journal of Mechanical Engineering Science},
year={2019},
volume={233},
number={6},
pages={2170-2176},
note={cited By 7},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85049112355&doi=10.1177%2f0954406218780508&partnerID=40&md5=c6089e8663cfe88d4c29292a82ac9025},
abstract={A secure control system is of great importance for unmanned aerial vehicles, especially in the condition of fault data injection. As the source of the feedback control system, the Inertial navigation system/Global position system (INS/GPS) is the premise of flight control system security. However, unmanned aerial vehicles have the requirement of lightweight and low cost for airborne equipment, which makes redundant device object unrealistic. Therefore, the method of fault detection and diagnosis is desperately needed. In this paper, a fault detection and diagnosis method based on fuzzy system and neural network is proposed. Fuzzy system does not depend on the mathematical model of the process, which overcomes the difficulties in obtaining the accurate model of unmanned aerial vehicles. Neural network has a strong self-learning ability, which could be used to optimize the membership function of fuzzy system. This paper is structured as follows: first, a Kalman filter observer is introduced to calculate the residual sequences caused by different sensor faults. Then, the sequences are transmitted to the fault detection and diagnosis system and fault type can be obtained. The proposed fault detection and diagnosis algorithm was implemented and evaluated with real datasets, and the results demonstrate that the proposed method can detect the sensor faults successfully with high levels of accuracy and efficiency. © IMechE 2018.},
}

@ARTICLE{Yuan2019337,
author={Yuan, C. and Liu, Z. and Zhang, Y.},
title={Learning-Based Smoke Detection for Unmanned Aerial Vehicles Applied to Forest Fire Surveillance},
journal={Journal of Intelligent and Robotic Systems: Theory and Applications},
year={2019},
volume={93},
number={1-2},
pages={337-349},
note={cited By 29},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85044451469&doi=10.1007%2fs10846-018-0803-y&partnerID=40&md5=0ef6dc079de8a4cb6e2c9108d3afc47a},
abstract={Forests are potentially and seriously threatened by fires which have caused huge damages and losses of life and properties every year. In general, it is easier to detect smoke than fire in its early stage. Developing an effective and safe smoke detection method is thereby critical for early forest fire fighting and preventing the fire developing into uncontrollable. This paper presents a learning-based fuzzy smoke detection approach intended to achieve an effective and early forest fire detection, while greatly reduce the negative impacts from clouds in the sky, illumination variations, and changes of forest features. First, a fuzzy-logic based smoke detection rule is designed for detecting and segmenting smoke regions in the visual images captured by the camera onboard an unmanned aerial vehicle (UAV). The differences of each two components of red, green, and blue (RGB) model and intensity in hue, saturation, and intensity (HSI) model of images are chosen as inputs of a fuzzy logic rule, while the smoke likelihood is selected as its output. Then, an extended Kalman filter (EKF) is further employed for reshaping the inputs and output of the fuzzy smoke detection rule on-line. It is expected to provide the smoke detection method with additional regulating flexibility adapting to variations of environmental conditions and reliable automatic detection performance. Next, the morphological operation is also adopted to remove imperfections induced by noises and textures distorted nonconvex/concave segments. Finally, extensive studies on several sets of images containing smoke under distinct environmental conditions are conducted to validate the proposed methodology. © 2018, Springer Nature B.V.},
}

@ARTICLE{Selim2019193,
author={Selim, S. and Sonmez, N.K. and Coslu, M. and Onur, I.},
title={Semi-automatic Tree Detection from Images of Unmanned Aerial Vehicle Using Object-Based Image Analysis Method},
journal={Journal of the Indian Society of Remote Sensing},
year={2019},
volume={47},
number={2},
pages={193-200},
note={cited By 9},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85057787223&doi=10.1007%2fs12524-018-0900-1&partnerID=40&md5=b56681149ee0076dfedcca5ebb47279e},
abstract={The aim of this study is detection of trees at low cost, fast and reliably through object-based image analysis method by using high-resolution unmanned aerial vehicles data. The study consists of three basic process stages. In the first stage, high-resolution aerial photographs were obtained by using unmanned aerial vehicles. Aerial photographs with approximately 1 cm spatial resolution were obtained from 30 m. flight height with 80% front overlap and 80% side overlap. Orthorectification, mosaicking, georeferencing and filtering processes were performed on the obtained photographs in order to make them ready for the analysis. Orthoimage in three spectral bands (Red, Green, Blue) and digital surface model were generated by processing the aerial images. The second stage of the study constitutes the most important process steps of object-based classification: They are segmentation and classification. In this phase, various parameters such as scale, shape and integrity were used to obtain the best result. Furthermore, accuracy assessments were performed through field observations. In the classification process step, a specified set of rules applied to segmentation result objects; thus, trees and other classes were determined in the study area. The generation of the rule sets was performed using the height information obtained from digital surface model and spectral data collected from orthoimages. Accuracy analysis was performed in the last stage of the study. The number of trees determined in the classification step was compared with the known number of the trees in the field. As the result of comparison, tree numbers and crown widths were found to be consistent. This study tests and implements a method that detects trees at low cost, fast and high accuracy which can be used in ecological studies and specially in determination of tree density. © 2018, Indian Society of Remote Sensing.},
}

@ARTICLE{Li2019688,
author={Li, W. and Qu, F. and Liu, P.},
title={Vehicle detection on unmanned aerial vehicle images based on saliency region detection},
journal={International Journal of Performability Engineering},
year={2019},
volume={15},
number={2},
pages={688-699},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85062886506&doi=10.23940%2fijpe.19.02.p33.688699&partnerID=40&md5=4c0eb6d8a6cde0a06c7c59e5a77e83a6},
abstract={The target detection and tracking technology of the unmanned aerial vehicle (UAV) is an important research direction in the field of UAV aerial photography. In order to effectively and accurately detect vehicles in a UAV platform and in complicated road environments, the authors proposed a vehicle detection method based on saliency region detection. First, the saliency map of the target is calculated by using the salient region detection method based on the optimized frequency-turned. Next, segmentation methods based on Boolean Map and OTSU are combined to determine the region of interest of the vehicle target in the saliency map image. Finally, a series of vehicle apparent features-based methods based on geometry, symmetry, and horizontal edge wave are used to determine the vehicle and eliminate the interference of roadside objects accurately. Experimental tests carried out from different datasets show excellent performance in multi-vehicle detection in terms of accuracy in complex traffic situations and under different scales and angles of aerial images, realizing fast vehicle detection on the UAV platform. © 2019 Totem Publisher, Inc. All rights reserved.},
}

@ARTICLE{Franceschini2019,
author={Franceschini, M.H.D. and Bartholomeus, H. and van Apeldoorn, D.F. and Suomalainen, J. and Kooistra, L.},
title={Feasibility of unmanned aerial vehicle optical imagery for early detection and severity assessment of late blight in Potato},
journal={Remote Sensing},
year={2019},
volume={11},
number={3},
art_number={224},
note={cited By 27},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85061357547&doi=10.3390%2frs11030224&partnerID=40&md5=068bc3a5922c0bb2375c4b4e0c19cc22},
abstract={Assessment of disease incidence and severity at farm scale or in agronomic trials is frequently performed based on visual crop inspection, which is a labor intensive task prone to errors associated with its subjectivity. Therefore, alternative methods to relate disease incidence and severity with changes in crop traits are of great interest. Optical imagery in the visible and near-infrared (Vis-NIR) can potentially be used to detect changes in crop traits caused by pathogen development. Also, cameras on-board of Unmanned Aerial Vehicles (UAVs) have flexible data collection capabilities allowing adjustments considering the trade-off between data throughput and its resolution. However, studies focusing on the use of UAV imagery to describe changes in crop traits related to disease infection are still lacking. More specifically, evaluation of late blight (Phytophthora infestans) incidence in potato concerning early discrimination of different disease severity levels has not been extensively reported. In this article, the description of spectral changes related to the development of potato late blight under low disease severity levels is performed using sub-decimeter UAV optical imagery. The main objective was to evaluate the sensitivity of the data acquired regarding early changes in crop traits related to disease incidence. For that, UAV images were acquired on four dates during the growing season (from 37 to 78 days after planting), before and after late blight was detected in the field. The spectral variability observed in each date was summarized using Simplex Volume Maximization (SiVM), and its relationship with experimental treatments (different crop systems) and disease severity levels (evaluated by visual assessment) was determined based on pixel-wise log-likelihood ratio (LLR) calculation. Using this analytical framework it was possible to identify considerable spectral changes related to late blight incidence in different treatments and also to disease severity level as low as between 2.5 and 5.0% of affected leaf area. Comparison of disease incidence and spectral information acquired using UAV (with 4-5 cm of spatial resolution) and ground-based imagery (with 0.1-0.2 cm of spatial resolution) indicate that UAV data allowed identification of patterns comparable to those described by ground-based images, despite some differences concerning the distribution of affected areas detected within the sampling units and an attenuation in the signal measured. Finally, although aggregated information at sampling unit level provided discriminative potential for higher levels of disease development, focusing on spectral information related to disease occurrence increased the discriminative potential of the data acquired. © 2019 by the authors.},
}

@ARTICLE{MahdinezhadGargari2019489,
author={Mahdinezhad Gargari, A. and Ebadi, H. and Esmaeili, F.},
title={An Efficient Algorithm for Detection of Image Stretching Error from a Collection of Images Acquired by Unmanned Aerial Vehicles},
journal={Arabian Journal for Science and Engineering},
year={2019},
volume={44},
number={1},
pages={489-504},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85060443956&doi=10.1007%2fs13369-018-3634-z&partnerID=40&md5=0b072d59d68309563d72390ba6d392e5},
abstract={Over the recent years, the advantages of using unmanned aerial vehicles (UAVs) have provided fascinating working areas, particularly for photogrammetric goals. One of the main problems preventing the UAV data to achieve fully automated processing is the image stretching error and reduced resolution or image blurring, which is caused by camera shake during shooting or slow shutter speed. Movements of the sensors may be due to normal motions during the flight, strong winds, lack of proper functioning of the gimbal stabilizer or an operator’s lack of skill for properly controlling the drone. Image blurring negatively affects data interpretation and visual analysis, which in turn raises challenges for detection and matching algorithms; as a result, the precision of automatic processing and accuracy of the extracted geometrical information would decrease. Time-consuming and costly manual methods are typically adopted to identify and remove images with radiometric errors. Such methods are tedious, especially for large datasets and bring about high margin of errors. In this paper, an automatic and reliable algorithm is presented to identify and distinguish blurred images. The aim is to extract the saturation blue difference (SBD) parameter from the sets of images. It is known that SBD value has a direct relationship with the amount of blurring. The numerical value of the parameter is determined based on the variation in the extracted edge pixels of blurred and non-blurred images. Evaluation on two datasets indicates that the proposed algorithm based on the selected threshold limit (defined with regard to the geometric and visual requirements of images) for the SBD values can recognize the images with the SBD values less than the threshold value as blurred images with 100% certainty and extract them from the sets of obtained images. © 2018, King Fahd University of Petroleum & Minerals.},
}

@CONFERENCE{Deeds20191078,
author={Deeds, J. and Engstrom, Z. and Gill, C. and Wood, Z. and Wang, J. and Ahn, I.S. and Lu, Y.},
title={Autonomous vision-based target detection using unmanned aerial vehicle},
journal={Midwest Symposium on Circuits and Systems},
year={2019},
volume={2018-August},
pages={1078-1081},
art_number={8623940},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85062218574&doi=10.1109%2fMWSCAS.2018.8623940&partnerID=40&md5=44fb9bb1342bb7463c3090d4138905a7},
abstract={In this paper, a vision-based target detection system using an Unmanned Aerial Vehicle (UAV) is developed to execute a mission plan. The mission plan is to autonomously take off to a specified altitude, fly to a waypoint with a predefined GPS coordinate, locate the target displayed by an AprilTag, hover above the target, then descend and land near the target. Our result shows that AprilTag is highly viable in UAV vision-based target detection. © 2018 IEEE},
}

@ARTICLE{Yang2019,
author={Yang, S. and Qin, H. and Liang, X. and Gulliver, T.A.},
title={An improved unauthorized unmanned aerial vehicle detection algorithm using radiofrequency-based statistical fingerprint analysis},
journal={Sensors (Switzerland)},
year={2019},
volume={19},
number={2},
art_number={274;},
note={cited By 8},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85060044118&doi=10.3390%2fs19020274&partnerID=40&md5=f6401f157f6c06551664fcefcacfe183},
abstract={Unmanned aerial vehicles (UAVs) are now readily available worldwide and users can easily fly them remotely using smart controllers. This has created the problem of keeping unauthorized UAVs away from private or sensitive areas where they can be a personal or public threat. This paper proposes an improved radio frequency (RF)-based method to detect UAVs. The clutter (interference) is eliminated using a background filtering method. Then singular value decomposition (SVD) and average filtering are used to reduce the noise and improve the signal to noise ratio (SNR). Spectrum accumulation (SA) and statistical fingerprint analysis (SFA) are employed to provide two frequency estimates. These estimates are used to determine if a UAV is present in the detection environment. The data size is reduced using a region of interest (ROI), and this improves the system efficiency and improves azimuth estimation accuracy. Detection results are obtained using real UAV RF signals obtained experimentally which show that the proposed method is more effective than other well-known detection algorithms. The recognition rate with this method is close to 100% within a distance of 2.4 km and greater than 90% within a distance of 3 km. Further, multiple UAVs can be detected accurately using the proposed method. © 2019 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@CONFERENCE{Min2019,
author={Min, Z. and Lin, L. and Aichen, W. and Xinhua, W.},
title={A novel farmland boundaries extraction and obstacle detection method based on unmanned aerial vehicle},
journal={2019 ASABE Annual International Meeting},
year={2019},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85084017525&doi=10.13031%2faim.201900369&partnerID=40&md5=5cbb0dbf1b06aac766e2207c16de80ed},
abstract={With the development of technology and the declining labor force, unmanned agricultural machinery is the inevitable development trend of agricultural machinery. The extraction of boundaries and obstacle detection are the key technology for unmanned agricultural machinery path planning. A novel method of farmland boundaries extraction and obstacle detection based on unmanned aerial vehicle was proposed in this paper. Firstly, to obtain the image of farmland, UAV flied at a low altitude with a camera and GPS, and each captured image has corresponding GPS information. Then image mosaic method was applied to get information on the entire field, where feature points were extracted by combining the improved SURF algorithm and Harris algorithm and refined feature points through combining Grid-KNN algorithm and RANSAC algorithm. After that, a transformation matrix was established by RANSAC algorithm, and the image of the UAV was spliced into a complete field map. Finally, farmland boundaries and obstacles were extracted based on the gPb algorithm through the complete field map. Experimental results show that the error between generated boundary and actual boundary is less than 0.2m, and all obstacles are identified and located. The novel method could be used in path planning and obstacle avoidance in unmanned agricultural machinery. © 2019 ASABE Annual International Meeting. All rights reserved.},
}

@CONFERENCE{Bernard2019,
author={Bernard, A. and Sciuchetti, G. and Lynch, C. and Sherpa, A. and Reiter, J. and Lum, C.W.},
title={Artificial light detection as a method for poacher detection from an unmanned aerial vehicle},
journal={AIAA Scitech 2019 Forum},
year={2019},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85083943955&doi=10.2514%2f6.2019-2284&partnerID=40&md5=d1a4ff8559243612961af562a94cc1dd},
abstract={Atypical methods of detection are required to accurately and consistently detect poachers in the African Savannah. A promising idea is utilizing unmanned aerial systems (UAS) to detect and monitor these poachers. This paper investigates the design and development a sensor system that can be mounted on a fixed wing UAS and integrated with other optical sensors. A trade study was conducted that determined that a light detection sensor had a strong possibility of success, but had to be developed using a light sensitive camera and a filtration script. Signal to noise ratio (SNR) was determined to be the main quantifiable metric for determining success, and initial feasibility calculations indicated that the intended design would perform well. The system was then successfully prototyped for flight testing. Several variables were measured including type of light source, weather conditions, camera mount angle, and direct or indirect light. Flight tests were successfully conducted, and post processing scripts were developed to flag images with light and determine SNR. It was found that the system delivered a higher SNR under cloudy weather, gave a decreasing SNR but increasing probability of detection by increasing mount angle and produced a higher SNR with light sources shined at the ground as opposed to directly at the UAS. Flight testing also determined the optimal exposure value of the system. © 2019, American Institute of Aeronautics and Astronautics Inc, AIAA. All rights reserved.},
}

@CONFERENCE{Lijia201947,
author={Lijia, C. and Yu, T. and Guo, Z.},
title={Adaptive observer-based fault detection and active tolerant control for unmanned aerial vehicles attitude system},
journal={IFAC-PapersOnLine},
year={2019},
volume={52},
number={24},
pages={47-52},
note={cited By 9},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85081053315&doi=10.1016%2fj.ifacol.2019.12.379&partnerID=40&md5=12d4a56aecc7cf7332b90ab2a5682548},
abstract={A robust adaptive observer combined with radial basis function neural network (RBFNN) is designed for the unmanned aerial vehicles (UAVs) fault-detection system is proposed in this paper. Firstly, the fault dynamics model with unknown disturbance of the unmanned aerial vehicle's attitude system is established, and a robust adaptive observer combined with radial basis function neural network is designed for the vehicle's fault-detection, then, the detected fault combined with a robust controller is applied to design the fault-tolerant controller. In the end, the stability and effective of the fault detection and tolerant system is proved by Lyapunov theory and simulation. © 2019 The Authors. Published by Elseiver Ltd. All rights reserved.},
}

@CONFERENCE{Yuan2019,
author={Yuan, C. and Liu, Z. and Hossain, A. and Zhang, Y.},
title={Fire detection using both infrared and visual images with application to unmanned aerial vehicle forest fire surveillance},
journal={Proceedings of the ASME Design Engineering Technical Conference},
year={2019},
volume={9},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85076394805&doi=10.1115%2fDETC2019-97895&partnerID=40&md5=cd8725619988d279e72248373707c304},
abstract={Forest fires are a universal problem that destroy a large amount of natural resources and creates environmental pollution. Forest firefighting is one of today’s most important events for natural and environmental resources protection and conservation. Unmanned aerial vehicle (UAV) with remote sensing system can offer a rapid, safe and low-cost approach for effective forest fire detection which have attracted researchers attention worldwide. In this paper, automatic detection of fire regions using both visual and infrared images is investigated. In order to improve the computational performance to satisfy the requirement of real-time processing, a reduced complexity fusion method is adopted in this research. Through testing the proposed approach on real video sequences, good detection performance is achieved and it is indicated that using multi-modal camera system to detect forest fire with application to firefighting UAV is very promising. Copyright © 2019 ASME.},
}

@ARTICLE{Kataev201955,
author={Kataev, M.Y. and Dadonova, M.M.},
title={Method of vegetation detection using rgb images made by unmanned aerial vehicles on the basis of colour and texture analysis},
journal={Light and Engineering},
year={2019},
volume={27},
number={8},
pages={55-62},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85074734617&doi=10.33383%2f2018-078&partnerID=40&md5=3e7d7b2503f15dec22e39c706a6d7ad8},
abstract={The article describes the capability of application of RGB 1 images made by digital cameras for detection of Earth surface (vegetation) types. A set of measures necessary to be taken for processing of the images made by unmanned aerial vehicles (UAV) in real-time is described. Application of analogue of vegetation index allows detecting vegetation on an RGB image, which increases the probability of correct detection of surface (vegetation) type. Methods of preliminary and thematic processing of images required for positive detection of surface types are considered. Texture analysis is applied for detection of vegetation type. The results of the processing of real images are provided. © 2019, LLC Editorial of Journal "Light Technik". All rights reserved.},
}

@ARTICLE{Wang201993937,
author={Wang, R. and Zhao, C. and Bai, Y. and Du, W. and Wang, J.},
title={An Actuator Fault Detection and Reconstruction Scheme for Hex-Rotor Unmanned Aerial Vehicle},
journal={IEEE Access},
year={2019},
volume={7},
pages={93937-93951},
art_number={8756018},
note={cited By 11},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85073892314&doi=10.1109%2fACCESS.2019.2927010&partnerID=40&md5=12bf898ac8702bbe6a81e36bc69cd31f},
abstract={The detection and the reconstruction of actuator faults in a flight control system are crucial to avoid negative impacts on the aircraft itself, as well as human and environmental systems. In this paper, an actuator fault detection and reconstruction scheme based on fault classification for the hex-rotor unmanned aerial vehicle are designed. First, the fault type of actuator is analyzed and classified, then an actuator fault model is established based on multiple fault classification. Second, a fault detection and reconstruction (FDR) scheme for the hex-rotor unmanned aerial vehicle is proposed. In the proposed scheme, a fault observer group based on an extended Kalman filter (EKF) is designed for fault detection and isolation, and the flight state feedback required by the fault observer group is provided by the multi-sensor navigation unit (MSNU). Then, a fault reconstruction algorithm of the actuator is proposed by using the output of the fault observer group. The designed FDR system is applied to hex-rotor unmanned aerial vehicle prototype for its evaluation. The simulation results show that the proposed design is capable of fault detection and the reconstruction of actuator faults, and the actual flight verifies the effectiveness of the proposed methods. © 2013 IEEE.},
}

@ARTICLE{Liang2019123,
author={Liang, C. and Miao, M. and Ma, J. and Yan, H. and Zhang, Q. and Li, X. and Li, T.},
title={Detection of GPS Spoofing Attack on Unmanned Aerial Vehicle System},
journal={Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
year={2019},
volume={11806 LNCS},
pages={123-139},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85072862820&doi=10.1007%2f978-3-030-30619-9_10&partnerID=40&md5=8c6a187410c85498b9108685f30219f2},
abstract={Most of the existing GPS spoofing detection schemes are vulnerable to the complex generative GPS spoofing attack, and require additional auxiliary equipments and extensive signal processing capabilities, leading to defects such as low real-time performance and large communication overhead which may not be available for the unmanned aerial vehicle (UAV, also known as drone) system. Motivated by the limitations of prior work, we propose a GPS spoofing detection scheme that requires minimal prior configuration and employs information fusion based on the GPS receiver and inertial measurement unit (IMU). We use a real-time model of tracking and calculating to derive the current location of the drones which are then contrasted with the location information received by the GPS receiver to judge whether the UAV system is under spoofing attack. Experiments show that, while the accuracy meets the requirements of detection, the proposed method can accurately determine whether the system is attacked within 8 s, with a detection rate of 98.6%. Compared with the existing schemes, the performance of real-time detecting is improved in our method while the detection rate is ensured. Even in our worst-case, we detect GPS spoofing attack within 28 s after the UAV system starts its mission. © 2019, Springer Nature Switzerland AG.},
}

@ARTICLE{Cao2019,
author={Cao, S. and Yu, Y. and Guan, H. and Peng, D. and Yan, W.},
title={Affine-function transformation-based object matching for vehicle detection from unmanned aerial vehicle imagery},
journal={Remote Sensing},
year={2019},
volume={11},
number={14},
art_number={1708},
note={cited By 6},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85071543757&doi=10.3390%2frs11141708&partnerID=40&md5=cf805f81737a008f1e082f3cbe73312d},
abstract={Vehicle detection from remote sensing images plays a significant role in transportation related applications. However, the scale variations, orientation variations, illumination variations, and partial occlusions of vehicles, as well as the image qualities, bring great challenges for accurate vehicle detection. In this paper, we present an affine-function transformation-based object matching framework for vehicle detection from unmanned aerial vehicle (UAV) images. First, meaningful and non-redundant patches are generated through a superpixel segmentation strategy. Then, the affine-function transformation-based object matching framework is applied to a vehicle template and each of the patches for vehicle existence estimation. Finally, vehicles are detected and located after matching cost thresholding, vehicle location estimation, and multiple response elimination. Quantitative evaluations on two UAV image datasets show that the proposed method achieves an average completeness, correctness, quality, and F1-measure of 0.909, 0.969, 0.883, and 0.938, respectively. Comparative studies also demonstrate that the proposed method achieves compatible performance with the Faster R-CNN and outperforms the other eight existing methods in accurately detecting vehicles of various conditions. © 2019 by the authors.},
}

@ARTICLE{Kartashov2019771,
author={Kartashov, V.M. and Oleynikov, V.N. and Sheyko, S.A. and Babkin, S.I. and Korytsev, I.V. and Zubkov, O.V.},
title={Peculiarities of small unmanned aerial vehicles detection and recognition},
journal={Telecommunications and Radio Engineering (English translation of Elektrosvyaz and Radiotekhnika)},
year={2019},
volume={78},
number={9},
pages={771-781},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85066440306&doi=10.1615%2fTelecomRadEng.v78.i9.30&partnerID=40&md5=5677c3d7b9727159c280343491f1acfd},
abstract={Review and analysis of methods for detection and recognition of unmanned aerial vehicles (UAVs) are carried out. The channels for the detection of UAVs - acoustic, optical, radar, infrared, radio channel are discussed. The advantages and disadvantages of the channels used are compared and appreciated. In the case of small UAVs, there are a number of significant difficulties and limitations. One of the directions in the UAVs detection is acoustic observation. The noise generated by the UAV propulsion system and the air propeller is a significant damasking feature. Creating and improving methods for detecting, guiding and recognizing small UAVs by the reception and processing their sound signals is an urgent task. When using such a method of detecting UAVs, frequency spectra, spectrograms, normalized autocorrelation functions, and phase portraits of acoustic signals are used. Estimates of spectral coefficients, determined by a discrete realization containing a predetermined number of samples, as well as parameters of autoregression models can serve as information signs of the UAVs sound image. ©2019 by Begell House, Inc.},
}

@ARTICLE{Oleynikov2019759,
author={Oleynikov, V.N. and Zubkov, O.V. and Kartashov, V.M. and Korytsev, I.V. and Babkin, S.I. and Sheiko, S.A.},
title={Investigation of detection and recognition efficiency of small unmanned aerial vehicles on their acoustic radiation},
journal={Telecommunications and Radio Engineering (English translation of Elektrosvyaz and Radiotekhnika)},
year={2019},
volume={78},
number={9},
pages={759-770},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85066425797&doi=10.1615%2fTelecomRadEng.v78.i9.20&partnerID=40&md5=a22afbb175367a2090bb264307250b96},
abstract={The features of acoustic spectrum of UAVs, spectrum of natural and industrial acoustic noise, noise spectrum of automobile and rail transport, and human speech spectrum were investigated. The method for recognition of UAV sound based on the Mel-frequency cepstral coefficients was proposed. The universal method for detecting UAV based on characteristic features of acoustic spectrum was proposed as well. Both methods were tested using experimental recordings of UAVs and noise sounds and got close well results. The universal recognition method has some worse recognition reliability and false alarm probability, but does not need creation of sound and noise images base. © 2019 by Begell House, Inc.},
}

@ARTICLE{Hu2019214,
author={Hu, Y. and Cao, Y. and Ding, M. and Zhuang, L.},
title={Airport detection for fixed-wing unmanned aerial vehicle landing using a hierarchical architecture},
journal={Journal of Aerospace Information Systems},
year={2019},
volume={16},
number={6},
pages={214-223},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85066400653&doi=10.2514%2f1.I010615&partnerID=40&md5=ba8cb077725ac4e85fe61418c5e20750},
abstract={Airport detection plays an important role in vision-based fixed-wing unmanned aerial vehicle landing. A large amount of image analysis is required for vision-based detection. This paper addresses the efficiency and difficulty of airport detection in the initial stage of landing. A hierarchical architecture and a decision criterion are proposed to quickly locate candidate airport regions. Then, the spatial-pyramid matching using sparse coding algorithm is used to obtain a more discriminative feature map representation of airports. A linear support vector machine is employed to recognize potential airports from feature maps. Several experiments are conducted to test the robustness and efficiency of the proposed algorithm. Promising results are obtained under challenging backgrounds and different weather conditions. Copyright © 2019 by the American Institute of Aeronautics and Astronautics, Inc. All rights reserved.},
}

@CONFERENCE{Huai2019,
author={Huai, B. and Wang, R. and Liu, Y. and Song, L. and Peng, Z.},
title={Missing pins detection for power equipment firmware using unmanned aerial vehicle images},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2019},
volume={10843},
art_number={108430S},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85062466392&doi=10.1117%2f12.2506338&partnerID=40&md5=bd92f50fd2b129c869d83f1c53caaac1},
abstract={Maintenance of power equipment is of great significance to ensure the safety and reliability of power equipment. This paper focuses on detecting missing pins of power equipment using Unmanned Aerial Vehicle （UAV） acquired images. We proposed a detection method based on image color histogram and scale invariant feature transform (SIFT). The first step calculates the H-S color histogram of screw image, utilizing histogram back projection method to obtain candidate regions of screw image in the to-be-matched image, applied Bhattacharyya distance as a measurement to compare the similarity of two histograms. Then, the SIFT feature is extracted from the screw image and the key points are matched with the SIFT feature of the candidate regions to detect the screws. Finally, this paper designs a method which uses convolutional neural network to judge whether the screw misses the pin. Experiments show that the proposed algorithm of missing pins detection based on UAV image can achieve competitive results to detect the defects in special scenes, and has good robustness, which satisfies the real-time and accuracy requirements. © 2019 SPIE.},
}

@ARTICLE{Li201934,
author={Li, Z. and Meng, C. and Zhou, F. and Ding, X. and Wang, X. and Zhang, H. and Guo, P. and Meng, X.},
title={Fast vision-based autonomous detection of moving cooperative target for unmanned aerial vehicle landing},
journal={Journal of Field Robotics},
year={2019},
volume={36},
number={1},
pages={34-48},
note={cited By 10},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85055162684&doi=10.1002%2frob.21815&partnerID=40&md5=a6953aacaae70d9027334939899d3cba},
abstract={We propose a fast and effective method, fast target detection (FTD), to detect the moving cooperative target for the unmanned aerial vehicle landing, and the target is composed of double circles and a cross. The purpose of our strategy is to land on the target. The FTD method needs to detect the target at the high and low heights. At the high height, the target appears completely and stably in the camera field. The FTD method can detect the circle and cross to rapidly reach the target center, named cross and circle–FTD (C2 − FTD). To detect the cross, we propose a slope distance equation to obtain the distance between two slopes. The proposed slopes cluster method, based on the distance equation and K-means, is used to determine the cross center. At the low height, the target appears incompletely and unstably. Therefore, FTD methods detect only the cross, named cross–FTD (C1 − FTD). We extract the cross features (CFs) based on line segments. Then, four CFs are combined based on graph theory. Experiments on our four datasets show that FTD has rapid speed and good performance. (Our method is implemented in C++ and is available at https://github.com/Li-Zhaoxi/UAV-Vision-Servo.) On the Mohamed Bin Zayed International Robotics Challenge datasets made we constructed, C2 − FTD detects the target from a 960 × 540 image approximately 20ms per pipeline with 82.24% F-measure and tracks target approximately 6.27ms per pipeline with 94.39% F-measure. C1 − FTD detects centers from a 480 × 270 image at approximately 4.69ms per image with 86.05% F-measure. © 2018 Wiley Periodicals, Inc.},
}

@ARTICLE{Wang2019885,
author={Wang, Y. and Ma, H. and Wei, S. and Zhang, S. and Feng, Z. and Wei, Z.},
title={Sound detection and alarm system of unmanned aerial vehicle},
journal={Advances in Intelligent Systems and Computing},
year={2019},
volume={752},
pages={885-898},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85053247720&doi=10.1007%2f978-981-10-8944-2_103&partnerID=40&md5=27d4d7c9dd49dc10a3acbe27da4ff8c1},
abstract={Unmanned aerial vehicles (UAVs) are widely applied in the civil domain. Meanwhile, the security issues concerning UAVs are emerging because the monitoring of small UAVs is difficult. In this paper, we designed a sound detection and alarm system for UAV monitoring. Firstly, the frequency domain feature extraction and Mel domain feature extraction are performed to obtain the features of UAV sound. The Mel frequency cepstral coefficient (MFCC) and support vector machine (SVM)-based sound detection method are designed. Besides, the real-time sound acquisition and detection are realized. The real test data has proved the efficiency of the designed UAV sound detection system. The advantages of the sound detection and alarm system in this paper are low cost and high accuracy, which may be widely applied in the area of UAV monitoring. © Springer Nature Singapore Pte Ltd. 2019.},
}

@CONFERENCE{Esfahlani20182757,
author={Esfahlani, S.S. and Cirstea, S. and Sanaei, A. and Cirstea, M.},
title={Fire detection of unmanned aerial vehicle in a mixed reality-based system},
journal={Proceedings: IECON 2018 - 44th Annual Conference of the IEEE Industrial Electronics Society},
year={2018},
pages={2757-2762},
art_number={8592764},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85061553417&doi=10.1109%2fIECON.2018.8592764&partnerID=40&md5=1c2b0ba52e408676dc4ae30c2805a4db},
abstract={This paper presents a system that combines robotic operating system (ROS) and computer vision techniques for fire detection in a mixed reality environment. We have collected video streams from a mini camera on an Unmanned Aerial Vehicle (UAV), where the navigation data relied on state-of-the-art Simultaneous Localization and Mapping (SLAM) system. The data collected onboard are communicated to the ground station and processed through the robotic operating system. A robust and efficient re-localisation SLAM was performed to recover from tracking failure and frame lost in the received data. The fire detection algorithm was developed based on the colour, movement attributes, temporal variation of fire intensity and its accumulation around a point. A mixed reality environment was used to visualise and test the proposed system. The observation and data analysis confirmed that the UAV could successfully detect fire and flame, fly towards and hover around it. © 2018 IEEE.},
}

@CONFERENCE{Krause20182299,
author={Krause, P. and Salahat, E. and Franklin, E.},
title={Diurnal thermal dormant landmine detection using unmanned aerial vehicles},
journal={Proceedings: IECON 2018 - 44th Annual Conference of the IEEE Industrial Electronics Society},
year={2018},
pages={2299-2304},
art_number={8591378},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85061537818&doi=10.1109%2fIECON.2018.8591378&partnerID=40&md5=b4edb77f97db32d7435dc5d87c517b75},
abstract={The detection of the metallic content of landmines is the predominant methodology employed to locate active mines. Contemporary landmines replace previously metal components with plastics, wood and glass to avoid detection. The situation has required increasingly sensitive metal detection equipment which may not always be available or effective. However, the internal explosives material has remained largely consistent. This paper exploits the changing thermal mass of this explosives material as it is heated by the sun, cooling at a delayed rate of the surrounding soil temperature. This change is recorded and measured by a thermal camera attached to an Unmanned Aerial Vehicle (UAV) over several diurnal cycles, and then analyzed to identify the location of a buried landmine. A series of thermal images of surrogate landmines captured in October-November 2017, revealed clear shapes, with >2 Kelvin thermal differences to their surroundings. This indicates that UAV thermal imaging can be used for landmine detection. The techniques and method presented in this paper can be easily replicated, resulting in the identification, removal of dormant landmines in most environments, saving lives and reducing casualties. © 2018 IEEE.},
}

@CONFERENCE{Dias2018357,
author={Dias, T.M. and Alves, V.C. and Alves Junior, H.M. and Pinheiro, L.F. and Pontes, R.S.G. and Araujo, G.M. and Lima, A.A. and Prego, T.M.},
title={Autonomous detection of mosquito-breeding habitats using an unmanned aerial vehicle},
journal={Proceedings - 15th Latin American Robotics Symposium, 6th Brazilian Robotics Symposium and 9th Workshop on Robotics in Education, LARS/SBR/WRE 2018},
year={2018},
pages={357-362},
art_number={8588576},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85061328694&doi=10.1109%2fLARS%2fSBR%2fWRE.2018.00070&partnerID=40&md5=f0134d27548567c290211927e2fd6791},
abstract={Every year, thousands of people die from diseases such as dengue fever, chikungunya, and zika. This public health problem is more evident in developing countries. All these illnesses have the same source in common: A mosquito scientifically known as Aedes Aegypti. In cities, the majority of mosquito-breeding habitats are man-made: bottles, tires, barrels, pots or any stagnant water. This paper proposes an innovative system to aid in determining mosquito-breeding habitats location by employing computer vision tools on aerial images. Tires and regions with stagnant water were selected as objects of study. For this, a dataset was created containing video sequences and telemetry data from an unmanned aerial vehicle (UAV) and the respective manual annotation in different scenarios. The features extracted from the videos (through HSV color space, histograms, and edge detection) were used to train a random forest classifier, resulting in an accuracy higher than 99% in the test set. The system is also capable of automatically determining the GPS coordinates of the possible mosquito breeding location with similar precision to commercial GPS equipment. © 2018 IEEE.},
}

@CONFERENCE{Zhang2018309,
author={Zhang, J. and Zhang, Q. and Shi, C.},
title={An unmanned aerial vehicle detection algorithm based on semantic segmentation and visual attention mechanism},
journal={ACM International Conference Proceeding Series},
year={2018},
pages={309-313},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85062782717&doi=10.1145%2f3297156.3297269&partnerID=40&md5=07b163dae61918152a5eeefc0b9a88c8},
abstract={Combined with semantic segmentation and visual attention mechanism, a new method for UAV detection in complex background is presented. The semantic segmentation of target image, which is implemented by Mask R-CNN, is used to exclude invalid regions. Then the processes of small target detection based on visual attention mechanism is built. This method is used to detecting the position of UAV in the sky. The effectiveness of algorithm proposed in this paper is proved by a large number of experiments. © 2018 Association for Computing Machinery.},
}

@CONFERENCE{Weihua2018,
author={Weihua, W. and Peizao, W. and Zhaodong, N.},
title={A Real-time Detection Algorithm for Unmanned Aerial Vehicle Target in Infrared Search System},
journal={2018 IEEE International Conference on Signal Processing, Communications and Computing, ICSPCC 2018},
year={2018},
art_number={8567718},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85060470245&doi=10.1109%2fICSPCC.2018.8567718&partnerID=40&md5=702be81db8d2fc2fd367f27386af002a},
abstract={Aiming at the difficulty of infrared target detection of 'low and slow small' unmanned aerial vehicles (UAV) in complex low-altitude background, this paper proposes a new target detection algorithm based on multiscale fusion filtering. Combined with spatial multiscale decomposition filtering and temporal multiscale difference processing, the algorithm can effectively overcome many difficulties such as complex Iow-altitude background interference, unknown target scale, unknown angular velocity and low target signal-to-noise ratio (SNR). The test result shows that the algorithm can effectively detect the UAV targets with different distances in complex Iow-altitude background, and the false alarm rate is low. The algorithm is realized in TI 6657 DSP and realizes 100Hz real-time processing of mid-wave infrared images with 640∗512 resolution, which has been effectively applied to the large-field circumferential scanning infrared search system developed by ATR Lab. © 2018 IEEE.},
}

@ARTICLE{Murray201845,
author={Murray, B. and Anderson, D.T. and Wescott, D.J. and Moorhead, R. and Anderson, M.F.},
title={Survey and insights into unmanned aerial-vehicle-based detection and documentation of clandestine graves and human remains},
journal={Human Biology},
year={2018},
volume={90},
number={1},
pages={45-61},
note={cited By 10},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85055911394&doi=10.13110%2fhumanbiology.90.1.03&partnerID=40&md5=ae14346a7f432cdb4adcae6243d0d44a},
abstract={Numerous biological and archaeological studies have demonstrated the legitimacy of remote sensing in anthropology. This article focuses on detecting and documenting terrestrial clandestine graves and surface remains (CGSR) of humans using unmanned aerial vehicles (UAVs), sensors, and automatic processing algorithms. CGSR is a problem of complex decision making under uncertainty that requires the identifĳication and intelligent reasoning about direct evidence of human remains and their environmental fĳingerprints. As such, it is as much an engineering and geospatial problem as it is an anthropology problem. This article is an efffort to survey existing work across disciplines and to provide insights and recommendations to assist future research. To support our claims, preliminary experiments were performed at the Forensic Anthropological Research Facility at Texas State University using UAVs, hyperspectral imaging, thermal imaging, and structure from motion. Prior work, our experience, and preliminary results indicate that both great potential and extreme challenges face remote sensing of CGSR. © 2018 Wayne State University Press, Detroit, Michigan 48201.},
}

@CONFERENCE{Fradi20181047,
author={Fradi, H. and Bracco, L. and Canino, F. and Dugelay, J.-L.},
title={Autonomous person detection and tracking framework using unmanned aerial vehicles (UAVs)},
journal={European Signal Processing Conference},
year={2018},
volume={2018-September},
pages={1047-1051},
art_number={8553010},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85059811537&doi=10.23919%2fEUSIPCO.2018.8553010&partnerID=40&md5=13c43a7cc8ba435f32267705789684c2},
abstract={While person tracking has made significant progress over the last few years, most of the existing approaches are of limited success in real-time applications using moving sensors. In particular, we emphasize in this paper the need for a visual tracker that enables autonomous navigation functionality to drones (UAVs), mainly to follow a specific target. To achieve this goal, a color-based detection framework is proposed. The approach includes as well the execution of control commands, which are essential to switch from the detection to automatically follow the detected target. Our proposed approach is evaluated on videos recorded by drones. The obtained results demonstrate the effectiveness of the proposed approach to accurately follow a target in real-time, and despite different challenges such as lighting changes, speed, and occlusions. © EURASIP 2018.},
}

@CONFERENCE{Zacharie2018230,
author={Zacharie, M. and Fuji, S. and Minori, S.},
title={Rapid Human Body Detection in Disaster Sites Using Image Processing from Unmanned Aerial Vehicle (UAV) Cameras},
journal={2018 International Conference on Intelligent Informatics and Biomedical Sciences, ICIIBMS 2018},
year={2018},
pages={230-235},
art_number={8549955},
note={cited By 7},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85060056312&doi=10.1109%2fICIIBMS.2018.8549955&partnerID=40&md5=fdd1251be461459ba8b235e3aa43a951},
abstract={The development and impact of technology on our everyday lives cannot be compared with the world our ancestors lived in several decades ago. This is described as the world of technology (WoT). But despite all the advancements in technologies, understanding of the mechanisms of nature and the damages caused via natural disasters, such as earthquakes, landslides, and flooding to mention only a few, are still very far away. In the effort of saving lives during natural disasters, such as earthquakes, this study introduces a rapid human body detection using image processing from UAV camera. The skin color from a female student is first extracted in RGB then converted to HSV. Next, opening and closing morphological operations are performed eight times each to remove all noise present in the image. Experimental tests were performed both indoor and outdoor, where the female student presented an object close and far to the camera to check the detection capability in both cases. The experiment results show that close or far, the camera can clearly detect both a human body and any part of a human body. The results of the experiment proves the merit of the proposed method. © 2018 IEEE.},
}

@ARTICLE{Xiong201823,
author={Xiong, J. and Liu, Z. and Lin, R. and Chen, S. and Chen, W. and Yang, Z.},
title={Unmanned Aerial Vehicle Vision Detection Technology of Green Mango on Tree in Natural Environment [自然环境下树上绿色芒果的无人机视觉检测技术]},
journal={Nongye Jixie Xuebao/Transactions of the Chinese Society for Agricultural Machinery},
year={2018},
volume={49},
number={11},
pages={23-29},
note={cited By 9},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85061374426&doi=10.6041%2fj.issn.1000-1298.2018.11.003&partnerID=40&md5=ff084894628f200968e8db6a12a25a93},
abstract={In order to detect the mango yield on trees rapidly, a green mango visual detection method based on unmanned aerial vehicle (UAV) was proposed. The deep learning technology and the YOLOv2 model were adopted to detect the mango images captured by UAV. Firstly, totally 471 images of the mango on trees were collected by the UAV. To meet the demand of diversity, totally 360 images included different shooting distances and different lighting situations were selected. Among which, 300 images were selected randomly as the training set, the other 60 images were used as the test set. Also, the shooting plan of the whole tree was designed. By image collecting and image mosaic, the integrated images of five mango trees were worked out for the yield estimating experiment of mango. After image collection, these images were marked manually and used to build the training set and the test set. The batch size and the initial learning rate were determined by experiments. During the model training, the learning rate was reduced gradually as the training times were changed. The mean average precision (MAP) of the trained model on the training set was 86.43%. By designing the experiments, the accuracy of mango recognition with images that containing different fruit numbers and different lighting conditions was worked out. Also, the yield estimation experiment was designed. The experimental results showed that the average running time of an image using the given algorithm was 0.08 s, while the accuracy of the teat set was 90.64% and the false recognition rate was 9.36%; the highest recognition accuracy of image with different numbers of fruits was 94.55% and the lowest was 88.05%. The recognition accuracy was 93.42% under the condition of direct sunlight, and the recognition accuracy was 87.18% under the condition of backlight. The average error of the yield estimation of mango tree was 12.79%. The result demonstrated that the algorithm was effective for mango in natural environment, which can provide technical support for estimating the yield of fruits and vegetables in intelligent agricultural production. © 2018, Chinese Society of Agricultural Machinery. All right reserved.},
}

@CONFERENCE{Hristov2018,
author={Hristov, G. and Raychev, J. and Kinaneva, D. and Zahariev, P.},
title={Emerging Methods for Early Detection of Forest Fires Using Unmanned Aerial Vehicles and Lorawan Sensor Networks},
journal={2018 28th EAEEIE Annual Conference, EAEEIE 2018},
year={2018},
art_number={8534245},
note={cited By 22},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85059017541&doi=10.1109%2fEAEEIE.2018.8534245&partnerID=40&md5=dd50d94cc1b482641834af6e3c20e29c},
abstract={Forest fires are occurring throughout the year with an increasing intensity in the summer and autumn periods. These events are mainly caused by the actions of humans, but different nature and environmental phenomena, like lightning strikes or spontaneous combustion of dried leafs or sawdust, can also be credited for their occurrence. Regardless of the reasons for the ignition of the forest fires, they usually cause devastating damage to both nature and humans. Forest fires are also considered as a main contributor to the air pollution, due to the fact that during every fire huge amounts of gases and particle mater are released in the atmosphere. To fight forest fires, different solutions were employed throughout the years. They ware primary aimed at the early detection of the fires. The simplest of these solutions is the establishment of a network of observation posts - both cheap and easy to accomplish, but also time-consuming for the involved people. The constant evolution of the information and communication technologies has led to the introduction of a new generation of solutions for early detection and even prevention of forest fires. ICT-based networks of cameras and sensors and even satellite-based solutions were developed and used in the last decades. These solutions have greatly decreased the direct involvement of humans in the forest fire detection process, but have also proven to be expensive and hard to maintain. In this paper we will discuss and present two different emerging solutions for early detection of forest fires. The first of these solutions involves the use of unmanned aerial vehicles (UAVs) with specialized cameras. Several different scenarios for the possible use of the drones for forest fire detection will be presented and analysed, including a solution with the use of a combination between a fixed-wind and a rotary-wing UAVs. In the next chapter of the paper, we will present and discuss the possibilities for development of systems for early forest fire detection using LoRaWAN sensor networks and we will analyse and present some of the hardware and software components for the realisation of such sensor networks. The paper will also provide another point-of-view, which will present the involvement of students in the development and in the use of both systems and we will analyse the advantages and the benefits, which the students will gain from their work on and with these solutions. © 2018 IEEE.},
}

@ARTICLE{NaveenKumar2018165,
author={Naveen Kumar, K. and Prasad, G. and Rajasekar, K. and Vadivelu, P. and Gollakota, S. and Kavinprabhu, S.K.},
title={A study on the forest fire detection using unmanned aerial vehicles},
journal={International Journal of Mechanical and Production Engineering Research and Development},
year={2018},
volume={8},
number={Special Issue 7},
pages={165-171},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85069657572&doi=10.24247%2fijmperddec201819&partnerID=40&md5=cc907cab400001b8a24d27bcd0baeb66},
abstract={Forest fires lead to the demolition of the forest and the wildlife that reside in them, and have a disastrous social, economic and environmental impact. Unmanned Aerial Vehicles (UAVs), due to their quick response capacity, low cost and without danger, as no human pilot onboard, with computer vision-based systems have great potential for monitoring and detecting forest fires. The integration of UAV technology with remote sensing techniques is a better solution for a forest fire. This article proposes a novel forest fire detection method using a payload calculation to carry a camera and thermal Image Sensing. A better performance is obtained to significantly improve the accuracy of forest fire detection and reduce false alarm rates. © TJPRC Pvt. Ltd.},
}

@ARTICLE{Yang2018,
author={Yang, S. and Talbot, R.W. and Frish, M.B. and Golston, L.M. and Aubut, N.F. and Zondlo, M.A. and Gretencord, C. and McSpiritt, J.},
title={Natural gas fugitive leak detection using an unmanned aerial vehicle: Measurement system description and mass balance approach},
journal={Atmosphere},
year={2018},
volume={9},
number={10},
art_number={383},
note={cited By 29},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85054397380&doi=10.3390%2fatmos9100383&partnerID=40&md5=fb6157b3e0308e497105e87428d81fa6},
abstract={Natural gas is an abundant resource across the United States, of which methane (CH4) is the main component. About 2% of extracted CH4 is lost through leaks. The Remote Methane Leak Detector (RMLD)-Unmanned Aerial Vehicle (UAV) system was developed to investigate natural gas fugitive leaks in this study. The system is composed of three major technologies: miniaturized RMLD (mini-RMLD) based on Backscatter Tunable Diode Laser Absorption Spectroscopy (TDLAS), an autonomous quadrotor UAV and simplified quantification and localization algorithms. With a miniaturized, downward-facing RMLD on a small UAV, the system measures the column-integrated CH4 mixing ratio and can semi-autonomously monitor CH4 leakage from sites associated with natural gas production, providing an advanced capability in detecting leaks at hard-to-access sites compared to traditional manual methods. Automated leak characterization algorithms combined with a wireless data link implement real-time leak quantification and reporting. This study placed particular emphasis on the RMLD-UAV system description and the quantification algorithm development based on a mass balance approach. Early data were gathered to test the prototype system and to evaluate the algorithm performance. The quantification algorithm derived in this study tended to underestimate the gas leak rates and yielded unreliable estimations in detecting leaks under 7 × 10-6 m3/s (~1 Standard Cubic Feet per Hour (SCFH)). Zero-leak cases can be ascertained via a skewness indicator, which is unique and promising. The influence of the systematic error was investigated by introducing simulated noises, of which Global Positioning System (GPS) noise presented the greatest impact on leak rate errors. The correlation between estimated leak rates and wind conditions were investigated, and steady winds with higher wind speeds were preferred to get better leak rate estimations, which was accurate to approximately 50% during several field trials. High precision coordinate information from the GPS, accurate wind measurements and preferred wind conditions, appropriate flight strategy and the relative steady survey height of the system are the crucial factors to optimize the leak rate estimations. © 2018 by the authors.},
}

@ARTICLE{Pan20183701,
author={Pan, Y. and Zhang, X. and Cervone, G. and Yang, L.},
title={Detection of Asphalt Pavement Potholes and Cracks Based on the Unmanned Aerial Vehicle Multispectral Imagery},
journal={IEEE Journal of Selected Topics in Applied Earth Observations and Remote Sensing},
year={2018},
volume={11},
number={10},
pages={3701-3712},
art_number={8454262},
note={cited By 40},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85052830256&doi=10.1109%2fJSTARS.2018.2865528&partnerID=40&md5=a6922afb359819db6db899fb4a9951b5},
abstract={Asphalt roads are the basic component of a land transportation system, and the quality of asphalt roads will decrease during the use stage because of the aging and deterioration of the road surface. In the end, some road pavement distresses may appear on the road surface, such as the most common potholes and cracks. In order to improve the efficiency of pavement inspection, currently some new forms of remote sensing data without destructive effect on the pavement are widely used to detect the pavement distresses, such as digital images, light detection and ranging, and radar. Multispectral imagery presenting spatial and spectral features of objects has been widely used in remote sensing application. In our study, the multispectral pavement images acquired by unmanned aerial vehicle (UAV) were used to distinguish between the normal pavement and pavement damages (e.g., cracks and potholes) using machine learning algorithms, such as support vector machine, artificial neural network, and random forest. Comparison of the performance between different data types and models was conducted and is discussed in this study, and indicates that a UAV remote sensing system offers a new tool for monitoring asphalt road pavement condition, which can be used as decision support for road maintenance practice. © 2008-2012 IEEE.},
}

@ARTICLE{Yang20183230,
author={Yang, J. and Yin, D. and Cheng, Q. and Shen, L.},
title={Two-layered mechanism of online unmanned aerial vehicles conflict detection and resolution},
journal={IEEE Transactions on Intelligent Transportation Systems},
year={2018},
volume={19},
number={10},
pages={3230-3244},
art_number={8194934},
note={cited By 8},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85038814961&doi=10.1109%2fTITS.2017.2771465&partnerID=40&md5=acd1a43abb8b4f5341570c17ec5fba8c},
abstract={This paper presents a study on short-term cooperative conflict detection and resolution (CDR) of unmanned aerial vehicles (UAVs). A two-layered CDR mechanism is proposed, which aims at guaranteeing safe separation, minimizing the overall cost of UAVs, and improving computational efficiency. In the first layer, the information from the environment is processed. In the second layer, conflicts among UAVs are resolved by applying the local centralized optimization method, with consideration given to the dynamic constraints of UAVs. This paper studies the safe separation constraints of pairwise conflicts in virtue of a geometry-based method. A heading change and speed change mixed conflict resolution approach is applied. To meet with the online planning requirements, the vectorized stochastic parallel gradient descent-based method is proposed to find the local optimal heading change solutions. The linear safe separation constraints on speeds are derived. A periodicity feature-based method is used to depart the feasible sub-regions for each pairwise conflict. A mixed integer linear programming model is established to find the optimal speed change solutions. The experiments results show that the proposed heading change algorithm could greatly reduce the summation of additional flight distances of UAVs, and influences on air traffic, compared with other short-term algorithms; the computational efficiency of this algorithm satisfies the online planning requirement. Comparing with the existing algorithm, our speed change algorithm reduces the number of feasible sub-regions to 2nc times lower, where nc is the number of pairwise conflict, and therefore, it reduces computation time dramatically. © 2018 IEEE.},
}

@CONFERENCE{Lopes-Esteves2018,
author={Lopes-Esteves, J. and Cottais, E. and Kasmi, C.},
title={Software Instrumentation of an Unmanned Aerial Vehicle for HPEM Effects Detection},
journal={2018 2nd URSI Atlantic Radio Science Meeting, AT-RASC 2018},
year={2018},
art_number={8471395},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85055782264&doi=10.23919%2fURSI-AT-RASC.2018.8471395&partnerID=40&md5=fed7707f965b3ee3ead714d1a618c4f1},
abstract={Unmanned aerial vehicles are spreading and their malicious use considered as a plausible threat against critical infrastructures. Their neutralization is of high interest for security aware organizations and high power directed energy weapons have been proposed. Therefore, the analysis of the susceptibility of such devices is of fundamental interest for both offensive and defensive purposes. Many studies were devoted to detecting the effects of electromagnetic interference on electronic devices and a recently proposed approach as shown to provide insight on the impact of hardware effects at the software level on tested targets. In this study, the application of this approach on a civilian unmanned aerial vehicle is proposed, consisting of designing and running specific software on the target in order to monitor well chosen observables during susceptibility testing. The methodology to run arbitrary software and to identify interesting observables is detailed. Interesting effects were detected, opening the scope to both neutralization and hardening strategies. © 2018 International Union of Radio Science URSI.},
}

@CONFERENCE{Wang2018439,
author={Wang, J. and Guo, W. and Pan, T. and Yu, H. and Duan, L. and Yang, W.},
title={Bottle Detection in the Wild Using Low-Altitude Unmanned Aerial Vehicles},
journal={2018 21st International Conference on Information Fusion, FUSION 2018},
year={2018},
pages={439-444},
art_number={8455565},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85054058826&doi=10.23919%2fICIF.2018.8455565&partnerID=40&md5=34ffdededb5eb91f941766fc90fbf4e5},
abstract={In this paper, we propose a new dataset and benchmark for low altitude UAV object detection, aiming to find and localize waste plastic bottles in the wild, as well as to inspire the development of object detection models to be capable of detecting small and transparent objects. To this end, we collect 25, 407 UAV images of bottles with various kinds of backgrounds. Unlike traditional horizontal bounding box based annotation methods, we use the oriented bounding box to accurately and compactly annotate the bottles, which provides more detailed information for subsequent robotic grasping. The fully annotated images contain 34, 791 bottles, each of which is annotated by an arbitrary (5 d.o.f.) quadrilateral. To build a baseline for bottle detection, we evaluate several state-of-the-art object detection algorithms on our UAV-Bottle Dataset (UAV-BD), such as Faster R-CNN, SSD, YOLOv2 and RRPN. We also present an analysis of the dataset along with baseline approaches. Both the dataset and benchmark are made publicly available to the vision community on our website to advance research in the area of object detection from UAVs. © 2018 ISIF},
}

@CONFERENCE{Kakillioglu2018,
author={Kakillioglu, B. and Velipasalar, S. and Rakha, T.},
title={Autonomous heat leakage detection from unmanned aerial vehicle-mounted thermal cameras},
journal={ACM International Conference Proceeding Series},
year={2018},
art_number={a11},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85056659181&doi=10.1145%2f3243394.3243696&partnerID=40&md5=8d01951afba5a64a8e943a08cd09d665},
abstract={The efficiency of thermal insulation of buildings has direct impact on power consumption for heating and ventilation. Thermal leaks are critical defects on building insulation. Infrared sensitive handheld thermal cameras are commonly used to perform manual inspection of buildings to detect thermal leaks by human experts. In this paper, we propose an algorithm that autonomously detects heat leakages from thermal images of building structures. The target platform for the proposed algorithm is an unmanned aerial vehicle (UAV) that collects thermal images of buildings, and detects heat leakages autonomously. Using UAVs, as opposed to the current practice of doing manual inspection, not only speeds up the process, but also provides the capability of capturing data from hard to reach places, such as roofs, in a more convenient and safe manner. For evaluation, thermal images have been captured both from inside, by a handheld camera, and outside. The outside thermal images have been captured by either a handheld camera or an IR camera installed on a UAV. Experimental results show that the proposed approach is very promising with overall precision and recall rates of 91% and 89%, respectively on handheld dataset, and 34% and 77%, respectively on the UAV dataset. © 2018 Association for Computing Machinery.},
}

@CONFERENCE{Plastiras2018,
author={Plastiras, G. and Kyrkou, C. and Theocharides, T.},
title={Efficient convnet-based object detection for unmanned aerial vehicles by selective tile processing},
journal={ACM International Conference Proceeding Series},
year={2018},
art_number={a3},
note={cited By 17},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85056635428&doi=10.1145%2f3243394.3243692&partnerID=40&md5=ce39506efad58f363593b74d50c01ad3},
abstract={Many applications utilizing Unmanned Aerial Vehicles (UAVs) require the use of computer vision algorithms to analyze the information captured from their on-board camera. Recent advances in deep learning have made it possible to use single-shot Convolutional Neural Network (CNN) detection algorithms that process the input image to detect various objects of interest. To keep the computational demands low these neural networks typically operate on small image sizes which, however, makes it difficult to detect small objects. This is further emphasized when considering UAVs equipped with cameras where due to the viewing range, objects tend to appear relatively small. This paper therefore, explores the trade-offs involved when maintaining the resolution of the objects of interest by extracting smaller patches (tiles) from the larger input image and processing them using a neural network. Specifically, we introduce an attention mechanism to focus on detecting objects only in some of the tiles and a memory mechanism to keep track of information for tiles that are not processed. Through the analysis of different methods and experiments we show that by carefully selecting which tiles to process we can considerably improve the detection accuracy while maintaining comparable performance to CNNs that resize and process a single image which makes the proposed approach suitable for UAV applications. © 2018 Association for Computing Machinery.},
}

@CONFERENCE{BinRamli2018101,
author={Bin Ramli, M.F. and Shamsudin, S.S. and Legowo, A.},
title={Safe avoidance path detection using multi sensor integration for small unmanned aerial vehicle},
journal={5th IEEE International Workshop on Metrology for AeroSpace, MetroAeroSpace 2018 - Proceedings},
year={2018},
pages={101-106},
art_number={8453521},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85053868746&doi=10.1109%2fMetroAeroSpace.2018.8453521&partnerID=40&md5=3bf0afa5adb58854d34331b32a98120f},
abstract={Achieving a robust obstacle detection system that can provide a safe avoidance path system for small UAV is very challenging. Due to size and weight constraints, very limited detection sensors can be equipped in the system. Prior works focused on a single sensing device which is either camera or range sensors based. However, these sensors have their own advantages and disadvantages in detecting the appearance of the obstacles. In this paper, a combination of both sensors based is proposed for a small UAV obstacle detection system. A small Lidar sensor is used as the initial detector of obstacle and queue for image capturing by the camera. Next, SURF algorithm is applied to find the obstacle regions and free space regions. This is done through the principal of object size changes and distance relationship in an image perspective. The proposed method was evaluated by conducting experiments in a real complex environment which consist of a textured and textureless obstacle. In the experiment conducted, we successfully detect and create a safe avoidance path for both situations. The textured situation gives a high success rate while textureless situation produces acceptable success rate until 60cm distance. © 2018 IEEE.},
}

@CONFERENCE{Choudhary2018560,
author={Choudhary, G. and Sharma, V. and You, I. and Yim, K. and Chen, I.-R. and Cho, J.-H.},
title={Intrusion Detection Systems for Networked Unmanned Aerial Vehicles: A Survey},
journal={2018 14th International Wireless Communications and Mobile Computing Conference, IWCMC 2018},
year={2018},
pages={560-565},
art_number={8450305},
note={cited By 16},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85053889909&doi=10.1109%2fIWCMC.2018.8450305&partnerID=40&md5=8db582b85833f70c97bc569b581bbe9b},
abstract={Unmanned Aerial Vehicles (UAV)-based civilian or military applications become more critical to serving civilian and/or military missions. The significantly increased attention on UAV applications also has led to security concerns particularly in the context of networked UAVs. Networked UAVs are vulnerable to malicious attacks over open-air radio space and accordingly intrusion detection systems (IDSs) have been naturally derived to deal with the vulnerabilities and/or attacks. In this paper, we briefly survey the state-of-the-art IDS mechanisms that deal with vulnerabilities and attacks under networked UAV environments. In particular, we classify the existing IDS mechanisms according to information gathering sources, deployment strategies, detection methods, detection states, IDS acknowledgment, and intrusion types. We conclude this paper with research challenges, insights, and future research directions to propose a networked UAVIDS system which meets required standards of effectiveness and efficiency in terms of the goals of both security and performance. © 2018 IEEE.},
}

@ARTICLE{Golston2018,
author={Golston, L.M. and Aubut, N.F. and Frish, M.B. and Yang, S. and Talbot, R.W. and Gretencord, C. and McSpiritt, J. and Zondlo, M.A.},
title={Natural gas fugitive leak detection using an unmanned aerial vehicle: Localization and quantification of emission rate},
journal={Atmosphere},
year={2018},
volume={9},
number={9},
art_number={333},
note={cited By 33},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85052972130&doi=10.3390%2fatmos9090333&partnerID=40&md5=ef77277ad5eb2c28d3776f840b6c963f},
abstract={We describe a set of methods for locating and quantifying natural gas leaks using a small unmanned aerial system equipped with a path-integrated methane sensor. The algorithms are developed as part of a system to enable the continuous monitoring of methane, supported by a series of over 200 methane release trials covering 51 release location and flow rate combinations. The system was found throughout the trials to reliably distinguish between cases with and without a methane release down to 2 standard cubic feet per hour (0.011 g/s). Among several methods evaluated for horizontal localization, the location corresponding to the maximum path-integrated methane reading performed best with a mean absolute error of 1.2 m if the results from several flights are spatially averaged. Additionally, a method of rotating the data around the estimated leak location according to the wind is developed, with the leak magnitude calculated from the average crosswind integrated flux in the region near the source location. The system is initially applied at the well pad scale (100-1000 m2 area). Validation of these methods is presented including tests with unknown leak locations. Sources of error, including GPS uncertainty, meteorological variables, data averaging, and flight pattern coverage, are discussed. The techniques described here are important for surveys of small facilities where the scales for dispersion-based approaches are not readily applicable. © 2018 by the authors.},
}

@ARTICLE{Fernandez201845100,
author={Fernandez, M.G. and Lopez, Y.A. and Arboleya, A.A. and Valdes, B.G. and Vaqueiro, Y.R. and Andres, F.L.-H. and Garcia, A.P.},
title={Synthetic aperture radar imaging system for landmine detection using a ground penetrating radar on board a unmanned aerial vehicle},
journal={IEEE Access},
year={2018},
volume={6},
pages={45100-45112},
art_number={8425684},
note={cited By 60},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85051025158&doi=10.1109%2fACCESS.2018.2863572&partnerID=40&md5=0f0692b8c4ab3b90e75b14be3176d651},
abstract={This paper presents a novel system to obtain images from the underground based on ground penetrating radar (GPR). The proposed system is composed by a radar module mounted on board an unmanned aerial vehicle (UAV), which allows the safe inspection of difficult-to-access areas without being in direct contact with the soil. Therefore, it can be used to detect dangerous buried objects, such as landmines. The radar measurements are coherently combined using a synthetic aperture radar (SAR) algorithm, which requires cm-level accuracy positioning system. In addition, a clutter removal technique is applied to mitigate the reflection at the air-soil interface (which is caused by impedance mismatching). Besides the aforementioned advantages, the system can detect both metallic and dielectric targets (due to the use of a radar instead of a metal detector) and it allows to obtain high-resolution underground images (due to the SAR processing). The algorithms and the UAV payload are validated with measurements in both controlled and real scenarios, showing the feasibility of the proposed system. © 2013 IEEE.},
}

@CONFERENCE{Leyuan2018,
author={Leyuan, S. and Wende, H. and Yifan, Z. and Yueke, W. and Jun, Y.},
title={GPS Spoofing Detection of Unmanned Aerial Vehicles by Dynamics Identification},
journal={2018 IEEE CSAA Guidance, Navigation and Control Conference, CGNCC 2018},
year={2018},
art_number={9019147},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85082444453&doi=10.1109%2fGNCC42960.2018.9019147&partnerID=40&md5=4aa17c91a63ce2971c04cec4dfc0fe41},
abstract={Global Positioning System (GPS) spoofing is a common mean to cheat an Unmanned Aerial Vehicle (UAV) which is guided by the INS/GPS integrated navigation system. Detecting the spurious GPS signal is the precondition of anti-spoofing for UAVs. A detection system of GPS spoofing is designed based on dynamics identification. The centroid motion model and attitude motion model were established. The measurement information from inertial measurement units (IMUs) and positioning information from GPS both are visualized responses to the dynamic laws of UAVs. These two types of measurement information were separately used to estimate the dynamics parameters of UAVs online using two Extended Kalman Filters (EKFs). The detection of spurious GPS signals was realized effectively based on the monitoring of relative estimation errors. Numerical simulations demonstrated that the dynamics parameters could be estimated online by the combined filters. And the precision and accuracy of filter #1, which was based on IMU information, were both higher than those of filter #2, which was based on GPS information. When the spurious GPS signal was just zero-order continuous with the true signal at the penetration point, a pulse relative error would occur at the penetration point; when the spurious GPS signal was first-order continuous with the true signal at the penetration point, a step relative error would occur. Furthermore, relative systematic errors matched with the period of spurious signals. © 2018 IEEE.},
}

@ARTICLE{Lin2018174,
author={Lin, C. and Chen, S.-Y. and Chen, C.-C. and Tai, C.-H.},
title={Detecting newly grown tree leaves from unmanned-aerial-vehicle images using hyperspectral target detection techniques},
journal={ISPRS Journal of Photogrammetry and Remote Sensing},
year={2018},
volume={142},
pages={174-189},
note={cited By 30},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85048279302&doi=10.1016%2fj.isprsjprs.2018.05.022&partnerID=40&md5=dad59e7f34b24244bb1f53440eb65b99},
abstract={Phenological events of tree leaves from initiation to senescence is generally influenced by temperature and water availability. Detection of newly grown leaves (NGL) is useful in the diagnosis of growth of trees, tree stress and even climatic change. Utilizing very high resolution UAV images, this paper examines the feasibility of NGL detection using hyperspectral detection algorithms and anomaly detectors. The issues of pixel resolution and hard decision thresholding in deriving accurate NGL maps are also explored. Results showed that the blind-detection algorithms RXDs are not suitable for NGL detection due to the spectra similarity between NGL and both mature leaves and grass, while brighter pixels, such as those produced by soil and concrete materials, are more easily recognized as anomaly in contrast to forest. Matching filter (MF) based detectors are, however, able to accurately detect NGL over forest stands and are even more effective in the sense of achieving satisfactory true positives and true negatives while providing minimal false alarms. Of the tested partial knowledge MF algorithms, the covariance matched filter based distance (KMFD) detector performed very well with overall accuracy (OA) 0.97 and kappa coefficient (κ^) 0.60 on a natural resolution of 6.75 cm image. When a variety of mature-leaf nonobjective targets are included in the detection, the orthogonal subspace projector (OSP) tends to suppress NGL pixels as an unwanted signature and this leads to poor detection. Conversely, the target constrained interference minimized filter (TCIMF) detector is still able to effectively detect NGL with a satisfactory OA and κ^ through effective matching filter of the target signature as the hard-decision threshold is subject to a level of 5% or 1% probability of false alarms. From decimeter resolution satellite images, the KMFD and TCIMF detectors are capable of achieving an accuracy of OA = 0.94 and κ^ = 0.56 or OA = 0.87 and κ^ = 0.48 for images with a resolution of 33.75 cm or 67.50 cm respectively. This indicates that hyperspectral target detection techniques have great potential in NGL detection via high spatial resolution satellite multispectral images. © 2018 International Society for Photogrammetry and Remote Sensing, Inc. (ISPRS)},
}

@ARTICLE{Lu20182315,
author={Lu, H. and Li, Y. and Mu, S. and Wang, D. and Kim, H. and Serikawa, S.},
title={Motor anomaly detection for unmanned aerial vehicles using reinforcement learning},
journal={IEEE Internet of Things Journal},
year={2018},
volume={5},
number={4},
pages={2315-2322},
note={cited By 265},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85028968216&doi=10.1109%2fJIOT.2017.2737479&partnerID=40&md5=b3c799dc824e4fc33f2199beb823e628},
abstract={Unmanned aerial vehicles (UAVs) are used in many fields including weather observation, farming, infrastructure inspection, and monitoring of disaster areas. However, the currently available UAVs are prone to crashing. The goal of this paper is the development of an anomaly detection system to prevent the motor of the drone from operating at abnormal temperatures. In this anomaly detection system, the temperature of the motor is recorded using DS18B20 sensors. Then, using reinforcement learning, the motor is judged to be operating abnormally by a Raspberry Pi processing unit. A specially built user interface allows the activity of the Raspberry Pi to be tracked on a Tablet for observation purposes. The proposed system provides the ability to land a drone when the motor temperature exceeds an automatically generated threshold. The experimental results confirm that the proposed system can safely control the drone using information obtained from temperature sensors attached to the motor. © 2017 IEEE.},
}

@CONFERENCE{Rosner2018,
author={Rosner, J. and Pȩszor, D. and Paszkuta, M. and Wereszczyński, K. and Wojciechowski, K. and Szender, M. and Mieszalski, D. and Zieliński, B.},
title={A system for automatic detection of potential landing sites for horizontally landing unmanned aerial vehicles},
journal={AIP Conference Proceedings},
year={2018},
volume={1978},
art_number={110006},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85049961135&doi=10.1063%2f1.5043764&partnerID=40&md5=76c35f03af8312079bca53b9786fc626},
abstract={We propose a multistage algorithm designed for automatic detection of possible landing sites for unmanned aerial vehicles (UAV). Presented system uses single camera mounted on UAV and device capable of highly-parallelized calculations. © 2018 Author(s).},
}

@CONFERENCE{Yang20183896,
author={Yang, Q. and Zhang, J. and Shi, G.},
title={Path planning for unmanned aerial vehicle passive detection under the framework of partially observable markov decision process},
journal={Proceedings of the 30th Chinese Control and Decision Conference, CCDC 2018},
year={2018},
pages={3896-3903},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85050869628&doi=10.1109%2fCCDC.2018.8407800&partnerID=40&md5=f5c698fce6889a8d84e25d152caed5c9},
abstract={In order to improve the UAV's autonomous target-tracking ability under the condition of passive detection, this paper established an unmanned aerial vehicle (UAV) path planning POMDP model in passive detection situation under the theoretical framework of Partially Observable Markov Decision Process (POMDP). A method of finite set of action was proposed based on the characteristics of path planning. The optimal operation was solved out by combining the method and Unscented Kalman Filter (UKF). The relevant simulation results show that the model can achieve efficient planning for UAV route, and control the UAV to effectively track target, therefore proving its validity in the process. © 2018 IEEE.},
}

@CONFERENCE{Ma20186344,
author={Ma, S. and Zhang, Y. and Xin, J. and Yi, Y. and Liu, D. and Liu, H.},
title={An early forest fire detection method based on unmanned aerial vehicle vision},
journal={Proceedings of the 30th Chinese Control and Decision Conference, CCDC 2018},
year={2018},
pages={6344-6349},
note={cited By 8},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85050859764&doi=10.1109%2fCCDC.2018.8408244&partnerID=40&md5=739db40fdc5db7e13ce7cc1a3c9bf3c9},
abstract={Traditional forest fire detection methods based on flame are subject to detection delays due to the later appearrance of flame than smoke. When the flame is detected, the fire might have already been spread and out of control. Therefore, the objective of this paper is to study new fire detection method based on smoke. First a quadrotor unmanned aerial vehicle (UAV) is adopted to capture the fire video; then the collected video sequence will be processed by a series of preprocessing including filtering and image enhancement; finally a new significance detection algorithm is investigated for early and efficient smoke detection. Experimental results show that the algorithm can detect smoke effectively. © 2018 IEEE.},
}

@CONFERENCE{Saribas20181,
author={Saribas, H. and Cevikalp, H. and Kahvecioglu, S.},
title={Car detection in images taken from unmanned aerial vehicles [Insansiz Hava Araçlarindan Alinan Görüntülerdeki Araçlarin Konumlarinin Bulunmasi]},
journal={26th IEEE Signal Processing and Communications Applications Conference, SIU 2018},
year={2018},
pages={1-4},
note={cited By 6},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85050823939&doi=10.1109%2fSIU.2018.8404201&partnerID=40&md5=fb10363937f8417677f5d0b83c29f1ee},
abstract={In recent years, unmanned aerial vehicles have become a popular research platform with many application areas such as military, civil, commercial and recreational areas, thanks to their high maneuverability, vertical take-off / landing, and outdoor and indoor use. Today, small, light, and very high powerful embedding systems have been developed. Therefore, many real-time computer vision applications can be run on unmanned aerial vehicle platforms by integrating such embedding systems onto these vehicles. In this work, the problem of car detection (localization) in images taken from unmanned aerial vehicles has been studied. To this end, we collected a new aerial image dataset by using quadcopters and different type of cameras. To solve the car detection problem, the results were compared by using both the Polyhedral Conic Classifier and the You Only Look Once (YOLO) algorithm which is considered one of the fastest deep neural network methods in the literature. © 2018 IEEE.},
}

@CONFERENCE{Dike20182273,
author={Dike, H.U. and Wu, Q. and Zhou, Y. and Liang, G.},
title={Unmanned Aerial Vehicle (UAV) Based Running Person Detection from a Real-Time Moving Camera},
journal={2018 IEEE International Conference on Robotics and Biomimetics, ROBIO 2018},
year={2018},
pages={2273-2278},
art_number={8665167},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85064122959&doi=10.1109%2fROBIO.2018.8665167&partnerID=40&md5=d2858cbbf211b9753fc23fa2f65b2aad},
abstract={The information captured by Unmanned Aerial Vehicles (UAVs) are highly exploited to detect a running person which is given in this paper. In this scheme, 11 frame per seconds and an adequate detection precision in outdoor background was realized, using one dispensation thread without resorting to distinct hardware. The high precision and realtime detection were made promising by two aids. First, we used a progression of preprocessing procedures to extract the regions of interest (ROI), this includes spatial domain analysis, calculating the optical flow in every two consecutive images and having a predefined threshold built on optical flow to select actual areas as ROIs. Secondly, we also used relatively minor-batch models to train our 5-layer convolutional neural networks (CNN) in order to realize an adequate detection ratio. The experiments from numerous videos shot in diverse time and locations proved that the proposed scheme can detect running person in outdoors efficiently and enhance the Realtime necessity with a very high detection ratio. © 2018 IEEE.},
}

@ARTICLE{Wang20181406,
author={Wang, R.-J. and Zhao, C.-J. and Bai, Y. and Zeng, Z.-Q. and Du, W.-H. and Duan, N.-Q.},
title={Faults detection and self-reconfiguration for execution units of Hex-Rotor unmanned aerial vehicle based on multiple fault classification [基于多故障分类的Hex-Rotor无人飞行器的执行单元故障检测与自重构]},
journal={Zhejiang Daxue Xuebao (Gongxue Ban)/Journal of Zhejiang University (Engineering Science)},
year={2018},
volume={52},
number={7},
pages={1406-1414},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85052592715&doi=10.3785%2fj.issn.1008-973X.2018.07.022&partnerID=40&md5=ad1c02ed1380c508f0f8d4074413f916},
abstract={The safety and reliability of the Hex-Rotor UAV were improved in order to detect the fault of the execution units of Hex-Rotor unmanned aerial vehicle (UAV) quickly and accurately. The faults detection and self-reconfiguration for execution units of Hex-Rotor UAV was proposed based on multiple fault classification. The lift model of the execution units was established based on the classification of the fault of the execution units. The fault observer group based on the extended Kalman filter (EKF) algorithm was constructed to achieve fault detection and isolation. Then a self-reconfigurable control algorithm based on multiple fault classification was designed by using the output signal of the fault observer group. The effectiveness of the proposed algorithm was verified by theoretical analysis, numerical simulation and actual flight. Results show that the algorithm can complete fault detection and isolation quickly and accurately, and ensure the stability of the attitude control of the Hex-Rotor UAV under fault condition. © 2018, Zhejiang University Press. All right reserved.},
}

@ARTICLE{Wang2018708,
author={Wang, X. and Deng, Y. and Duan, H.},
title={Edge-based target detection for unmanned aerial vehicles using competitive Bird Swarm Algorithm},
journal={Aerospace Science and Technology},
year={2018},
volume={78},
pages={708-720},
note={cited By 27},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85047267702&doi=10.1016%2fj.ast.2018.04.047&partnerID=40&md5=b5f32d9add976b893ef35f531eb6b7f7},
abstract={Target detection for unmanned aerial vehicles is an important issue in autonomous formation flight. In this paper, a novel target detection approach for unmanned aerial vehicle formation is proposed based on edge matching. The windowed edge potential function is utilized to describe the attraction field for similar edges. Afterwards, the edge-based target detection problem can be formulated as an optimization problem. An improved version of the bird swarm algorithm, which is called competitive bird swarm algorithm, is proposed to find the location, rotation angle and scale of a given template on a specific image. A strategy named “disturbing the local optimum” is designed to help the original bird swarm algorithm converge to the global optimal solution faster and more stably. Formation flight platforms, which consists of unmanned aerial vehicles moving in leader-follower pattern, are used in our experiments. Images obtained by vision sensors embedded in the leaders are used to verify the effectiveness of the proposed method. The proposed algorithm is tested on both indoor and outdoor images to demonstrate the robustness. Comparative experiments with other state-of-the-art algorithms, including genetic algorithm, particle swarm optimization, artificial bee colony algorithm, pigeon-inspired optimization, and the basic bird swarm algorithm, are also conducted. The results prove the superiority and robustness of the proposed target detection algorithm. © 2018 Elsevier Masson SAS},
}

@CONFERENCE{Zhou20181,
author={Zhou, W. and Wang, L. and Lu, B. and Jin, N. and Guo, L. and Liu, J. and Sun, H. and Liu, H.},
title={Unmanned Aerial Vehicle Detection Based on Channel State Information},
journal={2018 IEEE International Conference on Sensing, Communication and Networking, SECON Workshops 2018},
year={2018},
pages={1-5},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85050569453&doi=10.1109%2fSECONW.2018.8396360&partnerID=40&md5=d421af1f5ce992c5e79096ef2a05bc63},
abstract={Civilian unmanned aerial vehicles (UAVs) have been increasingly used in problematic ways. For instance, more and more UAVs disrupt flights and peep into privacy. This problem is likely to expand given the rapid proliferation of UAVs for commerce, monitoring, recreation, and other applications. In this paper, we propose a UAV presence detection system which identifies signal signatures by using the UAV's RF communication. We explore UAV's physical characteristics, including the mobility due to fast moving, spatiality due to UAV's 3D nature, and vibration due to its wing rotation. We consider whether the received UAV signals are uniquely differentiated from other wireless devices. We thoroughly analyze the angle of arrival (AoA) in 3D space, and flexibly apply super-resolution AoA estimation method to calculate the elevation in 3D place. We conduct spectrum on fine- grained channel state information data, and successfully detect the frequency of UAV vibration due to the rotation of UAV's propellers, and finally improve the accuracy through a clustering algorithm. Our system is prototyped and evaluated using commodity WiFi devices in real-world environment. Our system shows a good performance, which achieves 86.6% of accuracy, 87.3% of precision and 85.8% of recall. © 2018 IEEE.},
}

@ARTICLE{Freitas2018551,
author={Freitas, S. and Silva, H. and Almeida, J. and Silva, E.},
title={Hyperspectral Imaging for Real-Time Unmanned Aerial Vehicle Maritime Target Detection},
journal={Journal of Intelligent and Robotic Systems: Theory and Applications},
year={2018},
volume={90},
number={3-4},
pages={551-570},
note={cited By 18},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85031921485&doi=10.1007%2fs10846-017-0689-0&partnerID=40&md5=881aaa2a4f7823fa3a76787215e940e9},
abstract={This work address hyperspectral imaging systems use for maritime target detection using unmanned aerial vehicles. Specifically, by working in the creation of a hyperspectral real-time data processing system pipeline. We develop a boresight calibration method that allows to calibrate the position of the navigation sensor related to the camera imaging sensor, and improve substantially the accuracy of the target geo-reference. We also develop an unsupervised method for segmenting targets (boats) from their dominant background in real-time. We evaluated the performance of our proposed system for target detection in real-time with UAV flight data and present detection results comparing favorably our approach against other state-of- the-art method. © 2017, The Author(s).},
}

@ARTICLE{Falciglia20182399,
author={Falciglia, P.P. and Biondi, L. and Catalano, R. and Immè, G. and Romano, S. and Vagliasindi, F.G.A.},
title={Preliminary investigation for quali-quantitative characterization of soils contaminated with 241Am and 152Eu by low-altitude unmanned aerial vehicles (UAVs) equipped with small size γ-ray spectrometer: detection efficiency and minimum detectable activity (MDA) concentration assessment},
journal={Journal of Soils and Sediments},
year={2018},
volume={18},
number={6},
pages={2399-2409},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85019091395&doi=10.1007%2fs11368-017-1720-6&partnerID=40&md5=9fdab3425bc953de3ff4ded460c7793a},
abstract={Purpose: Localization and quali-quantitative characterization of radionuclide-contaminated soils are essential for healthcare and remediation activities. However, characterization activities are at the moment mainly based on very complex activities, generally dangerous for workers’ health. Unmanned aerial vehicles (UAVs) can be considered for this purpose, but the absence of data does not permit their use for a quantitative analysis. The main goal of this work is to obtain scientific information for successfully using UAVs in quali-quantitative characterization activities. Materials and methods: The influence of the main flight UAV condition parameters on the detection efficiency and minimum detectable activity (MDA) concentration was assessed at lab-scale, considering 241Am and 152Eu as simulated soil contaminants. Obtained data were compared with reference to clearance levels. Specifically, the altitude (h) and inclination (θ) with respect to the soil surface of a small size γ-ray semiconductor CdTe detector and detection time were investigated as flight parameters. h and θ were adopted in the range 0–70 cm and 0°–60°, respectively. Results and discussion: Main results reveal that in the case of 241Am contamination, a duration time of about 13 and 20 min is required for an altitude of 60 and 70 cm, respectively, if an inclination of zero is considered, whereas inclinations higher than 15° lead to much longer times, up to 40 min. In the presence of 152Eu, results reveal a more marked influence of the variables h and θ on the minimum detection time, with values higher for 241Am. In terms of MDA, in the case of 241Am, all the concentration values, with the exception of the highest θ investigated (60°), are below the Italian regulatory limit for altitudes lower than 35 cm and a detection time of 30 min. Higher h up to 50 cm can be considered, reducing the inclination up to 0°, whereas even higher altitudes make the detection of 241Am not possible. On the other hand, for 152Eu, the observed MDA values always make the contaminant detection possible. Conclusions: All achievements and the calculated fitting parameters are useful preliminary data in the quantitative characterization of soil surface contamination, representing a valuable tool in knowing the soil surface γ-ray activity of 241Am and 152Eu for each given detected value. In general, obtained results will allow a better understanding of the technique limits and operating methods required for characterization activities by UAVs with vertical take-off and landing system. © 2017, Springer-Verlag Berlin Heidelberg.},
}

@ARTICLE{Mahjri20181190,
author={Mahjri, I. and Dhraief, A. and Belghith, A. and Almogren, A.S.},
title={SLIDE: A Straight Line Conflict Detection and Alerting Algorithm for Multiple Unmanned Aerial Vehicles},
journal={IEEE Transactions on Mobile Computing},
year={2018},
volume={17},
number={5},
pages={1190-1203},
note={cited By 13},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85045092708&doi=10.1109%2fTMC.2017.2750144&partnerID=40&md5=9a8a5982311756e1176919f7cce08dde},
abstract={Conflict detection is an important research issue in Unmanned Aerial Vehicles to ensure safety and collision free flights. In this paper, we first propose a comprehensive analytical framework for a three dimensional conflict detection. Then, we propose SLIDE a new Straight LIne conflict DEtection and alerting algorithm for a set of UAVs to safely share a common airspace. SLIDE is fully distributed and requires a limited state information exchange between UAVs. The assumptions of precise state information and packet-loss free communications are relaxed so as to guarantee the applicability and efficiency of the algorithm in real world situations. A thorough discussion is also presented to deal with appropriate tuning of the different parameters of the collision detection framework. Extensive simulations based on OMNeT++ are used to validate SLIDE and evaluate its performance. Simulation results indicate that SLIDE guarantees a reduced number of false and missed alarms even in high density traffic scenarios and communication perturbed environments, yet it leaves adequate time to accomplish the required maneuver actions. © 2002-2012 IEEE.},
}

@ARTICLE{Amanatiadis2018,
author={Amanatiadis, A. and Bampis, L. and Karakasis, E.G. and Gasteratos, A. and Sirakoulis, G.},
title={Real-time surveillance detection system for medium-altitude long-endurance unmanned aerial vehicles},
journal={Concurrency and Computation: Practice and Experience},
year={2018},
volume={30},
number={7},
art_number={e4145},
note={cited By 8},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85017187797&doi=10.1002%2fcpe.4145&partnerID=40&md5=d7af36af91f0ab9badd7135a85ac42b6},
abstract={The detection of ambiguous objects, although challenging, is of great importance for any surveillance system and especially for an unmanned aerial vehicle, where the measurements are affected by the great observing distance. Wildfire outbursts and illegal migration are only some of the examples that such a system should distinguish and report to the appropriate authorities. More specifically, Southern European countries commonly suffer from those problems due to the mountainous terrain and thick forests that contain. Unmanned aerial vehicles like the “Hellenic Civil Unmanned Air Vehicle” project have been designed to address high-altitude detection tasks and patrol the borders and woodlands for any ambiguous activity. In this paper, a moment-based blob detection approach is proposed that uses the thermal footprint obtained from single infrared images and distinguishes human- or fire-sized and shaped figures. Our method is specifically designed so as to be appropriately integrated into hardware acceleration devices, such as General Purpose Computation on Graphics Processing Units (GPGPUs) and field programmable gate arrays, and takes full advantage of their respective parallelization capabilities succeeding real-time performances and energy efficiency. The timing evaluation of the proposed hardware accelerated algorithm's adaptations shows an achieved speedup of up to 7 times, as compared to a highly optimized CPU-only based version. Copyright © 2017 John Wiley & Sons, Ltd.},
}

@CONFERENCE{Wang20181746,
author={Wang, P. and Wang, W. and Wang, H.},
title={Infrared unmanned aerial vehicle targets detection based on multi-scale filtering and feature fusion},
journal={2017 3rd IEEE International Conference on Computer and Communications, ICCC 2017},
year={2018},
volume={2018-January},
pages={1746-1750},
note={cited By 6},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85049733624&doi=10.1109%2fCompComm.2017.8322839&partnerID=40&md5=63c369f2f4f05d1fd907d3cd8d3228d7},
abstract={A multi-scale filtering and feature fusion target detection algorithm is proposed based on the large-field infrared search system for the detection of Unmanned Aerial Vehicle (UAV) targets at different scales in low-altitude background. In the initial targets detection, the algorithm transforms the image sequence into different scales, then uses the median and Robinson filters to suppress the background. At the stage of false alarm elimination, it firstly fuses the filter results on the original scale, then extracts the characteristics of the fusion image and analyzes their inter-class relations. Finally, it designs a classifier based on confidence scoring mechanism to achieve real object confirmation and false alarm elimination. The experimental results show that the proposed algorithm can effectively eliminate the false alarm that has similar characteristics to the real targets. It has a good detection effect on the low speed moving UAV targets when the dimension prior information is unknown. © 2017 IEEE.},
}

@ARTICLE{Aniceto2018,
author={Aniceto, A.S. and Biuw, M. and Lindstrøm, U. and Solbø, S.A. and Broms, F. and Carroll, J.},
title={Monitoring marine mammals using unmanned aerial vehicles: Quantifying detection certainty},
journal={Ecosphere},
year={2018},
volume={9},
number={3},
art_number={e02122},
note={cited By 19},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85044218128&doi=10.1002%2fecs2.2122&partnerID=40&md5=f4eac112fd16e6fd3daec3a062652dec},
abstract={Unmanned aerial vehicles (UAVs) are increasingly being recognized as potentially useful for detection of marine mammals in their natural habitats, but an important consideration is the associated uncertainties in animal detection. We present a study based on field trials using UAVs to carry out image-based monitoring of cetaceans in two fjords in northern Norway. We conducted 12 missions to assess the effects of both environmental- and aircraft-related variables on detection certainty. Images were inspected for animal presence and its associated detection certainty. Images were also assessed for potentially important covariates such as wave turbulence (sea state), luminance, and glare. Aircraft variables such as altitude, pitch, and roll were combined into a single variable - pixel size. We recorded a total of 50 humpback whales, 63 killer whales (KW), and 118 unidentified sightings. We also recorded 57 harbor porpoise sightings. None of the environmental conditions (sea state, glare, and luminance) affected the detection certainty of harbor porpoises. In contrast, increasing sea state and luminance had negative and positive effects, respectively, on the detection certainty of humpback and KW. The detection certainty was not significantly affected by pixel size for both harbor porpoises, and humpback and KW. Our results indicate that at lower altitudes, variations in aircraft position (pitch and roll) do not have a variable effect on detection certainty. Overall, this study shows the importance of measuring variability in both environmental and flight-related variables, in order to attain unbiased estimates of detectability for UAV-based marine mammal surveys, particularly in Arctic and sub-Arctic regions. © 2018 Aniceto et al.},
}

@ARTICLE{Puliti2018,
author={Puliti, S. and Talbot, B. and Astrup, R.},
title={Tree-stump detection, segmentation, classification, and measurement using Unmanned aerial vehicle (UAV) imagery},
journal={Forests},
year={2018},
volume={9},
number={3},
art_number={102},
note={cited By 29},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85042724202&doi=10.3390%2ff9030102&partnerID=40&md5=b5eaea4f0cf61810c72bc64ada70a22b},
abstract={Unmanned aerial vehicles (UAVs) are increasingly used as tools to perform a detailed assessment of post-harvest sites. One of the potential use of UAV photogrammetric data is to obtain tree-stump information that can then be used to support more precise decisions. This study developed and tested a methodology to automatically detect, segment, classify, and measure tree-stumps. Among the potential applications for single stump data, this study assessed the possibility (1) to detect and map root- and butt-rot on the stumps using a machine learning approach, and (2) directly measure or model tree stump diameter from the UAV data. The results revealed that the tree-stumps were detected with an overall accuracy of 68-80%, and once the stump was detected, the presence of root- and butt-rot was detected with an accuracy of 82.1%. Furthermore, the root mean square error of the UAV-derived measurements or model predictions for the stump diameter was 7.5 cm and 6.4 cm, respectively, and with the former systematically under predicting the diameter by 3.3 cm. The results of this study are promising and can lead to the development of more cost-effective and comprehensive UAV post-harvest surveys. © 2018 by the authors.},
}

@ARTICLE{Guo2018317,
author={Guo, D. and Zhong, M. and Zhou, D.},
title={Multisensor data-fusion-based approach to airspeed measurement fault detection for unmanned aerial vehicles},
journal={IEEE Transactions on Instrumentation and Measurement},
year={2018},
volume={67},
number={2},
pages={317-327},
art_number={8168410},
note={cited By 29},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85038872037&doi=10.1109%2fTIM.2017.2735663&partnerID=40&md5=f46bfdabcf0bbce0d55947834719074f},
abstract={Fault detection (FD) plays an important role in guaranteeing system safety and reliability for unmanned aerial vehicles (UAVs). This paper focuses on developing an alternative approach to FD for airspeed sensor in UAVs by using data from gyros, accelerometers, global positioning system, and wind vanes. Based on the kinematics model of the UAV, an estimator is proposed to provide analytical redundancy using information from the above-mentioned sensors, which are commonly implemented on UAVs. This filter process is independent of the airspeed measurement and the aircraft dynamics model. Furthermore, we employ the observability rank criterion based on Lie derivatives and prove that the nonlinear system describing the airspeed kinematics is observable. The x2 test and cumulative sum detector are employed to detect the occurrence of airspeed measurement faults together. Finally, the performance of the proposed methodology has been evaluated through flight experiments of UAVs. © 1963-2012 IEEE.},
}

@CONFERENCE{Saadat2018,
author={Saadat, M.N. and Husen, M.N.},
title={An application framework for forest fire and haze detection with data acquisition using unmanned aerial vehicle},
journal={ACM International Conference Proceeding Series},
year={2018},
art_number={46},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85048431743&doi=10.1145%2f3164541.3164624&partnerID=40&md5=6317b93f92cb6bd17f55bcef4d002cb4},
abstract={An application framework is presented in this paper to mitigate the problems that cause the forest area to be harmed. Along with this, a sensor based data collection module is presented that will be enhancing monitoring facility in places in the forest or plants where usually human does not go regularly. The are many use cases of the proposed solutions, for example, it targets to detect the haze or forest fire in early stage so that it can't wide spread and cause severe damage to the forest itself and surrounded locality, object detection and intruder identification, raw imagery collection for finding the appropriate trees to be harvested in Timber industry. These functionalities reside on a remote server. This ongoing research considers supervised machine learning and big data implementation along with the custom system with unmanned aerial vehicles to be the career of designed system. We have proposed an application framework particularly to be cheap and easy to handle by non-technical persons and that it does not require large software system knowledge like Pix4D or DroneDeploy. This system will be useful for not only regular operations but also for research and development as well specially in the forestry and palm oil plantation surveillance, and sustainable timber industry that specially needs carefully collected imageries and data from objects inside the dense forests. © 2018 ACM.},
}

@CONFERENCE{Nüßler2018,
author={Nüßler, D. and Shoykhetbrod, A. and Gütgemann, S. and Küter, A. and Welp, B. and Pohl, N. and Krebs, C.},
title={Detection of unmanned aerial vehicles (UAV) in urban environments},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2018},
volume={10799},
art_number={107990R},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85079283693&doi=10.1117%2f12.2325637&partnerID=40&md5=a1593d104d1fd5eb7d8787fbd9f6d4c3},
abstract={The detection and tracking of UAV's is a critical task for public and military security. The main are the low flight height and the small radar cross section (RCS). The problems increase in an urban environment with many high buildings, especially when tall buildings block the line of sight. A new concept of distributed radar sensors was developed to close this gap. To reduce the impact of radar shadows in urban canyons, a surveillance grid of optical and radar sensors is necessary which covers the complete urban environment. The radar sensors build up different security sectors and monitor all access routes for attacking UAVs. Sophisticated cameras which offer night vision capabilities complete the sensor network to reduce the false alarm rate through these regular, declared UAV flights. Cameras allow the integration of a man in the loop which has the final responsibility to define a target as a threat or not. The system supports the operator with a database which based on optical and radar signature of most commercially available UAV's. © COPYRIGHT SPIE. Downloading of the abstract is permitted for personal use only.},
}

@ARTICLE{Moskalenko201819,
author={Moskalenko, V. and Dovbysh, A. and Naumenko, I. and Moskalenko, A. and Korobov, A.},
title={Improving the effectiveness of training the on-board object detection system for a compact unmanned aerial vehicle},
journal={Eastern-European Journal of Enterprise Technologies},
year={2018},
volume={4},
number={9},
pages={19-26},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85057751657&doi=10.15587%2f1729-4061.2018.139923&partnerID=40&md5=8816b3dd5c547459b3539e3f5560221f},
abstract={The model of object detector and the criterion of leaning effectiveness of the model were proposed. The model contains 7 first modules of the convolutional Squeezenet network, two convolutional multiscale layers and the information­extreme classifier. The multiplicative convolution of the particular criteria that takes into account the effectiveness of detection of objects in the image and accuracy of the classification analysis was considered as the criterion of learning effectiveness of the model. In this case, additional use of the orthogonal matching pursuit algorithm in calculating high­level features makes it possible to increase the accuracy of the model by 4 %. The training algorithm of object detector under conditions of a small size of labeled training datasets and limited computing resources available on board of a compact unmanned aerial vehicle was developed. The essence of the algorithm is to adapt the high­level layers of the model to the domain application area, based on the algorithms of growing sparse coding neural gas and simulated annealing. Unsupervised learning of high­level layers makes it possible to use effectively the unlabeled datasets from the domain area and determine the required number of neurons. It is shown that in the absence of fine tuning of convolutional layers, 69 % detection of objects in the images of the test dataset Inria Aerial Image was ensured. In this case, after fine tuning based on the simulated annealing algorithm, 95 % detection of the objects in test images is ensured. It was shown that the use of unsupervised pretraining makes it possible to increase the generalizing ability of decision rules and to accelerate the iteration process of finding the global maximum during supervised learning on the dataset of limited size. In this case, the overfitting effect is eliminated by optimal selection of the value of hyperparameter, characterizing the measure of coverage of the input data of by network neurons. © V. Moskalenko, A. Dovbysh, I. Naumenko, A. Moskalenko, A. Korobov, 2018.
Запропоновано модель детектора об'єктiв i критерiй ефективностi навчання моделi. Модель мiстить 7 перших модулiв згорткової мережi Squeezenet, два згортковi рiзномасштабнi шари, та iнформацiйно-екстремальний класифiкатор. Як критерiй ефективностi навчання моделi детектора розглядається мультиплiкативна згортка частин- них критерiїв, що враховує ефективнiсть виявлен- ня об'єктiв на зображеннi та точнiсть класифiка- цiйного аналiзу. При цьому додаткове використання алгоритму ортогонального узгодженого кодування при обчисленнi високорiвневих ознак дозволяє збiль- шити точнiсть моделi на 4 %. Розроблено алгоритм навчання детектора об'єк- тiв за умов малого обсягу розмiчених навчальних зразкiв та обмежених обчислювальних ресурсiв, доступних на борту малогабаритного безпiлотного апарату. Суть алгоритму полягає в адаптацiї верх- нiх шарiв моделi до доменної областi використання на основi алгоритмiв зростаючого розрiджено коду- ючого нейронного газу та симуляцiї вiдпалу. Навчання верхнiх шарiв без вчителя дозволяє ефективно вико- ристати нерозмiченi данi з доменної областi та визначити необхiдну кiлькiсть нейронiв. Показано, що за вiдсутностi тонкої настройки згорткових шарiв забезпечується 69 % виявлених об'єктiв на зображен- нях тестової вибiрки Inria Aerial Image. При цьому пiсля тонкої настройки на основi алгоритму симуля- цiї вiдпалу забезпечується 95 % виявлених об'єктiв на тестових зображеннях. Показано, що використання попереднього навчан- ня без вчителя дозволяє пiдвищити узагальнюючу здатнiсть вирiшальних правил та прискорити iте- рацiйний процес знаходження глобального максиму- му при навчаннi з учителем на вибiрцi обмежено- го обсягу. При цьому усунення ефекту перенавчання здiйснюється шляхом оптимального вибору значення гiперпараметру, що характеризує ступiнь покриття вхiдних даних нейронами мережi.},
}

@ARTICLE{Boonpook2018,
author={Boonpook, W. and Tan, Y. and Ye, Y. and Torteeka, P. and Torsri, K. and Dong, S.},
title={A deep learning approach on building detection from unmanned aerial vehicle-based images in riverbank monitoring},
journal={Sensors (Switzerland)},
year={2018},
volume={18},
number={11},
art_number={3921},
note={cited By 27},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85056629454&doi=10.3390%2fs18113921&partnerID=40&md5=f2ad8d7c75681464bb5c1416d62cd90c},
abstract={Buildings along riverbanks are likely to be affected by rising water levels, therefore the acquisition of accurate building information has great importance not only for riverbank environmental protection but also for dealing with emergency cases like flooding. UAV-based photographs are flexible and cloud-free compared to satellite images and can provide very high-resolution images up to centimeter level, while there exist great challenges in quickly and accurately detecting and extracting building from UAV images because there are usually too many details and distortions on UAV images. In this paper, a deep learning (DL)-based approach is proposed for more accurately extracting building information, in which the network architecture, SegNet, is used in the semantic segmentation after the network training on a completely labeled UAV image dataset covering multi-dimension urban settlement appearances along a riverbank area in Chongqing. The experiment results show that an excellent performance has been obtained in the detection of buildings from untrained locations with an average overall accuracy more than 90%. To verify the generality and advantage of the proposed method, the procedure is further evaluated by training and testing with another two open standard datasets which have a variety of building patterns and styles, and the final overall accuracies of building extraction are more than 93% and 95%, respectively. © 2018 by the authors. Licensee MDPI, Basel, Switzerland.},
}

@ARTICLE{Du2018375,
author={Du, D. and Qi, Y. and Yu, H. and Yang, Y. and Duan, K. and Li, G. and Zhang, W. and Huang, Q. and Tian, Q.},
title={The unmanned aerial vehicle benchmark: Object detection and tracking},
journal={Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
year={2018},
volume={11214 LNCS},
pages={375-391},
note={cited By 58},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85055113352&doi=10.1007%2f978-3-030-01249-6_23&partnerID=40&md5=e6f0f7deabf79197589322a12632dd3a},
abstract={With the advantage of high mobility, Unmanned Aerial Vehicles (UAVs) are used to fuel numerous important applications in computer vision, delivering more efficiency and convenience than surveillance cameras with fixed camera angle, scale and view. However, very limited UAV datasets are proposed, and they focus only on a specific task such as visual tracking or object detection in relatively constrained scenarios. Consequently, it is of great importance to develop an unconstrained UAV benchmark to boost related researches. In this paper, we construct a new UAV benchmark focusing on complex scenarios with new level challenges. Selected from 10 hours raw videos, about 80, 000 representative frames are fully annotated with bounding boxes as well as up to 14 kinds of attributes (e.g., weather condition, flying altitude, camera view, vehicle category, and occlusion) for three fundamental computer vision tasks: object detection, single object tracking, and multiple object tracking. Then, a detailed quantitative study is performed using most recent state-of-the-art algorithms for each task. Experimental results show that the current state-of-the-art methods perform relative worse on our dataset, due to the new challenges appeared in UAV based real scenes, e.g., high density, small object, and camera motion. To our knowledge, our work is the first time to explore such issues in unconstrained scenes comprehensively. The dataset and all the experimental results are available in https://sites.google.com/site/daviddo0323/. © Springer Nature Switzerland AG 2018.},
}

@ARTICLE{Shen201860812,
author={Shen, Q. and Liu, W. and Wang, L. and Liu, Y.},
title={Adaptive Beamforming for Target Detection and Surveillance Based on Distributed Unmanned Aerial Vehicle Platforms},
journal={IEEE Access},
year={2018},
volume={6},
pages={60812-60823},
art_number={8489853},
note={cited By 9},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85054671317&doi=10.1109%2fACCESS.2018.2875560&partnerID=40&md5=017c99b47c06403f44d9a9fe121ab42a},
abstract={A distributed sensor array network for target detection and surveillance is studied with sub-arrays placed on unmanned aerial vehicle (UAV) platforms, where arbitrary locations and rotation angles are allocated to each UAV-based sub-array in the predefined Cartesian coordinate system. In this model, one transmitter sends out a single signal and it is then reflected back from the targets and received by the distributed sensor array system. A joint reference signal-based beamformer (JRSB) is proposed for the static/slowly moving targets and UAV platforms where the Doppler effects can be ignored, leading to improved performance by exploiting the information collected by all the sub-arrays simultaneously. Then, the developed beamformer is extended to the dynamic case considering the Doppler effects, referred to as the frequency extended JRSB (FE-JRSB), achieving the potential maximum output signal to interference plus noise ratio (SINR) by exploiting the information across the potential frequencies of interest jointly. The output signal of the beamformer with increased SINR can be used to assist the extended target detection in the following processing. Simulation results show that both are able to extract the signals of interest while suppressing interfering signals, and a lower mean square error and a higher output SINR are achieved compared with a regular reference signal-based beamformer using a single sub-array. One unique feature of the provided solutions is that, although the signals involved are narrowband, the employed beamforming structure has to be wideband for it to be effective. © 2013 IEEE.},
}

@CONFERENCE{Brand2018,
author={Brand, J. and Küng, B. and Sartori, K. and Meier, L.},
title={Reliability for unmanned aerial vehicles through automatic flight data analyses: From single flight logs, to population statistics, to anomaly detection using artificial neural networks},
journal={AUVSI XPONENTIAL 2018},
year={2018},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85054660584&partnerID=40&md5=7b74a7473cfec6d7e0013002f2013685},
abstract={Recent progress in unmanned aerial vehicle (UAV) frameworks such as Dronecode has lead to extended technology adoption by end users. The increase in UAVs using Dronecode with its flight control software PX4 is reflected by a growing number of log files on the PX4 flight review server. As the numbers continue to grow, maintaining reliability of each individual UAV through manual analysis of flight data will become increasingly difficult. Automated analysis instead, has the potential to increase reliability of each UAV by accelerating development cycles which will eventually also lead to more reliable UAV operations. In this paper, we provide an overview of methods for automated flight data analysis and address their advantages and disadvantages. We present an implementation based on deep artificial neural networks that uses a Convolutional Autoencoder for automated anomaly detection in accelerometer data. Our preliminary results solely based on accelerometer data yielded an accuracy of 89.6% and thus demonstrated how deep artificial neural networks can be applied to automated flight data analysis. Finally, we also discuss the remaining challenges for improving the accuracy of our automatic anomaly detection model. © 2018 IQPC. All rights reserved.},
}

@CONFERENCE{Guo2018818,
author={Guo, D. and Wang, Y. and Zhong, M. and Zhao, Y.},
title={Fault detection and isolation for Unmanned Aerial Vehicle sensors by using extended PMI filter},
year={2018},
volume={51},
number={24},
pages={818-823},
note={cited By 6},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85054579106&doi=10.1016%2fj.ifacol.2018.09.669&partnerID=40&md5=a5d908fc77d1bfb309c1f34493669245},
abstract={Fault detection and isolation (FDI) plays an important role in guaranteeing system safety and reliability for unmanned aerial vehicles (UAVs). This paper focuses on developing a method for detecting UAV sensor faults by using existing sensors, such as pitot tube, gyro, accelerometer and wind angle sensor. We formulate the kinematics as a nonlinear state space system, which requires no dynamic information and thus is applicable to all aircraft. To illustrate the method, we investigate five fault-detection scenarios, namely, faulty pitot tube, angle-of-attack sensor, sideslip sensor, accelerometer and gyro, and design a FDI structure including five faulty sensors. Then, considering the unknown disturbance, the proportional and multiple integral (PMI) fault detection filter (FDF) is proposed for the state and input estimation. A structure including two residuals are employed to detect and isolate the faults of the proposed faulty sensors. Finally, the performance of the proposed methodology is evaluated through flight experiments of the UAV. © 2018},
}

@CONFERENCE{Ye2018,
author={Ye, D.H. and Li, J. and Chen, Q. and Wachs, J. and Bouman, C.},
title={Deep learning for moving object detection and tracking from a single camera in unmanned aerial vehicles (uavs)},
journal={IS and T International Symposium on Electronic Imaging Science and Technology},
year={2018},
art_number={IMAWM-466},
note={cited By 17},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85052947483&doi=10.2352%2fISSN.2470-1173.2018.10.IMAWM-466&partnerID=40&md5=6e9fde34277e59b443eca721e8fd58bb},
abstract={Unmanned Aerial Vehicles (UAVs) gain popularity in a wide range of civilian and military applications. Such emerging interest is pushing the development of effective collision avoidance systems which are especially crucial in a crowded airspace setting. Because of cost and weight limitations associated with UAVs' payload, the optical sensors, simply digital cameras, are widely used for collision avoidance systems in UAVs. This requires moving object detection and tracking algorithms from a video, which can be run on board efficiently. In this paper, we present a new approach to detect and track UAVs from a single camera mounted on a different UAV. Initially, we estimate background motions via a perspective transformation model and then identify moving object candidates in the background subtracted image through deep learning classifier trained on manually labeled datasets. For each moving object candidates, we find spatio-temporal traits through optical flow matching and then prune them based on their motion patterns compared with the background. Kalman filter is applied on pruned moving objects to improve temporal consistency among the candidate detections. The algorithm was validated on video datasets taken from a UAV. Results demonstrate that our algorithm can effectively detect and track small UAVs with limited computing resources. © 2018, Society for Imaging Science and Technology.},
}

@ARTICLE{Wang20183535,
author={Wang, B. and Chen, Y. and Liu, D. and Peng, X.},
title={An embedded intelligent system for on-line anomaly detection of unmanned aerial vehicle},
journal={Journal of Intelligent and Fuzzy Systems},
year={2018},
volume={34},
number={6},
pages={3535-3545},
note={cited By 11},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85049387004&doi=10.3233%2fJIFS-169532&partnerID=40&md5=bc723fcadc0bb7be31785e77da3c0db4},
abstract={On-line anomaly detection is critical for the safety of unmanned aerial vehicles (UAVs). However, the flight status assessment still depends on ground control stations, which cannot meet the time requirement for autonomous and safe flight. The lack of on-board intelligent anomaly detection systems makes it rather difficult for on-line flight status estimation and assessment. In order to achieve real-time monitoring of UAV flight status and enhance the reliability and safety of UAVs, an embedded intelligent system is designed to address the challenging issues of UAV on-line anomaly detection in this paper. During the flight, the status of sensors and key components are continuously detected via flight data which can reflect the current status of the UAV. The proposed embedded anomaly detection system includes two main parts: (1) a general heterogeneous computing architecture which is based on Xilinx Zynq-7000 SoC with dual-core Cortex A9 processors and Field Programmable Gate Arrays (FPGA), (2) an on-line anomaly detection intelligent algorithm which is based on least squares support vector machine (LS-SVM) prediction model and utilized as a demonstration that needs high computing performance. The simulation flight data are used to verify the proposed system, and the experimental results show that the proposed intelligent system is capable of effective UAV on-line anomaly detection. © 2018 - IOS Press and the authors. All rights reserved.},
}

@CONFERENCE{Nicholas2018,
author={Nicholas, R. and Driggers, R. and Shelton, D. and Furxhi, O.},
title={Infrared search and track performance estimates for detection of commercial unmanned aerial vehicles},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2018},
volume={10625},
art_number={106250Y},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85048117216&doi=10.1117%2f12.2305559&partnerID=40&md5=f7f8bae4cb4561b32db58fc2655b10aa},
abstract={Unmanned aerial vehicles (UAVs) have become more readily available in the past 5 years and are proliferating rapidly. New aviation regulations are accelerating the use of UAVs in many applications. As a result, there are increasing concerns of potential air threats in situational environments including commercial airport security and drug trafficking. In this study, radiometric signatures of commercially available miniature UAVs is determined for long-wave infrared (LWIR) bands in both clear sky and partial cloudy conditions. Results are presented that compare LWIR performance estimates for the detection of commercial UAVs via infrared search and track (IRST) systems with two candidate sensors. © 2018 SPIE.},
}

@ARTICLE{Kuželka2018241,
author={Kuželka, K. and Surový, P.},
title={Automatic detection and quantification of wild game crop damage using an unmanned aerial vehicle (UAV) equipped with an optical sensor payload: A case study in wheat},
journal={European Journal of Remote Sensing},
year={2018},
volume={51},
number={1},
pages={241-250},
note={cited By 13},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85047213412&doi=10.1080%2f22797254.2017.1419442&partnerID=40&md5=dff8a32e4f5f27cb4bf88e14ebaa953c},
abstract={Wildlife-induced damage of agricultural crops is an unfavorable consequence of elevated population densities of wild animals, especially wild boars. For the purposes of financial compensations for crop damage, provided by either governments or hunters responsible for game numbers, it is necessary to precisely assess the range of damage and temporal change. The use of an unmanned aerial vehicle (UAV) with an optical sensor payload represents a potential method of obtaining data of crop conditions without the necessity to enter the field and increase the damage. We propose a novel method for delineation of damaged areas via automatic segmentation of the crop field. Our method is based on photogrammetric reconstruction of the various crop heights within the field through the use of Structure from Motion technique with subsequent automatic classification. In this case study of wheat, the range of damage was estimated with an accuracy of 99.5% and 99.3% using field global navigation satellite system (GNSS) measurements and classification of an orthomosaic generated from UAV-based imagery, respectively. © 2018 The Author(s).},
}

@CONFERENCE{Phelps2018,
author={Phelps, D. and Gamagedara, K. and Waldron, J. and Patil, K. and Snyder, M.},
title={Ship air wake detection using a small fixed wing unmanned aerial vehicle},
journal={AIAA Aerospace Sciences Meeting, 2018},
year={2018},
number={210059},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85044408657&doi=10.2514%2f6.2018-0784&partnerID=40&md5=8961debf8cbd6788eeb6f86e265c1ee3},
abstract={A ship’s air wake is dynamically detected using an airborne inertial measurement unit and global positioning system attached to a fixed wing unmanned aerial system. The instrumented aircraft is used for validation of computational fluid dynamic simulations of naval ship air wakes. A simulation was completed using Gridtool, VGrid, and Kestral to validate the experimental data collection method. Forces from the experiment were collected and compared with that of a one-way coupled CFD simulation mimicking the physical experiment. Similar trends in forces that indicate detection of the ship air wake were observed in both experimental and simulation data. © 2018, American Institute of Aeronautics and Astronautics Inc, AIAA. All rights reserved.},
}

@ARTICLE{Xiao2018510,
author={Xiao, Y. and Zheng, H. and Yu, W.},
title={Automatic Crowd Detection Based on Unmanned Aerial Vehicle Thermal Imagery},
journal={Advances in Intelligent Systems and Computing},
year={2018},
volume={690},
pages={510-516},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85034590084&doi=10.1007%2f978-3-319-65978-7_77&partnerID=40&md5=3c08da734c227b259cbcf52bcb118172},
abstract={Automatic crowd detection is one of the most challenging problems in computer vision. Although the thermal image from Unmanned aerial vehicle (UAV) have prominent performance in perspective, but have some disadvantage, such as the platform motion, image instability and so on. In the thesis, the automatic crowd detection system is designed to tackle these disadvantage. The detection system consists of two parts: ROI extraction and SVM classification, circle gradient and geometric filtering are used in ROI extraction, a hybrid feature which combines circle gradient (CG) and histogram of oriented gradient (HOG) is used in SVM classifier. The experimental results prove that the approach performs dense crowd detection from thermal images effectively. © 2018, Springer International Publishing AG.},
}

@ARTICLE{Li2018295,
author={Li, Y. and Lu, H. and Kihara, K. and Guna, J. and Serikawa, S.},
title={Motor Anomaly Detection for Aerial Unmanned Vehicles Using Temperature Sensor},
journal={Studies in Computational Intelligence},
year={2018},
volume={752},
pages={295-304},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85033698798&doi=10.1007%2f978-3-319-69877-9_32&partnerID=40&md5=be90cda103779f33ea84ebdf5b0ed46f},
abstract={Aerial unmanned vehicle is widely used in many fields, such as weather observation, framing, inspection of infrastructure, monitoring of disaster areas. However, the current aerial unmanned vehicle is difficult to avoid falling in the case of failure. The purpose of this article is to develop an anomaly detection system, which prevents the motor from being used under abnormal temperature conditions, so as to prevent safety flight of the aerial unmanned vehicle. In the anomaly detection system, temperature information of the motor is obtained by DS18B20 sensors. Then, the reinforcement learning, a type of machine learning, is used to determine the temperature is abnormal or not by Raspberrypi processing unit. We also build an user interface to open the screen of Raspberrypi on laptop for observation. In the experiments, the effectiveness of the proposed system to stop the operation state of drone when abnormality exceeds the automatically learned motor temperature. The experimental results demonstrate that the proposed system is possibility for unmanned flight safely by controlling drone from information obtained by attaching temperature sensors. © Springer International Publishing AG 2018.},
}

@CONFERENCE{DaSilva20171,
author={Da Silva, B.R.F. and Nogueira, M.B. and Alsina, P.J. and De Albuquerque, G.L.A. and Dantas, J.B.D. and De Medeiros, A.A.D. and Santiago, G.S.},
title={Study on detection of boats using satellite imagery for use on unmanned aerial vehicles},
journal={Proceedings - 2017 LARS 14th Latin American Robotics Symposium and 2017 5th SBR Brazilian Symposium on Robotics, LARS-SBR 2017 - Part of the Robotics Conference 2017},
year={2017},
volume={2017-December},
pages={1-5},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85048524496&doi=10.1109%2fSBR-LARS-R.2017.8215300&partnerID=40&md5=3ecdd6283848ce9c3088ba29f01fa1a5},
abstract={This work presents the development of a system that performs the detection of boats from aerial images acquired by satellites. This will serve as a knowledge base for the implementation of a system to be implemented in a fleet of unmanned aerial vehicle. The main purpose of the system is to detect ships that are in the risk zone of rocket trajectory launched from Barreira do Inferno Launch Center - CLBI. In previous work the authors proposed an algorithm to perform boat detection, however the results showed a high incidence of false positives. In order to improve those results, we propose the use of the Histogram of Oriented Gradients descriptor in candidate images followed by machine learning teachniques such as Suport Vector Machine and K Nearest Neighbours to classify them. To validate the system some experimental results are shown using satellite images, since the aerial vehicle is under constuctions and there is no image database yet. © 2017 IEEE.},
}

@CONFERENCE{Madaan20173487,
author={Madaan, R. and Maturana, D. and Scherer, S.},
title={Wire detection using synthetic data and dilated convolutional networks for unmanned aerial vehicles},
journal={IEEE International Conference on Intelligent Robots and Systems},
year={2017},
volume={2017-September},
pages={3487-3494},
art_number={8206190},
note={cited By 22},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85041966832&doi=10.1109%2fIROS.2017.8206190&partnerID=40&md5=143100c0422718de573c2443bd2dfaee},
abstract={Wire detection is a key capability for safe navigation of autonomous aerial vehicles and is a challenging problem as wires are generally only a few pixels wide, can appear at any orientation and location, and are hard to distinguish from other similar looking lines and edges. We leverage the recent advances in deep learning by treating wire detection as a semantic segmentation task, and investigate the effectiveness of convolutional neural networks for the same. To find an optimal model in terms of detection accuracy and real time performance on a portable GPU, we perform a grid search over a finite space of architectures. Further, to combat the issue of unavailability of a large public dataset with annotations, we render synthetic wires using a ray tracing engine, and overlay them on 67K images from flight videos available on the internet. We use this synthetic dataset for pretraining our models before finetuning on real data, and show that synthetic data alone can lead to pretty accurate detections qualitatively as well. We also verify if providing explicit information about local evidence of wiry-ness in the form of edge and line detection results from a traditional computer vision method, as additional channels to the network input, makes the task easier or not. We evaluate our best models from the grid search on a publicly available dataset and show that they outperform previous work using traditional computer vision and various deep net baselines of FCNs, SegNet and E-Net, on both standard edge detection metrics and inference speed. Our top models run at more than 3Hz on the NVIDIA Jetson TX2 with input resolution of 480×640, with an Average Precision score of 0.73 on our test split of the USF dataset. © 2017 IEEE.},
}

@CONFERENCE{Duan2017638,
author={Duan, Y. and Zhao, Y. and Pang, J. and Liu, L. and Liu, D.},
title={Unmanned Aerial Vehicle Sensing Data Anomaly Detection by Relevance Vector Machine},
journal={Proceedings - 2017 International Conference on Sensing, Diagnostics, Prognostics, and Control, SDPC 2017},
year={2017},
volume={2017-December},
pages={638-641},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85047421211&doi=10.1109%2fSDPC.2017.125&partnerID=40&md5=409428915863514cb2187a3ce0be1b6c},
abstract={In recent years, Unmanned Aerial Vehicle (UAV) has been gaining more and more attention for military and civilian utilization. How to monitor its condition is a crucial problem. The accuracy of the sensing data is one of the basic requirements to achieve its correct condition. Thus, one kind of data anomaly detection approaches by Relevance Vector machine (RVM) is proposed in this article. By utilizing the visual UAV simulator FlgihtGear, the sensing data with anomalous data are generated. The effectiveness of the proposed approach for detecting the anomalous data contained in the sensing data is evaluated. © 2017 IEEE.},
}

@ARTICLE{Xiao20171575,
author={Xiao, J.-P. and Jiang, J.-C. and She, C.-D.},
title={Data attack detection for an unmanned aerial vehicle control system using innovation sequences},
journal={Kongzhi Lilun Yu Yingyong/Control Theory and Applications},
year={2017},
volume={34},
number={12},
pages={1575-1582},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85046800140&doi=10.7641%2fCTA.2017.70053&partnerID=40&md5=4a461c0b982a5e39ae5800a725a4c435},
abstract={With rapid advances in the fields of the Internet of things and autonomous systems, the network security of cyber-physical systems has attracted considerable attention. An unmanned aerial vehicle (UAV) is an intelligent device that relies on information communication and flight control systems to achieve autonomous flight. Consequently, its security is extremely important. This study proposes a new state estimation method that uses innovation sequences based on an extended Kalman filter for the detection of data attacks on a UAV. Our method can identify data attacks on tensors and control commands. First, a cyber-physical system model for a UAV is established, and the state estimation algorithm and data attack model are introduced. Then, a scalar detection statistic is constructed for data attack detection using innovation sequences, and the minus infinity norm method is introduced to reduce the false detection of data attacks while the aircraft is being maneuvered. Finally, simulation results show that the proposed detection method can effectively detect various threat patterns under a variety of circumstances for unmanned control systems. © 2017, Editorial Department of Control Theory & Applications South China University of Technology. All right reserved.},
}

@CONFERENCE{Li20173349,
author={Li, X. and Li, Z. and Fu, B. and Wu, B. and Liu, Y.},
title={A mini consumer grade unmanned aerial vehicle (UAV) for small scale terrace detection},
journal={International Geoscience and Remote Sensing Symposium (IGARSS)},
year={2017},
volume={2017-July},
pages={3349-3352},
art_number={8127715},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85041794234&doi=10.1109%2fIGARSS.2017.8127715&partnerID=40&md5=c4a1062d355df709a0b8574a5d29fd38},
abstract={The advent of photogrammetry using unmanned aerial vehicles (UAVs) has proved a cost effective and efficient alternative to traditional remote sensing techniques and Lidar. Considering lower cost and better flexibility, in this paper we conducted a survey and acquired high definition topographic data involving a mini consumer grade UAV. We aim to assess the accuracy of a mini consumer grade UAV production and check if the result can be used for terrace detection. As a result, our study derives ultra-high resolution orthophotos, image mosaic (with a resolution of 0.02m) and 3D models (with a resolution of 0.2m). The horizontal relative accuracy of the data is 0.38m while the vertical relative accuracy is 0.2m. For a research caring little about the absolute accuracy, the application of this kind of consumer grade UAVs is promising. © 2017 IEEE.},
}

@ARTICLE{Yuan2017635,
author={Yuan, C. and Liu, Z. and Zhang, Y.},
title={Aerial Images-Based Forest Fire Detection for Firefighting Using Optical Remote Sensing Techniques and Unmanned Aerial Vehicles},
journal={Journal of Intelligent and Robotic Systems: Theory and Applications},
year={2017},
volume={88},
number={2-4},
pages={635-654},
note={cited By 81},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85008496954&doi=10.1007%2fs10846-016-0464-7&partnerID=40&md5=bccee7af2c008c9b05ec613cb06fbc14},
abstract={Due to their fast response capability, low cost and without danger to personnel safety since there is no human pilot on-board, unmanned aerial vehicles (UAVs) with vision-based systems have great potential for monitoring and detecting forest fires. This paper proposes a novel forest fire detection method using both color and motion features for processing images captured from the camera mounted on a UAV which is moving during the whole mission period. First, a color-based fire detection algorithm with light computational demand is designed to extract fire-colored pixels as fire candidate regions by making use of chromatic feature of fire and obtaining fire candidate regions for further analysis. As the pose variations and low-frequency vibrations of UAV cause all objects and background in the images are moving, it is challenging to identify fires defending on a single motion based method. Two types of optical flow algorithms, a classical optical flow algorithm and an optimal mass transport optical flow algorithm, are then combined to compute motion vectors of the fire candidate regions. Fires are thereby expected to be distinguished from other fire analogues based on their motion features. Several groups of experiments are conducted to validate that the proposed method can effectively extract and track fire pixels in aerial video sequences. The good performance is anticipated to significantly improve the accuracy of forest fire detection and reduce false alarm rates without increasing much computation efforts. © 2017, Springer Science+Business Media Dordrecht.},
}

@CONFERENCE{Sushant20171360,
author={Sushant, S. and Anand, S. and James, T. and Aravind, V. and Narayanan, G.},
title={Localization of an unmanned aerial vehicle for crack detection in railway tracks},
journal={2017 International Conference on Advances in Computing, Communications and Informatics, ICACCI 2017},
year={2017},
volume={2017-January},
pages={1360-1365},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85042677392&doi=10.1109%2fICACCI.2017.8126030&partnerID=40&md5=f9cf69f8223284d13170e5bdff25e912},
abstract={An Unmanned Aerial Vehicle (UAV) has several applications in the modern scenario. It can be used for capturing live video footages for sports like cricket or football or even commercial applications. It can even be used for procuring images at places where human intervention is difficult and so, can find wide application in disaster management. This paper mainly deals with the localization of a UAV and how it can be applied for detecting cracks in a railway track using the concepts of image processing. The algorithm used for localizing the UAV is called Monte Carlo or Particle filter localization algorithm. The video taken from the UAV is processed by further extracting image frames and analyzing each of these image frames for detection of cracks along railway line. A real-time implementation of our proposed method can significantly reduce physical labor involved in crack detection and also reduces the risk of accidents. © 2017 IEEE.},
}

@CONFERENCE{FaizBinRamli2017,
author={Faiz Bin Ramli, M. and Legowo, A. and Shamsudin, S.S.},
title={Object Detection Technique for Small Unmanned Aerial Vehicle},
journal={IOP Conference Series: Materials Science and Engineering},
year={2017},
volume={260},
number={1},
art_number={012040},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85034443993&doi=10.1088%2f1757-899X%2f260%2f1%2f012040&partnerID=40&md5=c4a896de01e64f708df9c611b7e8f433},
abstract={Obstacle detection and avoidance is desirable for UAVs especially lightweight micro aerial vehicles and is challenging problem since it has payload constraints, therefore only limited sensor can be attached the vehicle. Usually the sensors incorporated in the system is either type vision based (monocular or stereo camera) or Laser based. However, each of the sensor has its own advantage and disadvantage, thus we built the obstacle detection and avoidance system based multi sensor (monocular sensor and LIDAR) integration. On top of that, we also combine SURF algorithm with Harris corner detector to determine the approximate size of the obstacles. In the initial experiment conducted, we successfully detect and determine the size of the obstacles with 3 different obstacles. The differences of length between real obstacles and our algorithm are considered acceptable which is about -0.4 to 3.6. © Published under licence by IOP Publishing Ltd.},
}

@CONFERENCE{Kamnik2017,
author={Kamnik, R. and Grajfoner, B. and Butyrin, A. and Perc, M.N.},
title={Rainwater harvesting and green area retention potential detection using commercial unmanned aerial vehicles},
journal={IOP Conference Series: Earth and Environmental Science},
year={2017},
volume={90},
number={1},
art_number={012113},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85034962885&doi=10.1088%2f1755-1315%2f90%2f1%2f012113&partnerID=40&md5=35531b91008f80fb7c5180f2a5cb5274},
abstract={The objective of this work is to use simple photogrammetry to evaluate rainwater harvesting and green area retention potential in Maribor, Slovenia city centre. Several sources of remote sensing data have been described and a field test with semi-professional drone was performed by means of computer evaluation of rainwater harvesting and green area retention potential. Some of the most important design parameters for rainwater harvesting systems as roof area and slope and available green areas were identified and evaluated. The results have shown that even semi-professional low budget drones can be successfully used for mapping areas of interest. The results of six-minute flight over twelve hectares of Maribor city centre were comparable with professional results of plane remote sensing. Image segmentation from orthomosaic together with elevation model has been used to detect roofs and green areas. © Published under licence by IOP Publishing Ltd.},
}

@CONFERENCE{Bombizov2017,
author={Bombizov, A. and Artishchev, S. and Loschilov, A. and Malyutin, N.},
title={An experimental detection of eletromagnetic radiation generated by unmanned aerial vehicles},
journal={AIP Conference Proceedings},
year={2017},
volume={1899},
art_number={060021},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85034230008&doi=10.1063%2f1.5009892&partnerID=40&md5=7c26fe27bc9becf83faf38f69f29bf8e},
abstract={The results of detection of electromagnetic radiation (EMR) generated by unmanned aerial vehicles (UAVs) are given. It is established that the sources of EMR are the UAV engines, the remote control and the UAV radio module. As an EMR sensor, an active ferrite antenna was used. The EMR of a quadrocopter and a single-screw UAV was investigated. It is shown that the first harmonic of the EMR source are in the range of 2-3 kHz, the 2nd and 3rd harmonics were observed also. It was noted that in the range of observed frequencies pulse signals generated by the remote control and the radio module of the quadrocopter were appeared and registered. The measurements are compared with measurements of Doppler frequencies when the quadrocopter is irradiated with a 9 GHz radar signal. It was shown that the spectra of these signals intersect, but in the spectrum of Doppler oscillations lower frequencies were observed. © 2017 Author(s).},
}

@ARTICLE{BinRamli2017441,
author={Bin Ramli, M.F. and Shamsudin, S.S. and Legowo, A.},
title={Obstacle detection technique using multi sensor integration for small unmanned aerial vehicle},
journal={Indonesian Journal of Electrical Engineering and Computer Science},
year={2017},
volume={8},
number={2},
pages={441-449},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85037649908&doi=10.11591%2fijeecs.v8.i2.pp441-449&partnerID=40&md5=07fd8aa0a194d6b7cff93f9b9449120e},
abstract={Achieving a robust obstacle detection system for small UAV is very challenging. Due to size and weight constraints, very limited detection sensors can be equipped in the system. Prior works focused on a single sensing device which is either camera or range sensors based. However, these sensors have their own advantages and disadvantages in detecting the appearance of the obstacles. In this paper, combination of both sensors based is proposed for a small UAV obstacle detection system. A small Lidar sensor is used as the initial detector and queue for image capturing by the camera. Next, SURF algorithm is applied to find the obstacle sizes estimation by searching the connecting feature points in the image frame. Finally, safe avoidance path for UAV is determined through the exterior feature points from the estimated width of the obstacle. The proposed method was evaluated by conducting experiments in real time with indoor environment. In the experiment conducted, we successfully detect and determine a safe avoidance path for the UAV on 6 different sizes and textures of the obstacles including textureless obstacles. © 2017 Institute of Advanced Engineering and Science. All rights reserved.},
}

@ARTICLE{Cristofaro20171584,
author={Cristofaro, A. and Johansen, T.A. and Aguiar, A.P.},
title={Icing detection and identification for unmanned aerial vehicles using adaptive nested multiple models},
journal={International Journal of Adaptive Control and Signal Processing},
year={2017},
volume={31},
number={11},
pages={1584-1607},
note={cited By 9},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85019643224&doi=10.1002%2facs.2787&partnerID=40&md5=13405d11f9180bfd62529258966e5b9d},
abstract={A multiple-model approach for icing diagnosis and identification in small unmanned aerial vehicles is proposed. The accretion of ice layers on wings and control surfaces modifies the shape of the aircraft and, consequently, alters the performance and controllability of the vehicle. Pitot tubes might be blocked due to icing, providing errors in the airspeed measurements. In this paper, we propose a nested multiple-model adaptive estimation framework to detect and estimate icing using standard sensors only, ie, a pitot tube and an inertial measurement unit. The architecture of the estimation scheme is based on 2 different time scales, ie, one for the accretion of ice on aircraft surfaces and one for the accretion of ice on sensors, and consists of 2 nested adaptive observers, namely, outer and inner loops, respectively. The case study of a typical small unmanned aerial vehicle supports and validates the proposed theoretical results. Copyright © 2017 John Wiley & Sons, Ltd.},
}

@CONFERENCE{Zhao2017289,
author={Zhao, C. and Shi, M. and Cai, Z. and Chen, C.},
title={Detection of unmanned aerial vehicle signal based on Gaussian mixture model},
journal={ICCSE 2017 - 12th International Conference on Computer Science and Education},
year={2017},
pages={289-293},
art_number={8085504},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85040103906&doi=10.1109%2fICCSE.2017.8085504&partnerID=40&md5=d5936bfff96f07e3d75e815fd247909e},
abstract={With the innovation and development of unmanned aerial vehicle(UAV) technology, small UAV has also begun to attract the people's attention. Because of its characteristic of remote control, small size, low cost and other advantages, it already has a wide range of applications. However, the management of UAV has become a common problem throughout the world. It is a prerequisite which is how to detect UAV. Nowadays, the wireless signal of the UAV can help us detect it. In the low-Altitude environment, due to the impact of noise, the first step is to identify the start-point of its single accurately. A detection algorithm for UAV signals with an adaptive threshold based on Gaussian mixture model(GMM) is proposed in this paper. The algorithm makes full use of the signal data characteristics, calculates the threshold using the GMM. Meanwhile, it does not need to set the fixed threshold manually. That means it can adaptively detect the wireless signal in a different noise environment. © 2017 IEEE.},
}

@CONFERENCE{Chen2017,
author={Chen, Y. and Wang, B. and Liu, W. and Liu, D.},
title={On-line and non-invasive anomaly detection system for unmanned aerial vehicle},
journal={2017 Prognostics and System Health Management Conference, PHM-Harbin 2017 - Proceedings},
year={2017},
art_number={8079160},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85039963714&doi=10.1109%2fPHM.2017.8079160&partnerID=40&md5=35c11043bdd9cf1d7943646952d4144f},
abstract={There are almost no on-board intelligent anomaly detection systems in most of the existing unmanned Aerial Vehicles (UAVs), and the flight status assessment still depends on ground control station. While, this method can't meet the requirement of real-time anomaly detection for UAV autonomous and safe flight. In order to achieve real-time monitoring of UAV flight status, and improve the reliability and safety of UAVs. In this paper, an on-line and non-invasive embedded anomaly detection system (EADS) is designed to solve the problem of UAV on-board anomaly detection in complex environment. During the flight, whether the sensors and hardware components are abnormal or not is continuously detected via flight data. The proposed embedded anomaly detection system is divided into two parts, (1) hardware platform for heterogeneous calculation is based on Xilinx Zynq-7000 SoC with dual-core Cortex A9 processors and Field Programmable Gate Arrays (FPGA); (2) on-line anomaly detection is based on least squares support vector machine (LS-SVM) algorithm, including flight data preprocessing and analysis. The flight data from Flight Gear is utilized for the demonstration of EADS, and the experiment results show that the proposed system is effective for UAV real-time anomaly detection. © 2017 IEEE.},
}

@CONFERENCE{Sun2017586,
author={Sun, H. and Song, G. and Wei, Z. and Zhang, Y. and Liu, S.},
title={Bilateral teleoperation of an unmanned aerial vehicle for forest fire detection},
journal={2017 IEEE International Conference on Information and Automation, ICIA 2017},
year={2017},
pages={586-591},
art_number={8078976},
note={cited By 6},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85039937431&doi=10.1109%2fICInfA.2017.8078976&partnerID=40&md5=6a34d86e959781698f0da0dd794c9e42},
abstract={In this paper, a bilateral aerial teleoperation system based on force feedback is proposed for monitoring and detecting the forest fires. First of all, an aerial teleoperation system is proposed to enforce the velocity synchronization of the master and the slave. Velocity synchronization is required to achieve motion tracking of the master and slave vehicles. A force reflection is provided to the operator to improve the perceptual sensitivity of the remote environment. In addition, a modified wave variables method is employed to deal with the time-varying delays in the aerial teleoperation system. Then, a forest fire detection algorithm utilizing both color and motion features is presented for detecting the forest fires. Finally, the experiments are conducted to validate the effectiveness of the proposed framework for forest fire detection. © 2017 IEEE.},
}

@ARTICLE{Mohan2017,
author={Mohan, M. and Silva, C.A. and Klauberg, C. and Jat, P. and Catts, G. and Cardil, A. and Hudak, A.T. and Dia, M.},
title={Individual tree detection from unmanned aerial vehicle (UAV) derived canopy height model in an open canopy mixed conifer forest},
journal={Forests},
year={2017},
volume={8},
number={9},
art_number={340},
note={cited By 175},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85029757506&doi=10.3390%2ff8090340&partnerID=40&md5=b628e8279c47b30876a26635c8c8b2eb},
abstract={Advances in Unmanned Aerial Vehicle (UAV) technology and data processing capabilities have made it feasible to obtain high-resolution imagery and three dimensional (3D) data which can be used for forest monitoring and assessing tree attributes. This study evaluates the applicability of low consumer grade cameras attached to UAVs and structure-from-motion (SfM) algorithm for automatic individual tree detection (ITD) using a local-maxima based algorithm on UAV-derived Canopy Height Models (CHMs). This study was conducted in a private forest at Cache Creek located east of Jackson city, Wyoming. Based on the UAV-imagery, we allocated 30 field plots of 20 m × 20 m. For each plot, the number of trees was counted manually using the UAV-derived orthomosaic for reference. A total of 367 reference trees were counted as part of this study and the algorithm detected 312 trees resulting in an accuracy higher than 85% (F-score of 0.86). Overall, the algorithm missed 55 trees (omission errors), and falsely detected 46 trees (commission errors) resulting in a total count of 358 trees. We further determined the impact of fixed tree window sizes (FWS) and fixed smoothing window sizes (SWS) on the ITD accuracy, and detected an inverse relationship between tree density and FWS. From our results, it can be concluded that ITD can be performed with an acceptable accuracy (F > 0.80) from UAV-derived CHMs in an open canopy forest, and has the potential to supplement future research directed towards estimation of above ground biomass and stem volume from UAV-imagery. © 2017 by the authors.},
}

@ARTICLE{Grimaccia20171221,
author={Grimaccia, F. and Leva, S. and Niccolai, A.},
title={PV plant digital mapping for modules' defects detection by unmanned aerial vehicles},
journal={IET Renewable Power Generation},
year={2017},
volume={11},
number={10},
pages={1221-1228},
note={cited By 31},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85029792183&doi=10.1049%2fiet-rpg.2016.1041&partnerID=40&md5=44f9e1987bf1a3d149526461fedc2228},
abstract={Nowadays plant monitoring and control of renewable energy sources can take advantage of the use of unmanned aerial technologies. This manuscript aims to develop an image post-processing tool for remote aerial images able to help operation and maintenance operators in photovoltaic (PV) defects detection using light unmanned aerial vehicles (UAVs). In particular, PV systems deployed in the field in the last ten years show often critical behaviour with a range of failures able to compromise the performance and energy yield of the power plants, thus they can greatly benefit of such novel technologies and tools. The described procedures are here tested on real plant data, with different kind of sensors, in order to find out potential advantages in fast fault detection tasks, using an automatic system for PV plants' mapping. The results of this research will be reported in order to provide an understanding of potential impact of image processing techniques based on UAV in the renewable energy sector. © The Institution of Engineering and Technology 2017.},
}

@CONFERENCE{Yong2017241,
author={Yong, D. and Yaqing, X. and Yuanpeng, Z. and Yu, P. and Datong, L.},
title={Unmanned aerial vehicle sensor data anomaly detection using kernel principle component analysis},
journal={ICEMI 2017 - Proceedings of IEEE 13th International Conference on Electronic Measurement and Instruments},
year={2017},
volume={2018-January},
pages={241-246},
note={cited By 10},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85047185128&doi=10.1109%2fICEMI.2017.8265777&partnerID=40&md5=bcc4b75186443f116c20bf284836ee6d},
abstract={Unmanned aerial vehicle (UAV) has attracted more and more attention for its unique advantages and has been widely used in the military and civilian areas. With expansion of functions of UAV and increased improvement of technical complexity, UAV reliability and security are particularly essential, especially large amount of fleets and insufficient redundancy cause high operating risk and more failures. Sensors are important components in UAVs. Detecting the sensing data can monitor UAV flight condition effectively and analyze the operating status, thus, it is necessary and feasible to detect anomaly with sensing data. Due to the large number of UAV sensors and the high dimensionality of sensing data, it poses a great challenge to the sensor anomaly detection of UAVs. While kernel principal component analysis (KPCA) can effectively deal with large numbers of samples and high dimensional data, and has advantages of simple model and high efficiency of dimensionality reduction. Thus, this work proposes a KPCA based sensor data anomaly detection method. Experimental results with UAV simulated data indicates that using the proposed method to detect the UAV sensing data can obtain satisfied performance. © 2017 IEEE.},
}

@ARTICLE{Xu20171845,
author={Xu, Y. and Yu, G. and Wu, X. and Wang, Y. and Ma, Y.},
title={An Enhanced Viola-Jones Vehicle Detection Method from Unmanned Aerial Vehicles Imagery},
journal={IEEE Transactions on Intelligent Transportation Systems},
year={2017},
volume={18},
number={7},
pages={1845-1856},
art_number={7726065},
note={cited By 53},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84994275151&doi=10.1109%2fTITS.2016.2617202&partnerID=40&md5=334074895bf8700c82ec60c5e539fc7d},
abstract={This research develops an advanced vehicle detection method, which improves the original Viola-Jones (V-J) object detection scheme for better vehicle detections from low-altitude unmanned aerial vehicle (UAV) imagery. The original V-J method is sensitive to objects' in-plane rotation, and therefore has difficulties in detecting vehicles with unknown orientations in UAV images. To address this issue, this research proposes a road orientation adjustment method, which rotates each UAV image once so that the roads and on-road vehicles on rotated images will be aligned with the horizontal direction and the V-J vehicle detector. Then, the original V-J can be directly applied to achieve better efficiency and accuracy. The enhanced V-J method is further applied for vehicle tracking. Testing results show that both vehicle detection and tracking methods are competitive compared with other existing methods. Future research will focus on expanding the current methods to detect other transport modes, such as buses, trucks, motorcycles, bicycles, and pedestrians. © 2017 IEEE.},
}

@CONFERENCE{Santos2017253,
author={Santos, T. and Moreira, M. and Almeida, J. and Dias, A. and Martins, A. and Dinis, J. and Formiga, J. and Silva, E.},
title={PLineD: Vision-based power lines detection for Unmanned Aerial Vehicles},
journal={2017 IEEE International Conference on Autonomous Robot Systems and Competitions, ICARSC 2017},
year={2017},
pages={253-259},
art_number={7964084},
note={cited By 26},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85026879785&doi=10.1109%2fICARSC.2017.7964084&partnerID=40&md5=1d3777cd234f1a9cd3737b06556849e3},
abstract={It is commonly accepted that one of the most important factors for assuring the high performance of an electrical network is the surveillance and the respective preventive maintenance. From a long time ago that TSOs and DSOs incorporate in their maintenance plans the surveillance of the grid, where is included the aerial power lines inspection. Those inspections started by human patrol, including structure climbing when needed and later were substituted by helicopters with powerful sensors and specialised technicians. More recently the Unmanned Aerial Vehicles (UAV) technology has been used, taking advantage of its numerous advantages. This paper addresses the problem of improving the real-time perception capabilities of UAVs for endowing them with capabilities for safe and robust autonomous and semi-autonomous operations. It presents a new vision based power line detection algorithm denoted by PLineD, able to improve the detection robustness even in the presence of image with background noise. The algorithm is tested in real outdoor images of a dataset with multiple backgrounds and weather conditions. The experimental results demonstrate that the proposed approach is effective and able to implemented in real-time image processing pipeline. © 2017 IEEE.},
}

@ARTICLE{Hodgson20171253,
author={Hodgson, A. and Peel, D. and Kelly, N.},
title={Unmanned aerial vehicles for surveying marine fauna: Assessing detection probability},
journal={Ecological Applications},
year={2017},
volume={27},
number={4},
pages={1253-1267},
note={cited By 48},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85020207933&doi=10.1002%2feap.1519&partnerID=40&md5=15b97f97543f82f1edc8532538d93e3a},
abstract={Aerial surveys are conducted for various fauna to assess abundance, distribution, and habitat use over large spatial scales. They are traditionally conducted using light aircraft with observers recording sightings in real time. Unmanned Aerial Vehicles (UAVs) offer an alternative with many potential advantages, including eliminating human risk. To be effective, this emerging platform needs to provide detection rates of animals comparable to traditional methods. UAVs can also acquire new types of information, and this new data requires a reevaluation of traditional analyses used in aerial surveys; including estimating the probability of detecting animals. We conducted 17 replicate UAV surveys of humpback whales (Megaptera novaeangliae) while simultaneously obtaining a 'census' of the population from land-based observations, to assess UAV detection probability. The ScanEagle UAV, carrying a digital SLR camera, continuously captured images (with 75% overlap) along transects covering the visual range of land-based observers. We also used ScanEagle to conduct focal follows of whale pods (n = 12, mean duration = 40 min), to assess a new method of estimating availability. A comparison of the whale detections from the UAV to the land-based census provided an estimated UAV detection probability of 0.33 (CV = 0.25; incorporating both availability and perception biases), which was not affected by environmental covariates (Beaufort sea state, glare, and cloud cover). According to our focal follows, the mean availability was 0.63 (CV = 0.37), with pods including mother/calf pairs having a higher availability (0.86, CV = 0.20) than those without (0.59, CV = 0.38). The follows also revealed (and provided a potential correction for) a downward bias in group size estimates from the UAV surveys, which resulted from asynchronous diving within whale pods, and a relatively short observation window of 9 s. We have shown that UAVs are an effective alternative to traditional methods, providing a detection probability that is within the range of previous studies for our target species. We also describe a method of assessing availability bias that represents spatial and temporal characteristics of a survey, from the same perspective as the survey platform, is benign, and provides additional data on animal behavior. © 2017 by the Ecological Society of America.},
}

@CONFERENCE{Lee201736,
author={Lee, J. and Wang, J. and Crandall, D. and Sabanovic, S. and Fox, G.},
title={Real-time, cloud-based object detection for unmanned aerial vehicles},
journal={Proceedings - 2017 1st IEEE International Conference on Robotic Computing, IRC 2017},
year={2017},
pages={36-43},
art_number={7926512},
note={cited By 68},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85020228778&doi=10.1109%2fIRC.2017.77&partnerID=40&md5=b087e0b27edae1de7eda9d348ddce9e3},
abstract={Real-Time object detection is crucial for many applications of Unmanned Aerial Vehicles (UAVs) such asreconnaissance and surveillance, search-And-rescue, and infras-Tructure inspection. In the last few years, Convolutional NeuralNetworks (CNNs) have emerged as a powerful class of modelsfor recognizing image content, and are widely considered inthe computer vision community to be the de facto standardapproach for most problems. However, object detection basedon CNNs is extremely computationally demanding, typicallyrequiring high-end Graphics Processing Units (GPUs) thatrequire too much power and weight, especially for a lightweightand low-cost drone. In this paper, we propose moving thecomputation to an off-board computing cloud, while keepinglow-level object detection and short-Term navigation onboard. We apply Faster Regions with CNNs (R-CNNs), a state-of-The-Art algorithm, to detect not one or two but hundreds of objecttypes in near real-Time. © 2017 IEEE.},
}

@ARTICLE{Javaid2017427,
author={Javaid, A.Y. and Jahan, F. and Sun, W.},
title={Analysis of Global Positioning System-based attacks and a novel Global Positioning System spoofing detection/mitigation algorithm for unmanned aerial vehicle simulation},
journal={Simulation},
year={2017},
volume={93},
number={5},
pages={427-441},
note={cited By 18},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85015029754&doi=10.1177%2f0037549716685874&partnerID=40&md5=2df2438b029d5e5af43e665ec1d6a8da},
abstract={Simulation test beds serve as a cost-effective and safe way to evaluate the system performance of various real world systems. With the rising concerns in the security of sensitive and critical systems, such as unmanned aerial vehicles (UAVs), a software simulation test bed is clearly the best choice given that the environment and various system components are modeled correctly. This becomes critical given the recently developed autonomous aerial vehicles. We therefore evaluate several available simulation test beds and use the most promising test bed to analyze the impact of Global Positioning System (GPS)-related attacks on navigation of UAVs. We also introduce a novel technique for GPS spoofing, attack detection, and mitigation. This paper presents GPS spoofing and GPS jamming attacks with their anatomy, design, and impact evaluation on navigation as well as a novel GPS spoofing mitigation and detection technique for UAVs, using UAVSim: an open source simulation test bed. © 2017 The Author(s).},
}

@ARTICLE{Byrne2017,
author={Byrne, J. and Laefer, D.F. and O'Keeffe, E.},
title={Maximizing feature detection in aerial unmanned aerial vehicle datasets},
journal={Journal of Applied Remote Sensing},
year={2017},
volume={11},
number={2},
art_number={025015},
note={cited By 9},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85022223838&doi=10.1117%2f1.JRS.11.025015&partnerID=40&md5=7fcbc8aadaafa83c544433809df1e6fa},
abstract={This paper compares several feature detectors applied to imagery from an unmanned aerial vehicle to find the best detection algorithm when applied to datasets that vary in translation and have little or no image overlap. Metrics of inliers and reconstruction accuracy of feature detectors are considered with respect to three-dimensional reconstruction results. The image matching results are tested experimentally, and an approach to detecting false matches is outlined. Results showed that although the detectors varied in the number of keypoints generated, a large number of inliers does not necessarily translate into more points in the final point cloud reconstruction and that the process of comparing a large quantity of redundant keypoints may outweigh the advantage of having the extra points. The results also showed that despite the development of keypoint detectors and descriptors, none of them consistently demonstrated a substantial improvement in the quality of structure from motion reconstruction when applied to a wide range of disparate urban and rural images. © 2017 Society of Photo-Optical Instrumentation Engineers (SPIE).},
}

@ARTICLE{Albetis2017,
author={Albetis, J. and Duthoit, S. and Guttler, F. and Jacquin, A. and Goulard, M. and Poilvé, H. and Féret, J.-B. and Dedieu, G.},
title={Detection of Flavescence dorée grapevine disease using Unmanned Aerial Vehicle (UAV) multispectral imagery},
journal={Remote Sensing},
year={2017},
volume={9},
number={4},
art_number={308},
note={cited By 85},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85017602253&doi=10.3390%2frs9040308&partnerID=40&md5=52dad807d1e3bf2c6452189c6d27e7ad},
abstract={Flavescence dorée is a grapevine disease affecting European vineyards which has severe economic consequences and containing its spread is therefore considered as a major challenge for viticulture. Flavescence dorée is subject to mandatory pest control including removal of the infected vines and, in this context, automatic detection of Flavescence dorée symptomatic vines by unmanned aerial vehicle (UAV) remote sensing could constitute a key diagnosis instrument for growers. The objective of this paper is to evaluate the feasibility of discriminating the Flavescence dorée symptoms in red and white cultivars from healthy vine vegetation using UAV multispectral imagery. Exhaustive ground truth data and UAV multispectral imagery (visible and near-infrared domain) have been acquired in September 2015 over four selected vineyards in Southwest France. Spectral signatures of healthy and symptomatic plants were studied with a set of 20 variables computed from the UAV images (spectral bands, vegetation indices and biophysical parameters) using univariate and multivariate classification approaches. Best results were achieved with red cultivars (both using univariate and multivariate approaches). For white cultivars, results were not satisfactory either for the univariate or the multivariate. Nevertheless, external accuracy assessment show that despite problems of Flavescence dorée and healthy pixel misclassification, an operational Flavescence dorée mapping technique using UAV-based imagery can still be proposed. © 2017 by the authors.},
}

@CONFERENCE{Lee2017252,
author={Lee, W. and Kim, S. and Lee, Y.-T. and Lee, H.-W. and Choi, M.},
title={Deep neural networks for wild fire detection with unmanned aerial vehicle},
journal={2017 IEEE International Conference on Consumer Electronics, ICCE 2017},
year={2017},
pages={252-253},
art_number={7889305},
note={cited By 33},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85018308708&doi=10.1109%2fICCE.2017.7889305&partnerID=40&md5=a165a0f5f9f33c4d8d88cc1befafda9d},
abstract={Wildfire threatens people's lives and livelihoods. Wildfires kill hundreds of thousand people worldwide each year. Disaster information services are required to save lives and reduce economic losses when wildfire occurs. However, manned airplanes are too expensive to operate for frequent wildland monitoring. Satellite images cannot be used for early wildfire detection due to low temporal resolution and low spatial resolution. Unmanned aerial vehicles are cost-effective means to provide high resolution images for wildfire detection. A wildfire detection system utilizing unmanned aerial vehicles was developed with deep convolutional neural networks. The system achieved high accuracy for wide range of aerial photographs. © 2017 IEEE.},
}

@CONFERENCE{Ueareeworakul2017332,
author={Ueareeworakul, P. and Saiyod, S.},
title={Obstacle detection algorithm for Unmanned Aerial Vehicles using binocular stereoscopic vision},
journal={2017 9th International Conference on Knowledge and Smart Technology: Crunching Information of Everything, KST 2017},
year={2017},
pages={332-337},
art_number={7886116},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85017502932&doi=10.1109%2fKST.2017.7886116&partnerID=40&md5=0f4907a94d79c2f97546dcdae4d352ea},
abstract={Unmanned Aerial Vehicles are currently gaining widespread adoption in multiple roles. In this paper, we proposes obstacle detection algorithm for unmanned aerial vehicles using stereoscopic vision. Depth of objects in the image could be calculated. There is also another important property of image captured by a stereo camera; if an object is at a certain position it will appear at a certain combination of location in images from left and right camera but not any other. This property can be used to detect obstacles by checking a number of sample point placed in a grid in front of the drone. For each point we then use the property stated above to check if locations in the image specified by the property matches. We have evaluated the effectiveness of this algorithm. This algorithm scored 17 out of 20 cases within acceptable time constraints, which demonstrated its worthiness for further developments. © 2017 IEEE.},
}

@ARTICLE{Poblete-Echeverría2017,
author={Poblete-Echeverría, C. and Olmedo, G.F. and Ingram, B. and Bardeen, M.},
title={Detection and segmentation of vine canopy in ultra-high spatial resolution RGB imagery obtained from Unmanned Aerial Vehicle (UAV): A case study in a commercial vineyard},
journal={Remote Sensing},
year={2017},
volume={9},
number={3},
art_number={268},
note={cited By 52},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85019391220&doi=10.3390%2frs9030268&partnerID=40&md5=7c531e170c9ad089d8a43e2bd7ecafec},
abstract={The use of Unmanned Aerial Vehicles (UAVs) in viticulture permits the capture of aerial Red-Green-Blue (RGB) images with an ultra-high spatial resolution. Recent studies have demonstrated that RGB images can be used to monitor spatial variability of vine biophysical parameters. However, for estimating these parameters, accurate and automated segmentation methods are required to extract relevant information from RGB images. Manual segmentation of aerial images is a laborious and time-consuming process. Traditional classification methods have shown satisfactory results in the segmentation of RGB images for diverse applications and surfaces, however, in the case of commercial vineyards, it is necessary to consider some particularities inherent to canopy size in the vertical trellis systems (VSP) such as shadow effect and different soil conditions in inter-rows (mixed information of soil and weeds). Therefore, the objective of this study was to compare the performance of four classification methods (K-means, Artificial Neural Networks (ANN), Random Forest (RForest) and Spectral Indices (SI)) to detect canopy in a vineyard trained on VSP. Six flights were carried out from post-flowering to harvest in a commercial vineyard cv. Carménère using a low-cost UAV equipped with a conventional RGB camera. The results show that the ANN and the simple SI method complemented with the Otsu method for thresholding presented the best performance for the detection of the vine canopy with high overall accuracy values for all study days. Spectral indices presented the best performance in the detection of Plant class (Vine canopy) with an overall accuracy of around 0.99. However, considering the performance pixel by pixel, the Spectral indices are not able to discriminate between Soil and Shadow class. The best performance in the classification of three classes (Plant, Soil, and Shadow) of vineyard RGB images, was obtained when the SI values were used as input data in trained methods (ANN and RForest), reaching overall accuracy values around 0.98 with high sensitivity values for the three classes. © 2017 by the authors.},
}

@ARTICLE{Jenie2017558,
author={Jenie, Y.I. and Van Kampen, E.-J. and Ellerbroek, J. and Hoekstra, J.M.},
title={Taxonomy of Conflict Detection and Resolution Approaches for Unmanned Aerial Vehicle in an Integrated Airspace},
journal={IEEE Transactions on Intelligent Transportation Systems},
year={2017},
volume={18},
number={3},
pages={558-567},
art_number={7519023},
note={cited By 28},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84979266050&doi=10.1109%2fTITS.2016.2580219&partnerID=40&md5=45abb5d8836e1e48e8a4fe88a86d1aab},
abstract={This paper proposes a taxonomy of conflict detection and resolution (CDR) approaches for operating unmanned aerial vehicles (UAVs) in an integrated airspace. Possible approaches for UAVs are surveyed and broken down based on their types of surveillance, coordination, maneuvering, and autonomy. The factors are combined back selectively, with regard to their feasibility for operation in an integrated airspace, into several 'generic approaches' that form the CDR taxonomy. These generic approaches are then attributed to a number of available methods in the literature to determine their position in the overall CDR scheme. The attribution shows that many proposed methods are actually unsuitable for operation in an integrated airspace. Furthermore, some part of the taxonomy does not have an adequate representative in the literature, suggesting the need to concentrate UAV CDR research more in those particular parts. Finally, a multilayered CDR architecture is built from the taxonomy, implementing the concept of defense in depth to ensure safe operation of UAVs in an integrated civil airspace. © 2000-2011 IEEE.},
}

@CONFERENCE{Herdjunanto2017,
author={Herdjunanto, S.},
title={Actuator fault signal isolation of an unmanned aerial vehicle (UAV) quadrotor based on detection filter},
journal={Proceedings of 2016 8th International Conference on Information Technology and Electrical Engineering: Empowering Technology for Better Future, ICITEE 2016},
year={2017},
art_number={7863232},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85015990269&doi=10.1109%2fICITEED.2016.7863232&partnerID=40&md5=1e273b2354725ae4983ca53cdfafd57c},
abstract={A quadrotor which has four actuators becomes an active object research in the area of identification, control related to each formation to cover certain area such as in the surveillance mission. The performance of the quadrotor is determined, one out of several possibilities, by the working condition of each actuators. Therefore, the states of healthiness of the actuators should be monitored. In other words, if there is an actuator fault signal, it should be isolated immediately. In this paper, a detection filter is proposed to solve actuator fault signal isolation on the quadrotor in hovering motion since the detection filter can generate decoupled detection space which corresponds to each actuator fault signal if mutually detectable requirement is satisfied. The result shows that mutually detectable requirement is satisfied by adding a virtual actuator vector and detection filter gain is succesfully calculated so that decoupled detection spaces can be obtained. © 2016 IEEE.},
}

@CONFERENCE{Mukadam2017,
author={Mukadam, K. and Sinh, A. and Karani, R.},
title={Detection of landing areas for unmanned aerial vehicles},
journal={Proceedings - 2nd International Conference on Computing, Communication, Control and Automation, ICCUBEA 2016},
year={2017},
art_number={7860044},
note={cited By 10},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85016195903&doi=10.1109%2fICCUBEA.2016.7860044&partnerID=40&md5=67c4a2742f83f9cd9baffcdf81bf133f},
abstract={Unmanned aerial vehicles (UAV), also referred to as drones, are a growing field in computer science with applications in military systems, delivery services, emergency relief and evacuation. One of the primary obstructions to the allowance of UAV journeys over populated areas is the lack of sophisticated automated systems that detect drone landing sites. In this paper, we propose a landing area detection system using machine learning and image processing. This system compares the suitability of various features (RGB Color Model, HSV Color Model, LBP, Edge Density) in determining a suitable drop-off point. Classification on these features has been carried out using Support Vector Machines (Linear, Polynomial and RBF Kernel).},
}

@CONFERENCE{Yuan20171870,
author={Yuan, C. and Ghamry, K.A. and Liu, Z. and Zhang, Y.},
title={Unmanned aerial vehicle based forest fire monitoring and detection using image processing technique},
journal={CGNCC 2016 - 2016 IEEE Chinese Guidance, Navigation and Control Conference},
year={2017},
pages={1870-1875},
art_number={7829074},
note={cited By 27},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85015160819&doi=10.1109%2fCGNCC.2016.7829074&partnerID=40&md5=5513342c6929286bbcd169c6988f6f20},
abstract={Early forest fire alarm systems are critical in making prompt response in the event of unexpected hazards. Cost-effective cameras, improvements in memory, and enhanced computation power have all enabled the design and real-time application of fire detecting algorithms using light and small-size embedded surveillance systems. This is vital in situations where the performance of traditional forest fire monitoring and detection techniques are unsatisfactory. This paper presents a forest fire monitoring and detection method with visual sensors onboard unmanned aerial vehicle (UAV). Both color and motion features of fire are adopted for the design of the studied forest fire detection strategies. This is for the purpose of improving fire detection performance, while reducing false alarm rates. Indoor experiments are conducted to demonstrate the effectiveness of the studied forest fire detection methodologies. © 2016 IEEE.},
}

@ARTICLE{Hu2017B214,
author={Hu, S. and Goldman, G.H. and Borel-Donohue, C.C.},
title={Detection of unmanned aerial vehicles using a visible camera system},
journal={Applied Optics},
year={2017},
volume={56},
number={3},
pages={B214-B221},
note={cited By 27},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85010223691&doi=10.1364%2fAO.56.00B214&partnerID=40&md5=20b69b895e54b22ce27b4e37367de845},
abstract={Unmanned aerial vehicles (UAVs) flown by adversaries are an emerging asymmetric threat to homeland security and the military. To help address this threat, we developed and tested a computationally efficient UAV detection algorithm consisting of horizon finding, motion feature extraction, blob analysis, and coherence analysis. We compare the performance of this algorithm against two variants, one using the difference image intensity as the motion features and another using higher-order moments. The proposed algorithm and its variants are tested using field test data of a group 3 UAV acquired with a panoramic video camera in the visible spectrum. The performance of the algorithms was evaluated using receiver operating characteristic curves. The results show that the proposed approach had the best performance compared to the two algorithmic variants. © 2017 Optical Society of America.},
}

@CONFERENCE{Farlik2017,
author={Farlik, J. and Kratky, M. and Casar, J. and Stary, V.},
title={Radar cross section and detection of small unmanned aerial vehicles},
journal={Proceedings of the 2016 17th International Conference on Mechatronics - Mechatronika, ME 2016},
year={2017},
art_number={7827857},
note={cited By 23},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85015281565&partnerID=40&md5=58f9f55c6dee2fe732474ddb0f6fc4ad},
abstract={Commercial availability of small UAV's and their capabilities raises the question of the ability to defend against these assets, which could be used, or misused, as the air threat. This paper brings results of the series of experiments with the commercial quadcopter DJI Phantom 2 Vision that were performed by Department of Air Defense Systems/University of Defense Brno members in laboratory (anechoic chamber) and in the exterior as well. Terrain tests were done using military Doppler radar, with respect to the laboratory-measured radar cross section. Besides this, the visibility, audibility and other aspects of possible misuse of the drone were determined and analyzed for to find possible and identify optimal means for their detection. © 2016 Czech Technical University in Prague.},
}

@CONFERENCE{Guldogan2017,
author={Guldogan, O. and Rotola-Pukkila, J. and Balasundaram, U. and Le, T.-H. and Mannar, K. and Chrisna, T.M. and Gabbouj, M.},
title={Automated tree detection and density calculation using unmanned aerial vehicles},
journal={VCIP 2016 - 30th Anniversary of Visual Communication and Image Processing},
year={2017},
art_number={7805572},
note={cited By 9},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85011088676&doi=10.1109%2fVCIP.2016.7805572&partnerID=40&md5=729d273db5f88372483337ced13f39c3},
abstract={Growth monitoring in tree plantation farms plays a crucial role in taking necessary actions from early stages to improve harvesting efficiency. Unmanned aerial vehicles (UAVs) provide a fast and efficient way to acquire data from large farms with difficult access. We propose a novel end-to-end system composed of multiple stages to identify areas where seeds have not grown as expected in young tree farms. The system acquires data from UAV flights to generate georeferenced orthophoto images. Next, local binary patterns, distance transform, and watershed segmentation methods are applied on images to detect trees. Finally, tree density distributions are calculated in the granularity of approximately 90 m2 tiles. We assessed the system performance by comparing detection results against a ground truth set of over 50000 trees from 16 orthophoto images for two tree species. The median deviation was 2 trees per tile for both species, where the median tree count was 14 and 9 per tile, respectively. © 2016 IEEE.},
}

@CONFERENCE{Pinkerman2017,
author={Pinkerman, C.W. and O’Connell, T.J. and Arena, A.S.},
title={Uncertainty analysis of avian approach to remote thermal updraft detection for unmanned aerial vehicles},
journal={AIAA Atmospheric Flight Mechanics Conference, 2017},
year={2017},
page_count={34},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85086057985&doi=10.2514%2f6.2017-1190&partnerID=40&md5=5abcd6af74c6211dc1fc385e1bd558a0},
abstract={Thermal updrafts can be utilized to increase an aircraft’s flight endurance and range. However, much of the discussion involving thermal updrafts comprise of flight techniques within known thermal updrafts while little is discussed over the detection of thermals without the influence of the upward or downward velocity components. This paper discusses an uncertainty analysis of using a single method for locating thermal updrafts which was hypothesized from looking at thermal detection from avian and RC viewpoints. An avian study was conducted to gather information on how avian soaring species locate thermal updrafts, in which no definitive answer was found. Of the possible theories of avian thermal location methods, combined with methods used from RC aircraft, a single method was studied through simulation and experimentation to construct possible applications to unmanned aerial systems. This method attempted to quantify wind shifts in the local area to give indication of the direction and location of local thermal updrafts. Due to the high magnitudes of uncertainty found during the experimental approach, and later portrayed in additional simulations, the tested method was shown to be unfavorable for use in remotely detecting thermal updrafts until additional methods can be added in order to minimize the uncertainty. © 2017, American Institute of Aeronautics and Astronautics Inc, AIAA. All rights reserved.},
}

@CONFERENCE{Omar20171,
author={Omar, T. and Nehdi, M.L.},
title={Thermal detection of subsurface delaminations in reinforced concrete bridge decks using unmanned aerial vehicle},
journal={American Concrete Institute, ACI Special Publication},
year={2017},
volume={2017-March},
number={SP 331},
pages={1-14},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85071913324&partnerID=40&md5=3c1816e871c06c6c8de46407b770be77},
abstract={Bridge deck condition assessment is commonly conducted through visual inspection by bridge inspectors. Considering the colossal backlog of aging bridge structures, there is a need to develop cost-effective and innovative solutions to evaluate bridge deck conditions on regular time intervals, without interrupting traffic. This makes remote sensing technologies viable options in the field of bridge inspection. This paper explores the potential for applying infrared thermography (IRT) using unmanned aerial vehicle (UAV) to detect and quantify subsurface delaminations in concrete bridge decks. The UAV-borne thermal sensing system focuses on acquiring thermal imagery using a UAV and extracting information from the image data. Two in-service concrete bridge decks were inspected using a high resolution thermal camera mounted on a UAV. The captured images were then enhanced and stitched together using a tailored procedure to produce a mosaic view of the entire bridge deck, indicating the size and geometry of the detected delaminated areas. The results were validated by conducting hammer sounding and half-cell potential testing on the same bridge decks. The findings reveal the capability of the technology to provide measurements comparable to those derived from traditional hands-on inspection methods. Thus, it can be an excellent aid in efficient bridge maintenance and repair decision-making. © 2017 American Concrete Institute. All rights reserved.},
}

@ARTICLE{Seier2017332,
author={Seier, G. and Sulzer, W. and Wecht, M. and Schöttl, S. and Sass, O.},
title={Change detection of a mountain creek using an unmanned aerial vehicle [Veränderungsdetektion eines wildbaches mittels unbemanntem luftfahrzeug]},
journal={AGIT- Journal fur Angewandte Geoinformatik},
year={2017},
volume={3},
pages={332-342},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85051975590&doi=10.14627%2f537633037&partnerID=40&md5=dc52dbeb7006367d0637862508fdfafc},
abstract={In 2011 a flood occurred in the small town of Oberwölz (Upper Styria). This was the reason for a fluvial-geomorphologic research project that was carried out for the catchment of Schöttlbach creek. In this study we focus on both, the results generated using an unmanned aerial vehicle (UAV) as well as the spatial focus that lies on the Krummeggerbach creek causing the sediment transport to the main area of deposition at the Schöttlbach creek. By doing two flight campaigns high resolution data was generated that, combined with independent validation measurements, allows meaningful insights concerning the change of the earth’s surface. The main outcome is a statement about the applicability of UAVs for river sciences. © Wichmann Verlag, VDE VERLAG GMBH · Berlin · Offenbach.},
}

@CONFERENCE{Alvarez-Montoya201777,
author={Alvarez-Montoya, J. and Carvajal-Castrillón, A. and Betancur-Agudelo, L. and Amaya-Fernández, F. and Nino-Navia, J. and Sierra-Pérez, J.},
title={Development of a remote acquisition and transmission system of strain measurements in an unmanned aerial vehicle for damage detection},
journal={Structural Health Monitoring 2017: Real-Time Material State Awareness and Data-Driven Safety Assurance - Proceedings of the 11th International Workshop on Structural Health Monitoring, IWSHM 2017},
year={2017},
volume={1},
pages={77-85},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85032456199&doi=10.12783%2fshm2017%2f13852&partnerID=40&md5=c83ab960002cd67497b61efb442e26b7},
abstract={Reliability is a key requirement in the aerospace industry. Therefore, structural health monitoring (SHM) applications using strain-field estimation and pattern recognition techniques are in development as an alternative to improve reliability and reduce maintenance costs, promising to ease damage detection on aerospace structures. However, some challenges need to be resolved before real implementation of these techniques. One of these challenges is to uncouple operational conditions changes in strain field from those related directly to damage. In this paper, the development of a strain measurement remote acquisition and transmission system on an unmanned aerial vehicle (UAV) using Fiber Grating Sensors (FBGs) is presented. Before flight testing, ground tests are carried out to emulate the dynamic loads that will be presented during flight. The strain data acquired are processed using unsupervised learning algorithms based on Self-Organizing Maps (SOM) and DS2L-SOM (density-based techniques) in order to classify different operational conditions. The results showed the capability of the system for classifying different load conditions for a UAV's main beam.},
}

@CONFERENCE{Phung2017823,
author={Phung, M.D. and Dinh, T.H. and Hoang, V.T. and Ha, Q.P.},
title={Automatic crack detection in built infrastructure using unmanned aerial vehicles},
journal={ISARC 2017 - Proceedings of the 34th International Symposium on Automation and Robotics in Construction},
year={2017},
pages={823-829},
note={cited By 18},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85032340481&doi=10.22260%2fisarc2017%2f0115&partnerID=40&md5=11d67958d77967cba0f65c69d640acb2},
abstract={This paper addresses the problem of crack detection which is essential for health monitoring of built infrastructure. Our approach includes two stages, data collection using unmanned aerial vehicles (UAVs) and crack detection using histogram analysis. For the data collection, a 3D model of the structure is first created by using laser scanners. Based on the model, geometric properties are extracted to generate way points necessary for navigating the UAV to take images of the structure. Then, our next step is to stick together those obtained images from the overlapped field of view. The resulting image is then clustered by histogram analysis and peak detection. Potential cracks are finally identified by using locally adaptive thresholds. The whole process is automatically carried out so that the inspection time is significantly improved while safety hazards can be minimised. A prototypical system has been developed for evaluation and experimental results are included.},
}

@ARTICLE{Negash2017551,
author={Negash, L. and Kim, S.-H. and Choi, H.-L.},
title={Distributed observes for cyberattack detection and isolation in formation-flying unmanned aerial vehicles},
journal={Journal of Aerospace Information Systems},
year={2017},
volume={14},
number={10},
pages={551-565},
note={cited By 12},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85030167318&doi=10.2514%2f1.I010531&partnerID=40&md5=57303964c48de53e51c128acf0aebbf2},
abstract={In this paper, cyberattack detection and isolation is studied for a network of formation-flying unmanned aerial vehicles.Astheunmannedaerial vehicles communicateto reach consensusontheir states while making the formation, the communication network among the unmanned aerial vehicles makes them vulnerable to a potential attack from malicious adversaries. Two types of attacks pertinent toa networkof unmanned aerial vehicles have been considered: a node attack on the unmanned aerial vehicles and a deception attack on the communication between the unmanned aerial vehicles. Unmanned aerial vehicle formation control involves using a consensus algorithm to maintain a prespecified formation. Two kindsofcyberattacksinthe unmanned aerial vehicle network (node and communication path deception) are considered with their respective models in the formation setup. A bank of unknown input observer-based distributed fault detection schemesaswellaswitharule basedonresidual generated using the bank of unknown input observers are proposedto detect the attacks and toidentify the compromised unmanned aerial vehicle in the formation. Furthermore, an algorithm is developed to remove the faulty unmanned aerial vehicle from the network and to keep the compromised unmanned aerial vehicle isolated once an attackis detected, while maintaining the flight formation with a missing unmanned aerial vehicle node.},
}

@ARTICLE{Jeong2017823,
author={Jeong, H.-J. and Lee, M.-J. and Lee, C.E. and Kim, S.-H. and Ha, Y.-G.},
title={Machine learning-based real-time anomaly detection for unmanned aerial vehicles with a cloud server},
journal={Journal of Internet Technology},
year={2017},
volume={18},
number={4},
pages={823-832},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85028467371&doi=10.6138%2fJIT.2017.18.4.20160130b&partnerID=40&md5=ee44aed35aa98818470dfe918f25f55d},
abstract={There has been an increase in the use of unmanned aerial vehicles (UAVs) for carrying out various tasks. UAVs are much smaller than manned aircrafts and do not risk the pilot's life, which makes UAVs more versatile and costeffective than regular aircrafts. However, UAVs are at risk when encountering unexpected events, such as control disruptions from intentional attacks. This raises securityand safety-related issues for the use of UAVs. To deal with such issues, this paper proposes a UAV control system that uses machine-learning technology to detect anomalies. The proposed system provides analytical redundancy by analyzing numerical data based on mathematical models. Machine learning generally requires large amounts of data to produce meaningful outcomes, and the proposed UAV control system meets these requirements since it has the ability to collect large amounts of data from UAVs. Two types of flight circumstances were simulated in an experiment. One involved the security of the UAV control system, and the other involved the safety of the UAV itself. A real-time anomaly detection system for the proposed UAV control system is also introduced and experimental results are described in detail.},
}

@CONFERENCE{Laurenzis2017,
author={Laurenzis, M. and Bacher, E. and Christnacher, F.},
title={Measuring laser reflection cross-sections of small unmanned aerial vehicles for laser detection, ranging and tracking},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2017},
volume={10191},
art_number={101910D},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85025176864&doi=10.1117%2f12.2261928&partnerID=40&md5=9233be53d541f7d75beb0e29cc997af3},
abstract={An increasing number of incidents are reported where small unmanned aerial vehicles (UAV) are involved flying at low altitude. Thus UAVs are becoming more and more a serious threat in civilian and military scenarios leading to serious danger to safety or privacy issues. In this context, the detection and tracking of small UAV flying at low altitude in urban environment or near background structures is a challenge for state of the art detection technologies. In this paper, we focus on detection, tracking and identification by laser sensing technologies that are Laser Gated Viewing and scanning LiDAR. The laser reflection cross-sections (LRCS) has direct impact on the probability to detection and capability for range measurement. Here, we present methods to determine the laser reflection cross-sections by experimental and computational approaches. © 2017 SPIE.},
}

@ARTICLE{Lif2017136,
author={Lif, P. and Näsström, F. and Tolt, G. and Hedström, J. and Allvar, J.},
title={Visual and IR-based target detection from unmanned aerial vehicle},
journal={Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
year={2017},
volume={10273 LNCS},
pages={136-144},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85025132575&doi=10.1007%2f978-3-319-58521-5_10&partnerID=40&md5=7d59fda481c941ef3a029a84ff466056},
abstract={In many situations it is important to detect and identify people and vehicles. In this study the purpose was to investigate subject’s performance to detect and estimate number of stationary people on the ground. The unmanned aerial vehicle used visual- and infrared sensor, wide and narrow field of view, and ground speed 8 m/s and 12 m/s. Participants watched synthetic video sequences captured from an unmanned aerial vehicle. The results from this study demonstrated that the ability to detect people was affected by type of sensor and field of view. It took significantly longer time to detect targets with the infrared sensor than with the visual sensor, and it took significantly longer time with wider field of view than with narrow field of view. The ability to assess number of targets was affected by type of sensor and speed, the infrared sensor causing more problems than the visual sensor. Also, performance decreased at higher speed. © Springer International Publishing AG 2017.},
}

@CONFERENCE{Laurenzis2017,
author={Laurenzis, M. and Hengy, S. and Hommes, A. and Kloeppel, F. and Shoykhetbrod, A. and Geibig, T. and Johannes, W. and Naz, P. and Christnacher, F.},
title={Multi-sensor field trials for detection and tracking of multiple small unmanned aerial vehicles flying at low altitude},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2017},
volume={10200},
art_number={102001A},
note={cited By 21},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85023204614&doi=10.1117%2f12.2261930&partnerID=40&md5=54309082257f38e6c256535f93b940ce},
abstract={Small unmanned aerial vehicles (UAV) flying at low altitude are becoming more and more a serious threat in civilian and military scenarios. In recent past, numerous incidents have been reported where small UAV were flying in security areas leading to serious danger to public safety or privacy. The detection and tracking of small UAV is a widely discussed topic. Especially, small UAV flying at low altitude in urban environment or near background structures and the detection of multiple UAV at the same time is challenging. Field trials were carried out to investigate the detection and tracking of multiple UAV flying at low altitude with state of the art detection technologies. Here, we present results which were achieved using a heterogeneous sensor network consisting of acoustic antennas, small frequency modulated continuous wave (FMCW) RADAR systems and optical sensors. While acoustics, RADAR and LiDAR were applied to monitor a wide azimuthal area (360°) and to simultaneously track multiple UAV, optical sensors were used for sequential identification with a very narrow field of view. © 2017 SPIE.},
}

@CONFERENCE{Shleymovich2017,
author={Shleymovich, M.P. and Medvedev, M.V. and Lyasheva, S.A.},
title={Image analysis in unmanned aerial vehicle on-board system for objects detection and recognition with the help of energy characteristics based on wavelet transform},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2017},
volume={10342},
art_number={1034210},
note={cited By 23},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85020084510&doi=10.1117%2f12.2270141&partnerID=40&md5=217b51b3aa07519b3abf4a755d37e462},
abstract={In this article the problem of image analysis in unmanned aerial vehicle on-board system for objects detection and recognition with the help of energy characteristics based on wavelet transform is described. The approach of salient points extraction based on wavelet transform is proposed. The salience of the points is substantiated with the energy estimates of their weights. On the basis of wavelet transform salient points extraction the method of image contour segmentation is proposed. For further image recognition the salient points descriptors constructed with the help of wavelet transform are used. The objects detection and recognition system for unmanned aerial vehicles based on proposed methods is simulated using the simulation platform. © 2017 SPIE.},
}

@ARTICLE{Liu2016,
author={Liu, K. and Ding, H. and Tang, G. and Na, J. and Huang, X. and Xue, Z. and Yang, X. and Li, F.},
title={Detection of catchment-scale gully-affected areas using Unmanned Aerial Vehicle (UAV) on the Chinese Loess Plateau},
journal={ISPRS International Journal of Geo-Information},
year={2016},
volume={5},
number={12},
art_number={238},
note={cited By 38},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85019580524&doi=10.3390%2fijgi5120238&partnerID=40&md5=56eab284408b1ee3f79bcee24b6a4442},
abstract={The Chinese Loess Plateau suffers from serious gully erosion induced by natural and human causes. Gully-affected areas detection is the basic work in this region for gully erosion assessment and monitoring. For the first time, an unmanned aerial vehicle (UAV) was applied to extract gully features in this region. Two typical catchments in Changwu and Ansai were selected to represent loess tableland and loess hilly regions, respectively. A high-powered quadrocopter (md4-1000) equipped with a non-metric camera was used for image acquisition. InPho and MapMatrix were applied for semi-automatic workflow including aerial triangulation and model generation. Based on the stereo-imaging and the ground control points, the highly detailed digital elevation models (DEMs) and ortho-mosaics were generated. Subsequently, an object-based approach combined with the random forest classifier was designed to detect gully-affected areas. Two experiments were conducted to investigate the influences of segmentation strategy and feature selection. Results showed that vertical and horizontal root-mean-square errors were below 0.5 and 0.2 m, respectively, which were ideal for the Loess Plateau region. The overall extraction accuracy in Changwu and Ansai achieved was 84.62% and 86.46%, respectively, which indicated the potential of the proposed workflow for extracting gully features. This study demonstrated that UAV can bridge the gap between field measurement and satellite-based remote sensing, obtaining a balance in resolution and efficiency for catchment-scale gully erosion research. © 2016 by the authors.},
}

@ARTICLE{Kim2016619,
author={Kim, D. and Youn, J. and Kim, C.},
title={Automatic detection of malfunctioning photovoltaic modules using unmanned aerial vehicle thermal infrared images},
journal={Journal of the Korean Society of Surveying, Geodesy, Photogrammetry and Cartography},
year={2016},
volume={34},
number={6},
pages={619-627},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85017562570&doi=10.7848%2fksgpc.2016.34.6.619&partnerID=40&md5=19fb8531de1ab62d66cf2f4de7697057},
abstract={Cells of a PV (photovoltaic) module can suffer defects due to various causes resulting in a loss of power output. As a malfunctioning cell has a higher temperature than adjacent normal cells, it can be easily detected with a thermal infrared sensor. A conventional method of PV cell inspection is to use a hand-held infrared sensor for visual inspection. The main disadvantages of this method, when applied to a large-scale PV power plant, are that it is time-consuming and costly. This paper presents an algorithm for automatically detecting defective PV panels using images captured with a thermal imaging camera from an UAV (unmanned aerial vehicle). The proposed algorithm uses statistical analysis of thermal intensity (surface temperature) characteristics of each PV module to verify the mean intensity and standard deviation of each panel as parameters for fault diagnosis. One of the characteristics of thermal infrared imaging is that the larger the distance between sensor and target, the lower the measured temperature of the object. Consequently, a global detection rule using the mean intensity of all panels in the fault detection algorithm is not applicable. Therefore, a local detection rule was applied to automatically detect defective panels using the mean intensity and standard deviation range of each panel by array. The performance of the proposed algorithm was tested on three sample images; this verified a detection accuracy of defective panels of 97% or higher. In addition, as the proposed algorithm can adjust the range of threshold values for judging malfunction at the array level, the local detection rule is considered better suited for highly sensitive fault detection compared to a global detection rule. In this study, we used a panel area extraction method that we previously developed; fault detection accuracy would be improved if panel area extraction from images was more precise. Furthermore, the proposed algorithm contributes to the development of a maintenance and repair system for large-scale PV power plants, in combination with a geo-referencing algorithm for accurate determination of panel locations using sensor-based orientation parameters and photogrammetry from ground control points.},
}

@CONFERENCE{Klavins2016400,
author={Klavins, E. and Zagursky, V.},
title={Unmanned Aerial Vehicle Movement Trajectory Detection in Open Environment},
journal={Procedia Computer Science},
year={2016},
volume={104},
pages={400-407},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85016087175&doi=10.1016%2fj.procs.2017.01.152&partnerID=40&md5=5f4239aa76b699e0fd5ba344489b7e83},
abstract={Unmanned aerial vehicles have become more widely used for entertainment, security, building inspection and for other similar tasks. Inertial Navigations Systems (INS) is one of the main area of research for UAVs to control their flights through buildings or near constructions where flight paths must be controlled or recorded. In this paper is collected some approaches, which can be used for UAV onboard trajectory determination where GPS cannot be used are determined. Approach includes onboard inertial measurement unit system and image sensors. Fusing UAVs controlling methods and computer vision gives possibility to increase inertial navigation system accuracy. To determine distance to obstacles dual vision cameras must be used. © 2017 The Authors.},
}

@ARTICLE{Dolgopolov20161,
author={Dolgopolov, A.V. and Kazantsev, P.A. and Bezuhliy, N.N.},
title={Ship detection in images obtained from the unmanned aerial vehicle (uav)},
journal={Indian Journal of Science and Technology},
year={2016},
volume={9},
number={46},
pages={1-7},
note={cited By 6},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85008640812&doi=10.17485%2fijst%2f2016%2fv9i46%2f107562&partnerID=40&md5=a108a516064142706cc3fd5c7315fde8},
abstract={Background/Objectives: The main objective of this work is the creation of a new algorithm for detecting ships in the high resolution images obtained by unmanned aerial vehicle. Method: To achieve the objective the developed ship detection algorithm uses two cascades: shape-based cascade and cascade based on automatically extracted features. Deep neural network autoencoder is applied for automatic feature extraction. Findings: Images from Google Maps, Yandex Maps, and a small fraction of the images taken from the Internet were used for training and testing the developed approach. In total, the dataset consists of 1000 images containing ships. On average, each image contains 5.1 ships. The dataset was divided into training (50%) and test (50%). Detection quality was estimated using the Recall and Precision metrics. Our study has shown that the combined use of shape-based cascade and cascade based on automatically extracted features allows achieving high quality (Recall: 0.95, Precision: 0.94) and performance in the problem of ship detection by UAV. The results demonstrate that the proposed method is comparable or slightly outperforms the state-of-the-art methods. Improvements/Applications: Applying the detector in real video from the UAV, it would be possible to improve performance by parallelization of this approach on the GPU.},
}

@ARTICLE{Scobie2016781,
author={Scobie, C.A. and Hugenholtz, C.H.},
title={Wildlife monitoring with unmanned aerial vehicles: Quantifying distance to auditory detection},
journal={Wildlife Society Bulletin},
year={2016},
volume={40},
number={4},
pages={781-785},
note={cited By 18},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84995677648&doi=10.1002%2fwsb.700&partnerID=40&md5=a6479cc3f871c4f102188372d7f71e8f},
abstract={There is growing application of small unmanned aerial vehicles (UAVs) for detecting, enumerating, and monitoring wildlife. However, little is known about how the sound from UAVs may be affecting wildlife being studied. We quantified sound levels of 2 UAVs to determine minimum altitudes they can fly before being aurally detected by wildlife. We tested a small quadcopter (SkyRanger; Aeryon Labs, Inc., Waterloo, ON, Canada) and a fixed-wing platform (eBee; Sensefly Ltd., Cheseaux-sur-Lausanne, Vaud, Switzerland) at the University of Calgary in Calgary, Alberta, Canada, between 1000 and 1200 hours on 27 September 2014. We modeled sound propagation and attenuation in relation to the lower hearing thresholds for 3 game species and 2 species of predators. Results indicate that the UAV sound levels differed in the lower frequency ranges, but were otherwise similar above 1.25 kHz. The domestic cat (Felis silvestris catus) has the lowest hearing threshold, with the capacity to hear both UAVs from the furthest distance; whereas, the mallard (Anas platyrhynchos) has the greatest hearing threshold, which means UAVs can be closer before being aurally detected. Because flying height is related to image resolution, our results indicate that the ability to detect some wildlife species may be affected by the need to fly higher to minimize sound disturbance, potentially requiring higher resolution cameras than those currently used. Also, additional flight permitting may be required if modeling indicates a UAV must fly at a greater height to avoid a behavioral response by the target species. © 2016 The Wildlife Society. © The Wildlife Society, 2016},
}

@ARTICLE{Yucel20164867,
author={Yucel, M.A. and Turan, R.Y.},
title={Areal Change Detection and 3D Modeling of Mine Lakes Using High-Resolution Unmanned Aerial Vehicle Images},
journal={Arabian Journal for Science and Engineering},
year={2016},
volume={41},
number={12},
pages={4867-4878},
note={cited By 16},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84979070960&doi=10.1007%2fs13369-016-2182-7&partnerID=40&md5=144c24db49d0c008df8ffc575571030d},
abstract={This study focuses on the Etili and Comakli open-pit coal mines, where mine lakes are most densely located within the Can Coal Basin (northwestern Turkey). The aim of our study was to create 3D terrain models of these mine lakes using high-resolution images from an unmanned aerial vehicle (UAV) and to quantify areal changes linked to anthropogenic and meteorological effects over the study period. In November 2014 and October 2015, a DJI F550 hexacopter was flown at elevations of 30–100 m, and images were acquired using a 12-megapixel camera. Nineteen flights were completed, with each flight acquiring between 109 and 554 images. 3D modeling of UAV images was carried out with Agisoft software, using the most common structure from motion algorithm. Its workflow, involving image matching, georeferencing, digital elevation modeling, orthomosaics, 3D point cloud, and 3D textured model creation, was used to generate our 3D terrain model for the mine lakes. Orthomosaics with 1–6 cm/pixel resolution were used to assess areal change in the mine lakes. Area was calculated using two different methods (digitization and classification) within the ArcGIS package; results of these two methods were compared. Our UAV study of open-pit mines rapidly and precisely determined changes in topography linked to anthropogenic and meteorological effects. It also proved to be an effective method of visualizing such effects over the short term. © 2016, King Fahd University of Petroleum & Minerals.},
}

@CONFERENCE{Li20164992,
author={Li, J. and Ye, D.H. and Chung, T. and Kolsch, M. and Wachs, J. and Bouman, C.},
title={Multi-target detection and tracking from a single camera in unmanned aerial vehicles (UAVs)},
journal={IEEE International Conference on Intelligent Robots and Systems},
year={2016},
volume={2016-November},
pages={4992-4997},
art_number={7759733},
note={cited By 50},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85006371225&doi=10.1109%2fIROS.2016.7759733&partnerID=40&md5=aeac3977b5f9740c9217900180e6637d},
abstract={Despite the recent flight control regulations, Unmanned Aerial Vehicles (UAVs) are still gaining popularity in civilian and military applications, as much as for personal use. Such emerging interest is pushing the development of effective collision avoidance systems. Such systems play a critical role UAVs operations especially in a crowded airspace setting. Because of cost and weight limitations associated with UAVs payload, camera based technologies are the de-facto choice for collision avoidance navigation systems. This requires multitarget detection and tracking algorithms from a video, which can be run on board efficiently. While there has been a great deal of research on object detection and tracking from a stationary camera, few have attempted to detect and track small UAVs from a moving camera. In this paper, we present a new approach to detect and track UAVs from a single camera mounted on a different UAV. Initially, we estimate background motions via a perspective transformation model and then identify distinctive points in the background subtracted image. We find spatio-temporal traits of each moving object through optical flow matching and then classify those candidate targets based on their motion patterns compared with the background. The performance is boosted through Kalman filter tracking. This results in temporal consistency among the candidate detections. The algorithm was validated on video datasets taken from a UAV. Results show that our algorithm can effectively detect and track small UAVs with limited computing resources. © 2016 IEEE.},
}

@CONFERENCE{Sapkota20161556,
author={Sapkota, K.R. and Roelofsen, S. and Rozantsev, A. and Lepetit, V. and Gillet, D. and Fua, P. and Martinoli, A.},
title={Vision-based unmanned aerial vehicle detection and tracking for sense and avoid systems},
journal={IEEE International Conference on Intelligent Robots and Systems},
year={2016},
volume={2016-November},
pages={1556-1561},
art_number={7759252},
note={cited By 33},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85006341237&doi=10.1109%2fIROS.2016.7759252&partnerID=40&md5=9a52ca831a5d520b989bc5bbc48dd979},
abstract={We propose an approach for on-line detection of small Unmanned Aerial Vehicles (UAVs) and estimation of their relative positions and velocities in the 3D environment from a single moving camera in the context of sense and avoid systems. This problem is challenging both from a detection point of view, as there are no markers on the targets available, and from a tracking perspective, due to misdetection and false positives. Furthermore, the methods need to be computationally light, despite the complexity of computer vision algorithms, to be used on UAVs with limited payload. To address these issues we propose a multi-staged framework that incorporates fast object detection using an AdaBoost-based approach, coupled with an on-line visual-based tracking algorithm and a recent sensor fusion and state estimation method. Our framework allows for achieving real-time performance with accurate object detection and tracking without any need of markers and customized, high-performing hardware resources. © 2016 IEEE.},
}

@CONFERENCE{Witczak201615,
author={Witczak, P. and Pazera, M. and Witczak, M. and Korbicz, J. and Theilliol, D.},
title={Thrust balance estimation of an unmanned aerial vehicle: Application to fault detection},
journal={Conference on Control and Fault-Tolerant Systems, SysTol},
year={2016},
volume={2016-November},
pages={15-20},
art_number={7739722},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85001948859&doi=10.1109%2fSYSTOL.2016.7739722&partnerID=40&md5=7ab9fff58700efcc8bc54d54574dbe17},
abstract={Due to uncertain flight conditions as well as faults, an outdoor performance of any unmanned aerial vehicle is a challenging task. Indeed, owing to weather conditions it is entirely different that any laboratory tests. While small and radio controlled drones are relatively common devices, they are still unruly while wind blows. Moreover, process and actuator faults may also significantly impair the overall system performance. All of these factors are reflected by the thrust balance. Thus, the main objective of this paper is to propose a scheme that can be used for simultaneous estimation the thrust balance as well as the state under uncertain environment. The estimated information allows performing decisions about the current faulty/fault-free situation of the system. The proposed approach is based on the paradigm, which can be relatively easily implemented on the chips dedicated to popular drones, such as Arduino or raspberry pi based solutions that are widely available. © 2016 IEEE.},
}

@CONFERENCE{Manoj20162385,
author={Manoj, Ch. and Saiteja, N. and Kumar, R.A. and Priyadarsini, M.J.P. and Murugesan, K. and Inabathini, S.R.},
title={Unmanned aerial vehicle based bomb detection},
journal={2016 International Conference on Advances in Computing, Communications and Informatics, ICACCI 2016},
year={2016},
pages={2385-2389},
art_number={7732412},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85007409156&doi=10.1109%2fICACCI.2016.7732412&partnerID=40&md5=e45a35fb7fe3323990d2fa827a53db9b},
abstract={In any Bomb rescue operation, time factor plays a vital role. As Bomb can explore at any moment, Our task is to reduce the time consuming to detect the Bomb when compared to manual detection. Detecting Bomb manually is highly risky and much time consuming process. In this paper we propose a new technique using 'Quadcopter' nothing but UA V (Unmanned Aerial Vehicle). It is an air vehicle which has multiple rotors (in our paper it is 4) and is controlled by the RC transmitter (joysticks). An attempt has been made to detect the bomb by using Geiger counter module. Geiger module can detect any type of radioactive radiation emitted from the Bomb. Bomb location information is sent to the user by making use of GPS and GSM modules. We integrated Geiger module, GPS module, GSM module, Arduino-UNO as a payload to the quadcopter. We need to pass the quadcopter on the area in which the operator wants to examine and if any Bomb is present, then Geiger tube detects it Then immediately Bomb location is sent to the operator's mobile by GPS and GSM modules. The main objective of this paper is to ensure the safety of the operator and to reduce the detection process time when compared to manual detection. © 2016 IEEE.},
}

@CONFERENCE{Silano20161018,
author={Silano, G. and Iannelli, L.},
title={An educational simulation platform for GPS-denied unmanned Aerial Vehicles aimed to the detection and tracking of moving objects},
journal={2016 IEEE Conference on Control Applications, CCA 2016},
year={2016},
pages={1018-1023},
art_number={7587947},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84994361843&doi=10.1109%2fCCA.2016.7587947&partnerID=40&md5=d3021511104e5243a1f1081350f1dd81},
abstract={The main motivation of this work is to show, for educational purposes, that the visual based object tracking problem can be illustrated through the simulation-in-the-loop approach: by using the MathWorks™ Virtual Reality Toolbox together with Matlab®, it is possible to simulate the behavior of a drone in a 3D environment when detection and control algorithms are run. Matlab VR is used due to the familiarity that students have with. In this way the attention can be moved to the classifier, the references generator and the trajectory tracking control. Each block is decoupled and independent, so it can be easily replaced with others thus simplifying the development phase. © 2016 IEEE.},
}

@CONFERENCE{Aleotti2016,
author={Aleotti, J. and Micconi, G. and Caselli, S. and Benassi, G. and Zambelli, N. and Calestani, D. and Zanichelli, M. and Bettelli, M. and Zappettini, A.},
title={Unmanned aerial vehicle equipped with spectroscopic CdZnTe detector for detection and identification of radiological and nuclear material},
journal={2015 IEEE Nuclear Science Symposium and Medical Imaging Conference, NSS/MIC 2015},
year={2016},
art_number={7582264},
note={cited By 10},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84994160261&doi=10.1109%2fNSSMIC.2015.7582264&partnerID=40&md5=87bbc8a9717fed604c0c5d36b1d3ab3a},
abstract={Localization and identification of nuclear and radiological material are main issues in case of nuclear accident or terrorist attack. In these cases, the use of a unmanned aerial vehicle would be highly recommended in order to preserve the safety of the human operators. For this purpose, we have integrated a compact, light, low power operating, CZT-based gamma ray detector on a commercially available UAV. The system allows exploration of potentially dangerous areas without a close exposure of the human operator. The operator is able to provide motion commands to the UAV while receiving force feedback from a 3DOF haptic interface. Force feedback provides an attractive basin around the location of the most intense detected radiation. A field experiment has been carried out and a 192Ir nuclear source has been localized and identified exploiting the novel teleoperation system. © 2015 IEEE.},
}

@CONFERENCE{Mahjri2016,
author={Mahjri, I. and Dhraief, A. and Belghith, A.},
title={A three dimensional scalable and distributed conflict detection algorithm for unmanned aerial vehicles},
journal={IEEE Wireless Communications and Networking Conference, WCNC},
year={2016},
volume={2016-September},
art_number={7565072},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84989914717&doi=10.1109%2fWCNC.2016.7565072&partnerID=40&md5=cd90407d9e916038c9c94e2fbba1f454},
abstract={This paper deals with conflict detection for Unmanned Aerial Vehicles (UAVs). We provide an exhaustive mathematical framework for 3D conflict detection and propose a novel distributed conflict detection algorithm. The suggested algorithm requires minimal communication. Indeed, only the state information (i.e., position and velocity vectors) is periodically exchanged between the UAVs. We carry out simulations, using the OMNET++ simulator, to evaluate its performance. Simulation results indicate that the proposed algorithm performs well in terms of false alarms, missed alarms and scalability to increased number of UAVs. © 2016 IEEE.},
}

@CONFERENCE{Inata2016,
author={Inata, H. and Say, S. and Ando, T. and Liu, J. and Shimamoto, S.},
title={Unmanned aerial vehicle based missing people detection system employing phased array antenna},
journal={IEEE Wireless Communications and Networking Conference, WCNC},
year={2016},
volume={2016-September},
art_number={7564674},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84989880957&doi=10.1109%2fWCNC.2016.7564674&partnerID=40&md5=3cf832058751068b1672f5f41b278204},
abstract={In this paper, we propose a system for detection of the missing people employing UAV which is able to move quickly and has a wide view from the air in the disaster area. However, an airplane type UAV does not always have a stable flight due to strong wind, rolling, and pitching. In order to detect and to respond the missing people promptly using the UAV, we propose the system which uses a phased array antenna and an angle detector. To implement the system, we assemble the phased array antenna and carry out an experiment to measure the characteristics of directivity, the directivity control characteristics, the return loss of the antenna, and the received power level to compare using and not using the phased array antenna in terms of efficiency and functionality. The experiment results show that the proposed system increase the received power level by adjusting the directivity of the antennas with short delay time. The results also confirm that the proposed system is practical in decreasing victims of disasters. © 2016 IEEE.},
}

@ARTICLE{Xue20161193,
author={Xue, T. and Zhong, M.-Y. and Li, G.},
title={Wavelet transform and parity space based actuator fault detection for unmanned aerial vehicle},
journal={Kongzhi Lilun Yu Yingyong/Control Theory and Applications},
year={2016},
volume={33},
number={9},
pages={1193-1199},
note={cited By 7},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85012248800&doi=10.7641%2fCTA.2016.60034&partnerID=40&md5=52039e8b474b1ad8619cf6677d6e4096},
abstract={The parity space based fault detection (FD) is one of the most common approaches by using the system input and output data over a time window and attracts considerable attention in practical applications. This approach is characterized by its straight forward manner in design and the generated residual is independent of the system initial state and input. However, high parity order has to make sure for improving the FD performance, which may lead to heavy computational task and very narrow frequency range of fault to be detected. To overcome this, the paper proposes to deal with the problem of actuator FD for unmanned aerial vehicle (UAV) by applying parity space approach and wavelet transform. Then the residual can be generated based on the parity relation between the inputs and outputs such that a ratio criterion of robustness to unknown input and sensitivity to fault is minimized. Moreover, with the selection of wavelet basis and residual evaluation for a group of residuals, the faults within broader frequency range can be detected. As a result, the parity space order can be efficiently reduced for some acceptable FD performance, hence, both the computational cost of residual evaluation function and the frequency range of fault can be improved. Finally, an example of UAV longitudinal system is used to demonstrate the effectiveness of the proposed method. © 2016, Editorial Department of Control Theory & Applications South China University of Technology. All right reserved.},
}

@ARTICLE{Fytsilis2016165,
author={Fytsilis, A.L. and Prokos, A. and Koutroumbas, K.D. and Michail, D. and Kontoes, C.C.},
title={A methodology for near real-time change detection between Unmanned Aerial Vehicle and wide area satellite images},
journal={ISPRS Journal of Photogrammetry and Remote Sensing},
year={2016},
volume={119},
pages={165-186},
note={cited By 17},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84974785101&doi=10.1016%2fj.isprsjprs.2016.06.001&partnerID=40&md5=e909a7be7000ed6b0627e14e253f3f64},
abstract={In this paper a novel integrated hybrid methodology for unsupervised change detection between Unmanned Aerial Vehicle (UAV) and satellite images, which can be utilized in various fields like security applications (e.g. border surveillance) and damage assessment, is proposed. This is a challenging problem mainly due to the difference in geographic coverage and the spatial resolution of the two images, as well as to the acquisition modes which lead to misregistration errors. The methodology consists of the following steps: (a) pre-processing, where the part of the satellite image that corresponds to the UAV image is determined and the UAV image is ortho-rectified using information provided by a Digital Terrain Model, (b) the detection of potential changes, which is based exclusively on intensity and image gradient information, (c) the generation of the region map, where homogeneous regions are produced by the previous potential changes via a seeded region growing algorithm and placed on the region map, and (d) the evaluation of the above regions, in order to characterize them as true changes or not. The methodology has been applied on demanding real datasets with very encouraging results. Finally, its robustness to the misregistration errors is assessed via extensive experimentation. © 2016 International Society for Photogrammetry and Remote Sensing, Inc. (ISPRS).},
}

@CONFERENCE{Inata2016222,
author={Inata, H. and Say, S. and Ando, T. and Liu, J. and Shimamoto, S.},
title={Unmanned aerial vehicle based missing people detection system employing phased array antenna},
journal={2016 IEEE Wireless Communications and Networking Conference Workshops, WCNCW 2016},
year={2016},
pages={222-227},
art_number={7552703},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84987941438&doi=10.1109%2fWCNCW.2016.7552703&partnerID=40&md5=33880d2731f3c7b57ede3bc6f80e258f},
abstract={In this paper, we propose a system for detection of the missing people employing UAV which is able to move quickly and has a wide view from the air in the disaster area. However, an airplane type UAV does not always have a stable flight due to strong wind, rolling, and pitching. In order to detect and to respond the missing people promptly using the UAV, we propose the system which uses a phased array antenna and an angle detector. To implement the system, we assemble the phased array antenna and carry out an experiment to measure the characteristics of directivity, the directivity control characteristics, the return loss of the antenna, and the received power level to compare using and not using the phased array antenna in terms of efficiency and functionality. The experiment results show that the proposed system increase the received power level by adjusting the directivity of the antennas with short delay time. The results also confirm that the proposed system is practical in decreasing victims of disasters. © 2016 IEEE.},
}

@CONFERENCE{Al-Kaff201692,
author={Al-Kaff, A. and Meng, Q. and Martin, D. and De La Escalera, A. and Armingol, J.M.},
title={Monocular vision-based obstacle detection/avoidance for unmanned aerial vehicles},
journal={IEEE Intelligent Vehicles Symposium, Proceedings},
year={2016},
volume={2016-August},
pages={92-97},
art_number={7535370},
note={cited By 31},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84983372764&doi=10.1109%2fIVS.2016.7535370&partnerID=40&md5=21cacb2888b7ff42ca489fe154a4f9dd},
abstract={Robust real-time obstacle detection/avoidance is a challenging problem especially for micro and small aerial vehicles due to the limited number of the on-board sensors due to the battery constraint and low payload. Usually lightweight sensors such as CMOS camera are the best choice comparing with laser or radar sensors. For real-time applications, most studies focus on using stereo cameras to reconstruct a 3D model of the obstacles or to estimate their depth. Instead, in this paper, a method that mimics the human behavior of detecting the state of the approaching obstacles using single camera is proposed. During the flight, this method is able to detect the changes of the size area of the obstacles. First, the method detects the feature points of the obstacles, and then extracts the obstacles that has probability of getting close. In addition, by comparing the changes in the area ratios of the obstacle in the image sequence, the method can decide if it is obstacle or not. Finally, by estimating the obstacle 2D position in the image and combining with the tracked waypoints, the UAV can take the action of avoidance. © 2016 IEEE.},
}

@CONFERENCE{Aydin20162125,
author={Aydin, M. and Kugu, E.},
title={Safe landing site detection using SRTM data for the Unmanned Aerial Vehicles [Insansiz Hava Araçlari için Srtm Verisi Kullanilarak Uygun Inis Alaninin Tespit Edilmesi]},
journal={2016 24th Signal Processing and Communication Application Conference, SIU 2016 - Proceedings},
year={2016},
pages={2125-2128},
art_number={7496192},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84982792284&doi=10.1109%2fSIU.2016.7496192&partnerID=40&md5=bad27d816fa8967e9a1eaecb85b38980},
abstract={In this work, it is aimed to determine the suitable landing zones for the Unmanned Aerial Vehicles (UAVs) in case of an emergency during their missions. SRTM (Shuttle Radar Topography Mission) maps were used to reach that aim. Nowadays, it is observed that the UAVs are being used densely for both military and civilian purposes. So, it is inevitable to make the UAVs smarter and make them more autonomous to minimize their dependence on a person. UAVs can have unexpected problems during their missions such as motor fault, communication cut etc. In this situation, a UAV should activate the emergency landing systems and realize the landing safely. Image segmentation and blob analysis are used to determine the possible landing zones on the SRTM data. In this proposed system, the landing of a UAV to unwanted zones is limited and the UAV is guidance to the predetermined safe zones. © 2016 IEEE.},
}

@ARTICLE{Seo2016,
author={Seo, C.-J.},
title={Vehicle detection using images taken by low-altitude Unmanned Aerial Vehicles (UAVs)},
journal={Indian Journal of Science and Technology},
year={2016},
volume={9},
number={24},
art_number={96057},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85010916091&doi=10.17485%2fijst%2f2016%2fv9i24%2f96057&partnerID=40&md5=0c6da3b230177017868d51a30a222a78},
abstract={Background/Objectives: This paper discusses the detection of vehicles in a dense area using low-altitude aerial images produced by unmanned aerial vehicles (UAVs). Vehicles in a dense area are difficult to detect accurately in images because of the narrow distance between parked vehicles. Methods/Statistical Analysis: This paper proposes a method that detects vehicles by applying a Histogram of Oriented Gradients (HOG) feature-extraction method to obtain information about vehicles found in images. Images used in the experiment were shot using a Phantom 3 Professional UAV developed by DJI Corp. Findings: Aerial images can be collected to measure traffic via a variety of methods. In recent years, studies on traffic volume using UAVs have been actively conducted. Until now, satellites, aircrafts, and helicopters have been used to obtain aerial images; however, the cost of such images is high, and these methods cannot respond to changes over time and weather in real time. As UAV technology has advanced in recent years, the methods of obtaining cost-effective and ultrahigh definition (UHD) aerial images have become available. The experimental results show the proposed approach can be used to detect vehicles that are densely packed in an area more effectively than the method using the conventional histogram of oriented gradients (HOG), which employs information about the brightness of images. Application/Improvements: In this paper, the detection of vehicles found in a densely packed area is performed using the HOG, which exhibits good adaptability to environmental changes.},
}

@ARTICLE{Yang2016,
author={Yang, J. and Yin, D. and Niu, Y. and Zhu, L.},
title={Cooperative conflict detection and resolution of civil unmanned aerial vehicles in metropolis},
journal={Advances in Mechanical Engineering},
year={2016},
volume={8},
number={6},
note={cited By 8},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84977139213&doi=10.1177%2f1687814016651195&partnerID=40&md5=42c08610b87bac78058a1f6737afd465},
abstract={Unmanned air vehicles have recently attracted attention of many researchers because of their potential civil applications. A systematic integration of unmanned air vehicles in non-segregated airspace is required that allows safe operation of unmanned air vehicles along with other manned aircrafts. One of the critical issues is conflict detection and resolution. This article proposes to solve unmanned air vehicles' conflict detection and resolution problem in metropolis airspace. First, the structure of metropolis airspace in the coming future is studied, and the airspace conflict problem between different unmanned air vehicles is analyzed by velocity obstacle theory. Second, a conflict detection and resolution framework in metropolis is proposed, and factors that have influences on conflict-free solutions are discussed. Third, the multi-unmanned air vehicle conflict resolution problem is formalized as a nonlinear optimization problem with the aim of minimizing overall conflict resolution consumption. The safe separation constraint is further discussed to improve the computation efficiency. When the speeds of conflict-involved unmanned air vehicles are equal, the nonlinear safe separation constraint is transformed into linear constraints. The problem is solved by mixed integer convex programming. When unmanned air vehicles are with unequal speeds, we propose to solve the nonlinear optimization problem by stochastic parallel gradient descent-based method. Our approaches are demonstrated in computational examples. © The Author(s) 2016.},
}

@ARTICLE{Rossi2016765,
author={Rossi, M. and Brunelli, D.},
title={Autonomous gas detection and mapping with unmanned aerial vehicles},
journal={IEEE Transactions on Instrumentation and Measurement},
year={2016},
volume={65},
number={4},
pages={765-775},
art_number={7369958},
note={cited By 84},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84953274223&doi=10.1109%2fTIM.2015.2506319&partnerID=40&md5=a6eeb15875bb16071117e60c836a10a1},
abstract={Unmanned aerial vehicles (UAVs) are nowadays largely employed in civil applications. One of the most promising applications is the environmental monitoring (or risk assessment). We propose a battery-powered eNose board that can be embedded with any type of drone. We evaluated the effectiveness of the sensing method by means of field experiments using the prototype as payload of a hexacopter. The results show that the analysis of the target environmental parameters is not perturbed by the air flow generated by propellers. The system is suitable for any type of mobile carrier (UAVs or wheeled robots), thanks to its lightweight and compact form factor. To further extend the limited flight autonomy of the carrier, we developed an optimal monitoring algorithm for gas leakage localization, a simulating framework to evaluate its performance, and we provide a design space exploration for solar-powered drones. © 1963-2012 IEEE.},
}

@ARTICLE{Ma2016,
author={Ma, Y. and Wu, X. and Yu, G. and Xu, Y. and Wang, Y.},
title={Pedestrian detection and tracking from low-resolution unmanned aerial vehicle thermal imagery},
journal={Sensors (Switzerland)},
year={2016},
volume={16},
number={4},
art_number={446},
note={cited By 68},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84961908104&doi=10.3390%2fs16040446&partnerID=40&md5=1725ec31943d29bd4e7a2b3e14ab35d5},
abstract={Driven by the prominent thermal signature of humans and following the growing availability of unmanned aerial vehicles (UAVs), more and more research efforts have been focusing on the detection and tracking of pedestrians using thermal infrared images recorded from UAVs. However, pedestrian detection and tracking from the thermal images obtained from UAVs pose many challenges due to the low-resolution of imagery, platform motion, image instability and the relatively small size of the objects. This research tackles these challenges by proposing a pedestrian detection and tracking system. A two-stage blob-based approach is first developed for pedestrian detection. This approach first extracts pedestrian blobs using the regional gradient feature and geometric constraints filtering and then classifies the detected blobs by using a linear Support Vector Machine (SVM) with a hybrid descriptor, which sophisticatedly combines Histogram of Oriented Gradient (HOG) and Discrete Cosine Transform (DCT) features in order to achieve accurate detection. This research further proposes an approach for pedestrian tracking. This approach employs the feature tracker with the update of detected pedestrian location to track pedestrian objects from the registered videos and extracts the motion trajectory data. The proposed detection and tracking approaches have been evaluated by multiple different datasets, and the results illustrate the effectiveness of the proposed methods. This research is expected to significantly benefit many transportation applications, such as the multimodal traffic performance measure, pedestrian behavior study and pedestrian-vehicle crash analysis. Future work will focus on using fused thermal and visual images to further improve the detection efficiency and effectiveness. © 2016 by the authors; licensee MDPI, Basel, Switzerland.},
}

@BOOK{Molina201681,
author={Molina, R.P. and Caballero, E.M.M. and Bravo, J.J.V. and Pino Serrato, I. and Rosa Carpintero Salvo, I. and Ruiz, L.G. and Manzano, G.M. and De Azcárate, F.G. and Clavero, F.C. and Madueño, J.M.M.},
title={Optical search by unmanned aerial vehicles: Fauna detection case study},
journal={Operations Research for Unmanned Systems},
year={2016},
pages={81-94},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85104370451&doi=10.1002%2f9781118918937.ch5&partnerID=40&md5=651ece1507a8063f1f62965481f4875c},
abstract={Many Mediterranean forests are still used for traditional hunting. To manage use of public lands for hunting and to regulate the hunting capacity within these territories, decision makers require accurate information about game populations, the conservation status of the forests, and conditions of environmental development. This chapter discusses the use of unmanned vehicles for sensing tasks and describes the approaches and considerations for effective search using census taking as an example. It explores the technological solutions to what historically were tasks conducted by humans, namely identification of a field of view, in situ flight planning to prevent gaps in coverage, and methods to ensure consistency throughout a task. Search planning for Unmanned Aerial Vehicles (UAV) operations occurs in four distinct phases: Preliminary Analysis, Flight Geometry Control, Image Preparation, and the Analysis and Identification of Individuals. UAVs can be considered as good platforms for the observation and estimation of gaming populations. © 2016 John Wiley & Sons Ltd.},
}

@CONFERENCE{Montanari2016253,
author={Montanari, R. and Tozadore, D.C. and Fraccaroli, E.S. and Romero, R.A.F.},
title={Ground Vehicle Detection and Classification by an Unmanned Aerial Vehicle},
journal={Proceedings - 12th LARS Latin American Robotics Symposium and 3rd SBR Brazilian Robotics Symposium, LARS-SBR 2015 - Part of the Robotics Conferences 2015},
year={2016},
pages={253-257},
art_number={7402174},
note={cited By 7},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84964334094&doi=10.1109%2fLARS-SBR.2015.64&partnerID=40&md5=02024c6ed3d14ed24fe5f0723349f475},
abstract={Rotary-wing unmanned aerial vehicles (UAV) are being widely used in different applications due to its several features, such as mobility, lightweight, embedded processing and capability of flying in different height levels. Among the possible applications they are used in surveillance tasks, agriculture environments monitoring, power lines inspections and diseases detection in crops. The images captured by the UAVs need to be examined in most of the applications. This analysis is usually done by experts, but a system that process the captured images in a autonomous way can speed up the results and more images can be processed in a lesser period, which is the ideal for real time applications. This work presents a system for vehicle detection aiming at surveillance task. The system is evaluated in terms of precision of detection of a particular type of vehicle. The video was shot using a monocular camera coupled with an aerial robot developed in our Lab. The experimental results demonstrate that the proposed system can be used for the vehicles tracking task under controlled conditions. © 2015 IEEE.},
}

@CONFERENCE{Pinkerman2016,
author={Pinkerman, C.W. and O’Connell, T.J. and Arena, A.S.},
title={Comparisons between avian and unmanned aerial vehicle approach to thermal updraft detection},
journal={AIAA Atmospheric Flight Mechanics Conference},
year={2016},
page_count={23},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85087239318&doi=10.2514%2f6.2016-1288&partnerID=40&md5=b7339324bb45265b5418a95c5576d08a},
abstract={Thermal updrafts can be utilized to increase an aircraft’s flight endurance and range. However, much of the discussion involving thermal updrafts comprise of flight techniques within a known thermal updraft and very little is discussed over the detection of thermals without the influence of the upward or downward velocity component. This paper discusses possible thermal locating methods discovered from looking at thermal detection primarily from an avian viewpoint. An avian study was conducted to gather information on how avian soaring species locate thermal updrafts, in which no definitive answer was found. Of the possible theories of avian thermal location methods, a single method was chosen for further study through experimentation to construct possible applications to unmanned aerial systems. By quantifying shifts in the local wind vector, the direction of local thermal updrafts was theorized to be able to be calculated. Due to uncertainty in experimental approach, this method is shown to be unfavorable for use in detecting thermal updrafts. © 2016, American Institute of Aeronautics and Astronautics Inc, AIAA. All rights reserved.},
}

@ARTICLE{Harvey201683,
author={Harvey, B. and O’young, S.},
title={Detection of continuous ground-based acoustic sources via unmanned aerial vehicles},
journal={Journal of Unmanned Vehicle Systems},
year={2016},
volume={4},
number={2},
pages={83-95},
note={cited By 6},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85073008993&doi=10.1139%2fjuvs-2015-0029&partnerID=40&md5=cc9eb64f8c834e5317ac40c1d630162a},
abstract={This paper presents the results of experiments that were conducted to partially establish the viability of utilizing acoustic sensing as a sense-and-avoid system for unmanned aerial vehicles (UAV). Experiments were conducted in which a UAV fitted with four acoustic sensors was flown under autopilot control at various altitudes over a loud speaker located on the ground acting as a continuous acoustic source. Various physical and digital noise reduction techniques were employed to enhance the recorded signals to allow increased detection ranges. Using standard free-field acoustic attenuation laws, maximum expected detection distances were calculated and presented. Depending on the acoustic source frequency signature and filtering method used, maximum expected detection distances ranged anywhere from 0.45 to 4.21 km on average with signal-to-noise ratios ranging from 10.3 to 37.0. Based on the results obtained, it is expected that acoustic techniques could facilitate the detection of an airborne source (aircraft) at distances great enough to facilitate an avoidance maneuver. © Canadian Science Publishing. All rights reserved.},
}

@ARTICLE{Jean2016196,
author={Jean, J.-H. and Liu, B.-S. and Chang, P.-Z. and Kuo, L.-C.},
title={Attitude detection and localization for unmanned aerial vehicles},
journal={Smart Science},
year={2016},
volume={4},
number={4},
pages={196-202},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85045522185&doi=10.1080%2f23080477.2016.1234426&partnerID=40&md5=01ae2300ee931fe9a2fcc76d4480c25e},
abstract={Over the past decade, unmanned aerial vehicles (UAV) have been developed rapidly for more and more applications among civilian uses such as reconnaissance, earth sensing, and scientific data collection. For achieving those applications, the UAVs have to be equipped with an accurate attitude detection and localization module to maintain a stable attitude and a correct heading direction during flight. This paper reports the implementation of an attitude detection and localization module for UAVs by integrating sensing data from the GPS sensor, inertial measurement unit (IMU), and digital compass. The module is realized based on the Arduino platform to compute the fused attitude and localization information and send the fused data to the ground station computer in real time. To avoid the data drift problem of the GPS sensor, the zero velocity updated algorithm is used to detect the zero motion of the vehicle from IMU measurements for deciding whether to update the localization information. © 2016 The Author(s).},
}

@CONFERENCE{Hommes2016,
author={Hommes, A. and Shoykhetbrod, A. and Noetel, D. and Stanko, S. and Laurenzis, M. and Hengy, S. and Christnacher, F.},
title={Detection of acoustic, electro-optical and RADAR signatures of small unmanned aerial vehicles},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2016},
volume={9997},
art_number={999701},
note={cited By 22},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85011097273&doi=10.1117%2f12.2242180&partnerID=40&md5=24d7bfde2994bbeeba2bf7f4bd5616d1},
abstract={We investigated signatures of small unmanned aerial vehicles (UAV) with different sensor technologies ranging from acoustical antennas, passive and active optical imaging devices to small-size FMCW RADAR systems. These sensor technologies have different advantages and drawbacks and can be applied in a complementary sensor network to benefit from their different strengths. © 2016 SPIE.},
}

@CONFERENCE{Ortiz-Torres2016272,
author={Ortiz-Torres, G. and López-Estrada, F.R. and Reyes-Reyes, J. and García-Beltrán, C.D. and Theilliol, D.},
title={An Actuator Fault Detection and Isolation method design for Planar Vertical Take-off and Landing Unmanned Aerial Vehicle modelled as a qLPV system},
journal={IFAC-PapersOnLine},
year={2016},
volume={49},
number={5},
pages={272-277},
note={cited By 12},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84991087306&doi=10.1016%2fj.ifacol.2016.07.125&partnerID=40&md5=f6d0fe107a4d971690642a73ddf96bfe},
abstract={This paper presents the design of a tracking controller and a fault detection and isolation system for a Planar Vertical Take-off and Landing (PVTOL) Unmanned Aerial Vehicle (UAV) under actuator faults. In order to control the PVTOL, the dynamic system is divided into three subsystems driven by the rotational, the altitude, and the position dynamics. The altitude and position subsystems are based on qLPV model while the rotational subsystem is linear. A linear observer applied to the rotational subsystem is considered to detect actuator faults, which can occur as failures (loss of a propeller or a motor) or partial faults (degradation). Furthermore, fault isolation is done by measuring roll velocity due to the actuator fault. In all cases, sufficient conditions for the existence of the observer and the controllers are given in terms of linear matrix inequalities (LMIs). Finally, simulations (on the nonlinear model) are done in order to illustrate the effectiveness of the proposed methodology. © 2016},
}

@ARTICLE{Tang2016,
author={Tang, J.W. and Shaikh-Husin, N. and Sheikh, U.U. and Marsono, M.N.},
title={FPGA-Based Real-Time Moving Target Detection System for Unmanned Aerial Vehicle Application},
journal={International Journal of Reconfigurable Computing},
year={2016},
volume={2016},
art_number={8457908},
note={cited By 15},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84965106309&doi=10.1155%2f2016%2f8457908&partnerID=40&md5=1845f7ce7de4e03e59fc4c8ab62884de},
abstract={Moving target detection is the most common task for Unmanned Aerial Vehicle (UAV) to find and track object of interest from a bird's eye view in mobile aerial surveillance for civilian applications such as search and rescue operation. The complex detection algorithm can be implemented in a real-time embedded system using Field Programmable Gate Array (FPGA). This paper presents the development of real-time moving target detection System-on-Chip (SoC) using FPGA for deployment on a UAV. The detection algorithm utilizes area-based image registration technique which includes motion estimation and object segmentation processes. The moving target detection system has been prototyped on a low-cost Terasic DE2-115 board mounted with TRDB-D5M camera. The system consists of Nios II processor and stream-oriented dedicated hardware accelerators running at 100 MHz clock rate, achieving 30-frame per second processing speed for 640 × 480 pixels' resolution greyscale videos. © 2016 Jia Wei Tang et al.},
}

@ARTICLE{Bold2016361,
author={Bold, S. and Sosorbaram, B. and Lee, S.R.},
title={Implementation of autonomous unmanned aerial vehicle with moving-object detection and face recognition},
journal={Lecture Notes in Electrical Engineering},
year={2016},
volume={376},
pages={361-370},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84959178977&doi=10.1007%2f978-981-10-0557-2_36&partnerID=40&md5=1deb1a394ac2e7787da826c91d345b14},
abstract={Various personal robots have developed for performing useful tasks autonomously without the human interaction. The development of human navigation and tracking in the real time environment will lead to the implementation of more advanced tasks that can performed by the autonomous robots. This project proposes a system that can track objects using Speeded Up Robust Feature (SURF) detection and human face recognition using Eigenface recognizer. In this paper, combinations of algorithms such as modified Eigenface, Haar-Cascade classifier and SURF resulted in a more robust system for object detection and face recognition. The proposed system was implemented on AR drone 2.0 using the Microsoft Visual Studio 2010 platform together with OpenCV. The testing of the proposed system carried out in an indoor environment in order to evaluate its performance in terms of detection distance, angle of detection, and accuracy of detection. 132 images of different people were used for face recognition at four different detection distances. The best average result of 92.22% was obtained at a detection distance of 50cm to 75cm. It noted that the detection accuracy decreases as the detection distance is increased. Furthermore, improve various limitations, strengths of the AR drone and the proposed algorithm. © Springer Science+Business Media Singapore 2016.},
}

@CONFERENCE{Seron201587,
author={Seron, M.M. and Johansen, T.A. and De Doná, J.A. and Cristofaro, A.},
title={Detection and estimation of icing in unmanned aerial vehicles using a bank of unknown input observers},
journal={2015 Australian Control Conference, AUCC 2015},
year={2015},
pages={87-92},
art_number={7361911},
note={cited By 9},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84964018535&partnerID=40&md5=94a0e32dabbd65abfd7aef4aea90bbaa},
abstract={Icing is regarded as a severe structural alteration affecting unmanned aerial vehicles (UAVs), since ice accretion on wings and control surfaces modifies the aircraft shape resulting in altered controllability and performance of the vehicle. We study the problem of detection of icing and estimation of its 'severity' factor in longitudinal control of UAVs. We propose to employ a bank of unknown input observers (UlOs), each designed to match a model of the aircraft under a particular level of icing taken from a quantisation of the icing's severity factor range of variation. The UIO design exploits the change in equilibrium conditions, caused by the icing effect, to identify a direction in the observer estimation error space that allows for aircraft icing detection and estimation. By selecting at each time the observer from the bank that yields the smallest value of a suitable residual signal, the icing severity factor can be estimated with an accuracy that is inversely proportional to the size of the quantisation level. © 2015 Engineers Australia.},
}

@ARTICLE{Pérez-Ortiz2015533,
author={Pérez-Ortiz, M. and Peña, J.M. and Gutiérrez, P.A. and Torres-Sánchez, J. and Hervás-Martínez, C. and López-Granados, F.},
title={A semi-supervised system for weed mapping in sunflower crops using unmanned aerial vehicles and a crop row detection method},
journal={Applied Soft Computing Journal},
year={2015},
volume={37},
pages={533-544},
art_number={3151},
note={cited By 92},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84941766152&doi=10.1016%2fj.asoc.2015.08.027&partnerID=40&md5=a192dda1e5d932862aa8757bc7d4220c},
abstract={This paper presents a system for weed mapping, using imagery provided by unmanned aerial vehicles (UAVs). Weed control in precision agriculture is based on the design of site-specific control treatments according to weed coverage. A key component is precise and timely weed maps, and one of the crucial steps is weed monitoring, by ground sampling or remote detection. Traditional remote platforms, such as piloted planes and satellites, are not suitable for early weed mapping, given their low spatial and temporal resolutions. Nonetheless, the ultra-high spatial resolution provided by UAVs can be an efficient alternative. The proposed method for weed mapping partitions the image and complements the spectral information with other sources of information. Apart from the well-known vegetation indexes, which are commonly used in precision agriculture, a method for crop row detection is proposed. Given that crops are always organised in rows, this kind of information simplifies the separation between weeds and crops. Finally, the system incorporates classification techniques for the characterisation of pixels as crop, soil and weed. Different machine learning paradigms are compared to identify the best performing strategies, including unsupervised, semi-supervised and supervised techniques. The experiments study the effect of the flight altitude and the sensor used. Our results show that an excellent performance is obtained using very few labelled data complemented with unlabelled data (semi-supervised approach), which motivates the use of weed maps to design site-specific weed control strategies just when farmers implement the early post-emergence weed control. © 2015 Elsevier B.V.},
}

@CONFERENCE{Cristofaro20151651,
author={Cristofaro, A. and Johansen, T.A. and Aguiar, A.P.},
title={Icing detection and identification for unmanned aerial vehicles: Multiple model adaptive estimation},
journal={2015 European Control Conference, ECC 2015},
year={2015},
pages={1651-1656},
art_number={7330774},
note={cited By 23},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84963877928&doi=10.1109%2fECC.2015.7330774&partnerID=40&md5=9a8fbeae26b0e3285d8652581256b8bf},
abstract={The accretion of ice layers on wings and control surfaces modifies the shape of the aircraft and, consequently, alters performance and controllability of the vehicle. In this paper we propose a multiple model adaptive estimation framework to detect icing affecting unmanned aerial vehicles using the following sensors: pitot tube (airspeed sensor), GPS and IMU. A case-study is provided as support and validation of theoretical results. © 2015 EUCA.},
}

@CONFERENCE{Rotondo2015984,
author={Rotondo, D. and Cristofaro, A. and Johansen, T.A. and Nejjari, F. and Puig, V.},
title={Icing detection in unmanned aerial vehicles with longitudinal motion using an LPV unknown input observer},
journal={2015 IEEE Conference on Control and Applications, CCA 2015 - Proceedings},
year={2015},
pages={984-989},
art_number={7320740},
note={cited By 16},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84964334628&doi=10.1109%2fCCA.2015.7320740&partnerID=40&md5=d3a66d73e697ad236d74f017aaf17433},
abstract={This paper proposes a linear parameter varying (LPV) unknown input observer for the diagnosis of actuator faults and icing in unmanned aerial vehicles (UAVs). The accretion of ice layers on wings and control surfaces modifies the shape of the aircraft and alters the performance and controllability of the vehicles. The correct detection of this phenomenon is of paramount importance for the efficient implementation of de-icing techniques. The advantage of deriving the unknown input observer within the LPV framework is the possibility to deal with the nonlinearities of the UAV model by embedding them within some varying parameters. Results obtained with a Zagi Flying Wing simulator are used to validate the effectiveness of the proposed approach. © 2015 IEEE.},
}

@ARTICLE{Zhang20151561,
author={Zhang, Y.-Z. and Liu, G.-X. and Li, S. and Huang, N.-N.},
title={Autonomous detection and tracking of multiple maneuvering targets for unmanned aerial vehicles},
journal={Kongzhi Lilun Yu Yingyong/Control Theory and Applications},
year={2015},
volume={32},
number={11},
pages={1561-1566},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84958650369&doi=10.7641%2fCTA.2015.50450&partnerID=40&md5=771382742456882531b243ba58fe46a8},
abstract={The interested targets in UAV (unmanned aerial vehicles) aerial image sequences are always small in size, and have significant changes in appearance when coupled with a lot of background noises, making the target detection and tracking a very difficult task. To solve these problems, this paper presents a method to autonomously detect and track multiple maneuvering targets in UAV aerial image sequences. Firstly, image features of the targets are extracted and classified through cascade classification algorithms to obtain the strong classifier of the targets; then, the targets can be autonomously detected by using the classifier. The detection results are associated and filtered through global optimal association algorithms to achieve the purpose of tracking and recognition of multiple maneuvering targets. The optimal association-cost matrix is simultaneously fused with distance and direction information which can improve the tracking robustness. Using the ground tanks in UAV aerial image sequences as the interested targets, the experimental results showed that the proposed method can autonomous detect and track multiple maneuvering targets with desired tracking robustness. © 2015, Editorial Department of Control Theory & Applications. All right reserved.},
}

@ARTICLE{Aldea2015,
author={Aldea, E. and Le Hégarat-Mascle, S.},
title={Robust crack detection for unmanned aerial vehicles inspection in an a-contrario decision framework},
journal={Journal of Electronic Imaging},
year={2015},
volume={24},
number={6},
art_number={061119},
note={cited By 24},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84954306663&doi=10.1117%2f1.JEI.24.6.061119&partnerID=40&md5=d07605ac5569c630e6ce34abcbc6c498},
abstract={We are interested in the performance of currently available algorithms for the detection of cracks in the specific context of aerial inspection, which is characterized by image quality degradation. We focus on two widely used families of algorithms based on minimal cost path analysis and on image percolation, and we highlight their limitations in this context. Furthermore, we propose an improved strategy based on a-contrario modeling which is able to withstand significant motion blur due to the absence of various thresholds which are usually required in order to cope with varying crack appearances and with varying levels of degradation. The experiments are performed on real image datasets to which we applied complex blur, and the results show that the proposed strategy is effective, while other methods which perform well on good quality data experience significant difficulties with degraded images. © 2015 SPIE and IS&T.},
}

@CONFERENCE{Branco2015,
author={Branco, L.H.C. and Segantine, P.C.L.},
title={MaNIAC-UAV - A methodology for automatic pavement defects detection using images obtained by Unmanned Aerial Vehicles},
journal={Journal of Physics: Conference Series},
year={2015},
volume={633},
number={1},
art_number={012122},
note={cited By 8},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84983456027&doi=10.1088%2f1742-6596%2f633%2f1%2f012122&partnerID=40&md5=f05d093786ac148b87db55ddc08c7fd6},
abstract={Intelligent Transportation Systems - ITS is a set of integrated technologies (Remote Sensing, Image Processing, Communications Systems and others) that aim to offer services and advanced traffic management for the several transportation modes (road, air and rail). Collect data on the characteristics and conditions of the road surface and keep them update is an important and difficult task that needs to be currently managed in order to reduce accidents and vehicle maintenance costs. Nowadays several roads and highways are paved, but usually there is insufficient updated data about current condition and status. There are different types of pavement defects on the roads and to keep them in good condition they should be constantly monitored and maintained according to pavement management strategy. This paper presents a methodology to obtain, automatically, information about the conditions of the highway asphalt pavement. Data collection was done through remote sensing using an UAV (Unmanned Aerial Vehicle) and the image processing and pattern recognition techniques through Geographic Information System.},
}

@CONFERENCE{Cristofaro2015207,
author={Cristofaro, A. and Johansen, T.A.},
title={An unknown input observer approach to icing detection for unmanned aerial vehicles with linearized longitudinal motion},
journal={Proceedings of the American Control Conference},
year={2015},
volume={2015-July},
pages={207-213},
art_number={7170736},
note={cited By 9},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84940906068&doi=10.1109%2fACC.2015.7170736&partnerID=40&md5=b961d7b0377df15fab0049928d1fd683},
abstract={The accretion of ice layers on wings and control surfaces modifies the shape of the aircraft and, consequently, alters performance and controllability of the vehicle. In this paper we propose an Unknown Input Observers framework to design icing diagnosis filters. A case-study is provided as support and validation of theoretical results. © 2015 American Automatic Control Council.},
}

@ARTICLE{Liu2015884,
author={Liu, X.-D. and Zhong, M.-Y. and Liu, H.},
title={EKF-based fault detection of unmanned aerial vehicle flight control system},
journal={Shanghai Jiaotong Daxue Xuebao/Journal of Shanghai Jiaotong University},
year={2015},
volume={49},
number={6},
pages={884-888},
note={cited By 9},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84938402791&doi=10.16183%2fj.cnki.jsjtu.2015.06.024&partnerID=40&md5=c6960c8b65b0790aeb29f7aad4f1b34a},
abstract={The unmanned aerial vehicle (UAV) flight control system is a typical multi-sensor closed-loop system. Since actuator faults and sensor faults could seriously affect the security and reliability of the system, fault detection of the UAV flight control system is of great significance. This paper deals with the problem of fault detection of the closed-loop nonlinear model of the UAV flight control system. The nonlinear model of longitudinal motion of the UAV in the presence of wind disturbance was introduced. The extended Kalman filter (EKF) was utilized for the residual generation. The Chi-square test was selected for the residual evaluation and the fault detection task for UAV closed-loop system was accomplished. Finally, based on the simulink platform of a certain type of UAV, simulation results are provided to illustrate the effectiveness of the approach proposed in the case of pitut fault and elevator fault. ©, 2015, Shanghai Jiao Tong University. All right reserved.},
}

@ARTICLE{Yuan2015783,
author={Yuan, C. and Zhang, Y. and Liu, Z.},
title={A survey on technologies for automatic forest fire monitoring, detection, and fighting using unmanned aerial vehicles and remote sensing techniques},
journal={Canadian Journal of Forest Research},
year={2015},
volume={45},
number={7},
pages={783-792},
note={cited By 299},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84933518794&doi=10.1139%2fcjfr-2014-0347&partnerID=40&md5=64cdeb8206602e8010a7d8fd7406de0b},
abstract={Because of their rapid maneuverability, extended operational range, and improved personnel safety, unmanned aerial vehicles (UAVs) with vision-based systems have great potential for monitoring, detecting, and fighting forest fires. Over the last decade, UAV-based forest fire fighting technology has shown increasing promise. This paper presents a systematic overview of current progress in this field. First, a brief review of the development and system architecture of UAV systems for forest fire monitoring, detection, and fighting is provided. Next, technologies related to UAV forest fire monitoring, detection, and fighting are briefly reviewed, including those associated with fire detection, diagnosis, and prognosis, image vibration elimination, and cooperative control of UAVs. The final section outlines existing challenges and potential solutions in the application of UAVs to forest firefighting. © 2015, (publisher). All Rights Reserved.},
}

@ARTICLE{Peña20155609,
author={Peña, J.M. and Torres-Sánchez, J. and Serrano-Pérez, A. and de Castro, A.I. and López-Granados, F.},
title={Quantifying efficacy and limits of unmanned aerial vehicle (UAV) technology for weed seedling detection as affected by sensor resolution},
journal={Sensors (Switzerland)},
year={2015},
volume={15},
number={3},
pages={5609-5626},
note={cited By 106},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84928668178&doi=10.3390%2fs150305609&partnerID=40&md5=ab73b3abd40a3fc8de705eba531390d1},
abstract={In order to optimize the application of herbicides in weed-crop systems, accurate and timely weed maps of the crop-field are required. In this context, this investigation quantified the efficacy and limitations of remote images collected with an unmanned aerial vehicle (UAV) for early detection of weed seedlings. The ability to discriminate weeds was significantly affected by the imagery spectral (type of camera), spatial (flight altitude) and temporal (the date of the study) resolutions. The colour-infrared images captured at 40 m and 50 days after sowing (date 2), when plants had 5–6 true leaves, had the highest weed detection accuracy (up to 91%). At this flight altitude, the images captured before date 2 had slightly better results than the images captured later. However, this trend changed in the visible-light images captured at 60 m and higher, which had notably better results on date 3 (57 days after sowing) because of the larger size of the weed plants. Our results showed the requirements on spectral and spatial resolutions needed to generate a suitable weed map early in the growing season, as well as the best moment for the UAV image acquisition, with the ultimate objective of applying site-specific weed management operations. © 2015 by the authors; licensee MDPI, Basel, Switzerland.},
}

@ARTICLE{Zhou2015297,
author={Zhou, H. and Kong, H. and Wei, L. and Creighton, D. and Nahavandi, S.},
title={Efficient road detection and tracking for unmanned aerial vehicle},
journal={IEEE Transactions on Intelligent Transportation Systems},
year={2015},
volume={16},
number={1},
pages={297-309},
art_number={6851187},
note={cited By 148},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84922460240&doi=10.1109%2fTITS.2014.2331353&partnerID=40&md5=fdada3792c442796bbeef1fdc3422da9},
abstract={An unmanned aerial vehicle (UAV) has many applications in a variety of fields. Detection and tracking of a specific road in UAV videos play an important role in automatic UAV navigation, traffic monitoring, and ground-vehicle tracking, and also is very helpful for constructing road networks for modeling and simulation. In this paper, an efficient road detection and tracking framework in UAV videos is proposed. In particular, a graph-cut-based detection approach is given to accurately extract a specified road region during the initialization stage and in the middle of tracking process, and a fast homography-based road-tracking scheme is developed to automatically track road areas. The high efficiency of our framework is attributed to two aspects: the road detection is performed only when it is necessary and most work in locating the road is rapidly done via very fast homography-based tracking. Experiments are conducted on UAV videos of real road scenes we captured and downloaded from the Internet. The promising results indicate the effectiveness of our proposed framework, with the precision of 98.4% and processing 34 frames per second for 1046 × 595 videos on average. © 2014 IEEE.},
}

@CONFERENCE{Kim2015,
author={Kim, H. and Sim, S.H. and Cho, S.},
title={Unmanned aerial vehicle (UAV)-powered concrete crack detection based on digital image processing},
journal={International Conference on Advances in Experimental Structural Engineering},
year={2015},
volume={2015-August},
note={cited By 23},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85048339606&partnerID=40&md5=c6e0a3a34ff49ad572f44608d3297b0d},
abstract={Civil infrastructure can suffer from concrete cracks due to the creep, shrinkage, diverse natural loading, aging, and corrosion of reinforcement. Concrete cracks are one of the important features when analyzing the current condition of concrete structures. The shape, length, and width information on concrete cracks are possible to conduct an initial maintenance for the structure safety. Generally, concrete cracks in structures are inspected by the inspector who evaluates the structural health by observing and measuring visual damages on the surface of concrete structures. However, the visual inspection is time consuming and costly, it is dangerous for specialists, and improper environments can cause evaluation errors. Recently, digital image processing (DIP) has been introduced as an alternative automatic crack assessment to the visual inspection. However, image processing has some issues to conduct the crack identification of large-scale infrastructure in terms of the time, cost, and safety. Recent advancements in UAV technologies have enabled low-cost, high-performance UAVs that can be adopted in diverse technologies. In this paper, a prototype of the UAV-based image processing is proposed to identify concrete cracks. From the field experiment, the calculated crack width is similar with the measured crack width by crack gauges. © International Conference on Advances in Experimental Structural Engineering. All rights reserved.},
}

@CONFERENCE{Jenie2015,
author={Jenie, Y.I. and van Kampen, E.-J. and Ellerbroek, J. and Hoekstra, J.M.},
title={Conflict detection and resolution system architecture for unmanned aerial vehicles in civil airspace},
journal={AIAA Infotech at Aerospace},
year={2015},
page_count={15},
note={cited By 7},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85015136396&doi=10.2514%2f6.2015-0483&partnerID=40&md5=479d82cc8b2e6a009222d457472e3b97},
abstract={A novel architecture for a general Unmanned Aerial Vehicle (UAV) Conflict Detection and Resolution (CD&R) system, in the context of their integration into the civilian airspace, is proposed in this paper. The architecture consists of layers of safety approaches, each representing a combination of different methods for surveillance, coordination, action, and decision. These are collected from a survey of various CD&R methods existing in both manned and unmanned domains. The combination process shows that some approaches are suitable, while others are not, for the context of UAV integration. The suitable approaches are then arranged using the’defense in depth’ concept, where each layer filters a specific type of intruder. The final arrangement is set as the proposed architecture, and implemented in an assumed UAV operation within the civil airspace. System and infrastructure considerations are discussed for several examples of prospective types of operation in the airspace. © 2015, American Institute of Aeronautics and Astronautics Inc. All rights received.},
}

@CONFERENCE{Karantzalos2015293,
author={Karantzalos, K. and Koutsourakis, P. and Kalisperakis, I. and Grammatikopoulos, L.},
title={Model-based building detection from low-cost optical sensors onboard unmanned aerial vehicles},
journal={International Archives of the Photogrammetry, Remote Sensing and Spatial Information Sciences - ISPRS Archives},
year={2015},
volume={40},
number={1W4},
pages={293-297},
note={cited By 8},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84974578266&doi=10.5194%2fisprsarchives-XL-1-W4-293-2015&partnerID=40&md5=67c01fc4fc7511772c00e260850d9d3b},
abstract={The automated and cost-effective building detection in ultra high spatial resolution is of major importance for various engineering and smart city applications. To this end, in this paper, a model-based building detection technique has been developed able to extract and reconstruct buildings from UAV aerial imagery and low-cost imaging sensors. In particular, the developed approach through advanced structure from motion, bundle adjustment and dense image matching computes a DSM and a true orthomosaic from the numerous GoPro images which are characterised by important geometric distortions and fish-eye effect. An unsupervised multi-region, graphcut segmentation and a rule-based classification is responsible for delivering the initial multi-class classification map. The DTM is then calculated based on inpaininting and mathematical morphology process. A data fusion process between the detected building from the DSM/DTM and the classification map feeds a grammar-based building reconstruction and scene building are extracted and reconstructed. Preliminary experimental results appear quite promising with the quantitative evaluation indicating detection rates at object level of 88% regarding the correctness and above 75% regarding the detection completeness.},
}

@CONFERENCE{Dvořák201583,
author={Dvořák, P. and Müllerová, J. and Bartaloš, T. and Brůna, J.},
title={Unmanned aerial vehicles for alien plant species detection and monitoring},
journal={International Archives of the Photogrammetry, Remote Sensing and Spatial Information Sciences - ISPRS Archives},
year={2015},
volume={40},
number={1W4},
pages={83-90},
note={cited By 33},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84974556001&doi=10.5194%2fisprsarchives-XL-1-W4-83-2015&partnerID=40&md5=93b89f9b6e60b9b1ed53b71e22c97649},
abstract={Invasive species spread rapidly and their eradication is difficult. New methods enabling fast and efficient monitoring are urgently needed for their successful control. Remote sensing can improve early detection of invading plants and make their management more efficient and less expensive. In an ongoing project in the Czech Republic, we aim at developing innovative methods of mapping invasive plant species (semi-automatic detection algorithms) by using purposely designed unmanned aircraft (UAV). We examine possibilities for detection of two tree and two herb invasive species. Our aim is to establish fast, repeatable and efficient computer-assisted method of timely monitoring, reducing the costs of extensive field campaigns. For finding the best detection algorithm we test various classification approaches (object-, pixel-based and hybrid). Thanks to its flexibility and low cost, UAV enables assessing the effect of phenological stage and spatial resolution, and is most suitable for monitoring the efficiency of eradication efforts. However, several challenges exist in UAV application, such as geometrical and radiometric distortions, high amount of data to be processed and legal constrains for the UAV flight missions over urban areas (often highly invaded). The newly proposed UAV approach shall serve invasive species researchers, management practitioners and policy makers.},
}

@CONFERENCE{Yang20152436,
author={Yang, J. and Yin, D. and Niu, Y. and Zhu, L.},
title={Unmanned aerial vehicles conflict detection and resolution in city airspace},
journal={2015 IEEE International Conference on Robotics and Biomimetics, IEEE-ROBIO 2015},
year={2015},
pages={2436-2441},
art_number={7419704},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84964556617&doi=10.1109%2fROBIO.2015.7419704&partnerID=40&md5=ab123a97dd09e3eb59c6b337af636769},
abstract={Unmanned air vehicles (UAVs) have recently attracted attention of many researchers because of their potential civilian applications. Many of these applications are in the city airspace. Before UAVs are used for civilian applications, a systematic integration of UAVs in non-segregated airspace is needed that allow safe operation of UAVs along with manned aircrafts. One of the critical capabilities for safe operation is conflict detection and resolution (CD&R). The UAVs CD&R problem is studied in this paper. Firstly, the airspace conflict problem is analyzed by geometrical method. Secondly, a hierarchical asynchronous conflict detection method is proposed. The cooperative UAVs conflict resolution method is then studied The conflict resolution problem is casted to a nonlinear optimization problem. When the speeds of conflict involved UAVs are equal, the nonlinear safe separation constraint between two UAVs is transformed into linear constraints and the problem is solved by mixed integer linear programming (MILP). When the speeds of UAVs are unequal, the nonlinear optimization problem is solved by stochastic parallel gradient descent (SPGD) based method. Finally, our approaches are demonstrated in two examples. © 2015 IEEE.},
}

@CONFERENCE{Kamate2015436,
author={Kamate, S. and Yilmazer, N.},
title={Application of Object Detection and Tracking Techniques for Unmanned Aerial Vehicles},
journal={Procedia Computer Science},
year={2015},
volume={61},
pages={436-441},
note={cited By 40},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84962713167&doi=10.1016%2fj.procs.2015.09.183&partnerID=40&md5=300b09064f9cf591e84964639a8c884c},
abstract={In this research, the information captured by Unmanned Aerial Vehicles (UAVs) are eminently utilized in detecting and tracking moving objects which pose a primary security threat against the United States southern border. Illegal trespassing and border encroachment by immigrants is a huge predicament against the United States border security force and the Department of Homeland Security. It becomes insurmountable to warranty suspicious behaviour, monitoring by human operators for long periods of time, due to the massive amount of data involved. The main objective of this research is to assist the human operators, by implementing intelligent visual surveillance systems which help in detecting and tracking suspicious or unusual events in the video sequence. The visual surveillance system requires fast and robust methods of detecting and tracking moving objects. In this research, we have investigated methods for detecting and tracking objects from UAVs. Moving objects were detected using adaptive background subtraction technique successfully and these detected objects were tracked by using Lucas-Kanade optical flow tracking, Continuously Adaptive Mean-Shift tracking based techniques. The simulation results show the efficacy of these techniques in detecting and tracking moving objects in the video sequences acquired by the UAV. © 2015 Published by Elsevier B.V.},
}

@ARTICLE{Yang201511467,
author={Yang, Y. and Fang, Y. and Huang, L.},
title={Edge detection method for unmanned aerial vehicle remote sensing image based on Zernike moments and 2D-Otsu algorithm},
journal={Electronic Journal of Geotechnical Engineering},
year={2015},
volume={20},
number={19},
pages={11467-11475},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84956851881&partnerID=40&md5=7f2eb3f867170bd54c7a98563ed44b60},
abstract={Proposed an edge detection method for Unmanned Aerial Vehicle(UAV) remote sensing images based on Zernike moments and 2D-Otsu algorithm. Firstly, the UAV remote sensing image is filtered in proposed method; then, the filtered UAV remote sensing image is segmented by 2D-Otsu algorithm, and obtained the target image to be processed; at last, the edge information is detected by Zernike moments, and evaluated the accuracy of results. Experimental results show that the proposed method is effective and reliable. © 2015 ejge.},
}

@BOOK{Chamseddine20151123,
author={Chamseddine, A. and Amoozgar, M.H. and Zhang, Y.M.},
title={Experimental validation of fault detection and diagnosis for unmanned aerial vehicles},
journal={Handbook of Unmanned Aerial Vehicles},
year={2015},
pages={1123-1155},
note={cited By 13},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84944566690&doi=10.1007%2f978-90-481-9707-1_41&partnerID=40&md5=a19cc9efe6706a1e44f0bb05abe18577},
abstract={This chapter investigates the problems of fault detection, diagnosis, and fault-tolerant control for unmanned aerial vehicles (UAVs). It presents first a detailed overview on the existing experimental works considering these problems in the literature. The existing works consider fixed-wing as well as rotorcraft UAVs including the single-rotor and the multi-rotor helicopters (also known as quadrotors). Later on, the chapter discusses three Kalman filters employed for actuator fault detection and diagnosis, namely, the unscented Kalman filter, the two-stage Kalman filter, and the adaptive two-stage Kalman filter. The three filters are experimentally applied to a quadrotor helicopter UAV test bed at the Department of Mechanical and Industrial Engineering of Concordia University. The obtained results are shown, compared, and discussed. © Springer Science+Business Media Dordrecht 2015.},
}

@ARTICLE{Rajkumar201521767,
author={Rajkumar, V. and Sathiendran, R. and Saravanan, K. and Hariharavarshan},
title={Autonomous unmanned aerial vehicle radiation detection system},
journal={International Journal of Applied Engineering Research},
year={2015},
volume={10},
number={9},
pages={21767-21775},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84934996383&partnerID=40&md5=d5b7cd733af74786f49f67655c267719},
abstract={The project being proposed is a low cost autonomous UAV which can also be manually controlled, includes live video feed and has fire andradiation detection capabilities. A quad copter will be used to serve this purpose. The main purpose of this system is to monitor the radiation levels and alert the base station if the radiation exceeds the acceptable level. It is also used for surveillance purpose, to have a watch over the activities in the nuclear sites. A Geiger counter will be used to measure the radiation level. The live video feed will be sent to the base station through WI-FI. A tracking system will be used in order to map the location of the device at each radiation measurement. This quad recharges itself automatically through the process of mutual induction which is a new idea we are implementing for recharging. The benefit of this project is to measure the radiation level in nuclear sites that are already undergoing radiation leakage and also to monitor radiation in properly functioning nuclear sites as a precautionary method. Currently a team of technicians with Geiger counters are sent inside the nuclear sites to detect radiation. This device will prevent the need of humans to perform such tasks and thereby reducing the potential risks with human lives and also to perform continuous monitoring in order to keep a check over radiation levels. © Research India Publications.},
}

@ARTICLE{Hong2015,
author={Hong, Z. and Tong, X. and Cao, W. and Jiang, S. and Chen, P. and Liu, S.},
title={Rapid three-dimensional detection approach for building damage due to earthquakes by the use of parallel processing of unmanned aerial vehicle imagery},
journal={Journal of Applied Remote Sensing},
year={2015},
volume={9},
number={1},
art_number={097292},
note={cited By 13},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84929346541&doi=10.1117%2f1.JRS.9.097292&partnerID=40&md5=3345bfe62dc8637837cb1c398bb40d53},
abstract={Rapid damage assessment after an earthquake is vital for an efficient emergency response. With the rapid development of unmanned aerial vehicles (UAVs), they can now be used to rapidly assess the building damage and have the advantages of real-time operation, flexibility, low cost, etc. However, UAV images are "big data," and UAVs can obtain hundreds of scene images in a short period of time. It is, therefore, important to speed up the processing time for UAVimages. This paper proposes a parallel processing approach for accelerating the speed of automatic three-dimensional (3-D) building damage detection, using a preseismic digital topographical map and postseismic UAV images. From the experimental results obtained from 3-D building damage detection of the 2013 Ya'an earthquake in Baoxing County, Sichuan province of China, the comparison of the parallel processing in terms of digital surface model generation using postseismic UAVimages shows that the total cost of the multicores central processing units (CPUs) and graphics processing unit-based implementation is about 11.0 times faster than the single-core CPU implementation. © 2015 Society of Photo-Optical Instrumentation Engineers.},
}

@ARTICLE{Abramov2015358,
author={Abramov, K.V. and Skribtsov, P.V. and Kazantsev, P.A.},
title={Image segmentation method selection for vehicle detection using unmanned aerial vehicle},
journal={Modern Applied Science},
year={2015},
volume={9},
number={5},
pages={358-366},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84928687875&doi=10.5539%2fmas.v9n5p358&partnerID=40&md5=b2549e9f489ba9cd2ee41d4bf9cd3d91},
abstract={This article discusses the possibility of applying the methods of allocating super pixels in the task for detecting moving and stationary vehicles in images obtained from the unmanned aerial vehicle (UAV) which flying over roads and parking lots. The paper will also consider the specificity of images obtained when shooting with the UAV, the specificity of the image processing, and formed the requirements for segmentation algorithm applicable to the task. Author of the article has developed the application required to measure the average image processing speed in the video stream and the application for evaluating vehicles partitioning quality. This application works with the test image, on which the location of the vehicle were determined by the human. A study was conducted of the several algorithms for image segmentation: LIC, Quick Shift, Felzenszwalb-Huttenlocher, and Model based clustering algorithm. The article presents data on the speed and accuracy of the evaluation of these algorithms in the task for UAV's images segmentation. In conclusion, author has chosen methods that suitable for their use in specific application task. For image segmentation, it was decided to use two of the most appropriate method: segmentation algorithm Felzenszwalb-Huttenlocher and developed by the author earlier algorithm based on the approach to clustering model based clustering. The article also discusses possible further ways of unification super pixels containing regions with vehicles. Further work will focus on the modification, parallelization and accelerate software implementation of FHS and MBC. The author will be also investigate the question of the possibility of Markov Chains to solving the task for super pixels association to the regions and the question of the applicability of the binary classification of regions for the detection of vehicles. © By the author(s).},
}

@ARTICLE{Abramov2015295,
author={Abramov, K.V. and Skribtsov, P.V. and Kazantsev, P.A.},
title={Image segmentation method selection for vehicle detection using unmanned aerial vehicle},
journal={Modern Applied Science},
year={2015},
volume={9},
number={5},
pages={295-303},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84928661659&doi=10.5539%2fmas.v9n5p295&partnerID=40&md5=294354c56a2bb03c0c5f69e8e9f1cf93},
abstract={This article discusses the possibility of applying the methods of allocating super pixels in the task for detecting moving and stationary vehicles in images obtained from the unmanned aerial vehicle (UAV) which flying over roads and parking lots. The paper will also consider the specificity of images obtained when shooting with the UAV, the specificity of the image processing, and formed the requirements for segmentation algorithm applicable to the task. Author of the article has developed the application required to measure the average image processing speed in the video stream and the application for evaluating vehicles partitioning quality. This application works with the test image, on which the location of the vehicle were determined by the human. A study was conducted of the several algorithms for image segmentation: LIC, Quick Shift, Felzenszwalb-Huttenlocher, and Model based clustering algorithm. The article presents data on the speed and accuracy of the evaluation of these algorithms in the task for UAV's images segmentation. In conclusion, author has chosen methods that suitable for their use in specific application task. For image segmentation, it was decided to use two of the most appropriate method: segmentation algorithm Felzenszwalb-Huttenlocher and developed by the author earlier algorithm based on the approach to clustering model based clustering. The article also discusses possible further ways of unification super pixels containing regions with vehicles. Further work will focus on the modification, parallelization and accelerate software implementation of FHS and MBC. The author will be also investigate the question of the possibility of Markov Chains to solving the task for super pixels association to the regions and the question of the applicability of the binary classification of regions for the detection of vehicles. © By the author(s).},
}

@ARTICLE{Su2015,
author={Su, A. and Sun, X. and Liu, H. and Zhang, X. and Yu, Q.},
title={Online cascaded boosting with histogram of orient gradient features for car detection from unmanned aerial vehicle images},
journal={Journal of Applied Remote Sensing},
year={2015},
volume={9},
number={1},
art_number={14538},
note={cited By 9},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84928394109&doi=10.1117%2f1.JRS.9.096063&partnerID=40&md5=ae86a4b1a0b29c7d20be21ba9c4de55d},
abstract={Car detection from unmanned aerial vehicle (UAV) images has become an important research field. However, robust and efficient car detection is still a challenging problem because of the cars' appearance variations and complicated background. We present an online cascaded boosting framework with histogram of orient gradient (HOG) features for car detection from UAV images. First, the HOG of the whole sliding window is computed to find the primary gradient direction that is used to estimate the car's orientation. The sliding window is then rotated according to the estimated car's orientation, and the HOG features in the rotated window are efficiently computed using the proposed four kinds of integral histograms. Second, to improve the performance of the weak classifiers, a new distance metric is employed instead of the Euclidean distance. Third, we propose an efficient online cascaded boosting for car detection by combining online boosting with soft cascade. Additionally, for the problem of imbalanced training samples, more positive samples are extracted in the rotated images, and for postprocessing, a confidence map is obtained to combine multiple detections and eliminate isolated false negatives. A set of experiments on real images shows the applicability and high efficiency of the proposed car detection method. © 2015 SPIE.},
}

@ARTICLE{Xiao20143248,
author={Xiao, H. and Liu, Y. and Wang, W. and Zhang, M.},
title={Motion detection algorithm for unmanned aerial vehicle nighttime surveillance},
journal={IEICE Transactions on Information and Systems},
year={2014},
volume={E97D},
number={12},
pages={3248-3251},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84914126713&doi=10.1587%2ftransinf.2014EDL8129&partnerID=40&md5=ce42d700d3de331cd39a7060e026b910},
abstract={In consideration of the image noise captured by photoelectric cameras at nighttime, a robust motion detection algorithm based on sparse representation is proposed in this study. A universal dictionary for arbitrary scenes is presented. Realistic and synthetic experiments demonstrate the robustness of the proposed approach. Copyright © 2014 The Institute of Electronics, Information and Communication Engineers.},
}

@ARTICLE{Calderón2014639,
author={Calderón, R. and Montes-Borrego, M. and Landa, B.B. and Navas-Cortés, J.A. and Zarco-Tejada, P.J.},
title={Detection of downy mildew of opium poppy using high-resolution multi-spectral and thermal imagery acquired with an unmanned aerial vehicle},
journal={Precision Agriculture},
year={2014},
volume={15},
number={6},
pages={639-661},
note={cited By 48},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84912028443&doi=10.1007%2fs11119-014-9360-y&partnerID=40&md5=2f07107024ae2bfdd45a4d11517c2167},
abstract={Downy mildew (DM) caused by the biotrophic obligate oomycete Peronospora arborescens (Berk.) is one of the most economically limiting diseases of opium poppy (Papaver somniferum L.) worldwide. The first symptoms appear as small chlorotic leaf lesions, which can evolve to curled and thickened tissues that become deformed and necrotic as the disease develops. The present study explored the use of high-resolution thermal and multi-spectral imagery as an indicator of DM infection. Work was conducted in two opium poppy field plots artificially infected by P. arborescens. Airborne thermal and multi-spectral imagery were acquired at 200 mm resolution on three dates in spring of 2009 using an unmanned aerial vehicle (UAV). Leaf reflectance and transmittance spectra of DM asymptomatic and symptomatic opium poppy leaves were measured using an integrating sphere. Simulation work was conducted with the coupled PROSPECT + SAILH radiative transfer model to assess the effects of the variability found in an opium poppy plot developing a DM epidemic on the normalized difference vegetation index (NDVI) and the green/red index (R550/R670) calculated from the multi-spectral imagery. The airborne flights enabled DM detection by using image-derived canopy temperature (Tc) normalized by air temperature (Tc − Ta) and the green/red index (R550/R670). Tmin for each grid unit was calculated to estimate pure-vegetation temperature removing background and soil effects. Tmin − Ta and R550/R670 were assessed as a function of aggregated NDVI clusters to compare asymptomatic and symptomatic plants normalized by similar growth levels. Results demonstrated that Tc − Ta and the R550/R670 index were related to physiological stress caused by DM infection. In addition, Tmin − Ta was found to decrease as the NDVI increased and symptomatic plants reached significantly higher (P &lt; 0.05) temperatures for an NDVI ≥0.6. The R550/R670 index was positively correlated with the NDVI, showing significantly higher values (P &lt; 0.05) in symptomatic plants with an NDVI ≥0.5. These results demonstrate the feasibility of detecting P. arborescens infection in opium poppy plants using high-resolution thermal and multi-spectral imagery acquired with an UAV. © 2014, Springer Science+Business Media New York.},
}

@ARTICLE{Peng20142292,
author={Peng, X. and Zhong, Q. and Rao, Z. and Yang, B. and Chen, C. and Su, L.},
title={Intelligent diagnostic techniques of transmission lines corona discharge defect based on ultraviolet detection from unmanned aerial vehicle},
journal={Gaodianya Jishu/High Voltage Engineering},
year={2014},
volume={40},
number={8},
pages={2292-2298},
note={cited By 19},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84907092741&doi=10.13336%2fj.1003-6520.hve.2014.08.006&partnerID=40&md5=e721d23681c21308750d77f5ecc03ab8},
abstract={Insulator diagnosis is an important task for power grid maintenance. Taking the ultraviolet (UV) images from unmanned aerial vehicle (UAV) as the experiment data, we experimentally diagnosed abnormality of the power grid. Firstly, UV images were selected from continues UV video. Secondly, suspected discharge areas were detected using the Otsu method and region grown method. Finally, locations of anomaly of high-voltage power lines insulators are obtained via the position and time synchronization information. Experimental results show that this method can automatically detect abnormal discharge position of insulators. The proposed method can be applied for power grid maintenance.},
}

@ARTICLE{Seo20141012,
author={Seo, D. and Kim, Y. and Kwon, S.},
title={Micro shear-stress sensor for separation detection during flight of unmanned aerial vehicles using a strain gauge},
journal={IEEE Sensors Journal},
year={2014},
volume={14},
number={4},
pages={1012-1019},
art_number={6677601},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84894781231&doi=10.1109%2fJSEN.2013.2292338&partnerID=40&md5=966290bbac2971becd9616151cfb8232},
abstract={A micro shear-stress sensor (MiSS) for real-time detection of flow separation in unmanned aerial vehicles was presented. The direct method was selected for the MiSS, and movement of its floating element was measured using a simple and highly reliable piezoresistive scheme. To realize the MiSS, a polysilicon strain gauge of the piezoresistor type with a very low temperature coefficient of resistivity (TCR) and high gauge factor was first developed. These two characteristics were adjusted by varying the boron concentration during fabrication. The strain gauge was also designed to evaluate the effect of size (width) on these characteristics. The TCR was almost zero and the gauge factor was 32 at a boron concentration of 1.5 × 1019cm -3. The characteristics were unaffected by its width (in the tens of micrometer range). The MiSS was designed and fabricated using the developed polysilicon strain gauge, and its performance was evaluated using a NACA0012 airfoil section in a wind tunnel. At a 0° angle of attack (AOA), the resistance of MiSS increased with the flow. At a 20° AOA, the resistance did not change owing to detachment of the flow caused by separation. In the real-time separation detection test, the resistance of MiSS decreased as soon as separation occurred. Hence, the separation detection ability of the developed MiSS using a polysilicon strain gauge was verified. © 2001-2012 IEEE.},
}

@CONFERENCE{Blyakhman2014,
author={Blyakhman, A.B. and Burov, V.N. and Myakinkov, A.V. and Ryndyk, A.G.},
title={Detection of unmanned aerial vehicles via multi-static forward scattering radar with airborne transmit positions},
journal={2014 International Radar Conference, Radar 2014},
year={2014},
art_number={7060334},
note={cited By 9},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84946688495&doi=10.1109%2fRADAR.2014.7060334&partnerID=40&md5=a1ffd732efb484fc5bd3f2178efe41f0},
abstract={The capabilities of detection of low-observable unmanned aerial vehicles via the forward scattering radar are considered. The configuration of multi-static forward scattering radar enabling the improvement of target detection efficiency is proposed. The forward scattering radar cross section of the widely spread unmanned aerial vehicles is calculated. The required power of the airborne transmitter is estimated. © 2014 IEEE.},
}

@ARTICLE{Zhang2014861,
author={Zhang, Y.P. and Cao, K.C.},
title={Development on fault detection and diagnosis of unmanned aerial vehicles},
journal={Applied Mechanics and Materials},
year={2014},
volume={494-495},
pages={861-864},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84894514230&doi=10.4028%2fwww.scientific.net%2fAMM.494-495.861&partnerID=40&md5=14baf2a33e53afa318de26680101f7f8},
abstract={The reliability of unmanned aerial vehicles (UAVs) has caught the attention of many researchers in the past decades. This paper presents a review on the development and important issues of state-of-the-art researches in the field of fault detection and diagnosis (FDD) techniques. Faults on an individual unmanned aerial vehicle or a group of unmanned aerial vehicles are considered for providing an overall picture of fault detection and diagnosis approaches. © (2014) Trans Tech Publications, Switzerland.},
}

@CONFERENCE{Idachaba2014217,
author={Idachaba, F.E.},
title={Unmanned aerial vehicles and dynamic pipeline pressure profiles: Tools for oil-spill detection and localization},
journal={Society of Petroleum Engineers - 30th Abu Dhabi International Petroleum Exhibition and Conference, ADIPEC 2014: Challenges and Opportunities for the Next 30 Years},
year={2014},
volume={1},
pages={217-225},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84994176864&doi=10.2118%2f171703-ms&partnerID=40&md5=35decab2a5b8b7bd4b224933e2b0b895},
abstract={Pipeline Oil spill is a major challenge with the Oil and Gas production process as it impacts negatively on the environment, the reputation and the finances of the operator. Real time pressure data from an Oil and Gas Pipeline can be used with specially developed algorithms to create dynamic pressure profiles of the pipeline. This profile shows the pressure map of the entire pipeline and it can be used to detect the onset of a leak. Production management systems can be configured in the exception based reporting mode to generate alerts whenever there is a variation in the pressure at any point on the pipeline. The location of pipeline right of way in remote locations increases the monitoring costs and response time in the event of a leak. This paper presents the deployment of Unmanned Aerial Vehicles (UAVs) as the first line of response to alerts generated by the production management systems and the dynamic pressure profiles to provide real time video feedback of the leak points. This will enable a rapid detection and localization of the leak points enabling the speedy deployment of the response teams. The combination of the dynamic pipeline pressure profile and the UAV will provide a rapid monitoring system for the entire pipeline network and facilitate rapid intervention in the event of a leak or any activity on the pipeline right of way providing real time video feedback of the area under investigation and eliminating response to spurious signals and false alarms. © 2014 Society of Petroleum Engineers.},
}

@CONFERENCE{Ellenberg20141788,
author={Ellenberg, A. and Kontsos, A. and Bartoli, I. and Pradhan, A.},
title={Masonry crack detection application of an unmanned aerial vehicle},
journal={Computing in Civil and Building Engineering - Proceedings of the 2014 International Conference on Computing in Civil and Building Engineering},
year={2014},
pages={1788-1795},
note={cited By 46},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84934280470&doi=10.1061%2f9780784413616.222&partnerID=40&md5=dd54ed26443bf6a8129b263ec803ab4f},
abstract={The predominant method for infrastructure evaluation is visual inspection. The large number and scale of inspections often make it difficult to catalog the location, size, and severity of the identified damage. Several nondestructive methods can be used to detect cracks, such as acoustic emission and ultrasound, but they require the installation of many sensors, typically involve measurements in a predetermined area, and often require post-processing. Though image-based crack detection is limited to inspecting surface cracks, it has advantages including speed, repeatability, and large area coverage. Furthermore, the use of image stitching can provide a comprehensive assessment of the health of the entire structure. This method could also be applied using an unmanned aerial vehicle (UAV). This paper discusses major challenges in automated crack detection and implementation on UAVs. © ASCE 2014.},
}

@CONFERENCE{Zhang2014948,
author={Zhang, G. and Zhu, Z. and Si, G. and Wei, X.},
title={Mosaic method based on feature points detection and tracking for unmanned aerial vehicle videos},
journal={2014 10th International Conference on Natural Computation, ICNC 2014},
year={2014},
pages={948-952},
art_number={6975967},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84926673481&doi=10.1109%2fICNC.2014.6975967&partnerID=40&md5=7e8735efee7389a7c0bee41a973a8766},
abstract={This paper explains and implements a fast image mosaic algorithm for unmanned aerial vehicle (UAV) sequence images. In this algorithm, feature points between images are matched using a modified Harris corner detection algorithm, and then an improved pyramid Lucas-Kanade optical flow algorithm and corner points matching authentication algorithm is used to achieve an effective match of the feature points. Next, the transformation parameters between two images are obtained for image transformation. Finally, synthetic algorithm of gradually progressive is used for image fusion. Experimental results show that the fast image mosaic method can get good results for the proposed video images which existing rotation, translation and noise distraction. © 2014 IEEE.},
}

@CONFERENCE{Pouzet2014266,
author={Pouzet, M. and Bonnin, P. and Laneurit, J. and Tessier, C.},
title={A robust real-time image algorithm for moving target detection from unmanned aerial vehicles (UAV)},
journal={ICINCO 2014 - Proceedings of the 11th International Conference on Informatics in Control, Automation and Robotics},
year={2014},
volume={1},
pages={266-273},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84910048195&doi=10.5220%2f0005052802660273&partnerID=40&md5=6a734dd5ef3283e9fac84211b7876d3e},
abstract={We propose a real time method for moving target detection from a camera embedded on a UAV. As the camera is moving, we must estimate the background motion in order to compensate it and then perform the moving target detection. This compensation is realized by an image registration method. For this, we use an hybrid method using global minimization and feature-based approaches, with a pyramidal implementation. The good results obtained for registration give us the potential moving targets. As some wrong detections still appear, due to noise, occlusions or local change of illuminations, we worked on a robust spatio-temporal tracker able to decide if potential targets are real moving targets or not. The algorithm must reach real time performances for VGA images at 30 fps with a standard PC. We have tested our method on different sequences and show the good results obtained thanks to the high precision in the image registration and the spatio-temporal tracker.},
}

@ARTICLE{Qin20147911,
author={Qin, R.},
title={An object-based hierarchical method for change detection using unmanned aerial vehicle images},
journal={Remote Sensing},
year={2014},
volume={6},
number={9},
pages={7911-7932},
note={cited By 58},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84907452177&doi=10.3390%2frs6097911&partnerID=40&md5=95edc235ca716c43fe5298078eb4b5d3},
abstract={There have been increasing demands for automatically monitoring urban areas in very high detail, and the Unmanned Aerial Vehicle (UAV) with auto-navigation (AUNA) system offers such capability. This study proposes an object-based hierarchical method to detect changes from UAV images taken at different times. It consists of several steps. In the first step, an octocopter with AUNA capability is used to acquire images at different dates. These images are registered automatically, based on SIFT (Scale-Invariant Feature Transform) feature points, via the general bundle adjustment framework. Thus, the Digital Surface Models (DSMs) and orthophotos can be generated for raster-based change analysis. In the next step, a multi-primitive segmentation method combining the spectral and geometric information is proposed for object-based analysis. In the final step, a multi-criteria decision analysis is carried out concerning the height, spectral and geometric coherence, and shape regularity for change determination. Experiments based on UAV images with five-centimeter ground resolution demonstrate the effectiveness of the proposed method, leading to the conclusion that this method is practically applicable for frequent monitoring. © 2014 by the authors.},
}

@ARTICLE{Firsov201469,
author={Firsov, S. and Plavynska, N. and Rudenko, K.},
title={Hardware and software package for search, detection and first aid means delivery in rough terrain on basis of a three rotor unmanned aerial vehicle},
journal={Transport Problems},
year={2014},
volume={9},
number={2},
pages={69-73},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84905386972&partnerID=40&md5=1369150ab2c2724f7affe7576fbb8aab},
abstract={The unmanned aerial vehicles are used for dangerous tasks solution. The search and detection of injured in rough terrain is one of them. Thus, vertical take-off unmanned aerial vehicles are of a special interest. A hardware and software package for the task solving is proposed in the article. © Copyright 2014 by Wydawnictwo Politechniki Śla{ogonek}skiej Gliwice.},
}

@CONFERENCE{Maire20132750,
author={Maire, F. and Mejias, L. and Hodgson, A. and Duclos, G.},
title={Detection of dugongs from unmanned aerial vehicles},
journal={IEEE International Conference on Intelligent Robots and Systems},
year={2013},
pages={2750-2756},
art_number={6696745},
note={cited By 18},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84893747808&doi=10.1109%2fIROS.2013.6696745&partnerID=40&md5=d40952725a91b388f7ab3a85933b7343},
abstract={Monitoring and estimation of marine populations is of paramount importance for the conservation and management of sea species. Regular surveys are used to this purpose followed often by a manual counting process. This paper proposes an algorithm for automatic detection of dugongs from imagery taken in aerial surveys. Our algorithm exploits the fact that dugongs are rare in most images, therefore we determine regions of interest partially based on color rarity. This simple observation makes the system robust to changes in illumination. We also show that by applying the extended-maxima transform on red-ratio images, submerged dugongs with very fuzzy edges can be detected. Performance figures obtained here are promising in terms of degree of confidence in the detection of marine species, but more importantly our approach represents a significant step in automating this type of surveys. © 2013 IEEE.},
}

@ARTICLE{Poirier2013303,
author={Poirier, N. and Hautefeuille, F. and Calastrenc, C.},
title={Low Altitude Thermal Survey by Means of an Automated Unmanned Aerial Vehicle for the Detection of Archaeological Buried Structures},
journal={Archaeological Prospection},
year={2013},
volume={20},
number={4},
pages={303-307},
note={cited By 24},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84889099231&doi=10.1002%2farp.1454&partnerID=40&md5=abf30a76dd62cdc431f4296953ade86e},
abstract={Airborne thermal prospecting is based on the principle that there is a fundamental difference between the thermal characteristics of buried remains and the environment in which they are buried. The French 'Archéodrone' project aims to combine the flexibility and low cost of using an airborne drone with the accuracy of the registration of a thermal digital camera. This combination allows the use of thermal prospection for archaeological detection at low altitude with high-resolution information, from a microregional scale to the site scale. The first results have allowed us to assess the contribution of this technique for the detection of ancient roads, land plots boundaries, site plans and underground caves. © 2013 John Wiley & Sons, Ltd.},
}

@ARTICLE{Xu20132265,
author={Xu, C. and Huang, D.},
title={Error analysis for target localization with unmanned aerial vehicle electro-optical detection platform},
journal={Yi Qi Yi Biao Xue Bao/Chinese Journal of Scientific Instrument},
year={2013},
volume={34},
number={10},
pages={2265-2270},
note={cited By 18},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84888086984&partnerID=40&md5=cb9fe8ec9ae05d4e6a116c70a8e59083},
abstract={Aiming at the problems of excessive measurement error factors and analysis difficulty of unmanned aerial vehicle (UAV) electro-optical detection platform (EODP) in target locating process, an error modeling and analysis method based on multi-factor theory is proposed. On the basis of the overall structure of UAV EODP, a target localization model is established according to the mapping relationship of the target from the geodetic coordinate system to photo-sensor coordinate system. The 9 factors, including UAV position and attitude error, EODP angle, range error and etc., are selected as variables; a target localization error calculation formula is derived. The flight experiment data are used to verify the effectiveness of this error calculation method. With simulation experiments, the influence of UAV position, attitude angle error, electro-optical sensor azimuth angle and elevation angle errors and laser ranging error on localization precision is analyzed; at the same time, the relationship between the measuring point of UAV and localization precision in actual application is pointed out: the lower the plane and the larger the pointing angle, the higher the target localization precision.},
}

@CONFERENCE{Kwon201317,
author={Kwon, H. and Yoder, J. and Baek, S. and Gruber, S. and Pack, D.},
title={Maximizing target detection under sunlight reflection on water surfaces with an autonomous unmanned aerial vehicle},
journal={2013 International Conference on Unmanned Aircraft Systems, ICUAS 2013 - Conference Proceedings},
year={2013},
pages={17-24},
art_number={6564669},
note={cited By 8},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84883065946&doi=10.1109%2fICUAS.2013.6564669&partnerID=40&md5=6fdd2dbbecdaf352325c394b5a712571},
abstract={Reflected sunlight can significantly impact vision-based object detection and tracking algorithms, especially ones based on an aerial platform operating over a marine environment. Unmanned aerial systems above a water surface may be unable to detect objects on the water surface due to sunlight glitter. Although the area affected by sunlight reflection may be limited, rapid course corrections of unmanned aerial vehicles (UAVs) - especially fixed-wing UAVs - is also limited by aerodynamics, making it challenging to determine a reasonable path that avoids sunlight reflection while maximizing chances to capture a target. In this paper, we propose an approach for autonomous UAV path planning that maximizes the accuracy of the estimated target location by minimizing the sunlight reflection influences. © 2013 IEEE.},
}

@CONFERENCE{Faughnan2013145,
author={Faughnan, M.S. and Hourican, B.J. and Macdonald, G.C. and Srivastava, M. and Wright, J.-P.A. and Haimes, Y.Y. and Andrijcic, E. and Guo, Z. and White, J.C.},
title={Risk analysis of Unmanned Aerial Vehicle hijacking and methods of its detection},
journal={2013 IEEE Systems and Information Engineering Design Symposium, SIEDS 2013},
year={2013},
pages={145-150},
art_number={6549509},
note={cited By 37},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84881323002&doi=10.1109%2fSIEDS.2013.6549509&partnerID=40&md5=8164cd19d6207484b08d931724b730e6},
abstract={The Federal Aviation Administration (FAA) is in the process of integrating Unmanned Aerial Vehicles (UAVs) into the National Airspace System (NAS) through the Next Generation Air Transportation System (NextGen). A critical component of integrating UAVs into the NAS is the timely identification and mitigation of cyber attacks that could overtake control of a UAV, without the UAV operator's knowledge of a security breach. In an effort to address this risk, this paper aims to achieve two objectives: (i) identify risks of cyber attacks on a UAV and (ii) create a methodology through which UAV operators are informed of such a security breach. The results of this study are intended to support the MITRE Corporation's efforts to identify and control risks associated with UAV integration into the NAS. To achieve the first objective the Capstone team utilized established risk assessment methodologies to identify risk scenarios and filter those scenarios into a manageable list. To achieve the second objective the team developed a methodology that measures the UAV velocity through two on-board systems and any significant difference in the two measures indicates a potential security breach. The team designed and performed an experiment using car movement to simulate UAV flight and performed statistical analysis on the results of the experiment. This contributed to a framework for determining a detection threshold for an alarm system to indicate a UAV may have been hijacked. The threshold accounts for a minimum difference between the two calculations of the velocity data and the duration of time in which this difference occurs, which can be calibrated to minimize Type I (false positive) and Type II (false negative) errors. The recommendation to the MITRE Corporation will contribute to the ongoing efforts to securely integrate UAVs into the NAS. © 2013 IEEE.},
}

@ARTICLE{Maier2013,
author={Maier, J. and Humenberger, M.},
title={Movement detection based on dense optical flow for unmanned aerial vehicles},
journal={International Journal of Advanced Robotic Systems},
year={2013},
volume={10},
art_number={146},
note={cited By 9},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84878410463&doi=10.5772%2f52764&partnerID=40&md5=536765183d4c8f43d891d18c25da6e14},
abstract={In this paper we present a novel computer vision-based movement detection algorithm which can be used for applications, such as human detection with unmanned aerial vehicles. The algorithm uses the deviation of all pixels from the anticipated geometry between 2 or more succeeding images to distinguish between moving and static scenes. This assumption is valid because only pixels which correspond to moving objects can violate the epipolar geometry. For the estimation of the fundamental matrix we present a new method for rejecting outliers which has, contrary to RANSAC, a predictable runtime and still delivers reliable results. To determine movement, especially in difficult areas, we introduce a novel local adaptive threshold method, a combined temporal smoothing strategy and further outlier elimination techniques. All this leads to promising results where more than 60% of all moving persons in our own recorded test set have been detected. © 2013 Maier and Humenberger; licensee InTech.},
}

@ARTICLE{Krerngkamjornkit20131077,
author={Krerngkamjornkit, R. and Simic, M.},
title={Human body detection in search and rescue operation conducted by unmanned aerial vehicles},
journal={Advanced Materials Research},
year={2013},
volume={655-657},
pages={1077-1085},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84874198906&doi=10.4028%2fwww.scientific.net%2fAMR.655-657.1077&partnerID=40&md5=22d724c970aec468192a6b91c120e563},
abstract={Human body detection is a fundamental research problem where computer vision could be applied. This research area has wide applications including surveillance, search and rescue missions. Building an effective human body detector framework under wide ranges of weather, lighting and environmental conditions is a challenge task. A variety of sensors and optimisation algorithms are proposed. This paper aims to review the human body detection methodology conducted by the Unmanned Aerial Vehicles (UAV), and the future research for the UAV search and rescue applications. © (2013) Trans Tech Publications, Switzerland.},
}

@CONFERENCE{Holz2013201,
author={Holz, D. and Nieuwenhuisen, M. and Droeschel, D. and Schreiber, M. and Behnke, S.},
title={Towards multimodal omnidirectional obstacle detection for autonomous unmanned aerial vehicles},
journal={International Archives of the Photogrammetry, Remote Sensing and Spatial Information Sciences - ISPRS Archives},
year={2013},
volume={40},
number={1W2},
pages={201-206},
note={cited By 22},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84903215651&partnerID=40&md5=698625bc5a2b8ec2a8913afaab3ce663},
abstract={Limiting factors for increasing autonomy and complexity of truly autonomous systems (without external sensing and control) are onboard sensing and onboard processing power. In this paper, we propose a hardware setup and processing pipeline that allows a fully autonomous UAV to perceive obstacles in (almost) all directions in its surroundings. Different sensor modalities are applied in order take into account the different characteristics of obstacles that can commonly be found in typical UAV applications. We provide a complete overview on the implemented system and present experimental results as a proof of concept.},
}

@CONFERENCE{Misnan2013289,
author={Misnan, M.F. and Arshad, N.H.M. and Shauri, R.L.A. and Abd Razak, N. and Thamrin, N.M. and Mahmud, S.F.},
title={Real-time vision based sensor implementation on unmanned aerial vehicle for features detection technique of low altitude mapping},
journal={Proceedings - 2013 IEEE Conference on Systems, Process and Control, ICSPC 2013},
year={2013},
pages={289-294},
art_number={6735149},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84897786968&doi=10.1109%2fSPC.2013.6735149&partnerID=40&md5=54e39dbeea80d19022233441b5eb76a9},
abstract={Feature detection is an important task for an autonomous vehicle in getting reference or guide in a agriculture field. Recently, a lot of sensors were implemented for feature detection of a field such as sonar sensor, laser range finder, infrared sensor which it is used as height estimation, size area measurement and path tracking that act as reference for desired measurement in creating a virtual map of the agriculture field which can be used as autonomous vehicle navigation process. A vision based sensor is implemented on the unmanned area vehicle for low altitude mapping. Real-time process with minimum computational process and light weight devices is required and utilized as it used UAV as the transportation element. An experimental setup utilized an analog camera as the front end sensor for the desired detection. The experimental surface is scanned by the analog vision sensor for sensor accuracy analysis used for feature detection application. The process technique is implemented via the medium speed 16-bit processor microcontroller which avoids the requirement of high-speed processor to do image processing. The vision sensor will be utilized into an unmanned aerial vehicle used for feature detection scheme for field measurement. The composing image produced is shown for comparison with the actual image as for performance analysis of the vision based sensor. The designed technique gave acceptable error of image accuracy that adequate to use for features detection on unmanned aeria vehicle. © 2013 IEEE.},
}

@CONFERENCE{Kriheli20131838,
author={Kriheli, B. and Levner, E. and Spivak, A.},
title={Optimization model of routing-and-searching for unmanned aerial vehicles in special target-detection operations},
journal={IFAC Proceedings Volumes (IFAC-PapersOnline)},
year={2013},
volume={46},
number={9},
pages={1838-1842},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84884300867&doi=10.3182%2f20130619-3-RU-3018.00354&partnerID=40&md5=77d837570f6e45b1bf20d8622ba3b2b2},
abstract={We model the problem of routing and search for a hidden target in a directed graph in which nodes represent possible target locations and arcs correspond to possible moves of an unmanned aerial vehicle (UAV) between them. Prior probabilities of locations are known for each target. The inspections are imperfect: a probability of overlooking the hidden target and a probability of a "false alarm" exist. The decision maker has to sequentially inspect the locations so that to find the target with the minimum cost, within a priori given level of confidence An index-based algorithm for finding the optimal search strategy is developed. © IFAC.},
}

@CONFERENCE{Reyes2012,
author={Reyes, H. and Kaabouch, N. and Semke, W. and Salle, S.},
title={Fuzzy logic technique for link loss detection during unmanned aerial vehicle flights},
journal={AIAA Infotech at Aerospace Conference and Exhibit 2012},
year={2012},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84880763235&partnerID=40&md5=f028f8ece9044c1c74672e70956c67b7},
abstract={This paper proposes a fuzzy logic technique to detect the loss of the UAV's communication link. The method consists in testing the channel when a communication failure is detected and sending diagnostic packages to the far end node of the link. To detect the loss of communication and determine the cause, four metrics are used: Bad Packet Ratio (BPR), Clear Channel Assessment (CCA), RSS Received Signal Strength (RSS), and Packet Delivery Ratio (PDR). A Fuzzy Inference System (FSI) uses these parameters to compute a Jamming Index (JI) and to determine if the link is functioning normally, or if it is lost due to jamming or other causes. Evaluation results show that the proposed technique is efficient in detecting the loss of communication and determining its cause. © 2012 by the American Institute of Aeronautics and Astronautics, Inc.},
}

@CONFERENCE{Huang20123049,
author={Huang, J. and Jiang, Z. and Li, S. and Xu, X. and Shi, X.},
title={Key technology research on fault detection and diagnosis for broken-wing small unmanned aerial vehicle},
journal={Proceedings of the World Congress on Intelligent Control and Automation (WCICA)},
year={2012},
pages={3049-3052},
art_number={6358394},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84872285867&doi=10.1109%2fWCICA.2012.6358394&partnerID=40&md5=e616ab0cbc85d205c5da5ebaff626379},
abstract={An accident with any component failure of the small unmanned aerial vehicle (SUAV) will happen in the operation process. At present the sensor and actuator faults are mostly studied and the damaged body considers very few. The research status of the air dynamics and fault detection and diagnosis (FDD) are firstly introduced in the paper. The methods of the pneumatic parameters and properties on the broken-wing SUAV and the key technologies of FDD are analyzed. At last the experiment of the broken-wing SUAV is established by using the FDD subsystems. A specific plan and research methods is provided through the paper. Meanwhile it provides the theory and research foundation for reconstruction control system. © 2012 IEEE.},
}

@CONFERENCE{Wang2012149,
author={Wang, X. and Li, B. and Geng, Q.},
title={Runway detection and tracking for unmanned aerial vehicle based on an improved canny edge detection algorithm},
journal={Proceedings of the 2012 4th International Conference on Intelligent Human-Machine Systems and Cybernetics, IHMSC 2012},
year={2012},
volume={2},
pages={149-152},
art_number={6305746},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84868142166&doi=10.1109%2fIHMSC.2012.132&partnerID=40&md5=522d70e0fc96d0f173bbf63bda899db2},
abstract={A new method based on an improved canny edge detection algorithm for the runway detection and tracking was presented in this paper. Though the traditional Canny Operator has high edge detection capability, it still can be interfered by grave image noise, as its detection accuracy cannot reach single pixel. This paper presented one method that combined Canny Operator with mean filter to represent the runway edge accurately. Then Hough Transform and Chain-Code was used for runway tracking. Experimental results show that this method can have better detection and tracking effect, besides the processing speed is also improved, that laid a favorable foundation for UAV visual navigation. © 2012 IEEE.},
}

@ARTICLE{Sun20123665,
author={Sun, Y. and Wu, C. and Zhang, Y. and Hu, N.},
title={Holes detection in wireless sensor network and redeploy route planning based on unmanned aerial vehicle},
journal={Journal of Information and Computational Science},
year={2012},
volume={9},
number={13},
pages={3665-3672},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84871465229&partnerID=40&md5=14f3e0d194c091ad293cff16fb15e41c},
abstract={The existence of coverage holes in Wireless Sensor Network (WSN) is a vital problem. This paper introduces a graphical method to detect coverage holes, and discusses the research on route planning for Unmanned Aerial Vehicle (UAV) in redeployment job. The paper presents an algorithm based on centroid calculation to locate the positions of the coverage holes. UAV is used to place the redeployment nodes. Considering UAVs characteristic, this paper assumes the route planning problem as the Traveling Salesman Problem (TSP), which can be solved by algorithms such as Genetic Algorithm (GA). The simulation result verifies that it is feasible to redeploy a WSN with these steps. 1548-7741/Copyright © 2012 Binary Information Press.},
}

@CONFERENCE{Yang2012411,
author={Yang, Y. and Liu, F. and Wang, P. and Luo, P. and Liu, X.},
title={Vehicle detection methods from an unmanned aerial vehicle platform},
journal={2012 IEEE International Conference on Vehicular Electronics and Safety, ICVES 2012},
year={2012},
pages={411-415},
art_number={6294294},
note={cited By 19},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84867208430&doi=10.1109%2fICVES.2012.6294294&partnerID=40&md5=2f92806402ea9199d542ea6bd598c70d},
abstract={Vehicle detection is one of the key requirements for traffic surveillance. In most Intelligent Transportation Systems(ITS), cameras are installed in fixed places, which limits the field of view(FOV) of the cameras. This paper presents a new vehicle detection approach by analysing airborne video captured from a quad rotor unmanned aerial vehicle(UAV). Different detection methods on videos of moving and static vehicles are used to meet the requirements of traffic surveillance. Moving vehicles are detected by a feature point tracking method based on the combination of scale invariant feature transform(SIFT) and Kanada-Lucas-Tomasi(KLT) matching algorithm, and an effective clustering method, while static vehicles are recognized by analysing the blob information after automatic road extraction. In order to increase the precision of detection, some pre-processing methods are added into the surveillance system. Experimental results indicate that the proposed approaches of vehicle detection can be realized with a high identification ratio. © 2012 IEEE.},
}

@ARTICLE{Conde2012495,
author={Conde, R. and Alejo, D. and Cobano, J.A. and Viguria, A. and Ollero, A.},
title={Conflict detection and resolution method for cooperating unmanned aerial vehicles},
journal={Journal of Intelligent and Robotic Systems: Theory and Applications},
year={2012},
volume={65},
number={1-4},
pages={495-505},
note={cited By 39},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84855452251&doi=10.1007%2fs10846-011-9564-6&partnerID=40&md5=d2867072601992c657e3b6dfca2f56bf},
abstract={This paper presents a Conflict Detection and Resolution (CDR) method for cooperating Unmanned Aerial Vehicles (UAVs) sharing airspace. The proposed method detects conflicts using an algorithm based on axis-aligned minimum bounding box and solves the detected conflicts cooperatively using a genetic algorithm that modifies the trajectories of the UAVs with an overall minimum cost. The method changes the initial flight plan of each UAV by adding intermediate waypoints that define the solution flight plan while maintaining their velocities. The method has been validated with many simulations and experimental results with multiple aerial vehicles platforms based on quadrotors in a common airspace. The experiments have been carried out in the multi-UAV aerial testbed of the Center for Advanced Aerospace Technologies (CATEC). © 2011 Springer Science+Business Media B.V.},
}

@ARTICLE{Zhang2012764,
author={Zhang, H. and Lu, W. and Tong, L.},
title={Design and implementation of a detection device for flight control system in unmanned aerial vehicle},
journal={Applied Mechanics and Materials},
year={2012},
volume={121-126},
pages={764-767},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-81255134837&doi=10.4028%2fwww.scientific.net%2fAMM.121-126.764&partnerID=40&md5=75054c2c8e947da03debf7233216bb3f},
abstract={Flight control system (FCS) is the command center for the unmanned aerial vehicle (UAV). A low-cost, high-precision micro-UAV attitude calibration table is designed by utilizing the structure of the vertical gyroscope of the flight attitude angle sensor. The detection device for the UAV FCS developed by loop-in-simulation achieves unmanned attitude calibration and overall performance detection of the FCS. The flight control system (FCS) receives a variety of commands from the ground command station to control the flight of aircrafts with varying attitudes. The FCS, together with the sensors, the servo system, and the flight system, make up a stable circuit for controlling the flight attitude and height; the airborne computer controls the engine speed as well as the temperature and achieves secure parking. Moreover, the system controls the safety recovery of the vehicles and manages a range of airborne flight parameters. Upon being acquired by the airborne computer and coded according to the format of the telemetry data flow, the parameters of various devices are transmitted in the standard RS-422 serial interface mode via the radio system to the ground control station.},
}

@CONFERENCE{Schwertfeger201161,
author={Schwertfeger, S. and Birk, A. and Bülow, H.},
title={Using iFMI spectral registration for video stabilization and motion detection by an Unmanned Aerial Vehicle (UAV)},
journal={9th IEEE International Symposium on Safety, Security, and Rescue Robotics, SSRR 2011},
year={2011},
pages={61-67},
art_number={6106770},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84855829197&doi=10.1109%2fSSRR.2011.6106770&partnerID=40&md5=75cbfe62628748c6f4a886258e1d489a},
abstract={Unmanned Aerial Vehicles (UAV), especially in the form of Micro Aerial Vehicles (MAV) are useful tools for reconnaissance, surveillance, and general situation assessment in safety, security, and rescue missions. Many UAV have meanwhile good autonomous flight capabilities, especially by tracking pre-planned routes via GPS or for station-keeping. Here it is shown how the video stream from an UAV can be analyzed to automatically detect motion in the scene while the vehicle is moving itself. Concretely, it is shown how a spectral image registration method, the improved Fourier Mellin Invariant method (iFMI), can be used for video stabilization and motion segmentation. The method is first analyzed with scenes containing artificial markers for ground truth evaluation. Furthermore, results from aerial video data from a quadcopter platform are presented. © 2011 IEEE.},
}

@CONFERENCE{Todorović2011785,
author={Todorović, B.M. and Orlic̀, V.D.},
title={Bayesian analysis of direct sequence spread spectrum unmanned aerial vehicle PPM control signal two-level detection},
journal={Proceedings - ISIE 2011: 2011 IEEE International Symposium on Industrial Electronics},
year={2011},
pages={785-789},
art_number={5984258},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-80052862275&doi=10.1109%2fISIE.2011.5984258&partnerID=40&md5=40800f22aee8b57a275f0e899e6b8ca7},
abstract={Direct sequence spread spectrum (DS-SS) technique is widely used in modern telecommunications and it represents the latest advancement in radio control systems. In this paper we present an optimization of DS-SS scheme for unmanned aerial vehicle (UAV) pulse position modulation (PPM) control signal protection based on two-level detection. A novel framework for Bayesian detection while keeping false start probability below some specified value is developed. Numerical results are compared to those obtained by one-level detection. © 2011 IEEE.},
}

@CONFERENCE{Shah2010,
author={Shah, S.I.A. and Wu, A.D. and Johnson, E.N.},
title={Visual marker detection in the presence of colored noise for unmanned aerial vehicles},
journal={AIAA Infotech at Aerospace 2010},
year={2010},
art_number={2010-3428},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-78649991385&partnerID=40&md5=706544ebb0fffda34ebb6449e32a38d6},
abstract={This paper develops a vision-based algorithm to detect a visual marker in real time and in the presence of excessive colored noise for Unmanned Aerial Vehicles. After using various image analysis techniques, including color histograms, filtering techniques and color space analyses, typical pixel-based characteristics of the visual marker were established. It was found that not only various color space based characteristics were significant, but also relationships between various channels across different color spaces were of great consequence. A block based search algorithm was then used to search for those established characteristics in real-time image data stream from a colored camera. A low cost noise and interference filter was also devised to handle excessive noise that was encountered during flight tests. The specific implementation scenario is that of detection of a Blue LED for GerogiaTech's participating aircraft into the International Aerial Robotics competition. The final algorithm that was implemented on GTAR lama aircraft, used both multiple thresholding and linear confidence level calculations and was successfully used in the competition in 2009. Copyright © 2010 by Syed Irtiza Ali Shah.},
}

@ARTICLE{Laura2010,
author={Laura, T.L. and Sanca, A.S. and Alsina, P.J. and Medeiros, A.A.D.},
title={Positioning of an unmanned aerial vehicle: An alternative for detection of pipeline corrosion [Posicionamento de um veiculo aereo nao tripulado: Uma alternativa para deteccao de corrosoes em dutos]},
journal={Brazilian Petroleum, Gas and Biofuels Institute [IBP] Rio Oil and Gas Conference (Rio De Janeiro, Brazil, 9/13-16/2010) Techn},
year={2010},
page_count={9},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84889262283&partnerID=40&md5=48530623e2b9d5ba3cdf9d14188d1ee7},
abstract={This work is part of the anomalies detecting project in pipelines and tanks in continuous supervision carried out by an multirotor helicopter unmanned aerial vehicle, developed at the Robotics Laboratory in Federal University of Rio Grande do Norte (UFRN). The article describes some preliminary procedures for performing tasks to inspection and monitoring in pipelines and tanks systems, such as the development of a hexarotor micro-air vehicle, altitude and attitude control, guidance using sensor fusion of inertial measurement unit and a monocular camera. For this purpose, a dynamic and 3D graphic simulator was implemented to the air vehicle for inspected environment. Algorithms were implemented to vehicle control and the feature extraction from the sequences of images which enabled their localization. Simulated and experimental results are shown.},
}

@CONFERENCE{Afridi20101125,
author={Afridi, M.J. and Awan, A.J. and Iqbal, J.},
title={AWG-detector: A machine learning tool for the accurate detection of anomalies due to wind gusts (AWG) in the adaptive altitude control unit of an aerosonde unmanned aerial vehicle},
journal={Proceedings of the 2010 10th International Conference on Intelligent Systems Design and Applications, ISDA'10},
year={2010},
pages={1125-1130},
art_number={5687036},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-79851479222&doi=10.1109%2fISDA.2010.5687036&partnerID=40&md5=84ba9518c29caea056fd932823010d41},
abstract={Use of unmanned Aerial Vehicles (UAVs) has gained significant importance in the recent years because of their ability to remotely monitor and perform various tasks in an autonomous manner. However, the control unit of such UAVs fails to adapt quickly when the UAVs are exposed to unpredictable and violent external disturbances such as violent wind gusts and extreme weather conditions. The cost of such adaptation failures can be extremely high and therefore, in order to use any crash preventing strategy, it is imperative to design and use intelligent tools for the early detection of such failures. In this paper we present a machine learning based autonomous tool - AWG-Detector - that detects Anomalies due to Wind Gusts (AWG), in our adaptive Altitude control unit of an Aerosonde UAV. This adaptive Altitude control unit comprises of a PI based Roll controller and a Hybrid neuro-fuzzy based Pitch controller. Experimental results show that our AWG-Detector achieves an accuracy of more than 99% in detecting anomalies due to wind gusts. To the best of our knowledge, this is the first study that targets the detection of Wind Gust anomalies in the Altitude control unit of an Aerosonde UAV by developing a comparison of five well-known machine learning techniques. © 2010 IEEE.},
}

@CONFERENCE{Andriluka20101740,
author={Andriluka, M. and Schnitzspan, P. and Meyer, J. and Kohlbrecher, S. and Petersen, K. and Von Stryk, O. and Roth, S. and Schiele, B.},
title={Vision based victim detection from unmanned aerial vehicles},
journal={IEEE/RSJ 2010 International Conference on Intelligent Robots and Systems, IROS 2010 - Conference Proceedings},
year={2010},
pages={1740-1747},
art_number={5649223},
note={cited By 77},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-78651477795&doi=10.1109%2fIROS.2010.5649223&partnerID=40&md5=3e6937d59304081bccd616bd71b5db3e},
abstract={Finding injured humans is one of the primary goals of any search and rescue operation. The aim of this paper is to address the task of automatically finding people lying on the ground in images taken from the on-board camera of an unmanned aerial vehicle (UAV). In this paper we evaluate various state-of-the-art visual people detection methods in the context of vision based victim detection from an UAV. The top performing approaches in this comparison are those that rely on flexible part-based representations and discriminatively trained part detectors. We discuss their strengths and weaknesses and demonstrate that by combining multiple models we can increase the reliability of the system. We also demonstrate that the detection performance can be substantially improved by integrating the height and pitch information provided by on-board sensors. Jointly these improvements allow us to significantly boost the detection performance over the current de-facto standard, which provides a substantial step towards making autonomous victim detection for UAVs practical. ©2010 IEEE.},
}

@ARTICLE{Yanmaz200926,
author={Yanmaz, E.},
title={Event detection using unmanned aerial vehicles: Ordered versus self-organized search},
journal={Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
year={2009},
volume={5918 LNCS},
pages={26-36},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-72449207484&doi=10.1007%2f978-3-642-10865-5_3&partnerID=40&md5=6d58581f6d17d70e5c24bf809bccfe28},
abstract={Event coverage problem in wireless sensor networks has drawn the interest of several researchers. While most of the previous work has been on static or ground mobile sensor networks, airborne sensor networks have also found its way into several civil and military applications such as environmental monitoring or battlefield assistance. In this work, we study the mobility pattern of an Unmanned Aerial Vehicle (UAV) network and explore the benefits of ordered and self-organized random mobility in terms of event detection performance, when the event is stationary and event duration is finite. Specifically, we compare the performance of a UAV network flying in parallel formation to a simple, distributed, locally-interactive coverage-based mobility model as well as legacy mobility models such as random walk and random direction. We study the event detection probability of the UAV network with both perfect and imperfect sensing capabilities. Our results show that when the timing constraints are highly stringent or when the UAV sensors have a high miss probability, flying in formation cannot achieve a high detection probability and a self-organized distributed mobility model is more effective. © 2009 Springer-Verlag.},
}

@CONFERENCE{Sarunic2009,
author={Sarunic, P.W. and Evans, R.J. and Moran, B.},
title={Control of unmanned aerial vehicles for passive detection and tracking of multiple emitters},
journal={IEEE Symposium on Computational Intelligence for Security and Defense Applications, CISDA 2009},
year={2009},
art_number={5356551},
note={cited By 7},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-77950559277&doi=10.1109%2fCISDA.2009.5356551&partnerID=40&md5=290b63c598c8b39a34f711880362d983},
abstract={An algorithm for trajectory optimization of autonomous aerial vehicles performing multiple target tracking is proposed. The problem is approached by formulating it as a partially observed Markov decision process (POMDP) and developing a moving-horizon solution taking into account short and long term costs. To evaluate the effectiveness of the approach a simulation involving multiple UAVs and targets is performed. © 2009 Crown Copyright.},
}

@CONFERENCE{Correia20091281,
author={Correia, J. and Bencatel, R. and Marçal, A.R.S. and Puga, A. and Sousa, J.B. and Gonçalves, G.M.},
title={Video based motion tracking and river detection with an unmanned aerial vehicle},
journal={Proceedings, 33rd International Symposium on Remote Sensing of Environment, ISRSE 2009},
year={2009},
pages={1281-1284},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84879909938&partnerID=40&md5=759b94944004f034bb84467b0a92317c},
abstract={Here we present a motion tracking algorithm and a fast river detection algorithm using a near infrared camera on-board an UAV. These algorithms have to run on a slow PC104. The motion tracking algorithm is based on the Normalized Cross-Correlation and the river detection algorithm uses Meyer's Watershed method. Simulation results with a video are presented.},
}

@CONFERENCE{Sarunic200937,
author={Sarunic, P.W. and Evans, R.J.},
title={Control of unmanned aerial vehicles performing multiple target passive detection and tracking},
journal={ISSNIP 2009 - Proceedings of 2009 5th International Conference on Intelligent Sensors, Sensor Networks and Information Processing},
year={2009},
pages={37-42},
art_number={5416774},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-77950939797&doi=10.1109%2fISSNIP.2009.5416774&partnerID=40&md5=0db19b17ad63eb475cd4a51bfa34d2fa},
abstract={Advances in a previously proposed algorithm for trajectory optimization of autonomous aerial vehicles performing multiple target tracking are presented. The algorithm involves a variant of the moving horizon control approach, built on a partially observed Markov decision process (POMDP) model of the sensor-target system. To evaluate the effectiveness of the advances a simulation involving multiple UAVs and targets is performed. © 2009 IEEE.},
}

@CONFERENCE{Donnay2009771,
author={Donnay, E.},
title={Use of unmanned aerial vehicle (UAV) for the detection and surveillance of marine oil spills in the belgian part of the north sea},
journal={Proceedings of the 32nd AMOP Technical Seminar on Environmental Contamination and Response},
year={2009},
volume={2},
pages={771-779},
note={cited By 11},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-70449673260&partnerID=40&md5=30d8ff52d538af44fb1357373ad91064},
abstract={Since the summer of 2008, unmanned aerial vehicles (UAV) of the Belgian Army have been deployed on a routine way above the southern part of the North Sea for the surveillance and the detection of oil spills. These UAV are of the B-Hunter type. They have been commissioned in 2000 by the Belgian Army for the purpose of military intelligence, reconnaissance and surveillance missions. They are fitted with a dual sensor gyrostabilized turret combining a daylight camera and a thermal infrared camera allowing for day and night observations. Live images of the sensors are transmitted in real time to the ground control station. The use of the B-Hunters for the detection of marine pollution finds its origin in a decision taken in 2003 by the Belgian Federal government aiming at an optimization of the operational resources for detecting illicit discharges by vessels and collecting evidence for prosecuting offenders. To that end, the Belgian authorities have developed a concept of marine environmental surveillance based on the combined use of four different surveillance platforms: remote sensing aircraft, helicopter, satellite and UAV. This concept is now fully implemented. The operations of all Belgian marine pollution surveillance platforms are coordinated from the Maritime Security Center (MIK) of the Belgian Coastguard structure where all relevant data are centralized and dispatched to the competent authorities for information and further action. The surveillance aircraft is used for routine patrol flights above the southern part of the North Sea. The satellite surveillance service provides for information in near real time about possible oil spills and other anomalies at the sea surface. Stand-by helicopters are used for rapid assessment of reported spills and sampling. The main advantages of the B-Hunter system are its long flight endurance of about 10 hours and the fact that it is undetectable thanks to its small size and low noise signature. The B-Hunter system offers additional possibilities for routine surveillance such as the continuous monitoring of a specific area (anchorage, shipping lane) or the tracking of a suspect vessel. The B-Hunters are also expected to play a useful role in case of a major accidental spill for the monitoring in real time of the progress of the response operations and for providing information for guiding the pollution combating vessels. The positive results of the campaigns of surveillance flights carried out in 2008 with the B-Hunter system above the Belgian waters have demonstrated the suitability of the use of UAV systems for the purpose of the surveillance of marine pollution caused by ships and other maritime surveillance tasks.},
}

@ARTICLE{Heredia20097566,
author={Heredia, G. and Caballero, F. and Maza, I. and Merino, L. and Viguria, A. and Ollero, A.},
title={Multi-Unmanned aerial vehicle (UAV) cooperative fault detection employing differential global positioning (DGPS), inertial and vision sensors},
journal={Sensors},
year={2009},
volume={9},
number={9},
pages={7566-7579},
note={cited By 56},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-70350033778&doi=10.3390%2fs90907566&partnerID=40&md5=2b659bb407d8d824aa0634696a9143ea},
abstract={This paper presents a method to increase the reliability of Unmanned Aerial Vehicle (UAV) sensor Fault Detection and Identification (FDI) in a multi-UAV context. Differential Global Positioning System (DGPS) and inertial sensors are used for sensor FDI in each UAV. The method uses additional position estimations that augment individual UAV FDI system. These additional estimations are obtained using images from the same planar scene taken from two different UAVs. Since accuracy and noise level of the estimation depends on several factors, dynamic replanning of the multi-UAV team can be used to obtain a better estimation in case of faults caused by slow growing errors of absolute position estimation that cannot be detected by using local FDI in the UAVs. Experimental results with data from two real UAVs are also presented. © 2009 by the authors.},
}

@ARTICLE{Cong2009938,
author={Cong, Y. and Li, X. and Tian, J. and Tang, Y.},
title={Real-time attitude angle estimation for unmanned aerial vehicle based on skyline detection},
journal={Yi Qi Yi Biao Xue Bao/Chinese Journal of Scientific Instrument},
year={2009},
volume={30},
number={5},
pages={938-943},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-67649231238&partnerID=40&md5=514448618aff190e5905636873f82b8a},
abstract={This paper presents an accurate, real-time skyline detection algorithm for Unmanned Aerial Vehicle (UAV). On the basis of the actual situation, a functional model of skyline energy is firstly established. In practical application, the linear constraint is analyzed to simplify the model to reduce computing time, and then using coarse-to-fine idea to extract the skyline. The rough local skyline is detected by a group of short horizon lines, and then the rough skyline is fitted by the rough local skylines. Finally the gradient based model is used to detect the accurate skyline, and the rolling angle of the UAV can be calculated by the final skyline. The results of the experiment show that the skyline detection algorithm has better robustness, accuracy and real-time.},
}

@ARTICLE{Yoon2009195,
author={Yoon, Y. and Gruber, S. and Krakow, L. and Pack, D.},
title={Autonomous target detection and localization using cooperative unmanned aerial vehicles},
journal={Lecture Notes in Control and Information Sciences},
year={2009},
volume={381},
pages={195-205},
note={cited By 7},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-54349088488&doi=10.1007%2f978-3-540-88063-9_12&partnerID=40&md5=f505a6d6e391d2f3978330a02b6d5ba2},
abstract={In this chapter we present sensor implementation issues encountered in developing a team of cooperative unmanned aerial vehicles (UAVs) for intelligence, surveillance and reconnaissance missions. UAVs that compose the cooperative team are equipped with heterogeneous sensors and onboard processing capability. The sensor information collected by each UAV is constantly shared among the neighboring UAVs and processed locally using Out-of-Order Sigma-Point Kalman Filtering (O3SPKF) techniques. Results from flight experiments support the effectiveness of the cooperative autonomous UAV technologies. © 2009 Springer Berlin Heidelberg.},
}

@CONFERENCE{Bateman20081246,
author={Bateman, F. and Noura, H. and Ouladsine, M.},
title={Active fault detection and isolation strategy for an unmanned aerial vehicle with redundant flight control surfaces},
journal={2008 Mediterranean Conference on Control and Automation - Conference Proceedings, MED'08},
year={2008},
pages={1246-1251},
art_number={4602147},
note={cited By 11},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-52949098336&doi=10.1109%2fMED.2008.4602147&partnerID=40&md5=54ac53830867dda2201750952eaefb06},
abstract={In this paper, a diagnosis system using unknown input observers in order to detect, isolate and estimate faulty control surface positions for a small UAV, is presented. As this aircraft is equipped with redundant actuators, flap and aileron positions are not input observable and an active diagnosis process has to be implemented. © 2008 IEEE.},
}

@CONFERENCE{Goad2008231,
author={Goad, A. and Schorer, D. and Sullenberger, J. and Yousuf, F. and Yu, A. and Donohue, G. and Hintz, K.},
title={Landmine detection utilizing an unmanned aerial vehicle},
journal={Proceedings of the 2008 IEEE Systems and Information Engineering Design Symposium, SIEDS 2008},
year={2008},
pages={231-236},
art_number={4559717},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-51749102248&doi=10.1109%2fSIEDS.2008.4559717&partnerID=40&md5=c92eb8cf083eef833839a20a0849ac82},
abstract={Landmines pose a great danger to people in many areas. It is imperative to correctly identify the location of landmines for proper removal. Hence, there is a need to efficiently and accurately identify locations of landmines. The objective of this project is to conduct preliminary system analysis of three unmanned aerial vehicles (UAVs) utilizing ground penetrating synthetic aperture radar (GPSAR) aiding in the detection of landmines. Moreover, the effort will aid in assessing the overall effectiveness of landmine detection utilizing a UAV. Three design alternatives are modeled and tested. The first design alternative is a MQ-1 Predator; a long-endurance UAV primarily used for reconnaissance and surveillance missions. The second alternative is a Shadow 600. The Shadow 600 is capable of carrying various payloads. The third design alternative is the Shadow 200 which can be launched from the ground using a catapult. Each design alternative carries an unfocused GPSAR utilizing the length of the fuselage to increase aperture efficiency. Using Satellite Tool Kit (STK) analysis software, design alternatives are assessed by their performance in scanning a one square kilometer area of interest (AOI). Critical figures of merit used to elicit system effectiveness include time on target (time that the radar pulses the landmine), area overlap percentage, area coverage, coverage speed, and energy consumption. Acquisition cost, operational cost, and maintenance cost of each design alternative are plotted against system effectiveness to identify the best alternative. ©2008 IEEE.},
}

@CONFERENCE{Hanna2008113,
author={Hanna, E. and Straznicky, P. and Goubran, R.},
title={Obstacle detection for low flying unmanned aerial vehicles using stereoscopic imaging},
journal={Conference Record - IEEE Instrumentation and Measurement Technology Conference},
year={2008},
pages={113-118},
art_number={4547014},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-51349121013&doi=10.1109%2fIMTC.2008.4547014&partnerID=40&md5=a919addb9c3071c4ba1c063c32d0d219},
abstract={This paper describes a stereoscopic imaging algorithm that is modified for obstacle detection in low flying Unmanned Aerial Vehicles (UAVs). In this type offlight, obstacle detection must be carried out quickly for the system to be effective in real time. Additionally, since the aircraft is close to the ground, the horizon is usually at the top ofthefield of view and obstacles must be distinguished from the clutter of the terrain. The sparse edge detection and reconstruction algorithm proposed, produces fast but partial reconstructions of the environment. One image is passed through a series of edge detectors to generate a very sparse outline of the environment. This outline is then correlated to the second image and the resulting reconstruction is added to a model of the environment. Although each individual reconstruction is incomplete, the overall result after a short initialization period is a model of the environment that is more comprehensive than a single stereoscopic correlation run with a more detailed edge detector. Simulation of the algorithm on test image patterns showed an increase in performance relative to the length of the sequence of stereo pairs. On average, the signal to noise ratio (SNR) for sparse edge reconstruction was significantly higher than that for single correlation with more detailed edge detectors. Additionally it was found that the processing speed of the sparse edge detection algorithm on a pair of stereoscopic images is faster than the processing carried out by a more detailed edge detector. A test flight was also carried out to test the algorithm in a more realistic scenario. The test confirmed that the sparse edge reconstruction algorithm resulted in a much more detailed view of the environment than if a single, more detailed edge detector had been used. © 2008 IEEE.},
}

@ARTICLE{Ducard2008225,
author={Ducard, G. and Geering, H.P.},
title={Efficient nonlinear actuator fault detection and isolation system for unmanned aerial vehicles},
journal={Journal of Guidance, Control, and Dynamics},
year={2008},
volume={31},
number={1},
pages={225-237},
note={cited By 92},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-43649093141&doi=10.2514%2f1.31693&partnerID=40&md5=51b05528db2cb91910ee64297bd0adf5},
abstract={In this paper, three main limitations of the classical implementation of the multiple-model adaptive-estimation method to isolate faults based on predefined fault hypotheses are highlighted. The first concerns the number of filters that must be designed to span the range of possible fault scenarios, which must be limited due to computational load. The second limitation appears when an actuator is locked at an arbitrary nonzero position that biases the residuals of the Kalman filters, leading to inaccurate fault detection and state estimation. Third, most of the implementations of a multiple-model adaptive-estimation method only work efficiently around predefined operating conditions. This paper presents a nonlinear actuator-fault detection and isolation system, which properly works over the entire operating envelope of an aircraft. Locked-in-place and floating actuator faults can be handled. The robustness of the fault detection and isolation system is enhanced by the usage of auxiliary excitation signals. The fault detection and isolation system is also capable of handling two simultaneous actuator failures with no increase of the computational load. The complete system was demonstrated in simulation with a nonlinear model of a model aircraft in moderate to severe wind conditions.},
}

@CONFERENCE{Sufi20071047,
author={Sufi, A.A.},
title={An SVD-based method of obstacle detection and efficient evasive maneuvering for unmanned aerial vehicles},
journal={Association for Unmanned Vehicle Systems International - Unmanned Systems North America Conference 2007},
year={2007},
volume={2},
pages={1047-1061},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-70449134552&partnerID=40&md5=13988a6b664ad6a47beebcfeea199d16},
abstract={Unmanned Aerial Vehicles (UAV's) have been the subject of immense research and development in recent years. Many applications require these aircrafts to travel in partially known, or sometimes even completely alien environments. In such surroundings, the UAV is desired to fly from some point A to B autonomously, avoiding obstacles in its path as it encounters them. This paper describes a reliable method of detecting obstacles and providing an alternative path so as to avoid the encountered obstacles efficiently. The problem is described and the solution is provided by way of examples. Results show that this method, coupled with other evasive maneuvering techniques, can significantly reduce the need for path planning algorithms.},
}

@ARTICLE{Chen20071313,
author={Chen, L. and Chen, Z.},
title={Vision-based runway obstacle detection scheme for unmanned combat aerial vehicles},
journal={Beijing Hangkong Hangtian Daxue Xuebao/Journal of Beijing University of Aeronautics and Astronautics},
year={2007},
volume={33},
number={11},
pages={1313-1316},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-37749021812&partnerID=40&md5=77b204d5c3690eab8d4977dccbda8f63},
abstract={A computer-vision-based runway obstacle detection scheme for an unmanned combat air vehicle (UCAV) was presented. The scheme combined the advantages of the feature-based and the flow-based obstacle detection algorithms. Instead of using gradient-based method, a multi-scale optical flow estimation method based on feature point matching was adopted, which make it possible to calculate sparse optical flow field directly from image sequences. Under some relative hypothesis, obstacle on the runway could be detected even with certain navigation errors. The detection sensitivity and the stage applicable for obstacle detection were also discussed. The obstacle detection scheme can run properly on the real-time simulation system for autonomous landing of the UCAV.},
}

@CONFERENCE{Bateman2007145,
author={Bateman, F. and Noura, H. and Ouladsine, M.},
title={Control surfaces fault detection and isolation for an unmanned aerial vehicle},
journal={3rd Int. Conf. on Advances in Vehicle Control and Safety 2007, AVCS 2007 and 3rd Int. Conf. on Integrated Modeling and Analysis in Applied Control and Automation, IMAACA 2007, Held at the IMSM 2007},
year={2007},
pages={145-150},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84900020115&partnerID=40&md5=2c2e32fcfab9b9a2c5afcef5ed38154a},
abstract={In this paper a fault detection and isolation method (FDI) for an Unmanned Aerial Vehicle (UAV) is presented. The proposed method deals with control surface failures while the aircraft is equipped with an autopilot. This method does not require the complete model of the system. Fault detection consists of exciting judiciously actuators and analyzing cross-correlations between measurements. The temporal and frequential properties of the signal are analyzed during transient of the failure. From this point of view, a wavelet analysis has been implemented to isolate the faulty control surfaces.},
}

@CONFERENCE{Bateman2007145,
author={Bateman, F. and Noura, H. and Ouladsine, M.},
title={Control surfaces fault detection and isolation for an Unmanned Aerial Vehicle},
journal={International Conference on Integrated Modeling and Analysis in Applied Control and Automation},
year={2007},
pages={145-150},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84897014551&partnerID=40&md5=ad9f16d9ddb7e6168af18c63547bac88},
abstract={In this paper a fault detection and isolation method (FDI) for an Unmanned Aerial Vehicle (UAV) is presented. The proposed method deals with control surface failures while the aircraft is equipped with an autopilot. This method does not require the complete model of the system. Fault detection consists of exciting judiciously actuators and analyzing cross- correlations between measurements. The temporal and frequential properties of the signal are analyzed during transient of the failure. From this point of view, a wavelet analysis has been implemented to isolate the faulty control surfaces.},
}

@CONFERENCE{Wang2006,
author={Wang, X.S. and Lee, B.S. and Sadjadi, F.},
title={AKSED: Adaptive knowledge-based system for event detection using collaborative unmanned aerial vehicles},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2006},
volume={6234},
art_number={62340Q},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-33748526233&doi=10.1117%2f12.667844&partnerID=40&md5=9c7b2f64845968f378626e3cc137ce67},
abstract={Advances in sensor technology and image processing have made it possible to equip unmanned aerial vehicles (UAVs) with economical, high-resolution, energy-efficient sensors. Despite the improvements, current UAVs lack autonomous and collaborative operation capabilities, due to limited bandwidth and limited on-board image processing abilities. The situation, however, is changing. In the next generation of UAVs, much image processing can be carried out onboard and communication bandwidth problem will improve. More importantly, with more processing power, collaborative operations among a team of autonomous UAVs can provide more Intelligent event detection capabilities. In this paper, we present ideas for developing a system enabling target recognitions by collaborative operations of autonomous UAVs. UAVs are configured in three stages: manufacturing, mission planning, and deployment. Different sets of information are needed at different stages, and the resulting outcome is an optimized event detection code deployed onto a UAV. The envisioned system architecture and the contemplated methodology, together with problems to be addressed, are presented.},
}

@CONFERENCE{Merino2006,
author={Merino, L. and Caballero, F. and Ollero, A.},
title={Applications of networked unmanned aerial vehicles to cooperative fire detection using grid-based data fusion techniques},
journal={IFAC Proceedings Volumes (IFAC-PapersOnline)},
year={2006},
volume={8},
number={PART 1},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-80051595898&doi=10.3182%2f20060906-3-it-2910.00087&partnerID=40&md5=668fe95f8b14bbbdc1feaf7d5aeb743c},
abstract={The paper presents a system for cooperative fire detection by means of a eet of networked heterogeneous UAVs. A grid is used to represent the probability of having fire in a certain position within a given area. Different sensors are considered: infrared and visual cameras and a specialized fire sensor. A Bayesian approach is followed for the integration of the sensor readings and the evolution of the grid as new information is available. The paper presents results from actual field experiments of small controlled fires. Copyright © 2006 IFAC.},
}

@CONFERENCE{Price20062854,
author={Price, A. and Pyke, J. and Ashiri, D. and Cornall, T.},
title={Real time object detection for an unmanned aerial vehicle using an FPGA based vision system},
journal={Proceedings - IEEE International Conference on Robotics and Automation},
year={2006},
volume={2006},
pages={2854-2859},
art_number={1642134},
note={cited By 18},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-33845631308&doi=10.1109%2fROBOT.2006.1642134&partnerID=40&md5=325fd918d12c15d319d3e1e52d2957bf},
abstract={Unmanned Aerial Vehicles (UAV's) are becoming more predominant in modern reconnaissance in both military and civilian applications. Object identification and tracking are typical elements of most missions [1]. While large and expensive UAV's operate in many theatres, there is a need for local intelligence gathering using small, low cost and often disposable UAV platforms. In many situations it may not be practical or desirable for the UAV to be relaying information to the ground via radio link. Similarly, waiting upon ground based control for instruction may also limit the usefulness of a UAV. While ground based control is common, full autonomy allows a UAV to operate beyond the range of human intervention. In such cases, the UAV must be capable of making decisions for itself based on information gained from its surroundings. This paper discusses the development of a vision processing system for a low-cost UAV with a total flying weight of under 3kg. The system has currently been tested using simulated and real aerial footage with a mission to detect the presence of cars and land vehicles in the field of view. Experiments were conducted using actual FPGA based hardware. This research was conducted by Ashiri and Pyke as part of an undergraduate thesis project in the Dept. Electrical and Computer Systems Engineering at Monash University. ©2006 IEEE.},
}

@CONFERENCE{Merino20051884,
author={Merino, L. and Caballero, F. and Martínez-de Dios, J.R. and Ollero, A.},
title={Cooperative fire detection using unmanned aerial vehicles},
journal={Proceedings - IEEE International Conference on Robotics and Automation},
year={2005},
volume={2005},
pages={1884-1889},
art_number={1570388},
note={cited By 91},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-33846144430&doi=10.1109%2fROBOT.2005.1570388&partnerID=40&md5=d38de94bc0753e4ce4b0b6c591167e2c},
abstract={The paper presents a framework for cooperative fire detection by means of a fleet of heterogeneous UAVs. Computer vision techniques are used to detect and localize fires from infrared and visual images and other data provided by the cameras and other sensors on-board the UAVs. The paper deals with the techniques used to decrease the uncertainty in fire detection and increase the accuracy in fire localisation by means of the cooperation of the information provided by several UAVs. The presented methods have been developed in the COMETS multi-UAV project. ©2005 IEEE.},
}

@CONFERENCE{Drozeski2005,
author={Drozeski, G.R. and Saha, B. and Vachtsevanos, G.J.},
title={A fault detection and reconfigurable control architecture for unmanned aerial vehicles},
journal={IEEE Aerospace Conference Proceedings},
year={2005},
volume={2005},
art_number={1559597},
note={cited By 44},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-33751511730&doi=10.1109%2fAERO.2005.1559597&partnerID=40&md5=51db14c7d29e1de15b11e3a93b788467},
abstract={The past decade has seen the development of several reconfigurable flight control strategies for unmanned aerial vehicles. Although the majority of the research is dedicated to fixed wing vehicles, simulation results do support the application of reconfigurable flight control to unmanned rotorcraft. This paper develops a fault tolerant control architecture that couples techniques for fault detection and identification with reconfigurable flight control to augment the reliability and autonomy of an unmanned aerial vehicle. The architecture is applicable to fixed and rotary wing aircraft. An adaptive neural network feedback linearization technique is employed to stabilize the vehicle after the detection of a fault. Actual flight test results support the validity of the approach on an unmanned helicopter. The fault tolerant control architecture recovers aircraft performance after the occurrence of four different faults in the flight control system: three swash-plate actuator faults and a collective actuator fault. All of these faults are catastrophic under nominal conditions. © 2005 IEEE.},
}

@CONFERENCE{Wang2005,
author={Wang, H. and Peng, J. and Li, L.},
title={Runway detection of an unmanned landing aerial vehicle based on vision},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2005},
volume={6043 II},
art_number={60432A},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-33644961097&doi=10.1117%2f12.654995&partnerID=40&md5=5c8f07d491f1aaedcc7e34eb9b239e59},
abstract={When an monocular vision-based unmanned aerial vehicle (UAV) based on vision is flown to the final approach fix to intercept the glide slope without the navigation of Global Positioning System (GPS), the position and orientation of the airport runway in image must be detected accurately so as to a host of suitable procedures have to be followed. The optimum length of the final approach is about five miles from the runway threshold. The front view of the runway, which is achieved at the moment, is very illegible. The approaching marking (cross bar) of the runway are showed as some white spots of high intensity and the complicated backgrounds of the airport are included in the images. In this case, spots with high intensity should be extracted and classified, some of these spots are just the images of the background noises and the pseudo-targets, which can't be separated with the spots of the runway as in the view there is no significant characteristic difference among them ostensibly. Fortunately, in the terrestrial coordinate space, most of the runway marks are located at the apexes of a rectangle, having some geometric relationships. The relationship among the projection coordinates of the runway spots in the images can be determined according to the perspective principle, the constraint condition of the rectangle as well as the front shot constraint condition of the target, by using this relationship, the runway approaching marks can be separated, the position and the direction of the runway in the images can be identified. In this paper, the clustering management is adopted so as to greatly reduce the computing time. The consequence of the experiments shows that by this algorithm, even from a place far away from the runway whose marks are unclear, we also can effectively detect the runway.},
}

@ARTICLE{Abd-Elrahman200537,
author={Abd-Elrahman, A. and Pearlstine, L. and Percival, F.},
title={Development of pattern recognition algorithm for automatic bird detection from unmanned aerial vehicle imagery},
journal={Surveying and Land Information Science},
year={2005},
volume={65},
number={1},
pages={37-45},
note={cited By 57},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-20444451175&partnerID=40&md5=1650efb1b4a067f1be7528285bc8b49c},
abstract={In this study a multi-stage pattern recognition algorithm was developed to identify individual birds using images captured by a small unmanned aerial vehicle (UAV) equipped with a progressive scan video recorder. The developed algorithm utilizes correlation matching in addition to spectral characteristics of photographed birds. Individual images of flights over a wildlife management area and an agricultural area in southern Florida were tested. Omission and commission errors were mostly less than 20 percent in tested images and frequently less than 10 percent. Further efforts to develop the algorithms and automatically determine the thresholds used in the algorithm are suggested. A visual C++ Graphical User Interface (GUI) was developed to facilitate the implementation and use of the developed algorithm.},
}

@CONFERENCE{Yan2001176,
author={Yan, W.},
title={Fault detection and multi-classifier fusion for unmanned aerial vehicles (UAVs)},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2001},
volume={4385},
pages={176-186},
note={cited By 6},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-0034941678&doi=10.1117%2f12.421106&partnerID=40&md5=6edcd0fef550584e96fa13b1732f439d},
abstract={UAVs demand more accurate fault accommodation for their mission manager and vehicle control system in order to achieve a reliability level that is comparable to that of a piloted aircraft. This paper attempts to apply multi-classifier fusion techniques to achieve the necessary performance of the fault detection function for the Lockheed Martin Skunk Works (LMSW) UAV Mission Manager. Three different classifiers that meet the design requirements of the fault detection of the UAV are employed. The binary decision outputs from the classifiers are then aggregated using three different classifier fusion schemes, namely, majority vote, weighted majority vote, and Naïve Bayes combination. All of the three schemes are simple and need no retraining. The three fusion schemes (except the majority vote that gives an average performance of the three classifiers') show the classification performance that is better than or equal to that of the best individual. The unavoidable correlation between the classifiers with binary outputs is observed in this study. We conclude that it is the correlation between the classifiers that limits the fusion schemes to achieve an even better performance.},
}

@CONFERENCE{Magrabi2000363,
author={Magrabi, S.M. and Gibbens, P.W.},
title={Decentralized fault detection and diagnosis in navigation systems for unmanned aerial vehicles},
journal={Record - IEEE PLANS, Position Location and Navigation Symposium},
year={2000},
pages={363-370},
note={cited By 19},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-0033692420&partnerID=40&md5=6bb7083060aa89ddbac18c2d24edaa3c},
abstract={Autonomous Unmanned Aerial Vehicles (UAVs) are a recent technological phenomenon sweeping the world stage. Full autonomy implies that the guidance and navigation system employed must exhibit the highest level of integrity. This paper looks at the parity space Fault Detection and Diagnosis (FDD) methods its applicability in fully autonomous guidance and navigation systems in a decentralized system architecture. Using the existing work as a starting point this paper identifies the effectiveness of these methods when applied to situations where both the hardware and analytical redundancy exist. One of the most important issues in FDD in navigation systems using redundant sensors relates to the integrity of the solution processing architecture. Recently this has motivated the development of multiple FDD solutions running on numerous separate processors in a decentralized computing network. Typical solutions to this problem are based on decentralized or multiple Kalman Filters running in parallel. This paper will address the use and merits of the Information Filter form of the Kalman Filter in a fully decentralized FDD framework.},
}


==> DroneDetection.tex <==

@ARTICLE{Dogru2022,
author={Dogru, S. and Marques, L.},
title={Drone Detection Using Sparse Lidar Measurements},
journal={IEEE Robotics and Automation Letters},
year={2022},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85123733442&doi=10.1109%2fLRA.2022.3145498&partnerID=40&md5=282c72dcfaf610892885e653288869b1},
abstract={Unmanned aerial vehicles (UAV) have been serving people, fulfilling various roles in research, industry and military, not to exclude personal entertainment. They have also been in use more often for malicious purposes, such as annoying neighbors, disrupting air-travel, attacking people or infrastructure. Therefore, motivated particularly by malicious uses, the research community has been interested in proposing solutions for detection of UAVs. In this work we present a ground based aerial target detection system using lidars, relying on sparse detections rather than dense point clouds, with the aim of not only detecting but also estimating their motion and active tracking. We lay a theoretical groundwork to analyse the performance of such a lidar based detection system and help understanding its limitations. The work is complemented with field experiments utilizing a state-of-the-art lidar and several drones of different sizes, showing effectiveness in both detection and tracking using sparse measurements. IEEE},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Pulido2022149,
author={Pulido, C. and Ceron, A.},
title={Towards Real-Time Drone Detection Using Deep Neural Networks},
journal={Smart Innovation, Systems and Technologies},
year={2022},
volume={255},
pages={149-159},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85119370707&doi=10.1007%2f978-981-16-4884-7_12&partnerID=40&md5=0f3c279ba0d1e9d31ec6548a795ca686},
abstract={The growing use of drones/unmanned aerial vehicles (UAV’s) has generated in the general public as well as in institutions the awareness of the possible misuse that can be given to these devices. For this reason, the detection of drones has become a necessity that poses in the case of detection using images a great difficulty due to its small size, in addition to the background that can make detection even more difficult. Regarding this work, the aim is not only to detect drones but also to distinguish the type of detected drone. Different networks were trained whereupon an analysis was conducted in which it was found that the YOLOv4tiny network with 416 × 416 input resolution presents the best results considering both the inference performance and the processing speed. © 2022, The Author(s), under exclusive license to Springer Nature Singapore Pte Ltd.},
publisher={Springer Science and Business Media Deutschland GmbH},
}

@ARTICLE{Sazdić-Jotić2022,
author={Sazdić-Jotić, B. and Pokrajac, I. and Bajčetić, J. and Bondžulić, B. and Obradović, D.},
title={Single and multiple drones detection and identification using RF based deep learning algorithm},
journal={Expert Systems with Applications},
year={2022},
volume={187},
art_number={115928},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85115947866&doi=10.1016%2fj.eswa.2021.115928&partnerID=40&md5=c95b79c41e2dfce066bb0fc3ff0ae60b},
abstract={Unmanned aerial systems, especially drones have gone through remarkable improvement and expansion in recent years. Drones have been widely utilized in many applications and scenarios, due to their low price and ease of use. However, in some applications drones can pose a malicious threat. To diminish risks to public security and personal privacy, it is necessary to deploy an effective and affordable anti-drone system in sensitive areas to detect, localize, identify, and defend against intruding malicious drones. This research article presents a new publicly available radio frequency drone dataset and investigates detection and identification methodologies to detect single or multiple drones and identify a single detected drone's type. Moreover, special attention in this paper has been underlined to examine the possibility of using deep learning algorithms, particularly fully connected deep neural networks as an anti-drone solution within two different radio frequency bands. We proposed a supervised deep learning algorithm with fully-connected deep neural network models that use raw drone signals rather than features. Regarding the research results, the proposed algorithm shows a lot of potentials. The probability of detecting a single drone is 99.8%, and the probability of type identification is 96.1%. Moreover, the results of multiple drones detection demonstrate an average accuracy of 97.3%. There have not been such comprehensive publications, to this time, in the open literature that have presented and enlightened the problem of multiple drones detection in the radio frequency domain. © 2021 Elsevier Ltd},
publisher={Elsevier Ltd},
}

@ARTICLE{Svanström2021,
author={Svanström, F. and Alonso-Fernandez, F. and Englund, C.},
title={A dataset for multi-sensor drone detection},
journal={Data in Brief},
year={2021},
volume={39},
art_number={107521},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85118496043&doi=10.1016%2fj.dib.2021.107521&partnerID=40&md5=3095c62ee92cebbc5d775ac4f372c8a4},
abstract={The use of small and remotely controlled unmanned aerial vehicles (UAVs), referred to as drones, has increased dramatically in recent years, both for professional and recreative purposes. This goes in parallel with (intentional or unintentional) misuse episodes, with an evident threat to the safety of people or facilities [1]. As a result, the detection of UAV has also emerged as a research topic [2]. Most of the existing studies on drone detection fail to specify the type of acquisition device, the drone type, the detection range, or the employed dataset. The lack of proper UAV detection studies employing thermal infrared cameras is also acknowledged as an issue, despite its success in detecting other types of targets [2]. Beside, we have not found any previous study that addresses the detection task as a function of distance to the target. Sensor fusion is indicated as an open research issue as well to achieve better detection results in comparison to a single sensor, although research in this direction is scarce too [3–6]. To help in counteracting the mentioned issues and allow fundamental studies with a common public benchmark, we contribute with an annotated multi-sensor database for drone detection that includes infrared and visible videos and audio files. The database includes three different drones, a small-sized model (Hubsan H107D+), a medium-sized drone (DJI Flame Wheel in quadcopter configuration), and a performance-grade model (DJI Phantom 4 Pro). It also includes other flying objects that can be mistakenly detected as drones, such as birds, airplanes or helicopters. In addition to using several different sensors, the number of classes is higher than in previous studies [4]. The video part contains 650 infrared and visible videos (365 IR and 285 visible) of drones, birds, airplanes and helicopters. Each clip is of ten seconds, resulting in a total of 203,328 annotated frames. The database is complemented with 90 audio files of the classes drones, helicopters and background noise. To allow studies as a function of the sensor-to-target distance, the dataset is divided into three categories (Close, Medium, Distant) according to the industry-standard Detect, Recognize and Identify (DRI) requirements [7], built on the Johnson criteria [8]. Given that the drones must be flown within visual range due to regulations, the largest sensor-to-target distance for a drone in the dataset is 200 m, and acquisitions are made in daylight. The data has been obtained at three airports in Sweden: Halmstad Airport (IATA code: HAD/ICAO code: ESMT), Gothenburg City Airport (GSE/ESGP) and Malmö Airport (MMX/ESMS). The acquisition sensors are mounted on a pan-tilt platform that steers the cameras to the objects of interest. All sensors and the platform are controlled with a standard laptop vis a USB hub. © 2021},
publisher={Elsevier Inc.},
}

@ARTICLE{Ahmed202115,
author={Ahmed, T. and Rahman, T. and Roy, B.B. and Uddin, J.},
title={Drone Detection by Neural Network Using GLCM and SURF Features},
journal={Journal of Information Systems and Telecommunication},
year={2021},
volume={9},
number={33},
pages={15-23},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85104721682&doi=10.52547%2fjist.9.33.15&partnerID=40&md5=8fede080c0ed5e7b09138f001ae4bef9},
abstract={This paper presents a vision-based drone detection method. There are a number of researches on object detection which includes different feature extraction methods – all of those are used distinctly for the experiments. But in the proposed model, a hybrid feature extraction method using SURF and GLCM is used to detect object by Neural Network which has never been experimented before. Both are very popular ways of feature extraction. Speeded-up Robust Feature (SURF) is a blob detection algorithm which extracts the points of interest from an integral image, thus converts the image into a 2D vector. The Gray-Level Co-Occurrence Matrix (GLCM) calculates the number of occurrences of consecutive pixels in same spatial relationship and represents it in a new vector- 8 × 8 matrix of best possible attributes of an image. SURF is a popular method of feature extraction and fast matching of images, whereas, GLCM method extracts the best attributes of the images. In the proposed model, the images were processed first to fit our feature extraction methods, then the SURF method was implemented to extract the features from those images into a 2D vector. Then for our next step GLCM was implemented which extracted the best possible features out of the previous vector, into a 8 × 8 matrix. Thus, image is processed in to a 2D vector and feature extracted from the combination of both SURF and GLCM methods ensures the quality of the training dataset by not just extracting features faster (with SURF) but also extracting the best of the point of interests (with GLCM). The extracted featured related to the pattern are used in the neural network for training and testing. Pattern recognition algorithm has been used as a machine learning tool for the training and testing of the model. In the experimental evaluation, the performance of proposed model is examined by cross entropy for each instance and percentage error. For the tested drone dataset, experimental results demonstrate improved performance over the state-of-art models by exhibiting less cross entropy and percentage error. © 2021. All Rights Reserved.},
publisher={Iranian Academic Center for Education, Culture and Research},
}

@ARTICLE{Lee202134237,
author={Lee, D.-H.},
title={CNN-based single object detection and tracking in videos and its application to drone detection},
journal={Multimedia Tools and Applications},
year={2021},
volume={80},
number={26-27},
pages={34237-34248},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85092404216&doi=10.1007%2fs11042-020-09924-0&partnerID=40&md5=bbf486a15020d78496728649fd80ee40},
abstract={This paper presents convolutional neural network (CNN)-based single object detection and tracking algorithms. CNN-based object detection methods are directly applicable to static images, but not to videos. On the other hand, model-free visual object tracking methods cannot detect an object until a ground truth bounding box of the target is provided. Moreover, many annotated video datasets of the target object are required to train both the object detectors and visual trackers. In this work, three simple yet effective object detection and tracking algorithms for videos are proposed to efficiently combine a state-of-the-art object detector and visual tracker for circumstances in which only a few static images of the target are available for training. The proposed algorithms are tested using a drone detection task and the experimental results demonstrated their effectiveness. © 2020, Springer Science+Business Media, LLC, part of Springer Nature.},
publisher={Springer},
}

@ARTICLE{Çetin20211871,
author={Çetin, E. and Barrado, C. and Pastor, E.},
title={Improving real-time drone detection for counter-drone systems},
journal={Aeronautical Journal},
year={2021},
volume={125},
number={1292},
pages={1871-1896},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85108189175&doi=10.1017%2faer.2021.43&partnerID=40&md5=698c9eeb9733033b6a86279c6ba0848a},
abstract={The number of unmanned aerial vehicles (UAVs, also known as drones) has increased dramatically in the airspace worldwide for tasks such as surveillance, reconnaissance, shipping and delivery. However, a small number of them, acting maliciously, can raise many security risks. Recent Artificial Intelligence (AI) capabilities for object detection can be very useful for the identification and classification of drones flying in the airspace and, in particular, are a good solution against malicious drones. A number of counter-drone solutions are being developed, but the cost of drone detection ground systems can also be very high, depending on the number of sensors deployed and powerful fusion algorithms. We propose a low-cost counter-drone solution composed uniquely by a guard-drone that should be able to detect, locate and eliminate any malicious drone. In this paper, a state-of-the-art object detection algorithm is used to train the system to detect drones. Three existing object detection models are improved by transfer learning and tested for real-time drone detection. Training is done with a new dataset of drone images, constructed automatically from a very realistic flight simulator. While flying, the guard-drone captures random images of the area, while at the same time, a malicious drone is flying too. The drone images are auto-labelled using the location and attitude information available in the simulator for both drones. The world coordinates for the malicious drone position must then be projected into image pixel coordinates. The training and test results show a minimum accuracy improvement of 22% with respect to state-of-the-art object detection models, representing promising results that enable a step towards the construction of a fully autonomous counter-drone system. © 2021 The Author(s). Published by Cambridge University Press on behalf of Royal Aeronautical Society.},
publisher={Cambridge University Press},
}

@CONFERENCE{Makirin2021,
author={Makirin, M.K. and Wastupranata, L.M. and Daffa, A.},
title={Onboard visual drone detection for drone chasing and collision avoidance},
journal={AIP Conference Proceedings},
year={2021},
volume={2366},
art_number={060013},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85115313401&doi=10.1063%2f5.0059987&partnerID=40&md5=2d14f42d526c07a40aea73af21a0c2a4},
abstract={We proposed a method for real-time detection of flying drones and UAVs that could be run with a limited computing device like an onboard computer for a drone. This method is approached from a machine learning perspective resulting in an object detection model to detect and localize multiple drones in a given image. The constraint is that the model will have to be lightweight and performant while still maintaining good accuracy. This leads us to choose SSD Mobilenet V2 model architecture to train and test how effective it is for detecting drones. Our method gained an average precision and recall of 0.586 and 0.622 (IoU 0.50-0.95, all area) respectively. © 2021 Author(s).},
publisher={American Institute of Physics Inc.},
}

@ARTICLE{Singha2021,
author={Singha, S. and Aydin, B.},
title={Automated drone detection using YOLOv4},
journal={Drones},
year={2021},
volume={5},
number={3},
art_number={95},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85115638681&doi=10.3390%2fdrones5030095&partnerID=40&md5=602ae52700c39773ff1ac0752b1e828d},
abstract={Drones are increasing in popularity and are reaching the public faster than ever before. Consequently, the chances of a drone being misused are multiplying. Automated drone detection is necessary to prevent unauthorized and unwanted drone interventions. In this research, we designed an automated drone detection system using YOLOv4. The model was trained using drone and bird datasets. We then evaluated the trained YOLOv4 model on the testing dataset, using mean average precision (mAP), frames per second (FPS), precision, recall, and F1-score as evaluation parameters. We next collected our own two types of drone videos, performed drone detections, and calculated the FPS to identify the speed of detection at three altitudes. Our methodology showed better performance than what has been found in previous similar studies, achieving a mAP of 74.36%, precision of 0.95, recall of 0.68, and F1-score of 0.79. For video detection, we achieved an FPS of 20.5 on the DJI Phantom III and an FPS of 19.0 on the DJI Mavic Pro. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
publisher={MDPI},
}

@ARTICLE{Al-Emadi2021,
author={Al-Emadi, S. and Al-Ali, A. and Al-Ali, A.},
title={Audio-based drone detection and identification using deep learning techniques with dataset enhancement through generative adversarial networks†},
journal={Sensors},
year={2021},
volume={21},
number={15},
art_number={4953},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85110553859&doi=10.3390%2fs21154953&partnerID=40&md5=eb11d513250c12d3519843b4337ea665},
abstract={Drones are becoming increasingly popular not only for recreational purposes but in day-to-day applications in engineering, medicine, logistics, security and others. In addition to their useful applications, an alarming concern in regard to the physical infrastructure security, safety and privacy has arisen due to the potential of their use in malicious activities. To address this problem, we propose a novel solution that automates the drone detection and identification processes using a drone’s acoustic features with different deep learning algorithms. However, the lack of acoustic drone datasets hinders the ability to implement an effective solution. In this paper, we aim to fill this gap by introducing a hybrid drone acoustic dataset composed of recorded drone audio clips and artificially generated drone audio samples using a state-of-the-art deep learning technique known as the Generative Adversarial Network. Furthermore, we examine the effectiveness of using drone audio with different deep learning algorithms, namely, the Convolutional Neural Network, the Recurrent Neural Network and the Convolutional Recurrent Neural Network in drone detection and identification. Moreover, we investigate the impact of our proposed hybrid dataset in drone detection. Our findings prove the advantage of using deep learning techniques for drone detection and identification while confirming our hypothesis on the benefits of using the Generative Adversarial Networks to generate real-like drone audio clips with an aim of enhancing the detection of new and unfamiliar drones. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
publisher={MDPI AG},
}

@CONFERENCE{Dani20211538,
author={Dani, R.R. and Kubde, R.R. and Sadhu, M.A.},
title={A Comprehensive Study of Various Techniques for Hostile Drone Detection and Their Classification},
journal={Proceedings of the 6th International Conference on Communication and Electronics Systems, ICCES 2021},
year={2021},
pages={1538-1543},
art_number={9489236},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113736789&doi=10.1109%2fICCES51350.2021.9489236&partnerID=40&md5=5721bb2749696013d9d3f8d0b6326704},
abstract={Today's atmosphere is being increasingly congested due to the proliferation of airborne objects such as small airplanes, helicopters, and unmanned aerial vehicles (drones) of varying forms and sizes. The UAVs can also become a major threat as they can be utilized in smuggling, industrial spy, robbery, and terrorism, besides enabling access to new technologies. Owing to its speed, agility, and altitude, it is hard to defend against a UAV incursion. Aerial defence systems are integrated with a wide range of sensors to efficiently track aircraft. There are several methods and techniques discussed in this paper that are ideal for this specific application. This paper also discusses the paradigm of drone detection using Radar and Imaging techniques and the classification of drones based on their size, features, flying height, and Unique Identification Number (UIN). © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Yang2021760,
author={Yang, F. and Xu, F. and Fioranelli, F. and Le Kernec, J. and Chang, S. and Long, T.},
title={Practical Investigation of a MIMO radar system capabilities for small drones detection},
journal={IET Radar, Sonar and Navigation},
year={2021},
volume={15},
number={7},
pages={760-774},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85104836532&doi=10.1049%2frsn2.12082&partnerID=40&md5=9059635bb87c5a1b766d7277672794a1},
abstract={The latest progress of the multiple-input multiple-output (MIMO) radar system developed for small drones detection at Beijing Institute of Technology is presented herein. A low-cost S-band MIMO scanning radar system is designed for the detection of small drones. A practical design optimisation and implementation of a sparse array covering the whole airspace, and a target-based MIMO radar array calibration method to improve the signal-to-noise ratio of the target are proposed. An experiment in the microwave chamber was conducted to verify the designed sparse-array beam-pattern, and measurement campaigns for small drones were performed to test the system performance where the radar achieved detection and tracking of a small DJI-Phantom 4 drone at a range of up to 5 km. Target features, including micro-Doppler and radar cross-section signatures were extracted to assist target classification. The experimental results indicate that the system has promising capability in small drones detection and tracking, despite the challenges of low dwell time on targets due to the scanning nature of the system. © 2021 The Authors. IET Radar, Sonar & Navigation published by John Wiley & Sons Ltd on behalf of The Institution of Engineering and Technology.},
publisher={John Wiley and Sons Inc},
}

@CONFERENCE{Mata-Moya2021,
author={Mata-Moya, D. and Rey-Maestre, N. and Gomez-Del-Hoyo, P.-J. and Rosado-Sanz, J. and Jarabo-Amores, M.-P.},
title={4D Passive Radar for Drone Detection and Tracking},
journal={Proceedings International Radar Symposium},
year={2021},
volume={2021-June},
art_number={9466190},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113909664&doi=10.23919%2fIRS51887.2021.9466190&partnerID=40&md5=e67a24dcd11615c34f7328241811abcc},
abstract={An upgraded version of IDEPAR demonstrator capable of detecting and extracting parameters from targets in a 4D measurements space(range, Doppler, azimuth and elevation) is presented to allow the localization of small aerial drones in the Cartesian space (x,y,z). A two-stage spatial filtering processing scheme based on a 2D reception antenna system provides target's directions of arrival (azimuth, elevation) for targets' localization in the Cartesian space. The PR system was validated in measurement campaigns using small drones confirming the location capabilities of the proposed approach. © 2021 German Institute of Navigation (DGON).},
publisher={IEEE Computer Society},
}

@CONFERENCE{Schneebeli2021,
author={Schneebeli, M. and Leuenberger, A. and Wabeke, L. and Kloke, K. and Kitching, C. and Siegenthaler, U. and Wellig, P.},
title={Drone detection with a multistatic C-band radar},
journal={Proceedings International Radar Symposium},
year={2021},
volume={2021-June},
art_number={9466200},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113895167&doi=10.23919%2fIRS51887.2021.9466200&partnerID=40&md5=e6cc8deb5e496d99af09971908d475bd},
abstract={The multistatic active surveillance radar system SAMURAI (Swiss African MUltistatic RAdar Initiative) was tested on its drone detection capabilities during two field campaigns in Switzerland. The C-band system, consisting of one transmit and two receive nodes, was geometrically and radiometrically calibrated with a specific multistatic target simulator. GPS trajectories of a DJI Phantom 4 drone were compared to the radar detections. It was found that the radar system's inherent pointing angle and range biases can be corrected in a straightforward manner by using the virtually generated radar targets as a reference. After the corrections were applied to the radar data, deviations between the drone's GPS position and the radar detections on the order of 5 m were found. © 2021 German Institute of Navigation (DGON).},
publisher={IEEE Computer Society},
}

@CONFERENCE{Rahman2021,
author={Rahman, S. and Robertson, D.A.},
title={FAROS-E: A compact and low-cost millimeter wave surveillance radar for real time drone detection and classification},
journal={Proceedings International Radar Symposium},
year={2021},
volume={2021-June},
art_number={9466175},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113891659&doi=10.23919%2fIRS51887.2021.9466175&partnerID=40&md5=d58bd0d201b911b6e01cdeaa5effa6a8},
abstract={This paper describes the system architecture and performance of the FAROS-E 77 GHz radar designed and built at the University of St Andrews for real time drone detection and classification (drone vs non-drone). The motivation behind the system is to demonstrate a highly reliable drone classification sensor for security surveillance in a compact, low-cost and potentially portable form factor. The low phase noise, coherent architecture exploits the high Doppler sensitivity available at millimeter wave frequencies, to enable robust micro-Doppler signature analysis and classification. Outdoor trials of FAROS-E have yielded high fidelity data and shown very promising results as a short-range system capable of detecting a DJI Phantom Standard 3 up to 300 m and classifying it up to 150m. The classification algorithm is capable of classifying the presence of a drone even when it is hovering stationary. © 2021 German Institute of Navigation (DGON).},
publisher={IEEE Computer Society},
}

@CONFERENCE{Heidger2021,
author={Heidger, R. and Lambercy, V. and Lambers, D.},
title={Tracking Analysis of Drone Detection Systems at Airports: Methodology and Results},
journal={Proceedings International Radar Symposium},
year={2021},
volume={2021-June},
art_number={9466192},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113871508&doi=10.23919%2fIRS51887.2021.9466192&partnerID=40&md5=c7bcded901564f2e3ebd6454725f2049},
abstract={This paper describes the methodology that has been established in the DFS to test Drone Detection Systems (DDS) at airports, as well as the global test results of the test campaign conducted at Frankfurt and Munich airports in summer and autumn 2020 together with Fraport and FMG. The test campaign was part of a feasibility study to evaluate, what small noncooperative UAS current DDS systems today can detect and track at large infrastructures like airports, and which limitations exist. © 2021 German Institute of Navigation (DGON).},
publisher={IEEE Computer Society},
}

@CONFERENCE{Ciesielski2021,
author={Ciesielski, M. and Stasiak, K. and Khyzhniak, M. and Jedrzejewski, K. and Zywek, M. and Brawata, S.},
title={Simultaneous Signal Processing with Multiple Coherent Processing Intervals in FMCW Radar for Drone Detection},
journal={Proceedings International Radar Symposium},
year={2021},
volume={2021-June},
art_number={9466232},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113850556&doi=10.23919%2fIRS51887.2021.9466232&partnerID=40&md5=9e780ebf8e7082c052f4df32d2a82fba},
abstract={The paper presents research on using multiple signal processors operating simultaneously with different coherent processing intervals. The papers focuses on considerations related to drone detection. Theoretical analysis of the problems arising in FMCW radars is provided and a solution utilizing multiple signal processors is proposed. Results of field trials are also presented. © 2021 German Institute of Navigation (DGON).},
publisher={IEEE Computer Society},
}

@CONFERENCE{Kabir2021,
author={Kabir, M.S. and Ndukwe, I.K. and Awan, E.Z.S.},
title={Deep Learning Inspired Vision based Frameworks for Drone Detection},
journal={3rd International Conference on Electrical, Communication and Computer Engineering, ICECCE 2021},
year={2021},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85115062215&doi=10.1109%2fICECCE52056.2021.9514124&partnerID=40&md5=3cf17f66190f9c86745bfaf6f4c60e7c},
abstract={Drone detection technology is a new frontier in defence systems. With increasing incidences of crimes and terroristic attacks using commercial drones, detection of unauthorized drones is critical for timely responses from law enforcement agencies. In this paper, the issues of unavailability of benchmark dataset and performance metrics for drone detection are addressed and three single shot detectors, based on YOLOv4, YOLOv5 and DETR architectures are presented. A maximum of 99% average precision (AP) with an average Intersection over Union (IOU) of 84% was achieved. The precision-recall curves corroborate the generalization and fitness of the trained detection models. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Zhang202123723,
author={Zhang, X. and Kusrini, K.},
title={Autonomous long-range drone detection system for critical infrastructure safety},
journal={Multimedia Tools and Applications},
year={2021},
volume={80},
number={15},
pages={23723-23743},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85101035500&doi=10.1007%2fs11042-020-10231-x&partnerID=40&md5=99c60df7dbad429c0b51661887d685fb},
abstract={The development of unmanned aerial vehicles has been identified as a potential source of a weapon for causing operational disruptions against critical infrastructures. To mitigate and neutralise the threat posed by the misuse of drones against malicious and terrorist activity, this paper presents a holistic design of a long-range autonomous drone detection platform. The novelty of the proposed system lies in the confluence between the design of hardware and software components to effective and efficient localisation of the intruder objects. The research presented in the paper proposes the design and validation of a situation awareness component which is interfaced with the hardware component for controlling the focal length of the camera. The continuous stream of media data obtained from the region of vulnerability is processed using the object detection that is built on region based fully connected neural network. The novelty of the proposed system relies on the processing of multi-threaded dual-media input streams that are evaluated to mitigate the latency of the system. Upon the successful detection of malicious drones, the system logs the occurrence of intruders that consists of both event description and the associated media evidence for the deployment of the mitigation strategy. The analytics platform that controls the signalling of the low-cost sensing equipment contains the NVIDIA GeForce GTX 1080 for detecting drones. The experimental testbeds developed for the validation of the proposed system has been constructed to include environments and situations that are commonly faced by critical infrastructure operators such as the area of protection, drone flight path, tradeoff between the angle of coverage against the distance of coverage. The validation of the proposed system has resulted in yielding a range of intruder drone detection by 250m with an accuracy of 95.5%. © 2021, The Author(s).},
publisher={Springer},
}

@CONFERENCE{Zhang2021,
author={Zhang, Y.D. and Xiang, X. and Li, Y. and Chen, G.},
title={Enhanced Micro-Doppler Feature Analysis for Drone Detection},
journal={IEEE National Radar Conference - Proceedings},
year={2021},
volume={2021-May},
art_number={9455228},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85112467486&doi=10.1109%2fRadarConf2147009.2021.9455228&partnerID=40&md5=eb65a4bbd8504c310b70b9a6083bc6c4},
abstract={As low-cost drones become more accessible, they pose various safety, security, and privacy threats. As such, it becomes increasingly important to detect their presence, locate and track their positions, and classify their types in real time. In this paper, we perform time-frequency analyses of drone Doppler and micro-Doppler signatures to provide enhanced drone detection and feature extraction capabilities. The analyses are based on the combined use of spectrogram and inverse Radon transform (IRT). The paired property of propeller blades associated with a rotor is further utilized to compute the IRT product for enhanced performance. It is demonstrated that the IRT and IRT product images, when expressed in terms of the rotation frequency and blade position phase, provide flexibility and effectiveness for the presentation and estimation of these parameters. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Blake2021,
author={Blake, W. and Burger, I.},
title={Small Drone Detection Using Airborne Weather Radar},
journal={IEEE National Radar Conference - Proceedings},
year={2021},
volume={2021-May},
art_number={9455224},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85112409525&doi=10.1109%2fRadarConf2147009.2021.9455224&partnerID=40&md5=6c477d1199d71ab2451eb461315f8b23},
abstract={As small commercial and hobby drones increase in popularity, there is a desire to monitor and avoid these drones. This paper focuses on how small drones such as the DJI Phantom 3 and DJI Inspire could be detected using existing weather radar hardware already installed in many airplanes. Garmin's GWX 80 airborne weather radar was used to demonstrate this potential. Only software modifications were made to the aviation certified hardware for the feasibility of this approach. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Liu2021,
author={Liu, H. and Fan, K. and Ouyang, Q. and Li, N.},
title={Real-time small drones detection based on pruned yolov4},
journal={Sensors},
year={2021},
volume={21},
number={10},
art_number={3374},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85105444029&doi=10.3390%2fs21103374&partnerID=40&md5=b5524dee7146413d58000b027561cc5b},
abstract={To address the threat of drones intruding into high-security areas, the real-time detection of drones is urgently required to protect these areas. There are two main difficulties in real-time detection of drones. One of them is that the drones move quickly, which leads to requiring faster detectors. Another problem is that small drones are difficult to detect. In this paper, firstly, we achieve high detection accuracy by evaluating three state-of-the-art object detection methods: RetinaNet, FCOS, YOLOv3 and YOLOv4. Then, to address the first problem, we prune the convolutional channel and shortcut layer of YOLOv4 to develop thinner and shallower models. Furthermore, to improve the accuracy of small drone detection, we implement a special augmentation for small object detection by copying and pasting small drones. Experimental results verify that compared to YOLOv4, our pruned-YOLOv4 model, with 0.8 channel prune rate and 24 layers prune, achieves 90.5% mAP and its processing speed is increased by 60.4%. Additionally, after small object augmentation, the precision and recall of the pruned-YOLOv4 almost increases by 22.8% and 12.7%, respectively. Experiment results verify that our pruned-YOLOv4 is an effective and accurate approach for drone detection. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
publisher={MDPI AG},
}

@ARTICLE{Beranek2021260,
author={Beranek, C.T. and Roff, A. and Denholm, B. and Howell, L.G. and Witt, R.R.},
title={Trialling a real-time drone detection and validation protocol for the koala (Phascolarctos cinereus)},
journal={Australian Mammalogy},
year={2021},
volume={43},
number={2},
pages={260-264},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85087788781&doi=10.1071%2fAM20043&partnerID=40&md5=1030cd895d14b4daa182b277c7349103},
abstract={Remotely piloted aircraft system (RPAS), or drone, technology has emerged as a promising survey method for the cryptic koala. We demonstrate an in-field protocol for wild koala RPAS surveys which provides real-time validation of thermal signatures. During 15 trial flights using a quadcopter drone (DJI Matrice 200 v2) we successfully detected and validated koala thermal signatures (n = 12) using two in-field approaches: Validation by on-ground observer (n = 10) and validation using 4K footage captured and reviewed directly after the survey (n = 2). We also provide detectability considerations relative to survey time, temperature, wildlife-RPAS interactions and detection of non-target species, which can be used to further inform RPAS survey protocols. © 2021 CSIRO. All rights reserved.},
publisher={CSIRO},
}

@CONFERENCE{Teo2021875,
author={Teo, M.I. and Seow, C.K. and Wen, K.},
title={5G Radar and Wi-Fi Based Machine Learning on Drone Detection and Localization},
journal={2021 IEEE 6th International Conference on Computer and Communication Systems, ICCCS 2021},
year={2021},
pages={875-880},
art_number={9449224},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113335396&doi=10.1109%2fICCCS52626.2021.9449224&partnerID=40&md5=290e39f9f3d074ead5638d921ba479d4},
abstract={Drone usages have been proliferating for various government initiatives, commercial benefits and civilian leisure purposes. Drone mismanagement especially civilian usage drones can easily expose threat and vulnerability of the Government Public Key Infrastructures (PKI) that hold crucial operations, affecting the survival and economic of the country. As such, detection and location identification of these drones are crucial immediately prior to their payload action. Existing drone detection solutions are bulky, expensive and hard to setup in real time. With the advent of 5G and Internet of Things (IoT), this paper proposes a cost effective bistatic radar solution that leverages on 5G cellular spectrum to detect the presence and localize the drone. Coupled with K-Nearest Neighbours (KNN) Machine Learning (ML) algorithm, the features of Non- Line of Sight (NLOS) transmissions by 5G radar and Received Signal Strength Indicator (RSSI) emitted by drone are used to predict the location of the drone. The proposed 5G radar solution can detect the presence of a drone in both outdoor and indoor environment with accuracy of 100%. Furthermore, it can localize the drone with an accuracy of up to 75%. These results have shown that a cost effective radar machine learning system, operating on the 5G cellular network spectrum can be developed to successfully identify and locate a drone in real-time. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Trapal2021162,
author={Trapal, D.D.C. and Leong, B.C.C. and Ng, H.W. and Zhong, J.T.G. and Srigrarom, S. and Chan, T.H.},
title={Improvement of Vision-based Drone Detection and Tracking by Removing Cluttered Background, Shadow and Water Reflection with Super Resolution},
journal={2021 6th International Conference on Control and Robotics Engineering, ICCRE 2021},
year={2021},
pages={162-168},
art_number={9435671},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85107773816&doi=10.1109%2fICCRE51898.2021.9435671&partnerID=40&md5=6acf92e6bf850762c7b7e6875c5e5303},
abstract={Detection and tracking of small and fast moving aerial targets especially drones has got attention nowadays. This paper focuses on the vision-based technique using images taken from observing cameras. In real life situations, the target drone objects maybe are hidden in the cluttered background such as trees shadow or foliage, rows of buildings, and other kind of scenery that will hinder the clear indication of the drones. The object is further confused by the presence of its shadow and reflection from the water or glass wall reflection. For vision-based objection, the clarity and the ambiguity of the target images in the video stream are the key for effective and successful target detection and tracking. Here, we present the improvement by mitigating the effect of cluttered background, shadow and water reflection to the target images. We applied the schemes to make the drone more visible and more clear. We also implemented super resolution to increase the image resolution for more precise detection and tracking. As a result, the target drone could be detected and tracked throughout the sample clips. The comparative tracking results using DCF are presented. Likewise, we applied the water removal scheme to eliminate the reflection to avoid confusion to the tracker. With this, just the correct drone targets were detected and tracked. Overall, the drones could be detected and tracked all the way, as long as they appeared in the camera scene. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Aledhari2021,
author={Aledhari, M. and Razzak, R. and Parizi, R.M. and Srivastava, G.},
title={Sensor Fusion for Drone Detection},
journal={IEEE Vehicular Technology Conference},
year={2021},
volume={2021-April},
art_number={9448699},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85112401473&doi=10.1109%2fVTC2021-Spring51267.2021.9448699&partnerID=40&md5=2d1ddefc7484a1fa71b3b18e8bd9500b},
abstract={With the rapid development of commercial drones, drone detection and classification have emerged and grown recently. Drone detection works to detect unmanned aerial vehicles (UAVs). Usually, systems for drone detection utilize a combination of one or more sensors and some methodology. Many unique technologies and methods are used to detect drones. However, each type of technology offers its benefits and limitations. Most approaches use computer vision or machine learning, but one methodology that has not been given much attention is Sensor Fusion. Sensor Fusion has less uncertainty than most methods, making it suitable for drone detection. In this paper, we propose an artificial neural network-based detection system that uses a deep neural network (DNN) to process the RF data and a convolutional neural network (CNN) to process image data. The features from CNNs and DNNs are concatenated and input into another DNN, which outputs a single prediction score of drone presence. Our model achieved a validation accuracy of 75% that shows the feasibility of a sensor fusion based technique for drone detection. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Kolamunna2021,
author={Kolamunna, H. and Dahanayaka, T. and Li, J. and Seneviratne, S. and Thilakaratne, K. and Zomaya, A.Y. and Seneviratne, A.},
title={DronePrint: Acoustic Signatures for Open-set Drone Detection and Identification with Online Data},
journal={Proceedings of the ACM on Interactive, Mobile, Wearable and Ubiquitous Technologies},
year={2021},
volume={5},
number={1},
art_number={3448115},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85103617755&doi=10.1145%2f3448115&partnerID=40&md5=17c6a7cfc90ea02b91d25045125725cc},
abstract={With the ubiquitous availability of drones, they are adopted benignly in multiple applications such as cinematography, surveying, and legal goods delivery. Nonetheless, they are also being used for reconnaissance, invading personal or secure spaces, harming targeted individuals, smuggling drugs and contraband, or creating public disturbances. These malicious or improper use of drones can pose significant privacy and security threats in both civilian and military settings. Therefore, it is vital to identify drones in different environments to assist the decisions on whether or not to contain unknown drones. While there are several methods proposed for detecting the presence of a drone, they have limitations when it comes to low visibility, limited access, or hostile environments. In this paper, we propose DronePrint that uses drone acoustic signatures to detect the presence of a drone and identify the make and the model of the drone. We address the shortage of drone acoustic data by relying on audio components of online videos. In drone detection, we achieved 96% accuracy in a closed-set scenario, and 86% accuracy in a more challenging open-set scenario. Our proposed method of cascaded drone identification, where a drone is identified for its 'make' followed by the 'model' of the drone achieves 90% overall accuracy. In this work, we cover 13 commonly used commercial and consumer drone models, which is to the best of understanding is the most comprehensive such study to date. Finally, we demonstrate the robustness of DronePrint to drone hardware modifications, Doppler effect, varying SNR conditions, and in realistic open-set acoustic scenes. © 2021 ACM.},
publisher={Association for Computing Machinery},
}

@CONFERENCE{Geschke2021,
author={Geschke, R.H. and Shoykhetbrod, A. and Brauns, R. and Schwabig, C. and Wickmann, S. and Leuchs, S. and Krebs, C. and Kuter, A. and Nussler, D.},
title={Post-integration Antenna Characterisation for a V-band Drone-detection Radar},
journal={15th European Conference on Antennas and Propagation, EuCAP 2021},
year={2021},
art_number={9411016},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85105435735&doi=10.23919%2fEuCAP51087.2021.9411016&partnerID=40&md5=2a66042adf9bf39ea6362b11b64d0a53},
abstract={A drone detection FMCW radar operating from 57 to 64 GHz band has one transmit and two receiving fan-beam antennas. Due to the close integration of the system and enclosure, aspects related to board layout such as direct transmitter antenna to receiver antenna coupling and packaging effects reduce the antenna beamwidths and may reduce antenna efficiency. Post-integration diagnostic methods are presented to test the antenna system performance. The concept of a combined transmit-receive radiation pattern in combination with a large planar reflector is introduced and used to characterise radar fan-beam antenna patterns. The system is used as an uncalibrated network analyser to characterise the two fan-beam pairs with the influence of the packaging included. © 2021 EurAAP.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Park20211791,
author={Park, J. and Park, J.-S. and Bae, K.-B. and Park, S.-O.},
title={Advanced Stationary Point Concentration Technique for Leakage Mitigation and Small Drone Detection with FMCW Radar},
journal={IEEE Transactions on Microwave Theory and Techniques},
year={2021},
volume={69},
number={3},
pages={1791-1804},
art_number={9339993},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85100510402&doi=10.1109%2fTMTT.2021.3052190&partnerID=40&md5=8616002a9e13d4e1d87fc5836f8de3b0},
abstract={With the increase in threats posed by small drones, the development of radars to detect such drones has become a key necessity. In earlier studies, we proposed the stationary point concentration (SPC) technique for small drone detection using frequency-modulated continuous-wave (FMCW) radar. The SPC technique is a novel approach for mitigating leakage, which is an inherent problem in FMCW radar. The SPC technique improves the signal-to-noise ratio of small drones by reducing the noise floor and provides accurate distance and velocity information of such drones. However, this technique has shortcomings in its realization. In this article, we present the drawbacks of this technique and propose an advanced SPC (A-SPC) technique. The proposed technique can overcome the drawbacks of the SPC technique while implementing the benefits of the SPC technique. The experimental results verify the proposed A-SPC technique and demonstrate its robustness and usefulness. © 1963-2012 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Park2021737,
author={Park, J. and Park, S.-O.},
title={Improved drone detection in FMCW Radar using SPC Technique (invited talk)},
journal={2020 International Symposium on Antennas and Propagation, ISAP 2020},
year={2021},
pages={737-738},
art_number={9391464},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85104500313&doi=10.23919%2fISAP47053.2021.9391464&partnerID=40&md5=ad5f4c51ae22da60f40fcabd76a5111b},
abstract={This paper introduces the stationary point concentration (SPC) technique, one of the state-of-the-art techniques for detecting small drones with frequency modulated continuous wave radars. A novel approach of the SPC technique is explained, and representative experimental results are shown. Finally, the promising potentials of the SPC technique are discussed. © 2021 IEICE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Semkin2021223,
author={Semkin, V. and Yin, M. and Hu, Y. and Mezzavilla, M. and Rangan, S.},
title={Drone detection and classification based on radar cross section signatures},
journal={2020 International Symposium on Antennas and Propagation, ISAP 2020},
year={2021},
pages={223-224},
art_number={9391260},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85104496955&doi=10.23919%2fISAP47053.2021.9391260&partnerID=40&md5=13b4bfa36a5b409fa9fb27b354392e10},
abstract={In this work, we show how drone detection and classification can be enabled by leveraging a database of radar cross section (RCS) signatures. First, we present a set of measurement results of the RCS of a carbon fiber drone model at 28 GHz. The measurements were performed in an anechoic chamber and provide essential information about the RCS signature of the specific drone. Then, we assess the RCS-based detection probability and the range error by running simulations in urban environments. The drones were positioned at different distances, from 30m to 90m, and the RCS signatures used for the detection and classification were obtained experimentally. © 2021 IEICE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Ohlenbusch20216,
author={Ohlenbusch, M. and Ahrens, A. and Rollwage, C. and Bitzer, J.},
title={Robust drone detection for acoustic monitoring applications},
journal={European Signal Processing Conference},
year={2021},
volume={2021-January},
pages={6-10},
art_number={9287433},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85099318868&doi=10.23919%2fEusipco47968.2020.9287433&partnerID=40&md5=c3e7331f08ab67dc49eb5f292ac2e8e2},
abstract={Commercially available light-weight unmanned aerial vehicles (UAVs) present a challenge for public safety, e.g. espionage, transporting dangerous goods or devices. Therefore, countermeasures are necessary. Usually, detection of UAVs is a first step. Along many other modalities, acoustic detection seems promising. Recent publications show interesting results by using machine and deep learning methods. The acoustic detection of UAVs appears to be particularly difficult in adverse situations, such as in heavy wind noise or in the presence of construction noise. In this contribution, the typical feature set is extended to increase separation of background noise and the UAV signature noise. The decision algorithm utilized is support vector machine (SVM) classification. The classification is based on an extended training dataset labeled to support binary classification. The proposed method is evaluated in comparison to previously published algorithms, on the basis of a dataset recorded from different acoustic environments, including unknown UAV types. The results show an improvement over existing methods, especially in terms of false-positive detection rate. For a first step into real-time embedded systems a recursive feature elimination method is applied to reduce the model dimensionality. The results indicate only a slight decreases in detection performance. © 2021 European Signal Processing Conference, EUSIPCO. All rights reserved.},
publisher={European Signal Processing Conference, EUSIPCO},
}

@CONFERENCE{Srigrarom2021,
author={Srigrarom, S. and Sie, N.J.L. and Cheng, H. and Chew, K.H. and Lee, M. and Ratsamee, P.},
title={Multi-camera Multi-drone Detection, Tracking and Localization with Trajectory-based Re-identification},
journal={2021 2nd International Symposium on Instrumentation, Control, Artificial Intelligence, and Robotics, ICA-SYMP 2021},
year={2021},
art_number={9358454},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85102508687&doi=10.1109%2fICA-SYMP50206.2021.9358454&partnerID=40&md5=252f23d2f6e3c6adbfd8d8fc6b3dd48c},
abstract={This paper presents a real-time multiple camera system for detecting, tracking and localizing multiple moving drones simultaneously in a 3 dimension space. The distinct feature of the system is in its target re-identification process, which provides for information fusion among cameras based on the targets' trajectories and relative locations. Drones are detected by the multiple camera system based on motion-based blob detection, and the 2D locations of each drone in individual camera frames are tracked by A geometry- and camera-based model. From the paths of the tracked drones, their trajectories are examined using drone track feature variable. Cross-correlated among cameras for object re-identifications will allow the individual 2D position information to be integrated into overall global 3D positions of all the tracked drones from all cameras. Preliminary outdoor flight demonstrations with 2 drones flying in formation and using 3 cameras show optimal results. The system is able to detect, track, localize and re-identifying individual drone with average positional error of 8%. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{WeiXun2021,
author={Wei Xun, D.T. and Lim, Y.L. and Srigrarom, S.},
title={Drone detection using YOLOv3 with transfer learning on NVIDIA Jetson TX2},
journal={2021 2nd International Symposium on Instrumentation, Control, Artificial Intelligence, and Robotics, ICA-SYMP 2021},
year={2021},
art_number={9358449},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85102488569&doi=10.1109%2fICA-SYMP50206.2021.9358449&partnerID=40&md5=ae6ad5ae58b864696f708b4e20c4432b},
abstract={The rise of drones in the recent years largely due to the advancements of drone technology which provide drones the ability to perform many more complex tasks autonomously with the incorporation of technologies such as computer vision, object avoidance and artificial intelligence. However, the misuse of drones such as the Gatwick Airport drone incident resulted in major disruptions which affected approximately 140,000 passengers. To deter this from happening in the future, drone surveillance are extremely crucial. With this, it will be achieved firstly by detection and followed by tracking of drones. This paper presents and investigates the use of a deep learning object detector, YOLOv3 with pretrained weights and transfer learning to train YOLOv3 to specifically detect drones. We demonstrated that the detection results from YOLOv3 after machine learning had an average accuracy of 88.9% at input image size of 416 × 416. Finally, we integrated into NVIDIA Jetson TX2 for real-time drone detection. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Salman2021335,
author={Salman, S. and Mir, J. and Farooq, M.T. and Malik, A.N. and Haleemdeen, R.},
title={Machine Learning Inspired Efficient Audio Drone Detection using Acoustic Features},
journal={Proceedings of 18th International Bhurban Conference on Applied Sciences and Technologies, IBCAST 2021},
year={2021},
pages={335-339},
art_number={9393232},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85104663735&doi=10.1109%2fIBCAST51254.2021.9393232&partnerID=40&md5=08a2f9d93b937f5dd78569e1acd82886},
abstract={With the recent proliferation of drones in the consumer market, drone detection has become critical to address the security and privacy issues raised by drone technology. This paper presents an efficient method for drone detection based on the drone's acoustic signature. Five different features are analyzed and compared to determine the best audio descriptor for drone detection. The selected features include Mel-frequency cepstral coefficients, Gammatone cepstral coefficients, linear prediction coefficients, spectral roll-off, and zero-crossing rate. Different support vector machine (SVM) classifier models are trained and tested on a large diverse database using 10-fold and 20% data holdout cross-validation schemes to evaluate the individual feature performance for efficient drone detection. Experimental results indicate that Gammatone cepstral coefficients are the most efficient features for audio drone detection. Further, the medium Gaussian SVM trained on all the investigated features achieves the classification accuracy of 99.9% with 99.8% recall and 100% precision, outperforming the compared existing state-of-the-art audio drone detection methods. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Alsoliman2021166,
author={Alsoliman, A. and Rigoni, G. and Levorato, M. and Pinotti, C. and Tippenhauer, N.O. and Conti, M.},
title={COTS Drone Detection using Video Streaming Characteristics},
journal={ACM International Conference Proceeding Series},
year={2021},
pages={166-175},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85098731548&doi=10.1145%2f3427796.3428480&partnerID=40&md5=6fa92f45d9f9e4e3b3ff9a96bc8068c3},
abstract={Cheap commercial off-the-shelf (COTS) drones have become widely available for consumers in recent years. Unfortunately, they also provide low-cost capabilities for attackers. Therefore, effective methods to detect the presence of non-cooperating rogue drones within a restricted area are highly required. Approaches based on detection of control traffic have been proposed but were not yet shown to work against other benign traffic, such as that generated by wireless security cameras. In this work, we propose a novel drone detection framework based on a Random Forest classification model. In essence, the framework leverages specific patterns in video traffic transmitted by drones. The patterns consist of repetitive synchronization packets (denoted as pivots) which we use as features in the proposed machine learning classifier. We show that our framework can achieve up to 99% detection accuracy over an encrypted WiFi channel using only 20 packets originated from the drone. Our system is able to identify drone transmissions even among very similar WiFi transmission (such as a security camera video stream) and in a noisy scenario with background traffic. © 2021 ACM.},
publisher={Association for Computing Machinery},
}

@CONFERENCE{Topalli2021,
author={Topalli, M.T. and Yilmaz, M. and Corapsiz, M.F.},
title={Real Time Implementation of Drone Detection using TensorFlow and MobileNetV2-SSD},
journal={7th International Conference on Electrical, Electronics and Information Engineering: Technological Breakthrough for Greater New Life, ICEEIE 2021},
year={2021},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85123580383&doi=10.1109%2fICEEIE52663.2021.9616846&partnerID=40&md5=667de7e16166a4af25044a388c84f974},
abstract={Drones are Unmanned Aerial Vehicles (UAV) that can be controlled by remote control or software methods. In recent years with the developing technology, drones have started to be used in all areas of our lives. The two most important factors that make drones attractive to use are low price and easy control. Today, UAVs, which provide convenience to people in many fields such as photography, video shooting, advertising, firefighting and search-rescue activities. Also, UAV is used by terrorist organizations in attack actions. Anti-drone systems are used to detect and locate such malicious drones. In this study, a prototype drone detection system called ATA-DRN is designed against drone threats. While creating ATA-DRN, 2 digital servo motors, Raspberry Pi 4 development board, high resolution Web Cam, 7inch HDMI LCD and power supply is used. With this designed system, drone approaching to the target is automatically detected with image processing methods without the need for manpower. In the study, first of all, a data set is obtained from pictures of different types of drones. The data set obtained is divided into two groups as train (80%) and test (20%) in order to train. The model to be used in real-time drone analysis is obtained using TensorFlow and MobileNetV2-SSD. Experiments are carried out by transferring the obtained model to the Raspberry Pi 4 development board. The accuracy of the model created as a result of experimental studies has been proven. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Suh2021,
author={Suh, H.-S. and Meng, J. and Nguyen, T. and Venkataramanaiah, S.K. and Kumar, V. and Cao, Y. and Seo, J.-S.},
title={Algorithm-Hardware Co-Optimization for Energy-Efficient Drone Detection on Resource-Constrained FPGA},
journal={2021 International Conference on Field-Programmable Technology, ICFPT 2021},
year={2021},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85123165019&doi=10.1109%2fICFPT52863.2021.9609840&partnerID=40&md5=37404b2e370f0265457ab580d1bd5a3f},
abstract={Convolutional neural network (CNN) based object detection has achieved very high accuracy, e.g. single-shot multi-box detectors (SSD) can efficiently detect and localize various objects in an input image. However, they require a high amount of computation and memory storage, which makes it difficult to perform efficient inference on resource-constrained hardware devices such as drones or unmanned aerial vehicles (UAVs). Drone/UAV detection is an important task for applications including surveillance, defense, and multi-drone self-localization and formation control. In this paper, we designed and co-optimized algorithm and hardware for energy-efficient drone detection on resource-constrained FPGA devices. We trained SSD object detection algorithm with a custom drone dataset. For inference, we employed low-precision quantization and adapted the width of the SSD CNN model. To improve throughput, we use dual-data rate operations for DSPs to effectively double the throughput with limited DSP counts. For different SSD algorithm models, we analyze accuracy or mean average precision (mAP) and evaluate the corresponding FPGA hardware utilization, DRAM communication, throughput optimization. Our proposed design achieves a high mAP of 88.42% on the multi-drone dataset, with a high energy-efficiency of 79 GOPS/W and throughput of 158 GOPS using Xilinx Zynq ZU3EG FPGA device on the Open Vision Computer version 3 (OVC3) platform. Our design achieves 2.7X higher energy efficiency than prior works using the same FPGA device, at a low-power consumption of 1.98 W. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Medaiyese202158,
author={Medaiyese, O.O. and Syed, A. and Lauf, A.P.},
title={Machine Learning Framework for RF-Based Drone Detection and Identification System},
journal={Proceedings of 2nd 2021 International Conference on Smart Cities, Automation and Intelligent Computing Systems, ICON-SONICS 2021},
year={2021},
pages={58-64},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85123055247&doi=10.1109%2fICON-SONICS53103.2021.9617168&partnerID=40&md5=ef3a8626d21290ba24223510f0d64b3e},
abstract={The emergence of drones has added a new dimension to privacy and security issues. There are little or no strict regulations on the people that can purchase or own a drone. For this reason, people can take advantage of these aircraft to intrude into restricted or private areas. A drone detection and identification (DDI) system is one of the ways of detecting and identifying the presence of a drone in an area. DDI systems can employ different sensing techniques such as radio frequency (RF) signals, video, sounds, and thermal imaging for detecting an intruding drone. In this work, we propose a machine learning RF-based DDI system that uses low band RF signals from drone-to-flight controller communication. We develop three machine learning models using the XGBoost algorithm to detect and identify the presence of a drone, the type of the drone, and the operational mode of drones. For these three XGBoost models, we evaluated the models using 10-fold cross validation and we achieve average accuracy of 99.96%, 90.73%, and 70.09% respectively. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Phung2021189,
author={Phung, K.-P. and Lu, T.-H. and Nguyen, T.-T. and Le, N.-L. and Nguyen, H.-H. and Hoang, V.-P.},
title={Multi-model Deep Learning Drone Detection and Tracking in Complex Background Conditions},
journal={International Conference on Advanced Technologies for Communications},
year={2021},
volume={2021-October},
pages={189-194},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85122942707&doi=10.1109%2fATC52653.2021.9598317&partnerID=40&md5=1efcc3b7b42865ce80289e93f937799d},
abstract={The recent popularity of drones with quadcopter layouts is threatening public safety and personal privacy. With the ability to hover and perform complex maneuvers even in indoor conditions, equipped with video cameras as well as capable of carrying hazardous materials, drones can truly become a security threat, especially to vulnerable organizations. Therefore, detecting and tracking drones in secured areas poses an urgent task for the surveillance system. In this paper, we design a real-time drone detection and tracking system with the combination of multiple deep learning and computer vision techniques: 1) Yolo-v4 model for detecting drones and 2) visual models for tracking drones. Besides, we have collected and labeled a larger drone dataset by mixing the existing datasets with our collected images. We evaluated three deep learning models for drone detection on this dataset and acquired the Yolo-V4 model to be the highest detection performance with AP = 34.63%. Combining this detection model and the existing visual tracking modules can boost the drone tracking up to more than 20fps for different backgrounds at around 700m by using an usual PC without GPU. © 2021 IEEE.},
publisher={IEEE Computer Society},
}

@ARTICLE{Chahrour2021123950,
author={Chahrour, H. and Dansereau, R.M. and Rajan, S. and Balaji, B.},
title={Target Detection through Riemannian Geometric Approach with Application to Drone Detection},
journal={IEEE Access},
year={2021},
volume={9},
pages={123950-123963},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85114740423&doi=10.1109%2fACCESS.2021.3105594&partnerID=40&md5=5f06f173522e8409142f0d36e032a9ed},
abstract={Radar detection of small drones in presence of noise and clutter is considered from a differential geometry viewpoint. The drone detection problem is challenging due to low radar cross section (RCS) of drones, especially in cluttered environments and when drones fly low and slow in urban areas. This paper proposes two detection techniques, the Riemannian-Brauer matrix (RBM) and the angle-based hybrid-Brauer (ABHB), to improve the probability of drone detection under small sample size and low signal-to-clutter ratio (SCR). These techniques are based on the regularized Burg algorithm (RBA), the Brauer disc (BD) theorem, and the Riemannian mean and distance. Both techniques exploit the RBA to obtain a Toeplitz Hermitian positive definite (THPD) covariance matrix from each snapshot and apply the BD theorem to cluster the clutter-plus-noise THPD covariance matrices. The proposed Riemannian-Brauer matrix technique is based on the Riemannian distance between the Riemannian mean of clutter-plus-noise cluster and potential targets. The proposed angle-based hybrid-Brauer technique uses the Euclidean tangent space and the Riemannian geodesical distances between the Riemannian mean, the Riemannian median and the potential target point. The angle at the potential target on the manifold is computed using the law of cosines on the manifold. The proposed detection techniques show advantage over the fast Fourier transform, the Riemannian distance-based matrix and the Kullback-Leibler (KLB) divergence detectors. The validity of both proposed techniques are demonstrated with real data. © 2013 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Shuhaywin20214220,
author={Shuhaywin, A.B. and Almeshkhas, F. and Mejjaouli, S.},
title={Establishing drone detection system by using deep learning and YOLOv3 formatting},
journal={Proceedings of the International Conference on Industrial Engineering and Operations Management},
year={2021},
pages={4220-4230},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85114264350&partnerID=40&md5=2220debaca7e78742b8530b73aa5655b},
abstract={Using a machine-vision detection based on deep learning system, the study established using darknet framework to identify and making the drone detection system. Using the darknet, YOLOv3 algorithm and OpenCV, the system was implemented on our computer to identify drones based on the live feed obtained from camera or uploaded image. The system was implemented to track and recognize drones on a different background. The project methodology is based on four different stages, gathering the dataset, annotation, training the system and testing the system. The project was able to identify the drones with an average success rate of 99% and 100% from live videos and uploaded images, respectively. The project showed that because of the deep learning strength, the detection was robust against changes in light intensity and the existence of background effects in different environmental conditions. © IEOM Society International.},
publisher={IEOM Society},
}

@ARTICLE{Flak2021114574,
author={Flak, P.},
title={Drone Detection Sensor with Continuous 2.4 GHz ISM Band Coverage Based on Cost-Effective SDR Platform},
journal={IEEE Access},
year={2021},
volume={9},
pages={114574-114586},
art_number={9513316},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113316401&doi=10.1109%2fACCESS.2021.3104738&partnerID=40&md5=cfd5a2b504fc46cfcdab4c7397ebc30a},
abstract={The development of Unmanned Aerial Vehicles (UAVs), commonly referred to as drones, has introduced revolutionary changes in many areas over the past few years. However, aside from opening new possibilities, the usage of drones in an irresponsible and dangerous manner leads to many hazardous incidents. This paper presents a drone detection sensor with a continuous 2.400 GHz-2.483 GHz operational frequency range for detection methods based on passive radio frequency imaging techniques. The implementation based on Software Defined Radio (SDR) and Field Programmable Logic Array (FPGA) hardware that overcomes the 40 MHz real-time bandwidth limit of other popular SDRs is presented utilizing low-cost off-the-shelf components. Furthermore, a hardware realization of the signal processing chain for specific detection algorithms is proposed to minimize the throughput between SDR and the companion computer and offload software computations. The device validation is made in a laboratory and real-life scenario and presented in relation to the sensor used in other works. In addition to the increased real-time bandwidth, the measurements show a 9 dB reduction in detection sensitivity compared to the reference receiver, in line with the analog RF front-end specifications. The final analysis demonstrates the proposed device's relevance as a sensor for obtaining machine learning datasets and as a part of a final anti-drone system. © 2013 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Basak2021,
author={Basak, S. and Rajendran, S. and Pollin, S. and Scheers, B.},
title={Combined RF-based drone detection and classification},
journal={IEEE Transactions on Cognitive Communications and Networking},
year={2021},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85112640839&doi=10.1109%2fTCCN.2021.3099114&partnerID=40&md5=5d3f7866c1bb0dd90849ea26a59dd5b0},
abstract={Despite several beneficial applications, unfortunately, drones are also being used for illicit activities such as drug trafficking, firearm smuggling or to impose threats to security-sensitive places like airports and nuclear power plants. The existing drone localization and neutralization technologies work on the assumption that the drone has already been detected and classified. Although we have observed a tremendous advancement in the sensor industry in this decade, there is no robust drone detection and classification method proposed in the literature yet. This paper focuses on radio frequency (RF) based drone detection and classification using the frequency signature of the transmitted signal. We have created a novel drone RF dataset using commercial drones and presented a detailed comparison between a two-stage and combined detection and classification framework. The detection and classification performance of both frameworks are presented for a single-signal and simultaneous multi-signal scenario. With detailed analysis, we show that You Only Look Once (YOLO) framework provides better detection performance compared to the Goodness-of-Fit (GoF) spectrum sensing for a simultaneous multi-signal scenario and good classification performance comparable to Deep Residual Neural Network (DRNN) framework. IEEE},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Zhang2021425,
author={Zhang, Y.},
title={RF-based drone detection using machine learning},
journal={Proceedings - 2021 2nd International Conference on Computing and Data Science, CDS 2021},
year={2021},
pages={425-428},
art_number={9463220},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85112395611&doi=10.1109%2fCDS52072.2021.00079&partnerID=40&md5=856c415a7a8f9f95c14fafaa59fa790f},
abstract={Drones or unmanned aerial vehicles have become a new option for multiple tasks including delivery, photograph, etc. However, the small size and flight ability of drones make it easier to break through any barriers and intrude important facilities. With an increasing safety concern of drone incursions, the research for an effective drone detection and identification approach has drawn a lot of attention in recent years. Among existing methods, passive radio frequency sensing is both reliable and cost-effective. However, previous studies are evaluating both machine learning and statistical methods on private datasets under different settings. To make a fair comparison, we evaluate six machine learning models on an open drone dataset for RF-based drone detection in this paper. The results demonstrate that XGBoost achieves the state-of-the-art results on this pioneering dataset. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Almasri2021208,
author={Almasri, M.},
title={Deep learning for RF-based drone detection and identification using welch's method},
journal={Proceedings of the 10th International Conference on Data Science, Technology and Applications, DATA 2021},
year={2021},
pages={208-214},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85111768869&doi=10.5220%2f0010530302080214&partnerID=40&md5=486752452eaf8696da50c2b6336f4fc9},
abstract={Radio Frequency (RF) combined with the deep learning methods promised a solution to detect the presence of the drones. Indeed, the classical techniques (i.e. radar, vision and acoustics, etc.) suffer several drawbacks such as difficult to detect the small drones, false alarm of flying birds or balloons, the influence of the wind on the performance, etc. For an effective drones's detection, two main stages should be established: Feature extraction and feature classification. The proposed approach in this paper is based on a novel feature extraction method and an optimized deep neural network (DNN). At first, we present a novel method based on Welch to extract meaningful features from the RF signal of drones. Later on, three optimized Deep Neural Network (DNN) models are considered to classify the extracted features. The first DNN model can be used to detect the presence of the drones and contains two classes. The second DNN help us to detect and recognize the type of the drone with 4 classes: A class for each drone and the last one for the RF background activities. In the third model, 10 classes have been considered: the presence of the drone, its type, and its flight mode (i.e. Stationary, Hovering, flying with or without video recording). Our proposed approach can achieve an average accuracy higher than 94% and it significantly improves the accuracy, up to 30%, compared to existing methods. Copyright © 2021 by SCITEPRESS - Science and Technology Publications, Lda. All rights reserved},
publisher={SciTePress},
}

@ARTICLE{Uddin202163456,
author={Uddin, Z. and Nebhen, J. and Altaf, M. and Orakzai, F.A.},
title={Independent Vector Analysis Inspired Amateur Drone Detection through Acoustic Signals},
journal={IEEE Access},
year={2021},
volume={9},
pages={63456-63462},
art_number={9410561},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85104596461&doi=10.1109%2fACCESS.2021.3074966&partnerID=40&md5=e7db64f28b0681a233304cb4714efde8},
abstract={Detection of amateur drones (AmDrs) is mandatory requirement of various defence organizations and is also required to protect human life. In literature, various researchers contributed in this regard and developed different algorithms utilizing video, thermal, radio frequencies and acoustic signals. However, inefficiency of the existing techniques is reported in different atmospheric conditions. In this paper, acoustic signal processing is performed based on independent vector analysis (IVA) to detect AmDrs in the field. This technique is capable to detect more than one AmDrs in the sensing field at a time in the presence of strong interfering sources. The IVA is a relatively new and practically applicable technique of blind source separation and is more efficient than the independent component analysis technique. In the proposed technique, recorded mixed signals through multiple microphones are first un-mixed through using the IVA technique. Then various features of the separated signals are extracted. These features include Root Mean Square (RMS) values, Power Spectral Density (PSD) and Mel Frequency Cepstral coefficients (MFCC). Finally, signals classification is performed through Support Vector Machines (SVM)and K Nearest Neighbor (KNN) to detect AmDrs in the field. Performance evaluation of the proposed technique is carried out through simulations and observed the superior performance of the proposed technique. © 2013 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Sharjeel2021128,
author={Sharjeel, A. and Naqvi, S.A.Z. and Ahsan, M.},
title={Real time drone detection by moving camera using COROLA and CNN algorithm},
journal={Journal of the Chinese Institute of Engineers, Transactions of the Chinese Institute of Engineers,Series A},
year={2021},
volume={44},
number={2},
pages={128-137},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85099420933&doi=10.1080%2f02533839.2020.1856725&partnerID=40&md5=727cd024352f7084218052edb2ac4333},
abstract={Widespread and careless use of unmanned aerial vehicles, such as drones, often raises serious privacy and security issues. To some extent, timely and accurate detection of drones enables observers to counteract unwarranted intrusion and other forms of their misuse. This is not an easy task, however, drones, on one hand, being small in size, are difficult to spot in general. On the other hand, they fly at low altitudes and against a background containing several look-alike objects. In this work, a hybrid approach for the detection of drones by the moving spy drone camera is presented which combines Contiguous Outlier Representation via Online Low-rank Approximation (COROLA) and Convolutional Neural Network (CNN). The COROLA technique is used for detecting a small moving object present in a scene and the CNN algorithm is employed for accurate drone recognition in a wide array of complex backgrounds. This hybrid technique is robust and time-efficient as it obviates full processing of the entire image sequence. To demonstrate the effectiveness of our proposed approach, we have compared its performance with R-STIC (Regression on Spatial-Temporal Image Cube), a state-of-the-art detection method, under different real-life scenarios. The obtained results show that the proposed hybrid approach is better than R-STIC, in terms of computational efficiency, accuracy, and robustness. © 2020 The Chinese Institute of Engineers.},
publisher={Taylor and Francis Ltd.},
}

@ARTICLE{Singh2021416,
author={Singh, A.K. and Bae, K.-B. and Park, S.-O.},
title={NLFM pulse radar for drone detection using predistortion technique},
journal={Journal of Electromagnetic Waves and Applications},
year={2021},
volume={35},
number={3},
pages={416-429},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85096109532&doi=10.1080%2f09205071.2020.1844598&partnerID=40&md5=75ef32c6ddc72ff0aa4ab7e5f419e2be},
abstract={The development of radar technology for the detection of small drones is getting attention of researchers. In this work, the detection of drones using Ku-band radar system has been discussed. We have utilized the advantage of nonlinear frequency modulation (NLFM) waveform for the suppression of range sidelobes. The performance and sensitivity of a radar system can be related with the linearity of system response. Here, we have made an effort to minimize non-linearity in the radar system response by using digital predistortion method. In this method, amplitude weighting coefficients have been calculated based on the received data. We have used FPGA-based transceiver for intermediate frequency (IF) signal generation and data acquisition, along with Ku-band up-down converters. The radar system was first calibrated for desired frequency band using amplitude predistortion method. In this article, experiment results for the detection of single drone and two drones using NLFM pulse signal are presented. © 2020 Informa UK Limited, trading as Taylor & Francis Group.},
publisher={Taylor and Francis Ltd.},
}

@ARTICLE{Sun20204795,
author={Sun, H. and Geng, W. and Shen, J. and Liu, N. and Liang, D. and Zhou, H.},
title={Deeper SSD: Simultaneous up-sampling and down-sampling for drone detection},
journal={KSII Transactions on Internet and Information Systems},
year={2020},
volume={14},
number={12},
pages={4795-4815},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85099333280&doi=10.3837%2ftiis.2020.12.010&partnerID=40&md5=3a7b7a1b480f9c90008bc4f04bd09985},
abstract={Drone detection can be considered as a specific sort of small object detection, which has always been a challenge because of its small size and few features. For improving the detection rate of drones, we design a Deeper SSD network, which uses large-scale input image and deeper convolutional network to obtain more features that benefit small object classification. At the same time, in order to improve object classification performance, we implemented the up-sampling modules to increase the number of features for the low-level feature map. In addition, in order to improve object location performance, we adopted the down-sampling modules so that the context information can be used by the high-level feature map directly. Our proposed Deeper SSD and its variants are successfully applied to the self-designed drone datasets. Our experiments demonstrate the effectiveness of the Deeper SSD and its variants, which are useful to small drone's detection and recognition. These proposed methods can also detect small and large objects simultaneously. © 2020 KSII},
publisher={Korean Society for Internet Information},
}

@CONFERENCE{Mahdavi2020,
author={Mahdavi, F. and Rajabi, R.},
title={Drone Detection Using Convolutional Neural Networks},
journal={6th Iranian Conference on Signal Processing and Intelligent Systems, ICSPIS 2020},
year={2020},
art_number={9349620},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85101770647&doi=10.1109%2fICSPIS51611.2020.9349620&partnerID=40&md5=b7172620cf89b63aad73c0e7831801ed},
abstract={In image processing, it is essential to detect and track air targets, especially UAVs. In this paper, we detect the flying drone using a fisheye camera. In the field of diagnosis and classification of objects, there are always many problems that prevent the development of rapid and significant progress in this area. During the previous decades, a couple of advanced classification methods such as convolutional neural networks and support vector machines have been developed. In this study, the drone was detected using three methods of classification of convolutional neural network (CNN), support vector machine (SVM), and nearest neighbor. The outcomes show that CNN, SVM, and nearest neighbor have total accuracy of 93%, 88%, and 80%, respectively. Compared with other classifiers with the same experimental conditions, the accuracy of the convolutional neural network classifier is satisfactory. © 2020 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Yi2020204,
author={Yi, J. and Srigrarom, S.},
title={Near-Parallel Binocular-Like Camera Pair for Multi-Drone Detection and 3D Localization},
journal={16th IEEE International Conference on Control, Automation, Robotics and Vision, ICARCV 2020},
year={2020},
pages={204-210},
art_number={9305485},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85100087134&doi=10.1109%2fICARCV50220.2020.9305485&partnerID=40&md5=2d5c3192bef36c9f25b0e50af0df02ed},
abstract={The paper presents the concept of using a pair of cameras that are setup near and almost parallel to each other to do detection and 3D localization of multiple drone at far distance away. These setup of the two cameras resemble the binocular cameras, as such the 3D positions of the detected drones can be estimated by epipolar-like geometry. For the special case of detecting the multiple drones at a distance, quick depth distance approximation based on similar triangles is also proposed. Sample field tests of detecting and tracking multiple drones at near and far distances in open areas are presented. The depth distances obtained are comparable to the actual GPS readings from the detected drones. © 2020 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Pratt2020,
author={Pratt, H. and Evans, B. and Rowntree, T. and Reid, I. and Wiederman, S.},
title={Recurrent Motion Neural Network for Low Resolution Drone Detection},
journal={2020 Digital Image Computing: Techniques and Applications, DICTA 2020},
year={2020},
art_number={9363377},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85102653283&doi=10.1109%2fDICTA51227.2020.9363377&partnerID=40&md5=2272ec353a4a0a6cab913bf5e8365237},
abstract={Drones are becoming increasingly prevalent in everyday usage with many commercial applications in fields such as construction work and agricultural surveying. Despite their common commercial use, drones have been recently used with malicious intent, such as airline disruptions at Gatwick Airport. With the emerging issue of safety concerns for the public and other airspace users, detecting and monitoring active drones in an area is crucial. This paper introduces a recurrent convolutional neural network (CNN) specifically designed for drone detection. This CNN can detect drones from down-sampled images by exploiting the temporal information of drones in flight and outperforms a state-of-the-art conventional object detector. Due to the lightweight and low resolution nature of this network, it can be mounted on a small processor and run at near real-time speeds. © 2020 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{M.Alaboudi2020278,
author={M. Alaboudi, M. and Abu Talib, M. and Nasir, Q.},
title={Radio frequency-based techniques of drone detection and classification using machine learning},
journal={ACM International Conference Proceeding Series},
year={2020},
pages={278-282},
art_number={3449348},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85108145264&doi=10.1145%2f3449301.3449348&partnerID=40&md5=419d1472ae846696eb3660f5f791c579},
abstract={This research paper provides a comprehensive survey review on drone detection using Radio Frequency (RF)-based techniques along with machine learning and localization algorithms. RF signals proved its effectiveness in detecting drones, however, due to the lack of a published survey, this research paper reviews the newly emerged RF-based techniques by addressing the implemented methods and discussing the results obtained in terms of the testing environment, range of detection and accuracy of the system. In this survey review, thirty conference and journal papers have been collected, however only selected papers have been discussed depending on the contribution and limited space of the paper. Finally, this survey also discusses the challenges encountered in drone detection using RF due to its great impact on the efficiency of the system. © 2020 ACM.},
publisher={Association for Computing Machinery},
}

@CONFERENCE{Huang2020,
author={Huang, A. and Sevigny, P. and Balaji, B. and Rajan, S.},
title={Radar Micro-Doppler-based Rotary Drone Detection using Parametric Spectral Estimation Methods},
journal={Proceedings of IEEE Sensors},
year={2020},
volume={2020-October},
art_number={9278678},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85098689652&doi=10.1109%2fSENSORS47125.2020.9278678&partnerID=40&md5=663950eb7d1ee398abbe458d850faff7},
abstract={Micro-Doppler methods of detecting and classifying small UAVs are limited in range due to the weak radar returns from their plastic propellers. Smaller windows of data instead of longer windows are used for detection as stationarity assumptions often fail for longer windows. Traditional non-parametric methods may be inadequate as they have limited spectral resolution with smaller windows and may provide false detection when radar returns are weak. A rotary drone detector using the number of Helicopter Rotation Modulation (HERM) lines is considered in this paper. Two parametric methods for estimating the number of HERM lines, Minimum Description Length (MDL) and Akaike Information Criterion (AIC), are considered for detection purposes. Experiments using real data acquired using a micro-helicopter drone and a commercial ultra-wide band radar reveal that MDL performs significantly better than AIC and the traditional Fourier-based non-parametric estimation methods. © 2020 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Garcia2020559,
author={Garcia, A.J. and Min Lee, J. and Kim, D.S.},
title={Anti-Drone System: A Visual-based Drone Detection using Neural Networks},
journal={International Conference on ICT Convergence},
year={2020},
volume={2020-October},
pages={559-561},
art_number={9289397},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85098963671&doi=10.1109%2fICTC49870.2020.9289397&partnerID=40&md5=854abf6e0d43829f248c90f0afe7dd19},
abstract={A system that secures an area from trespassing drones that might bring threat is in demand these days since drones became easily-available to the public and it became easier to operate. This paper proposes an anti-drone system that uses visual sensing to detect drones. A Faster R-CNN (Region-based Convolutional Neural Network) with ResNet-101 (Residual Neural Network-101) networks are used in this paper using a dataset from the SafeShore project. The network's accuracy is 93.40% and it has successfully detected drones in the simulation that has been done. © 2020 IEEE.},
publisher={IEEE Computer Society},
}

@CONFERENCE{Karpovich202077,
author={Karpovich, P. and Kareneuski, S. and Zielinski, T.P.},
title={Practical results of drone detection by passive coherent DVB-T2 radar},
journal={Proceedings International Radar Symposium},
year={2020},
volume={2020-October},
pages={77-81},
art_number={9253800},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85097307558&doi=10.23919%2fIRS48640.2020.9253800&partnerID=40&md5=64193c037b00b9c377a8b2d41a53535e},
abstract={In this paper practical results of drone detection and tracking in a DVB-T2 passive radar system are presented. DVB-T2 signal from TV tower was used to detect and measure distance and velocity of a drone. To increase SNR, adaptive filtering and re-modulation of DVB-T2 signal were applied before the detection. Since integration time of the reflected signal is large, a non-trivial range-Doppler matrix calculation algorithm was used to reduce the computational expense. Detection was done by CFAR algorithm. Finally, it was shown that peaks from drone's propellers are visible in range-Doppler matrix what can be used for its type identification, and application of multiple TV-tower signals has been suggested. © 2020 Warsaw University of Technology.},
publisher={IEEE Computer Society},
}

@ARTICLE{Demir20201625,
author={Demir, B. and Ergunay, S. and Nurlu, G. and Popovic, V. and Ott, B. and Wellig, P. and Thiran, J.-P. and Leblebici, Y.},
title={Real-time high-resolution omnidirectional imaging platform for drone detection and tracking},
journal={Journal of Real-Time Image Processing},
year={2020},
volume={17},
number={5},
pages={1625-1635},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85074700180&doi=10.1007%2fs11554-019-00921-7&partnerID=40&md5=ca09300a973af4909bdf83c5d8857a02},
abstract={Drones have become steadily affordable, which raises privacy and security concerns as well as interest in drone detection systems. On the other hand, drone detection is a challenging task due to small dimensions of drones, difficulty of long-distance detection, strict real-time constraints and necessity of wide angle coverage for drones. Although different radar and audio-assisted drone detection systems have been presented, they suffer from the cost, range, or interference problems. On the contrary, a long-range detection can be obtained by a vision-based system. Aiming that, we propose a real-time moving object detection and tracking system optimized for drone detection using 16 cameras with 20 MP resolution. The proposed system detects drones from short range and long range with 360∘ surveillance coverage owing high-performance ultra-high-resolution (320 MP) video-processing capability. It is able to detect drones with 100 cm diameter from 700 m distance despite deceptive background. It is interference free, so multiple systems can properly operate in the vicinity without effecting each other. It integrates processing power of embedded systems with flexibility of software to generate a full platform for drone detection and tracking. © 2019, Springer-Verlag GmbH Germany, part of Springer Nature.},
publisher={Springer},
}

@CONFERENCE{Martelli2020,
author={Martelli, T. and Cabrera, O. and Colone, F. and Lombardo, P.},
title={Exploitation of Long Coherent Integration Times to Improve Drone Detection in DVB-S based Passive Radar},
journal={IEEE National Radar Conference - Proceedings},
year={2020},
volume={2020-September},
art_number={9266624},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85098597794&doi=10.1109%2fRadarConf2043947.2020.9266624&partnerID=40&md5=c11d038bf2b948ba64ec556f60f31684},
abstract={In this paper, we consider the exploitation of long coherent integration times for improving the detection of small drones in a DVB-S based Passive Radar (PR). In fact, since these low-flying objects are characterized by very small RCS values, their detection is challenging especially when using DVB-S signals as source of opportunity, typically received with low power levels. In this work, in order to benefit from the use of extended coherent integration times, the target range and Doppler migration effects have been properly compensated. Then, the effectiveness of the adopted detection scheme has been tested against real data collected by a multi-polarimetric DVB-S based PR receiver developed at Sapienza University of Rome. The reported results show that the coherent integration time can be increased up to a few seconds thus improving the drone detection capability of the considered system. © 2020 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Zulkifli2020,
author={Zulkifli, S. and Balleri, A.},
title={Design and Development of K-Band FMCW Radar for Nano-Drone Detection},
journal={IEEE National Radar Conference - Proceedings},
year={2020},
volume={2020-September},
art_number={9266538},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85098536006&doi=10.1109%2fRadarConf2043947.2020.9266538&partnerID=40&md5=e432c2d5a152ce0dee62c68b0b96214a},
abstract={Nano-drones, are insect-like size drones with a capability of intrusion to provide intelligence and potentially violate secure establishments and public privacy rights. Nano-drones are already an existing technology which is becoming more and more available, portable, affordable and easily operated. As such, they may soon become a plausible defence and security threat. This paper presents the design and development of a K-Band FMCW radar prototype for nano-drone detection. The FMCW radar prototype consists of connectorised components operating at a carrier frequency of 24 GHz and offer high parameter selection flexibility. Experiments have been carried out in order to evaluate the system performance. Results show that a small Arcade PICO Drone Nano Quadcopter (smaller than 5 cm) could be detected, and that its micro-Doppler signature could be extracted from data. © 2020 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Abdullah2020,
author={Abdullah, R.S.A.R. and Musa, S.A. and Rashid, N.E.A. and Sali, A. and Salah, A.A. and Ismail, A.},
title={Passive forward-scattering radar using digital video broadcasting satellite signal for drone detection},
journal={Remote Sensing},
year={2020},
volume={12},
number={18},
art_number={3075},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85092268648&doi=10.3390%2fRS12183075&partnerID=40&md5=cc4b708be21a21a6e3555b65a0907b31},
abstract={This paper presents a passive radar system using a signal of opportunity from Digital Video Broadcasting Satellite (DVB-S). The ultimate purpose of the system is to be used as an air traffic monitoring and surveillance system. However, the work focuses on drone detection as a proof of the concept. Detecting a drone by using satellite-based passive radar possess inherent challenges, such as the small radar cross section and low speed. Therefore, this paper proposes a unique method by leveraging the advantage of forward-scattering radar (FSR) topology and characteristics to detect a drone, in other words, the system is known as a passive FSR (p-FSR) system. In the signal-processing algorithm, the empirical mode decomposition (EMD) is applied to the received signal to extract the unique feature vector of the micro-Doppler frequency from the drone's rotating blades. The paper highlights the p-FSR experimental setup and experiment campaign to detect drones. The experimental results show the feasibility of the p-FSR using a signal transmitted from a satellite to detect flying drone crossing the forward-scatter baseline between the satellite and ground station. © 2020 by the authors.},
publisher={MDPI AG},
}

@ARTICLE{Seidaliyeva20201,
author={Seidaliyeva, U. and Akhmetov, D. and Ilipbayeva, L. and Matson, E.T.},
title={Real-time and accurate drone detection in a video with a static background},
journal={Sensors (Switzerland)},
year={2020},
volume={20},
number={14},
pages={1-18},
art_number={3856},
note={cited By 20},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85087622606&doi=10.3390%2fs20143856&partnerID=40&md5=4056a8e6bd2c26d89290db38a268ac5e},
abstract={With the increasing number of drones, the danger of their illegal use has become relevant. This has necessitated the creation of automatic drone protection systems. One of the important tasks solved by these systems is the reliable detection of drones near guarded objects. This problem can be solved using various methods. From the point of view of the price–quality ratio, the use of video cameras for a drone detection is of great interest. However, drone detection using visual information is hampered by the large similarity of drones to other objects, such as birds or airplanes. In addition, drones can reach very high speeds, so detection should be done in real time. This paper addresses the problem of real-time drone detection with high accuracy. We divided the drone detection task into two separate tasks: the detection of moving objects and the classification of the detected object into drone, bird, and background. The moving object detection is based on background subtraction, while classification is performed using a convolutional neural network (CNN). The experimental results showed that the proposed approach can achieve an accuracy comparable to existing approaches at high processing speed. We also concluded that the main limitation of our detector is the dependence of its performance on the presence of a moving background. © 2020 by the authors. Licensee MDPI, Basel, Switzerland.},
publisher={MDPI AG},
}

@CONFERENCE{Salhi2020,
author={Salhi, M. and Boudriga, N.},
title={Multi-array spherical LIDAR system for drone detection},
journal={International Conference on Transparent Optical Networks},
year={2020},
volume={2020-July},
art_number={9203381},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85092452815&doi=10.1109%2fICTON51198.2020.9203381&partnerID=40&md5=0afd0f4f5cb66f010e6e2a826a8f661a},
abstract={The detection of unmanned aerial vehicles (UAVs) represents a necessity to protect critical areas and infrastructures against potential attacks performed by these UAVs. Different detection solutions have been proposed in the literature. They include conventional radars, radio frequency signal detection, acoustic detection, as well as light detection and ranging (Lidar). Using cameras, the latter technology is new and promising, yet controversial for its feasibility and cost effectiveness. In this paper, we propose a multi-array Lidar system that is capable of detecting potential UAVs using visible light communication. The system is composed of laser sources and laser concentrators. These transmitting/receiving elements are arranged through arrays along a spherical form including a photodiode at its centre. The reflected optical energy reaching the concentrators is transmitted to this central photodiode. The work assesses the feasibility and effectiveness of the solution through an in-depth examination of the design parameters. This includes the sensors' characteristics, the elements positioning and interspace, as well as the dimensions of the monitored cylinder. © 2020 IEEE.},
publisher={IEEE Computer Society},
}

@CONFERENCE{Koksal20204439,
author={Koksal, A. and Ince, K.G. and Aydin Alatan, A.},
title={Effect of annotation errors on drone detection with YOLOv3},
journal={IEEE Computer Society Conference on Computer Vision and Pattern Recognition Workshops},
year={2020},
volume={2020-June},
pages={4439-4447},
art_number={9150631},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85090130528&doi=10.1109%2fCVPRW50498.2020.00523&partnerID=40&md5=4bbfa5146b65be1e440f91019f2f94bd},
abstract={Following the recent advances in deep networks, object detection and tracking algorithms with deep learning backbones have been improved significantly; however, this rapid development resulted in the necessity of large amounts of annotated labels. Even if the details of such semi-automatic annotation processes for most of these datasets are not known precisely, especially for the video annotations, some automated labeling processes are usually employed. Unfortunately, such approaches might result with erroneous annotations. In this work, different types of annotation errors for object detection problem are simulated and the performance of a popular state-of-the-art object detector, YOLOv3, with erroneous annotations during training and testing stages is examined. Moreover, some inevitable annotation errors in Anti-UAV Challenge dataset is also examined in this manner, while proposing a solution to correct such annotation errors of this valuable data set. © 2020 IEEE.},
publisher={IEEE Computer Society},
}

@CONFERENCE{Behera20201012,
author={Behera, D.K. and Raj, A.B.},
title={Drone Detection and Classification using Deep Learning},
journal={Proceedings of the International Conference on Intelligent Computing and Control Systems, ICICCS 2020},
year={2020},
pages={1012-1016},
art_number={9121150},
note={cited By 19},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85087452192&doi=10.1109%2fICICCS48265.2020.9121150&partnerID=40&md5=3cad9228db1498f00868540b706f8666},
abstract={This paper presents a systematic approach to drone detection and classification using deep learning with different modalities. The YOLOv3 object detector is used to detect the moving or still objects. It uses a computer vision-based approach as a reliable solution. The convolutional neural network helps to extract features from images and to detect the object with maximum accuracy. The model is trained with a proper dataset and trained for 150 epoch only to detect various types of drones. A convolutional neural network with modern object detection methods shows an excellent approach for real-time detection of drones. © 2020 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Park20201858,
author={Park, J. and Jung, D.-H. and Bae, K.-B. and Park, S.-O.},
title={Range-Doppler Map Improvement in FMCW Radar for Small Moving Drone Detection Using the Stationary Point Concentration Technique},
journal={IEEE Transactions on Microwave Theory and Techniques},
year={2020},
volume={68},
number={5},
pages={1858-1871},
art_number={8957391},
note={cited By 6},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85084850484&doi=10.1109%2fTMTT.2019.2961911&partnerID=40&md5=bb279d0b2889e9e317e3b3ac3feb927b},
abstract={Given the rapidly growing drone market, the development of drone detection radars has become highly important to prevent drones from damaging lives and property. Frequency-modulated continuous-wave (FMCW) radars have been frequently used for drone detection. Among the architectures of FMCW radar, a heterodyne architecture that involves different local oscillators and produces beat signals at the IF stage has often been chosen. The FMCW radar, however, has a chronic problem called leakage. In an earlier study, we proposed the stationary point concentration (SPC) technique to improve the signal-to-noise ratio (SNR) of small drones by reducing the increase in noise floor caused by leakage. We demonstrated that the proposed technique increases the SNR of small hovering drones in the 1-D power spectrum. In this article, we newly analyze the practical problems in the heterodyne FMCW radar system. One is the 2-D noise floor increase in the range-Doppler (r-D) map due to the leakage, and the other is unwanted Doppler shifts. Then, we propose an upgraded theory and realization method of the SPC technique for the detection of the small moving drone by improving the r-D map. We prove that the proposed method not only reduces the 2-D noise floor by mitigating the leakage but also removes the unwanted Doppler shifts by the phase calibration. Consequently, we show that the proposed method increases the SNR of the small moving drone and corrects its velocity information at the same time in the r-D map. © 1963-2012 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Kavitha20201366,
author={Kavitha, T. and Lakshmi, K.},
title={A drone detection system for preventing security threats using YOLO deep learning network},
journal={International Journal of Advanced Science and Technology},
year={2020},
volume={29},
number={5 Special Issue},
pages={1366-1376},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85083963617&partnerID=40&md5=d0d66ad26522be4084a5745f16b1331c},
abstract={There has been a tremendous increase of use of UAVs or drones in the recent years. It is used in many fields such as aerial photography, shipping and delivery, crowd monitoring, crop monitoring in agriculture, law enforcement and surveillance etc. The cost of these devices become very low and makes it highly accessible to common public. It also increases the work efficiency and accuracy. Sometimes these drones are used for capturing information from secured areas by trespassing. This has raised several security concerns. In order to protect privacy and security at important locations, several solutions have been proposed in recent years. The drones are detected by using radio frequencies, acoustic waves, optic sensors and radars but they have certain limitations. Hence, this paper focuses on deep learning-based computer vision technique for detecting drones. To eradicate such security threats, the existing techniques for drone detection have been analyzed and designed a robust system based on You Only Look Once (YOLO) object detection algorithm. The YOLO based drone detection system performed well and produced results better than the other compared system. © 2020 SERSC.},
publisher={Science and Engineering Research Support Society},
}

@ARTICLE{Uddin2020236,
author={Uddin, Z. and Altaf, M. and Bilal, M. and Nkenyereye, L. and Bashir, A.K.},
title={Amateur Drones Detection: A machine learning approach utilizing the acoustic signals in the presence of strong interference},
journal={Computer Communications},
year={2020},
volume={154},
pages={236-245},
note={cited By 8},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85080874387&doi=10.1016%2fj.comcom.2020.02.065&partnerID=40&md5=679d83ca6c2c966c81b2112aa181570b},
abstract={Owing to small size, sensing capabilities and autonomous nature, the Unmanned Air Vehicles (UAVs) have enormous applications in various areas e.g., remote sensing, navigation, archaeology, journalism, environmental science, and agriculture. However, the un-monitored deployment of UAVs called the amateur drones (AmDr) can lead to serious security threats and risk to human life and infrastructure. Therefore, timely detection of the AmDr is essential for the protection and security of sensitive organizations, human life and other vital infrastructure. AmDrs can be detected using different techniques based on sound, video, thermal, and radio frequencies. However, the performance of these techniques is limited in sever atmospheric conditions. In this paper, we propose an efficient un-supervise machine learning approach of independent component analysis (ICA) to detect various acoustic signals i.e., sounds of bird, airplanes, thunderstorm, rain, wind and the UAVs in practical scenario. After unmixing the signals, the features like Mel Frequency Cepstral Coefficients (MFCC), the power spectral density (PSD) and the Root Mean Square Value (RMS) of the PSD are extracted by using ICA. The PSD and the RMS of PSD signals are extracted by first passing the signals from octave band filter banks. Based on the above features the signals are classified using Support Vector Machines (SVM)and K Nearest Neighbour (KNN)to detect the presence or absence of AmDr. Unique feature of the proposed technique is the detection of a single or multiple AmDrs at a time in the presence of multiple acoustic interfering signals. The proposed technique is verified through extensive simulations and it is observed that the RMS values of PSD with KNN performs better than the MFCC with KNN and SVM. © 2020 Elsevier B.V.},
publisher={Elsevier B.V.},
}

@ARTICLE{Shi20202731,
author={Shi, Z. and Chang, X. and Yang, C. and Wu, Z. and Wu, J.},
title={An Acoustic-Based Surveillance System for Amateur Drones Detection and Localization},
journal={IEEE Transactions on Vehicular Technology},
year={2020},
volume={69},
number={3},
pages={2731-2739},
art_number={8950116},
note={cited By 10},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85082063635&doi=10.1109%2fTVT.2020.2964110&partnerID=40&md5=f9ed2b64e134858cebaf71ddcda18fac},
abstract={Due to cost reduction and device miniaturization, amateur drones are now widely used in numerous civilian and commercial applications. However, the abuse of amateur drones has resulted in emerging threats to personal privacy and public security. To alleviate these threats, we design an acoustic-based surveillance system, which can achieve the capacity of amateur drones detection and localization with 24/7 (24 hours per day and 7 days per week under normal circumstances) availability. In the designed system, a detection fusion algorithm and a TDOA estimation algorithm based on the Bayesian filter are applied to improve the performance of drone detection and localization. Field experiments are carried out, and the results demonstrate that the designed system can detect and locate an amateur drone in real time with high accuracy and 24/7 availability. © 1967-2012 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Sciancalepore2020,
author={Sciancalepore, S. and Ibrahim, O.A. and Oligeri, G. and Di Pietro, R.},
title={PiNcH: An effective, efficient, and robust solution to drone detection via network traffic analysis},
journal={Computer Networks},
year={2020},
volume={168},
art_number={107044},
note={cited By 18},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85076546502&doi=10.1016%2fj.comnet.2019.107044&partnerID=40&md5=2338a5e886850121c1e54c7e3595bd7c},
abstract={We propose Picking a Needle in a Haystack (PiNcH), a methodology to detect the presence of a drone, its current status, and its movements by leveraging just the communication traffic exchanged between the drone and its Remote Controller (RC). PiNcH is built applying standard classification algorithms to the eavesdropped traffic, analyzing features such as packets inter-arrival time and size. PiNcH is fully passive and it requires just cheap and general-purpose hardware. To evaluate the effectiveness of our solution, we collected real communication traces originated by a drone running the widespread ArduCopter open-source firmware, currently mounted on-board of a wide range (30+) of commercial amateur drones. Then, we tested our solution against different publicly available wireless traces. The results prove that PiNcH can efficiently and effectively: (i) identify the presence of the drone in several heterogeneous scenarios; (ii) identify the current state of a powered-on drone, i.e., flying or lying on the ground; (iii) discriminate the movements of the drone; and, finally, (iv) enjoy a reduced upper bound on the time required to identify a drone with the requested level of assurance. The effectiveness of PiNcH has been also evaluated in the presence of both heavy packet loss and evasion attacks. In this latter case, the adversary modifies on purpose the profile of the traffic of the drone-RC link to avoid the detection. In both the cited cases, PiNcH continues enjoying a remarkable performance. Further, the comparison against state of the art solution confirms the superior performance of PiNcH in several scenarios. Note that all the drone-controller generated data traces have been released as open-source, to allow replicability and foster follow-up. Finally, the quality and viability of our solution, do prove that network traffic analysis can be successfully adopted for drone identification and status discrimination, and pave the way for future research in the area. © 2019},
publisher={Elsevier B.V.},
}

@CONFERENCE{Al-Emadi202029,
author={Al-Emadi, S. and Al-Senaid, F.},
title={Drone Detection Approach Based on Radio-Frequency Using Convolutional Neural Network},
journal={2020 IEEE International Conference on Informatics, IoT, and Enabling Technologies, ICIoT 2020},
year={2020},
pages={29-34},
art_number={9089489},
note={cited By 12},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85085478429&doi=10.1109%2fICIoT48696.2020.9089489&partnerID=40&md5=e9652f8067c99f9d4b2398018e913222},
abstract={Recently, Unmanned Aerial Vehicles, also known as drones, are becoming rapidly popular due to the advancement of their technology and the significant decrease in their cost. Although commercial drones have proven their effectiveness in many day to day applications such as cinematography, agriculture monitoring and search and rescue, they are also being used in malicious activities that are targeting to harm individuals and societies which raises great privacy, safety and security concerns. In this research, we propose a new drone detection solution based on the Radio Frequency (RF) emitted during the live communication session between the drone and its controller using a Deep Learning (DL) technique, namely, the Convolutional Neural Network (CNN). The results of the study have proven the effectiveness of using CNN for drone detection with accuracy and F1 score of over 99.7% and drone identification with accuracy and F1 score of 88.4%. Moreover, the results yielded from this experiment have outperformed those reported in the literature for RF based drone detection using Deep Neural Networks. © 2020 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Allahham2020112,
author={Allahham, M.S. and Khattab, T. and Mohamed, A.},
title={Deep Learning for RF-Based Drone Detection and Identification: A Multi-Channel 1-D Convolutional Neural Networks Approach},
journal={2020 IEEE International Conference on Informatics, IoT, and Enabling Technologies, ICIoT 2020},
year={2020},
pages={112-117},
art_number={9089657},
note={cited By 8},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85085474950&doi=10.1109%2fICIoT48696.2020.9089657&partnerID=40&md5=9bfa150bcc4868e361e8a1b11465ffa8},
abstract={Commercial unmanned aerial vehicles, or drones, are getting increasingly popular in the last few years. The fact that these drones are highly accessible to public may bring a range of security and technical issues to sensitive areas such as airfields and military bases. Consequently, drone detection and state identification are becoming very crucial and essential for governments and security agencies. This paper proposes a deep learning based approach for drone detection, type identification and state identification using a multi-channel 1-dimensional convolutional neural network. The deep learning model is trained utilizing a publicly published database for drone's radio frequency signals. The proposed model can be used to produce new features that can represent the whole dataset in a more compact form which enables the use of classical machine learning algorithms for classification. © 2020 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Chen202081,
author={Chen, H. and Wang, Z. and Zhang, L.},
title={Collaborative spectrum sensing for illegal drone detection: A deep learning-based image classification perspective},
journal={China Communications},
year={2020},
volume={17},
number={2},
pages={81-92},
art_number={9020299},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85081655115&doi=10.23919%2fJCC.2020.02.007&partnerID=40&md5=398ce42462246b681ca5a7ad25d1cd4f},
abstract={Drones, also known as mini-unmanned aerial vehicles (UAVs), are enjoying great popularity in recent years due to their advantages of low cost, easy to pilot and small size, which also makes them hard to detect. They can provide real time situational awareness information by live videos or high definition pictures and pose serious threats to public security. In this article, we combine collaborative spectrum sensing with deep learning to effectively detect potential illegal drones with states of high uncertainty. First, we formulate the detection of potential illegal drones under illegitimate access and rogue power emission as a quaternary hypothesis test problem. Then, we propose an algorithm of image classification based on convolutional neural network which converts the cooperative spectrum sensing data at a sensing slot into one image. Furthermore, to exploit more information and improve the detection performance, we develop a trajectory classification algorithm which converts the flight process of the drones in consecutive multiple sensing slots into trajectory images. In addition, simulations are provided to verify the proposed methods' performance under various parameter configurations. © 2013 China Institute of Communications.},
publisher={Editorial Department of China Communications},
}

@ARTICLE{Lee2020213,
author={Lee, S.J. and Jung, J.H. and Yu, J.-W.},
title={TX Leakage Canceller for Small Drone Detection Radar in 2-GHz Band},
journal={IEEE Microwave and Wireless Components Letters},
year={2020},
volume={30},
number={2},
pages={213-215},
art_number={8998608},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85079742921&doi=10.1109%2fLMWC.2019.2959441&partnerID=40&md5=9ef0b3ab2b584d31a88d0dca043140f6},
abstract={A transmitter leakage canceller (TLC) having high isolation from a transmitter (TX) to a receiver (RX) is proposed, which is for a single antenna continuous-wave (CW) radar in the 2-GHz band. The proposed TLC is based on three points to obtain sufficient TX-to-RX isolation in a bandwidth of tens of MHz. The first is the use of a quasi-balanced structure in a leakage path and an antileakage path, which makes both signals in the two paths similar in a wide bandwidth. The second point is the adoption of active circuits in the antileakage path, which provides sufficient cancellation between the two signals. However, this adoption makes both signals in two paths with different phase slopes versus frequency; therefore, the sufficient cancellation is confined to a narrow bandwidth. The last is the application of a delay line in the leakage path, which compensates the different phase slopes. Thus, a bandwidth feature of tens of MHz is obtained. Laboratory measurements show more than 60 dB TX-to-RX isolation for an arbitrary targeted 20-MHz bandwidth from 2.3 to 2.7 GHz. © 2001-2012 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Pham20202965,
author={Pham, G.N. and Nguyen, P.H.},
title={Drone detection experiment based on image processing and machine learning},
journal={International Journal of Scientific and Technology Research},
year={2020},
volume={9},
number={2},
pages={2965-2971},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85079555266&partnerID=40&md5=befa3b02c6a14ea30350625da119967b},
abstract={Drones are widely used in the field of information gathering and tracking, even they could be used to attacked targets. Therefore, the drone detection for the restricted areas or special zones is important and necessary. This paper focuses on the drone detection problem based on image processing for the restricted areas or special zones where used cameras for monitoring. The proposed solution detects drones from the captured images based on training the Haar-like features. The dataset of drone images is used in the Haar training process to generate a Haar-cascade model of drones. This model is then used to detect drones from images captured by the camera. The proposed solution is implemented and experimented with single cameras installed for any place including indoor environment and outdoor environment. Experimental results proved that the proposed solution could exactly detect drones for any zone or the restricted areas. The average accuracy of the proposed solution in the experimented environments is 91.9 %, and it provides an easy and economical solution for user. IJSTR © 2020.},
publisher={International Journal of Scientific and Technology Research},
}

@CONFERENCE{Svanström20207265,
author={Svanström, F. and Englund, C. and Alonso-Fernandez, F.},
title={Real-time drone detection and tracking with visible, thermal and acoustic sensors},
journal={Proceedings - International Conference on Pattern Recognition},
year={2020},
pages={7265-7272},
art_number={9413241},
note={cited By 6},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85109250336&doi=10.1109%2fICPR48806.2021.9413241&partnerID=40&md5=2fca213bab1dd99da7d217f33a31f4af},
abstract={This paper explores the process of designing an automatic multi-sensor drone detection system. Besides the common video and audio sensors, the system also includes a thermal infrared camera, which is shown to be a feasible solution to the drone detection task. Even with slightly lower resolution, the performance is just as good as a camera in visible range. The detector performance as a function of the sensor-to-target distance is also investigated. In addition, using sensor fusion, the system is made more robust than the individual sensors, helping to reduce false detections. To counteract the lack of public datasets, a novel video dataset containing 650 annotated infrared and visible videos of drones, birds, airplanes and helicopters is also presented1. The database is complemented with an audio dataset of the classes drones, helicopters and background noise. © 2020 IEEE},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Sommer2020,
author={Sommer, L. and Schumann, A.},
title={Deep learning-based drone detection in infrared imagery with limited training data},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2020},
volume={11542},
art_number={1154204},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85096365614&doi=10.1117%2f12.2574171&partnerID=40&md5=f105d82088e98a2cd7918679fe4e825e},
abstract={The increased availability and capabilities of drones in the consumer market has lead to increased risk in air traffic control and other public safety concerns. Automated drone detection systems can help to generate alerts and increase reaction time by security forces. Recently proposed approaches and systems are usually based on a combination of sensors and machine learning to carry out the detection of drones. While electro-optical imagery is the most prevalent modality, infrared sensors can complement it by providing better visibility in certain situations with cluttered background or low light conditions. A key limitation when using infrared data is the limited availability of data for training machine learning methods. In this work, we specifically focus on the task of drone detection in infrared imagery. Our main focus lies on investigating how the small amount of available infrared data can be compensated for. We approach this problem through three different types of experiments. First, we compare a detector resulting from training on limited infrared data with a detector trained on more diverse optical data. We then propose and evaluate several methods for pre-processing optical data in such a way that it better resembles the characteristics of infrared data. Finally, we train detectors on a combination of infrared and pre-processed optical data and evaluate the trade-off between amount of available infrared data and achieved accuracy of the resulting detector. We evaluate all detectors on our own set of diverse infrared recordings. Our results show that suitable pre-processing of optical data can significantly improve the resulting accuracy and performs much better than training solely on limited infrared data. © 2020 SPIE},
publisher={SPIE},
}

@ARTICLE{Sun2020130697,
author={Sun, H. and Yang, J. and Shen, J. and Liang, D. and Ning-Zhong, L. and Zhou, H.},
title={TIB-Net: Drone Detection Network with Tiny Iterative Backbone},
journal={IEEE Access},
year={2020},
volume={8},
pages={130697-130707},
art_number={9141228},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85089524311&doi=10.1109%2fACCESS.2020.3009518&partnerID=40&md5=91412e44e3c84ea850ec66db0c85ab03},
abstract={With the widespread application of drone in commercial and industrial fields, drone detection has received increasing attention in public safety and others. However, due to various appearance of small-size drones, changeable and complex environments, and limited memory resources of edge computing devices, drone detection remains a challenging task nowadays. Although deep convolutional neural network (CNN) has shown powerful performance in object detection in recent years, most existing CNN-based methods cannot balance detection performance and model size well. To solve the problem, we develop a drone detection network with tiny iterative backbone named TIB-Net. In this network, we propose a structure called cyclic pathway, which enhances the capability to extract effective features of small object, and integrate it into existing efficient method Extremely Tiny Face Detector (EXTD). This method not only significantly improves the accuracy of drone detection, but also keeps the model size at an acceptable level. Furthermore, we integrate spatial attention module into our network backbone to emphasize information of small object, which can better locate small-size drone and further improve detection performance. In addition, we present massive manual annotations of object bounding boxes for our collected 2860 drone images as a drone benchmark dataset, which is now publicly available1. In this work, we conduct a series of experiments on our collected dataset to evaluate TIB-Net, and the result shows that our proposed method achieves mean average precision of 89.2% with model size of 697.0KB, which achieves the state-of-the-art results compared with existing methods. © 2013 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Yeung2020,
author={Yeung, C.K.A. and Lo, B.F. and Torborg, S.},
title={Drone Detection via Low Complexity Zadoff-Chu Sequence Root Estimation},
journal={2020 IEEE 17th Annual Consumer Communications and Networking Conference, CCNC 2020},
year={2020},
art_number={9045243},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85085490888&doi=10.1109%2fCCNC46108.2020.9045243&partnerID=40&md5=70790c6c24f948749a80f9904676c3d1},
abstract={The fast growth of drone applications in industrial, commercial and consumer domains in recent years has caused great security, safety and privacy concerns. For this reason, a demand for solutions of drone detection and monitoring in consumer market can be foreseen in the near future. For detecting drones that employ Zadoff-Chu (ZC) sequences for synchronization, these ZC sequences can be used to determine their presence in the air. However, it is a great challenge to blindly detect thousands of unknown ZC sequences possibly used by the drones in real time. Existing solutions mainly developed for LTE systems cannot be directly applied to the blind detection of ZCs in drones without incurring huge cost. In this paper, a low-complexity cost effective blind ZC detection method based on double differential is proposed for low-cost drone detection and monitoring systems. Signal-to-noise ratio (SNR) lower bounds are analytically derived for low and high SNR regimes. Monte Carlo simulations show the proposed scheme performs well in moderate and high SNR. © 2020 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Sun20193667,
author={Sun, H. and Oh, B.-S. and Guo, X. and Lin, Z.},
title={Improving the Doppler Resolution of Ground-Based Surveillance Radar for Drone Detection},
journal={IEEE Transactions on Aerospace and Electronic Systems},
year={2019},
volume={55},
number={6},
pages={3667-3673},
art_number={8631137},
note={cited By 8},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85065534249&doi=10.1109%2fTAES.2019.2895585&partnerID=40&md5=9bdbf9b282ab8f3751282c160eaec9c2},
abstract={In this paper, we propose to use an iterative adaptive approach to perform the Doppler processing in ground-based surveillance radar for drone detection. It overcomes the limited dwell time and improves the Doppler resolution, and therefore significantly enhances the discrimination of micro-Doppler signature and the correct classification of drones. In addition, the target detectability is also improved. This approach is validated in the field experiments conducted with a commercial portable ground-based surveillance radar. © 1965-2011 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Sharma2019449,
author={Sharma, V. and Kumari, M.},
title={Drone Detection Mechanism using Radiocommunication Technology and Internet Protocol Address},
journal={Proceedings of the 2nd International Conference on Smart Systems and Inventive Technology, ICSSIT 2019},
year={2019},
pages={449-453},
art_number={8987972},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85080062789&doi=10.1109%2fICSSIT46314.2019.8987972&partnerID=40&md5=841ab7a7f0dfe415a5a6493f289254b6},
abstract={Unmanned Aerial Vehicles (UAVs) are among the real significant advances that have various significant and advantageous applications. But recently the threats imposed by Unmanned Aerial Vehicles (UAVs), especially small drones, have increased to a greater extent. Unmanned Aerial Vehicles(UAVs) are being misused nowadays for various illegal activities including terrorism and smuggling. Recently, there have been situations where they enter private or confined property. To kill such exercises, a framework has been structured which can distinguish and detect the nearness of obscure little aerial targets, for example, Unmanned Aerial Vehicles (UAVs), specifically small drones. The system is based on the concept of Radio Communication(RC) technology and Internet Protocol(IP) address. This framework is devised such that it detects Internet Protocol(IP) addresses in certain range and using the detected Internet Protocol(IP) addresses and presence or absence of radio waves, detects the presence of Unmanned Aerial Vehicles(UAVs). This system is capable of detecting the presence of unknown Unmanned Aerial Vehicles(UAVs) in certain range. This paper reports on the prototype of the same. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Sedunov2019,
author={Sedunov, A. and Haddad, D. and Salloum, H. and Sutin, A. and Sedunov, N. and Yakubovskiy, A.},
title={Stevens Drone Detection Acoustic System and Experiments in Acoustics UAV Tracking},
journal={2019 IEEE International Symposium on Technologies for Homeland Security, HST 2019},
year={2019},
art_number={9032916},
note={cited By 6},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85078740995&doi=10.1109%2fHST47167.2019.9032916&partnerID=40&md5=f05665e8b9991d975cae8cb3f3ec9c14},
abstract={Concerns about improper use of Unmanned Aerial Vehicles (UAVs, also unmanned aerial systems or UAS) led to the development of various methods for their detection, tracking, and classification. One of the methods is using acoustics. Advantages of passive acoustics include the low cost of acoustic systems, finding of the Direction of Arrival (DOA) and localization by simple means; and classification of UAV sounds by acoustic signature. Stevens Institute of Technology has developed and built the Drone Acoustic Detection System (DADS) that can detect, track and classify UAVs based on the propeller noise. The system consists of three or more microphone nodes. The microphones in each node are arranged in a tetrahedron with configurable size. The microphone data is transferred over WiFi in real-time to a central computer, where it is processed. The Stevens DADS system was investigated in numerous field tests together with several other directional arrays including a 16-channel two-tier cross array, the OptiNav 40-microphone phased array, and parabolic and shot gun microphones. Multirotor UAVs of different sizes were employed in testing, including DJI models Phantom 4, M600 and S1000. The test results of the different systems were compared. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Al-Sa'd201986,
author={Al-Sa'd, M.F. and Al-Ali, A. and Mohamed, A. and Khattab, T. and Erbad, A.},
title={RF-based drone detection and identification using deep learning approaches: An initiative towards a large open source drone database},
journal={Future Generation Computer Systems},
year={2019},
volume={100},
pages={86-97},
note={cited By 44},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85065643831&doi=10.1016%2fj.future.2019.05.007&partnerID=40&md5=70cec981a0d638ffc1f8c6eed12edd9d},
abstract={The omnipresence of unmanned aerial vehicles, or drones, among civilians can lead to technical, security, and public safety issues that need to be addressed, regulated and prevented. Security agencies are in continuous search for technologies and intelligent systems that are capable of detecting drones. Unfortunately, breakthroughs in relevant technologies are hindered by the lack of open source databases for drone's Radio Frequency (RF) signals, which are remotely sensed and stored to enable developing the most effective way for detecting and identifying these drones. This paper presents a stepping stone initiative towards the goal of building a database for the RF signals of various drones under different flight modes. We systematically collect, analyze, and record raw RF signals of different drones under different flight modes such as: off, on and connected, hovering, flying, and video recording. In addition, we design intelligent algorithms to detect and identify intruding drones using the developed RF database. Three deep neural networks (DNN) are used to detect the presence of a drone, the presence of a drone and its type, and lastly, the presence of a drone, its type, and flight mode. Performance of each DNN is validated through a 10-fold cross-validation process and evaluated using various metrics. Classification results show a general decline in performance when increasing the number of classes. Averaged accuracy has decreased from 99.7% for the first DNN (2-classes), to 84.5% for the second DNN (4-classes), and lastly, to 46.8% for the third DNN (10-classes). Nevertheless, results of the designed methods confirm the feasibility of the developed drone RF database to be used for detection and identification. The developed drone RF database along with our implementations are made publicly available for students and researchers alike. © 2019 Elsevier B.V.},
publisher={Elsevier B.V.},
}

@CONFERENCE{Bouzayene2019,
author={Bouzayene, I. and Mabrouk, K. and Gharsallah, A. and Kholodnyak, D.},
title={Scan Radar Using an Uniform Rectangular Array for Drone Detection with Low RCS},
journal={Mediterranean Microwave Symposium},
year={2019},
volume={2019-October},
art_number={9157299},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85090321961&doi=10.1109%2fMMS48040.2019.9157299&partnerID=40&md5=ce478e30d20adf5a8011caa7059700fd},
abstract={Drones are becoming more and more available to the general public for leisure activities and exploited in commercial applications, this boom in drone use has contributed to the emergence of new threats in security applications. Because of their great agility and small size, UAV can be used for numerous missions and are very challenging to detect. Radar technology with its all-weather capability can play an important role in detecting UAV-based threats and in protecting critical assets, but standard radar is ill-prepared for UAV detection: UAVs are low-velocity aircraft with a very weak radar. A radar simulation is discussed and preliminary results are presented. In general, an X-band radar with electronic scanning capability can contribute to a reliable and affordable solution for detecting UAV threats. Radar could be the technology of choice for detecting the drone, signature. © 2019 IEEE.},
publisher={IEEE Computer Society},
}

@CONFERENCE{Huang201913,
author={Huang, R. and Du, X.-Y. and Hu, W.-D.},
title={Phase Compensation Based Multi-frame Coherent Integration for Drone Detection with Radar},
journal={Proceedings of the 2019 IEEE International Conference on Unmanned Systems, ICUS 2019},
year={2019},
pages={13-18},
art_number={8995972},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85080880270&doi=10.1109%2fICUS48101.2019.8995972&partnerID=40&md5=3dfcd51cbfb0c4d235011a4a3da3839c},
abstract={In order to improve the detection ability of small and weak targets such as drones, a multi-frame coherent integration(MFCI) method based on phase compensation is proposed. The phase information of the multi-frame radar echoes is first analyzed and the maximum likelihood estimation(MLE) model of the motion parameters is established. Due to the target motion, the phenomena of migration through range and Doppler cells will occur in the successive frames of target echoes. In order to achieve coherent integration in multiple frames, all the orientations of the multi-frame signal are searched within a certain initial radial velocity and radial acceleration range. The trajectory of each moving target and the corresponding motion parameter values are then obtained, while the phase of the multi-frame signal is located in the same range and the Doppler cell corresponding to a target, thereby improving the detection performance of the weak targets. To further reduce the amount of computation, the influence of radial acceleration on the detection performance of weak targets is studied. Simulation and measured data experiments show that the proposed algorithm can accurately detect drones with less computational complexity. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Bae2019,
author={Bae, K.-B. and Park, J. and Kim, D.-H. and Park, S.-O.},
title={Drone Detection with Linear Chirp Pulse Radar using Coherent Pulse Integration},
journal={2019 International Symposium on Antennas and Propagation, ISAP 2019 - Proceedings},
year={2019},
art_number={8963414},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85079011039&partnerID=40&md5=749e7f61922e57c7d2824c479f10371d},
abstract={This paper discusses the detection of small drone with linear chirp pulse radar system. The system employs 14.1GHz as RF center frequency with bandwidth 200MHz to cover Linear Chirp Pulse (LCP) whose chirp rate is 80MHz. The LCP is radiated and received through quasi-monostatic antennas with the gain of 16dBi. The system also includes digital down converter to obtain IQ signal from LCP received at RX antenna. Finally, Matched filtering of the LCP is performed to maximize the SNR of the signal reflected from the drone. In the actual performance measurement, the drone signal was detected up to 400m distance in real-time using Coherent Pulse Integration (CPI). The raw data is obtained as csv file and then later processed with MATLAB. © 2019 Antenna Branch of Chinese Institute of Electronics.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Park2019,
author={Park, J. and Bae, K.-B. and Jung, D.-H. and Park, S.-O.},
title={Micro-Drone Detection with FMCW Radar Based on Stationary Point Concentration Technique},
journal={2019 International Symposium on Antennas and Propagation, ISAP 2019 - Proceedings},
year={2019},
art_number={8963107},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85078965527&partnerID=40&md5=2267df120fbea87df0c74eae84895ed6},
abstract={This paper shows an interesting detection performance of frequency modulated continuous wave (FMCW) radar. We challenge to detect a micro-drone whose size is about a little finger. Applying the stationary point concentration (SPC) technique, we overcome the inherent problem of leakage in the FMCW radar and set a new record for ultra-small drone detection. The SPC technique attenuates the phase noise of the leakage, and this leads to the reduction of the noise floor in the power spectrum. Therefore, we can expect to detect the beat signal of the micro-drone buried in the noise floor due to its extremely small radar cross section. Experimental results demonstrate that the noise floor is significantly reduced, and the micro-drone buried in the noise floor is detected well. © 2019 Antenna Branch of Chinese Institute of Electronics.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Yang2019,
author={Yang, F. and Qu, K. and Hao, M. and Liu, Q. and Chen, X. and Xu, F.},
title={Practical Investigation of a MIMO Radar System for Small Drones Detection},
journal={2019 International Radar Conference, RADAR 2019},
year={2019},
art_number={9078960},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85084956125&doi=10.1109%2fRADAR41533.2019.171348&partnerID=40&md5=f60fd2cbdccc377001e787c18de7f62f},
abstract={This study presents the latest progress of the MIMO radar system developed for small drones detection. The sparse array optimization method in practical situation is proposed and a target-based MIMO radar array calibration method is presented to improve the signal-to-noise ratio of the target. Experiment in the microwave chamber is conducted to verify the designed sparse array beam pattern and measurement campaigns for small drones are performed to test the system performance. Experimental results and analysis show that the system has good capability in small drones detection and tracking. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Al-Nuaim2019183,
author={Al-Nuaim, T. and Alam, M. and Aldowesh, A.},
title={Low-cost implementation of a multiple-input multiple-output radar prototype for drone detection},
journal={Proceedings Elmar - International Symposium Electronics in Marine},
year={2019},
volume={2019-September},
pages={183-186},
art_number={8918664},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85077554671&doi=10.1109%2fELMAR.2019.8918664&partnerID=40&md5=620f14e799c5f469f55e2eb0c7638222},
abstract={The usage of micro-Unmanned Aerial Vehicles (UAVs) has witnessed an enormous increase recently. Detection of such drones became a necessity nowadays to prevent any harmful activities. Typically, such targets have low velocity and low Radar Cross Section (RCS), making them indistinguishable from clutter and phase noise. Multiple-Input Multiple-Output (MIMO) Radars have many potentials; they increase the degrees of freedom on both transmit and receive ends. Such architecture allows for flexibility in operation, through utilizing the direct access to every element in the transmit/ receive array. MIMO systems allow for several array processing techniques, permitting the system to stare at targets for longer times, which improves the Doppler resolution. In this paper, a 2 × 2 low-cost MIMO radar prototype is developed using Software Defined Radio (SDR) technology, and its performance is evaluated against a slow-moving low radar cross section micro-UAV used by hobbyists. © 2019 IEEE.},
publisher={Croatian Society Electronics in Marine - ELMAR},
}

@CONFERENCE{Sheikh2019,
author={Sheikh, M.U. and Ghavimi, F. and Ruttik, K. and Jantti, R.},
title={Drone detection and classification using cellular network: A machine learning approach},
journal={IEEE Vehicular Technology Conference},
year={2019},
volume={2019-September},
art_number={8891229},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85075244234&doi=10.1109%2fVTCFall.2019.8891229&partnerID=40&md5=7fcc3eb754086277879cb9d6750ba7f5},
abstract={The main target of this paper is to propose a preferred set of features from a cellular network for using as predictors to do the classification between the rogue flying drone User Equipments (UEs) and regular UEs for different Machine Learning (ML) models. Furthermore, the target is to study four different machine learning models i.e. Decision Tree (DT), Logistic Regression (LR). Discriminant Analysis (DA) and K-Nearest Neighbour (KNN) in this paper, and evaluate/compare their performance in terms of identifying the flying drone UE using three performance metrics i.e. True Positive Rate (TPR), False Positive Rate (FPR) and area under Receiver Operating Characteristic (ROC) curve. The simulations are performed using an agreed 3GPP scenario, and a MATLAB machine learning tool box. All considered ML models provide high drone detection probability for drones flying at 60 m and above height. However, the true drone detection probability degrades for drones at lower altitude. Whereas, the fine DT method and the coarse KNN model performs relatively better compared with LR and DA at low altitude, and therefore can be considered as a preferable choice for a drone classification problem. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Aldowesh2019203,
author={Aldowesh, A. and Binkhamis, T. and Alnuaim, T. and Alzogaiby, A.},
title={Low Power Digital Array Radar for Drone Detection and Micro-Doppler Classification},
journal={2019 Signal Processing Symposium, SPSympo 2019},
year={2019},
pages={203-206},
art_number={8882033},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85074939707&doi=10.1109%2fSPS.2019.8882033&partnerID=40&md5=910444761223c597ecb6be218d7673d6},
abstract={Due to the ever-increasing threat of micro-Unmanned Aerial Vehicles (UAVs), a necessity arises for robust detection and classification methods. Generally, radar sensor face difficulties in discriminating micro-UAVs from flying birds, as they have comparable Radar Cross Section (RCS) and velocity profiles. Exploiting the uniqueness of their respective micro-Doppler signature could alleviate the issue. In this paper, an experimental investigation is conducted to analyze different micro-Doppler signatures for different consumer drones in different frequency bands, with the aim to clearly distinguish a drone from other flying targets with similar characteristics. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Craye2019,
author={Craye, C. and Ardjoune, S.},
title={Spatio-temporal semantic segmentation for drone detection},
journal={2019 16th IEEE International Conference on Advanced Video and Signal Based Surveillance, AVSS 2019},
year={2019},
art_number={8909854},
note={cited By 18},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85074797380&doi=10.1109%2fAVSS.2019.8909854&partnerID=40&md5=844b1929ed75e84a25875281e2ac9007},
abstract={The democratization of drones over the past decade has opened wide cracks in airspace security. Research in drone detection and neutralization for critical infrastructures is a very active area with a number of open issues, such as robust detection of drones based on opto-electronic imaging. Indeed, drones at a certain distance only represent a few pixel points on an image, even on a high resolution camera, and can be easily mistaken for birds or any other flying objects in the airspace. In this context, we propose a spatio-temporal semantic segmentation approach based on convolutional neural networks. We handle the problem of detecting very small targets by using a U-Net architecture to identify areas of interest within the larger image. Then, we use a classification network, ResNet, to determine whether those areas contain a drone or not. To further help the localization and classification process, we provide spatiotemporal input patches to our networks. Drones are mostly moving targets, and birds do not follow the same kinds of trajectories; therefore, this additional feature significantly increases overall performance. This work was carried out in the context of the 2019 Drone-vs-Bird detection Challenge. The evaluation is conducted on the provided dataset under several configurations. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Nalamati2019,
author={Nalamati, M. and Kapoor, A. and Saqib, M. and Sharma, N. and Blumenstein, M.},
title={Drone detection in long-range surveillance videos},
journal={2019 16th IEEE International Conference on Advanced Video and Signal Based Surveillance, AVSS 2019},
year={2019},
art_number={8909830},
note={cited By 19},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85074766085&doi=10.1109%2fAVSS.2019.8909830&partnerID=40&md5=43cc8abf956394d22103009723198283},
abstract={The usage of small drones/UAVs has significantly increased recently. Consequently, there is a rising potential of small drones being misused for illegal activities such as terrorism, smuggling of drugs, etc. posing high-security risks. Hence, tracking and surveillance of drones are essential to prevent security breaches. The similarity in the appearance of small drone and birds in complex background makes it challenging to detect drones in surveillance videos. This paper addresses the challenge of detecting small drones in surveillance videos using popular and advanced deep learning-based object detection methods. Different CNN-based architectures such as ResNet-101 and Inception with Faster-RCNN, as well as Single Shot Detector (SSD) model was used for experiments. Due to sparse data available for experiments, pre-trained models were used while training the CNNs using transfer learning. Best results were obtained from experiments using Faster-RCNN with the base architecture of ResNet-101. Experimental analysis on different CNN architectures is presented in the paper, along with the visual analysis of the test dataset. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{DeQuevedo20191437,
author={De Quevedo, A.D. and Urzaiz, F.I. and Menoyo, J.G. and López, A.A.},
title={Drone detection and radar-cross-section measurements by RAD-DAR},
journal={IET Radar, Sonar and Navigation},
year={2019},
volume={13},
number={9},
pages={1437-1447},
note={cited By 10},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85071233759&doi=10.1049%2fiet-rsn.2018.5646&partnerID=40&md5=6058161749424ac745115cdb196d65fd},
abstract={RAD-DAR is a frequency-modulated-continuous-wave radar demonstrator, working at X-band, completely designed and constructed by the authors' research group following the ubiquitous-radar concept. After introducing its main hardware and software blocks, with special emphasis to its off-line signal processing and data processing, this study presents the results of a drone detection test, where RAD-DAR achieved a DJI-Phantom 4 detection and tracking at a range up to 3 km. The system performance is discussed with different flights including an attack manoeuvre, and a free flight, which helps to highlight their advantages in surveillance tasks due to the RAD-DAR staring nature. Furthermore, range, speed and azimuth accuracies are discussed, considering the drone global positioning system data. Finally, this study shows a statistical radar cross-section study based on the processed data of the drone and attempts to classify this target by means of Swerling models. © The Institution of Engineering and Technology 2019.},
publisher={Institution of Engineering and Technology},
}

@CONFERENCE{Abbasi2019,
author={Abbasi, K. and Batool, A. and Fawad and Asghar, M.A. and Saeed, A. and Khan, M.J. and Ur Rehman, M.},
title={A Vision-Based Amateur Drone Detection Algorithm for Public Safety Applications},
journal={2019 UK/China Emerging Technologies, UCET 2019},
year={2019},
art_number={8881879},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85074919038&doi=10.1109%2fUCET.2019.8881879&partnerID=40&md5=43bd2d5d5e074a9d9c8d33c0bb6e0453},
abstract={Drones will be widely used in the smart cities of the future for the wireless approach, supplying goods, and for conserving the security of smart cities. Apart from the various benefits of the drones, they pose significant challenges and public concerns that need to be tackled. We propose an amenable framework to detect malicious drone and ensure public safety. The proposed model is validated using 400 images with various challenges such as occlusion, scale variation, blurriness, background clutter, and low illumination. After extracting the features using ResNet50 model, we applied SVM's RBF kernel for the classification. The classification accuracy presented in the confusion matrix for this model came out to be the highest in comparison to other state-of-the-art models. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Hamatapa2019,
author={Hamatapa, R. and Vongchumyen, C.},
title={Image processing for drones detection},
journal={Proceeding - 5th International Conference on Engineering, Applied Sciences and Technology, ICEAST 2019},
year={2019},
art_number={8802578},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85071731152&doi=10.1109%2fICEAST.2019.8802578&partnerID=40&md5=e9a3803c9d735e21a2246b3d9b9e5958},
abstract={Presently, Drones Quadcopter has caused tremendous problems threatening the military security boundary and the area under Thai Army's surveillance. This article presents a conceptual framework for detecting and tracking unmanned aircraft by applying image processing. Study and analysis Compare advantages and disadvantages in order to develop and provide suitable equipment and tools Replacement of imported high-priced With limiting factors, namely distance, time, terrain And interference resistance The researchers used the camera USB 3.0 Cameras and Open Source Computer Vision (OpenCV) as a software development library on Linux operating systems to automatically record movies. In order to bring the image to analyze and distinguish the object classification by using Machine Learning through a sample of correct information and some incorrect information. Which when detecting, the installed device will calculate the coordinates detected, lock the target, track the movement Voice notification and report. The experiment was conducted by using Anova to test various factors affecting the detection, such as speed, light, color and size in 350 feet with the equipment we installed. The results of the experiment concluded that there was only a speed that had an effect at 22.65. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@BOOK{Cianca201975,
author={Cianca, E. and Di Domenico, S. and De Sanctis, M. and Rossi, T.},
title={EM-based drone-detection/identification for safety purposes},
journal={Security within CONASENSE Paragon},
year={2019},
pages={75-84},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85106563716&partnerID=40&md5=8e522c5bbd43df916890522911cae715},
abstract={Drone surely could be effectively used to improve the safety in several applications (e.g., transport applications, surveillance). On the other hand, they also represent a threat to safety and security. Therefore, both for civil and military applications, it is crucial to develop cost-effective detection systems to warn of the presence of drones. In many military applications, it is also important to be able to identify the drone at some extent (the model, dimension etc.). This Chapter reviews the main approaches proposed for drone detection/identification, mainly focusing on the class of techniques based on the analysis of some Electromagnetic (EM) signature, which includes: 1. Detection based on the analysis of the signature of Radio Frequency (RF) signals intentionally emitted by the drone. 2. Detection based on the analysis of the signature of more general EM signals not intentionally emitted by the drone. 3. Detection based on the analysis of the signature of RF signals reflected by the drone and transmitted by sources of opportunity. Some original results are presented and open challenges highlighted. © 2019 River Publishers. All rights reserved.},
publisher={River Publishers},
}

@CONFERENCE{Al-Emadi2019459,
author={Al-Emadi, S. and Al-Ali, A. and Mohammad, A. and Al-Ali, A.},
title={Audio based drone detection and identification using deep learning},
journal={2019 15th International Wireless Communications and Mobile Computing Conference, IWCMC 2019},
year={2019},
pages={459-464},
art_number={8766732},
note={cited By 25},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85072648004&doi=10.1109%2fIWCMC.2019.8766732&partnerID=40&md5=a98bf02cf101498ad35beea2b45bd2d3},
abstract={In recent years, unmanned aerial vehicles (UAVs) have become increasingly accessible to the public due to their high availability with affordable prices while being equipped with better technology. However, this raises a great concern from both the cyber and physical security perspectives since UAVs can be utilized for malicious activities in order to exploit vulnerabilities by spying on private properties, critical areas or to carry dangerous objects such as explosives which makes them a great threat to the society. Drone identification is considered the first step in a multi-procedural process in securing physical infrastructure against this threat. In this paper, we present drone detection and identification methods using deep learning techniques such as Convolutional Neural Network (CNN), Recurrent Neural Network (RNN) and Convolutional Recurrent Neural Network (CRNN). These algorithms will be utilized to exploit the unique acoustic fingerprints of the flying drones in order to detect and identify them. We propose a comparison between the performance of different neural networks based on our dataset which features audio recorded samples of drone activities. The major contribution of our work is to validate the usage of these methodologies of drone detection and identification in real life scenarios and to provide a robust comparison of the performance between different deep neural network algorithms for this application. In addition, we are releasing the dataset of drone audio clips for the research community for further analysis. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Musa2019,
author={Musa, S.A. and Rsa, R.A. and Sali, A. and Isma'Il, A. and Rashid, N.E.A.},
title={DVBS based forward scattering radar for drone detection},
journal={Proceedings International Radar Symposium},
year={2019},
volume={2019-June},
art_number={8767456},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85069924832&doi=10.23919%2fIRS.2019.8767456&partnerID=40&md5=4cdd64c869693f2cb9e698d1e08baade},
abstract={The drone detection challenge of implementing satellite base passive radar for air surveillance among others were low received power, short integration time, target receiver ranges etc. Following some identified benefits of forward scattering radar (FSR) geometry over conventional radars such as improved radar cross section RCS value irrespective of radar absorbing material (RAM), direct signal perturbation and high resolutions, this paper aimed at a feasibility study of implementing passive FSR by using Measat3a/3/3b Malaysian Satellite for a drone detection. This was achieved by analyzing the signal properties such as ambiguity function, power budget, target-to-receiver range profile. The paper further validated the claim with an actual signal from the Measat3 satellite. The resulted analysis of the signal ambiguity, minimum acceptable signal-to-Noise ratio (SNR) and the range profile was encouraging hence, manifesting the possibility of implementing this satellite for drone detection in FSR geometry. © 2019 German Institute of Navigation (DGON).},
publisher={IEEE Computer Society},
}

@CONFERENCE{Shinde2019289,
author={Shinde, C. and Lima, R. and Das, K.},
title={Multi-view Geometry and Deep Learning Based Drone Detection and Localization},
journal={2019 5th Indian Control Conference, ICC 2019 - Proceedings},
year={2019},
pages={289-294},
art_number={8715593},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85066635626&doi=10.1109%2fINDIANCC.2019.8715593&partnerID=40&md5=0f98338a93e57d4b1529b60ee355cb30},
abstract={A real-time vision based detection and 3D pose estimation of intruder Unmanned Aerial Vehicles (UAVs) is presented. Proposed method utilizes a cooperative team of UAVs mounted with monocular camera to detect the intruder UAV and simultaneously localize it. Detection is performed by using YOLOv2 deep learning network architecture while the position is obtained using multi-view geometry. General dynamics of the drone are considered to improve the target position estimate obtained from the image based estimate. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Ryden2019,
author={Ryden, H. and Redhwan, S.B. and Lin, X.},
title={Rogue Drone Detection: A Machine Learning Approach},
journal={IEEE Wireless Communications and Networking Conference, WCNC},
year={2019},
volume={2019-April},
art_number={8886040},
note={cited By 7},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85074749102&doi=10.1109%2fWCNC.2019.8886040&partnerID=40&md5=0e3d6ad15ea9cd96bbf85be2382f3680},
abstract={The emerging, practical and observed issue of how to detect rogue drones carrying terrestrial user equipment (UE) on mobile networks is addressed in this paper. This issue has drawn much attention since the rogue drones may generate excessive interference to mobile networks and may not be allowed by regulations in some regions. In this paper, we propose a novel machine learning approach to identify the rogue drones in mobile networks based on radio measurements. We apply two classification machine learning models, Logistic Regression, and Decision Tree, using features from radio measurements to identify the rogue drones. Simulation results show that the proposed machine learning solutions can achieve high rogue drone detection rate for high altitudes while not mis-classifying regular ground based UEs as rogue drone UEs. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Fang2019,
author={Fang, X. and Min, R. and Cao, Z. and Pi, Y.},
title={A coherent integration method for drone detection via PSIAF-KT-SFT},
journal={2019 IEEE Radar Conference, RadarConf 2019},
year={2019},
art_number={8835565},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85073102081&doi=10.1109%2fRADAR.2019.8835565&partnerID=40&md5=dbc7025857149eb583e13241948da8ff},
abstract={In this paper, the coherent integration for drone detection is considered and a method based on parametric symmetric instantaneous autocorrelation function (PSIAF), keystone transform (KT) and scaled Fourier transform (SFT), i.e., PSIAF-KT-SFT, is presented. To be specific, the PSIAF is first applied to eliminate the quadratic range migration (RM) and Doppler frequency migration (DFM) induced by the acceleration. Then, the residual linear RM can be removed by KT and SFT. After that, the motion parameters of drone can be estimated via the Fourier transform (FT) with respect to the lag time. Based on the estimated motion parameters, the coherent integration can be achieved and the target energy can be accumulated at one point, which can be used for drone detection. Finally, the simulations and real experiment are performed to demonstrate the effectiveness. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Jin2019,
author={Jin, R. and Jiang, J. and Qi, Y. and Lin, D. and Song, T.},
title={Drone detection and pose estimation using relational graph networks},
journal={Sensors (Switzerland)},
year={2019},
volume={19},
number={6},
art_number={1479},
note={cited By 15},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85063965882&doi=10.3390%2fs19061479&partnerID=40&md5=c9f6571e06a119bd5428eb77b196be7c},
abstract={With the upsurge in use of Unmanned Aerial Vehicles (UAVs), drone detection and pose estimation by using optical sensors becomes an important research subject in cooperative flight and low-altitude security. The existing technology only obtains the position of the target UAV based on object detection methods. To achieve better adaptability and enhanced cooperative performance, the attitude information of the target drone becomes a key message to understand its state and intention, e.g., the acceleration of quadrotors. At present, most of the object 6D pose estimation algorithms depend on accurate pose annotation or a 3D target model, which costs a lot of human resource and is difficult to apply to non-cooperative targets. To overcome these problems, a quadrotor 6D pose estimation algorithm was proposed in this paper. It was based on keypoints detection (only need keypoints annotation), relational graph network and perspective-n-point (PnP) algorithm, which achieves state-of-the-art performance both in simulation and real scenario. In addition, the inference ability of our relational graph network to the keypoints of fourmotors was also evaluated. The accuracy and speed were improved significantly compared with the state-of-the-art keypoints detection algorithm. © 2019 by the authors. Licensee MDPI, Basel, Switzerland.},
publisher={MDPI AG},
}

@ARTICLE{Anwar20192526,
author={Anwar, M.Z. and Kaleem, Z. and Jamalipour, A.},
title={Machine Learning Inspired Sound-Based Amateur Drone Detection for Public Safety Applications},
journal={IEEE Transactions on Vehicular Technology},
year={2019},
volume={68},
number={3},
pages={2526-2534},
art_number={8616877},
note={cited By 67},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85063268841&doi=10.1109%2fTVT.2019.2893615&partnerID=40&md5=67048e28db8737300a105a236a170928},
abstract={In recent years, popularity of unmanned air vehicles enormously increased due to their autonomous moving capability and applications in various domains. This also results in some serious security threats, that needs proper investigation and timely detection of the amateur drones (ADr) to protect the security sensitive institutions. In this paper, we propose the novel machine learning (ML) framework for detection and classification of ADr sounds out of the various sounds like bird, airplanes, and thunderstorm in the noisy environment. To extract the necessary features from ADr sound, Mel frequency cepstral coefficients (MFCC), and linear predictive cepstral coefficients (LPCC) feature extraction techniques are implemented. After feature extraction, support vector machines (SVM) with various kernels are adopted to accurately classify these sounds. The experimental results verify that SVM cubic kernel with MFCC outperform LPCC method by achieving around 96.7% accuracy for ADr detection. Moreover, the results verified that the proposed ML scheme has more than 17% detection accuracy, compared with correlation-based drone sound detection scheme that ignores ML prediction. © 1967-2012 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Park20191221,
author={Park, J. and Park, S. and Kim, D.-H. and Park, S.-O.},
title={Leakage mitigation in heterodyne FMCW radar for small drone detection with stationary point concentration technique},
journal={IEEE Transactions on Microwave Theory and Techniques},
year={2019},
volume={67},
number={3},
pages={1221-1232},
art_number={8605523},
note={cited By 27},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85062601083&doi=10.1109%2fTMTT.2018.2889045&partnerID=40&md5=11296dcb9780c8004494799ee34659a6},
abstract={To prevent potential hazards posed by fast-evolving drones, it is of importance to develop a radar system for drone detection. Frequency modulated continuous wave (FMCW) radars are widely used for that purpose. Heterodyne architectures are preferred for them to mitigate dc offset errors. Having said that, FMCW radars suffer from permanent leakage from the transmitter into the receiver. The leakage phase noise raises the total noise floor and limits the radar sensitivity. Here, we propose a stationary point concentration (SPC) technique in order to overcome the challenges. The SPC technique concentrates the leakage phase noise on a stationary point to alleviate the impact of the noise. The technique can be realized using digital signal processing without additional hardware. The results show that the proposed technique significantly lowers the noise floor. © 2018 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Wang2019433,
author={Wang, Z. and Qi, L. and Tie, Y. and Ding, Y. and Bai, Y.},
title={Drone Detection Based on FD-HOG Descriptor},
journal={Proceedings - 2018 International Conference on Cyber-Enabled Distributed Computing and Knowledge Discovery, CyberC 2018},
year={2019},
pages={433-436},
art_number={8644586},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85063145266&doi=10.1109%2fCyberC.2018.00084&partnerID=40&md5=6657d876de16f62325a32302b0076bdc},
abstract={The rapid development of Unmanned Aerial Vehicle (UAV) technology, also known as drones, has made people benefit in many ways, but it also brings privacy and security issues, such as appeared at private place, airports, prisons, etc. Therefore, the detection of drones in a specific area is crucial. Video detection is an effective method with various advantages. In this paper, we have used the background subtraction method to detect the moving object in the video sequence which recorded by static cameras, then extracted the global Fourier descriptors and the local HOG features of the moving object images. Finally, the FD+HOG features have been sent to the SVM classifier for classification and recognition. Our algorithm is simple and efficient, an overall with 98% accuracy was obtained in our data set. © 2018 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Seo2019,
author={Seo, Y. and Jang, B. and Im, S.},
title={Drone Detection Using Convolutional Neural Networks with Acoustic STFT Features},
journal={Proceedings of AVSS 2018 - 2018 15th IEEE International Conference on Advanced Video and Signal-Based Surveillance},
year={2019},
art_number={8639425},
note={cited By 9},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85063251483&doi=10.1109%2fAVSS.2018.8639425&partnerID=40&md5=03bf052d7171a6061b73ed58200310fd},
abstract={As the use of drones has raised in the city, the regulation of malicious usage of drones is an important issue. However, it is difficult to detect a drone due to its miniaturization and modification. In this paper, we investigate the performance of using the convolutional neural networks (CNN) for detecting drones with the acoustic signals received by a microphone. Since the harmonic characteristics of drones are different from those of the objects that produce similar noise including scooters and motorcycles, the two-dimensional feature employed in the study is made of the normalized short time Fourier transform (STFT) magnitude. The performance of the proposed approach is evaluated in terms of detection rate and false alarm rate under various environments. The dataset used in this study consists of the measurements through experiments. The experiments are carried out in the open space with a hovering drone, which is DJI Phantom 3 or Phantom 4. The dataset contains 68,931 frames of drone sound and 41,958 frames of non-drone sound. For the 100-epoch model, the detection rate is 98.97 % and the false alarm rate is 1.28, while the 10-epoch model demonstrates the detection rate of 98.77 % and the false alarm rate of 1.62 %. © 2018 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Minz2019,
author={Minz, L. and Kang, H.-S. and Azim, M.T. and Aziz, R.S. and Park, S.-O.},
title={Wide-beam Choke Horn Antenna for Small Drone Detection},
journal={ISAP 2018 - 2018 International Symposium on Antennas and Propagation},
year={2019},
art_number={8627548},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85062788915&partnerID=40&md5=3e2d7097a0318eb5756f5897e754b070},
abstract={A conventional narrow beam scanning antenna radar systems are inept in detection of small RCS drones. A wide-beam choke horn antennas are proposed for the surveillance system in order to detect and track a small object like drones. The proposed choke horn antenna is derived from sector beam pattern synthesis. The designed antenna has a wide beam width of 700 and has a low field level in the horizontal plane (-40dB w.r.t. main beam), which is crucial for high isolation among Rx and between Tx and Rx as well. © 2018 KIEES.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Li2019101527,
author={Li, T. and Wen, B. and Tian, Y. and Wang, S. and Yin, Y.},
title={Optimized Radar Waveform Parameter Design for Small Drone Detection Based on Echo Modeling and Experimental Analysis},
journal={IEEE Access},
year={2019},
volume={7},
pages={101527-101538},
art_number={8772049},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85079762663&doi=10.1109%2fACCESS.2019.2931087&partnerID=40&md5=06d156b608f328bf5837183b6ce8976a},
abstract={Monitoring small drones is significant for security requirements, but it is challenging because of small drones' low radar cross section (RCS) and hovering ability. In order to analyze the effect of radar waveform on the echo spectra and optimize the waveform design, an analytical expression of the rotor's temporal RCS is desired. Integral model, a widely used radar echo model of the rotor's temporal RCS, does not involve the electromagnetic scattering, thus it cannot be applied to all frequency bands. The method of moments (MoM) is a strictly numerical method based on the Maxwell's equations, but cannot obtain the analytical expression. Hence, this paper proposes a new method combing the integral model and MoM to model the rotor's temporal RCS in very high frequency (VHF) band. The linear frequency modulation (LFM) signal which has a high Doppler tolerance and a large gain bandwidth product is adopted in optimizing waveform parameters design. Based on the new method, the analytical expression of LFM echo is also derived. Moreover, the spectral spread over range and Doppler dimension caused by the rotating rotors is analyzed in detail. A criterion for optimizing the LFM waveform parameters for small drone detection is presented. Field experiments confirm the validity of the echo model and waveform parameters optimization criterion, and the full Acrylonitrile Butadiene Styrene small drone is successfully detected in VHF band. In addition, experiments are implemented to verify the applicability of the echo model and waveform parameters optimization method to other drones with different size. © 2013 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Doroftei201920,
author={Doroftei, D. and De Cubber, G.},
title={Using a qualitative and quantitative validation methodology to evaluate a drone detection system},
journal={Acta IMEKO},
year={2019},
volume={8},
number={4},
pages={20-27},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85078848965&doi=10.21014%2facta_imeko.v8i4.682&partnerID=40&md5=8561520b4ff6c1ec7b1d70b6b33e12fe},
abstract={Now that the use of drones is becoming more common, the need to regulate the access to airspace for these systems is becoming more pressing. A necessary tool in order to do this is a means of detecting drones. Numerous parties have started the development of such drone detection systems. A big problem with these systems is that the evaluation of the performance of drone detection systems is a difficult operation that requires the careful consideration of all technical and non-technical aspects of the system under test. Indeed, weather conditions and small variations in the appearance of the targets can have a huge difference on the performance of the systems. In order to provide a fair evaluation, it is therefore paramount that a validation procedure that finds a compromise between the requirements of end users (who want tests to be performed in operational conditions) and platform developers (who want statistically relevant tests) is followed. Therefore, we propose in this article a qualitative and quantitative validation methodology for drone detection systems. The proposed validation methodology seeks to find this compromise between operationally relevant benchmarking (by providing qualitative benchmarking under varying environmental conditions) and statistically relevant evaluation (by providing quantitative score sheets under strictly described conditions). © 2019 International Measurement Confederation (IMEKO). All rights reserved.},
publisher={International Measurement Confederation (IMEKO)},
}

@ARTICLE{Taha2019138669,
author={Taha, B. and Shoufan, A.},
title={Machine Learning-Based Drone Detection and Classification: State-of-the-Art in Research},
journal={IEEE Access},
year={2019},
volume={7},
pages={138669-138682},
art_number={8846214},
note={cited By 54},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85078236502&doi=10.1109%2fACCESS.2019.2942944&partnerID=40&md5=575c82fa20e3d8f40b3156f9d4894e5f},
abstract={This paper presents a comprehensive review of current literature on drone detection and classification using machine learning with different modalities. This research area has emerged in the last few years due to the rapid development of commercial and recreational drones and the associated risk to airspace safety. Addressed technologies encompass radar, visual, acoustic, and radio-frequency sensing systems. The general finding of this study demonstrates that machine learning-based classification of drones seems to be promising with many successful individual contributions. However, most of the performed research is experimental and the outcomes from different papers can hardly be compared. A general requirement-driven specification for the problem of drone detection and classification is still missing as well as reference datasets which would help in evaluating different solutions. © 2013 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Huber2019,
author={Huber, S. and Wellig, P. and Heutschi, K.},
title={Determination of the detection threshold of human observers in acoustic drone detection},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2019},
volume={11158},
art_number={111580L},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85078152144&doi=10.1117%2f12.2533174&partnerID=40&md5=af0a1d59fb4677ef5b6fa0422ca42e7d},
abstract={Background: Nowadays, small drones are inexpensive and can be purchased and used very easily. Unfortunately, they are also relatively easy to convert to weapons. As they become more widespread, these drones may become a serious security risk. One possible way to address this threat could be the early detection of small drones by using acoustic cameras. However, the question arises as to how good the detection performance of such cameras is, compared to that of a human observer. The goal of this project was to determine the acoustic detection-threshold of human observers for drones in the presence of ambient noise. Methods: Nineteen subjects volunteered to take part in the study. The constancy method was used to determine the detection threshold. During the test, the study participants were presented with a recording of a DJI Phantom2 Vision+ drone that varied in level in steps of 1dB over a range of 27dB around the estimated threshold value. The signals were superimposed by three different kinds of ambient noise which were presented in three successive test-runs. The subjects wore headphones over which they heard the ongoing ambient noise while they were presented with the drone sound at random intervals and levels. The test signal was on for 2 seconds during which the trial subject had to confirm the detection of the drone sound by pressing an assigned key on a notebook. Results: We've found detection thresholds for white noise, water or highway noise at -17dB, -18dB and -17dB respectively, expressed as level differences between test signal and noise. Comparison of our results with the detection performance of human observers in a simulated drone detection scenario, reproduced by loudspeakers in an anechoic chamber, showed good agreement. Further, it seems possible to assess the detection performance of an acoustic camera using our results. Copyright © 2019 SPIE.},
publisher={SPIE},
}

@CONFERENCE{Müller2019,
author={Müller, T. and Erdnüß, B.},
title={Robust drone detection with static VIS and SWIR cameras for day and night counter-UAV},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2019},
volume={11166},
art_number={111660B},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85077318440&doi=10.1117%2f12.2537940&partnerID=40&md5=ed04b50c349fab64b6eedcf5c13f4864},
abstract={Considerable progress with unmanned aerial vehicles (UAVs) has led to an increasing need for counter-UAV systems to detect present, potentially threatening or misused drones. Therefore, a UAV detection algorithm has been developped recently for day and night operation. Whereas high resolution VIS cameras enable to detect UAVs in daylight in further distances, surveillance at night is performed with a short wave infrared (SWIR) camera. The proposed method is based on temporal median computation, structural adaptive image differencing, codebook-based background learning, local density computation, and shape analysis of foreground structures to perform an improved near range change detection for UAVs. Areas with moving scene parts, like leaves in the wind or driving cars on a street, are recognized to minimize false alarms. This paper presents a significant improvement with respect to some of the most challenging tasks in this field, e.g., increasing the UAV detection sensitivity in front of trees with waving leaves, false alarm minimization, and avoiding the background model update problem. The provided results illustrate the reached performance in a variety of different situations. © 2019 SPIE.},
publisher={SPIE},
}

@ARTICLE{Musa201916,
author={Musa, S.A. and Abdullah, R.S.A.R. and Sali, A. and Ismail, A. and Rashid, N.E.A. and Ibrahim, I.P. and Salah, A.A.},
title={A review of copter drone detection using radar systems},
journal={Defence S and T Technical Bulletin},
year={2019},
volume={12},
number={1},
pages={16-38},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85072774419&partnerID=40&md5=021fb3184bb9977290054a6df9ec5007},
abstract={The exponential growth of copter drone usage and the threats posed by drone users, such as unauthorised imaging and filming in restricted areas, illegal surveillance, air collisions, drug smuggling, terrorist attacks, and radio frequency (RF) jamming, have led to many efforts and research projects aimed at drone detection. The attempted methodologies include using acoustics, cameras, cascades (audio-visual) and radio frequency. In addition, there are the nontechnical methods such as shooting and netting. This paper presents radar systems as a method for copter drone detection. It presents the state of the art review of the efforts so far made towards detecting drones given preference to radar systems for micro-Doppler-based analysis. It also introduces passive forward scatter radar (PFSR) as an emerging methodology, presenting its reported achievements for both ground and airborne target detection. In an attempt to improve the detection of low-profile targets, this paper discusses the basic parameters aiding Doppler and micro-Doppler analysis of a copter drone. The paper concludes by proposing digital video broadcasting satellite (DVBS) based PFSR for drone detection due to its improved capabilities, thereby making micro- Doppler analysis for a low-profile target, a feasible endeavour. © 2019, Science and Technology Research Institute for Defence.},
publisher={Science and Technology Research Institute for Defence},
}

@CONFERENCE{Bello2019,
author={Bello, A. and Biswal, B. and Shetty, S. and Kamhoua, C. and Gold, K.},
title={Radio frequency classification toolbox for drone detection},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2019},
volume={11006},
art_number={110061Y},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85072574963&doi=10.1117%2f12.2514759&partnerID=40&md5=e14fe88cfefbab09beb3625798aa87e6},
abstract={There is a need for Radio Frequency Signal Classification (RF-Class) toolbox which can monitor, detect, and classify wireless signals. Rapid developments in the unmanned aerial systems (UAS) have made its usage in a variety of offensive as well as defensive applications especially in military, high priority and sensitive government sites. The ability to accurately classify over-The-Air radio signals will provide insights into spectrum utilization, device fingerprinting and protocol identification. These insights can help the Warfighter to constantly be informed about adversarys transmitters capabilities without their knowledge. Recently, few researches have proposed feature-based machine learning techniques to classify RF signals. However, these researches are mostly evaluated on simulated environments, less accurate, and failed to explore advance machine learning techniques. In this research, we proposed a feature-engineering based signal classification (RF-class) toolbox which implements RF signal detection, Cyclostationary Features Extraction and Feature engineering, Automatic Modulation Recognition to automatically recognize modulation as well as sub-modulation types of the received signal. To demonstrate the feasibility and accuracy of our approach, we have evaluated the performance on a real environment with an UAS (Drone DJI Phantom 4). Our initial experimental result showed that we were able to detect presence of drone signal successfully when power on and transmitting. And further experiments are under progress. © COPYRIGHT SPIE. Downloading of the abstract is permitted for personal use only.},
publisher={SPIE},
}

@CONFERENCE{Doroftei201994,
author={Doroftei, D. and De Cubber, G.},
title={Qualitative and quantitative validation of drone detection systems},
journal={21st International Symposium on Measurement and Control in Robotics, ISMCR 2018},
year={2019},
pages={94-97},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85072317302&partnerID=40&md5=8e31b6a7a347ac1d19dc342783a21af1},
abstract={As drones are more and more entering our world, so comes the need to regulate the access to airspace for these systems. A necessary tool in order to do this is a means of detecting these drones. Numerous commercial and non-commercial parties have started the development of such drone detection systems. A big problem with these systems is that the evaluation of the performance of drone detection systems is a difficult operation, which requires the careful consideration of all technical and non-technical aspects of the system under test. Indeed, weather conditions and small variations in the appearance of the targets can have a huge difference on the performance of the systems. In order to provide a fair evaluation and an honest comparison between systems, it is therefore paramount that a stringent validation procedure is followed. Moreover, the validation methodology needs to find a compromise between the often contrasting requirements of end users (who want tests to be performed in operational conditions) and platform developers (who want tests to be performed that are statistically relevant). Therefore, we propose in this paper a qualitative and quantitative validation methodology for drone detection systems. The proposed validation methodology seeks to find this compromise between operationally relevant benchmarking (by providing qualitative benchmarking under varying environmental conditions) and statistically relevant evaluation (by providing quantitative score sheets under strictly described conditions). © (2018) by the International Measurement Confederation (IMEKO). All rights reserved.},
publisher={International Measurement Confederation (IMEKO)},
}

@ARTICLE{Yi2019359,
author={Yi, K.Y. and Kyeong, D. and Seo, K.},
title={Deep learning based drone detection and classification},
journal={Transactions of the Korean Institute of Electrical Engineers},
year={2019},
volume={68},
number={2},
pages={359-363},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85062906099&doi=10.5370%2fKIEE.2019.68.2.359&partnerID=40&md5=8a853f62f87ed98ed16975405409adab},
abstract={As commercial drones have been widely used, concerns for collision accidents with people and invading secured properties are emerging. The detection of drone is a challenging problem. The deep learning based object detection techniques for detecting drones have been applied, but limited to the specific cases such as detection of drones from bird and/or background. We have tried not only detection of drones, but classification of different drones with an end-to-end model. YOLOv2 is used as an object detection model. In order to supplement insufficient data by shooting drones, data augmentation from collected images is executed. Also transfer learning from ImageNet for YOLOv2 darknet framework is performed. The experimental results for drone detection with average IoU and recall are compared and analysed. ? The Korean Institute of Electrical Engineers. Copyright ⓒ The Korean Institute of Electrical Engineers.},
publisher={Korean Institute of Electrical Engineers},
}

@ARTICLE{Fang2019472,
author={Fang, X. and Lu, C. and Zhang, M. and Min, R.},
title={Micro drone detection and parameters estimation based on micro-doppler of blades},
journal={Lecture Notes in Electrical Engineering},
year={2019},
volume={463},
pages={472-478},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85048656429&doi=10.1007%2f978-981-10-6571-2_57&partnerID=40&md5=28f3d36b0b8eab5f17237f107467149a},
abstract={Small unmanned aerial vehicles (UAVs) or micro drones are widely used for many applications in these years. But the misuse of micro drones may cause security issues. The problem of micro drone detection and parameters estimation is considered in this paper. Micro Doppler signatures of the drone’s rotating rotor blades are applied to identify micro drone. Firstly, the signal mathematical model of drone’s rotating multi-rotor blades is built and the flashes are used for detection. Then, the relationship between the micro Doppler signatures and the parameters of drones is analyzed. Furthermore, parameters, such as the number of blades, the number of rotor, the rotation rate and the length of blade, are estimated in this article. Finally, the results show that the effectiveness of the proposed method. © Springer Nature Singapore Pte Ltd. 2019.},
publisher={Springer Verlag},
}

@CONFERENCE{Carrio20181034,
author={Carrio, A. and Vemprala, S. and Ripoll, A. and Saripalli, S. and Campoy, P.},
title={Drone Detection Using Depth Maps},
journal={IEEE International Conference on Intelligent Robots and Systems},
year={2018},
pages={1034-1037},
art_number={8593405},
note={cited By 16},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85063002552&doi=10.1109%2fIROS.2018.8593405&partnerID=40&md5=900de0d0c8125401bceea47acfa1ffed},
abstract={Obstacle avoidance is a key feature for safe Unmanned Aerial Vehicle (UAV) navigation. While solutions have been proposed for static obstacle avoidance, systems enabling avoidance of dynamic objects, such as drones, are hard to implement due to the detection range and field-of-view (FOV) requirements, as well as the constraints for integrating such systems on-board small UAVs. In this work, a dataset of 6k synthetic depth maps of drones has been generated and used to train a state-of-the-art deep learning-based drone detection model. While many sensing technologies can only provide relative altitude and azimuth of an obstacle, our depth map-based approach enables full 3D localization of the obstacle. This is extremely useful for collision avoidance, as 3D localization of detected drones is key to perform efficient collision-free path planning. The proposed detection technique has been validated in several real depth map sequences, with multiple types of drones flying at up to 2 m/s, achieving an average precision of 98.7 %, an average recall of 74.7 % and a record detection range of 9.5 meters. © 2018 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{DeQuevedo2018,
author={De Quevedo, A.D. and Urzaiz, F.I. and Menoyo, J.G. and López, A.A.},
title={Drone Detection and RCS Measurements with Ubiquitous Radar},
journal={2018 International Conference on Radar, RADAR 2018},
year={2018},
art_number={8557320},
note={cited By 17},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85060138187&doi=10.1109%2fRADAR.2018.8557320&partnerID=40&md5=0d02a7bdc95b917c35b8ed5891af72cf},
abstract={This paper presents experimental results on commercial-drone detection with a ubiquitous frequency modulated continuous wave (FMCW) radar system, working at 8.75 GHz (X-band). The system and its main blocks are briefly introduced. Subsequently, the document presents the chosen scenario for the tests, and shows the results of the offline signal processing, achieving a DJI-Phantom-4 detection at a range up to 2 km. The results are illustrated with range-Doppler matrices and detection figures. Range, speed and azimuth accuracies are discussed, considering the drone GPS data. Finally, the paper introduces a statistical radar-cross-section (RCS) study based on the processed data, in order to classify the drone as a Swerling target, and discusses the drone average RCS. © 2018 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Choi2018,
author={Choi, B. and Oh, D. and Kim, S. and Chong, J.-W. and Li, Y.-C.},
title={Long-range drone detection of 24 G FMCW radar with E-plane sectoral horn array},
journal={Sensors (Switzerland)},
year={2018},
volume={18},
number={12},
art_number={4171},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85057545444&doi=10.3390%2fs18124171&partnerID=40&md5=b83bad140d325edcad0be4170e537507},
abstract={In this work, a 24-GHz frequency-modulated continuous-wave (FMCW) radar system with two sectoral horn antennas and one transmitting lens antenna for long-range drone detection is presented. The present work demonstrates the detection of a quadcopter-type drone using the implemented radar system up to a distance of 1 km. Moreover, a 3D subspace-based algorithm is proposed for the joint range-azimuth-Doppler estimation of long-range drone detection. The effectiveness of the long-range drone detection is verified with the implemented radar system through a variety of experiments in outdoor environments. This is the first such demonstration for long-range drone detection with a 24-GHz FMCW radar. © 2018 by the authors. Licensee MDPI, Basel, Switzerland.},
publisher={MDPI AG},
}

@CONFERENCE{Jarabo-Amores2018313,
author={Jarabo-Amores, M.P. and Mata-Moya, D. and Gomez-Del-Hoyo, P.J. and Barcena-Humanes, J.L. and Rosado-Sanz, J. and Rey-Maestre, N. and Rosa-Zurera, M.},
title={Drone detection feasibility with passive radars},
journal={2018 15th European Radar Conference, EuRAD 2018},
year={2018},
pages={313-316},
art_number={8546549},
note={cited By 12},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85060376387&doi=10.23919%2fEuRAD.2018.8546549&partnerID=40&md5=597aed919e050c4862601668a6afe838},
abstract={Drones are considered an important threat for critical infrastructures, and for people in crowded environments, because they can carry explosives, chemicals, or biological agents, cameras, etc. Passive radars are emerging sensor technologies that use non-cooperative illuminators instead of a dedicated transmitter. This feature makes them attractive candidates due to the absence of transmitted power. In this work, the viability of passive radars for detecting drone-like targets has been studied. Theoretical coverage studies based on bistatic radar cross section simulations and complex propagation models predict the possibility of drone detection with passive radars. Theoretical results have been validated with real experiments using the IDEPAR demonstrator, developed at the University of Alcalá. © 2018 European Microwave Association.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Lee20181131,
author={Lee, D.R. and Gyu La, W. and Kim, H.},
title={Drone Detection and Identification System using Artificial Intelligence},
journal={9th International Conference on Information and Communication Technology Convergence: ICT Convergence Powered by Smart Intelligence, ICTC 2018},
year={2018},
pages={1131-1133},
art_number={8539442},
note={cited By 21},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85059458820&doi=10.1109%2fICTC.2018.8539442&partnerID=40&md5=feec4d6dabc978442a05656332d845c6},
abstract={As drone attracts much interest, the drone industry has opened their market to ordinary people, making drones to be used in daily lives. However, as it got easier for drone to be used by more people, safety and security issues have raised as accidents are much more likely to happen: colliding into people by losing control or invading secured properties. For safety purposes, it is essential for observers and drone to be aware of an approaching drone. In this paper, we introduce a comprehensive drone detection system based on machine learning. This system is designed to be operable on drones with camera. Based on the camera images, the system deduces location on image and vendor model of drone based on machine classification. The system is actually built with OpenCV library. We collected drone imagery and information for learning process. The system's output shows about 89 percent accuracy. © 2018 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Kim2018,
author={Kim, B.H. and Khan, D. and Bohak, C. and Choi, W. and Lee, H.J. and Kim, M.Y.},
title={V-RBNN based small drone detection in augmented datasets for 3D LADAR system},
journal={Sensors (Switzerland)},
year={2018},
volume={18},
number={11},
art_number={3825},
note={cited By 21},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85056406585&doi=10.3390%2fs18113825&partnerID=40&md5=887a7e1b43a17c38e28a51e75b3873d3},
abstract={A common countermeasure to detect threatening drones is the electro-optical infrared (EO/IR) system. However, its performance is drastically reduced in conditions of complex background, saturation and light reflection. 3D laser sensor LiDAR is used to overcome the problems of 2D sensors like EO/IR, but it is not enough to detect small drones at a very long distance because of low laser energy and resolution. To solve this problem, A 3D LADAR sensor is under development. In this work, we study the detection methodology adequate to the LADAR sensor which can detect small drones at up to 2 km. First, a data augmentation method is proposed to generate a virtual target considering the laser beam and scanning characteristics, and to augment it with the actual LADAR sensor data for various kinds of tests before full hardware system developed. Second, a detection algorithm is proposed to detect drones using voxel-based background subtraction and variable radially bounded nearest neighbor (V-RBNN) method. The results show that 0.2 m L2 distance and 60% expected average overlap (EAO) indexes are satisfied for the required specification to detect 0.3 m size of small drones. © 2018 by the authors. Licensee MDPI, Basel, Switzerland.},
publisher={MDPI AG},
}

@CONFERENCE{Kosolyudhthasarn2018,
author={Kosolyudhthasarn, P. and Visoottiviseth, V. and Fall, D. and Kashihara, S.},
title={Drone Detection and Identification by Using Packet Length Signature},
journal={Proceeding of 2018 15th International Joint Conference on Computer Science and Software Engineering, JCSSE 2018},
year={2018},
art_number={8457352},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85057755102&doi=10.1109%2fJCSSE.2018.8457352&partnerID=40&md5=574a19fec2dc07a8163fffb821e92584},
abstract={Unmanned Aerial Vehicle (UAV) as known as Drone has been becoming very popular around the world. However, a consumer UAV can be controlled from a long distance to record a video of occupants without permission, which causes privacy issues. Existing drone detection systems are required specific hardware and specialists to operate and deploy which are expensive for personal use. In this paper, we propose a drone detection and identification system which utilizes inexpensive commercial off-the-shelf (COTS) hardware and does not requires specialist knowledge to deploy. Our technical approach is to passively listen to the wireless signal between drone and its controller to observe for packet transmission characteristics of each drone. We evaluate our prototype system with three types of drones, which are Spark, AR, and Dobby. Our experiment results illustrate the feasibility of using the data frame length to identify the type of flying drone within 20 seconds. © 2018 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Zywek2018,
author={Zywek, M. and Krawczyk, G. and Malanowski, M.},
title={Experimental results of drone detection using noise radar},
journal={Proceedings International Radar Symposium},
year={2018},
volume={2018-June},
art_number={8447988},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85053631756&doi=10.23919%2fIRS.2018.8447988&partnerID=40&md5=3306d3be6891aba9322d9b08eff9a6fc},
abstract={The paper deals with detection of drones using noise radar. The radar under consideration is a low-power, continuous-wave narrow-band noise radar. First, thethe-oretical analysis concerning power budget and velocity resolution is carried out. Next, the experimental setup is described. The results of a small drone detection are presented. It is demonstrated that in the experiment, the drone detection range was in the order of 300 m. © 2018 German Institute of Navigation - DGON.},
publisher={IEEE Computer Society},
}

@CONFERENCE{DeQuevedo2018,
author={De Quevedo, A.D. and Urzaiz, F.I. and Menoyo, J.G. and Lopez, A.A.},
title={Drone detection with x-band ubiquitous radar},
journal={Proceedings International Radar Symposium},
year={2018},
volume={2018-June},
art_number={8447942},
note={cited By 8},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85053624493&doi=10.23919%2fIRS.2018.8447942&partnerID=40&md5=c6321d18df2b5cb6fe83590a82ffa7ed},
abstract={This paper presents the design and experimental results on commercial-drone detection with a ubiquitous frequency modulated continuous wave (FMCW) radar system demonstrator, working at 8.75 GHz (X-band). The demonstrator is introduced and its main blocks are described, with particular attention to the PC-based signal processor. Subsequently, the document presents the chosen scenario for the tests, and shows the results of the offline processing, achieving a DJI-Phantom-4 detection at a range up to 2 km. The results are illustrated with range-Doppler matrices and detection figures. Range, speed and azimuth accuracies are discussed, considering the drone GPS data. Finally, the paper introduces statistical radar-cross-section (RCS) studies based on the processed data, in order to classify the drone as a Swerling target, and discusses the drone average RCS. © 2018 German Institute of Navigation - DGON.},
publisher={IEEE Computer Society},
}

@CONFERENCE{Stasiak2018521,
author={Stasiak, K. and Ciesielski, M. and Kurowska, A. and Przybysz, W.},
title={A study on using different kinds of continuous-wave radars operating in C-band for drone detection},
journal={MIKON 2018 - 22nd International Microwave and Radar Conference},
year={2018},
pages={521-526},
note={cited By 8},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85050780669&doi=10.23919%2fMIKON.2018.8405275&partnerID=40&md5=ea42a9a4838c8a20e59c57296add85ea},
abstract={The paper focuses on results of field trials for drone detection using CW (Continuous-Wave) radars operating in the C-band. The experiments have involved two different implementations of FMCW (Frequency-Modulated Continuous-Wave) radar and an implementation of CW noise radar. The theoretical comparison of the FMCW and noise radar, along with the description of their implementations is included. The obtained results are presented and discussed. For the conclusion, the limitations of each implementation are identified and recom-mendations for its usage in considered application are provided. © 2018 Warsaw University of Technology.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Basak20181,
author={Basak, S. and Scheers, B.},
title={Passive radio system for real-time drone detection and DoA estimation},
journal={2018 International Conference on Military Communications and Information Systems, ICMCIS 2018},
year={2018},
pages={1-6},
note={cited By 9},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85050262355&doi=10.1109%2fICMCIS.2018.8398721&partnerID=40&md5=91d132200c12b2b910ad9b216ac974d6},
abstract={The principal objective behind the development of passive radio system is to detect and localize mini remotely piloted aircraft systems (RPAS) and their operators in three dimensions (3D). This paper describes the system architecture, detection procedure and intermediate test results. Goodness-of-Fit (GoF) based spectrum sensing is used to detect the frequency of the transmitted signal of mini-RPAS and its controller. The direction of arrival (DoA) is estimated with the MUSIC algorithm. The implementation of GoF-based wideband spectrum sensing and one dimensional DoA estimation including spatial smoothing and automatic source number detection are detailed in this paper. Several test results are presented to validate the real time operation of the passive radio system. © 2018 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Jian20181146,
author={Jian, M. and Lu, Z. and Chen, V.C.},
title={Drone detection and tracking based on phase-interferometric Doppler radar},
journal={2018 IEEE Radar Conference, RadarConf 2018},
year={2018},
pages={1146-1149},
note={cited By 33},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85049928482&doi=10.1109%2fRADAR.2018.8378723&partnerID=40&md5=72e95fda4ec128ff0efa9abff67b10ea},
abstract={In this paper, drone detection and tracking based on phase-interferometry are investigated. Data collected by a simple dual-channel Doppler radar is used for implementing the joint range-Doppler-azimuth processing. Experimental results show that micro drones can be detected and tracked by applying the joint range-Doppler-azimuth processing. Features extracted from the range-Doppler-azimuth domain can be used to identify drones. © 2018 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Fang201833542,
author={Fang, G. and Yi, J. and Wan, X. and Liu, Y. and Ke, H.},
title={Experimental Research of Multistatic Passive Radar with a Single Antenna for Drone Detection},
journal={IEEE Access},
year={2018},
volume={6},
pages={33542-33551},
note={cited By 29},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85048170961&doi=10.1109%2fACCESS.2018.2844556&partnerID=40&md5=878b8d68a98c82f29f207d24d04066e6},
abstract={Digital television signals are attractive illuminations of opportunity for the passive radars in the field of low altitude and slow speed target detection. The digital television standard permits reconstruction of a reference signal using the received signal in surveillance channel, which enables a single-antenna digital television based passive radar (SDPR) processing. This paper investigates the practical feasibility of a multistatic SDPR (MSDPR) for the drone detection. First, the detection range of the SDPR is analyzed in terms of signal processing procedures involving multipath energy, extracted reference signal purity, and receiving antenna. Second, according to the characteristics of the SDPR, the reference signal extraction is analyzed. In addition, considering that the SDPR cannot locate and track the detected target, a novel MSDPR processing method is proposed. The core idea of this method is to use the optimal reference signal extracted from the receiving station with the least interference as the shared reference signal in MSDPR, which can greatly improve the system detection capability. Finally, the small drone detection experiments using the MSDPR are presented. The theoretical considerations are demonstrated using the experimental data. © 2013 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Kim2018188,
author={Kim, B.-K. and Park, J. and Park, S.-J. and Kim, T.-W. and Jung, D.-H. and Kim, D.-H. and Kim, T. and Park, S.-O.},
title={Drone Detection with Chirp-Pulse Radar Based on Target Fluctuation Models},
journal={ETRI Journal},
year={2018},
volume={40},
number={2},
pages={188-196},
note={cited By 8},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85045404841&doi=10.4218%2fetrij.2017-0090&partnerID=40&md5=0823d2152394c92c06ab01d1c8041473},
abstract={This paper presents a pulse radar system to detect drones based on a target fluctuation model, specifically the Swerling target model. Because drones are small atypical objects and are mainly composed of non-conducting materials, their radar cross-section value is low and fluctuating. Therefore, determining the target fluctuation model and applying a proper integration method are important. The proposed system is herein experimentally verified and the results are discussed. A prototype design of the pulse radar system is based on radar equations. It adopts three different pulse modes and a coherent pulse integration to ensure a high signal-to-noise ratio. Outdoor measurements are performed with a prototype radar system to detect Doppler frequencies from both the drone frame and blades. The results indicate that the drone frame and blades are detected within an instrumental maximum range. Additionally, the results show that the drone's frame and blades are close to the Swerling 3 and 4 target models, respectively. By the analysis of the Swerling target models, proper integration methods for detecting drones are verified and can thus contribute to increasing in detectability. © 2018 ETRI},
publisher={John Wiley and Sons Inc.},
}

@CONFERENCE{Liu2018,
author={Liu, H. and Qu, F. and Liu, Y. and Zhao, W. and Chen, Y.},
title={A drone detection with aircraft classification based on a camera array},
journal={IOP Conference Series: Materials Science and Engineering},
year={2018},
volume={322},
number={5},
art_number={052005},
note={cited By 16},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85045847009&doi=10.1088%2f1757-899X%2f322%2f5%2f052005&partnerID=40&md5=417f08c1de3726d3bd69a544aa54edf2},
abstract={In recent years, because of the rapid popularity of drones, many people have begun to operate drones, bringing a range of security issues to sensitive areas such as airports and military locus. It is one of the important ways to solve these problems by realizing fine-grained classification and providing the fast and accurate detection of different models of drone. The main challenges of fine-grained classification are that: (1) there are various types of drones, and the models are more complex and diverse. (2) the recognition test is fast and accurate, in addition, the existing methods are not efficient. In this paper, we propose a fine-grained drone detection system based on the high resolution camera array. The system can quickly and accurately recognize the detection of fine grained drone based on hd camera. © Published under licence by IOP Publishing Ltd.},
publisher={Institute of Physics Publishing},
}

@CONFERENCE{Häfner2018,
author={Häfner, S. and Röding, M. and Sommerkorn, G. and Müller, R. and Thomä, R.S. and Del Galdo, G. and Goerlich, J.},
title={Contribution to drone detection by exploiting parameter estimation for a prototype mm-wave radar system},
journal={WSA 2018 - 22nd International ITG Workshop on Smart Antennas},
year={2018},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85081589669&partnerID=40&md5=fa255759863f850eb84c39d254144dca},
abstract={An estimator to infer parameters from radar measurements is presented, applicable for further detection and localisation of unmanned aircraft systems. The problem of parameter estimation is presented as an inverse problem, necessitating a model of the measurement data. Based on the data model, a maximum-likelihood based objective function is derived. The objective function is minimised by a framework similar to the RIMAX framework, including joint parameter and model order estimation. A SIMO radar system is presented and employed to test and demonstrate the estimators capability in simulations as well as test measurements with flying UASs. © 2018 VDE VERLAG GMBH ∙ Berlin ∙ Offenbach},
publisher={VDE Verlag GmbH},
}

@CONFERENCE{James2018,
author={James, J.V. and Cazzolato, B.S. and Grainger, S. and O'Carroll, D.C. and Wiederman, S.D.},
title={An insect-inspired detection algorithm for aerial drone detection},
journal={Australasian Conference on Robotics and Automation, ACRA},
year={2018},
volume={2018-December},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85071583336&partnerID=40&md5=a0a18278cb0dbdb2ddbef1af96368e84},
abstract={Flying insects display remarkable visual abilities which can serve as inspiration for target detection algorithms. For example, biologically inspired models of neurons in the dragonfly brain have previously been evaluated for their ability to detect moving targets from a ground-based robotic platform. Here we evaluate the performance of a model tuned to a specific biological task (detection of prey and conspecifics), applied to a very different endeavour - the detection of airborne drones as viewed by another drone. We identify the circumstances for success and failure with the prey-detection model, whilst varying the computational complexity of the task with a reduction in spatial sampling. This evaluation provides substantial insight into how the bio-inspired algorithm may be generalised for other automatic target detection tasks, such as in the detection of unmanned aerial vehicles. © 2018 Australasian Robotics and Automation Association. All rights reserved.},
publisher={Australasian Robotics and Automation Association},
}

@ARTICLE{Ryu20181146,
author={Ryu, J. and Kim, S.},
title={Data driven proposal and deep learning-based small infrared drone detection [데이터 기반 영역 제안 및 심층 학습 분류 네트워크를 이용한 소형 적외선 드론 검출]},
journal={Journal of Institute of Control, Robotics and Systems},
year={2018},
volume={24},
number={12},
pages={1146-1151},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85058642831&doi=10.5302%2fJ.ICROS.2018&partnerID=40&md5=c68276af7636c1292162e4a66cc03619},
abstract={In this paper, we propose a data-driven and deep-learning based classification scheme for small infrared target detection. Previous studies have shown feasible performance using conventional computer vision techniques, such as spatial and temporal filters. However, those handcrafted approaches are not optimized due to the nature of the application fields. Recently, deep-learning has shown excellent performance for many computer vision problems. The proposed data-driven proposal and convolutional neural network (DDP-CNN) approach can generate possible target locations through the DDP, and final targets are recognized through the CNN for classification. According to the experimental results using drone databases, the DDP-CNN shows an 0.85 average precision (AP) of target detection. © ICROS 2018.},
publisher={Institute of Control, Robotics and Systems},
}

@CONFERENCE{Kim2018,
author={Kim, B.H. and Khan, D. and Bohak, C. and Kim, J.K. and Choi, W. and Lee, H.J. and Kim, M.Y.},
title={Ladar data generation fused with virtual targets and visualization for small drone detection system},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2018},
volume={10797},
art_number={107970I},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85056655170&doi=10.1117%2f12.2500525&partnerID=40&md5=22dd81a8a3b89ed919b212a546fc4926},
abstract={For detection of a small target using electro-optical systems, multi-band 2D image sensors are used such as visible, NIR, MWIR, and LWIR. However, 2D imaging systems are not capable to detect a very small target and they are also not capable of calculating target 3D position coordinates to develop the strategic counter method. 3D sensors (e.g. Lidar, RGBD and stereo camera) are utilized to control unmanned vehicles for detecting threats and response for specific situations. Conventional Lidar systems are unable to detect small drone threat at distances higher than their maximum detecting range of 100 ?1/4 120 meters. To overcome this limitation, laser radar (LADAR) systems are being developed, which allow the detection at distances up to 2 kilometers. In the development of LADAR, it is difficult to acquire datasets that contain cases of long distant targets. In this study, a fusion data generation with virtual targets technique based on minimum real LADAR initial map dataset is proposed, and precise small target detection method using voxel-based clustering and classification are studied. We present the process of data fusion generation and the experimental results for a small target detection. The presented approach also includes effective visualization of high-resolution 3D data and the results of small target detection in real time. This study is expected to contribute to the optimization of a drone threat detection system for various environments and characteristics. © 2018 SPIE.},
publisher={SPIE},
}

@ARTICLE{Wu201822,
author={Wu, M. and Xie, W. and Shi, X. and Shao, P. and Shi, Z.},
title={Real-time drone detection using deep learning approach},
journal={Lecture Notes of the Institute for Computer Sciences, Social-Informatics and Telecommunications Engineering, LNICST},
year={2018},
volume={251},
pages={22-32},
note={cited By 8},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85055545933&doi=10.1007%2f978-3-030-00557-3_3&partnerID=40&md5=2058c0baff0488bd8fea647ad20060ec},
abstract={The arbitrary use of drones poses great threat to public safety and personal privacy. It is necessary to detect the intruding drones in sensitive areas in real time. In this paper, we design a real-time drone detector using deep learning approach. Specifically, we improve a well-performed deep learning model, i.e., You Only Look Once, by modifying its structure and tuning its parameters to better accommodate drone detection. Considering that a robust detector needs to be trained using a large amount of training images, we also propose a semi-automatically dataset labelling method based on Kernelized Correlation Filters tracker to speed up the pre-processing of the training images. At last, the performance of our detector is verified via extensive experiments. © ICST Institute for Computer Sciences, Social Informatics and Telecommunications Engineering 2018.},
publisher={Springer Verlag},
}

@CONFERENCE{Wang2018,
author={Wang, J. and Yue, X. and Liu, Y. and Song, H. and Yuan, J. and Yang, T. and Seker, R.},
title={Integrating ground surveillance with aerial surveillance for enhanced amateur drone detection},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2018},
volume={10652},
art_number={106520E},
note={cited By 6},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85049210221&doi=10.1117%2f12.2304531&partnerID=40&md5=bc431397c3bc7ed97e8a796c1b300da0},
abstract={Unmanned Aerial Systems (UASs) are becoming increasingly popular for amateur use, but their arbitrary deployment poses severe public safety threats to critical infrastructures, such as airports. Typically an Amateur Unmanned Aerial System (AUAS) communicates with a ground control station (GCS) through a telemetry radio, which keeps transmitting data in poor connection conditions. The accuracy of AUASs detection is of great significance. In this paper, we propose a novel surveillance framework which leverages Surveillance Unmanned Aerial Systems (SUASs) to detect AUASs. The approximate position of an AUAS is first estimated by Ground Surveillance Nodes (GSNs) with radio receivers, and SUASs are then activated to determine its precise position. Different from previous research, this framework not only leverages both ground and aerial surveillance capabilities, but also integrates both radio and image processing techniques, thus achieving enhanced AUAS detection capability. This platform has the potential to be integrated with other advanced technologies, providing the recognition of radio signals and imagery for a holistic solution of effective AUAS detection. © 2018 SPIE.},
publisher={SPIE},
}

@ARTICLE{Solomitckii201843,
author={Solomitckii, D. and Gapeyenko, M. and Semkin, V. and Andreev, S. and Koucheryavy, Y.},
title={Technologies for Efficient Amateur Drone Detection in 5G Millimeter-Wave Cellular Infrastructure},
journal={IEEE Communications Magazine},
year={2018},
volume={56},
number={1},
pages={43-50},
art_number={8255736},
note={cited By 65},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85040720734&doi=10.1109%2fMCOM.2017.1700450&partnerID=40&md5=78d5cd7bc30d2f75041145e26ed4b126},
abstract={Unmanned aerial vehicles, also called drones, are recently gaining increased research attention across various fields due to their flexibility and application potential. The steady increase in the number of amateur drones demands more stringent regulations on their allowed route, mass, and load. However, these regulations may be violated accidentally or deliberately. In these cases, spying with drones, transfer of dangerous payloads, or losing reliable drone control can represent a new hazard for people, governments, and business sector. The technologies to detect, track, and disarm possible aerial threats are therefore in prompt demand. To this end, ubiquitous cellular networks, and especially 5G infrastructures based on the use of millimeter-wave radio modules, may be efficiently leveraged to offer the much needed drone detection capabilities. In this work, we propose to exploit 5G millimeter-wave deployments to detect violating amateur drones. We argue that the prospective 5G infrastructure may provide all the necessary technology elements to support efficient detection of small-sized drones. We therefore outline a novel technology and system design perspective, including such considerations as the density of base stations, their directional antennas, and the available bandwidth, among others, as well as characterize their impact with our ray-based modeling methods. © 1979-2012 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Park20171,
author={Park, S. and Park, S.-O.},
title={Configuration of an X-band FMCW radar targeted for drone detection},
journal={2017 International Symposium on Antennas and Propagation, ISAP 2017},
year={2017},
volume={2017-January},
pages={1-2},
note={cited By 13},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85046354170&doi=10.1109%2fISANP.2017.8228912&partnerID=40&md5=945d445da387de5733c6dbef59232531},
abstract={This paper discusses the detection of drone with Frequency-Modulated Continuous-Wave (FMCW) Radar system. The system employs 11GHz to 11.15GHz frequency bandwidth to generate sawtooth linear wave through bistatic antennas with the gain of 33.7dBi, and the output transmitter power is 35dBm. Metal baffles were placed between and each side of the antennas to minimize the direct path interference. The system also includes digital down converter to obtain IQ signal with minimum mismatch. In the actual performance measurement, the drone signal was detected up to more than 500m distance in real-Time with the error of less than 0.1%. The data has been saved as bin file and then later processed with MATLAB. © 2017 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Aker2017,
author={Aker, C. and Kalkan, S.},
title={Using deep networks for drone detection},
journal={2017 14th IEEE International Conference on Advanced Video and Signal Based Surveillance, AVSS 2017},
year={2017},
art_number={8078539},
note={cited By 81},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85039915587&doi=10.1109%2fAVSS.2017.8078539&partnerID=40&md5=c81a1879a8b64d8219c65f581a1fa711},
abstract={Drone detection is the problem of finding the smallest rectangle that encloses the drone(s) in a video sequence. In this study, we propose a solution using an end-to-end object detection model based on convolutional neural networks. To solve the scarce data problem for training the network, we propose an algorithm for creating an extensive artificial dataset by combining background-subtracted real images. With this approach, we can achieve precision and recall values both of which are high at the same time. © 2017 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Kwag2017,
author={Kwag, Y.-K. and Woo, I.-S. and Kwak, H.-Y. and Jung, Y.-H.},
title={Multi-mode SDR radar platform for small air-vehicle Drone detection},
journal={2016 CIE International Conference on Radar, RADAR 2016},
year={2017},
art_number={8059254},
note={cited By 10},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85034623748&doi=10.1109%2fRADAR.2016.8059254&partnerID=40&md5=27461eaf76ef6e3a1833f9cf460ddfc8},
abstract={This paper presents the new development results of the multi-band, multi-mode software-defined radar (SDR) platform. The SDR platform consists of a hardware-based platform and software-based platform. The multi-band RF modules are implemented using the selectable S, X, K-bands, and multi-mode are implemented using selectable waveforms of CW, Pulse, FMCW, and LFM Chirp as well as radar processing algorithm libraries and open API software module. For the performance evaluation of this new SDR platform, an air-vehicle detection program is successfully tested using a small Drone flying on the runway for air traffic safety applications. © 2016 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Nuss2017,
author={Nuss, B. and Sit, L. and Fennel, M. and Mayer, J. and Mahler, T. and Zwick, T.},
title={MIMO OFDM radar system for drone detection},
journal={Proceedings International Radar Symposium},
year={2017},
art_number={8008141},
note={cited By 18},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85028600049&doi=10.23919%2fIRS.2017.8008141&partnerID=40&md5=347cd0f4835760a4b299c120bd2977fd},
abstract={This paper presents a system setup based on MIMO OFDM radar that can be used for drone detection and detection of unpiloted aerial vehicles (UAVs) in general. In recent years UAVs have become more and more popular not only for commercial use but also as a private gadget. However, these drones can also be misused as a weapon by criminals, spies and terrorists. Therefore many research is done to be able to detect drones and prevent further harm. One possible approach is radar that has already been used successfully in automotive and military applications and offers many advantages like weather and daylight independent operation. It is also possible to detect drones that are emitting no electrical or optical signals. However, there are still many challenges that have to be solved before the implementation of reliably operating systems. This paper presents a system approach based on MIMO OFDM radar that can be used to survey large areas simultaneously and detect flying drones. Additionally, verification measurements with a drone in a real world scenario are presented demonstrating the successful operation of the system. © 2017 DGON.},
publisher={IEEE Computer Society},
}

@CONFERENCE{Ochodnicky2017613,
author={Ochodnicky, J. and Matousek, Z. and Babjak, M. and Kurty, J.},
title={Drone detection by Ku-band battlefield radar},
journal={ICMT 2017 - 6th International Conference on Military Technologies},
year={2017},
pages={613-616},
art_number={7988830},
note={cited By 25},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85029382382&doi=10.1109%2fMILTECHS.2017.7988830&partnerID=40&md5=6c271a03cd31a0341b2da8b8569ccbe7},
abstract={The intensive research and development efforts in the area of unmanned aerial vehicles (UAV) detection for security applications is observed in the last decade. The published research results are focused on applications in particular domains (e.g. acoustic, ultrasonic, optical, infrared, radiofrequency..) whereas the probability characteristics for each assumed application evaluation are needed. This paper includes the theoretical analysis of battlefield pulse radar detection probability and range for small UAV. The interdependence between Signal-to-Noise Ratio (SNR) and small UAV Radar Cross Section (RCS) is derived. The results of dynamic flight test series conducted to evaluate the detection performance of three drone size categories by pulse Ku-band short range battlefield radar are presented. Some dependences of the SNR and probability of detection on the drone sizes are determined. © 2017 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Gaigals20171,
author={Gaigals, G. and Vavilina, E.},
title={Simulation of compressed sensing based passive radar for drone detection},
journal={Proceedings of the 5th IEEE Workshop on Advances in Information, Electronic and Electrical Engineering, AIEEE 2017},
year={2017},
volume={2018-January},
pages={1-5},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85050589967&doi=10.1109%2fAIEEE.2017.8270552&partnerID=40&md5=f15c8021653d6fd19855532e2ad0e63b},
abstract={Nowadays drones and RC planes come more and more popular since they are widely available. People enjoy filming from drones even in drone strictly forbidden places ignoring prohibition signs. That often makes problems for specialists working in an environment with demanded radio emission free zone. To avoid drones from flying in prohibited areas a drone radar is needed. This paper represents feasibility study on passive radar for drone detection using novel signal processing technique and Monte Carlo method. Radar simulation was made to study impact of different factors on the drone detection quality simulating different antennas setups: Regular and irregular placement of the antennas, similar and different directivity antennas, stationary and randomly pointed antennas. Results show the impact of different drone quantity, antennas directivity, antennas placement, antennas rotation on the drone detection quality. © 2017 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Liu2017402,
author={Liu, H. and Wei, Z. and Chen, Y. and Pan, J. and Lin, L. and Ren, Y.},
title={Drone Detection Based on an Audio-Assisted Camera Array},
journal={Proceedings - 2017 IEEE 3rd International Conference on Multimedia Big Data, BigMM 2017},
year={2017},
pages={402-406},
art_number={7966780},
note={cited By 48},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85027700679&doi=10.1109%2fBigMM.2017.57&partnerID=40&md5=7f763c398d2bbd8d50cc32e0aec94c8c},
abstract={In recent years, small, inexpensive UAV - also known as drone - has made great progress, which brings privacy and security issues. Drone detection is one of the important methods to solve these problems. The main challenges of drone detection are: (1) A drone is very confusing with other flying objects such as a bird, (2) the low-flying UAV occlusion happens very frequent, and (3) the existing surveillance coverage is limited. Camera array can be used for large-scale airspace observation. In this paper, we propose a modular camera array system with audio assistance, which consists of dozens of high-definition cameras and multiple microphones, to monitor drones. It can be mounted on a carrier after reducing the size. The system captures the image and audio information of the surroundings in various directions. The system can integrate the information of multiple sensors, and identify the characteristics of the drone to achieve higher efficiency of drone monitoring. © 2017 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Liu20171493,
author={Liu, Y. and Wan, X. and Tang, H. and Yi, J. and Cheng, Y. and Zhang, X.},
title={Digital television based passive bistatic radar system for drone detection},
journal={2017 IEEE Radar Conference, RadarConf 2017},
year={2017},
pages={1493-1497},
art_number={7944443},
note={cited By 55},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85021419679&doi=10.1109%2fRADAR.2017.7944443&partnerID=40&md5=7cbcedaff2505e77bc5d4dad04a83e6a},
abstract={Recently, the widespread availability of consumer grade drones is responsible for the new concerns of air traffic control. This paper investigates the feasibility of drone detection by passive bistatic radar (PBR) system. Wuhan University has successfully developed a digitally multichannel PBR system, which is dedicated for the drone detection. Two typical trials with a cooperative drone have been designed to examine the system's capability of small drone detection. The agreement between experimental results and ground truth indicate the effectiveness of sensing and processing method, which verifies the practicability and prospects of drone detection by this digitally multichannel PBR system. © 2017 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Hindle20176,
author={Hindle, P.},
title={Drone detection and location systems},
journal={Microwave Journal},
year={2017},
volume={2017-June},
pages={6-8},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85025176897&partnerID=40&md5=eedeca1b80a81875ad941a2de556eecb},
publisher={Horizon House},
}

@ARTICLE{Shin2017340,
author={Shin, D.-H. and Jung, D.-H. and Kim, D.-C. and Ham, J.-W. and Park, S.-O.},
title={A Distributed FMCW Radar System Based on Fiber-Optic Links for Small Drone Detection},
journal={IEEE Transactions on Instrumentation and Measurement},
year={2017},
volume={66},
number={2},
pages={340-347},
art_number={7762208},
note={cited By 60},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84999089902&doi=10.1109%2fTIM.2016.2626038&partnerID=40&md5=4c85f6e694f4041a18d72f4d9b3ef726},
abstract={This paper discusses a distributed frequency modulation continuous wave radar system. This K-band radar system has high sensitivity, linearity, and flatness to detect low-radar cross section targets and measure their range and velocity. To reduce the leakage between a transmitter and a receiver, the system uses not RF cables but fiber-optic links that have low distortion characteristics and low propagation loss. The transmitter and the receiver are each mounted on a designed fixture to reduce the ground reflections. In addition, they are located on different platforms to reduce the leakage signal flowing directly from the transmitter to the receiver. Measurements in terms of the range and the velocity of a small drone have been carried out to evaluate the proposed distributed radar system. The results show that we can clearly detect the small drone within a 500 m range, which demonstrates the high sensitivity of the system and high isolation between the transmitter and the receiver. © 2016 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Chadwick2017,
author={Chadwick, A.D.},
title={Micro-drone detection using software-defined 3G passive radar},
journal={IET Conference Publications},
year={2017},
volume={2017},
number={CP728},
note={cited By 11},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85048671668&doi=10.1049%2fcp.2017.0419&partnerID=40&md5=d1e86ce500eba382a7b0a6fbccc243b0},
abstract={The detection and discrimination of micro-drones is a challenging sensing problem. A passive radar approach offers many of the strengths of active radar sensing, including the use of micro-Doppler for target classification, without the additional size, weight, cost, power, licencing requirements and potential coverage restrictions of a dedicated transmitter. This paper demonstrates the feasibility of micro-drone detection, including the characteristic micro-Doppler features that provide a basis for differentiation from non-drone objects, using a software-defined radio receiver and UMTS 3G signals as a non-cooperative source of illumination at ground level. © 2017 Institution of Engineering and Technology. All rights reserved.},
publisher={Institution of Engineering and Technology},
}

@CONFERENCE{Bernardini201760,
author={Bernardini, A. and Mangiatordi, F. and Pallotti, E. and Capodiferro, L.},
title={Drone detection by acoustic signature identification},
journal={IS and T International Symposium on Electronic Imaging Science and Technology},
year={2017},
pages={60-64},
note={cited By 55},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85041497695&doi=10.2352%2fISSN.2470-1173.2017.10.IMAWM-168&partnerID=40&md5=5bb4647cc5f6ac65314ca7d8d70344b5},
abstract={In the last years, the ductility and easiness of usage of unmanned aerial vehicles (UAV) and their affordable cost have increased the drones use by industry and private users. However, drones carry the potential of many illegal activities from smuggling illicit material, unauthorized reconnaissance and surveillance of targets and individuals, to electronic and kinetic attacks in the worse threatening scenarios. As a consequence, it has become important to develop effective and affordable countermeasures to report of a drone flying over critical areas. In this context, our research chooses different short term parametrization in time and frequency domain of environmental audio data to develop a machine learning based UAV warning system which employs the support vector machines to understand and recognize the drone audio fingerprint. Preliminary experimental results have shown the effectiveness of the proposed approach. © 2017, Society for Imaging Science and Technology.},
publisher={Society for Imaging Science and Technology},
}

@ARTICLE{Neduchal2017162,
author={Neduchal, P. and Berka, F. and Železný, M.},
title={Stationary device for drone detection in urban areas},
journal={Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
year={2017},
volume={10459 LNAI},
pages={162-169},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85029514304&doi=10.1007%2f978-3-319-66471-2_18&partnerID=40&md5=f5a279d522721277b458164165bdc5ba},
abstract={Drones became popular and useful in the last years. There are a lot of companies engaged in the unmanned aviation as well as ordinary people who want fly for fun. The problem arises when a drone is used against the law. Thus, the question of people protection against flying drones has to be addressed. This paper is focused on the creation of the stationary drone detection device suitable for using in urban areas. The main contribution of the paper is a detection approach composed of three parts. The motion detection, object description and classification. Moreover, the Robot Operating System is used in the proposed system in order to create an easily modifiable system. The performance of the proposed approach is tested in a couple of experiments. The system is able to distinguish a drone from e.g. a car or a walking person and it is able to work in real time. © 2017, Springer International Publishing AG.},
publisher={Springer Verlag},
}

@ARTICLE{Sturdivant20177123,
author={Sturdivant, R.L. and Chong, E.K.P.},
title={Systems Engineering Baseline Concept of a Multispectral Drone Detection Solution for Airports},
journal={IEEE Access},
year={2017},
volume={5},
pages={7123-7138},
art_number={7911176},
note={cited By 22},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85028743652&doi=10.1109%2fACCESS.2017.2697979&partnerID=40&md5=9c331454ca3efeb03d31c9d568856e99},
abstract={The baseline concept for a multispectral drone detection (MSDD) system for use in airports is generated. The baseline development process is based on a modified system of systems architecting with ilities (SAI) method. The solution uses multiple independent sensors, which when the sensor outputs are combined, provide functionality that the individual systems were never intended to provide. Also, several sensors are pre-existing and have their own funding, operations, and management. The problem of drone detection is described and examples are given, which justify the need for the system. Then the specific need for airport protection is described. The result is a feasible baseline design that is capable of meeting the need. © 2013 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Müller2017,
author={Müller, T.},
title={Robust drone detection for day/night counter-UAV with static VIS and SWIR cameras},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2017},
volume={10190},
art_number={1019018},
note={cited By 41},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85022188249&doi=10.1117%2f12.2262575&partnerID=40&md5=1fb6194bbd271860c7e770355d6554ae},
abstract={Recent progress in the development of unmanned aerial vehicles (UAVs) has led to more and more situations in which drones like quadrocopters or octocopters pose a potential serious thread or could be used as a powerful tool for illegal activities. Therefore, counter-UAV systems are required in a lot of applications to detect approaching drones as early as possible. In this paper, an efficient and robust algorithm is presented for UAV detection using static VIS and SWIR cameras. Whereas VIS cameras with a high resolution enable to detect UAVs in the daytime in further distances, surveillance at night can be performed with a SWIR camera. First, a background estimation and structural adaptive change detection process detects movements and other changes in the observed scene. Afterwards, the local density of changes is computed used for background density learning and to build up the foreground model which are compared in order to finally get the UAV alarm result. The density model is used to filter out noise effects, on the one hand. On the other hand, moving scene parts like moving leaves in the wind or driving cars on a street can easily be learned in order to mask such areas out and suppress false alarms there. This scene learning is done automatically simply by processing without UAVs in order to capture the normal situation. The given results document the performance of the presented approach in VIS and SWIR in different situations. © COPYRIGHT SPIE.},
publisher={SPIE},
}

@CONFERENCE{Yoon2017,
author={Yoon, J.H. and Xu, H. and Garcia Carrillo, L.R.},
title={Advanced Doppler radar physiological sensing technique for drone detection},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2017},
volume={10188},
art_number={101880S},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85022093990&doi=10.1117%2f12.2262758&partnerID=40&md5=929bef2c5dd5ec7a4da6b6bfd72f396f},
abstract={A 24 GHz medium-range human detecting sensor, using the Doppler Radar Physiological Sensing (DRPS) technique, which can also detect unmanned aerial vehicles (UAVs or drones), is currently under development for potential rescue and anti-drone applications. DRPS systems are specifically designed to remotely monitor small movements of non-metallic human tissues such as cardiopulmonary activity and respiration. Once optimized, the unique capabilities of DRPS could be used to detect UAVs. Initial measurements have shown that DRPS technology is able to detect moving and stationary humans, as well as largely non-metallic multi-rotor drone helicopters. Further data processing will incorporate pattern recognition to detect multiple signatures (motor vibration and hovering patterns) of UAVs. © 2017 SPIE.},
publisher={SPIE},
}

@ARTICLE{Korobiichuk201720,
author={Korobiichuk, I. and Nowicki, M. and Danik, Y.G. and Dupelich, S. and Samchyshyn, O.},
title={The selection methods for multisensor system elements of drone detection},
journal={Advances in Intelligent Systems and Computing},
year={2017},
volume={543},
pages={20-26},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85009476909&doi=10.1007%2f978-3-319-48923-0_3&partnerID=40&md5=70289612ae8128ff077dc1f0a47264b8},
abstract={The application of the existing means for drones detection is rather troublesome due to the miniaturization of board equipment, usage of composite materials and special paint. The possible way to resolve this problem is to combine the technical solution means which function on the basis of physical phenomena and which are crucial for drones detection. The partial indexes and criteria of the effective functioning of multisensory systems of the surrounding area control are determined. The selection method of means for multisensory drone detection system is developed. © Springer International Publishing AG 2017.},
publisher={Springer Science and Business Media Deutschland GmbH},
}

@CONFERENCE{Lee2016291,
author={Lee, S.J. and Jung, J.H. and Park, B.},
title={Possibility verification of drone detection radar based on pseudo random binary sequence},
journal={ISOCC 2016 - International SoC Design Conference: Smart SoC for Intelligent Things},
year={2016},
pages={291-292},
art_number={7799792},
note={cited By 8},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85010420431&doi=10.1109%2fISOCC.2016.7799792&partnerID=40&md5=bf4186dcd8e41f5e5e6dd12b5ebf3cee},
abstract={This paper presents the possibility verification of a drone detection radar based on pseudo random binary sequence (PRBS). It contains the design of a probing signal and resultant specifications of the radar, measurement setup using commercial signal generator/analyzer and antennas, and laboratory/outdoor measurements. Measurements in the 2 CHy. band with 6 dBm transmit condition show the drone detection at the range over 100 in. © 2016 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Drozdowicz2016,
author={Drozdowicz, J. and Wielgo, M. and Samczynski, P. and Kulpa, K. and Krzonkalla, J. and Mordzonek, M. and Bryl, M. and Jakielaszek, Z.},
title={35 GHz FMCW drone detection system},
journal={Proceedings International Radar Symposium},
year={2016},
volume={2016-June},
art_number={7497351},
note={cited By 56},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84982806276&doi=10.1109%2fIRS.2016.7497351&partnerID=40&md5=ba17ab9655dbc12864dd90823682fcab},
abstract={This paper presents an experimental system dedicated for the detection and tracking of small aerial targets such as Unmanned Aerial Vehicles (UAVs) in particular small drones (multirotors). The system was proposed in response to increasing drone popularity and the related threats. The hardware and software parts of the system are covered, including the analogue front-end, FPGA based pre-processing and PC based processing, detection and tracking. Real life trials are described with promising results provided. Further research on the subject is proposed. © 2016 IEEE.},
publisher={IEEE Computer Society},
}

@CONFERENCE{Popovic2016,
author={Popovic, V. and Ott, B. and Wellig, P. and Leblebici, Y.},
title={Near-infrared high-resolution real-time omnidirectional imaging platform for drone detection},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2016},
volume={9997},
art_number={999706},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85011060280&doi=10.1117%2f12.2241322&partnerID=40&md5=177e3440945e68f50c86a83c3874ddfa},
abstract={Recent technological advancements in hardware systems have made higher quality cameras. State of the art panoramic systems use them to produce videos with a resolution of 9000 x 2400 pixels at a rate of 30 frames per second (fps).1 Many modern applications use object tracking to determine the speed and the path taken by each object moving through a scene. The detection requires detailed pixel analysis between two frames. In fields like surveillance systems or crowd analysis, this must be achieved in real time.2 In this paper, we focus on the system-level design of multi-camera sensor acquiring near-infrared (NIR) spectrum and its ability to detect mini-UAVs in a representative rural Swiss environment. The presented results show the UAV detection from the trial that we conducted during a field trial in August 2015. © 2016 SPIE.},
publisher={SPIE},
}


==> DroneTracking.tex <==

@CONFERENCE{Patel2022,
author={Patel, M. and Ferguson, P.},
title={Drone-Based Cable-Suspended Payload Tracking and Estimation Using Simulated LiDAR Measurements and an Extended Kalman Filter},
journal={AIAA Science and Technology Forum and Exposition, AIAA SciTech Forum 2022},
year={2022},
art_number={AIAA 2022-2290},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85123885344&doi=10.2514%2f6.2022-2290&partnerID=40&md5=030734b00130c70dbd6e1b7fe4042954},
abstract={The ability of drones to navigate through remote terrain and avoid ground-based vehicular traffic has led to an increase in remote sensing studies and drone-based transportation services. Such applications require a payload to be suspended from the drone via a cable which can introduce instability in the drone’s flight resulting from the sway of the suspended payload. Therefore, to maintain a stable flight it is key to measure the position of the payload relative to the drone. This study uses a Vicon motion capture system to measure the position of the drone and simulated Light Detection and Ranging (LiDAR) measurements for the position of the payload. LiDAR measurements are simulated using a LiDAR noise model developed from experimental results using the Velodyne VLP-16TM sensor. A nonlinear dynamic model of a drone-based single cable-suspended payload is developed and a discrete Extended Kalman Filter is used to obtain an accurate estimate of the position of the drone and the position of the payload relative to the drone. © 2022, American Institute of Aeronautics and Astronautics Inc.. All rights reserved.},
publisher={American Institute of Aeronautics and Astronautics Inc, AIAA},
}

@ARTICLE{Ateya20224677,
author={Ateya, A.A. and Algarni, A.D. and Koucheryavy, A. and Soliman, N.F.},
title={Drone-based AI/IoT Framework for Monitoring, Tracking and Fighting Pandemics},
journal={Computers, Materials and Continua},
year={2022},
volume={71},
number={2},
pages={4677-4699},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85122723986&doi=10.32604%2fcmc.2022.021850&partnerID=40&md5=4ab4c240b4f3479e766d4584e2105ce5},
abstract={Since World Health Organization (WHO) has declared the Coronavirus disease (COVID-19) a global pandemic, the world has changed. All life’s fields and daily habits have moved to adapt to this new situation. According to WHO, the probability of such virus pandemics in the future is high, and recommends preparing for worse situations. To this end, this work provides a framework for monitoring, tracking, and fighting COVID-19 and future pandemics. The proposed framework deploys unmanned aerial vehicles (UAVs), e.g.; quadcopter and drone, integrated with artificial intelligence (AI) and Internet of Things (IoT) to monitor and fight COVID-19. It consists of two main systems; AI/IoT for COVID-19 monitoring and drone-based IoT system for sterilizing. The two systems are integrated with the IoT paradigm and the developed algorithms are implemented on distributed fog units connected to the IoT network and controlled by software-defined networking (SDN). The proposed work is built based on a thermal camera mounted in a face-shield, or on a helmet that can be used by people during pandemics. The detected images, thermal images, are processed by the developed AI algorithm that is built based on the convolutional neural network (CNN). The drone system can be called, by the IoT system connected to the helmet, once infected cases are detected. The drone is used for sterilizing the area that contains multiple infected people. The proposed framework employs a single centralized SDN controller to control the network operations. The developed system is experimentally evaluated, and the results are introduced. Results indicate that the developed framework provides a novel, efficient scheme for monitoring and fighting COVID-19 and other future pandemics. © 2022 Tech Science Press. All rights reserved.},
publisher={Tech Science Press},
}

@ARTICLE{Balamurugan2022,
author={Balamurugan, N.M. and Mohan, S. and Adimoolam, M. and John, A. and reddy G, T. and Wang, W.},
title={DOA tracking for seamless connectivity in beamformed IoT-based drones},
journal={Computer Standards and Interfaces},
year={2022},
volume={79},
art_number={103564},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85114037711&doi=10.1016%2fj.csi.2021.103564&partnerID=40&md5=ffe345a148f5be583af7a85364fa51ba},
abstract={In recent times, there has been a surge of interest around the usage of adaptive antenna arrays of Internet of Things (IoT) based Drones in the communication systems. Adaptive antenna arrays have the ability to form customized radiation patterns based on the changes in the environment by employing methods for estimating Direction of Arrival (DOA) and adaptive beamforming. Nevertheless, upon deploying adaptive antenna arrays in complex IoT platforms, the radiation patterns that result from the use of such adaptive algorithms may be adjusted to the preceding location of the node and not attuned to the current location. These issues that arise due to mobility can be resolved by continuously tracking the DOA of the intended target. As DOA is time varying in an IoT Drone environment, existing algorithms for estimating the DOA like MUltiple SIgnal Classification (MUSIC) and Estimation of Signal Parameter via Rotational Invariance Techniques (ESPRIT) cannot be used to track the signal subspace recursively, as they are based on batch eigenvalue decomposition which is highly time consuming with a time complexity of O(n3). Furthermore, DOA estimation algorithms do not result in robust subspace estimates when the Signal to Noise Ratio (SNR) is low.The main novelty of the proposed work is a low computational complexity subspace tracking algorithm for tracking DOA in order to provide seamless connectivity. Simulation results show that the proposed DOA tracking takes lesser time for tracking the current location of the drone target as opposed to conventional DOA estimation methods. Furthermore,it is observed that the tracking process remains unaffected by SNR. © 2021},
publisher={Elsevier B.V.},
}

@ARTICLE{Niwa2021,
author={Niwa, H. and Sawai, Y.},
title={Verification of the detection performance of drone radio telemetry for tracking the movement of frogs},
journal={Drones},
year={2021},
volume={5},
number={4},
art_number={139},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85120086343&doi=10.3390%2fdrones5040139&partnerID=40&md5=1475b9e0da386878bd439e0c2b97aa00},
abstract={Elucidating the various behavioral and ecological uses of animal habitats is the basis for the conservation and management of animal species. Therefore, tracking the movement of animals is necessary. Biotelemetry is used for tracking the movement of animals. By mounting a radio telemetry receiver and antenna on a drone, the time and labor required for surveying animals can be reduced. In addition, it is easy to track difficult-to-reach areas such as rice paddies and forests, and the environment is not invaded by the survey. We think that this drone radio telemetry will be the best method for tracking the movement of small amphibians, such as frogs. However, in order to put the method to practical use, the accuracy of the system needs to be verified. Approximately 26 ha of area in Sogabe, Kameoka City, Kyoto Prefecture, Japan was investigated in this study. We selected and validated the location where frogs are likely to enter farmlands. The location where the detection of movement is expected to be stable are 5 cm deep areas in the soil, gaps in masonry, and under plastic bags, whereas areas in which the detection is likely to be unstable are areas deeper than 5 cm in the soil, covered concrete channels, and grass. By calculating the geographic center, the location of the nanotag could be estimated with an accuracy of less than 16 m. We successfully showed that the drone radio telemetry system used in this study is capable of detecting and tracking the movement of animals with high spatial and temporal resolutions. However, we suggest that the detection of movement may be interrupted depending on the location of the target animal and more than three detections are needed to guarantee the accuracy of the estimation. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
publisher={MDPI},
}

@ARTICLE{Filippi2021,
author={Filippi, M. and Hanlon, R. and Rypina, I.I. and Hodges, B.A. and Peacock, T. and Schmale, D.G., III},
title={Tracking a surrogate hazardous agent (Rhodamine dye) in a coastal ocean environment using in situ measurements and concentration estimates derived from drone images},
journal={Remote Sensing},
year={2021},
volume={13},
number={21},
art_number={4415},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85118746384&doi=10.3390%2frs13214415&partnerID=40&md5=fd0dfedfa4450345c4c67823ab7a6aee},
abstract={New tools and technology are needed to track hazardous agents such as oil and red tides in our oceans. Rhodamine dye (a surrogate hazardous agent) was released into the Atlantic ocean in August 2018, and experiments were conducted to track the movement of the dye near the water surface within three hours following the release. A DrOne Water Sampling SystEm (DOWSE), consisting of a 3D-printed sampling device tethered to a drone, was used to collect 26 water samples at different locations around the dye plume. Rhodamine concentrations were measured from the drone water samples using a fluorometer and ranged from 1 to 93 ppb. Dye images were taken during the drone-sampling of surface water containing dye and at about 10 m above the sampling point. These images were post-processed to estimate dye concentrations across the sampling domain. A comparison of calibrated heat maps showed that the altitude images yielded dye distributions that were qualitatively similar to those from images taken near the ocean surface. Moreover, the association between red ratios and dye concentrations yielded trendlines explaining up to 67% of the variation. Drones may be used to detect, track and assist in mitigating hazardous agents in the future. © 2020 by the authors. Licensee MDPI, Basel, Switzerland.},
publisher={MDPI},
}

@ARTICLE{Teixidó2021,
author={Teixidó, P. and Gómez-Galán, J.A. and Caballero, R. and Pérez-Grau, F.J. and Hinojo-Montero, J.M. and Muñoz-Chavero, F. and Aponte, J.},
title={Secured perimeter with electromagnetic detection and tracking with drone embedded and static cameras},
journal={Sensors},
year={2021},
volume={21},
number={21},
art_number={7379},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85118402820&doi=10.3390%2fs21217379&partnerID=40&md5=99c2f1cd8d576a97d7e43d5737b1d1dc},
abstract={Perimeter detection systems detect intruders penetrating protected areas, but modern solutions require the combination of smart detectors, information networks and controlling software to reduce false alarms and extend detection range. The current solutions available to secure a perimeter (infrared and motion sensors, fiber optics, cameras, radar, among others) have several prob-lems, such as sensitivity to weather conditions or the high failure alarm rate that forces the need for human supervision. The system exposed in this paper overcomes these problems by combining a perimeter security system based on CEMF (control of electromagnetic fields) sensing technology, a set of video cameras that remain powered off except when an event has been detected. An autono-mous drone is also informed where the event has been initially detected. Then, it flies through computer vision to follow the intruder for as long as they remain within the perimeter. This paper covers a detailed view of how all three components cooperate in harmony to protect a perimeter effectively, without having to worry about false alarms, blinding due to weather conditions, clearance areas, or privacy issues. The system also provides extra information of where the intruder is or has been, at all times, no matter whether they have become mixed up with more people or not during the attack. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
publisher={MDPI},
}

@ARTICLE{Lee202134237,
author={Lee, D.-H.},
title={CNN-based single object detection and tracking in videos and its application to drone detection},
journal={Multimedia Tools and Applications},
year={2021},
volume={80},
number={26-27},
pages={34237-34248},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85092404216&doi=10.1007%2fs11042-020-09924-0&partnerID=40&md5=bbf486a15020d78496728649fd80ee40},
abstract={This paper presents convolutional neural network (CNN)-based single object detection and tracking algorithms. CNN-based object detection methods are directly applicable to static images, but not to videos. On the other hand, model-free visual object tracking methods cannot detect an object until a ground truth bounding box of the target is provided. Moreover, many annotated video datasets of the target object are required to train both the object detectors and visual trackers. In this work, three simple yet effective object detection and tracking algorithms for videos are proposed to efficiently combine a state-of-the-art object detector and visual tracker for circumstances in which only a few static images of the target are available for training. The proposed algorithms are tested using a drone detection task and the experimental results demonstrated their effectiveness. © 2020, Springer Science+Business Media, LLC, part of Springer Nature.},
publisher={Springer},
}

@CONFERENCE{Koryttsev2021318,
author={Koryttsev, I. and Sheiko, S. and Kartashov, V. and Zubkov, O. and Oleynikov, V. and Selieznov, I. and Anohin, M.},
title={Practical Aspects of Range Determination and Tracking of Small Drones by Their Video Observation},
journal={2020 IEEE International Conference on Problems of Infocommunications Science and Technology, PIC S and T 2020 - Proceedings},
year={2021},
pages={318-322},
art_number={9468047},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85114443718&doi=10.1109%2fPICST51311.2020.9468047&partnerID=40&md5=f07e95196cc57a6d79033fd1a6491e46},
abstract={Different methods used for drones detection and estimation of their parameters (radar, acoustical, optical etc.). Among them optical methods can perform an important role in a precise definition of drones' coordinates, their tracking and recognition. The paper is devoted to the primary signal processing in the passive optical system with two channels of video observation and photosensitive matrices. The considered configuration of the optical system allows estimate a distance from a drone and realize its angle tracking on the base of measuring linear parallaxes of drones light images projected onto matrices. Experimental results include corrections of lens distortions. © 2020 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Zhu20214058,
author={Zhu, P. and Zheng, J. and Du, D. and Wen, L. and Sun, Y. and Hu, Q.},
title={Multi-Drone-Based Single Object Tracking with Agent Sharing Network},
journal={IEEE Transactions on Circuits and Systems for Video Technology},
year={2021},
volume={31},
number={10},
pages={4058-4070},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85098760520&doi=10.1109%2fTCSVT.2020.3045747&partnerID=40&md5=8606d1c8dfda5c05f34bbec0a73e0fa2},
abstract={Drones equipped with cameras (UAVs) can dynamically track the target in the air from a broader view compared with static cameras or moving sensors over the ground. However, it is still challenging to accurately track the target using a single drone due to several factors such as appearance variations and severe occlusions. To this end, we collect a new Multi-Drone single Object Tracking (MDOT) dataset that consists of 92 groups of video clips with 113, 918 high resolution frames taken by two drones and 63 groups of video clips with 145, 875 high resolution frames taken by three drones. Besides, two evaluation metrics are specially designed for multi-drone single object tracking, i.e., automatic fusion score (AFS) and ideal fusion score (IFS). Moreover, the agent sharing network (ASNet) is proposed by integrating self-supervised template sharing, target re-detection, and view-Aware fusion of the target from multiple drones into a unified framework, which can improve the tracking accuracy significantly compared with single drone tracking. Extensive experiments on MDOT show that our ASNet significantly outperforms recent state-of-The-Art trackers. The dataset can be found in https://github.com/VisDrone/MultiDrone. © 1991-2012 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Koundinya2021,
author={Koundinya, P.N. and Sanjukumar, N.T. and Rajalakshmi, P.},
title={A Comparative analysis of Algorithms for Pedestrian Tracking using Drone Vision},
journal={2021 IEEE 4th International Conference on Computing, Power and Communication Technologies, GUCON 2021},
year={2021},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85119100684&doi=10.1109%2fGUCON50781.2021.9573995&partnerID=40&md5=605da6bf96e87c530778a5594e4a32de},
abstract={In recent years, there has been an upsurge in the use of drones for various applications such as intelligent transportation, smart agriculture, military, product delivery, etc. With the advancement of high computational edge devices which can support Machine Learning and Deep Learning algorithms, various functions such as object detection and object tracking can be performed in real-time. Though there are many tracking algorithms available for object tracking, there is always a tradeoff between accuracy and their run-time. Executing computationally expensive algorithms is largely bottle-necked by hardware constraints. This paper has compared different object tracking algorithms (both conventional and Deep learning-based) based on tracking accuracy, speed of tracking, and computational complexity of each algorithm. The comparison is based on the accuracy of detection and tracking of an object at the beginning, end, or time of any occlusion scenario in the drone's video. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Upadhyay2021,
author={Upadhyay, J. and Rawat, A. and Deb, D.},
title={Multiple drone navigation and formation using selective target tracking-based computer vision},
journal={Electronics (Switzerland)},
year={2021},
volume={10},
number={17},
art_number={2125},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85114097896&doi=10.3390%2felectronics10172125&partnerID=40&md5=dfe25729da060b7ea3d36f512d58d786},
abstract={Autonomous unmanned aerial vehicles work seamlessly within the GPS signal range, but their performance deteriorates in GPS-denied regions. This paper presents a unique collaborative computer vision-based approach for target tracking as per the image’s specific location of interest. The proposed method tracks any object without considering its properties like shape, color, size, or pattern. It is required to keep the target visible and line of sight during the tracking. The method gives freedom of selection to a user to track any target from the image and form a formation around it. We calculate the parameters like distance and angle from the image center to the object for the individual drones. Among all the drones, the one with a significant GPS signal strength or nearer to the target is chosen as the master drone to calculate the relative angle and distance between an object and other drones considering approximate Geo-location. Compared to actual measurements, the results of tests done on a quadrotor UAV frame achieve 99% location accuracy in a robust environment inside the exact GPS longitude and latitude block as GPS-only navigation methods. The individual drones communicate to the ground station through a telemetry link. The master drone calculates the parameters using data collected at ground stations. Various formation flying methods help escort other drones to meet the desired objective with a single high-resolution first-person view (FPV) camera. The proposed method is tested for Airborne Object Target Tracking (AOT) aerial vehicle model and achieves higher tracking accuracy. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
publisher={MDPI},
}

@ARTICLE{Yamada2021,
author={Yamada, T. and Itoyama, K. and Nishida, K. and Nakadai, K.},
title={Assessment of sound source tracking using multiple drones equipped with multiple microphone arrays},
journal={International Journal of Environmental Research and Public Health},
year={2021},
volume={18},
number={17},
art_number={9039},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113489297&doi=10.3390%2fijerph18179039&partnerID=40&md5=78acb90e850ac824cc9059418d3c95f1},
abstract={Drone audition techniques are helpful for listening to target sound sources from the sky, which can be used for human searching tasks in disaster sites. Among many techniques required for drone audition, sound source tracking is an essential technique, and thus several tracking methods have been proposed. Authors have also proposed a sound source tracking method that utilizes multiple microphone arrays to obtain the likelihood distribution of the sound source locations. These methods have been demonstrated in benchmark experiments. However, the performance against various sound sources with different distances and signal-to-noise ratios (SNRs) has been less evaluated. Since drone audition often needs to listen to distant sound sources and the input acoustic signal generally has a low SNR due to drone noise, making a performance assessment against source distance and SNR is essential. Therefore, this paper presents a concrete evaluation of sound source tracking methods using numerical simulation, focusing on various source distances and SNRs. The simulated results captured how the tracking performance will change when the sound source distance and SNR change. The proposed approach based on location distribution estimation tended to be more robust against distance increase, while existing approaches based on directional estimation tended to be more robust against decreasing SNR. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
publisher={MDPI},
}

@ARTICLE{Barbary2021277,
author={Barbary, M. and ElAzeem, M.H.A.},
title={Drones tracking based on robust Cubature Kalman-TBD-Multi-Bernoulli filter},
journal={ISA Transactions},
year={2021},
volume={114},
pages={277-290},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85098634933&doi=10.1016%2fj.isatra.2020.12.042&partnerID=40&md5=b4a00dd6a26279d94484196c3f92956d},
abstract={The problem of nonlinear tracking and detection of small unmanned aerial vehicles and micro-drone targets is very challenging and has received great attention recently. Recently, the Cubature Kalman-multi-Bernoulli filter which employs a third-degree spherical-radical cubature rule has been presented to handle the nonlinear models. The Cubature Kalman filter is more principled and accurate in mathematical terms. In addition, a recent multi-Bernoulli filter based on variational Bayesian approximation has been presented with the estimation the fluctuation of variances of measurement. However, Cubature Kalman and variational Bayesian-Multi-Bernoulli filters are unsuitable for tracking the micro-drones because of the unknown probability of detection. As we known, the track-before-detect (TBD) schemes was an effective method for tracking the small objects. In this work, a novel robust Cubature Kalman-Multi-Bernoulli filter with variational Bayesian-TBD is proposed jointing with estimate the fluctuated variances of measurement. The improved filter is an effective method to solve the problem of detection profile estimation for micro-drones. A novel implementation with a non-linear Cubature Kalman Gaussian mixture and Inverse Gamma approximation is presented to estimate a hybrid kinematic state of micro-drones. The simulation results confirm the effectiveness and robustness of the proposed algorithm. © 2020 ISA},
publisher={ISA - Instrumentation, Systems, and Automation Society},
}

@ARTICLE{Zaidi2021,
author={Zaidi, A. and Kazim, M. and Weng, R. and Wang, D. and Zhang, X.},
title={Distributed Observer-Based Leader Following Consensus Tracking Protocol for a Swarm of Drones},
journal={Journal of Intelligent and Robotic Systems: Theory and Applications},
year={2021},
volume={102},
number={3},
art_number={64},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85108085373&doi=10.1007%2fs10846-021-01401-6&partnerID=40&md5=5ebc12a294bf08dad91a67e5065d8682},
abstract={This paper addresses the issue of cooperative control concerning the output synchronization of the linear time-invariant multi-input multi-output multi-agent system i.e., multi-unmanned aerial vehicle (a swarm of the drone), by designing observer-based consensus protocol with directed communication topology. Considering the leader following consensus tracking problem, an observer-based protocol is designed to obtain desirable output synchronization. The protocol design consists of a local observer for the leader drone and a distributed observer for the follower drones. Observer gains are optimized through a multi-step algorithm based on linear quadratic regulator controller and linear matrix inequalities. Most of the existing literature on cooperative control considers full state information for the controller as well as observer design. However, the protocol for the controller and observer design for consensus tracking of multi-unmanned aerial vehicles presented in this paper considers that only the relative partial states information from the corresponding neighboring drones are utilized. The designed algorithm is robust and guarantees that all the states of follower drones track the states of the leader drone and the consensus is achieved asymptotically even in the presence of external disturbances. Finally, considering the ideal and perturbed system, the efficacy of the analytical results are illustrated by comparative analysis using numerical simulations. © 2021, The Author(s), under exclusive licence to Springer Nature B.V.},
publisher={Springer Science and Business Media B.V.},
}

@ARTICLE{Woodgate2021,
author={Woodgate, J.L. and Makinson, J.C. and Rossi, N. and Lim, K.S. and Reynolds, A.M. and Rawlings, C.J. and Chittka, L.},
title={Harmonic radar tracking reveals that honeybee drones navigate between multiple aerial leks},
journal={iScience},
year={2021},
volume={24},
number={6},
art_number={102499},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85107271495&doi=10.1016%2fj.isci.2021.102499&partnerID=40&md5=2155106a6304bbe01ac197bc161b724a},
abstract={Male honeybees (drones) are thought to congregate in large numbers in particular “drone congregation areas” to mate. We used harmonic radar to record the flight paths of individual drones and found that drones favored certain locations within the landscape which were stable over two years. Drones often visit multiple potential lekking sites within a single flight and take shared flight paths between them. Flights between such sites are relatively straight and begin as early as the drone's second flight, indicating familiarity with the sites acquired during initial learning flights. Arriving at congregation areas, drones display convoluted, looping flight patterns. We found a correlation between a drone's distance from the center of each area and its acceleration toward the center, a signature of collective behavior leading to congregation in these areas. Our study reveals the behavior of individual drones as they navigate between and within multiple aerial leks. © 2021 The Author(s)},
publisher={Elsevier Inc.},
}

@CONFERENCE{Mata-Moya2021,
author={Mata-Moya, D. and Rey-Maestre, N. and Gomez-Del-Hoyo, P.-J. and Rosado-Sanz, J. and Jarabo-Amores, M.-P.},
title={4D Passive Radar for Drone Detection and Tracking},
journal={Proceedings International Radar Symposium},
year={2021},
volume={2021-June},
art_number={9466190},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113909664&doi=10.23919%2fIRS51887.2021.9466190&partnerID=40&md5=e67a24dcd11615c34f7328241811abcc},
abstract={An upgraded version of IDEPAR demonstrator capable of detecting and extracting parameters from targets in a 4D measurements space(range, Doppler, azimuth and elevation) is presented to allow the localization of small aerial drones in the Cartesian space (x,y,z). A two-stage spatial filtering processing scheme based on a 2D reception antenna system provides target's directions of arrival (azimuth, elevation) for targets' localization in the Cartesian space. The PR system was validated in measurement campaigns using small drones confirming the location capabilities of the proposed approach. © 2021 German Institute of Navigation (DGON).},
publisher={IEEE Computer Society},
}

@CONFERENCE{Harman2021,
author={Harman, S. and Ahmad, B.I.},
title={The Need for Simultaneous Tracking and Recognition in Drone Surveillance Radar},
journal={Proceedings International Radar Symposium},
year={2021},
volume={2021-June},
art_number={9466222},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113882484&doi=10.23919%2fIRS51887.2021.9466222&partnerID=40&md5=39a6c57d14efdad945b14b4fdad9aa37},
abstract={This paper focuses on the need for good target recognition in order to provide effective tracking and on good tracking to provide effective recognition in the application of radar to drone surveillance. The joint function, merging drone tracking and recognition, referred to as Simultaneous Tracking and Recognition (STaR) of drones is discussed and the benefits are presented through examples. This includes real measurements from Aveillant's Gamekeeper Radar. © 2021 German Institute of Navigation (DGON).},
publisher={IEEE Computer Society},
}

@CONFERENCE{Heidger2021,
author={Heidger, R. and Lambercy, V. and Lambers, D.},
title={Tracking Analysis of Drone Detection Systems at Airports: Methodology and Results},
journal={Proceedings International Radar Symposium},
year={2021},
volume={2021-June},
art_number={9466192},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113871508&doi=10.23919%2fIRS51887.2021.9466192&partnerID=40&md5=c7bcded901564f2e3ebd6454725f2049},
abstract={This paper describes the methodology that has been established in the DFS to test Drone Detection Systems (DDS) at airports, as well as the global test results of the test campaign conducted at Frankfurt and Munich airports in summer and autumn 2020 together with Fraport and FMG. The test campaign was part of a feasibility study to evaluate, what small noncooperative UAS current DDS systems today can detect and track at large infrastructures like airports, and which limitations exist. © 2021 German Institute of Navigation (DGON).},
publisher={IEEE Computer Society},
}

@CONFERENCE{Liang20211337,
author={Liang, N.S.J. and Srigrarom, S.},
title={Multi-camera multi-target drone tracking systems with trajectory-based target matching and re-identification},
journal={2021 International Conference on Unmanned Aircraft Systems, ICUAS 2021},
year={2021},
pages={1337-1344},
art_number={9476845},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85111466987&doi=10.1109%2fICUAS51884.2021.9476845&partnerID=40&md5=e7d53d6af9245dca1d0efbf1acfd4fa5},
abstract={This paper presents the integrated use of multiple cameras to detect, track and localize multiple moving objects, especially drones, in real-time by computer vision. The algorithm of the integrated system incorporates target tracking, localizing and identifying schemes, with the ability to use multiple cameras from different viewing angles and simultaneously track moving objects in the cameras' frames. Moving objects are detected by hybrid detection (motion-based blob detection appearance-based detection), and movements are predicted with Extended Kalman Filter. For motion-based detection, the trajectories of the tracked objects are analyzed using trajectory features variable. For appearance-based detection, motion is tracked with Yolo V3 detection algorithm. The integrated target identification algorithm matches and re-identifies targets between frames (intra-camera) and among cameras (inter-camera). This algorithm subsequently cross-correlate every tracked object in the different camera frames, and pair all the tracked targets to each other so that the cameras track the same objects for subsequent 3D localization. We tested our multi-cameras system to track multiple aerial and ground targets, and were successful in the re-identification of targets in real time. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Anastasiou2021927,
author={Anastasiou, A. and Makrigiorgis, R. and Kolios, P. and Panayiotou, C.},
title={Hyperion: A Robust Drone-based Target Tracking System},
journal={2021 International Conference on Unmanned Aircraft Systems, ICUAS 2021},
year={2021},
pages={927-933},
art_number={9476687},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85111435049&doi=10.1109%2fICUAS51884.2021.9476687&partnerID=40&md5=fd877456b5288f9b4ce307698d6fed2e},
abstract={Recent advances in mobile computing and embedded systems have had a transformative impact in the field of Unmanned Aircraft Systems (UASs). These advances have unlocked a great number of new capabilities ranging from realtime machine learning for detection and tracking of targets, and autonomous intelligent control for mission-critical trajectory planning. This paper introduces Hyperion, a robust detect, track and follow algorithm for UASs, leveraging and integrating various computer vision techniques and a combination of two proportional integral derivative (PID) controllers for following a moving vehicle. The proposed system is evaluated under real settings using off-the-shelf hardware and an elaborated comparison is made with a variety of state-of-the-art trackers available in the OpenCV library. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Sie20211085,
author={Sie, N.J. and Xuan Seah, S. and Chan, J.J. and Yi, J. and Chew, K.H. and Hooi Chan, T. and Srigrarom, S. and Holzapfel, F. and Hesse, H.},
title={Vision-based drones tracking using correlation filters and linear integrated multiple model},
journal={ECTI-CON 2021 - 2021 18th International Conference on Electrical Engineering/Electronics, Computer, Telecommunications and Information Technology: Smart Electrical System and Technology, Proceedings},
year={2021},
pages={1085-1090},
art_number={9454735},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85112805697&doi=10.1109%2fECTI-CON51831.2021.9454735&partnerID=40&md5=8b0bcd38e95202661430602feb767ba0},
abstract={This paper presents the use of Correlation Filters and Integrated Multiple Model (IMM) for filtering the position measurement of fast moving drones acquired by computer vision, with probability for model selection. The maneuvering movement of the drones are often non-linear making it hard to be estimated by a simple Kalman filter. Instead of using a non-linear filter which are more complex and non-universal, this paper attempt to integrate multiple filters to estimate the drone position using low computational cost. The IMM switches between the Constant Velocity (CV), Constant Acceleration (CA) and a Constant Turn (CT) model with a Markov Chain in different flight scenario depending on the drone movement. Other filters i.e. Kernelized Correlation Filter (KCF), Particle Filter (PF) and Discriminative Correlation Filter (DCF) models are also presented for direct comparison. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Patru2021138,
author={Patru, G.-C. and Vasilescu, I. and Rosner, D. and Tudose, D.},
title={Aerial Drone Platform for Asset Tracking Using an Active Gimbal},
journal={Proceedings - 2021 23rd International Conference on Control Systems and Computer Science Technologies, CSCS 2021},
year={2021},
pages={138-142},
art_number={9481038},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85112069331&doi=10.1109%2fCSCS52396.2021.00030&partnerID=40&md5=6843e6e74f86d795270818ea7e5610bb},
abstract={We present a low cost quadrotor drone platform capable of visual servoing using an on-board camera placed on an active gimbal and on-board computation. The drone was built using basic off-the-shelf components and a few custom 3D printed parts and open source software. We plan to use this platform for visual inspection using autonomous navigation including takeoff, tracking and landing. Most commercial platforms that we investigated are significantly more expensive and are not flexible enough for the task we envision. We demonstrate the performance of our system on a simple task of visual servoing above a fiduciary marker. A key element is the active gimbal which is driven to maintain the target in the center of the field-of-view, regardless of the drone maneuvers. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Yeom2021,
author={Yeom, S. and Nam, D.-H.},
title={Moving vehicle tracking with a moving drone based on track association},
journal={Applied Sciences (Switzerland)},
year={2021},
volume={11},
number={9},
art_number={4046},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85105792869&doi=10.3390%2fapp11094046&partnerID=40&md5=0fa28d97c8c8fadbfdff1951d618abfd},
abstract={The drone has played an important role in security and surveillance. However, due to the limited computing power and energy resources, more efficient systems are required for surveillance tasks. In this paper, we address detection and tracking of moving vehicles with a small drone. A moving object detection scheme has been developed based on frame registration and subtraction followed by morphological filtering and false alarm removing. The center position of the detected object area is the input to the tracking target as a measurement. The Kalman filter estimates the position and velocity of the target based on the measurement nearest to the state prediction. We propose a new data association scheme for multiple measurements on a single target. This track association method consists of the hypothesis testing between two tracks and track fusion through track selection and termination. We reduce redundant tracks on the same target and maintain the track with the least estimation error. In the experiment, drones flying at an altitude of 150 m captured two videos in an urban environment. There are a total of 9 and 23 moving vehicles in each video; the detection rates are 92% and 89%, respectively. The number of valid tracks is significantly reduced from 13 to 10 and 56 to 26 in the first and the second video, respectively. In the first video, the average position RMSE of two merged tracks are improved by 83.6% when only the fused states are considered. In the second video, the average position and velocity RMSE are 1.21 m and 1.97 m/s, showing the robustness of the proposed system. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
publisher={MDPI AG},
}

@CONFERENCE{Trapal2021162,
author={Trapal, D.D.C. and Leong, B.C.C. and Ng, H.W. and Zhong, J.T.G. and Srigrarom, S. and Chan, T.H.},
title={Improvement of Vision-based Drone Detection and Tracking by Removing Cluttered Background, Shadow and Water Reflection with Super Resolution},
journal={2021 6th International Conference on Control and Robotics Engineering, ICCRE 2021},
year={2021},
pages={162-168},
art_number={9435671},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85107773816&doi=10.1109%2fICCRE51898.2021.9435671&partnerID=40&md5=6acf92e6bf850762c7b7e6875c5e5303},
abstract={Detection and tracking of small and fast moving aerial targets especially drones has got attention nowadays. This paper focuses on the vision-based technique using images taken from observing cameras. In real life situations, the target drone objects maybe are hidden in the cluttered background such as trees shadow or foliage, rows of buildings, and other kind of scenery that will hinder the clear indication of the drones. The object is further confused by the presence of its shadow and reflection from the water or glass wall reflection. For vision-based objection, the clarity and the ambiguity of the target images in the video stream are the key for effective and successful target detection and tracking. Here, we present the improvement by mitigating the effect of cluttered background, shadow and water reflection to the target images. We applied the schemes to make the drone more visible and more clear. We also implemented super resolution to increase the image resolution for more precise detection and tracking. As a result, the target drone could be detected and tracked throughout the sample clips. The comparative tracking results using DCF are presented. Likewise, we applied the water removal scheme to eliminate the reflection to avoid confusion to the tracker. With this, just the correct drone targets were detected and tracked. Overall, the drones could be detected and tracked all the way, as long as they appeared in the camera scene. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Sie2021139,
author={Sie, N.J. and Srigrarom, S. and Huang, S.},
title={Field Test Validations of Vision-based Multi-camera Multi-drone Tracking and 3D Localizing with Concurrent Camera Pose Estimation},
journal={2021 6th International Conference on Control and Robotics Engineering, ICCRE 2021},
year={2021},
pages={139-144},
art_number={9435654},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85107766876&doi=10.1109%2fICCRE51898.2021.9435654&partnerID=40&md5=fa3061c3d01f6d685364d3cc5f65b41e},
abstract={This paper reports the field test validations of the recently proposed vision-based real-time multi-camera setups for detecting, tracking and 3D localizing multiple aerial targets (mainly drones). We also propose the additional concurrent camera pose estimation when the camera poses are not known beforehand. This extra step can be used alongside (in parallel) with the drone tracking and localizing process. We conducted flight tests using 2 drones flying in 2 specific scenarios, and used 3 cameras to observe, detect, track and locate the positions of both drones in global frame. The efficacy of our technique is measured by the accuracy of the temporal and spatial positions of the observed drones, against the drones' own GPS recordings. Our initial results show reasonable accuracy, i.e. ±1m at 50m, as such, the proposed vision-based methods can be used for drone detection and tracking. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Pavliv20211455,
author={Pavliv, M. and Schiano, F. and Reardon, C. and Floreano, D. and Loianno, G.},
title={Tracking and Relative Localization of Drone Swarms with a Vision-Based Headset},
journal={IEEE Robotics and Automation Letters},
year={2021},
volume={6},
number={2},
pages={1455-1462},
art_number={9324934},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85099723615&doi=10.1109%2fLRA.2021.3051565&partnerID=40&md5=7d1eab81195955500e46f1d03c8ec2c5},
abstract={We address the detection, tracking, and relative localization of the agents of a drone swarm from a human perspective using a headset equipped with a single camera and an Inertial Measurement Unit (IMU). We train and deploy a deep neural network detector on image data to detect the drones. A joint probabilistic data association filter resolves the detection problems and couples this information with the headset IMU data to track the agents. In order to estimate the drones' relative poses in 3D space with respect to the human, we use an additional deep neural network that processes image regions of the drones provided by the tracker. Finally, to speed up the deep neural networks' training, we introduce an automated labeling process relying on a motion capture system. Several experimental results validate the effectiveness of the proposed approach. The approach is real-time, does not rely on any communication between the human and the drones, and can scale to a large number of agents, often called swarms. It can be used to spatially task a swarm of drones and also employed without a headset for formation control and coordination of terrestrial vehicles. © 2016 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Lu2021205,
author={Lu, P. and Ding, Y. and Wang, C.},
title={Multi-small target detection and tracking based on improved yolo and sift for drones},
journal={International Journal of Innovative Computing, Information and Control},
year={2021},
volume={17},
number={1},
pages={205-224},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85100698692&doi=10.24507%2fijicic.17.01.205&partnerID=40&md5=21fe14bdf957c4f985783a73e14cf0eb},
abstract={Multi-target tracking algorithms applied to drones often face more detection algorithm, while achieving active tracking of small targets and fast-moving targets. In response to these problems, this paper proposes a multi-small target detection and tracking method based on improved YOLO and SIFT for drones. First, we prune the network of the YOLO algorithm. Through sparse training, channel pruning, and network adjust-ment, the drone can deploy a target detection network with a smaller model. Secondly, we propose a method of adaptive threshold and minimum distance and optimize SIFT feature extraction, achieve effective detection of small targets, and improve tracking accuracy and success rate. Finally, we consider the needs of the UAV to track fast-moving targets, we use scale and position information to complete the data association, and the UAV can effectively track fast-moving targets. The algorithm of this paper is evaluat-ed by the VisDrone 2019 MOT benchmark data set. The leading evaluation indicators MOTA and MOTP are 38.7 and 75.7. The secondary evaluation indicators IDF1, ML, and FN, etc. all perform better. The algorithm meets the complex task requirements of multi-target tracking for UAVs. © ICIC International.},
publisher={ICIC International},
}

@ARTICLE{Tohma2021155,
author={Tohma, E. and Tadakuma, K. and Chinen, H. and Suriyon, T. and Anezaki, T.},
title={Wild animal detection and tracking drone system using centerline extraction [中心線抽出を用いたドローンによる野生動物の発見及び追跡システムの提案]},
journal={IEEJ Transactions on Industry Applications},
year={2021},
volume={141},
number={2},
pages={155-160},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85100165765&doi=10.1541%2fieejias.141.155&partnerID=40&md5=f2e156ec01c95af4b5398be300f17431},
abstract={In recent years, damage by wild animals has become a serious problem, primarily in rural areas in Japan. In 2018, the amount of crop damage was estimated at approximately 15.7 billion yen. As a solution to this problem, a wild animal detection and expulsion system by drone has been devised, however, there are problems where the FPV operation requires human cost and the drone is operational only in a narrow area. It is essential that autonomous wide-area long-distance flight is required to realize the practical and full-scale use of drones. The authors have been developing a non-GPS autonomous control drone system for power line inspection, animal detection, and tracking. In this study, we propose a detection and tracking system with autonomous wide-area flight drones to prevent damage by wild animals. We verified the effectiveness of our combination of a deep learning system trained by images taken by a drone equipped with a camera having a wide field of view and flying at low altitude for image magnification, and our centerline extraction method for more accurate discrimination of wild boars. © 2021 The Institute of Electrical Engineers of Japan.},
publisher={Institute of Electrical Engineers of Japan},
}

@CONFERENCE{Yi2021,
author={Yi, J. and Chew, K.H. and Srigrarom, S.},
title={Enabling Continuous Drone Tracking across Translational Scene Transitions through Frame-Stitching},
journal={2021 2nd International Symposium on Instrumentation, Control, Artificial Intelligence, and Robotics, ICA-SYMP 2021},
year={2021},
art_number={9358444},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85102533218&doi=10.1109%2fICA-SYMP50206.2021.9358444&partnerID=40&md5=10d74e3d4953c9de3eb9a7f800506a91},
abstract={This paper introduces a method for enabling the continuous tracking of drones across translational scene transitions through the introduction of a stationary global frame. The main benefit of such a method is that it allows current pan-tilt-zoom (PTZ) cameras commonly used in security applications to be used in the domain of drone tracking. The first step in the process is to correct for lens distortion with the intrinsic parameters of the camera obtained through calibration. The motion of the camera frame is then estimated using the optical flow of tracked features from frame to frame. Information obtained about the translational motion of the frame is then used to construct a global frame on which object tracking is performed. Results from the comparison of object detection and tracking performed on two clips with and without pre-processing to construct the global frame show an improvement in tracking performance when the technique was applied to the video. The method was shown to successfully compensate for the relative velocity of objects in the frame relative to the frame, with no sudden changes of velocity during the scene transition. In addition, the introduction of a global frame enabled the continuous tracking of a stationary drone that was reassigned to a new track in the original video. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Srigrarom2021,
author={Srigrarom, S. and Sie, N.J.L. and Cheng, H. and Chew, K.H. and Lee, M. and Ratsamee, P.},
title={Multi-camera Multi-drone Detection, Tracking and Localization with Trajectory-based Re-identification},
journal={2021 2nd International Symposium on Instrumentation, Control, Artificial Intelligence, and Robotics, ICA-SYMP 2021},
year={2021},
art_number={9358454},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85102508687&doi=10.1109%2fICA-SYMP50206.2021.9358454&partnerID=40&md5=252f23d2f6e3c6adbfd8d8fc6b3dd48c},
abstract={This paper presents a real-time multiple camera system for detecting, tracking and localizing multiple moving drones simultaneously in a 3 dimension space. The distinct feature of the system is in its target re-identification process, which provides for information fusion among cameras based on the targets' trajectories and relative locations. Drones are detected by the multiple camera system based on motion-based blob detection, and the 2D locations of each drone in individual camera frames are tracked by A geometry- and camera-based model. From the paths of the tracked drones, their trajectories are examined using drone track feature variable. Cross-correlated among cameras for object re-identifications will allow the individual 2D position information to be integrated into overall global 3D positions of all the tracked drones from all cameras. Preliminary outdoor flight demonstrations with 2 drones flying in formation and using 3 cameras show optimal results. The system is able to detect, track, localize and re-identifying individual drone with average positional error of 8%. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Yamada2021394,
author={Yamada, T. and Itoyama, K. and Nishida, K. and Nakadai, K.},
title={Sound Source Tracking Using Integrated Direction Likelihood for Drones with Microphone Arrays},
journal={2021 IEEE/SICE International Symposium on System Integration, SII 2021},
year={2021},
pages={394-399},
art_number={9382619},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85103739038&doi=10.1109%2fIEEECONF49454.2021.9382619&partnerID=40&md5=9bd6cbbdf73a198b342a01e653223971},
abstract={This paper presents a method for sound source localization and tracking using drones with microphone arrays. Signal processing with multiple microphone arrays enables us to estimate the sound source location via triangulation strategies. However in drone applications, triangulation approaches have difficulties in stable estimation of direction due to drone noise. Accordingly, we propose a novel method we call PArticle Filtering with Integrated MUSIC (PAFIM). PAFIM uses the strategy of direct localization which estimates the location likelihood distribution rather than estimating sound source directions. In this way, sound source locations can be estimated robustly than discrete triangulation. Numerical simulations demonstrated that PAFIM is effective in tracking moving sound sources with a root mean square error within 15% of sound source distance. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Safaei202155,
author={Safaei, A. and Sharf, I.},
title={Adaptive model-free formation-tracking controller and observer for collaborative payload transport by four drones},
journal={2021 IEEE International Symposium on Safety, Security, and Rescue Robotics, SSRR 2021},
year={2021},
pages={55-62},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85123623964&doi=10.1109%2fSSRR53300.2021.9597872&partnerID=40&md5=f3780c8bedc72678cb74810e978f3801},
abstract={In this paper, a solution is provided for collaborative transportation of a rigid payload by four quadrotors, while a desired formation topology is maintained among the vehicles. Each quadrotor is connected to the payload using a rigid link, where the joints to the payload are located on two perpendicular lines through the center of mass of the payload. The proposed solution includes an adaptive control scheme comprising several modules. Each module is responsible for controlling the motion of a specific subsystem of the entire payload-links-quadrotors system. Since an adaptive model-free control algorithm is utilized for tracking the desired set-points for each module, no information on the inertial parameters of the drones is required. The formation topology is achieved among the quadrotors by a geometry-based solution. Moreover, by utilizing a special linear Kalman filter for estimating the unit vectors along the connecting rigid links, the requirement for position and velocity estimation of the drones is revoked. Instead, the position and velocity of the payload must be estimated by using appropriate sensors. The solution is validated via numerical simulation of transporting a payload along a time-varying trajectory. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Marcos2021,
author={Marcos, J.T.C. and Utete, S.W.},
title={Animal Tracking within a Formation of Drones},
journal={Proceedings of 2021 IEEE 24th International Conference on Information Fusion, FUSION 2021},
year={2021},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85123425876&partnerID=40&md5=a1bc588fc70488b2d9d3951505344cdc},
abstract={In this study, we develop a distributed system that can be used by unmanned aerial vehicles (UAVs) or drones for single-animal tracking in terrestrial settings. The system involves a video object tracking (VOT) solution and a drone formation. The proposed VOT solution is based on the particle filter (PF) with two measurement providers: a colour image segmentation (CIS) approach and a machine learning (ML) technique. They are switched based on the structural similarity (SSIM) index between the initial and the current target appearances to mitigate the limitation of computational resources of civilian drones, and to ensure good tracking performance. At first, the deep learning object detector You Only Look Once version three (YOLOv3) is used as the second measurement provider. The proposed VOT solution has been tested on wildlife footage recorded by drones (and obtained from an animal behaviour group). The tests demonstrate amongst other results that the proposed VOT solution is more efficient when YOLOv3 is replaced by other methods such as boosting and channel and spatial reliability tracking (CSRT). The results suggest the utility of the proposed VOT solution in single-animal tracking with cooperative drones for wildlife preservation. © 2021 International Society of Information Fusion (ISIF).},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Liu2021,
author={Liu, C. and Jian, Z. and Xie, M. and Cheng, I.},
title={A Real-Time Mobile Application for Cattle Tracking using Video Captured from a Drone},
journal={2021 International Symposium on Networks, Computers and Communications, ISNCC 2021},
year={2021},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85123425738&doi=10.1109%2fISNCC52172.2021.9615648&partnerID=40&md5=da9922cf084debae79928cd9b380e6cd},
abstract={In many countries, governments have issued laws on cattle traceability, which require farmers to keep track of their livestock. While there are many algorithms to monitor cattle in confined indoor environments, monitoring cattle of a large number in outdoor pastures is still an open research problem. In recent years, with the advancement of unmanned aerial vehicles, e.g., drones, cattle monitoring can be based on images captured by drones. However, the challenges include image analysis in real-time, and keeping track of a dynamic scene (cattle movements) based on a moving sensor device. In this work, we develop an iOS application that can send captured herd images to our deep-learning-based server for cow segmentation and counting. Furthermore, the app can guide the operator to control the drone flight route and viewing perspectives. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Phung2021189,
author={Phung, K.-P. and Lu, T.-H. and Nguyen, T.-T. and Le, N.-L. and Nguyen, H.-H. and Hoang, V.-P.},
title={Multi-model Deep Learning Drone Detection and Tracking in Complex Background Conditions},
journal={International Conference on Advanced Technologies for Communications},
year={2021},
volume={2021-October},
pages={189-194},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85122942707&doi=10.1109%2fATC52653.2021.9598317&partnerID=40&md5=1efcc3b7b42865ce80289e93f937799d},
abstract={The recent popularity of drones with quadcopter layouts is threatening public safety and personal privacy. With the ability to hover and perform complex maneuvers even in indoor conditions, equipped with video cameras as well as capable of carrying hazardous materials, drones can truly become a security threat, especially to vulnerable organizations. Therefore, detecting and tracking drones in secured areas poses an urgent task for the surveillance system. In this paper, we design a real-time drone detection and tracking system with the combination of multiple deep learning and computer vision techniques: 1) Yolo-v4 model for detecting drones and 2) visual models for tracking drones. Besides, we have collected and labeled a larger drone dataset by mixing the existing datasets with our collected images. We evaluated three deep learning models for drone detection on this dataset and acquired the Yolo-V4 model to be the highest detection performance with AP = 34.63%. Combining this detection model and the existing visual tracking modules can boost the drone tracking up to more than 20fps for different backgrounds at around 700m by using an usual PC without GPU. © 2021 IEEE.},
publisher={IEEE Computer Society},
}

@CONFERENCE{Chen20212839,
author={Chen, G. and Wang, W. and He, Z. and Wang, L. and Yuan, Y. and Zhang, D. and Zhang, J. and Zhu, P. and Van Gool, L. and Han, J. and Hoi, S. and Hu, Q. and Liu, M. and Sciarrone, A. and Sun, C. and Garibotto, C. and Tran, D.N.-N. and Lavagetto, F. and Haleem, H. and Motorcu, H. and Ates, H.F. and Nguyen, H.-H. and Jeon, H.-J. and Bisio, I. and Jeon, J.W. and Li, J. and Pham, L.H. and Jeon, M. and Feng, Q. and Li, S. and Tran, T.H.-P. and Pan, X. and Song, Y.-M. and Yao, Y. and Du, Y. and Xu, Z. and Luo, Z.},
title={VisDrone-MOT2021: The Vision Meets Drone Multiple Object Tracking Challenge Results},
journal={Proceedings of the IEEE International Conference on Computer Vision},
year={2021},
volume={2021-October},
pages={2839-2846},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85122776407&doi=10.1109%2fICCVW54120.2021.00318&partnerID=40&md5=ae844c8f5ec548c634fca39509c6f9f2},
abstract={Vision Meets Drone: Multiple Object Tracking (VisDrone-MOT2021) challenge - the forth annual activity organized by the VisDrone team - focuses on benchmarking UAV MOT algorithms in realistic challenging environments. It is held in conjunction with ICCV 2021. VisDrone-MOT2021 contains 96 video sequences in total, including 56 sequences (~24K frames) for training, 7 sequences (~3K frames) for validation and 33 sequences (~13K frames) for testing. Bounding-box annotations for novel object categories are provided every frame and temporally consistent instance IDs are also given. Additionally, occlusion ratio and truncation ratio are provided as extra useful annotations. The results of eight state-of-the-art MOT algorithms are reported and discussed. We hope that our VisDrone-MOT2021 challenge will facilitate future research and applications in the field of UAV vision. The website of our challenge can be found at http://www.aiskyeye.com/. © 2021 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Watanabe2021,
author={Watanabe, S. and Mukai, M.},
title={Optimal trajectory generation of a drone for wheelchair tracking using mixed-integer programming},
journal={Artificial Life and Robotics},
year={2021},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85119193234&doi=10.1007%2fs10015-021-00710-1&partnerID=40&md5=4c14f850210966df838b71d944ad9374},
abstract={This study considers the optimal-trajectory generation problem in which a drone recognizes a wheelchair with an onboard camera while avoiding collision with obstacles. The optimal-trajectory generation was developed as a mixed-integer programming problem. The same method was used to recognize the wheelchair. In this regard, the optimal-trajectory generation problem was solved at each time step using model predictive control, and the first element of the optimal input was applied. The MATLAB optimization toolbox was used to solve this problem. As a result, the drone could avoid obstacles while recognizing the wheelchair that moved to the target trajectory considering the signals transmitted by the drone. © 2021, International Society of Artificial Life and Robotics (ISAROB).},
publisher={Springer Japan},
}

@ARTICLE{Zhu2021,
author={Zhu, P. and Wen, L. and Du, D. and Bian, X. and Fan, H. and Hu, Q. and Ling, H.},
title={Detection and Tracking Meet Drones Challenge},
journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
year={2021},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85117829718&doi=10.1109%2fTPAMI.2021.3119563&partnerID=40&md5=c43578b3a3e4c36018e9c9059ebd75da},
abstract={Drones, or general UAVs, equipped with cameras have been fast deployed with a wide range of applications, including agriculture, aerial photography, and surveillance. Consequently, automatic understanding of visual data collected from drones becomes highly demanding, bringing computer vision and drones more and more closely. To promote and track the developments of object detection and tracking algorithms, we have organized three challenge workshops in conjunction with ECCV 2018, ICCV 2019 and ECCV 2020, attracting more than 100 teams around the world. We provide a large-scale drone captured dataset, VisDrone, which includes four tracks, i.e., (1) image object detection, (2) video object detection, (3) single object tracking, and (4) multi-object tracking. We first present a thorough review of object detection and tracking datasets and benchmarks, and discuss the challenges of collecting large-scale drone-based object detection and tracking datasets with fully manual annotations. Being the largest such dataset ever published, VisDrone enables extensive evaluation and investigation of visual analysis algorithms for the drone platform. We provide a detailed analysis of the current state of the field of large-scale object detection and tracking on drones, and conclude the challenge as well as propose future directions. IEEE},
publisher={IEEE Computer Society},
}

@CONFERENCE{Wen20217808,
author={Wen, L. and Du, D. and Zhu, P. and Hu, Q. and Wang, Q. and Bo, L. and Lyu, S.},
title={Detection, Tracking, and Counting Meets Drones in Crowds: A Benchmark},
journal={Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
year={2021},
pages={7808-7817},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85117415528&doi=10.1109%2fCVPR46437.2021.00772&partnerID=40&md5=80daa8aeaace5518fd87ae6406bad1f9},
abstract={To promote the developments of object detection, tracking and counting algorithms in drone-captured videos, we construct a benchmark with a new drone-captured large-scale dataset, named as DroneCrowd, formed by 112 video clips with 33, 600 HD frames in various scenarios. Notably, we annotate 20, 800 people trajectories with 4.8 million heads and several video-level attributes. Meanwhile, we design the Space-Time Neighbor-Aware Network (STNNet) as a strong baseline to solve object detection, tracking and counting jointly in dense crowds. STNNet is formed by the feature extraction module, followed by the density map estimation heads, and localization and association subnets. To exploit the context information of neighboring objects, we design the neighboring context loss to guide the association subnet training, which enforces consistent relative position of nearby objects in temporal domain. Extensive experiments on our DroneCrowd dataset demonstrate that STNNet performs favorably against the state-of-the-arts. © 2021 IEEE},
publisher={IEEE Computer Society},
}

@ARTICLE{Trinh2021137148,
author={Trinh, P.V. and Carrasco-Casado, A. and Okura, T. and Tsuji, H. and Kolev, D.R. and Shiratama, K. and Munemasa, Y. and Toyoshima, M.},
title={Experimental Channel Statistics of Drone-to-Ground Retro-Reflected FSO Links with Fine-Tracking Systems},
journal={IEEE Access},
year={2021},
volume={9},
pages={137148-137164},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85117238064&doi=10.1109%2fACCESS.2021.3117266&partnerID=40&md5=eeefbfecf0b6e5f5f7108e2727e7cef5},
abstract={The utilization of drones as flying base stations (BSs) in the sixth-generation (6G) cellular networks has attracted much attention recently. In this context, free-space optical (FSO) systems could be deployed to provide high-capacity fronthaul/backhaul links between drones and ground BSs. Particularly, a drone-to-ground FSO communication link can be established by equipping the drone with a modulating retro-reflector (MRR) to modulate the incoming optical beam and reflect the modulated beam back along the same path. This helps to alleviate stringent pointing requirements from the drone while satisfying the limited size, weight, and power (SWaP) consumption requirements. Nevertheless, the underlying physical channel effects of this aerial retro-reflected FSO system have never been experimentally explored in the literature. In this paper, we report, for the first time, the experimental channel statistics of a drone-to-ground retro-reflected FSO link, offering practical insights into the angle-of-arrival (AoA) fluctuations at the receiver, the channel coherence time, the probability of fade, the level crossing rate, the average fade duration, and the time-frequency channel characteristics. Our results are expected to serve as practical sources of reference for the theoretical performance analyses and engineering designs of drone-based retro-reflected FSO systems. © 2013 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@BOOK{Boudjit2021101,
author={Boudjit, K. and Larbes, C. and Ramzan, N.},
title={Visual object tracking by quadrotor AR.Drone using artificial neural networks and fuzzy logic controller},
journal={AI for Emerging Verticals: Human-robot computing, sensing and networking},
year={2021},
pages={101-132},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85114587940&doi=10.1049%2fPBPC034E_ch5&partnerID=40&md5=22b353d97881277f343009e3b600b24d},
abstract={In this chapter, we consider the visual object-tracking problem in order to find an efficient and useful method for UAV. The aim of this study is to demonstrate the feasibility and the potential of incorporating Al into autonomous target tracking for UAVs applications. A proof-of-concept prototype was developed based on the UAV platform Parrot AR.Drone 2.0 and by using the Robot Operating System (ROS) and the package ardrone_autonomy simulated in Gazebo simulator. In the first section of this work, a fuzzy logic controller (FLC) is used for visual object tracking by using the AR.Drone 2.0 and visual information feedback. Fuzzy logic is used for its ability to shape the control surfaces generated by the rules of the fuzzy inference system. In order to guarantee a correct recognition of the target by the AR.Drone 2.0, a quick response (QR) code and ar track_alvar package in ROS have been used as target marker. Visual feedback is provided by identification of visual tags, using open-source software FuzzyLite to calculate the tag identification match and orientation. The proposed algorithm is based on a small number of input parameters, which reduces the requirements for high computing power. The developed algorithm was validated by simulation studies and in-flight tests. Chapter Contents: • 5.1 Introduction • 5.2 System overview • 5.2.1 Control system • 5.2.2 Quadrotor dynamic model • 5.3 Fuzzy-logic-based identification and target tracking • 5.3.1 Simulation studies • 5.3.2 Experimental setup • 5.4 Artificial neural networks (ANN) for target identification and tracking using a quadrotor • 5.4.1 Design of the neural network • 5.4.1.1 Input layer • 5.4.1.2 Output layer • 5.4.1.3 Data collection and training phase • 5.4.2 Simulation results • 5.4.3 Experimental validation and results • 5.5 Conclusion • References. © The Institution of Engineering and Technology 2021.},
publisher={Institution of Engineering and Technology},
}

@ARTICLE{Chang2021427,
author={Chang, Y.},
title={Inflight Tracking Method with Beacon System and Scouting Drone},
journal={Lecture Notes in Electrical Engineering},
year={2021},
volume={715},
pages={427-433},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85101506842&doi=10.1007%2f978-981-15-9343-7_59&partnerID=40&md5=e6a93fd880bb6d35877f1365c0a7c829},
abstract={In this study, we designed an inflight tracking method that can track the current position and the flight route of the target drone through the beacon system and GPS from the scout drone in the beacon range of the target drone. The scouting drone can fly and approach to the inflight target drone to receive the beacon signal in range. If the scout drone receives the beacon signal from a target drone, it checks the beacon information and transmits it to the control center with its GPS data to identify and track the target drone. The inflight tracking method can calculate the current position and flight route of the target drone through the two or more GPS data and flight data at the check positions from the scout drone. The precision of the inflight tracking method can be affected by the critical distance and the number of check positions. To enhance the tracking precision, the scout drone checks two or three different check positions within the critical distance from the inflight target drone. The experimental results showed the proposed inflight tracking method has at least over 92% in the worst case of the experimental environment. © 2021, Springer Nature Singapore Pte Ltd.},
publisher={Springer Science and Business Media Deutschland GmbH},
}

@CONFERENCE{Estrada20211,
author={Estrada, C. and Sun, L.},
title={Trajectory tracking control of a drone-guided hose system for fluid delivery},
journal={AIAA Scitech 2021 Forum},
year={2021},
pages={1-11},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85100306479&partnerID=40&md5=7b796e81ffb0ca1a2a8348a4fde84885},
abstract={In this paper, we present a nonlinear trajectory-tracking controller for a multicopter to delivea pressurized fluid through an attached hose system. The three-dimensional (3D) dynamic modeof the entire system is derived that incorporates multicopter dynamics, the reaction force from the release of the fluid, and the force applied by the weight of the hose. The magnitude of the fluid-release reaction force is calculated using the Newton's second law. The force applied by thhose weight onto the mutlicopter dynamics is determined using a catenary approach for a low-tension cable. The nonlinear model predictive control (MPC) technique was applied to develothe controller that is able to drive the multicopter to track two predened 3D trajectories whiltaking the operational constraints of the multicopter into account. The simulation results show the effectiveness of the MPC controller. © 2021, American Institute of Aeronautics and Astronautics Inc, AIAA. All rights reserved.},
publisher={American Institute of Aeronautics and Astronautics Inc, AIAA},
}

@CONFERENCE{Fussi20211,
author={Fussi, M. and Corsi, E. and Rinaldi, G. and Alibani, M. and Pollini, L.},
title={Simultaneous tracking of multiple drones using convolutional neural networks and optical flow},
journal={AIAA Scitech 2021 Forum},
year={2021},
pages={1-11},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85099805074&partnerID=40&md5=7149ab425780d505836abceb56d30149},
abstract={The aim of this paper is to implement a multi-object tracker for detecting, discriminating and following multiple drones on the 2D image plane. The main system consists in a neural network trained for detecting drones on the image plane. Once the drones are identified, their Region Of Interest information are sent to the Kalman filter based tracking system in order to compute position estimates. Each detected drone is given an ID using the Global Nearest Neighbor and Auction Algorithms, then the tracking system employs a set of Kalman filters and each measure is assigned to the respective estimate/filter using the unique ID. In order to reduce the effects of the neural network computation (e.g detection) time, every position estimate is corrected using Optical Flow. Results are evaluated through MOT (Multi-Object Tracking) Metrics, aiming to demonstrate the benefits of implementing Optical Flow algorithms for building a robust multi-tracking system. © 2021, American Institute of Aeronautics and Astronautics Inc, AIAA. All rights reserved.},
publisher={American Institute of Aeronautics and Astronautics Inc, AIAA},
}

@ARTICLE{Oleksyn20211,
author={Oleksyn, S. and Tosetto, L. and Raoult, V. and Williamson, J.E.},
title={Drone-based tracking of the fine-scale movement of a coastal stingray (Bathytoshia brevicaudata)},
journal={Remote Sensing},
year={2021},
volume={13},
number={1},
pages={1-24},
art_number={40},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85098771914&doi=10.3390%2frs13010040&partnerID=40&md5=897ac87ec5610360c46f5b2f246a9a14},
abstract={Coastal ecosystems are under threat from a range of anthropogenic impacts that disrupt habitat connectivity and the ability for animals to move within them. Understanding fine-scale animal movement provides insight into how animals are responding to these pressures, and underpins effective ecological management and conservation strategies. This study used drones to investigate the drivers of the fine-scale movement of rays in coastal estuaries using the short-tail stingray (Bathytoshia brevicaudata) as a model species. Smaller rays swam with more regular bursts of speed and greater sinuosity than larger individuals, indicating that rays of different sizes alter their fine-scale movement behavior to maintain energetic efficiency. Rays were less likely to spend time resting and swam faster on the high tide compared to the outgoing tide. They were also more likely to exhibit bursts of speed at noon (11 am to 1 pm) than at other times of day. Body size, tide and time of day all influenced ray movement. Understanding the ecological variables that influence the fine-scale movement of rays and the potential for human activities to alter natural behaviors is integral to the implementation of effective management strategies for this group of animals and their ecosystems. © 2021, MDPI AG. All rights reserved.},
publisher={MDPI AG},
}

@ARTICLE{Shin20211,
author={Shin, J.-M. and Kim, Y.-S. and Ban, T.-W. and Choi, S. and Kang, K.-M. and Ryu, J.-Y.},
title={Position tracking techniques using multiple receivers for anti-drone systems},
journal={Sensors (Switzerland)},
year={2021},
volume={21},
number={1},
pages={1-14},
art_number={35},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85098670763&doi=10.3390%2fs21010035&partnerID=40&md5=c639a79645c9d19242a90f07eb961df0},
abstract={The need for drone traffic control management has emerged as the demand for drones increased. Particularly, in order to control unauthorized drones, the systems to detect and track drones have to be developed. In this paper, we propose the drone position tracking system using multiple Bluetooth low energy (BLE) receivers. The proposed system first estimates the target’s location, which consists of the distance and angle, while using the received signal strength indication (RSSI) signals at four BLE receivers and gradually tracks the target based on the estimated distance and angle. We propose two tracking algorithms, depending on the estimation method and also apply the memory process, improving the tracking performance by using stored previous movement information. We evaluate the proposed system’s performance in terms of the average number of movements that are required to track and the tracking success rate. © 2020 by the authors. Licensee MDPI, Basel, Switzerland.},
publisher={MDPI AG},
}

@ARTICLE{Xu20211626,
author={Xu, Y. and Peng, J. and Ye, H. and Zhong, W. and Wei, Q.},
title={Design of Real-Time Vehicle Tracking System for Drones Based on ROS},
journal={Advances in Intelligent Systems and Computing},
year={2021},
volume={1274 AISC},
pages={1626-1637},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85093109385&doi=10.1007%2f978-981-15-8462-6_186&partnerID=40&md5=daebcdb5f50bde1e5b80bb5c239f4847},
abstract={When using vehicles to hunt down criminal vehicles, the difficulty of chasing criminals is increased due to factors such as vision, surrounding environment and road conditions. In order to solve this problem, we have designed a real-time vehicle tracking system based on ROS. The system uses Pixhawk as the flight control platform in the hardware part. Its internal integrated attitude control module and altitude control module are mainly responsible for controlling the attitude of the aircraft to achieve the effect of stable flight of the aircraft. The GPS module is responsible for acquiring coordinate position data, so that the aircraft can achieve the fixed point effect. This system solves the problem that a processor has insufficient resources when processing relatively large data. Compared with using vehicles to chase criminal vehicles, this system can solve the problem of increasing the difficulty of chasing criminals due to factors such as visual field, surrounding environment and road conditions. This system greatly improves the pursuit efficiency. © 2021, The Editor(s) (if applicable) and The Author(s), under exclusive license to Springer Nature Singapore Pte Ltd.},
publisher={Springer Science and Business Media Deutschland GmbH},
}

@ARTICLE{Cajo2021528,
author={Cajo, R. and Zhao, S. and Plaza, D. and De Keyser, R. and Ionescu, C.},
title={A fractional order predictive control for trajectory tracking of the ar.drone quadrotor},
journal={Lecture Notes in Electrical Engineering},
year={2021},
volume={695 LNEE},
pages={528-537},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85091315012&doi=10.1007%2f978-3-030-58653-9_51&partnerID=40&md5=91b85cf3808ca75824a3408bc7d5b8c6},
abstract={A fractional-order model predictive control with extended prediction self-adaptive control (FOMPC-EPSAC) strategy is proposed for the AR.Drone quadrotor system. The objective is to achieve an optimal trajectory tracking control for an AR.Drone quadrotor by using a fractional order integral cost function in the conventional MPC-EPSAC algorithm. In addition, a particle swarm optimization (PSO) algorithm is applied to find the optimal weighting matrices, which depend on the terms ($$\alpha $$, $$\beta $$) of the fractional order cost function. Some simulation results show the superiority of FOMPC-EPSAC over conventional MPC-EPSAC with respect to trajectory tracking and robustness under wind disturbances. © The Editor(s) (if applicable) and The Author(s), under exclusive license to Springer Nature Switzerland AG 2021.},
publisher={Springer Science and Business Media Deutschland GmbH},
}

@ARTICLE{Guo2020,
author={Guo, J. and Ahmad, I. and Chang, K.H.},
title={Classification, positioning, and tracking of drones by HMM using acoustic circular microphone array beamforming},
journal={Eurasip Journal on Wireless Communications and Networking},
year={2020},
volume={2020},
number={1},
art_number={9},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85077507201&doi=10.1186%2fs13638-019-1632-9&partnerID=40&md5=6a5717f70f3fd8dbf78af3c10b815ced},
abstract={This paper addresses issues with monitoring systems that identify and track illegal drones. The development of drone technologies promotes the widespread commercial application of drones. However, the ability of a drone to carry explosives and other destructive materials may pose serious threats to public safety. In order to reduce these threats, we propose an acoustic-based scheme for positioning and tracking of illegal drones. Our proposed scheme has three main focal points. First, we scan the sky with switched beamforming to find sound sources and record the sounds using a microphone array; second, we perform classification with a hidden Markov model (HMM) in order to know whether the sound is a drone or something else. Finally, if the sound source is a drone, we use its recorded sound as a reference signal for tracking based on adaptive beamforming. Simulations are conducted under both ideal conditions (without background noise and interference sounds) and non-ideal conditions (with background noise and interference sounds), and we evaluate the performance when tracking illegal drones. © 2020, The Author(s).},
publisher={Springer},
}

@CONFERENCE{Hilal2020108,
author={Hilal, A.A. and Mismar, T.},
title={Drone Positioning System Based on Sound Signals Detection for Tracking and Photography},
journal={11th Annual IEEE Information Technology, Electronics and Mobile Communication Conference, IEMCON 2020},
year={2020},
pages={108-115},
art_number={9284851},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85099299507&doi=10.1109%2fIEMCON51383.2020.9284851&partnerID=40&md5=85f4d678efe48fd3007f75a457a1b337},
abstract={This paper aims to build a positioning system that allows a Drone to locate a sound source effectively. The system consists of an application that communicates remotely with three sensors to compute the location of an object. The collected data from the sensors will be used to find the intersection point where the sound originates. All system components are built to work wirelessly to avoid any wiring problems by populating the data from the sensors, then instructing the Drone to move and capture a picture. This work is convenient in many sites, like tracking an object motion to do some tasks or following its operator by detecting the voice. The experiments showed consistent actions, when the sensors identify the sound signal, the process of computing, transmitting, and Drone moving was very successful. In all trials, the Drone detected the sound and was moving toward the source directly. Then, a picture was captured approximately one meter away far from the object, which is an appropriate distance. © 2020 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Papaioannou20207919,
author={Papaioannou, S. and Kolios, P. and Panayiotou, C.G. and Polycarpou, M.M.},
title={Cooperative simultaneous tracking and jamming for disabling a rogue drone},
journal={IEEE International Conference on Intelligent Robots and Systems},
year={2020},
pages={7919-7926},
art_number={9340835},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85102412665&doi=10.1109%2fIROS45743.2020.9340835&partnerID=40&md5=1e6b469d3f74bff2cdfc2a2ee14369ec},
abstract={This work investigates the problem of simultaneous tracking and jamming of a rogue drone in 3D space with a team of cooperative unmanned aerial vehicles (UAVs). We propose a decentralized estimation, decision and control framework in which a team of UAVs cooperate in order to a) optimally choose their mobility control actions that result in accurate target tracking and b) select the desired transmit power levels which cause uninterrupted radio jamming and thus ultimately disrupt the operation of the rogue drone. The proposed decision and control framework allows the UAVs to reconfigure themselves in 3D space such that the cooperative simultaneous tracking and jamming (CSTJ) objective is achieved; while at the same time ensures that the unwanted inter-UAV jamming interference caused during CSTJ is kept below a specified critical threshold. Finally, we formulate this problem under challenging conditions i.e., uncertain dynamics, noisy measurements and false alarms. Extensive simulation experiments illustrate the performance of the proposed approach. © 2020 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Chaoraingern2020145,
author={Chaoraingern, J. and Tipsuwanporn, V. and Numsomran, A.},
title={Modified adaptive sliding mode control for trajectory tracking of mini-drone quadcopter unmanned aerial vehicle},
journal={International Journal of Intelligent Engineering and Systems},
year={2020},
volume={13},
number={5},
pages={145-158},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85090380213&doi=10.22266%2fijies2020.1031.14&partnerID=40&md5=2a59482fbb712eaf3f89adeae8b495f7},
abstract={Unmanned Aerial Vehicles are among the most widely attracting interest, especially in the applications of transportation, inspection, and surveillance. The great mechanisms for motion control are set to become a vital factor in performing the robust and accurate stabilized flight relied on perturbations and disturbances. This paper presents modified adaptive sliding mode control for trajectory tracking of mini-drone quadcopter unmanned aerial vehicles, which aims at demonstrating the effectiveness of nonlinear adaptive control strategy for achieving the desired performance of the mini-drone quadcopter system. Besides providing mathematical modeling and nonlinear dynamic characteristic details of mini-drone quadcopter actuated system, the modified adaptive sliding mode algorithm is developed using adaptation law based on Lyapunov stability approach then applied on the attitude loop and the altitude loop control system so that the nonlinear adaptive behavior of the controller enables the compensation of disturbances and parameter perturbations. The effectiveness validations of the proposed control technique compared with the traditional approach are performed through the Matlab simulation. The results have been illustrated that the modified adaptive sliding mode control can decrease the error performance indexes to the minimum ISE at 1.041 m2 and the zero percentage of overshoot while enables excellent stability and robustness even in the presence of parameter perturbations and disturbance. © 2020, Intelligent Network and Systems Society.},
publisher={Intelligent Network and Systems Society},
}

@ARTICLE{Demir20201625,
author={Demir, B. and Ergunay, S. and Nurlu, G. and Popovic, V. and Ott, B. and Wellig, P. and Thiran, J.-P. and Leblebici, Y.},
title={Real-time high-resolution omnidirectional imaging platform for drone detection and tracking},
journal={Journal of Real-Time Image Processing},
year={2020},
volume={17},
number={5},
pages={1625-1635},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85074700180&doi=10.1007%2fs11554-019-00921-7&partnerID=40&md5=ca09300a973af4909bdf83c5d8857a02},
abstract={Drones have become steadily affordable, which raises privacy and security concerns as well as interest in drone detection systems. On the other hand, drone detection is a challenging task due to small dimensions of drones, difficulty of long-distance detection, strict real-time constraints and necessity of wide angle coverage for drones. Although different radar and audio-assisted drone detection systems have been presented, they suffer from the cost, range, or interference problems. On the contrary, a long-range detection can be obtained by a vision-based system. Aiming that, we propose a real-time moving object detection and tracking system optimized for drone detection using 16 cameras with 20 MP resolution. The proposed system detects drones from short range and long range with 360∘ surveillance coverage owing high-performance ultra-high-resolution (320 MP) video-processing capability. It is able to detect drones with 100 cm diameter from 700 m distance despite deceptive background. It is interference free, so multiple systems can properly operate in the vicinity without effecting each other. It integrates processing power of embedded systems with flexibility of software to generate a full platform for drone detection and tracking. © 2019, Springer-Verlag GmbH Germany, part of Springer Nature.},
publisher={Springer},
}

@CONFERENCE{Jarabo-Amores2020,
author={Jarabo-Amores, M.-P. and Mata-Moya, D. and Gomez-Del-Hoyo, P.-J. and Del-Rey-Maestre, N. and Rosado-Sanz, J.},
title={On the Impact of Drone Airscrews Signature on Passive Radar Detection and Tracking Stages},
journal={IEEE National Radar Conference - Proceedings},
year={2020},
volume={2020-September},
art_number={9266658},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85098582302&doi=10.1109%2fRadarConf2043947.2020.9266658&partnerID=40&md5=ac6f2fdb8999169787cc939f7bccdcfa},
abstract={In this paper, the impact of the drone airscrews signature in passive radars exploiting Digital Video Broadcasting signals is tackled. Beamforming techniques optimized to minimize the variance of the interference using the statistical characterization of real clutter data followed by a CFAR detector are used to detect drones and their associated airscrews signature. An independent bi-dimensional tracker based on the Kalman filter is proposed to tackle the drone and airscrews tracking process, and to extract micro-Doppler signature features. Real radar data acquired by a technological demonstrator developed at the University of Alcalá were used to evaluate the proposed solution. Results proved the suitability of the proposed detection and tracking schemes for airscrews signature feature extraction. Ansys HFSS electromagnetic simulator validated the results. © 2020 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Srigrarom2020615,
author={Srigrarom, S. and Hoe Chew, K.},
title={Hybrid motion-based object detection for detecting and tracking of small and fast moving drones},
journal={2020 International Conference on Unmanned Aircraft Systems, ICUAS 2020},
year={2020},
pages={615-621},
art_number={9213912},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85094978319&doi=10.1109%2fICUAS48674.2020.9213912&partnerID=40&md5=6b3a625e05b0a0c4ad29592c29b60c95},
abstract={A hybrid detecting and tracking system that is made especially for small and fast moving drones in which the other existing techniques cannot detect is presented. This new automatic system integrates geometry estimation, 2D object detection, 3D localization, trajectory estimation and tracking for dynamic scene interpretation. This caters to moving cameras, e.g. those mounted on a separate flying platform. The technique is built on the unified two-step real-time algorithm for detection and tracking of moving objects (DATMO) in dynamic outdoor environments. The first step is built on the motion-based detection approach for early detection of an object when the targeted object is still far away and appears very small in the scene. The second step is based on the appearance-based detection approach for continual detection, further identification and verification of the object. The camera's own position is estimated by 3D triangulation of the static landscape in the scene, doubled up as ground truth. This includes both the pan-tilt-zoom motion and the camera's vibration compensation. Therefore, the drone can be tracked, even when the camera is in motion and/or under jittery condition. As a result, the position of the tracked drone in the global inertial coordinate is further improved. Subsequently, the drone motion is tracked using the Extended Kalman Filter scheme. Initial results show that this hybrid system is able to detect a small drone from a distance away in less than a few frames after such a drone appears in the scene. The drone is always tracked as long as it is in the camera's field of view. As this technique is vision-based, this drone detection and tracking system can expand to detect multiple drones. © 2020 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Zhou2020,
author={Zhou, H. and Ni, B.},
title={Tracking of drone flight by neural network Siamese-RPN},
journal={Proceedings - 2020 6th International Conference on Engineering, Applied Sciences and Technology, ICEAST 2020},
year={2020},
art_number={9165441},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85091984976&doi=10.1109%2fICEAST50382.2020.9165441&partnerID=40&md5=77fe44bc4ab70154b9b3827ba896a3e1},
abstract={Recently deep learning has made a great progress in the image classification and video object tracking. However the speed of traditional region proposal algorithms is too slow and become a bottleneck. Researchers have proposed a lot of neural networks for the improvements. With the region proposal network proposed, neural network can finish the computation enabling cost-free region proposals, which make it possible to do real-time detection and tracking. This paper will set up a system which can detect and track drone by using neural networks such as Faster R-CNN and Siamese-RPN. © 2020 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Hamdi2020,
author={Hamdi, A. and Salim, F. and Kim, D.Y.},
title={DroTrack: High-speed drone-based object tracking under uncertainty},
journal={IEEE International Conference on Fuzzy Systems},
year={2020},
volume={2020-July},
art_number={9177571},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85090502234&doi=10.1109%2fFUZZ48607.2020.9177571&partnerID=40&md5=d812ed4752293897e36d11218c741fd9},
abstract={We present DroTrack, a high-speed visual single-object tracking framework for drone-captured video sequences. Most of the existing object tracking methods are designed to tackle well-known challenges, such as occlusion and cluttered backgrounds. The complex motion of drones, i.e., multiple degrees of freedom in three-dimensional space, causes high uncertainty. The uncertainty problem leads to inaccurate location predictions and fuzziness in scale estimations. DroTrack solves such issues by discovering the dependency between object representation and motion geometry. We implement an effective object segmentation based on Fuzzy C Means (FCM). We incorporate the spatial information into the membership function to cluster the most discriminative segments. We then enhance the object segmentation by using a pre-trained Convolution Neural Network (CNN) model. DroTrack also leverages the geometrical angular motion to estimate a reliable object scale. We discuss the experimental results and performance evaluation using two datasets of 51, 462 drone-captured frames. The combination of the FCM segmentation and the angular scaling increased DroTrack precision by up to 9% and decreased the centre location error by 162 pixels on average. DroTrack outperforms all the high-speed trackers and achieves comparable results in comparison to deep learning trackers. DroTrack offers high frame rates up to 1000 frame per second (fps) with the best location precision, more than a set of state-of-the-art real-time trackers. © 2020 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Donaire2020,
author={Donaire, J.A. and Galí, N. and Gulisova, B.},
title={Tracking visitors in crowded spaces using zenith images: Drones and time-lapse},
journal={Tourism Management Perspectives},
year={2020},
volume={35},
art_number={100680},
note={cited By 7},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85083784216&doi=10.1016%2fj.tmp.2020.100680&partnerID=40&md5=e4d3ae2be83993919c6aeaf697bc9b2d},
abstract={The aim of this article is to analyse the extent to which zenith images can be used to study visitor behaviour in crowded spaces. The paper presents two studies of zenith image capture in two micro-spaces (both monumental heritage sites) in the north-east of Spain: the first used drone images to conduct a quantitative study on patterns of visitor use at Empúries archaeological site; and the second was a qualitative study on conflicts of use in Cathedral Square, Girona, using time-lapse photography from a fixed camera. Results of the study show that visitor behaviour at the sites does not alter in peak season when spaces become increasingly crowded. © 2020 Elsevier Ltd},
publisher={Elsevier B.V.},
}

@ARTICLE{Nguyen20201266,
author={Nguyen, N.T. and Prodan, I. and Lefèvre, L.},
title={Flat trajectory design and tracking with saturation guarantees: a nano-drone application},
journal={International Journal of Control},
year={2020},
volume={93},
number={6},
pages={1266-1279},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85052058030&doi=10.1080%2f00207179.2018.1502474&partnerID=40&md5=599029b899aa66ff4decf432ddeb4eef},
abstract={This paper deals with the problem of trajectory planning and tracking of a quadcopter system based on the property of differential flatness. First, B-spline characterisations of the flat output allow for optimal trajectory generation subject to waypoint constraints, thrust and angle constraints while minimising the trajectory length. Second, the proposed tracking control strategy combines feedback linearisation and nested saturation control via flatness. The control strategy provides bounded inputs (thrust, roll and pitch angles) while ensuring the overall stability of the tracking error dynamics. The control parameters are chosen based on the information of the a priori given reference trajectory. Moreover, conditions for the existence of these parameters are presented. The effectiveness of the trajectory planning and the tracking control design is analysed and validated through simulation and experimental results over a real nano-quadcopter platform, the Crazyflie 2.0. © 2018, © 2018 Informa UK Limited, trading as Taylor & Francis Group.},
publisher={Taylor and Francis Ltd.},
}

@CONFERENCE{Famili2020,
author={Famili, A. and Park, J.-M.J.},
title={ROLATIN: Robust Localization and Tracking for Indoor Navigation of Drones},
journal={IEEE Wireless Communications and Networking Conference, WCNC},
year={2020},
volume={2020-May},
art_number={9120619},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85087284057&doi=10.1109%2fWCNC45663.2020.9120619&partnerID=40&md5=5d991b173d79822a6b33eb105eafc1ab},
abstract={In many drone applications, drones need the ability to fly fully or partially autonomously to carry out their mission. To enable such fully/partially autonomous flights, the ground control station that is supporting the drone's operation needs to constantly localize and track the drone, and send this information to the drone's navigation controller to enable autonomous/semiautonomous navigation. In outdoor environments, localization and tracking can be readily carried out using GPS and the drone's Inertial Measurement Units (IMUs). However, in indoor areas or GPS-denied environments, such an approach is not feasible. In this paper, we propose a localization and tracking scheme for drones called ROLATIN (Robust Localization and Tracking for Indoor Navigation of drones) that was specifically devised for GPS-denied environments. Instead of GPS signals, ROLATIN relies on speakergenerated ultrasonic acoustic signals to estimate the target drone's location and track its movement. Compared to vision and RF signal-based methods, our scheme offers a number of advantages in terms of performance and cost. © 2020 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Tao2020463,
author={Tao, L. and Hong, T. and Chao, X.},
title={Drone identification and location tracking based on YOLOv3 [基于YOLOv3的无人机识别与定位追踪]},
journal={Gongcheng Kexue Xuebao/Chinese Journal of Engineering},
year={2020},
volume={42},
number={4},
pages={463-468},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85084657549&doi=10.13374%2fj.issn2095-9389.2019.09.10.002&partnerID=40&md5=9886fcd3c298392dc440f5898d521b69},
abstract={In recent years, increasing incidents of drone intrusion have occurred, and the drone collisions have become common. As a result, accidents may occur in densely populated areas. Therefore, drone monitoring is an important research topic in the field of security. Although many types of drone monitoring programs exist, most of them are costly and difficult to implement. To solve this problem, in the 5G context, this study proposed a method of using a city's existing monitoring network to acquire data based on a deep learning algorithm for drone target detection, constructing a recognizable drone, and tracking the unmanned aerial vehicle. The method used the improved YOLOv3 (You only look once) model to detect the presence of drones in video frames. The YOLOv3 algorithm is the third generation version of the YOLO series, belonging to the one-stage target detection algorithm. This algorithm has significant advantages over the two-stage type of algorithm in speed. YOLOv3 outputs the position information of the drone in the video frame. According to the position information, the PID (Proportion integration differentiation) algorithm was used to adjust the center of the camera to track the drone. Then, the parameters of the plurality of cameras were used to calculate the actual coordinates of the drone, thereby realizing the positioning. We built the dataset by taking photos of the drone's flight, searching and downloading drone pictures from the Internet, and labeling the drones in the image by using the labelImg tool. The dataset was classified according to the number of rotors of the drone. In the experiment, the detection model was trained by the dataset classified by the number of rotors. The trained model can achieve 83.24% accuracy and 88.15% recall rate on the test set, and speed of 20 frames per second on the computer equipped with NVIDIA GTX 1060 for real-time tracking. © All right reserved.},
publisher={Science Press},
}

@ARTICLE{Chang20203161,
author={Chang, Y. and Zhou, H. and Wang, X. and Shen, L. and Hu, T.},
title={Cross-Drone Binocular Coordination for Ground Moving Target Tracking in Occlusion-Rich Scenarios},
journal={IEEE Robotics and Automation Letters},
year={2020},
volume={5},
number={2},
pages={3161-3168},
art_number={9006781},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85081700285&doi=10.1109%2fLRA.2020.2975713&partnerID=40&md5=a31fa9edb331777149312ebb14354a82},
abstract={How to work effectively under occlusion-rich environments remains a challenge for airborne vision-based ground target tracking, due to the natural limitation of monocular vision. Given this, a novel cross-drone binocular coordination approach, inspired by the efficient coordination of human eyes, is proposed and developed. The idea, derived from neural models of the human visual system, is to utilize distributed target measurements to overcome occlusion effects. Eventually, a binocular coordination controller is developed. It enables two distributed pan-tilt cameras to execute synergistic movements similar to human eyes. The proposed approach is able to work based on binocular or monocular vision, and hence it is practically appropriate for various environments. Both testbed experiments and field experiments are conducted for performance evaluation. Testbed experiments highlight its advantages over independent tracking in terms of accuracy while being robust to a partial perception ratio of up to 43%. Field experiments with a pair of drones further demonstrate its effectiveness in the real-world scenarios. © 2016 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Song20201696,
author={Song, W. and Li, S. and Chang, T. and Hao, A. and Zhao, Q. and Qin, H.},
title={Cross-view contextual relation transferred network for unsupervised vehicle tracking in drone videos},
journal={Proceedings - 2020 IEEE Winter Conference on Applications of Computer Vision, WACV 2020},
year={2020},
pages={1696-1705},
art_number={9093382},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85085472501&doi=10.1109%2fWACV45572.2020.9093382&partnerID=40&md5=61691aca9fb5728811c7d2eee654ca4e},
abstract={Recently CNN-centric object tracking methods have been gaining tremendous success in ground-view videos, however, it remains hard to cope with vehicle tracking in unmanned aerial vehicle (UAV) videos. The key difficulties mainly stem from lacking large-scale well-labeled training datasets and view-invariant appearance model for fast-moving drone-view vehicles. We enhance the vehicle's cross-view feature by exploring relations between the pivotal context and the target to facilitate unsupervised vehicle tracking. The relation is modeled as the relevance of the target and its contextual regions in the tracking task. Specifically, we propose a contextual relation actor-critic (CRAC) framework integrates an actor-critic agent with a dual GAN learning mechanism, which aims to dynamically search the related contextual regions and transfer the relations from ground-view to drone-view videos while retaining the discriminative features. We demonstrate that CRAC could be applied to several state-of-the-art trackers by extensive experiments and ablation studies on four public benchmarks. All the experiments confirm that, our CRAC can improve the performance of state-of-the-art methods in terms of accuracy, robustness, and versatility. © 2020 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Pham2020,
author={Pham, H.A. and Soriano, T. and Ngo, V.H. and Gies, V.},
title={Distributed adaptive neural network control applied to a formation tracking of a group of low-cost underwater drones in hazardous environments},
journal={Applied Sciences (Switzerland)},
year={2020},
volume={10},
number={5},
art_number={1732},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85081980126&doi=10.3390%2fapp10051732&partnerID=40&md5=32da075ecf072039b645612a6485f503},
abstract={This paper addresses a formation tracking problem of multiple low-cost underwater drones by implementing distributed adaptive neural network control (DANNC). It is based on a leader-follower architecture to operate in hazardous environments. First, unknown parameters of underwater vehicle dynamics, which are important requirements for real-world applications, are approximated by a neural network using a radial basis function. More specifically, those parameters are only calculated by local information, which can be obtained by an on-board camera without using an external positioning system. Secondly, a potential function is employed to ensure there is no collision between the underwater drones. We then propose a desired configuration of a group of unmanned underwater vehicles (UUVs) as a time-variant function so that they can quickly change their shape between them to facilitate the crossing in a narrow area. Finally, three UUVs, based on a robot operating system (ROS) platform, are used to emphasize the realistic low-cost aspect of underwater drones. The proposed approach is validated by evaluating in different experimental scenarios. © 2020 by the authors.},
publisher={MDPI AG},
}

@ARTICLE{Paredes2020,
author={Paredes, J.A. and Álvarez, F.J. and Aguilera, T. and Aranda, F.J.},
title={Precise drone location and tracking by adaptive matched filtering from a top-view ToF camera},
journal={Expert Systems with Applications},
year={2020},
volume={141},
art_number={112989},
note={cited By 7},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85072872514&doi=10.1016%2fj.eswa.2019.112989&partnerID=40&md5=4b7c87435862bd245b4f8bcc6389c31e},
abstract={Nowadays the use of drones is rapidly growing, and the autonomous navigation capability depends on knowing their position at any time. The precision and robustness of a local positioning system for these devices is of particular importance in takeoff and landing maneuvers, especially in GPS-denied environments. The main contribution of this work lies in the development of a precise local positioning and tracking system for drones. For this purpose, a ToF camera has been installed on the ceiling in order to make use of its depth maps. Taking as a reference the disturbance caused by a quadrotor in one of these maps, a novel 2D matched filter has been designed based on a Gaussian wavelet. This filter allows the system to quickly detect all drones flying in the scene. Moreover, it is dynamically adapted to the image portion that they occupy, taking into account the variation of this parameter with their flying altitude, which has also been theoretically determined. The whole algorithm leads to a precise 3D drone positioning. In addition, the proposed system is also robust against short-time occlusions, since the measurements history can be used to predict future positions, thus avoiding the complete loss of tracking. © 2019 Elsevier Ltd},
publisher={Elsevier Ltd},
}

@ARTICLE{Kai202018,
author={Kai, Y. and Munir, H.M.U. and Onda, M. and Adachi, Y. and Hayama, J. and Zhao, Y. and Tanioka, T. and Locsin, R. and Takase, K. and Dino, M.J.S.},
title={Evaluation of the Remote-controlled Drone System using an Eye-tracking device through the Internet for patients in bedridden conditions},
journal={Enfermeria Clinica},
year={2020},
volume={30},
pages={18-22},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85079774704&doi=10.1016%2fj.enfcli.2019.12.005&partnerID=40&md5=bf60940f60ce6aa7b4de5514c4f4219c},
abstract={In many countries, the rate of aging in their population is rapidly increasing. It is expected that this increasing trend influences the number of patients in bedridden states who have difficulty moving their extremities, such as those patients with amyotrophic lateral sclerosis (ALS). The patients are limited in many aspects of their daily lives; this includes not seeing what is outside of their rooms, affecting their quality of life (QOL). Thus, this study aims to evaluate the Remote-controlled Drone System using the Eye-tracking device through the Internet (RDSEI) to improve QOL for patients in bedridden conditions. The novel RDSEI is proposed and developed by the Kai laboratory. The RDSEI consists of a drone, a transmitter, a control screen, an eye-tracking device, a video capture device, a server computer, and a client computer. The subjects of this experimental evaluation of the RDSEI were five healthy male adults (average age: 20.6 years old). Experimental results indicated that all the subjects could control the drone easily by using this system, although there were delays, blurriness, and freezing of the video. Therefore, it was concluded that by using this system, the subjects could control the drone by only their eye movements, thereby enabling them to see the outside world through the drone's camera. In the future, the patients will be able to control the RDSEI from remote locations and converse with persons in remote locations. © 2019 Elsevier España, S.L.U.},
publisher={Elsevier Doyma},
}

@CONFERENCE{Gözen202010082,
author={Gözen, D. and Özer, S.},
title={Visual object tracking in drone images with deep reinforcement learning},
journal={Proceedings - International Conference on Pattern Recognition},
year={2020},
pages={10082-10089},
art_number={9413316},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85110437567&doi=10.1109%2fICPR48806.2021.9413316&partnerID=40&md5=8d8523943d903916bb794f6e5f5fcc1b},
abstract={There is an increasing demand on utilizing camera equipped drones and their applications in many domains varying from agriculture to entertainment and from sports events to surveillance. In such drone applications, an essential and a common task is tracking an object of interest visually. Drone (or UAV) images have different properties when compared to the ground taken (natural) images and those differences introduce additional complexities to the existing object trackers to be directly applied on drone applications. Some important differences among those complexities include (i) smaller object sizes to be tracked and (ii) different orientations and viewing angles yielding different texture and features to be observed. Therefore, new algorithms trained on drone images are needed for the drone-based applications. In this paper, we introduce a deep reinforcement learning (RL) based single object tracker that tracks an object of interest in drone images by estimating a series of actions to find the location of the object in the next frame. This is the first work introducing a single object tracker using a deep RL-based technique for drone images. Our proposed solution introduces a novel reward function that aims to reduce the total number of actions taken to estimate the object's location in the next frame and also introduces a different backbone network to be used on low resolution images. Additionally, we introduce a set of new actions into the action library to better deal with the above-mentioned complexities. We compare our proposed solutions to a state of the art tracking algorithm from the recent literature and demonstrate up to 3.87% improvement in precision and 3.6% improvement in IoU values on the VisDrone2019 data set. We also provide additional results on OTB-100 data set and show up to 3.15% improvement in precision on the OTB-100 data set when compared to the same previous state of the art algorithm. Lastly, we analyze the ability to handle some of the challenges faced during tracking, including but not limited to occlusion, deformation, and scale variation for our proposed solutions. © 2020 IEEE},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Svanström20207265,
author={Svanström, F. and Englund, C. and Alonso-Fernandez, F.},
title={Real-time drone detection and tracking with visible, thermal and acoustic sensors},
journal={Proceedings - International Conference on Pattern Recognition},
year={2020},
pages={7265-7272},
art_number={9413241},
note={cited By 6},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85109250336&doi=10.1109%2fICPR48806.2021.9413241&partnerID=40&md5=2fca213bab1dd99da7d217f33a31f4af},
abstract={This paper explores the process of designing an automatic multi-sensor drone detection system. Besides the common video and audio sensors, the system also includes a thermal infrared camera, which is shown to be a feasible solution to the drone detection task. Even with slightly lower resolution, the performance is just as good as a camera in visible range. The detector performance as a function of the sensor-to-target distance is also investigated. In addition, using sensor fusion, the system is made more robust than the individual sensors, helping to reduce false detections. To counteract the lack of public datasets, a novel video dataset containing 650 annotated infrared and visible videos of drones, birds, airplanes and helicopters is also presented1. The database is complemented with an audio dataset of the classes drones, helicopters and background noise. © 2020 IEEE},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Zhang2020638,
author={Zhang, X. and Jiao, L. and Liu, X. and Li, X. and Zhang, W. and Zhu, H. and Zhang, J.},
title={A Deep Learning Filter for Visual Drone Single Object Tracking},
journal={Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
year={2020},
volume={12538 LNCS},
pages={638-650},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85101785168&doi=10.1007%2f978-3-030-66823-5_38&partnerID=40&md5=7225f8989e49509aaff0db09b24a36a8},
abstract={Object tracking is one of the most important topics in computer vision. In visual drone tracking, it is an extremely challenging due to various factors, such as camera motion, partial occlusion, and full occlusion. In this paper, we propose a deep learning filter method to relieve the above problems, which is to obtain a priori position of the object at the subsequent frame and predict its trajectory to follow up the object during occlusion. Our tracker adopts the geometric transformation of the surrounding of the object to prevent the bounding box of the object lost, and it uses context information to integrate its motion trend thereby tracking the object successfully when it reappears. Experiments on the VisDrone-SOT2018 test dataset and the VisDrone-SOT2020 val dataset illustrate the effectiveness of the proposed approach. © 2020, Springer Nature Switzerland AG.},
publisher={Springer Science and Business Media Deutschland GmbH},
}

@ARTICLE{Stadler2020604,
author={Stadler, D. and Sommer, L.W. and Beyerer, J.},
title={PAS Tracker: Position-, Appearance- and Size-Aware Multi-object Tracking in Drone Videos},
journal={Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
year={2020},
volume={12538 LNCS},
pages={604-620},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85101779406&doi=10.1007%2f978-3-030-66823-5_36&partnerID=40&md5=12e2cc955cb288ce85486e6ea2a5b580},
abstract={While most multi-object tracking methods based on tracking-by-detection use either spatial or appearance cues for associating detections or apply one cue after another, our proposed PAS tracker employs a novel similarity measure that combines position, appearance and size information jointly to make full use of object representations. We further extend the PAS tracker by introducing a filtering technique to remove false positive detections, particularly in crowded scenarios, and apply a camera motion compensation model to align track positions across frames. To provide high quality detections as input for the proposed tracker, the performance of eight state-of-the-art object detectors is compared on the VisDrone MOT dataset, on which the PAS tracker achieves state-of-the-art performance and ranks 3rd in the VisDrone2020 MOT challenge. In an ablation study, we demonstrate the effectiveness of the introduced tracking components and the impact of the employed detections on the tracking performance is analyzed in detail. © 2020, Springer Nature Switzerland AG.},
publisher={Springer Science and Business Media Deutschland GmbH},
}

@ARTICLE{Fan2020713,
author={Fan, H. and Du, D. and Wen, L. and Zhu, P. and Hu, Q. and Ling, H. and Shah, M. and Pan, J. and Schumann, A. and Dong, B. and Stadler, D. and Xu, D. and Bunyak, F. and Seetharaman, G. and Liu, G. and Haritha, V. and Hrishikesh, P.S. and Han, J. and Palaniappan, K. and Zhu, K. and Sommer, L.W. and Zhang, L. and Shine, L. and Yao, M. and Al-Shakarji, N.M. and Li, S. and Sun, T. and Sai, W. and Yu, W. and Wu, X. and Hong, X. and Wei, X. and Zhao, X. and Zhao, Y. and Gong, Y. and Yao, Y. and He, Y. and Zhao, Z. and Xie, Z. and Yang, Z. and Xu, Z. and Luo, Z. and Duan, Z.},
title={VisDrone-MOT2020: The Vision Meets Drone Multiple Object Tracking Challenge Results},
journal={Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
year={2020},
volume={12538 LNCS},
pages={713-727},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85101770013&doi=10.1007%2f978-3-030-66823-5_43&partnerID=40&md5=a7555e1e2cc6e29718ab32a2887872c6},
abstract={The Vision Meets Drone (VisDrone2020) Multiple Object Tracking (MOT) is the third annual UAV MOT tracking evaluation activity organized by the VisDrone team, in conjunction with European Conference on Computer Vision (ECCV 2020). The VisDrone-MOT2020 consists of 79 challenging video sequences, including 56 videos (∼ 24K frames) for training, 7 videos (∼ 3K frames) for validation and 17 videos (∼ 6K frames) for evaluation. All frames in these sequences are manually annotated with high-quality bounding boxes. Results of 12 participating MOT algorithms are presented and analyzed in detail. The challenging results, video sequences as well as the evaluation toolkit are made available at http://aiskyeye.com/. By holding VisDrone-MOT2020 challenge, we hope to facilitate future research and applications of MOT algorithms on drone videos. © 2020, Springer Nature Switzerland AG.},
publisher={Springer Science and Business Media Deutschland GmbH},
}

@ARTICLE{Fan2020728,
author={Fan, H. and Wen, L. and Du, D. and Zhu, P. and Hu, Q. and Ling, H. and Shah, M. and Wang, B. and Dong, B. and Yuan, D. and Wang, D. and Zhou, D. and Sun, H. and Ghanei-Yakhdan, H. and Lu, H. and Khaghani, J. and Zhou, J. and Wang, K. and Pang, L. and Zhang, L. and Cheng, L. and Lin, L. and Ding, L. and Fan, N. and Wang, P. and Zhang, P. and Ma, R. and Marvasti-Zadeh, S.M. and Kasaei, S. and Chen, S. and Lai, S. and Xu, T. and He, W. and Wu, X. and Hou, X. and Zhu, X. and Gao, Y. and Zhao, Y. and Wang, Y. and Xu, Y. and Sun, Y. and Yang, Y. and Li, Y. and Wang, Z. and He, Z. and He, Z. and Luo, Z. and Huang, Z. and Zhang, Z. and Zhang, Z. and Yi, Z.},
title={VisDrone-SOT2020: The Vision Meets Drone Single Object Tracking Challenge Results},
journal={Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
year={2020},
volume={12538 LNCS},
pages={728-749},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85101750735&doi=10.1007%2f978-3-030-66823-5_44&partnerID=40&md5=77caf265c4fe0389ee2de72505cdaed9},
abstract={The Vision Meets Drone (VisDrone2020) Single Object Tracking is the third annual UAV tracking evaluation activity organized by the VisDrone team, in conjunction with European Conference on Computer Vision (ECCV 2020). The VisDrone-SOT2020 Challenge presents and discusses the results of 13 participating algorithms in detail. By using ensemble of different trackers trained on several large-scale datasets, the top performer in VisDrone-SOT2020 achieves better results than the counterparts in VisDrone-SOT2018 and VisDrone-SOT2019. The challenging results, collected videos as well as the valuation toolkit are made available at http://aiskyeye.com/. By holding VisDrone-SOT2020 challenge, we hope to provide the community a dedicated platform for developing and evaluating drone-based tracking approaches. © 2020, Springer Nature Switzerland AG.},
publisher={Springer Science and Business Media Deutschland GmbH},
}

@ARTICLE{Chen2020489,
author={Chen, P.-Y. and Chen, G.-Y.},
title={The design of a tld and fuzzy-pid controller based on the autonomous tracking system for quadrotor drones},
journal={Intelligent Automation and Soft Computing},
year={2020},
volume={26},
number={3},
pages={489-500},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85090527761&doi=10.32604%2fiasc.2020.013925&partnerID=40&md5=be9fe3dbf6482e77f5f573610d020cba},
abstract={The objective of this paper is to design a new Quadrotor Autonomous Following System, and the main three contents are as follows: Object tracking, quadrotor attitude determination and the controller. The image tracking portion performs object detection and keeps tracking by way of the Tracking-Learning-Detection (TLD), and gets the information of the target motion estimation positions. The attitude determination of the Quadrotor has adopted the Inertial Navigation System and sensors of the accelerometer, gyroscope and electronic compass, etc. for retrieving the information. The Kalman filter is also utilized for estimating the current values in order to reduce external interference, improve the accuracy, and obtain the current posture of the Quadrotor. As for the control method, the mathematical modeling on the Quadrotor is performed first so that the Quadrotor can obtain the correct posture through the three-axis compensations, and then the fuzzy-PID controller may obtain the three-axis following angles for output to execute the commands and track the users. Finally the feasibility of this method is verified by using the flying software simulation and tangible flight experiments. © 2020, Tech Science Press. All rights reserved.},
publisher={Tech Science Press},
}

@CONFERENCE{Guerlin2020,
author={Guerlin, L. and Pannetier, B. and Rombaut, M. and Derome, M.},
title={Study on group target tracking to counter swarms of drones},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2020},
volume={11423},
art_number={1142304},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85088130774&doi=10.1117%2f12.2558119&partnerID=40&md5=4489c70229870130796c41ff741f2308},
abstract={This article focuses on Group Target Tracking (GTT) to counter swarms of drones using Random Finite Sets (RFSs) and Random Matrix (RM) approaches. Tracking swarms of drones is analog to tracking extended targets that are characterized by their continuously evolving shape and composition. Extended target tracking for groups of targets finds various applications in the literature because detecting and tracking each individual target of a group is computationally demanding and unnecessary if the group itself can be modeled. Elliptic shapes offers a suitable representation for most groups, and their inference is quite inexpensive with the random matrix approach. Indeed, they are efficient when coupled with random finite sets based filters, which represents the current state of the art for Bayesian multi-target tracking. In this work, a practical implementation of a labeled Poisson/Multi-Bernoulli filter using random matrices for group target tracking is proposed. This study compares several random matrix prediction and update algorithms with and without random finite sets based filters on several dataset. © 2020 SPIE.},
publisher={SPIE},
}

@CONFERENCE{Yamada2020796,
author={Yamada, T. and Itoyama, K. and Nishida, K. and Nakadai, K.},
title={Sound Source Tracking by Drones with Microphone Arrays},
journal={Proceedings of the 2020 IEEE/SICE International Symposium on System Integration, SII 2020},
year={2020},
pages={796-801},
art_number={9026185},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85082598868&doi=10.1109%2fSII46433.2020.9026185&partnerID=40&md5=afa9009b63892d1eaeae335376614452},
abstract={This paper presents a method for sound source localization and tracking using drones with microphone arrays. Microphone array processing is an established technique for estimating the direction of a sound source. However, for search and rescue applications, mere sound source direction is insufficient since sound source location in terms of direction and distance is essential. Accordingly, we propose a novel method we call Multiple Triangulation and Gaussian Sum Filter Tracking (MT-GSFT). MT-GSFT obtains the sound source location by triangulation using microphone arrays attached to multiple drones. Since triangulation results differ among pairs of arrays, they are transformed into a probabilistic representation using a Gaussian mixture, then a Gaussian sum filter is applied to estimate the sound source trajectory. Numerical simulation demonstrated MT-GSFT is effective in removing outliers in sound source localization to track sound sources better than the Linear Intersection method. © 2020 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Lee202051,
author={Lee, C. and Semwal, S.K.},
title={Evaluation of RSSI as a Non-visual Target Tracking Technique for Drone Applications},
journal={Advances in Intelligent Systems and Computing},
year={2020},
volume={1129 AISC},
pages={51-59},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85081542152&doi=10.1007%2f978-3-030-39445-5_6&partnerID=40&md5=af592ba869b04a97370f1276938ed52a},
abstract={Visual tracking algorithms for drone applications is a common technique for tracking and following targets. However, partial or full occlusion can cause visual trackers to lose its target or even begin following the wrong target. To combat this challenge, non-visual tracking algorithms can be used in parallel to provide more robust tracking in environments where line-of-sight cannot be guaranteed. In this study, a non-visual tracking technique using RSSI (Received Signal Strength Indicator) is evaluated for its suitability in drone applications. The study results show a RMS error of 1.17 ft. for the RSSI technique within a 10 foot radius in outdoors environments, which is an improvement over the current reported accuracy of GPS. However, interference from multipath fading in indoors settings remains a significant challenge for the RSSI technique, and modifications to the RSSI technique to mitigate multipath fading are proposed as future work. © Springer Nature Switzerland AG 2020.},
publisher={Springer},
}

@ARTICLE{Cifuentes-García2020668,
author={Cifuentes-García, C. and González-Medina, D. and García-Varea, I.},
title={People Detection and Tracking Using an On-Board Drone Camera},
journal={Advances in Intelligent Systems and Computing},
year={2020},
volume={1093 AISC},
pages={668-680},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85079088469&doi=10.1007%2f978-3-030-36150-1_55&partnerID=40&md5=930443194ae0937a27278291839ea9cc},
abstract={The problem of people detection and tracking in unmanned ground vehicles has been studied in depth in computer vision and autonomous robotics research communities. Different well-known proposals have already been proposed to solve the problem of people detection and tracking using machine vision algorithms. However, for unmanned aerial vehicles, it is still a subject of research today. The lack of high-quality sensors and on-board cameras and the capability to process the data collected in real-time makes it difficult to achieve optimal solutions in real-time. In this work, we propose to use machine vision algorithms to process in real-time the images collected by the camera of a drone and subsequently performing the detection and tracking of people who are located in the environment. The proposal was experimentally evaluated comparing different semantic segmentation techniques. Finally, to validate the proposal, a real scenario was created and carried out, which consisted of detecting and tracking people with a drone autonomously in a controlled environment. © 2020, Springer Nature Switzerland AG.},
publisher={Springer},
}

@ARTICLE{Dogru2020392,
author={Dogru, S. and Baptista, R. and Marques, L.},
title={Tracking Drones with Drones Using Millimeter Wave Radar},
journal={Advances in Intelligent Systems and Computing},
year={2020},
volume={1093 AISC},
pages={392-402},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85079084673&doi=10.1007%2f978-3-030-36150-1_32&partnerID=40&md5=b5d7b31619169e1add30c2d34b008ae9},
abstract={The use of drones has seen a surge in the last few years with their employment in a large variety of applications. However, this popularity has also made improper drone use a threat to privacy, economy and human lives, requiring the development of methods to detect and track drones. In this work, we present and experimentally validate an airborne drone detection system that utilizes a millimeter wave radar system to detect and follow target drones. © 2020, Springer Nature Switzerland AG.},
publisher={Springer},
}

@ARTICLE{Jácome2020135,
author={Jácome, R.N. and Huertas, H.L. and Procel, P.C. and Garcés, A.G.},
title={Fuzzy Logic for Speed Control in Object Tracking Inside a Restricted Area Using a Drone},
journal={Smart Innovation, Systems and Technologies},
year={2020},
volume={152},
pages={135-145},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85068374176&doi=10.1007%2f978-981-13-9155-2_12&partnerID=40&md5=596b776b470dccef4c5b6986ec28b3c6},
abstract={This article presents the autonomous speed and positioning control for a drone using fuzzy logic to track a target within a restricted area. Classical controllers present a problem, as in general they only support one input and one output and a system model is always required. For this application, it is necessary to analyze two inputs, the position in “x” and the position in “y” of an object that will be recognized by the drone through artificial vision. The goal is to control the speed at which the drone moves according to the position of the object detected by the machine vision within a restricted area, resulting in a faster or slower movement that will improve the tracking of a moving target by delivering real-time object monitoring information to the user in order to take some action based on this information. © 2020, Springer Nature Singapore Pte Ltd.},
publisher={Springer Science and Business Media Deutschland GmbH},
}

@CONFERENCE{Sun20191863,
author={Sun, X. and Zhang, W.},
title={Implementation of Target Tracking System Based on Small Drone},
journal={Proceedings of 2019 IEEE 4th Advanced Information Technology, Electronic and Automation Control Conference, IAEAC 2019},
year={2019},
pages={1863-1866},
art_number={8997682},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85081181305&doi=10.1109%2fIAEAC47372.2019.8997682&partnerID=40&md5=4a7fd730507ef47965d555a8c076ec03},
abstract={The small drone has the advantages of low cost, fast response, convenient carrying and good maneuverability, and has broad application prospects in military, civilian, video shooting and other fields.It has a wide application prospect in military, civil, video shooting and other fields. With the development of camera technology and the development of image processing technology, computer vision technology has been increasingly applied to small drones.In this paper, small drone is taken as an applicable platform, and relevant theoretical research and comprehensive experiments are carried out around monocular vision feature point extraction and matching, UAV target tracking strategy, etc. Finally, a target tracking system is built to realize real-time face tracking. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Fujiwara20192239,
author={Fujiwara, N. and Jiang, M. and Takaki, T. and Ishii, I. and Shimasaki, K.},
title={Super-telephoto drone tracking using HFR-video-based vibration source localization},
journal={IEEE International Conference on Robotics and Biomimetics, ROBIO 2019},
year={2019},
pages={2239-2244},
art_number={8961695},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85079069150&doi=10.1109%2fROBIO49542.2019.8961695&partnerID=40&md5=822ca0ed5b5ab04da4c58c70e3f63f09},
abstract={In this paper, we propose a super-telephoto drone surveillance system that can search and track a flying drone at a 1 km distance or more within an area spanning hundreds of square meters. By constructing a mirror-drive high-speed pan-tilt control system with a super-telephoto camera lens, remote drone surveillance becomes possible owing to the acquisition of high spatial resolution images of target objects. We adopted a vibration-based drone localization algorithm that can simultaneously detect fast-rotating drone-propellers in an high-frame-rate video using a pixel-level short-time Fourier transform to achieve robust surveillance under various challenging conditions for super-telephoto video-shooting such as low luminance and heat haze. The effectiveness of the super-telephoto drone tracking system is demonstrated by conducting a drone searching and tracking experiment at a 1 km distance using an 800-mm focal length lens with a mirror-drive video-shooting system. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Unlu2019,
author={Unlu, E. and Zenou, E. and Riviere, N. and Dupouy, P.-E.},
title={Deep learning-based strategies for the detection and tracking of drones using several cameras},
journal={IPSJ Transactions on Computer Vision and Applications},
year={2019},
volume={11},
number={1},
art_number={7},
note={cited By 35},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85069679620&doi=10.1186%2fs41074-019-0059-x&partnerID=40&md5=71095e7b029b06cd5032f33c1eed5497},
abstract={Commercial Unmanned aerial vehicle (UAV) industry, which is publicly known as drone, has seen a tremendous increase in last few years, making these devices highly accessible to public. This phenomenon has immediately raised security concerns due to fact that these devices can intentionally or unintentionally cause serious hazards. In order to protect critical locations, the academia and industry have proposed several solutions in recent years. Computer vision is extensively used to detect drones autonomously compared to other proposed solutions such as RADAR, acoustics and RF signal analysis thanks to its robustness. Among these computer vision-based approaches, we see the preference of deep learning algorithms thanks to their effectiveness. In this paper, we are presenting an autonomous drone detection and tracking system which uses a static wide-angle camera and a lower-angle camera mounted on a rotating turret. In order to use memory and time efficiently, we propose a combined multi-frame deep learning detection technique, where the frame coming from the zoomed camera on the turret is overlaid on the wide-angle static camera’s frame. With this approach, we are able to build an efficient pipeline where the initial detection of small sized aerial intruders on the main image plane and their detection on the zoomed image plane is performed simultaneously, minimizing the cost of resource exhaustive detection algorithm. In addition to this, we present the integral system including tracking algorithms, deep learning classification architectures and the protocols. © 2019, The Author(s).},
publisher={Springer Berlin Heidelberg},
}

@CONFERENCE{Amador2019344,
author={Amador, J.M. and Martinez-de Dios, J.R. and Paneque, J.L. and Ollero, A.},
title={An Agile Low-cost Testbed for Multi-Drone Target Tracking},
journal={2019 International Workshop on Research, Education and Development on Unmanned Aerial Systems, RED-UAS 2019},
year={2019},
pages={344-351},
art_number={8999718},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85081257541&doi=10.1109%2fREDUAS47371.2019.8999718&partnerID=40&md5=ca26bc751da137119b0fd495333d5d04},
abstract={Most existing aerial robotics testbeds have significant set-up and maintenance costs that restrict their use. This paper presents a low-cost multi-drone testbed for agile and safe performing proof-of-concept experiments. It uses low-weight, low-size Crazyflies drones and low-cost lighthouse positioning system for drone pose estimations. Its flexible and modular ROS-based architecture can be used to easily test multi-drone perception, control and planning techniques and can easily integrate bigger drones. The presented testbed does not require a dedicated room and can be set-up in less than one hour. The paper presents the testbed and validates its operation with multi-drone target tracking experiments. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Sedunov2019,
author={Sedunov, A. and Haddad, D. and Salloum, H. and Sutin, A. and Sedunov, N. and Yakubovskiy, A.},
title={Stevens Drone Detection Acoustic System and Experiments in Acoustics UAV Tracking},
journal={2019 IEEE International Symposium on Technologies for Homeland Security, HST 2019},
year={2019},
art_number={9032916},
note={cited By 6},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85078740995&doi=10.1109%2fHST47167.2019.9032916&partnerID=40&md5=f05665e8b9991d975cae8cb3f3ec9c14},
abstract={Concerns about improper use of Unmanned Aerial Vehicles (UAVs, also unmanned aerial systems or UAS) led to the development of various methods for their detection, tracking, and classification. One of the methods is using acoustics. Advantages of passive acoustics include the low cost of acoustic systems, finding of the Direction of Arrival (DOA) and localization by simple means; and classification of UAV sounds by acoustic signature. Stevens Institute of Technology has developed and built the Drone Acoustic Detection System (DADS) that can detect, track and classify UAVs based on the propeller noise. The system consists of three or more microphone nodes. The microphones in each node are arranged in a tetrahedron with configurable size. The microphone data is transferred over WiFi in real-time to a central computer, where it is processed. The Stevens DADS system was investigated in numerous field tests together with several other directional arrays including a 16-channel two-tier cross array, the OptiNav 40-microphone phased array, and parabolic and shot gun microphones. Multirotor UAVs of different sizes were employed in testing, including DJI models Phantom 4, M600 and S1000. The test results of the different systems were compared. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Zhang2019899,
author={Zhang, H. and Lei, Z. and Wang, G. and Hwang, J.-N.},
title={Eye in the sky: Drone-based object tracking and 3D localization},
journal={MM 2019 - Proceedings of the 27th ACM International Conference on Multimedia},
year={2019},
pages={899-907},
note={cited By 10},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85074808866&doi=10.1145%2f3343031.3350933&partnerID=40&md5=5aa4c0daea02c95032678e26f9041c96},
abstract={Drones, or general UAVs, equipped with a single camera have been widely deployed to a broad range of applications, such as aerial photography, fast goods delivery and most importantly, surveillance. Despite the great progress achieved in computer vision algorithms, these algorithms are not usually optimized for dealing with images or video sequences acquired by drones, due to various challenges such as occlusion, fast camera motion and pose variation. In this paper, a drone-based multi-object tracking and 3D localization scheme is proposed based on the deep learning based object detection. We first combine a multi-object tracking method called TrackletNet Tracker (TNT) which utilizes temporal and appearance information to track detected objects located on the ground for UAV applications. Then, we are also able to localize the tracked ground objects based on the group plane estimated from the Multi-View Stereo technique. The system deployed on the drone can not only detect and track the objects in a scene, but can also localize their 3D coordinates in meters with respect to the drone camera. The experiments have proved our tracker can reliably handle most of the detected objects captured by drones and achieve favorable 3D localization performance when compared with the state-of-the-art methods. © 2019 Association for Computing Machinery.},
publisher={Association for Computing Machinery, Inc},
}

@CONFERENCE{Respall2019477,
author={Respall, V.M. and Sellami, S. and Afanasyev, I.},
title={Implementation of autonomous visual detection, tracking and landing for AR.Drone 2.0 quadcopter},
journal={Proceedings - International Conference on Developments in eSystems Engineering, DeSE},
year={2019},
volume={October-2019},
pages={477-482},
art_number={9072990},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85084410982&doi=10.1109%2fDeSE.2019.00093&partnerID=40&md5=a9d0b243da21855f8361e8f427516687},
abstract={This paper presents the design and implementation of a system where an autonomous aerial vehicle (UAV) has to detect, track and land in the vicinity of a moving Unmanned Ground Vehicle (UGV). The quadcopter needs, using camerabased data, to identify and track the UGV platform. A colorbased detection algorithm is employed to detect the UGV position and Kernelized Correlation Filters (KCF) are taken for its tracking. For suppressing the false positive cases of the detection algorithm, and to double check the presence of the UGV in an image frame, the ORB (Oriented FAST and rotated BRIEF) feature detector is used. Then the UGV position detected in the image frame is used in a PD feedback control loop in the quadcopter's controller that enables the actual tracking of the moving UGV in the horizontal plane, while another PID controller stabilizes the UAV altitude. The proposed approach was initially tested in Gazebo simulator, and then in real environment with Parrot AR.Drone 2.0 and Plato robots (as UAV and UGV correspondingly). The results show that the proposed system can detect and track the UGV in online mode without artificial markers and perform robust UAV landing. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Du2019199,
author={Du, D. and Zhu, P. and Wen, L. and Bian, X. and Ling, H. and Hu, Q. and Zheng, J. and Peng, T. and Wang, X. and Zhang, Y. and Bo, L. and Shi, H. and Zhu, R. and Han, B. and Zhang, C. and Liu, G. and Wu, H. and Wen, H. and Wang, H. and Fan, J. and Chen, J. and Gao, J. and Zhang, J. and Zhou, J. and Zhou, J. and Wang, J. and Wan, J. and Kittler, J. and Zhang, K. and Huang, K. and Yang, K. and Zhang, K. and Huang, L. and Zhou, L. and Shi, L. and DIng, L. and Wang, N. and Wang, P. and Hu, Q. and Laganière, R. and Ma, R. and Zhang, R. and Zou, S. and Zhao, S. and Li, S. and Zhu, S. and Li, S. and Ge, S. and Xuan, S. and Xu, T. and He, T. and Shi, W. and Song, W. and Hu, W. and Zhang, W. and Zhu, W. and Yu, X. and Wang, X. and Wu, X. and Li, X. and Li, X. and Yin, X. and Zhang, X. and Zhao, X. and Xue, X. and Lei, X. and Yang, X. and Gao, Y. and Zhao, Y. and Xu, Y. and Li, Y. and Wang, Y. and Yang, Y. and Yang, Y. and Li, Y. and Wang, Z. and Feng, Z. and Zhang, Z. and Yu, Z. and Duan, Z. and Sun, Z.},
title={VisDrone-SOT2019: The vision meets drone single object tracking challenge results},
journal={Proceedings - 2019 International Conference on Computer Vision Workshop, ICCVW 2019},
year={2019},
pages={199-212},
art_number={9022632},
note={cited By 8},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85082495614&doi=10.1109%2fICCVW.2019.00029&partnerID=40&md5=f2193041095171b5d5d8050960d158ad},
abstract={The Vision Meets Drone (VisDrone2019) Single Object Tracking challenge is the second annual research activity focusing on evaluating single-object tracking algorithms on drones, held in conjunction with the International Conference on Computer Vision (ICCV 2019). The VisDrone-SOT2019 Challenge goes beyond its VisDrone-SOT2018 predecessor by introducing 25 more challenging sequences for long-term tracking. We evaluate and discuss the results of 22 participating algorithms and 19 state-of-the-art trackers on the collected dataset. The challenge results are publicly available at the website: http://www.aiskyeye.com/. WeexpecttheVisDrone-SOTchallenge to boost the research in single object tracking field. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Pan2019135,
author={Pan, S. and Tong, Z. and Zhao, Y. and Zhao, Z. and Su, F. and Zhuang, B.},
title={Multi-object tracking hierarchically in visual data taken from drones},
journal={Proceedings - 2019 International Conference on Computer Vision Workshop, ICCVW 2019},
year={2019},
pages={135-143},
art_number={9022119},
note={cited By 6},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85082451115&doi=10.1109%2fICCVW.2019.00022&partnerID=40&md5=f4375b6bd13c8f2f3eb1e6a7aed3dcd8},
abstract={Visual understanding tasks on the drone platform have gained considerable attention recently due to the rapid development of drones. In this paper, we present a hierarchical multi-target tracker (HMTT) for visual data taken from drones. Our approach is specifically directed against sequences shot from drone's view with several stages hierarchically performed. The detector detects objects taken from different viewing angles and the detections are filtered to ensure the correctness. Moreover, we propose a method to locate the frames in the case of camera's fast move by two-norm of the homography matrix. Based on that, performance on Multi-Object Tracking is improved with the involvement of Single Object Tracking and a re-identification subnet. Our method participated in the Multi-Object Tracking Challenge (Task 4) of VisDrone2019 benchmark and achieved state-of-the-art performance. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Ardo201946,
author={Ardo, H. and Nilsson, M.},
title={Multi target tracking from drones by learning from generalized graph differences},
journal={Proceedings - 2019 International Conference on Computer Vision Workshop, ICCVW 2019},
year={2019},
pages={46-54},
art_number={9022400},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85082448559&doi=10.1109%2fICCVW.2019.00012&partnerID=40&md5=615e0b8638380511c8fc4843ba83c775},
abstract={Formulating the multi object tracking problem as a network flow optimization problem is a popular choice. The weights of such network flow problem can be learnt efficiently from training data using a recently introduced concept called Generalized Graph Differences (GGD). This allows a general tracker implementation to be specialized to drone videos by training it on the VisDrone dataset. Two modifications to the original GGD is introduced in this paper and a result with an average precision of 23.09 on the test set of VisDrone 2019 was achieved. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Wen2019189,
author={Wen, L. and Zhu, P. and Du, D. and Bian, X. and Ling, H. and Hu, Q. and Zheng, J. and Peng, T. and Wang, X. and Zhang, Y. and Bo, L. and Shi, H. and Zhu, R. and Jadhav, A. and Dong, B. and Lall, B. and Liu, C. and Zhang, C. and Wang, D. and Ni, F. and Bunyak, F. and Wang, G. and Liu, G. and Seetharaman, G. and Li, G. and Ardö, H. and Zhang, H. and Yu, H. and Lu, H. and Hwang, J.-N. and Mu, J. and Hu, J. and Palaniappan, K. and Chen, L. and DIng, L. and Lauer, M. and Nilsson, M. and Al-Shakarji, N.M. and Mukherjee, P. and Huang, Q. and Laganière, R. and Chen, S. and Pan, S. and Kaushik, V. and Shi, W. and Tian, W. and Li, W. and Chen, X. and Zhang, X. and Zhang, Y. and Zhao, Y. and Wang, Y. and Song, Y. and Yao, Y. and Chen, Z. and Xu, Z. and Xiao, Z. and Tong, Z. and Luo, Z. and Sun, Z.},
title={VisDrone-MOT2019: The vision meets drone multiple object tracking challenge results},
journal={Proceedings - 2019 International Conference on Computer Vision Workshop, ICCVW 2019},
year={2019},
pages={189-198},
art_number={9022306},
note={cited By 8},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85082437423&doi=10.1109%2fICCVW.2019.00028&partnerID=40&md5=5a657822e678b8b695ac6dffef322581},
abstract={The Vision Meets Drone Multiple Object Tracking (MOT) Challenge 2019 is the second annual activity focusing on evaluating multi-object tracking algorithms on drones, held in conjunction with the 17-th International Conference on Computer Vision (ICCV 2019). Results of 12 submitted MOT algorithms on the collected drone-based dataset are presented. Meanwhile, we also report the results of 6 state-of-the-art MOT algorithms, and provide a comprehensive analysis and discussion of the results. The results of all submissions are publicly available at the website: http://www.aiskyeye.com/. The challenge results show that MOT on drones is far from being solved. We believe the challenge can largely boost the research and development in MOT on drone platforms. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Kim20191627,
author={Kim, T. and Wee, I. and Shim, D.H.},
title={Occlusion Robust Object Detection and Tracking on a Real-time Drone},
journal={International Conference on Control, Automation and Systems},
year={2019},
volume={2019-October},
pages={1627-1631},
art_number={8971546},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85079104572&doi=10.23919%2fICCAS47443.2019.8971546&partnerID=40&md5=842d8f202273121a35d63bb16e9d53fb},
abstract={This paper presents a vision-based tracking algorithm for real-time drone. This method consists of cnn based object detection and object tracking using the result of detector. The detector outputs a class label and a binary mask of the object. The tracker uses this binary mask to extract object features from the background. We use this information to estimate the accurate target location and tracking the target to each frame considering the similarity between target and each detected object feature vector. We validate this method using real-time drone. © 2019 Institute of Control, Robotics and Systems - ICROS.},
publisher={IEEE Computer Society},
}

@CONFERENCE{Stallone2019,
author={Stallone, R. and Massardo, M. and Montanari, G. and Buono, D. and Madia, D. and Merko, R.},
title={Omega360 an innovative radar for detection and tracking of small drones},
journal={2019 International Radar Conference, RADAR 2019},
year={2019},
art_number={9078999},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85084949640&doi=10.1109%2fRADAR41533.2019.171273&partnerID=40&md5=398ee70074fec4a4789fb4508424c41d},
abstract={The steadily increasing number of small unmanned aerial vehicles (UAV) commonly known as drones implies the need to detect and track them in order to avoid dangerous impacts with other flying objects and to prevent threats. A promising way for detecting, tracking and recognizing drones is to employ radar systems with a long integration time. This paper describes the performance results obtained with an innovative 2D ubiquitous radar, called Omega360, in an Outdoor Test Range sited in San Benedetto del Tronto (Italy). The ubiquity characteristic of Omega360 is obtained with a circular antenna capable of simultaneous staring beams, created by means of Digital Beam Forming, that allow to cover continuously 360 degrees in azimuth. The paper shows how the prolonged time on target provided by the staring beams permits long integration time and then the ability to detect low observability targets such as small drones in a natural environment. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Cetinkaya2019274,
author={Cetinkaya, O.T. and Sandal, S. and Bostanci, E. and Guzel, M.S. and Osmanoglu, M. and Kanwal, N.},
title={A Fuzzy Rule Based Visual Human Tracking System for Drones},
journal={UBMK 2019 - Proceedings, 4th International Conference on Computer Science and Engineering},
year={2019},
pages={274-279},
art_number={8907104},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85076208192&doi=10.1109%2fUBMK.2019.8907104&partnerID=40&md5=7d90bfb19fcda6bef5b700ab7f3fa4d2},
abstract={Drone sales are on the rise with each passing year and more and more people are embracing the idea of owning these devices. These unmanned aerial vehicles are now finding more practical and innovative solutions about daily problems. And also, body detection and face recognition tasks are becoming a new trend in the security authentication systems. In the light of these facts, a real time tracker algorithm is developed to track a specified human face with DJI Phantom 3 drone. After recognizing the human face, his body is detected and it is tracked. In order to improve the tracking accuracy in outdoor environments a Kalman Filter is used. When the drone misses the target, the Filter will track him for a certain time. After that a Fuzzy Logic algorithm is used to maneuver the drone towards to the human in real time. Results show that, the developed tracking system can be used to detect a human for all of the programmable drones. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Baggenstoss2019,
author={Baggenstoss, P.M. and Springer, M. and Oispuu, M. and Kurth, F.},
title={Efficient phase-based acoustic tracking of drones using a microphone array},
journal={European Signal Processing Conference},
year={2019},
volume={2019-September},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85075607680&doi=10.23919%2fEUSIPCO.2019.8902972&partnerID=40&md5=d4b581d8748faa1b3bd363cffe087b3c},
abstract={An efficient phase-based acoustic detection and tracking algorithm for drones is presented. The algorithm separately tracks the time difference of arrival (TDOA) of the incoming signal with respect to microphone pairs based on the phase in the discrete Fourier transform (DFT) bins. The direction of arrival (DOA) of the drone is determined by forming a solution curve corresponding to each TDOA, then clustering the curve intersections. The algorithm avoids the computationally expensive grid-search over DOA, so is significantly more efficient than beamforming. The proposed algorithm and the maximum likelihood (ML) processor (beamformer) are compared in simulated and real data scenarios. Using simulated data, the ML estimator is shown to agree with the Cramér-Rao lower bound (CRLB) and the proposed algorithm is shown to approach the performance of ML at higher SNR. In real data scenarios, the phase-based algorithm implemented with simple alpha-beta TDOA trackers consistently tracked the target through difficult maneuvers at short and long range, showing no degradation with respect to the beamformer. Other potential advantages include robustness against interference and ability to create phase-based spectrograms for classification. © 2019 IEEE},
publisher={European Signal Processing Conference, EUSIPCO},
}

@CONFERENCE{Park2019,
author={Park, J.-Y. and Kim, S.-T. and Lee, J.-K. and Ham, J.-W. and Oh, K.-Y.},
title={Automatic Inspection Drone with Deep Learning-based Auto-tracking Camera Gimbal to Detect Defects in Power Lines},
journal={ACM International Conference Proceeding Series},
year={2019},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85117539747&doi=10.1145%2f3387168.3387176&partnerID=40&md5=ca42eb033cc08f67e64d668dc9c69b80},
abstract={The traditional drone inspection performed by human operators is unsuited for the purpose of inspecting power transmission lines, because steel towers and their spans are too high and wide to be inspected with a 250 m line of sight. For this reason, the KEPCO Research Institute developed a new inspection drone system that can automatically fly a predetermined flight path based on the GPS coordinates of steel towers, filming a video of power transmission lines with a high definition camera and a thermal imaging camera. In this system, a camera gimbal with the cameras was still controlled by a human operator from a long distance away. When the drone approached close to a steel tower, however, the camera gimbal was often unable to be controlled and real-time video transmission for the gimbal operator was sometimes interrupted due to radio-frequency interference from steel structure and energized power conductors. To solve such a control problem in the field, we also developed an auto-tracking camera gimbal that can automatically track and photograph power facilities on the basis of Deep Learning. With the automatic gimbal, the entire inspection process can be fully automated. The effectiveness of the developed overall system was confirmed through field tests. © 2019 ACM.},
publisher={Association for Computing Machinery},
}

@CONFERENCE{Han2019414,
author={Han, X. and Wang, C. and Li, Y. and Wu, X.},
title={A trajectory optimization algorithm for drone target localization and tracking},
journal={2019 IEEE International Conference on Real-Time Computing and Robotics, RCAR 2019},
year={2019},
volume={2019-August},
pages={414-419},
art_number={9043968},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85089142027&doi=10.1109%2fRCAR47638.2019.9043968&partnerID=40&md5=f5571a5a42491340df72d6c0206b8fbd},
abstract={Accurate positioning is the premise for the drone to successfully capture the target, this paper proposes a solution to the positioning failure caused by the relatively severe jitter of the drone and the target. In this paper, the Improved Kernel Correlation Filter (KCF) is used for target tracking, and the improved Kalman filter is used to smooth the input signal in real time, which reduces the continuous jitter of the drone. The advantage of this approach is that it will not cause misjudgment from the deviation where the measured value is too large. Further, the hysteresis is also significantly improved. The experimental works are carried out on a M100 UAV to verify the improved KCF and the improved Kalman algorithm, respectively. The results showed the effectiveness of the proposed approach. © 2018 IEEE},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Qiantian2019143,
author={Qiantian, Z. and Yonghua, F. and Pengpeng, Y.},
title={Climbing Trajectory Tracking Control of Unmanned Drone based on Total Energy Principle},
journal={2019 IEEE International Conference on Power, Intelligent Computing and Systems, ICPICS 2019},
year={2019},
pages={143-146},
art_number={8942408},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85077961928&doi=10.1109%2fICPICS47731.2019.8942408&partnerID=40&md5=c9b9d1f6fafa5158bb49d489c4b0b3c9},
abstract={In order to make the unmanned drone with energy limitation under the biasing condition still climb to the cruising altitude, a new height controller was designed inspired by the total energy control theory, and the influence of the speed deviation was introduced to adjust the elevator for the total energy distribution, so as to solve the coupling problem between longitudinal trajectory control and velocity control. Taking a certain type of target machine as the object, the simulation is carried out under two kinds of extreme biasing conditions. By comparing the simulation results of the traditional and improved control structure, it shows that the new controller is effective in practical engineering applications. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Vayssade2019767,
author={Vayssade, J.-A. and Arquet, R. and Bonneau, M.},
title={Automatic activity tracking of goats using drone camera},
journal={Computers and Electronics in Agriculture},
year={2019},
volume={162},
pages={767-772},
note={cited By 19},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85065736985&doi=10.1016%2fj.compag.2019.05.021&partnerID=40&md5=275aa1cd756088dfbb7f2f37023c5afd},
abstract={Monitoring the position of animals in the outdoors can provide useful information in ecology and in agriculture. A common method is to use active sensors, such as GPS, to record their positions at constant intervals of time. But using active sensors can rapidly become expensive when several animals have to be monitored at the same time. Another method is to use a passive sensor to monitor the entire flock of animals. In this article, we propose a method to process images taken by a commercial drone in order to automate the tracking of animal activities. We developed a method that automatically detects goats from the images and tracks their activity using a combination of thresholding and supervised classification methods. We tested our method on 571 drone images taken over 11 days and found a sensitivity of 74% for animal detection and 78.3% for activity detection. © 2019 Elsevier B.V.},
publisher={Elsevier B.V.},
}

@CONFERENCE{Fernandes2019,
author={Fernandes, A. and Baptista, M. and Fernandes, L. and Chaves, P.},
title={Drone, Aircraft and Bird Identification in Video Images Using Object Tracking and Residual Neural Networks},
journal={Proceedings of the 11th International Conference on Electronics, Computers and Artificial Intelligence, ECAI 2019},
year={2019},
art_number={9042167},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85079516058&doi=10.1109%2fECAI46879.2019.9042167&partnerID=40&md5=bc25f7fbed5b9428e79f5664d9ed07d5},
abstract={As maritime smuggling is being combatted more effectively, the criminal 'modus operandi' consists more frequently of using small aircraft and drones for drug transport. To address this issue, we report our efforts to develop a system capable of accurately tracking suspicious flying objects and identifying them on video streams. Our solution consists in coupling classical computer vision with deep learning to perform tracking and object detection. A discrete Kalman filter is used to predict the location of each object being tracked while the Hungarian algorithm is used to match objects between successive frames. Whenever a potential target is considered suspicious the input images are zoomed and fed into a deep learning pipeline that separates images into the classes aircraft, drones, birds or clouds. A literature survey indicates that this problem with important applications is yet to be fully explored. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Caillouet201935,
author={Caillouet, C. and Giroire, F. and Razafindralambo, T.},
title={Efficient data collection and tracking with flying drones},
journal={Ad Hoc Networks},
year={2019},
volume={89},
pages={35-46},
note={cited By 18},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85062658387&doi=10.1016%2fj.adhoc.2019.01.011&partnerID=40&md5=9fc2fee8aaed790986f81003495314db},
abstract={Data collection is an important mechanism for wireless sensor networks to be viable. This paper addresses the Aerial Data Collection Problem (ADCP) from a set of mobile wireless sensors located on the ground, using a fleet of flying devices. The objective is i) to deploy a set of Unmanned Aerial Vehicles (UAVs) in a 3D space to cover and collect data from all the mobile wireless sensors at each time step through a ground-to-air communication, ii) to send these data to a central base station using multi-hop wireless air-to-air communications through the network of UAVs, iii) while minimizing the total deployment cost (communication and deployment) over time. The Aerial Data Collection Problem (ADCP) is a complex time and space coverage, and connectivity problem. We first present a mixed-integer linear program solving ADCP optimally for small instances. Then, we develop a second model solved by column generation for larger instances, with optimal or heuristic pricing programs. Results show that our approach provides very accurate solutions minimizing the data collection cost. Moreover, only a very small number of columns are generated throughout the resolution process, showing the efficiency of our approach. © 2019 Elsevier B.V.},
publisher={Elsevier B.V.},
}

@CONFERENCE{Rusdi2019,
author={Rusdi, J.F. and Salam, S. and Abu, N.A. and Sahib, S. and Naseer, M. and Abdullah, A.A.},
title={Drone Tracking Modelling Ontology for Tourist Behavior},
journal={Journal of Physics: Conference Series},
year={2019},
volume={1201},
number={1},
art_number={012032},
note={cited By 9},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85067679023&doi=10.1088%2f1742-6596%2f1201%2f1%2f012032&partnerID=40&md5=d2da8a210c0449ee336a23a880d83f77},
abstract={Availability of internet access is one of the needs for tourists when traveling. Unfortunately, the availability of access is quite limited when in a tourist destination, usually Wi-Fi also generally uses a closed system that cannot be accessed by just anyone, except those who get access keys only. This paper provides a solution for the model of internet access for tourists provided by Tourism Service Providers, by utilizing drone technology as an access point. In addition, this model also provides services to track the position of tourists who spread and facilities for communication between tourists, especially for certain conditions, such as the occurrence of saturation for tourists while in one of the tourist destinations. © Published under licence by IOP Publishing Ltd.},
publisher={Institute of Physics Publishing},
}

@CONFERENCE{Dressel20191905,
author={Dressel, L. and Kochenderfer, M.J.},
title={Hunting drones with other drones: Tracking a moving radio target},
journal={Proceedings - IEEE International Conference on Robotics and Automation},
year={2019},
volume={2019-May},
pages={1905-1912},
art_number={8794243},
note={cited By 11},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85071471386&doi=10.1109%2fICRA.2019.8794243&partnerID=40&md5=931f23a5915d0916c4e6ebca0e9e79f9},
abstract={Unauthorized drone flights near aircraft, airports, and emergency operations compromise the safety of passengers and bystanders. A detection system that can quickly find and track drones could help mitigate the risk of unauthorized drone flights. In this work, we show how a consumer drone outfitted with antennas and commodity radios can autonomously localize another drone by its telemetry radio emissions. We show how a non-myopic planner improves tracking performance over traditionally used greedy, one-step planners. Improved tracking is validated with simulations and the system is demonstrated with real drones in flight tests. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Moolan-Feroze20197713,
author={Moolan-Feroze, O. and Karachalios, K. and Nikolaidis, D.N. and Calway, A.},
title={Improving drone localisation around wind turbines using monocular model-based tracking},
journal={Proceedings - IEEE International Conference on Robotics and Automation},
year={2019},
volume={2019-May},
pages={7713-7719},
art_number={8794156},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85071469999&doi=10.1109%2fICRA.2019.8794156&partnerID=40&md5=020ef862b00ba64a4615d75ec256bdfb},
abstract={We present a novel method of integrating image-based measurements into a drone navigation system for the automated inspection of wind turbines. We take a model-based tracking approach, where a 3D skeleton representation of the turbine is matched to the image data. Matching is based on comparing the projection of the representation to that inferred from images using a convolutional neural network. This enables us to find image correspondences using a generic turbine model that can be applied to a wide range of turbine shapes and sizes. To estimate 3D pose of the drone, we fuse the network output with GPS and IMU measurements using a pose graph optimiser. Results illustrate that the use of the image measurements significantly improves the accuracy of the localisation over that obtained using GPS and IMU alone. © 2019 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Thai2019,
author={Thai, V.-P. and Zhong, W. and Pham, T. and Alam, S. and Duong, V.},
title={Detection, tracking and classification of aircraft and drones in digital towers using machine learning on motion patterns},
journal={Integrated Communications, Navigation and Surveillance Conference, ICNS},
year={2019},
volume={2019-April},
art_number={8735238},
note={cited By 13},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85068036283&doi=10.1109%2fICNSURV.2019.8735238&partnerID=40&md5=df6734f1e61d40165a06cd041bee4710},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Nguyen20194563,
author={Nguyen, H.D. and Na, I.S. and Kim, S.H. and Lee, G.S. and Yang, H.J. and Choi, J.H.},
title={Multiple human tracking in drone image},
journal={Multimedia Tools and Applications},
year={2019},
volume={78},
number={4},
pages={4563-4577},
note={cited By 7},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85047391409&doi=10.1007%2fs11042-018-6141-z&partnerID=40&md5=2ddc275d7551b0a1940181508c1c24be},
abstract={Object tracking, especially human tracking is one of the challenging research problems in computer vision. Although the performance has gained some positive changes recently, there is still room for improvement. In this paper, we introduce an approach for human detection and tracking using Convolution Neural Network (CNN) and Hungarian Algorithm (HA). A CNN is used to localize multiple human beings from frame to frame in a video stream. This deep CNN is known as Faster R-CNN which achieved the state of the art performance in object detection problem. In the tracking process, we solve the data association problem in visual tracking using HA. A detected person will be assigned to a tracklet based on the data distribution in the video frame. The experimental results show that our system can deal with the videos captured from different scenarios in near real-time. © 2018, Springer Science+Business Media, LLC, part of Springer Nature.},
publisher={Springer New York LLC},
}

@CONFERENCE{Yazid2019146,
author={Yazid, E. and Garrat, M. and Santoso, F.},
title={Optimal PD Tracking Control of a Quadcopter Drone Using Adaptive PSO Algorithm},
journal={2018 International Conference on Computer, Control, Informatics and its Applications: Recent Challenges in Machine Learning for Computing Applications, IC3INA 2018 - Proceeding},
year={2019},
pages={146-151},
art_number={8629504},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85062840716&doi=10.1109%2fIC3INA.2018.8629504&partnerID=40&md5=c7488666b1cdb5be1377014ad0d24c91},
abstract={Trajectory tracking control for quadcopter drone is a challenging work since the system is multi-input multi-output system, highly non-linear rigid body dynamics and severe cross-coupling. This paper copes that challenges by proposing the adaptive particle swarm optimization (APSO) to optimize the gains of proportional-derivative (PD) controller. The effectiveness of the proposed control algorithm is tested under constant and varying step functions as well as sine function. PSO-based optimal PD and Ziegler-Nichols (ZN)-based optimal PD controllers are taken as benchmarks. The results show that the APSO-PD controller produces shorter settling time with no overshoots than the benchmarks under the predefined trajectories. © 2018 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Unlu2019,
author={Unlu, E. and Zenou, E. and Riviere, N. and Dupouy, P.-E.},
title={An autonomous drone surveillance and tracking architecture},
journal={IS and T International Symposium on Electronic Imaging Science and Technology},
year={2019},
volume={2019},
number={15},
art_number={AVM-035},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85078066430&doi=10.2352%2fISSN.2470-1173.2019.15.AVM-035&partnerID=40&md5=f25b40abb78f2370289a12084f6b93f2},
abstract={In this work, we present a computer vision and machine learning backed autonomous drone surveillance system, in order to protect critical locations. The system is composed of a wide angle, high resolution daylight camera and a relatively narrow angle thermal camera mounted on a rotating turret. The wide angle daylight camera allows the detection of flying intruders, as small as 20 pixels with a very low false alarm rate. The primary detection is based on YOLO convolutional neural network (CNN) rather than conventional background subtraction algorithms due its low false alarm rate performance. At the same time, the tracked flying objects are tracked by the rotating turret and classified by the narrow angle, zoomed thermal camera, where classification algorithm is also based on CNNs. The training of the algorithms is performed by artificial and augmented datasets due to scarcity of infrared videos of drones. © 2019, Society for Imaging Science and Technology},
publisher={Society for Imaging Science and Technology},
}

@CONFERENCE{Dackiw2019360,
author={Dackiw, J.-N.A. and Foltman, A. and Garivani, S. and Kaseman, K. and Sollazzo, A.},
title={Cyber-physical UAV Navigation and Operation Drone Localization and Accuracy Validation through Onboard Odometry and External Motion Tracking Comparison},
journal={Ubiquity and Autonomy - Paper Proceedings of the 39th Annual Conference of the Association for Computer Aided Design in Architecture, ACADIA 2019},
year={2019},
pages={360-367},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85085727829&partnerID=40&md5=78c5cf74a709ebc142782838e7e8aa43},
abstract={The purpose of this paper is to present a work in progress pertaining to drone pose estimation and flight calibration. This paper intends to underline the increasing importance of determining alternative path planning instruments through accurate localization for Unmanned Aerial Vehicles (UAVs) with the purpose of achieving complex flight operations for the emerging applications of autonomous robotics in surveying, design, fabrication, and on-site operations. This research is based on the implementation of novel technologies such as Augmented Reality (AR), Robot Operating System (ROS), and computational approaches to define a drone calibration methodology, leveraging existing methods for drone path planning. Drones are equipped with measurement systems to provide geo-location and time information such as onboard Global Positioning System (GPS) sensors, and Inertial Measurement Units (IMU). As stated in previous research, to increase navigation capabilities, measurements and data processing algorithms have a critical role (Daponte et al. 2015). The outcome of this work in progress showcases valuable results in calculating and assessing accurate positioning for UAVs, and developing data exchanges in transmission, reception, and tracking. © Ubiquity and Autonomy - Paper Proceedings of the 39th Annual Conference of the Association for Computer Aided Design in Architecture, ACADIA 2019. All rights reserved.},
publisher={ACADIA},
}

@CONFERENCE{Jung2019,
author={Jung, I.-J. and Ih, J.-G.},
title={Acoustic localization and tracking of the multiple drones},
journal={INTER-NOISE 2019 MADRID - 48th International Congress and Exhibition on Noise Control Engineering},
year={2019},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85084160406&partnerID=40&md5=5d12463b67127706fb9eb5946c74bc9a},
abstract={Due to the social problems in the intrusion of privacy and the collision hazard, monitoring of the drones are needed for the regulations. To enhance the identification of multiple drones flying at a specific zone simultaneously, a new localization method other than the optical or electromagnetic methods is needed. In this work, a method to use the acoustic cues of the drone is presented, and the three-dimensional acoustic intensimetry (3DAI) is employed for the localization. The 3DAI implements the compensation algorithm for the spectral bias error of the probe configured in a tetrahedron shape. The blade passing frequency and its harmonics radiated from the quadcopter drones are adopted as the acoustical cues for the detection. The test for single drone is done within an anechoic chamber to estimate the localization error in the real-time. For the multiple drones, the test is carried out for the localization by using recorded sounds of three drones having different rotor sizes. The results show that the mean azimuth and elevation angle error is less than 5° for localization of multiple drones. The localization result is fine when BPFs are distinguishable, but, for the case with spectral overlap, it bears a large error. © INTER-NOISE 2019 MADRID - 48th International Congress and Exhibition on Noise Control Engineering. All Rights Reserved.},
publisher={SOCIEDAD ESPANOLA DE ACUSTICA - Spanish Acoustical Society, SEA},
}

@ARTICLE{Liu2019362,
author={Liu, Y. and Lian, Z. and Ding, J. and Guo, T.},
title={Multiple Objects Tracking Based Vehicle Speed Analysis with Gaussian Filter from Drone Video},
journal={Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
year={2019},
volume={11935 LNCS},
pages={362-373},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85077125524&doi=10.1007%2f978-3-030-36189-1_30&partnerID=40&md5=97c060fcb3492e40af0e09d84e50a8a8},
abstract={Vehicle speed analysis based on the video is a challenging task in the field of traffic safety, which has high requirements for accuracy and computational burden. The drone’s video is taken from a top-down perspective, providing more complete view comparing to the common surveillance cameras in poles. In this paper, we introduce a Gaussian Filter to deal with the estimated speed data which are extracted by a multiple objects tracking method composed of You Only Look Once (YOLOv3) and Kalman Filter. We exploit the capability of Gaussian Filter to suppress data noise appearing in the process of tracking vehicles from drone videos, and thus use the filter to solve the case where the estimated vehicle speed is fluctuated along the ongoing direction. On the other hand, we built a vehicle dataset from the drone’s videos we mentioned above which additionally contains vehicle’s real speed information. Experimental results showed that our method is effective to improve the accuracy of vehicle speed estimated by our tracking module. It can improve Mean Squared error (MSE) accuracy 80.5% on experimental data. © 2019, Springer Nature Switzerland AG.},
publisher={Springer},
}

@CONFERENCE{Li2019194,
author={Li, S. and Durdevic, P. and Yang, Z.},
title={Optimal Tracking Control Based on Integral Reinforcement Learning for An Underactuated Drone},
journal={IFAC-PapersOnLine},
year={2019},
volume={52},
number={8},
pages={194-199},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85076256773&doi=10.1016%2fj.ifacol.2019.08.048&partnerID=40&md5=2b6ca39236c5e5235b890a85949eacf3},
abstract={A drone is desirable to perform various flying missions with different loads while always guaranteeing optimal flying performance. In this paper, an integral reinforcement learning algorithm is developed for a drone such that it can learn optimal control policy online. The drone is described by an underactuated nonlinear model and the inner-outer loop control strategy is applied for the navigation control. In the outer loop an optimal controller is designed to minimize a cost function with input saturation, and a policy iteration based integral reinforcement learning (IRL) algorithm is proposed. Critic-actor neural networks (NNs) are further applied for online implementation of the IRL algorithm. In the inner loop a quaternion based feedback attitude controller is designed to guarantee system stability. A simulation study is finally provided to demonstrate the effectiveness of the proposed IRL algorithm. © 2019, IFAC (International Federation of Automatic Control) Hosting by Elsevier Ltd. All rights reserved.},
publisher={Elsevier B.V.},
}

@ARTICLE{Lu20191941,
author={Lu, X. and Chen, Z. and Wang, L. and Li, R. and Zhai, C.},
title={RF-Drone: Multi-tag system for RF-ID enables drone tracking in GPS-denied environments},
journal={IEICE Transactions on Communications},
year={2019},
volume={E102B},
number={10},
pages={1941-1950},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85073237627&doi=10.1587%2ftranscom.2018DRP0005&partnerID=40&md5=31dd44ac148e4d3e35b397c4d49115f5},
abstract={In resent years, providing location services for mobile targets in a closed environment has been a growing interest. In order to provide good localization and tracking performance for drones in GPS-denied scenarios, this paper proposes a multi-tag radio frequency identification (RFID) system that is easy to equip and does not take up the limited resources of the drone which is not susceptible to processor performance and cost constraints compared with computer vision based approaches. The passive RFID tags, no battery equipped, have an ultra-high resolution of millimeter level. We attach multiple tags to the drone and form multiple sets of virtual antenna arrays during motion, avoiding arranging redundant antennas in applications, and calibrating the speed chain to improve tracking performance. After combining the strap-down inertial navigation system (SINS) carried by the drone, we have established a coupled integration model that can suppress the drift error of SINS with time. The experiment was designed in bi-dimensional and three-dimensional scenarios, and the integrated positioning system based on SINS/RFID was evaluated. Finally, we discussed the impact of some parameters, this innovative approach is verified in real scenarios. Copyright © 2019 The Institute of Electronics, Information and Communication Engineers},
publisher={Institute of Electronics, Information and Communication, Engineers, IEICE},
}

@ARTICLE{He20191998,
author={He, Q. and Shao, X. and Chen, W. and Li, X. and Yang, X. and Sun, T.},
title={Adaptive multi-scale tracking target algorithm through drone},
journal={IEICE Transactions on Communications},
year={2019},
volume={E102B},
number={10},
pages={1998-2005},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85073233006&doi=10.1587%2ftranscom.2018DRP0040&partnerID=40&md5=fedaa898f0de48e5c1e03651c525e870},
abstract={In order to solve the influence of scale change on target tracking using the drone, a multi-scale target tracking algorithm is proposed which based on the color feature tracking algorithm. The algorithm realized adaptive scale tracking by training position and scale correlation filters. It can first obtain the target center position of next frame by computing the maximum of the response, where the position correlation filter is learned by the least squares classifier and the dimensionality reduction for color features is analyzed by principal component analysis. The scale correlation filter is obtained by color characteristics at 33 rectangular areas which is set by the scale factor around the central location and is reduced dimensions by orthogonal triangle decomposition. Finally, the location and size of the target are updated by the maximum of the response. By testing 13 challenging video sequences taken by the drone, the results show that the algorithm has adaptability to the changes in the target scale and its robustness along with many other performance indicators are both better than the most state-of-the-art methods in illumination Variation, fast motion, motion blur and other complex situations. Copyright © 2019 The Institute of Electronics, Information and Communication Engineers.},
publisher={Institute of Electronics, Information and Communication, Engineers, IEICE},
}

@ARTICLE{Oliveira2019,
author={Oliveira, M.T.D. and Miranda, R.K. and Costa, J.P.C.L.D. and Almeida, A.L.F.D. and Sousa, R.T.D.},
title={Low cost antenna array based drone tracking device for outdoor environments},
journal={Wireless Communications and Mobile Computing},
year={2019},
volume={2019},
art_number={5437908},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85068849795&doi=10.1155%2f2019%2f5437908&partnerID=40&md5=6f7d7359d52a07c4b66bfcee838b6167},
abstract={Applications of direction of arrival (DoA) techniques have dramatically increased in various areas ranging from the traditional wireless communication systems and rescue operations to GNSS systems and drone tracking. Particularly, police forces and security companies have drawn their attention to drone tracking devices, in order to provide the safeness of citizens and of clients, respectively. In this paper, we propose a low cost antenna array based drone tracking device for outdoor environments. The proposed solution is divided into hardware and software parts. The hardware part of the proposed device is based on off-the-shelf components such as an omnidirectional antenna array, a 4-channel software defined radio (SDR) platform with carrier frequency ranging from 70 MHz to 6 GHz, a FPGA motherboard, and a laptop. The software part includes algorithms for calibration, model order selection (MOS), and DoA estimation, including specific preprocessing steps and a tensor-based estimator to increase the DoA accuracy. We evaluate the performance of our proposed low cost solution in outdoor scenarios. According to our measurement campaigns, we show that when the array is in the front fire position, i.e., with a DoA ranging from-60° to 60°, the maximum and the average DoA errors are 6° and 1,9°, respectively. © 2019 Marcos T. de Oliveira et al.},
publisher={Hindawi Limited},
}

@ARTICLE{Rohan201969575,
author={Rohan, A. and Rabah, M. and Kim, S.-H.},
title={Convolutional Neural Network-Based Real-Time Object Detection and Tracking for Parrot AR Drone 2},
journal={IEEE Access},
year={2019},
volume={7},
pages={69575-69584},
art_number={8723347},
note={cited By 30},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85067241645&doi=10.1109%2fACCESS.2019.2919332&partnerID=40&md5=89296d33f2f1efa959011e06c363d9c4},
abstract={Recent advancements in the field of Artificial Intelligence (AI) have provided an opportunity to create autonomous devices, robots, and machines characterized particularly with the ability to make decisions and perform tasks without human mediation. One of these devices, Unmanned Aerial Vehicles (UAVs) or drones are widely used to perform tasks like surveillance, search and rescue, object detection and target tracking, parcel delivery (recently started by Amazon), and many more. The sensitivity in performing said tasks demands that drones must be efficient and reliable. For this, in this paper, an approach to detect and track the target object, moving or still, for a drone is presented. The Parrot AR Drone 2 is used for this application. Convolutional Neural Network (CNN) is used for object detection and target tracking. The object detection results show that CNN detects and classifies object with a high level of accuracy (98%). For real-time tracking, the tracking algorithm responds faster than conventionally used approaches, efficiently tracking the detected object without losing it from sight. The calculations based on several iterations exhibit that the efficiency achieved for target tracking is 96.5%. © 2013 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Zhu2019496,
author={Zhu, P. and Wen, L. and Du, D. and Bian, X. and Ling, H. and Hu, Q. and Wu, H. and Nie, Q. and Cheng, H. and Liu, C. and Liu, X. and Ma, W. and Wang, L. and Schumann, A. and Wang, D. and Ortego, D. and Luna, E. and Michail, E. and Bochinski, E. and Ni, F. and Bunyak, F. and Zhang, G. and Seetharaman, G. and Li, G. and Yu, H. and Kompatsiaris, I. and Zhao, J. and Gao, J. and Martínez, J.M. and San Miguel, J.C. and Palaniappan, K. and Avgerinakis, K. and Sommer, L. and Lauer, M. and Liu, M. and Al-Shakarji, N.M. and Acatay, O. and Giannakeris, P. and Zhao, Q. and Ma, Q. and Huang, Q. and Vrochidis, S. and Sikora, T. and Senst, T. and Song, W. and Tian, W. and Zhang, W. and Zhao, Y. and Bai, Y. and Wu, Y. and Wang, Y. and Li, Y. and Pi, Z. and Ma, Z.},
title={VisDrone-VDT2018: The vision meets drone video detection and tracking challenge results},
journal={Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
year={2019},
volume={11133 LNCS},
pages={496-518},
note={cited By 15},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85061726485&doi=10.1007%2f978-3-030-11021-5_29&partnerID=40&md5=5c450a77ce7f62dd0683f1fb7b7822ed},
abstract={Drones equipped with cameras have been fast deployed to a wide range of applications, such as agriculture, aerial photography, fast delivery, and surveillance. As the core steps in those applications, video object detection and tracking attracts much research effort in recent years. However, the current video object detection and tracking algorithms are not usually optimal for dealing with video sequences captured by drones, due to various challenges, such as viewpoint change and scales. To promote and track the development of the detection and tracking algorithms with drones, we organized the Vision Meets Drone Video Detection and Tracking (VisDrone-VDT2018) challenge, which is a subtrack of the Vision Meets Drone 2018 challenge workshop in conjunctiohe 15th European Conference on Computer Vision (ECCV 2018). Specifically, this workshop challenge consists of two tasks, (1) video object detection, and (2) multi-object tracking. We present a large-scale video object detection and tracking dataset, which consists of 79 video clips with about 1.5 million annotated bounding boxes in 33, 366 frames. We also provide rich annotations, including object categories, occlusion, and truncation ratios for better data usage. Being the largest such dataset ever published, the challenge enables extensive evaluation, investigation and tracking the progress of object detection and tracking algorithms on the drone platform. We present the evaluation protocol of the VisDrone-VDT2018 challenge and the results of the algorithms on the benchmark dataset, which are publicly available on the challenge website: http://www.aiskyeye.com/. We hope the challenge largely boost the research and development in related fields. © Springer Nature Switzerland AG 2019.},
publisher={Springer Verlag},
}

@ARTICLE{Wen2019469,
author={Wen, L. and Zhu, P. and Du, D. and Bian, X. and Ling, H. and Hu, Q. and Liu, C. and Cheng, H. and Liu, X. and Ma, W. and Nie, Q. and Wu, H. and Wang, L. and Perera, A.G. and Zhang, B. and Heo, B. and Liu, C. and Li, D. and Michail, E. and Chen, H. and Liu, H. and Li, H. and Kompatsiaris, I. and Cheng, J. and Fan, J. and Zhang, J. and Choi, J.Y. and Li, J. and Yang, J. and Choi, J. and Zhao, J. and Han, J. and Zhang, K. and Duan, K. and Song, K. and Avgerinakis, K. and Lee, K. and Ding, L. and Lauer, M. and Giannakeris, P. and Zhang, P. and Wang, Q. and Xu, Q. and Huang, Q. and Liu, Q. and Laganière, R. and Zhang, R. and Yun, S. and Zhu, S. and Wu, S. and Vrochidis, S. and Tian, W. and Zhang, W. and Chen, W. and Hu, W. and Wang, W. and Zhang, W. and Ding, W. and He, X. and Li, X. and Zhang, X. and Luo, X. and Hu, X. and Meng, Y. and Kuai, Y. and Zhao, Y. and Li, Y. and Yang, Y. and Zhang, Y. and Wang, Y. and Qi, Y. and Deng, Z. and He, Z.},
title={VisDrone-SOT2018: The vision meets drone single-object tracking challenge results},
journal={Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
year={2019},
volume={11133 LNCS},
pages={469-495},
note={cited By 9},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85061699928&doi=10.1007%2f978-3-030-11021-5_28&partnerID=40&md5=ff81d7b52a8e8617fd119f09ba411029},
abstract={Single-object tracking, also known as visual tracking, on the drone platform attracts much attention recently with various applications in computer vision, such as filming and surveillance. However, the lack of commonly accepted annotated datasets and standard evaluation platform prevent the developments of algorithms. To address this issue, the Vision Meets Drone Single-Object Tracking (VisDrone-SOT2018) Challenge workshop was organized in conjunction with the 15th European Conference on Computer Vision (ECCV 2018) to track and advance the technologies in such field. Specifically, we collect a dataset, including 132 video sequences divided into three non-overlapping sets, i.e., training (86 sequences with 69, 941 frames), validation (11 sequences with 7,046 frames), and testing (35 sequences with 29, 367 frames) sets. We provide fully annotated bounding boxes of the targets as well as several useful attributes, e.g., occlusion, background clutter, and camera motion. The tracking targets in these sequences include pedestrians, cars, buses, and animals. The dataset is extremely challenging due to various factors, such as occlusion, large scale, pose variation, and fast motion. We present the evaluation protocol of the VisDrone-SOT2018 challenge and the results of a comparison of 22 trackers on the benchmark dataset, which are publicly available on the challenge website: http://www.aiskyeye.com/. We hope this challenge largely boosts the research and development in single object tracking on drone platforms. © Springer Nature Switzerland AG 2019.},
publisher={Springer Verlag},
}

@CONFERENCE{Wang20182511,
author={Wang, L. and Sanchez-Matilla, R. and Cavallaro, A.},
title={Tracking a moving sound source from a multi-rotor drone},
journal={IEEE International Conference on Intelligent Robots and Systems},
year={2018},
pages={2511-2516},
art_number={8594483},
note={cited By 11},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85063013801&doi=10.1109%2fIROS.2018.8594483&partnerID=40&md5=3a2de526d0fe5e689aa14cd8774a6dc6},
abstract={We propose a method to track from a multi-rotor drone a moving source, such as a human speaker or an emergency whistle, whose sound is mixed with the strong ego-noise generated by rotating motors and propellers. The proposed method is independent of the specific drone and does not need pre-training nor reference signals. We first employ a time-frequency spatial filter to estimate, on short audio segments, the direction of arrival of the moving source and then we track these noisy estimations with a particle filter. We quantitatively evaluate the results using a ground-truth trajectory of the sound source obtained with an on-board camera and compare the performance of the proposed method with baseline solutions. © 2018 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Raoult20181,
author={Raoult, V. and Tosetto, L. and Williamson, J.E.},
title={Drone-based high-resolution tracking of aquatic vertebrates},
journal={Drones},
year={2018},
volume={2},
number={4},
pages={1-14},
art_number={37},
note={cited By 31},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85063291480&doi=10.3390%2fdrones2040037&partnerID=40&md5=cd80a914f1b50692cafa5f0d1b847a06},
abstract={Determining the small-scale movement patterns of marine vertebrates usually requires invasive active acoustic tagging or in-water monitoring, with the inherent behavioural impacts of those techniques. In addition, these techniques rarely allow direct continuous behavioural assessments or the recording of environmental interactions, especially for highly mobile species. Here, we trial a novel method of assessing small-scale movement patterns of marine vertebrates using an unmanned aerial vehicle that could complement longer-term tracking approaches. This approach is unlikely to have behavioural impacts and provides high accuracy and high frequency location data (10 Hz), while subsequently allowing quantitative trajectory analysis. Unmanned aerial vehicle tracking is also relatively low cost compared to single-use acoustic and GPS tags. We tracked 14 sharks for up to 10 min in a shallow lagoon of Heron Island, Australia. Trajectory analysis revealed that Epaulette sharks (Hemiscyllium ocellatum) displayed sinusoidal movement patterns, while Blacktip Reef Sharks (Carcharhinus melanopterus) had more linear trajectories that were similar to those of a Lemon shark (Negaprion acutidens). Individual shark trajectory patterns and movement speeds were highly variable. Results indicate that Epaulette sharks may be more mobile during diurnal low tides than previously thought. The approach presented here allows the movements and behaviours of marine vertebrates to be analysed at resolutions not previously possible without complex and expensive acoustic arrays. This method would be useful to assess the habitat use and behaviours of sharks and rays in shallow water environments, where they are most likely to interact with humans. © 2018 by the authors. Licensee MDPI, Basel, Switzerland.},
publisher={MDPI AG},
}

@ARTICLE{Khan20183485,
author={Khan, M. and Heurtefeux, K. and Mohamed, A. and Harras, K.A. and Hassan, M.M.},
title={Mobile Target Coverage and Tracking on Drone-Be-Gone UAV Cyber-Physical Testbed},
journal={IEEE Systems Journal},
year={2018},
volume={12},
number={4},
pages={3485-3496},
art_number={8207649},
note={cited By 31},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85038850518&doi=10.1109%2fJSYST.2017.2777866&partnerID=40&md5=a692cbbc7c185d0603964b9b56cfdbb2},
abstract={Mobile wireless sensor networks have been extensively deployed for enhancing environmental monitoring and surveillance. The availability of low-cost mobile robots equipped with a variety of sensors makes them promising in target coverage tasks. They are particularly suitable where quick, inexpensive, or nonlasting visual sensing solutions are required. In this paper, we consider the problem of low complexity target tracking to cover and follow moving targets using flying robots. We tackle this problem by clustering targets while estimating the camera location and orientation for each cluster separately through a cover-set coverage method. We also leverage partial knowledge of target mobility to enhance the efficiency of our proposed algorithms. Three computationally efficient approaches are developed: predictive fuzzy, predictive incremental fuzzy, and local incremental fuzzy. The objective is to find a compromise among coverage efficiency, traveled distance, number of drones required, and complexity. The targets move according to one of the following three possible mobility patterns: random waypoint, Manhattan grid, and reference point group mobility patterns. The feasibility of our algorithms and their performance are also tested on a real-world indoor testbed called drone-be-gone, using Parrot AR.Drone quadcopters. The deployment confirms the results obtained with simulations and highlights the suitability of the proposed solutions for real-time applications. © 2007-2012 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Tansuriyavong2018351,
author={Tansuriyavong, S. and Koja, H. and Kyan, M. and Anezaki, T.},
title={The Development of Wildlife Tracking System Using Mobile Phone Communication Network and Drone},
journal={2018 International Conference on Intelligent Informatics and Biomedical Sciences, ICIIBMS 2018},
year={2018},
pages={351-354},
art_number={8549936},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85060059911&doi=10.1109%2fICIIBMS.2018.8549936&partnerID=40&md5=2d204523073a378b5dddd87ebecf0c88},
abstract={In recent year, damaging crops by wildlife is becoming serious all over the country. On the other hand, unmanned aerial vehicle systems such as GPS, communication technology and drone have been further developed, and it is becoming possible to develop an automatic tracking system that accurately grasps the position of wildlife. Therefore, in this research, to elucidate the ecology and behavioral characteristics of wildlife, we aim to develop an automatic tracking system using drone. From the experimental results, it was confirmed that the GPS tracking by the drone is possible by sending a command using the mobile phone communication network. In this paper, we report about these details. © 2018 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Granillo201838,
author={Granillo, O.D.M. and Beltran, Z.Z.},
title={Real-Time Drone (UAV) Trajectory Generation and Tracking by Optical Flow},
journal={Proceedings - 2018 International Conference on Mechatronics, Electronics and Automotive Engineering, ICMEAE 2018},
year={2018},
pages={38-43},
art_number={8743121},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85068839301&doi=10.1109%2fICMEAE.2018.00014&partnerID=40&md5=6b4313163813653c16d0e9f7bfa3ea19},
abstract={Vision systems in drones, specifically Unmanned Aerial Vehicles (UAV) are currently used for retrieving real-time video of the area to fly over, nevertheless commercially there are no identification nor control applications for this type of aircrafts. Some existing technologies for trajectory generation are based on cubic polynomials and Bezier curves [5] but this paper presents the implementation of an optical flow algorithm that assures to track and control the trajectory in a quadrotor drone in real time, determining the distance between the drone and a certain objective as well as the speed calculation and its displacement direction by the means of the implementation of the Lucas-Kanade (LK) algorithm. The core purpose of this paper is to achieve a low-cost and faster (due to the UAV's dynamics) solution besides the implementation of a Global Positioning System (GPS) using an Inertial Navigation System (INS) to generate an aerial trajectory, therefore it can be generated in real time converting the UAV into a semi-autonomous aircraft. The aerial robot's dynamic model was obtained by the Euler-Lagrange method, the image processing is based on the pin-hole model of a camera and optical flow. The main advantages and results obtained through the experimentation was first to correctly detect the line, and by LK implementation on OpenCV the line was correctly tracked by the drone achieving this with a low computational cost and with the possibility of indoor use covering the applications where the GPS is not able to work. © 2018 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Sasaki201811735,
author={Sasaki, T. and Kudalkar, S.N. and Bertoletti, N. and Anderson, K.S.},
title={DRONE: Direct Tracking of DNA Cytidine Deamination and Other DNA Modifying Activities},
journal={Analytical Chemistry},
year={2018},
volume={90},
number={20},
pages={11735-11740},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85054401660&doi=10.1021%2facs.analchem.8b01405&partnerID=40&md5=5f83a708b94e656fb7fd264281537bfa},
abstract={Enzymes that catalyze DNA modifying activities including cytidine deamination and cytosine methylation play important biological roles and have been implicated pathologically in diseases such as cancer. Here, we report Direct Resolution of ONE dalton difference (DRONE), an ultra high performance liquid chromatography (UHPLC)-based analytical method to track a single dalton change in the cytosine-to-uracil conversion catalyzed by the human apolipoprotein B m-RNA editing catalytic polypeptide-like 3 (APOBEC3) cytidine deaminases, implicated in cancer and antiviral defense. Additionally, we demonstrate broad applicability by tracking other important DNA modifications and assessing epigenetic enzyme inhibition. We have extended our methodology to obtain data on two distinct deamination events in the same oligonucleotide substrate designed from a putative APOBEC substrate, diversifying the utility of the described method. DRONE provides an important foundation for in-depth analysis of DNA-modifying enzymes and versatile detection of novel DNA modifications of interest. Copyright © 2018 American Chemical Society.},
publisher={American Chemical Society},
}

@CONFERENCE{Yamaguchi20181137,
author={Yamaguchi, T. and Takaba, K.},
title={Remote Tracking Control of a Quadrotor-Type Drone Subject to Uncertain Time Delays},
journal={2018 57th Annual Conference of the Society of Instrument and Control Engineers of Japan, SICE 2018},
year={2018},
pages={1137-1143},
art_number={8492685},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85056745907&doi=10.23919%2fSICE.2018.8492685&partnerID=40&md5=25262a724c850624ec4e1587c06b0036},
abstract={This work is concerned with the remote position tracking control of a quadrotor-type drone via visual feedback. The stability or transient response of the drone may be significantly deteriorated by the adverse effect of time delays due to wireless communication and image processing. In general, these delays are difficult to estimate in advance. To achieve good control performance in the presence of such uncertain delays, we design a robust feedback controller in terms of linear matrix inequalities based on the guaranteed cost control technique. The effectiveness of the proposed method is verified by numerical simulations and an experimental result. © 2018 The Society of Instrument and Control Enginners - SICE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Do20181047,
author={Do, T.T. and Ahn, H.},
title={Visual-GPS combined ‘follow-me’ tracking for selfie drones},
journal={Advanced Robotics},
year={2018},
volume={32},
number={19},
pages={1047-1060},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85050962531&doi=10.1080%2f01691864.2018.1501278&partnerID=40&md5=28c38ed6c9ddead1804dcd2b95ccb2e9},
abstract={The ‘follow-me’ mode, where the drone autonomously follows and captures the user or target, is a new and attractive feature for camera drones, especially selfie drones. For this purpose, today’s commercial drones use the difference between two GPS data in the drone and user-side mobile GCS, e.g. a smartphone, but the targeting performance is often not satisfactory due to the inaccuracy of the GPS data, ranging from a few to tens of meters. Visual tracking can be considered for a solution to this problem, but the reliability of visual tracking is still questionable for long-term tracking in un-expected operating environments. The paper proposes a hybrid approach that combines the high accuracy of a visual tracking algorithm in short-term tracking and the reliability of GPS-based one in long-term tracking. The experiment with our prototype drone system demonstrates that the proposed combined approach can accomplish the follow-me operation very successfully, capturing the target in the center of video contents over 50% higher accuracy than the GPS-based ones. Also, the extreme scenario experiments verify the system can recover vision tracking failure and Wi-Fi failure quickly in a short-term, e.g. 3–7 s. © 2018, © 2018 Taylor & Francis and The Robotics Society of Japan.},
publisher={Robotics Society of Japan},
}

@CONFERENCE{Chang2018573,
author={Chang, X. and Yang, C. and Wu, J. and Shi, X. and Shi, Z.},
title={A Surveillance System for Drone Localization and Tracking Using Acoustic Arrays},
journal={Proceedings of the IEEE Sensor Array and Multichannel Signal Processing Workshop},
year={2018},
volume={2018-July},
pages={573-577},
art_number={8448409},
note={cited By 27},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85053598809&doi=10.1109%2fSAM.2018.8448409&partnerID=40&md5=d4ec0d633505809085aad4f57c0c5663},
abstract={The wide proliferation of drones has posed great threats to personal privacy and public security, which makes it urgent to monitor the drones in the sensitive areas. Drone surveillance using acoustic arrays, as a promising method, could localize and track the drones effectively. In this paper, we develop a systematic method for drone localization and tracking by using acoustic arrays. Specifically, we develop a time difference of arrival (TDOA) estimation algorithm based on Gauss priori probability density function to overcome the multipath effect and the low signal-to-noise ratio (SNR), and design a localization method by making full use of the TDOA estimation results, followed by tracking the drone by Kalman filter. Finally, field experiments are carried out to verify the effectiveness and performance of the proposed methods. The results show that they can achieve good performance in drone localization and tracking. © 2018 IEEE.},
publisher={IEEE Computer Society},
}

@CONFERENCE{Jian20181146,
author={Jian, M. and Lu, Z. and Chen, V.C.},
title={Drone detection and tracking based on phase-interferometric Doppler radar},
journal={2018 IEEE Radar Conference, RadarConf 2018},
year={2018},
pages={1146-1149},
note={cited By 33},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85049928482&doi=10.1109%2fRADAR.2018.8378723&partnerID=40&md5=72e95fda4ec128ff0efa9abff67b10ea},
abstract={In this paper, drone detection and tracking based on phase-interferometry are investigated. Data collected by a simple dual-channel Doppler radar is used for implementing the joint range-Doppler-azimuth processing. Experimental results show that micro drones can be detected and tracked by applying the joint range-Doppler-azimuth processing. Features extracted from the range-Doppler-azimuth domain can be used to identify drones. © 2018 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Jeong2018773,
author={Jeong, J. and Kim, J. and Yoon, T.S. and Park, J.B.},
title={Drone-based power-line tracking system},
journal={Transactions of the Korean Institute of Electrical Engineers},
year={2018},
volume={67},
number={6},
pages={773-781},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85049689259&doi=10.5370%2fKIEE.2018.67.6.773&partnerID=40&md5=5b42d287e0d31a09da33cb08a2639041},
abstract={In recent years, a study of power-line inspection using an unmanned aerial vehicle (UAV) has been actively conducted. However, relevant studies have been conducting power-line inspection with an UAV operated by manual control, and they have developed just power-line detection algorithm on aerial images. To overcome limitations of existing research, we propose a drone-based power-line tracking system in this paper. The main contributions of this paper are to operate developed system under configured environment and to develop a power-line detection algorithm in real-time. Developed system is composed of the power-line detection and the image-based tracking control. To detect a power-line in real-time, a region of interest (ROI) image is extracted. Furthermore, clustering algorithm is used in order to discriminate the power-line from background. Finally, the power-line is detected by using the Hough transform, and a center position and a tilt angle are estimated by using the Kalman filter to control a drone smoothly. We design a position controller and an attitude controller for image-based tracking control, and both controllers are designed based on the proportional-derivative (PD) control method. The interaction between the position controller and the attitude controller makes the drone track the power-line. Several experiments were carried out in environments where conditions are similar to actual environments, which demonstrates the superiority of the developed system. Copyright © The Korean Institute of Electrical Engineers.},
publisher={Korean Institute of Electrical Engineers},
}

@CONFERENCE{Seiber2018377,
author={Seiber, C. and Nowlin, D. and Landowski, B. and Tolentino, M.E.},
title={Tracking hazardous aerial plumes using IoT-enabled drone swarms},
journal={IEEE World Forum on Internet of Things, WF-IoT 2018 - Proceedings},
year={2018},
volume={2018-January},
pages={377-382},
note={cited By 16},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85050378799&doi=10.1109%2fWF-IoT.2018.8355118&partnerID=40&md5=de1755faebb7a7d963cdfc10c92d4aa7},
abstract={Emergency response teams are charged with ensuring citizen safety from life-threatening events such as structural fires, vehicle accidents, and hazardous material spills. While managing such events is dangerous, the release of hazardous materials, such as toxic chemicals, into the atmosphere is particularly challenging. Upon arrival at a scene, response teams must quickly identify the hazardous substance and the contaminated area to limit exposure to nearby population centers. For airborne toxins, this assessment is complicated by environmental conditions, such as changes in wind speed and direction that can cause hazardous, aerial plumes to move dynamically. Without a way to dynamically monitor and assess atmospheric conditions during these events, response teams must conservatively predict the extent of the contaminated area and then orchestrate evacuations and reroute traffic to ensure the safety of nearby populations. In this paper, we propose outfitting swarms of drones with Internet of Things (IoT) sensor platforms to enable dynamic tracking of hazardous aerial plumes. Augmenting drones with sensors enables emergency response teams to maintain safe distances during hazard identification, minimizing first response team exposure. Additionally, we integrate sensor-based particulate detection with autonomous drone flight control providing the capability to dynamically identify and track the boundaries of aerial plumes in real time. This enables first responders to visually identify plume movement and better predict and isolate the impact area. We describe the composition of our prototype IoT-enhanced drone system and describe our initial evaluations. © 2018 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Guvenc201875,
author={Guvenc, I. and Koohifar, F. and Singh, S. and Sichitiu, M.L. and Matolak, D.},
title={Detection, Tracking, and Interdiction for Amateur Drones},
journal={IEEE Communications Magazine},
year={2018},
volume={56},
number={4},
pages={75-81},
note={cited By 103},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85045884574&doi=10.1109%2fMCOM.2018.1700455&partnerID=40&md5=48c0c81d2e8d45da2eb2a2e7b0f0dba4},
abstract={Unmanned aerial vehicles, also known as drones, are expected to play major roles in future smart cities, for example, by delivering goods and merchandise, serving as mobile hotspots for broadband wireless access, and maintaining surveillance and security. The goal of this survey article is to study various potential cyber and physical threats that may arise from the use of UAVs, and subsequently review various ways to detect, track, and interdict malicious drones. In particular, we review techniques that rely on ambient radio frequency signals (emitted from UAVs), radars, acoustic sensors, and computer vision techniques for detection of malicious UAVs. We present some early experimental and simulation results on range estimation of UAVs and receding horizon tracking of UAVs. Finally, we summarize common techniques that are considered for interdiction of UAVs. © 1979-2012 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Yang20181,
author={Yang, W.-S. and Chun, M.-H. and Jang, G.-W. and Baek, J.-H. and Kim, S.-H.},
title={A study on smart drone using quadcopter and object tracking techniques},
journal={Proceedings of the 2017 4th International Conference on Computer Applications and Information Processing Technology, CAIPT 2017},
year={2018},
volume={2018-January},
pages={1-4},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85048198847&doi=10.1109%2fCAIPT.2017.8320658&partnerID=40&md5=cddb94611520ce5e26539124a38f2adf},
abstract={In this research, we developed a smart drone system based on quad copter with integrated object tracking algorithm for scene analysis. We tool advantage of theory of quad rotor flight and PID control for not only stable hovering but also stable image acquisition. For object tracking, we integrated color information and optical flow with nonlinear matched filter of spatial frequency domain. Furthermore, we proposed a solution for safer experiment environment configuration. © 2017 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Stark201844,
author={Stark, D.J. and Vaughan, I.P. and Evans, L.J. and Kler, H. and Goossens, B.},
title={Combining drones and satellite tracking as an effective tool for informing policy change in riparian habitats: a proboscis monkey case study},
journal={Remote Sensing in Ecology and Conservation},
year={2018},
volume={4},
number={1},
pages={44-52},
note={cited By 14},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85021806255&doi=10.1002%2frse2.51&partnerID=40&md5=88746aebefeb6d3d2d682490b11c559e},
abstract={Rapid reaction times to undesirable events are becoming increasingly important for the protection and conservation of habitats and species. This study demonstrates how Unmanned Aerial Vehicles, or drones, and satellite tracking of individual animals can be combined to identify important conservation issues (e.g. deforestation). When quickly disseminated, the information can lead to a rapid change in conservation policy. An adult male proboscis monkey, belonging to a one-male social group, was GPS tracked for 6 months in Sabah, Malaysian Borneo during 2012. Riparian habitats featured heavily (25.4% of total time, 88.6% of all sleeping sites) in the group's home range. A fixed-wing drone was used in 2015 to map the habitat in high-resolution. These data revealed that 47.54 ha of forest had been cleared shortly before the drone flights. GPS tagging data revealed the importance of this area for a one-male proboscis monkey group. A total of 30.1% of the proboscis monkeys' home range area had been cleared, as well as 11.4% of sleeping sites. Furthermore, drone images revealed that the felling extended to the river's edge, disregarding water resources laws requiring riparian reserves of a minimum of 20 m. Following this discovery, a press release including drone imagery combined with GPS data, was published linking habitat destruction to a species that is economically important for the tourism industry in Sabah. The day following dissemination of the data, the Sabah State Government ordered an immediate cessation on further land clearing at sensitive riparian reserves along the river. We propose that this combination of satellite and aerial data provides potential for an effective conservation tool for endangered, iconic and economically important species. This visually compelling data, feasible over large spatial scales, can directly inform policy change in a quick and timely manner. © 2017 The Authors. Remote Sensing in Ecology and Conservation published by John Wiley & Sons Ltd on behalf of Zoological Society of London},
publisher={Wiley-Blackwell},
}

@ARTICLE{Yoo2018336,
author={Yoo, H.-J. and Kim, B.-H.},
title={Study on the space monitoring drone solution using motion detection and tracking algorithm},
journal={Journal of Advanced Research in Dynamical and Control Systems},
year={2018},
volume={10},
number={14 Special Issue},
pages={336-343},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85061840151&partnerID=40&md5=914cd51be396137fab92bb0cfbdbd646},
abstract={Background/Objectives: Currently, most of the CCTV systems are used for space monitoring and inspection. However, the CCTV surveillance system has a problem in that it has to be monitored 24 hours in the central control and management room. In addition, there are problems such as additional installation and additional financial expenses such as additional installation of CCTV due to blind spot generation. Methods/Statistical analysis: In this paper, we designed a motion detection and tracking algorithm and applied it to a drone to study real-time space monitoring. For this purpose, a heterogeneous integrated module such as motion sensor, breakage sensor, and impact sensor designed for real-time spatial monitoring and management. In addition, when abnormal data is detected through the GPS coordinates of the space, it is immediately transmitted to the drones. Finally, we applied the motion tracking algorithm to study the solution of real-time space image transmission and object tracking. Findings: In this paper, we have systematically designed motion object tracking technology, heterogeneous sensor integration module technology, and wireless communication interworking technology for the proposed drone solution. As a result, it recognizes motion objects obtained through image data, and distinguishes backgrounds and objects for tracking motion objects. In addition, the BLE module is the main chip, and the thermal sensor and the impact sensor are designed as an integrated board type module. And, it is designed to efficiently transmit small data packets over long distance with minimum power consumption through LoRa communication network. Improvements/Applications: Through this research, unlike the existing CCTV surveillance equipment, it can be differentiated that it can monitor the space by the actual surveillance response. In other words, it does not require 24-hour monitoring and can be prevented in advance through real-time tracking. In addition, it is a unique solution that can prepare future measures through image pattern analysis. © 2018, Institute of Advanced Scientific Research, Inc.. All rights reserved.},
publisher={Institute of Advanced Scientific Research, Inc.},
}

@ARTICLE{Lee20186071,
author={Lee, M.-H. and Yeom, S.},
title={Multiple target detection and tracking on urban roads with a drone},
journal={Journal of Intelligent and Fuzzy Systems},
year={2018},
volume={35},
number={6},
pages={6071-6078},
note={cited By 6},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85054632164&doi=10.3233%2fJIFS-169847&partnerID=40&md5=5587d27f772748b844d515b8f006f833},
abstract={Recently, drone technology has developed rapidly for various purposes. A drone is very useful for aerial surveillance due to its remote sensing capability. Multiple target detection and tracking are essential to recognize any harmful threats in advance, however the image captured at a distance is easily degraded due to blurring and noise as well as low resolution. This paper addresses the detection and tracking of moving vehicles with drone imaging. A drone captures video sequences of multiple moving vehicles from a distance. Cars and buses are the objects of interests driving on urban roads. The detection step consists of frame difference followed by thresholding and morphological operation considering the size of region of interest (ROI). The centroids of the ROI's are considered measurements for tracking. Tracking is performed with interacting multiple model (IMM) filtering, which estimate the state of vectors and covariance matrices using multiple modes of Kalman filtering. The measurements in the validation region are associated with established tracks by the nearest neighbor rule. In the experiment, total seven moving cars and buses are captured at a long distance by a drone. It will be shown that the proposed method well detects the moving vehicles and achieves a good accuracy in estimating their locations. © 2018 - IOS Press and the authors. All rights reserved.},
publisher={IOS Press},
}

@ARTICLE{Boudjit20181013,
author={Boudjit, K. and Larbes, C. and Ramzan, N.},
title={Ann design and implementation for real-time object tracking using quadrotor ar.Drone 2.0},
journal={Journal of Experimental and Theoretical Artificial Intelligence},
year={2018},
volume={30},
number={6},
pages={1013-1035},
note={cited By 7},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85053040527&doi=10.1080%2f0952813X.2018.1509896&partnerID=40&md5=d447547cb1ec29541f703c1080a6beee},
abstract={This paper aims to use a visual-based control mechanism to control a quadrotor, which is in pursuit of a target. The non-linear nature of a quadrotor, on onehand,andthedifficulty of obtaining an exact model for it, on the other hand, constitute two serious challenges in designing a controller for this UAV. A potential solution for such problems is the use of intelligent control methods such as those that rely on ANNs. A novel technique based on ANNs is proposed in this work for the identification and tracking of targets. Multilayer perceptron is used for this purpose. Experimental results and simulations are shown to demonstrate the feasibility of the proposed method for target tracking. © 2018 Informa UK Limited, trading as Taylor & Francis Group.},
publisher={Taylor and Francis Ltd.},
}

@ARTICLE{Son2018,
author={Son, Y. and Noh, J. and Choi, J. and Kim, Y.},
title={GyrosFinger: Fingerprinting drones for location tracking based on the outputs of MEMS gyroscopes},
journal={ACM Transactions on Privacy and Security},
year={2018},
volume={21},
number={2},
art_number={10},
note={cited By 8},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85042617779&doi=10.1145%2f3177751&partnerID=40&md5=de2f9a8ad5f461f6d0925446003e7af3},
abstract={Drones are widely used for various purposes such as delivery, aerial photography, and surveillance. Considering the increasing drone-related services, tracking the locations of drones can cause security threats such as escaping from drone surveillance, disturbing drone-related services, and capturing drones. For wirelessly monitoring the status of drones, telemetry is used, and this status information contains various data such as latitude and longitude, calibrated sensor outputs, and sensor offsets. Because most of the telemetry implementation supports neither authentication nor encryption, an attacker can obtain the status information of the drones by using an appropriate wireless communication device such as software-defined radio. While the attacker knows the locations of the drones from the status information, this information is not sufficient for tracking drones because the status information does not include any identity information that can bind the identity of the drone with its location. In this article, we propose a fingerprinting method for drones in motion for the binding of the identity of the drone with its location. Our fingerprinting method is based on the sensor outputs included in the status information, i.e., the offsets of micro-electro mechanical systems (MEMS) gyroscope, an essential sensor for maintaining the attitude of drones. We found that the offsets of MEMS gyroscopes are different from each other because of manufacturing mismatches, and the offsets of five drones obtained through their telemetry are distinguishable and constant during their flights. To evaluate the performance of our fingerprinting method on a larger scale, we collected the offsets from 70 stand-alone MEMS gyroscopes to generate fingerprints. Our experimental results show that, when using the offsets of three and two axes calculated from 128 samples of the raw outputs per axis as fingerprints, the F-scores of the proposed method reach 98.78% and 94.47%, respectively. The offsets collected after a month are also fingerprinted with F-scores of 96.58% and 78.45% under the same condition, respectively. The proposed fingerprinting method is effective, robust, and persistent. Additionally, unless the MEMS gyroscope is not replaced, our fingerprinting method can be used for drone tracking even when the target drones are flying. © 2018 ACM.},
publisher={Association for Computing Machinery},
}

@ARTICLE{Chen2018131,
author={Chen, P. and Dang, Y. and Liang, R. and Zhu, W. and He, X.},
title={Real-Time Object Tracking on a Drone with Multi-Inertial Sensing Data},
journal={IEEE Transactions on Intelligent Transportation Systems},
year={2018},
volume={19},
number={1},
pages={131-139},
art_number={8054712},
note={cited By 40},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85030776761&doi=10.1109%2fTITS.2017.2750091&partnerID=40&md5=c18562b34f2c84dfd3d33f78f81b2890},
abstract={Real-time object tracking on a drone under a dynamic environment has been a challenging issue for many years, with existing approaches using off-line calculation or powerful computation units on board. This paper presents a new lightweight real-time onboard object tracking approach with multi-inertial sensing data, wherein a highly energy-efficient drone is built based on the Snapdragon flight board of Qualcomm. The flight board uses a digital signal processor core of the Snapdragon 801 processor to realize PX4 autopilot, an open-source autopilot system oriented toward inexpensive autonomous aircraft. It also uses an ARM core to realize Linux, robot operating systems, open-source computer vision library, and related algorithms. A lightweight moving object detection algorithm is proposed that extracts feature points in the video frame using the oriented FAST and rotated binary robust independent elementary features algorithm and adapts a local difference binary algorithm to construct the image binary descriptors. The K-nearest neighbor method is then used to match the image descriptors. Finally, an object tracking method is proposed that fuses inertial measurement unit data, global positioning system data, and the moving object detection results to calculate the relative position between coordinate systems of the object and the drone. All the algorithms are run on the Qualcomm platform in real time. Experimental results demonstrate the superior performance of our method over the state-of-the-art visual tracking method. © 2000-2011 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Park2017696,
author={Park, J. and Kim, D.H. and Shin, Y.S. and Lee, S.-H.},
title={A comparison of convolutional object detectors for real-time drone tracking using a PTZ camera},
journal={International Conference on Control, Automation and Systems},
year={2017},
volume={2017-October},
pages={696-699},
note={cited By 18},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85044476793&doi=10.23919%2fICCAS.2017.8204318&partnerID=40&md5=3c00be6c4f69925ea70b9e75d9d35cb0},
abstract={As highly maneuverable drones are available at the low price, the threats that might be caused by the drone attacks has been increased. Recent object detectors have been dramatically improved in accuracy by using convolutional neural networks, and these can be utilized to identify hostile drones. In this paper, we examine state-of-the-arts convolutional object detectors for a real-time drone detection and tracking system using a Pan-Tilt-Zoom (PTZ) camera. In the drone detection and tracking system, an object detector is used to identify whether an image from the PTZ camera contains a drone, and our system generates PTZ actions to track the detected drone. To detect small size drones in real-time, an appropriate object detector should be selected. This paper compares six convolutional object detectors in the accuracy and speed. © 2017 Institute of Control, Robotics and Systems - ICROS.},
publisher={IEEE Computer Society},
}

@CONFERENCE{Shirai20171589,
author={Shirai, J. and Yamaguchi, T. and Takaba, K.},
title={Remote visual servo tracking control of drone taking account of time delays},
journal={2017 56th Annual Conference of the Society of Instrument and Control Engineers of Japan, SICE 2017},
year={2017},
volume={2017-November},
pages={1589-1594},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85044121013&doi=10.23919%2fSICE.2017.8105559&partnerID=40&md5=4465451a9ec759879aee62b2defa0791},
abstract={The use of drones has recently been expected in many applications such as exploration in dangerous areas, security surveillance, and logistics. Accurate position control of the drones is required in these applications. This work is concerned with the remote position tracking control of a quadrotor-type drone via visual feedback control. The transient response or stability of the drone may be significantly deteriorated by the adverse effect of the time delays due to wireless communication and image processing. In this work, we construct the LQI optimal servo control system for the linearized drone model with state augmentation to cope with the time delays. The effectiveness of the proposed method is verified by a simulation and an experiment. © 2017 The Society of Instrument and Control Engineers - SICE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Smyczyński2017734,
author={Smyczyński, P. and Starzec, L. and Granosik, G.},
title={Autonomous drone control system for object tracking: Flexible system design with implementation example},
journal={2017 22nd International Conference on Methods and Models in Automation and Robotics, MMAR 2017},
year={2017},
pages={734-738},
art_number={8046919},
note={cited By 13},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85035342759&doi=10.1109%2fMMAR.2017.8046919&partnerID=40&md5=5eda89f5f7038d88a85a93bc48e1fba8},
abstract={This paper contains presentation of the flexible control system for an autonomous UAV (unmanned air vehicle). The complete description of hardware and software solutions used to realize autonomous flight are presented in this work. Main objective of the research was to develop software which provides ease of adjustment and extendibility to drone system with different equipment. Presented system is utilizable on various hardware platforms and is capable of realizing different missions with minimal adjustments. Described concept significantly simplifies designing complex system by introducing modular architecture. Presented method of dividing software components into modules with single functionality minimizes amount of work necessary to adjust system in case of changes in hardware. Presented general concept of system architecture is backed up with real life working model designed for tracking and landing on moving target. This paper contains detailed description of algorithms used in the project. Landing area detection is accomplished with vision system. Canny's edge detection algorithm with contour shape analysis algorithm is used for marker detection. Lucas-Kanade optical flow algorithm is applied for tracking detected pattern. Mission planning is realized as dedicated state machine developed for this particular task. System design is built with use of ROS (Robot Operating System) and is utilizing its subscriber-publisher method of data exchange between separated software units. Especially designed frame is used as hardware platform. Exemplary system is realized with Raspberry Pi 3 as onboard computer and Pixhawk flight controller. This concept and the exemplary system is a result of preparation for Mohamed Bin Zayed International Robotic Challenge 2017 in Abu Dhabi. Results from experiments performed as trials for the competition and future prospects are presented in this paper. © 2017 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Lee20171123,
author={Lee, K.-U. and Choi, Y.-H.},
title={Dynamic surface control based tracking control for a drone equipped with a manipulator},
journal={Transactions of the Korean Institute of Electrical Engineers},
year={2017},
volume={66},
number={7},
pages={1123-1130},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85030552443&doi=10.5370%2fKIEE.2017.66.7.1123&partnerID=40&md5=7e8fbba95b54d4c78c5213053faeb655},
abstract={This paper deals with the dynamic surface control based tracking control for a drone equipped with a 2-DOF manipulator. First, the dynamics of drone and 2-DOF manipulator are derived separately. And we obtain the combined model of a drone equipped with a manipulator considering the inertia and the reactive torque generated by a manipulator. Second, a dynamic surface control based attitude and altitude control method is presented. Also, multiple sliding mode control based position control method is presented. The system stability and convergence of tracking errors are proven using Lyapunov stability theory. Finally, the simulation results are given to verify the effectiveness of the proposed control method. Copyright © The Korean Institute of Electrical Engineers.},
publisher={Korean Institute of Electrical Engineers},
}

@CONFERENCE{Multerer2017299,
author={Multerer, T. and Ganis, A. and Prechtel, U. and Miralles, E. and Meusling, A. and Mietzner, J. and Vossiek, M. and Loghi, M. and Ziegler, V.},
title={Low-cost jamming system against small drones using a 3D MIMO radar based tracking},
journal={European Microwave Week 2017: "A Prime Year for a Prime Event", EuMW 2017 - Conference Proceedings; 14th European Microwave Conference, EURAD 2017},
year={2017},
volume={2018-January},
pages={299-302},
note={cited By 28},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85046269598&doi=10.23919%2fEURAD.2017.8249206&partnerID=40&md5=746efdb368b7d3720dfdf1252cbe952f},
abstract={This paper presents an anti-drone system which consists of a 3D Frequency Modulated Continuous Wave (FMCW) Multiple Input Multiple Output (MIMO) radar and a directional jammer working at 2.4 GHz. The radar is continuously scanning a certain area and waits until a target enters the area to secure. A tracking algorithm evaluates the movement of the target. If a potential threat is identified, the directional antenna, mounted on a two-axis gimbal, is steered to the target. With the use of a directional antenna, the control signal of the drone can be superimposed by a strong jamming signal which makes controlling of the drone impossible. Even if the drone would move further or back to its base station, the radar would track it and continue blocking the communication. This way, it is possible to secure critical infrastructure against most of the commercially available drones using WiFi frequencies or Global Positioning System (GPS) for control and payload transmission. The paper presents the system, its potential applications and a field demonstration. © 2017 European Microwave Association.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Ponnuswamy2017,
author={Ponnuswamy, D. and Kumar, S.S.},
title={Design and realization of an energy efficient vision-based autonomous target tracking drone using LabVIEW},
journal={Proceedings of 2016 Online International Conference on Green Engineering and Technologies, IC-GET 2016},
year={2017},
art_number={7916707},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85020207712&doi=10.1109%2fGET.2016.7916707&partnerID=40&md5=797ef2ab855a548db8c32a3eb09c7942},
abstract={UAVs based surveillance system adopted in various countries for undergoing rescue services in mountainous terrains during natural calamities, highly vehicular traffic regions and in fire rescue operations. The static altitude maintenance requires frequent recharging of batteries with poor flight time. The Centralized Altitude Scheduling (CAS) and Localized Altitude Scheduling (LAS) Algorithms cannot produce the optimum solution even for small instances because the altitude of the drone is calculated in prior to the surveillance action, it may be suitable for the static targets but produces inefficient results for the mobile target objects. The options and features available to the users in existing autonomous surveillance system are minimum and cannot be used in places other than the application it is designed for. © 2016 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Gowda201777,
author={Gowda, M. and Manweiler, J. and Dhekne, A. and Choudhury, R.R. and Weisz, J.D.},
title={Integrating glonass with gps for drone orientation tracking},
journal={Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
year={2017},
volume={10340 LNCS},
pages={77-92},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85088912148&doi=10.1007%2f978-3-319-67235-9_7&partnerID=40&md5=3b9201206888753a78cd4a7712c7e4b9},
abstract={In addition to position sensing, GPS receivers can be leveraged for orientation sensing too. We place multiple GPS receivers on drones and translate their relative positions into orientation. Such an orthogonal mode of orientation sensing provides failsafe under Inertial sensor failures – a primary cause of drone crashes today. This paper integrates GLONASS satellite measurements with GPS for enhancing the orientation accuracy. Accurate estimate of orientation depends upon high precision relative positioning of the GPS receivers. While GPS carrier phases provide high precision ranging data, the phases are noisy and wrap after every wavelength which introduces ambiguity. Moreover, GPS signals experience poor SNR and loss of satellite locks under aggressive flights. This can severely limit both the accuracy and the amount of carrier phase data available. Fortunately, integrating the ubiquitously available Russian GLONASS satellites with GPS can double the amount of observations and substantially improve the robustness of orientation estimates. However, the fusion is non-trivial because of the operational difference between FDMA based GLONASS and CDMA based GPS. This paper proposes a temporal differencing scheme for fusion of GLONASS and GPS measurements, through a system called SafetyNet. Results from 11 sessions of 5–7 min flights report median orientation accuracies of 2◦ even under overcast weather conditions. © Springer International Publishing AG 2017.},
publisher={Springer},
}

@ARTICLE{Okutake2017593,
author={Okutake, T. and Uchida, N. and Yamamoto, N.},
title={Proposal of collaborative object tracking methods by multi-drones for flight surveillance systems},
journal={Lecture Notes on Data Engineering and Communications Technologies},
year={2017},
volume={2},
pages={593-600},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85056391608&doi=10.1007%2f978-3-319-49106-6_58&partnerID=40&md5=4daf2537256fcc8e35db9b8f811f8be1},
abstract={Although there are rapid growth the drone’s applications such as surveillance systems and delivery systems in recent years, the problems of the accidents are also increasing conversely. Therefore, this paper discusses the collaborative object tracking methods by multi-drones. The proposed methods consist of the function of the motion tracking and the WiFi detections for each drone, and choose a proper level of emergent procedures in order to avoid the drone’s accident in various circumstances. Then, the prototype system of the proposed methods is introduced and discussed for the future works. © Springer International Publishing AG 2017.},
publisher={Springer Science and Business Media Deutschland GmbH},
}

@ARTICLE{Eu2017260,
author={Eu, K.S. and Yap, K.M. and Tan, W.C.},
title={A simulation study of micro-drone chemical plume tracking performance in tree farm environments},
journal={Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
year={2017},
volume={10645 LNCS},
pages={260-269},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85035101937&doi=10.1007%2f978-3-319-70010-6_24&partnerID=40&md5=4eb6c313c7721aeed99c486cd3c466c7},
abstract={Chemical plume tracking (CPT) technology is the mean of tracking the flow of specific chemical plume in the air, to locate the source. Nowadays, CPT technology, for instance, a micro-drone based chemical plume tracking robot, has great potential in identifying hidden explosives, illegal drugs and blood for police and military purposes. However, environmental factors such as obstacles on site can change the wind vectors will cause inconsistent odor plume propagation. With most of the previous work conducted from numerous researchers carried out in empty open space, this paper studies the influence of obstacles on site towards CPT’s performance, which the simulation focus in one specific environment, a tree farm, with different density of trees or trees’ spacing. For this paper, we developed a 3D gas dispersion simulator with mobile robot olfaction (MRO) capability. Through the simulation, correlation between the impacts of tree farm density factor to CPT’s performance is found out, where higher tree density (or smaller tree spacing distance) can significantly reduce the performance of CPT. This study is an important fundamental contribution for drone’s CPT operation in agriculture application beneficial to future use, such as smell tracking of mature fruits in tree farm. © Springer International Publishing AG 2017.},
publisher={Springer Verlag},
}

@ARTICLE{Pilté2017301,
author={Pilté, M. and Bonnabel, S. and Barbaresco, F.},
title={Drone tracking using an innovative UKF},
journal={Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
year={2017},
volume={10589 LNCS},
pages={301-309},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85033698230&doi=10.1007%2f978-3-319-68445-1_35&partnerID=40&md5=a7c8a22b3b81a0b0bc3564feb3c08975},
abstract={This paper addresses the drone tracking problem, using a model based on the Frenet-Serret frame. A kinematic model in 2D, representing intrinsic coordinates of the drone is used. The tracking problem is tackled using two recent filtering methods. On the one hand, the Invariant Extended Kalman Filter (IEKF), introduced in [1] is tested, and on the other hand, the second step of the filtering algorithm, i.e. the update step of the IEKF is replaced by the update step of the Unscented Kalman Filter (UKF), introduced in [2]. These two filters are compared to the well known Extended Kalman Filter. The estimation precision of all three algorithms are computed on a real drone tracking problem. © 2017, Springer International Publishing AG.},
publisher={Springer Verlag},
}

@CONFERENCE{Kamei2016512,
author={Kamei, K. and Narumi, K. and Shuto, D.},
title={Adaptive Color Tracking for Particle Filter to Control a Drone in a Forest},
journal={Proceedings - 2016 Joint 8th International Conference on Soft Computing and Intelligent Systems and 2016 17th International Symposium on Advanced Intelligent Systems, SCIS-ISIS 2016},
year={2016},
pages={512-517},
art_number={7801701},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85010284781&doi=10.1109%2fSCIS-ISIS.2016.0114&partnerID=40&md5=433524555d7761b23b5d2dbe4c3c2f80},
abstract={Recently, drones have been used for many purposes. The investigation of tree growth in a forest is also one of the expectations for drone applications. The aim of this paper is that a drone recognizes a color marker which is set to a tree from an image, and a drone approaches to that tree, and then return to the goal zone. To solve the task, we propose to apply the algorithm of Particle Filter for the color marker recognition. The difficulty of applying image processing at a forest is that degree of luminance changes drastically, due to incident light through the trees. To overcome this difficulty, we attempt the method to update the tracking color by a time period. From the results of experiments, our proposal has been able to deal with changes in luminance intensity, and then a drone with our proposal has solved a part of the task for competition. © 2016 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Gowda2016280,
author={Gowda, M. and Manweiler, J. and Dhekne, A. and Choudhury, R.R. and Weisz, J.D.},
title={Tracking drone orientation with multiple GPS receivers},
journal={Proceedings of the Annual International Conference on Mobile Computing and Networking, MOBICOM},
year={2016},
volume={0},
number={1},
pages={280-293},
note={cited By 22},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84994169082&doi=10.1145%2f2973750.2973768&partnerID=40&md5=a74b573c2da5e25216f15068cdb99925},
abstract={Inertial sensors continuously track the 3D orientation of a flying drone, serving as the bedrock for maneuvers and stabilization. However, even the best inertial measurement units (IMU) are prone to various types of correlated failures. We consider using multiple GPS receivers on the drone as a failsafe mechanism for IMU failures. The core challenge is in accurately computing the relative locations between each receiver pair, and translating these measurements into the drone's 3D orientation. Achieving IMU-like orientation requires the relative GPS distances to be accurate to a few centimeters - a difficult task given that GPS today is only accurate to around 1-4 meters. Moreover, GPS-based orientation needs to be precise even under sharp drone maneuvers, GPS signal blockage, and sudden bouts of missing data. This paper designs SafetyNet, an off-the-shelf GPS-only system that addresses these challenges through a series of techniques, culminating in a novel particle filter framework running over multi-GNSS systems (GPS, GLONASS, and SBAS). Results from 11 sessions of 5-7 minute flights report median orientation accuracies of 2° even under overcast weather conditions. Of course, these improvements arise from an increase in cost due to the multiple GPS receivers, however, when safety is of interest, we believe that tradeoff is worthwhile. © 2016 ACM.},
publisher={Association for Computing Machinery},
}

@ARTICLE{Dorj20163043,
author={Dorj, B. and Kang, D.C. and Lee, D.J.},
title={Vision based target tracking control of a multirotor drone using raspberry Pi embedded module},
journal={Advanced Science Letters},
year={2016},
volume={22},
number={10},
pages={3043-3046},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85009083365&doi=10.1166%2fasl.2016.7995&partnerID=40&md5=5081ed9778ddac75c00bc9bbf31eb600},
abstract={In this paper, we present the design of a quadrotor vision system using a Raspberry Pi camera. The vision system of quadrotor is able to doing image process, and connecting ground control computer while autonomous flights. We developed control algorithm based on a combination of the vision system and IMU, range sensor measurements, in order to estimate the velocity of the quadrotor in its body frame. The results of the simulation and experiment shown the effectiveness of our approach in an unknown environment. © 2016 American Scientific Publishers. All rights reserved.},
publisher={American Scientific Publishers},
}

@CONFERENCE{Chakrabarty201625,
author={Chakrabarty, A. and Morris, R. and Bouyssounouse, X. and Hunt, R.},
title={Autonomous indoor object tracking with the Parrot AR.Drone},
journal={2016 International Conference on Unmanned Aircraft Systems, ICUAS 2016},
year={2016},
pages={25-30},
art_number={7502612},
note={cited By 23},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84979779834&doi=10.1109%2fICUAS.2016.7502612&partnerID=40&md5=9c5bd30b53e234b7a03225a07557269a},
abstract={This article presents an image-based visual servoing system for indoor visual tracking of 3D moving objects by an Unmanned Aerial Vehicle. This system autonomously follows a 3D moving target object, maintaining it with a fixed distance and centered on its image plane. The initial setup is tested in a detailed simulation environment. The system is then validated on flights in indoor scenarios using the Parrot AR.Drone and the CMT tracker, demonstrating the robustness of the system to differences in object features, environmental clutter, and target trajectory. The obtained results indicate that the proposed system is suitable for complex controls task, such object surveillance and pursuit. © 2016 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Curetti2016,
author={Curetti, M. and Serra, M. and Bravo, S.G. and Flesia, A.G. and Mathé, L.},
title={Use of inertial and altimeter information for rectified searches in image target tracking for drone applications},
journal={2015 16th Workshop on Information Processing and Control, RPIC 2015},
year={2016},
art_number={7497177},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84982150681&doi=10.1109%2fRPIC.2015.7497177&partnerID=40&md5=370a8fc8bf4829ba074588e8753e4100},
abstract={In this paper, a model for target tracking with data fusion taken from inertial and altimeter sensors for a quadcopter is proposed. With some environmental restrains and using INS/altitude data, the new position and template changes are predicted. The model dynamics is estimated on the basis of the specifications of the UAV IRIS+, with a pointgrey blackfly camera (PGE-13E4C-CS), a gimbal (TAROT 2D), and a Laser Rangefinder (SF02). Simulation results are shown. © 2015 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Ouchatti2016414,
author={Ouchatti, Z. and Bensaid, A. and Moutaouakkil, F. and Medromi, H.},
title={Deterministic Method of Visual Servoing: Robust Object Tracking by Drone},
journal={Proceedings - Computer Graphics, Imaging and Visualization: New Techniques and Trends, CGiV 2016},
year={2016},
pages={414-422},
art_number={7467749},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84973661640&doi=10.1109%2fCGiV.2016.87&partnerID=40&md5=9ffc458ee661544bf39744e7a777921b},
abstract={This work is part of an application context, focused on the analysis of images flow acquired by a cameraembedded in a drone, controlled by a control station. Specifically, we are interested in the coupling vision-command, in order to develop a control system that allowsan autonomous navigation and operation of the UnmannedAerial Vehicle in complex environments where the use ofvisual sensors appears to be essential for moving the dronein a controlled manner but also to be capable of increasingthe stability of the UAV. We propose the state of the artin image-based visual servoing, focused on the control ofunmanned aerial vehicles and allows moving from a currentposition to a desired position according the observed scenewhile also improving the flight performance (stability andaccuracy). Our contribution will be in the proposal of acontrol approach capable to tracking an object byintroducing the concept of real-time and subsequently uses avisual memory in the form of keyframes to automaticallyreproduce a route already made. © 2016 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Bartak201635,
author={Bartak, R. and Vykovsky, A.},
title={Any object tracking and following by a flying drone},
journal={Proceedings - 14th Mexican International Conference on Artificial Intelligence: Advances in Artificial Intelligence, MICAI 2015},
year={2016},
pages={35-41},
art_number={7429411},
note={cited By 14},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84987776731&doi=10.1109%2fMICAI.2015.12&partnerID=40&md5=fd529a25b1087de90fb4fefdaae0dbf4},
abstract={AR.Drone is a quadcopter with onboard sensors including a frontal camera. The drone can be controlled from a computer via WiFi. This paper describes a method for autonomous tracking of a selected object by AR.Drone. We utilize a computer-vision approach called tracking-learning-detection (TLD) to track an arbitrary object selected by a user in the video-stream going from the front camera of the drone. Information about location of the tracked object is then used to guide the drone using the proportional-integral-derivative (PID) controller. The method was implemented in software FollowMe. © 2015 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Velez201673,
author={Velez, P. and Certad, N. and Ruiz, E.},
title={Trajectory Generation and Tracking Using the AR.Drone 2.0 Quadcopter UAV},
journal={Proceedings - 12th LARS Latin American Robotics Symposium and 3rd SBR Brazilian Robotics Symposium, LARS-SBR 2015 - Part of the Robotics Conferences 2015},
year={2016},
pages={73-78},
art_number={7402144},
note={cited By 7},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84964324520&doi=10.1109%2fLARS-SBR.2015.33&partnerID=40&md5=c78567ca7c330585a037355ad9634c8d},
abstract={Trajectory generation and tracking algorithms were developed using ROS (Robot Operating System) for the AR. Drone 2.0 quad copter. Flight paths were created with cubic polynomials and Bezier curves. A PID controller was implemented to drive the AR. Drone from its current position to the desired coordinate point for the trajectory tracking task. Additionally, a navigation method was implemented using attractive and repulsive artificial potential fields to carry out obstacle-Avoidance and goal-reaching tasks. The software was tested using simulations in Gazebo and the real AR. Drone. The drone's global position was estimated using an Extended Kalman Filter and visual landmarks. © 2015 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{OsvaldoEscobar201635,
author={Osvaldo Escobar, D. and M. Beatriz Bernábe, L. and López, A.S. and Rogelio González, V.},
title={Real time drone object tracking using histograms of oriented gradients and particle filters},
journal={Proceedings of a Special Session - 15th Mexican International Conference on Artificial Intelligence: Advances in Artificial Intelligence, MICAI 2016},
year={2016},
pages={35-40},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85117808320&doi=10.1109%2fMICAI-2016.2016.00014&partnerID=40&md5=c411ba245e1541122e12f079b165beed},
abstract={Unmanned Aerial Systems have various applications in the areas of military and surveillance. The use of computer vision as a sensory input provides an increased visual capacity which can be used by several robotic platforms to perform tasks. Its use can be found in the control and navigation of aerial vehicles, or for other forms of remote sensing. In this work, we present the development of a framework which is capable of developing an exact tracking of a person or an object and follow it autonomously. The tracking and following is performed without any help of GPS, only using the front monocular camera of the drone and the computation work is done by a laptop. © 2016 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Imamura2016333,
author={Imamura, Y. and Okamoto, S. and Lee, J.H.},
title={Human tracking by a multi-rotor drone using HOG features and linear SVM on images captured by a monocular camera},
journal={Lecture Notes in Engineering and Computer Science},
year={2016},
volume={1},
pages={333-338},
note={cited By 5},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84978696328&partnerID=40&md5=7dfa1069f232d8e9b94454cd047991bf},
abstract={In recent years, many researches of the drone (unmanned vehicles) have been carried out. Above all, the drone such as a multi-rotor craft might monitor and track suspicious person and find sufferers from disasters because it can move freely in the air. In the present research, a method was proposed that a multi-rotor drone can track a human by processing the two-dimensional images captured by a monocular camera installed on the multi-rotor drone. Furthermore, it can detect human without the differences of colors and movements of a target by using the Histograms of Oriented gradients (HOG) features and the linear Support Vector Machine (SVM). Then, it was shown that the multi-rotor drone could track a human by the proposed method.},
publisher={Newswood Limited},
}

@CONFERENCE{Busset2015,
author={Busset, J. and Perrodin, F. and Wellig, P. and Ott, B. and Heutschi, K. and Rühl, T. and Nussbaumer, T.},
title={Detection and tracking of drones using advanced acoustic cameras},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2015},
volume={9647},
art_number={96470F},
note={cited By 86},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84961631716&doi=10.1117%2f12.2194309&partnerID=40&md5=599adc7043b68e68e80e3f1aa3bc2a62},
abstract={Recent events of drones flying over city centers, official buildings and nuclear installations stressed the growing threat of uncontrolled drone proliferation and the lack of real countermeasure. Indeed, detecting and tracking them can be difficult with traditional techniques. A system to acoustically detect and track small moving objects, such as drones or ground robots, using acoustic cameras is presented. The described sensor, is completely passive, and composed of a 120-element microphone array and a video camera. The acoustic imaging algorithm determines in real-time the sound power level coming from all directions, using the phase of the sound signals. A tracking algorithm is then able to follow the sound sources. Additionally, a beamforming algorithm selectively extracts the sound coming from each tracked sound source. This extracted sound signal can be used to identify sound signatures and determine the type of object. The described techniques can detect and track any object that produces noise (engines, propellers, tires, etc). It is a good complementary approach to more traditional techniques such as (i) optical and infrared cameras, for which the object may only represent few pixels and may be hidden by the blooming of a bright background, and (ii) radar or other echo-localization techniques, suffering from the weakness of the echo signal coming back to the sensor. The distance of detection depends on the type (frequency range) and volume of the noise emitted by the object, and on the background noise of the environment. Detection range and resilience to background noise were tested in both, laboratory environments and outdoor conditions. It was determined that drones can be tracked up to 160 to 250 meters, depending on their type. Speech extraction was also experimentally investigated: the speech signal of a person being 80 to 100 meters away can be captured with acceptable speech intelligibility. © 2015 SPIE.},
publisher={SPIE},
}

@ARTICLE{Woods2015857,
author={Woods, A.C. and La, H.M.},
title={Dynamic target tracking and obstacle avoidance using a drone},
journal={Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
year={2015},
volume={9474},
pages={857-866},
note={cited By 18},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84952683975&doi=10.1007%2f978-3-319-27857-5_76&partnerID=40&md5=b12c2e90ebc664a23f3bf224b3879aec},
abstract={This paper focuses on tracking dynamic targets using a low cost, commercially available drone. The approach presented utilizes a computationally simple potential field controller expanded to operate not only on relative positions, but also relative velocities. A brief background on potential field methods is given, and the design and implementation of the proposed controller is presented. Experimental results using an external motion capture system for localization demonstrate the ability of the drone to track a dynamic target in real time as well as avoid obstacles in its way. © Springer International Publishing Switzerland 2015.},
publisher={Springer Verlag},
}

@CONFERENCE{Boudjit2015223,
author={Boudjit, K. and Larbes, C.},
title={Detection and implementation autonomous target tracking with a quadrotor AR.Drone},
journal={ICINCO 2015 - 12th International Conference on Informatics in Control, Automation and Robotics, Proceedings},
year={2015},
volume={2},
pages={223-230},
note={cited By 29},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84943547576&doi=10.5220%2f0005523102230230&partnerID=40&md5=422440ff8edc78dd06d6ff919e4e8145},
abstract={Nowadays, There Are Many Robotic Applications Being Developed to Do Tasks Autonomously without Any Interactions or Commands from Human, Therefore, Developing a System Which Enables a Robot to Do Surveillance Such as Detection and Tracking of a Moving Object Will Lead Us to More Advanced Tasks Carried out by Robots in the Future, AR.Drone Is a Flying Robot Platform That Is Able to Take Role as UAV (Unmanned Aerial Vehicle), Usage of Computer Vision Algorithm Such as Hough Transform Makes It Possible for Such System to Be Implemented on AR.Drone, in This Research, the Developed Algorithm Is Able to Detect and Track an Object with Certain Shape, then the Algorithm Is Successfully Implemented on AR.Drone Quadcopter for Detection and Tracking.},
publisher={SciTePress},
}

@ARTICLE{Prayitno2014819,
author={Prayitno, A. and Indrawati, V. and Utomo, G.},
title={Trajectory tracking of AR.Drone quadrotor using fuzzy logic controller},
journal={Telkomnika (Telecommunication Computing Electronics and Control)},
year={2014},
volume={12},
number={4},
pages={819-828},
note={cited By 20},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84923129981&doi=10.12928%2fTELKOMNIKA.v12i4.368&partnerID=40&md5=d83a90e296b8f7a46d4d3c0e03fddc48},
abstract={In this paper, Fuzzy Logic Controller (FLC) is implemented in the AR.Drone quadrotor in order to make it follow a given trajectory reference. The distance between the position and angle of the AR.Drone to the reference point is used as the input of the FLC. As for the output, pitch value and yaw rate will be the controlling signal for the AR.Drone. The navigation data of the AR.Drone are forward speed (vx), sideward speed (vy), and yaw. These navigation data are going to be used to estimate positions and orientation of the AR.Drone. To compensate for the y-position drift, the value of vy is also used as a criterion to determine the roll compensation. The FLC algorithm is implemented to AR.Drone 2.0 Elite Edition using LabVIEW software. Also, the algorithm has been tested in various trajectories such as a straight line, a straight line with a perpendicular turn, a rectangular trajectory and a curved trajectory. The results have shown that AR.Drone can follow a given trajectory with various initial positions and orientations quite well.},
publisher={Universitas Ahmad Dahlan},
}

@CONFERENCE{Santana2014756,
author={Santana, L.V. and Brandao, A.S. and Sarcinelli-Filho, M. and Carelli, R.},
title={A trajectory tracking and 3D positioning controller for the AR.Drone quadrotor},
journal={2014 International Conference on Unmanned Aircraft Systems, ICUAS 2014 - Conference Proceedings},
year={2014},
pages={756-767},
art_number={6842321},
note={cited By 66},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84904565652&doi=10.1109%2fICUAS.2014.6842321&partnerID=40&md5=346e3d905e3a4a870526657667142e16},
abstract={In this paper a complete framework is proposed, to deal with trajectory tracking and positioning with an AR.Drone Parrot quadrotor flying in indoor environments. The system runs in a centralized way, in a computer installed in a ground station, and is based on two main structures, namely a Kalman Filter (KF) to track the 3D position of the vehicle and a nonlinear controller to guide it in the accomplishment of its flight missions. The KF is designed aiming at estimating the states of the vehicle, fusing inertial and visual data. The nonlinear controller is designed with basis on a dynamic model of the AR.Drone, with the closed-loop stability proven using the theory of Lyapunov. Finally, experimental results are presented, which demonstrate the effectiveness of the proposed framework. © 2014 IEEE.},
publisher={IEEE Computer Society},
}

@CONFERENCE{Boddhu2013,
author={Boddhu, S.K. and McCartney, M. and Ceccopieri, O. and Williams, R.L.},
title={A collaborative smartphone sensing platform for detecting and tracking hostile drones},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2013},
volume={8742},
art_number={874211},
note={cited By 21},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84884136066&doi=10.1117%2f12.2014530&partnerID=40&md5=ea1ffec39d206ddfb31c60995fb7a388},
abstract={In recent years, not only United States Armed Services but other Law-enforcement agencies have shown increasing interest in employing drones for various surveillance and reconnaissance purposes. Further, recent advancements in autonomous drone control and navigation technology have tremendously increased the geographic extent of dronebased missions beyond the conventional line-of-sight coverage. Without any sophisticated requirement on data links to control them remotely (human-in-loop), drones are proving to be a reliable and effective means of securing personnel and soldiers operating in hostile environments. However, this autonomous breed of drones can potentially prove to be a significant threat when acquired by antisocial groups who wish to target property and life in urban settlements. To further escalate the issue, the standard detection techniques like RADARs, RF data link signature scanners, etc..., prove futile as the drones are smaller in size to evade successful detection by a RADAR based system in urban environment and being autonomous, have the capability of operating without a traceable active data link (RF). Hence, towards investigating possible practical solutions for the issue, the research team at AFRL's Tec^Edge Labs under SATE and YATE programs has developed a highly scalable, geographically distributable and easily deployable smartphone-based collaborative platform that can aid in detecting and tracking unidentified hostile drones. In its current state, this collaborative platform built on the paradigm of Human-as-Sensors, consists primarily of an intelligent Smartphone application that leverages appropriate sensors on the device to capture a drone's attributes (flight direction, orientation, shape, color, etc..,) with real-time collaboration capabilities through a highly composable sensor cloud and an intelligent processing module (based on a Probabilistic model) that can estimate and predict the possible flight path of a hostile drone based on multiple (geographically distributed) observation data points. This developed collaborative sensing platform has been field tested and proven to be effective in providing real-time alerting mechanism for the personnel in the field to avert or subdue the potential damages caused by the detected hostile drones. © 2013 SPIE.},
}

@CONFERENCE{Zorbas201380,
author={Zorbas, D. and Razafindralambo, T. and Luigi, D.P.P. and Guerriero, F.},
title={Energy efficient mobile target tracking using flying drones},
journal={Procedia Computer Science},
year={2013},
volume={19},
pages={80-87},
note={cited By 64},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84896927426&doi=10.1016%2fj.procs.2013.06.016&partnerID=40&md5=38c87585a459ab2132c1f389f4172671},
abstract={This paper focuses on the energy efficiency problem where camera equipped flying drones are able to detect and follow mobile events that happen on the ground. We give a mathematical formulation of the problem of minimizing the total energy consumption of a fleet of drones when coverage of all events is required. Due to the extremely high complexity of the binary optimization problem, the optimum solution cannot be obtained even for small instances. On the contrary, we present LAS, a localized solution for the aforementioned problem which takes into account the ability of the drones to fly at lower altitudes in order to conserve energy. We simulate LAS and we compare its performance to a centralized algorithm and to an approach that uses static drones to cover all the terrain. Our findings show that LAS performs similar to the centralized algorithm, while it outperforms the static approach by up to 150% in terms of consumed energy. Finally, the simulation results show that LAS is very sustainable in presence of communication errors. © 2013 The Authors. Published by Elsevier B.V.},
publisher={Elsevier B.V.},
}

@CONFERENCE{Dang2013146,
author={Dang, C.-T. and Pham, H.-T. and Pham, T.-B. and Truong, N.-V.},
title={Vision based ground object tracking using AR.Drone quadrotor},
journal={2013 International Conference on Control, Automation and Information Sciences, ICCAIS 2013},
year={2013},
pages={146-151},
art_number={6720545},
note={cited By 19},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84894136431&doi=10.1109%2fICCAIS.2013.6720545&partnerID=40&md5=4626e22ab76e84db8c55adbbe9ad6ae9},
abstract={This paper presents an approach to the ground object tracking problem of the low cost AR.Drone quadrotor via its integrated vision systems. It consists of three major components: (1) on-board vision based object detection and localization, (2) comprehensive empirical models of X-Y coordinate motion of the quad rotor and (3) closed-loop PD controllers on the ground station to generate steering commands via Wifi connection. The developed platform has been extensively validated in various testing environments, demonstrating its effectiveness. © 2013 IEEE.},
publisher={IEEE Computer Society},
}

@ARTICLE{Plaw2012344,
author={Plaw, A. and Fricker, M.S.},
title={Tracking the Predators: Evaluating the US Drone Campaign in Pakistan},
journal={International Studies Perspectives},
year={2012},
volume={13},
number={4},
pages={344-365},
note={cited By 15},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84868618646&doi=10.1111%2fj.1528-3585.2012.00465.x&partnerID=40&md5=c4fb1134e5d8a82569e90566b0e55085},
abstract={This article examines the strategic wisdom of the US Predator drone campaign in Pakistan, particularly in light of the dramatic expansion in the number of strikes that has occurred under the Obama administration. First, it examines whether there is a compelling rationale for any drone strikes in Pakistan by evaluating the justification advanced by US authorities and the three main criticisms that have been leveled against the campaign. With the help of an original database of drone strikes and their effects compiled by the authors of the article, it shows that the criticisms lack merit and that some strikes may be justified in principle. Second, it turns to the reasons explaining the dramatic increase in strikes over the past 2 years. On examination, it finds that the arguments supporting the expansion of the campaign are forceful but not necessarily decisive. In the third section it considers some objections to an expanded campaign. Finally, in the closing section, it weighs these considerations against the points favoring the expansion of the drone strikes. The article ends with the conclusion that on balance it would be prudent to shift back towards a more narrowly focused campaign concentrating on al-Qaeda, the Afghan Taliban and only leaders of the Pakistani Taliban. © 2012 International Studies Association.},
}

@CONFERENCE{Müller2011,
author={Müller, T. and Müller, M.},
title={Vision-based drone flight control and crowd or riot analysis with efficient color histogram based tracking},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2011},
volume={8020},
art_number={80200R},
note={cited By 6},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-80052724388&doi=10.1117%2f12.884213&partnerID=40&md5=c1d648ae3178070cbdaf69fe5b407fe0},
abstract={Object tracking is a direct or indirect key issue in many different military applications like visual surveillance, automatic visual closed-loop control of UAVs (unmanned aerial vehicles) and PTZ-cameras, or in the field of crowd evaluations in order to detect or analyse a riot emergence. Of course, a high robustness is the most important feature of the underlying tracker, but this is hindered significantly the more the tracker needs to have low calculation times. In the UAV application introduced in this paper the tracker has to be extraordinarily quick. In order to optimize the calculation time and the robustness in combination as far as possible, a highly efficient tracking procedure is presented for the above mentioned application fields which relies on well-known color histograms but uses them in a novel manner. This procedure bases on the calculation of a color weighting vector representing the significances of object colors like a kind of an object-s color finger print. Several examples from the above mentioned military applications are shown to demonstrate the practical relevance and the performance of the presented tracking approach. © 2011 SPIE.},
}

@CONFERENCE{Louvat2007154,
author={Louvat, B. and Bonnaud, L. and Marchand, N. and Bouvier, G.},
title={Tracking features with global motion compensation for drone camera servoing},
journal={Proceedings of IAPR Conference on Machine Vision Applications, MVA 2007},
year={2007},
pages={154-157},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84872541445&partnerID=40&md5=7f7532dd2f4d5533a60ab79f0a9da651},
abstract={This paper deals with visual servoing for a pan and tilt camera embedded in a drone. Video is transmitted to the ground where images are processed on a PC, and turret controls are sent back to the drone. The objective is to track any fixed object on the ground without knowledge about shape or texture and to keep it centered in the image. In order to achieve this task an algorithm that combines feature-based and global motion estimation is proposed. This algorithm provides a good robustness to very strong video transmission noise and works at a frame rate close to 25 fps. The control of the system is based on a double closed loop, which achieves a fast convergence to the desired position. Experimentation in real conditions shows the effectiveness of the proposed scheme.},
}

@CONFERENCE{Miller1990693,
author={Miller, James J. and Tannenholz, Philip H.},
title={Improved Drone tracking control system transponder},
journal={International Telemetering Conference (Proceedings)},
year={1990},
volume={26},
pages={693-702},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-0025636631&partnerID=40&md5=3c0f941328f495e974e190a5e182204c},
abstract={Improved performance has been achieved in the new Herley design of the Model MD700C-1 Drone Tracking and Control System, C-band Command and Control Transponder. The approach for obtaining better radio frequency rejection, automatic gain control, local oscillator stability, and power supply efficiency is described. New hybrid microwave integrated circuit application techniques were used to design a small local oscillator, tunable over the 5400 to 5900 MHz range with a frequency drift of less than ± 1 MHz. This low frequency drift allowed the use of a 4 pole immediate amplifier filter, 60 dB down, at 40 MHz bandwidth, which, when coupled with the three cavity radio frequency preselector filter, provides 7 pole out of band rejection for unwanted radar signals operating at close frequencies. To augment the out of band rejection, a new form of 75 dB dynamic range automatic gain control was used, which combines signal attenuation with a circuit that reduces immediate frequency noise with increasing signal. This allows rejection of the radars own in-band multipath signals by reducing the gain and threshold sensitivity. To reduce power consumption and heat while operating over a wide voltage range, a switching mode regulator and a non-saturating core power supply was designed to operate at 80% efficiency. Compared to units in field use over the past 10 years, the new design shows improvements of 400 percent in local oscillator frequency stability, 30 percent in out of band frequency rejection, 66 percent in the automatic gain control dynamic range, and 60 percent in power supply efficiency. The MD700C-1 was developed by Herley Industries for the USAF SMALC, and is currently in production.},
publisher={Publ by Int Foundation for Telemetering, Woodland Hills, CA, United States},
}


==> NewWork.tex <==
\section{UAV Detection and Tracking using Imaging} % 85 Paper

@ARTICLE{Wu201822,
	author={Wu, M. and Xie, W. and Shi, X. and Shao, P. and Shi, Z.},
	title={Real-time drone detection using deep learning approach},
	journal={Lecture Notes of the Institute for Computer Sciences, Social-Informatics and Telecommunications Engineering, LNICST},
	year={2018},
	volume={251},
	pages={22-32},
	note={cited By 8},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85055545933\&doi=10.1007\%2f978-3-030-00557-3_3\&partnerID=40\&md5=2058c0baff0488bd8fea647ad20060ec},
	abstract={The arbitrary use of drones poses great threat to public safety and personal privacy. It is necessary to detect the intruding drones in sensitive areas in real time. In this paper, we design a real-time drone detector using deep learning approach. Specifically, we improve a well-performed deep learning model, i.e., You Only Look Once, by modifying its structure and tuning its parameters to better accommodate drone detection. Considering that a robust detector needs to be trained using a large amount of training images, we also propose a semi-automatically dataset labelling method based on Kernelized Correlation Filters tracker to speed up the pre-processing of the training images. At last, the performance of our detector is verified via extensive experiments. © ICST Institute for Computer Sciences, Social Informatics and Telecommunications Engineering 2018.},
	publisher={Springer Verlag},
}

@CONFERENCE{Kim2018,
	author={Kim, B.H. and Khan, D. and Bohak, C. and Kim, J.K. and Choi, W. and Lee, H.J. and Kim, M.Y.},
	title={Ladar data generation fused with virtual targets and visualization for small drone detection system},
	journal={Proceedings of SPIE - The International Society for Optical Engineering},
	year={2018},
	volume={10797},
	art_number={107970I},
	note={cited By 4},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85056655170\&doi=10.1117\%2f12.2500525\&partnerID=40\&md5=22dd81a8a3b89ed919b212a546fc4926},
	abstract={For detection of a small target using electro-optical systems, multi-band 2D image sensors are used such as visible, NIR, MWIR, and LWIR. However, 2D imaging systems are not capable to detect a very small target and they are also not capable of calculating target 3D position coordinates to develop the strategic counter method. 3D sensors (e.g. Lidar, RGBD and stereo camera) are utilized to control unmanned vehicles for detecting threats and response for specific situations. Conventional Lidar systems are unable to detect small drone threat at distances higher than their maximum detecting range of 100 ?1/4 120 meters. To overcome this limitation, laser radar (LADAR) systems are being developed, which allow the detection at distances up to 2 kilometers. In the development of LADAR, it is difficult to acquire datasets that contain cases of long distant targets. In this study, a fusion data generation with virtual targets technique based on minimum real LADAR initial map dataset is proposed, and precise small target detection method using voxel-based clustering and classification are studied. We present the process of data fusion generation and the experimental results for a small target detection. The presented approach also includes effective visualization of high-resolution 3D data and the results of small target detection in real time. This study is expected to contribute to the optimization of a drone threat detection system for various environments and characteristics. © 2018 SPIE.},
	publisher={SPIE},
}

@CONFERENCE{Liu2018,
	author={Liu, H. and Qu, F. and Liu, Y. and Zhao, W. and Chen, Y.},
	title={A drone detection with aircraft classification based on a camera array},
	journal={IOP Conference Series: Materials Science and Engineering},
	year={2018},
	volume={322},
	number={5},
	art_number={052005},
	note={cited By 16},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85045847009\&doi=10.1088\%2f1757-899X\%2f322\%2f5\%2f052005\&partnerID=40\&md5=417f08c1de3726d3bd69a544aa54edf2},
	abstract={In recent years, because of the rapid popularity of drones, many people have begun to operate drones, bringing a range of security issues to sensitive areas such as airports and military locus. It is one of the important ways to solve these problems by realizing fine-grained classification and providing the fast and accurate detection of different models of drone. The main challenges of fine-grained classification are that: (1) there are various types of drones, and the models are more complex and diverse. (2) the recognition test is fast and accurate, in addition, the existing methods are not efficient. In this paper, we propose a fine-grained drone detection system based on the high resolution camera array. The system can quickly and accurately recognize the detection of fine grained drone based on hd camera. © Published under licence by IOP Publishing Ltd.},
	publisher={Institute of Physics Publishing},
}

@ARTICLE{Kim2018,
	author={Kim, B.H. and Khan, D. and Bohak, C. and Choi, W. and Lee, H.J. and Kim, M.Y.},
	title={V-RBNN based small drone detection in augmented datasets for 3D LADAR system},
	journal={Sensors (Switzerland)},
	year={2018},
	volume={18},
	number={11},
	art_number={3825},
	note={cited By 21},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85056406585\&doi=10.3390\%2fs18113825\&partnerID=40\&md5=887a7e1b43a17c38e28a51e75b3873d3},
	abstract={A common countermeasure to detect threatening drones is the electro-optical infrared (EO/IR) system. However, its performance is drastically reduced in conditions of complex background, saturation and light reflection. 3D laser sensor LiDAR is used to overcome the problems of 2D sensors like EO/IR, but it is not enough to detect small drones at a very long distance because of low laser energy and resolution. To solve this problem, A 3D LADAR sensor is under development. In this work, we study the detection methodology adequate to the LADAR sensor which can detect small drones at up to 2 km. First, a data augmentation method is proposed to generate a virtual target considering the laser beam and scanning characteristics, and to augment it with the actual LADAR sensor data for various kinds of tests before full hardware system developed. Second, a detection algorithm is proposed to detect drones using voxel-based background subtraction and variable radially bounded nearest neighbor (V-RBNN) method. The results show that 0.2 m L2 distance and 60\% expected average overlap (EAO) indexes are satisfied for the required specification to detect 0.3 m size of small drones. © 2018 by the authors. Licensee MDPI, Basel, Switzerland.},
	publisher={MDPI AG},
}

@CONFERENCE{Lee20181131,
	author={Lee, D.R. and Gyu La, W. and Kim, H.},
	title={Drone Detection and Identification System using Artificial Intelligence},
	journal={9th International Conference on Information and Communication Technology Convergence: ICT Convergence Powered by Smart Intelligence, ICTC 2018},
	year={2018},
	pages={1131-1133},
	art_number={8539442},
	note={cited By 21},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85059458820\&doi=10.1109\%2fICTC.2018.8539442\&partnerID=40\&md5=feec4d6dabc978442a05656332d845c6},
	abstract={As drone attracts much interest, the drone industry has opened their market to ordinary people, making drones to be used in daily lives. However, as it got easier for drone to be used by more people, safety and security issues have raised as accidents are much more likely to happen: colliding into people by losing control or invading secured properties. For safety purposes, it is essential for observers and drone to be aware of an approaching drone. In this paper, we introduce a comprehensive drone detection system based on machine learning. This system is designed to be operable on drones with camera. Based on the camera images, the system deduces location on image and vendor model of drone based on machine classification. The system is actually built with OpenCV library. We collected drone imagery and information for learning process. The system's output shows about 89 percent accuracy. © 2018 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Yi2019359,
	author={Yi, K.Y. and Kyeong, D. and Seo, K.},
	title={Deep learning based drone detection and classification},
	journal={Transactions of the Korean Institute of Electrical Engineers},
	year={2019},
	volume={68},
	number={2},
	pages={359-363},
	note={cited By 2},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85062906099\&doi=10.5370\%2fKIEE.2019.68.2.359\&partnerID=40\&md5=8a853f62f87ed98ed16975405409adab},
	abstract={As commercial drones have been widely used, concerns for collision accidents with people and invading secured properties are emerging. The detection of drone is a challenging problem. The deep learning based object detection techniques for detecting drones have been applied, but limited to the specific cases such as detection of drones from bird and/or background. We have tried not only detection of drones, but classification of different drones with an end-to-end model. YOLOv2 is used as an object detection model. In order to supplement insufficient data by shooting drones, data augmentation from collected images is executed. Also transfer learning from ImageNet for YOLOv2 darknet framework is performed. The experimental results for drone detection with average IoU and recall are compared and analysed. ? The Korean Institute of Electrical Engineers. Copyright ⓒ The Korean Institute of Electrical Engineers.},
	publisher={Korean Institute of Electrical Engineers},
}

@CONFERENCE{Wang2019433,
	author={Wang, Z. and Qi, L. and Tie, Y. and Ding, Y. and Bai, Y.},
	title={Drone Detection Based on FD-HOG Descriptor},
	journal={Proceedings - 2018 International Conference on Cyber-Enabled Distributed Computing and Knowledge Discovery, CyberC 2018},
	year={2019},
	pages={433-436},
	art_number={8644586},
	note={cited By 4},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85063145266\&doi=10.1109\%2fCyberC.2018.00084\&partnerID=40\&md5=6657d876de16f62325a32302b0076bdc},
	abstract={The rapid development of Unmanned Aerial Vehicle (UAV) technology, also known as drones, has made people benefit in many ways, but it also brings privacy and security issues, such as appeared at private place, airports, prisons, etc. Therefore, the detection of drones in a specific area is crucial. Video detection is an effective method with various advantages. In this paper, we have used the background subtraction method to detect the moving object in the video sequence which recorded by static cameras, then extracted the global Fourier descriptors and the local HOG features of the moving object images. Finally, the FD+HOG features have been sent to the SVM classifier for classification and recognition. Our algorithm is simple and efficient, an overall with 98\% accuracy was obtained in our data set. © 2018 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Jin2019,
	author={Jin, R. and Jiang, J. and Qi, Y. and Lin, D. and Song, T.},
	title={Drone detection and pose estimation using relational graph networks},
	journal={Sensors (Switzerland)},
	year={2019},
	volume={19},
	number={6},
	art_number={1479},
	note={cited By 15},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85063965882\&doi=10.3390\%2fs19061479\&partnerID=40\&md5=c9f6571e06a119bd5428eb77b196be7c},
	abstract={With the upsurge in use of Unmanned Aerial Vehicles (UAVs), drone detection and pose estimation by using optical sensors becomes an important research subject in cooperative flight and low-altitude security. The existing technology only obtains the position of the target UAV based on object detection methods. To achieve better adaptability and enhanced cooperative performance, the attitude information of the target drone becomes a key message to understand its state and intention, e.g., the acceleration of quadrotors. At present, most of the object 6D pose estimation algorithms depend on accurate pose annotation or a 3D target model, which costs a lot of human resource and is difficult to apply to non-cooperative targets. To overcome these problems, a quadrotor 6D pose estimation algorithm was proposed in this paper. It was based on keypoints detection (only need keypoints annotation), relational graph network and perspective-n-point (PnP) algorithm, which achieves state-of-the-art performance both in simulation and real scenario. In addition, the inference ability of our relational graph network to the keypoints of fourmotors was also evaluated. The accuracy and speed were improved significantly compared with the state-of-the-art keypoints detection algorithm. © 2019 by the authors. Licensee MDPI, Basel, Switzerland.},
	publisher={MDPI AG},
}

@CONFERENCE{Shinde2019289,
	author={Shinde, C. and Lima, R. and Das, K.},
	title={Multi-view Geometry and Deep Learning Based Drone Detection and Localization},
	journal={2019 5th Indian Control Conference, ICC 2019 - Proceedings},
	year={2019},
	pages={289-294},
	art_number={8715593},
	note={cited By 3},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85066635626\&doi=10.1109\%2fINDIANCC.2019.8715593\&partnerID=40\&md5=0f98338a93e57d4b1529b60ee355cb30},
	abstract={A real-time vision based detection and 3D pose estimation of intruder Unmanned Aerial Vehicles (UAVs) is presented. Proposed method utilizes a cooperative team of UAVs mounted with monocular camera to detect the intruder UAV and simultaneously localize it. Detection is performed by using YOLOv2 deep learning network architecture while the position is obtained using multi-view geometry. General dynamics of the drone are considered to improve the target position estimate obtained from the image based estimate. © 2019 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Hamatapa2019,
	author={Hamatapa, R. and Vongchumyen, C.},
	title={Image processing for drones detection},
	journal={Proceeding - 5th International Conference on Engineering, Applied Sciences and Technology, ICEAST 2019},
	year={2019},
	art_number={8802578},
	note={cited By 2},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85071731152\&doi=10.1109\%2fICEAST.2019.8802578\&partnerID=40\&md5=e9a3803c9d735e21a2246b3d9b9e5958},
	abstract={Presently, Drones Quadcopter has caused tremendous problems threatening the military security boundary and the area under Thai Army's surveillance. This article presents a conceptual framework for detecting and tracking unmanned aircraft by applying image processing. Study and analysis Compare advantages and disadvantages in order to develop and provide suitable equipment and tools Replacement of imported high-priced With limiting factors, namely distance, time, terrain And interference resistance The researchers used the camera USB 3.0 Cameras and Open Source Computer Vision (OpenCV) as a software development library on Linux operating systems to automatically record movies. In order to bring the image to analyze and distinguish the object classification by using Machine Learning through a sample of correct information and some incorrect information. Which when detecting, the installed device will calculate the coordinates detected, lock the target, track the movement Voice notification and report. The experiment was conducted by using Anova to test various factors affecting the detection, such as speed, light, color and size in 350 feet with the equipment we installed. The results of the experiment concluded that there was only a speed that had an effect at 22.65. © 2019 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Abbasi2019,
	author={Abbasi, K. and Batool, A. and Fawad and Asghar, M.A. and Saeed, A. and Khan, M.J. and Ur Rehman, M.},
	title={A Vision-Based Amateur Drone Detection Algorithm for Public Safety Applications},
	journal={2019 UK/China Emerging Technologies, UCET 2019},
	year={2019},
	art_number={8881879},
	note={cited By 3},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85074919038\&doi=10.1109\%2fUCET.2019.8881879\&partnerID=40\&md5=43bd2d5d5e074a9d9c8d33c0bb6e0453},
	abstract={Drones will be widely used in the smart cities of the future for the wireless approach, supplying goods, and for conserving the security of smart cities. Apart from the various benefits of the drones, they pose significant challenges and public concerns that need to be tackled. We propose an amenable framework to detect malicious drone and ensure public safety. The proposed model is validated using 400 images with various challenges such as occlusion, scale variation, blurriness, background clutter, and low illumination. After extracting the features using ResNet50 model, we applied SVM's RBF kernel for the classification. The classification accuracy presented in the confusion matrix for this model came out to be the highest in comparison to other state-of-the-art models. © 2019 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Nalamati2019,
	author={Nalamati, M. and Kapoor, A. and Saqib, M. and Sharma, N. and Blumenstein, M.},
	title={Drone detection in long-range surveillance videos},
	journal={2019 16th IEEE International Conference on Advanced Video and Signal Based Surveillance, AVSS 2019},
	year={2019},
	art_number={8909830},
	note={cited By 19},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85074766085\&doi=10.1109\%2fAVSS.2019.8909830\&partnerID=40\&md5=43cc8abf956394d22103009723198283},
	abstract={The usage of small drones/UAVs has significantly increased recently. Consequently, there is a rising potential of small drones being misused for illegal activities such as terrorism, smuggling of drugs, etc. posing high-security risks. Hence, tracking and surveillance of drones are essential to prevent security breaches. The similarity in the appearance of small drone and birds in complex background makes it challenging to detect drones in surveillance videos. This paper addresses the challenge of detecting small drones in surveillance videos using popular and advanced deep learning-based object detection methods. Different CNN-based architectures such as ResNet-101 and Inception with Faster-RCNN, as well as Single Shot Detector (SSD) model was used for experiments. Due to sparse data available for experiments, pre-trained models were used while training the CNNs using transfer learning. Best results were obtained from experiments using Faster-RCNN with the base architecture of ResNet-101. Experimental analysis on different CNN architectures is presented in the paper, along with the visual analysis of the test dataset. © 2019 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

{\color{red}
@CONFERENCE{Sheikh2019,
	author={Sheikh, M.U. and Ghavimi, F. and Ruttik, K. and Jantti, R.},
	title={Drone detection and classification using cellular network: A machine learning approach},
	journal={IEEE Vehicular Technology Conference},
	year={2019},
	volume={2019-September},
	art_number={8891229},
	note={cited By 3},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85075244234\&doi=10.1109\%2fVTCFall.2019.8891229\&partnerID=40\&md5=7fcc3eb754086277879cb9d6750ba7f5},
	abstract={The main target of this paper is to propose a preferred set of features from a cellular network for using as predictors to do the classification between the rogue flying drone User Equipments (UEs) and regular UEs for different Machine Learning (ML) models. Furthermore, the target is to study four different machine learning models i.e. Decision Tree (DT), Logistic Regression (LR). Discriminant Analysis (DA) and K-Nearest Neighbour (KNN) in this paper, and evaluate/compare their performance in terms of identifying the flying drone UE using three performance metrics i.e. True Positive Rate (TPR), False Positive Rate (FPR) and area under Receiver Operating Characteristic (ROC) curve. The simulations are performed using an agreed 3GPP scenario, and a MATLAB machine learning tool box. All considered ML models provide high drone detection probability for drones flying at 60 m and above height. However, the true drone detection probability degrades for drones at lower altitude. Whereas, the fine DT method and the coarse KNN model performs relatively better compared with LR and DA at low altitude, and therefore can be considered as a preferable choice for a drone classification problem. © 2019 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}}

@ARTICLE{Sun2020130697,
	author={Sun, H. and Yang, J. and Shen, J. and Liang, D. and Ning-Zhong, L. and Zhou, H.},
	title={TIB-Net: Drone Detection Network with Tiny Iterative Backbone},
	journal={IEEE Access},
	year={2020},
	volume={8},
	pages={130697-130707},
	art_number={9141228},
	note={cited By 4},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85089524311\&doi=10.1109\%2fACCESS.2020.3009518\&partnerID=40\&md5=91412e44e3c84ea850ec66db0c85ab03},
	abstract={With the widespread application of drone in commercial and industrial fields, drone detection has received increasing attention in public safety and others. However, due to various appearance of small-size drones, changeable and complex environments, and limited memory resources of edge computing devices, drone detection remains a challenging task nowadays. Although deep convolutional neural network (CNN) has shown powerful performance in object detection in recent years, most existing CNN-based methods cannot balance detection performance and model size well. To solve the problem, we develop a drone detection network with tiny iterative backbone named TIB-Net. In this network, we propose a structure called cyclic pathway, which enhances the capability to extract effective features of small object, and integrate it into existing efficient method Extremely Tiny Face Detector (EXTD). This method not only significantly improves the accuracy of drone detection, but also keeps the model size at an acceptable level. Furthermore, we integrate spatial attention module into our network backbone to emphasize information of small object, which can better locate small-size drone and further improve detection performance. In addition, we present massive manual annotations of object bounding boxes for our collected 2860 drone images as a drone benchmark dataset, which is now publicly available1. In this work, we conduct a series of experiments on our collected dataset to evaluate TIB-Net, and the result shows that our proposed method achieves mean average precision of 89.2\% with model size of 697.0KB, which achieves the state-of-the-art results compared with existing methods. © 2013 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Pham20202965,
	author={Pham, G.N. and Nguyen, P.H.},
	title={Drone detection experiment based on image processing and machine learning},
	journal={International Journal of Scientific and Technology Research},
	year={2020},
	volume={9},
	number={2},
	pages={2965-2971},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85079555266\&partnerID=40\&md5=befa3b02c6a14ea30350625da119967b},
	abstract={Drones are widely used in the field of information gathering and tracking, even they could be used to attacked targets. Therefore, the drone detection for the restricted areas or special zones is important and necessary. This paper focuses on the drone detection problem based on image processing for the restricted areas or special zones where used cameras for monitoring. The proposed solution detects drones from the captured images based on training the Haar-like features. The dataset of drone images is used in the Haar training process to generate a Haar-cascade model of drones. This model is then used to detect drones from images captured by the camera. The proposed solution is implemented and experimented with single cameras installed for any place including indoor environment and outdoor environment. Experimental results proved that the proposed solution could exactly detect drones for any zone or the restricted areas. The average accuracy of the proposed solution in the experimented environments is 91.9 \%, and it provides an easy and economical solution for user. IJSTR © 2020.},
	publisher={International Journal of Scientific and Technology Research},
}

@ARTICLE{Chen202081,
	author={Chen, H. and Wang, Z. and Zhang, L.},
	title={Collaborative spectrum sensing for illegal drone detection: A deep learning-based image classification perspective},
	journal={China Communications},
	year={2020},
	volume={17},
	number={2},
	pages={81-92},
	art_number={9020299},
	note={cited By 3},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85081655115\&doi=10.23919\%2fJCC.2020.02.007\&partnerID=40\&md5=398ce42462246b681ca5a7ad25d1cd4f},
	abstract={Drones, also known as mini-unmanned aerial vehicles (UAVs), are enjoying great popularity in recent years due to their advantages of low cost, easy to pilot and small size, which also makes them hard to detect. They can provide real time situational awareness information by live videos or high definition pictures and pose serious threats to public security. In this article, we combine collaborative spectrum sensing with deep learning to effectively detect potential illegal drones with states of high uncertainty. First, we formulate the detection of potential illegal drones under illegitimate access and rogue power emission as a quaternary hypothesis test problem. Then, we propose an algorithm of image classification based on convolutional neural network which converts the cooperative spectrum sensing data at a sensing slot into one image. Furthermore, to exploit more information and improve the detection performance, we develop a trajectory classification algorithm which converts the flight process of the drones in consecutive multiple sensing slots into trajectory images. In addition, simulations are provided to verify the proposed methods' performance under various parameter configurations. © 2013 China Institute of Communications.},
	publisher={Editorial Department of China Communications},
}

@ARTICLE{Kavitha20201366,
	author={Kavitha, T. and Lakshmi, K.},
	title={A drone detection system for preventing security threats using YOLO deep learning network},
	journal={International Journal of Advanced Science and Technology},
	year={2020},
	volume={29},
	number={5 Special Issue},
	pages={1366-1376},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85083963617\&partnerID=40\&md5=d0d66ad26522be4084a5745f16b1331c},
	abstract={There has been a tremendous increase of use of UAVs or drones in the recent years. It is used in many fields such as aerial photography, shipping and delivery, crowd monitoring, crop monitoring in agriculture, law enforcement and surveillance etc. The cost of these devices become very low and makes it highly accessible to common public. It also increases the work efficiency and accuracy. Sometimes these drones are used for capturing information from secured areas by trespassing. This has raised several security concerns. In order to protect privacy and security at important locations, several solutions have been proposed in recent years. The drones are detected by using radio frequencies, acoustic waves, optic sensors and radars but they have certain limitations. Hence, this paper focuses on deep learning-based computer vision technique for detecting drones. To eradicate such security threats, the existing techniques for drone detection have been analyzed and designed a robust system based on You Only Look Once (YOLO) object detection algorithm. The YOLO based drone detection system performed well and produced results better than the other compared system. © 2020 SERSC.},
	publisher={Science and Engineering Research Support Society},
}

@CONFERENCE{Behera20201012,
	author={Behera, D.K. and Raj, A.B.},
	title={Drone Detection and Classification using Deep Learning},
	journal={Proceedings of the International Conference on Intelligent Computing and Control Systems, ICICCS 2020},
	year={2020},
	pages={1012-1016},
	art_number={9121150},
	note={cited By 19},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85087452192\&doi=10.1109\%2fICICCS48265.2020.9121150\&partnerID=40\&md5=3cad9228db1498f00868540b706f8666},
	abstract={This paper presents a systematic approach to drone detection and classification using deep learning with different modalities. The YOLOv3 object detector is used to detect the moving or still objects. It uses a computer vision-based approach as a reliable solution. The convolutional neural network helps to extract features from images and to detect the object with maximum accuracy. The model is trained with a proper dataset and trained for 150 epoch only to detect various types of drones. A convolutional neural network with modern object detection methods shows an excellent approach for real-time detection of drones. © 2020 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Koksal20204439,
	author={Koksal, A. and Ince, K.G. and Aydin Alatan, A.},
	title={Effect of annotation errors on drone detection with YOLOv3},
	journal={IEEE Computer Society Conference on Computer Vision and Pattern Recognition Workshops},
	year={2020},
	volume={2020-June},
	pages={4439-4447},
	art_number={9150631},
	note={cited By 4},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85090130528\&doi=10.1109\%2fCVPRW50498.2020.00523\&partnerID=40\&md5=4bbfa5146b65be1e440f91019f2f94bd},
	abstract={Following the recent advances in deep networks, object detection and tracking algorithms with deep learning backbones have been improved significantly; however, this rapid development resulted in the necessity of large amounts of annotated labels. Even if the details of such semi-automatic annotation processes for most of these datasets are not known precisely, especially for the video annotations, some automated labeling processes are usually employed. Unfortunately, such approaches might result with erroneous annotations. In this work, different types of annotation errors for object detection problem are simulated and the performance of a popular state-of-the-art object detector, YOLOv3, with erroneous annotations during training and testing stages is examined. Moreover, some inevitable annotation errors in Anti-UAV Challenge dataset is also examined in this manner, while proposing a solution to correct such annotation errors of this valuable data set. © 2020 IEEE.},
	publisher={IEEE Computer Society},
}

@ARTICLE{Seidaliyeva20201,
	author={Seidaliyeva, U. and Akhmetov, D. and Ilipbayeva, L. and Matson, E.T.},
	title={Real-time and accurate drone detection in a video with a static background},
	journal={Sensors (Switzerland)},
	year={2020},
	volume={20},
	number={14},
	pages={1-18},
	art_number={3856},
	note={cited By 20},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85087622606\&doi=10.3390\%2fs20143856\&partnerID=40\&md5=4056a8e6bd2c26d89290db38a268ac5e},
	abstract={With the increasing number of drones, the danger of their illegal use has become relevant. This has necessitated the creation of automatic drone protection systems. One of the important tasks solved by these systems is the reliable detection of drones near guarded objects. This problem can be solved using various methods. From the point of view of the price–quality ratio, the use of video cameras for a drone detection is of great interest. However, drone detection using visual information is hampered by the large similarity of drones to other objects, such as birds or airplanes. In addition, drones can reach very high speeds, so detection should be done in real time. This paper addresses the problem of real-time drone detection with high accuracy. We divided the drone detection task into two separate tasks: the detection of moving objects and the classification of the detected object into drone, bird, and background. The moving object detection is based on background subtraction, while classification is performed using a convolutional neural network (CNN). The experimental results showed that the proposed approach can achieve an accuracy comparable to existing approaches at high processing speed. We also concluded that the main limitation of our detector is the dependence of its performance on the presence of a moving background. © 2020 by the authors. Licensee MDPI, Basel, Switzerland.},
	publisher={MDPI AG},
}

@ARTICLE{Demir20201625,
	author={Demir, B. and Ergunay, S. and Nurlu, G. and Popovic, V. and Ott, B. and Wellig, P. and Thiran, J.-P. and Leblebici, Y.},
	title={Real-time high-resolution omnidirectional imaging platform for drone detection and tracking},
	journal={Journal of Real-Time Image Processing},
	year={2020},
	volume={17},
	number={5},
	pages={1625-1635},
	note={cited By 2},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85074700180\&doi=10.1007\%2fs11554-019-00921-7\&partnerID=40\&md5=ca09300a973af4909bdf83c5d8857a02},
	abstract={Drones have become steadily affordable, which raises privacy and security concerns as well as interest in drone detection systems. On the other hand, drone detection is a challenging task due to small dimensions of drones, difficulty of long-distance detection, strict real-time constraints and necessity of wide angle coverage for drones. Although different radar and audio-assisted drone detection systems have been presented, they suffer from the cost, range, or interference problems. On the contrary, a long-range detection can be obtained by a vision-based system. Aiming that, we propose a real-time moving object detection and tracking system optimized for drone detection using 16 cameras with 20 MP resolution. The proposed system detects drones from short range and long range with 360∘ surveillance coverage owing high-performance ultra-high-resolution (320 MP) video-processing capability. It is able to detect drones with 100 cm diameter from 700 m distance despite deceptive background. It is interference free, so multiple systems can properly operate in the vicinity without effecting each other. It integrates processing power of embedded systems with flexibility of software to generate a full platform for drone detection and tracking. © 2019, Springer-Verlag GmbH Germany, part of Springer Nature.},
	publisher={Springer},
}


@CONFERENCE{Garcia2020559,
	author={Garcia, A.J. and Min Lee, J. and Kim, D.S.},
	title={Anti-Drone System: A Visual-based Drone Detection using Neural Networks},
	journal={International Conference on ICT Convergence},
	year={2020},
	volume={2020-October},
	pages={559-561},
	art_number={9289397},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85098963671\&doi=10.1109\%2fICTC49870.2020.9289397\&partnerID=40\&md5=854abf6e0d43829f248c90f0afe7dd19},
	abstract={A system that secures an area from trespassing drones that might bring threat is in demand these days since drones became easily-available to the public and it became easier to operate. This paper proposes an anti-drone system that uses visual sensing to detect drones. A Faster R-CNN (Region-based Convolutional Neural Network) with ResNet-101 (Residual Neural Network-101) networks are used in this paper using a dataset from the SafeShore project. The network's accuracy is 93.40\% and it has successfully detected drones in the simulation that has been done. © 2020 IEEE.},
	publisher={IEEE Computer Society},
}

@CONFERENCE{Pratt2020,
	author={Pratt, H. and Evans, B. and Rowntree, T. and Reid, I. and Wiederman, S.},
	title={Recurrent Motion Neural Network for Low Resolution Drone Detection},
	journal={2020 Digital Image Computing: Techniques and Applications, DICTA 2020},
	year={2020},
	art_number={9363377},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85102653283\&doi=10.1109\%2fDICTA51227.2020.9363377\&partnerID=40\&md5=2272ec353a4a0a6cab913bf5e8365237},
	abstract={Drones are becoming increasingly prevalent in everyday usage with many commercial applications in fields such as construction work and agricultural surveying. Despite their common commercial use, drones have been recently used with malicious intent, such as airline disruptions at Gatwick Airport. With the emerging issue of safety concerns for the public and other airspace users, detecting and monitoring active drones in an area is crucial. This paper introduces a recurrent convolutional neural network (CNN) specifically designed for drone detection. This CNN can detect drones from down-sampled images by exploiting the temporal information of drones in flight and outperforms a state-of-the-art conventional object detector. Due to the lightweight and low resolution nature of this network, it can be mounted on a small processor and run at near real-time speeds. © 2020 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Yi2020204,
	author={Yi, J. and Srigrarom, S.},
	title={Near-Parallel Binocular-Like Camera Pair for Multi-Drone Detection and 3D Localization},
	journal={16th IEEE International Conference on Control, Automation, Robotics and Vision, ICARCV 2020},
	year={2020},
	pages={204-210},
	art_number={9305485},
	note={cited By 1},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85100087134\&doi=10.1109\%2fICARCV50220.2020.9305485\&partnerID=40\&md5=2d5c3192bef36c9f25b0e50af0df02ed},
	abstract={The paper presents the concept of using a pair of cameras that are setup near and almost parallel to each other to do detection and 3D localization of multiple drone at far distance away. These setup of the two cameras resemble the binocular cameras, as such the 3D positions of the detected drones can be estimated by epipolar-like geometry. For the special case of detecting the multiple drones at a distance, quick depth distance approximation based on similar triangles is also proposed. Sample field tests of detecting and tracking multiple drones at near and far distances in open areas are presented. The depth distances obtained are comparable to the actual GPS readings from the detected drones. © 2020 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Mahdavi2020,
	author={Mahdavi, F. and Rajabi, R.},
	title={Drone Detection Using Convolutional Neural Networks},
	journal={6th Iranian Conference on Signal Processing and Intelligent Systems, ICSPIS 2020},
	year={2020},
	art_number={9349620},
	note={cited By 1},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85101770647\&doi=10.1109\%2fICSPIS51611.2020.9349620\&partnerID=40\&md5=b7172620cf89b63aad73c0e7831801ed},
	abstract={In image processing, it is essential to detect and track air targets, especially UAVs. In this paper, we detect the flying drone using a fisheye camera. In the field of diagnosis and classification of objects, there are always many problems that prevent the development of rapid and significant progress in this area. During the previous decades, a couple of advanced classification methods such as convolutional neural networks and support vector machines have been developed. In this study, the drone was detected using three methods of classification of convolutional neural network (CNN), support vector machine (SVM), and nearest neighbor. The outcomes show that CNN, SVM, and nearest neighbor have total accuracy of 93\%, 88\%, and 80\%, respectively. Compared with other classifiers with the same experimental conditions, the accuracy of the convolutional neural network classifier is satisfactory. © 2020 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Sun20204795,
	author={Sun, H. and Geng, W. and Shen, J. and Liu, N. and Liang, D. and Zhou, H.},
	title={Deeper SSD: Simultaneous up-sampling and down-sampling for drone detection},
	journal={KSII Transactions on Internet and Information Systems},
	year={2020},
	volume={14},
	number={12},
	pages={4795-4815},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85099333280\&doi=10.3837\%2ftiis.2020.12.010\&partnerID=40\&md5=3a7b7a1b480f9c90008bc4f04bd09985},
	abstract={Drone detection can be considered as a specific sort of small object detection, which has always been a challenge because of its small size and few features. For improving the detection rate of drones, we design a Deeper SSD network, which uses large-scale input image and deeper convolutional network to obtain more features that benefit small object classification. At the same time, in order to improve object classification performance, we implemented the up-sampling modules to increase the number of features for the low-level feature map. In addition, in order to improve object location performance, we adopted the down-sampling modules so that the context information can be used by the high-level feature map directly. Our proposed Deeper SSD and its variants are successfully applied to the self-designed drone datasets. Our experiments demonstrate the effectiveness of the Deeper SSD and its variants, which are useful to small drone's detection and recognition. These proposed methods can also detect small and large objects simultaneously. © 2020 KSII},
	publisher={Korean Society for Internet Information},
}

@ARTICLE{Sharjeel2021128,
	author={Sharjeel, A. and Naqvi, S.A.Z. and Ahsan, M.},
	title={Real time drone detection by moving camera using COROLA and CNN algorithm},
	journal={Journal of the Chinese Institute of Engineers, Transactions of the Chinese Institute of Engineers,Series A},
	year={2021},
	volume={44},
	number={2},
	pages={128-137},
	note={cited By 1},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85099420933\&doi=10.1080\%2f02533839.2020.1856725\&partnerID=40\&md5=727cd024352f7084218052edb2ac4333},
	abstract={Widespread and careless use of unmanned aerial vehicles, such as drones, often raises serious privacy and security issues. To some extent, timely and accurate detection of drones enables observers to counteract unwarranted intrusion and other forms of their misuse. This is not an easy task, however, drones, on one hand, being small in size, are difficult to spot in general. On the other hand, they fly at low altitudes and against a background containing several look-alike objects. In this work, a hybrid approach for the detection of drones by the moving spy drone camera is presented which combines Contiguous Outlier Representation via Online Low-rank Approximation (COROLA) and Convolutional Neural Network (CNN). The COROLA technique is used for detecting a small moving object present in a scene and the CNN algorithm is employed for accurate drone recognition in a wide array of complex backgrounds. This hybrid technique is robust and time-efficient as it obviates full processing of the entire image sequence. To demonstrate the effectiveness of our proposed approach, we have compared its performance with R-STIC (Regression on Spatial-Temporal Image Cube), a state-of-the-art detection method, under different real-life scenarios. The obtained results show that the proposed hybrid approach is better than R-STIC, in terms of computational efficiency, accuracy, and robustness. © 2020 The Chinese Institute of Engineers.},
	publisher={Taylor and Francis Ltd.},
}

@CONFERENCE{Shuhaywin20214220,
	author={Shuhaywin, A.B. and Almeshkhas, F. and Mejjaouli, S.},
	title={Establishing drone detection system by using deep learning and YOLOv3 formatting},
	journal={Proceedings of the International Conference on Industrial Engineering and Operations Management},
	year={2021},
	pages={4220-4230},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85114264350\&partnerID=40\&md5=2220debaca7e78742b8530b73aa5655b},
	abstract={Using a machine-vision detection based on deep learning system, the study established using darknet framework to identify and making the drone detection system. Using the darknet, YOLOv3 algorithm and OpenCV, the system was implemented on our computer to identify drones based on the live feed obtained from camera or uploaded image. The system was implemented to track and recognize drones on a different background. The project methodology is based on four different stages, gathering the dataset, annotation, training the system and testing the system. The project was able to identify the drones with an average success rate of 99\% and 100\% from live videos and uploaded images, respectively. The project showed that because of the deep learning strength, the detection was robust against changes in light intensity and the existence of background effects in different environmental conditions. © IEOM Society International.},
	publisher={IEOM Society},
}

@CONFERENCE{Phung2021189,
	author={Phung, K.-P. and Lu, T.-H. and Nguyen, T.-T. and Le, N.-L. and Nguyen, H.-H. and Hoang, V.-P.},
	title={Multi-model Deep Learning Drone Detection and Tracking in Complex Background Conditions},
	journal={International Conference on Advanced Technologies for Communications},
	year={2021},
	volume={2021-October},
	pages={189-194},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85122942707\&doi=10.1109\%2fATC52653.2021.9598317\&partnerID=40\&md5=1efcc3b7b42865ce80289e93f937799d},
	abstract={The recent popularity of drones with quadcopter layouts is threatening public safety and personal privacy. With the ability to hover and perform complex maneuvers even in indoor conditions, equipped with video cameras as well as capable of carrying hazardous materials, drones can truly become a security threat, especially to vulnerable organizations. Therefore, detecting and tracking drones in secured areas poses an urgent task for the surveillance system. In this paper, we design a real-time drone detection and tracking system with the combination of multiple deep learning and computer vision techniques: 1) Yolo-v4 model for detecting drones and 2) visual models for tracking drones. Besides, we have collected and labeled a larger drone dataset by mixing the existing datasets with our collected images. We evaluated three deep learning models for drone detection on this dataset and acquired the Yolo-V4 model to be the highest detection performance with AP = 34.63\%. Combining this detection model and the existing visual tracking modules can boost the drone tracking up to more than 20fps for different backgrounds at around 700m by using an usual PC without GPU. © 2021 IEEE.},
	publisher={IEEE Computer Society},
}

@CONFERENCE{Suh2021,
	author={Suh, H.-S. and Meng, J. and Nguyen, T. and Venkataramanaiah, S.K. and Kumar, V. and Cao, Y. and Seo, J.-S.},
	title={Algorithm-Hardware Co-Optimization for Energy-Efficient Drone Detection on Resource-Constrained FPGA},
	journal={2021 International Conference on Field-Programmable Technology, ICFPT 2021},
	year={2021},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85123165019\&doi=10.1109\%2fICFPT52863.2021.9609840\&partnerID=40\&md5=37404b2e370f0265457ab580d1bd5a3f},
	abstract={Convolutional neural network (CNN) based object detection has achieved very high accuracy, e.g. single-shot multi-box detectors (SSD) can efficiently detect and localize various objects in an input image. However, they require a high amount of computation and memory storage, which makes it difficult to perform efficient inference on resource-constrained hardware devices such as drones or unmanned aerial vehicles (UAVs). Drone/UAV detection is an important task for applications including surveillance, defense, and multi-drone self-localization and formation control. In this paper, we designed and co-optimized algorithm and hardware for energy-efficient drone detection on resource-constrained FPGA devices. We trained SSD object detection algorithm with a custom drone dataset. For inference, we employed low-precision quantization and adapted the width of the SSD CNN model. To improve throughput, we use dual-data rate operations for DSPs to effectively double the throughput with limited DSP counts. For different SSD algorithm models, we analyze accuracy or mean average precision (mAP) and evaluate the corresponding FPGA hardware utilization, DRAM communication, throughput optimization. Our proposed design achieves a high mAP of 88.42\% on the multi-drone dataset, with a high energy-efficiency of 79 GOPS/W and throughput of 158 GOPS using Xilinx Zynq ZU3EG FPGA device on the Open Vision Computer version 3 (OVC3) platform. Our design achieves 2.7X higher energy efficiency than prior works using the same FPGA device, at a low-power consumption of 1.98 W. © 2021 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Topalli2021,
	author={Topalli, M.T. and Yilmaz, M. and Corapsiz, M.F.},
	title={Real Time Implementation of Drone Detection using TensorFlow and MobileNetV2-SSD},
	journal={7th International Conference on Electrical, Electronics and Information Engineering: Technological Breakthrough for Greater New Life, ICEEIE 2021},
	year={2021},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85123580383\&doi=10.1109\%2fICEEIE52663.2021.9616846\&partnerID=40\&md5=667de7e16166a4af25044a388c84f974},
	abstract={Drones are Unmanned Aerial Vehicles (UAV) that can be controlled by remote control or software methods. In recent years with the developing technology, drones have started to be used in all areas of our lives. The two most important factors that make drones attractive to use are low price and easy control. Today, UAVs, which provide convenience to people in many fields such as photography, video shooting, advertising, firefighting and search-rescue activities. Also, UAV is used by terrorist organizations in attack actions. Anti-drone systems are used to detect and locate such malicious drones. In this study, a prototype drone detection system called ATA-DRN is designed against drone threats. While creating ATA-DRN, 2 digital servo motors, Raspberry Pi 4 development board, high resolution Web Cam, 7inch HDMI LCD and power supply is used. With this designed system, drone approaching to the target is automatically detected with image processing methods without the need for manpower. In the study, first of all, a data set is obtained from pictures of different types of drones. The data set obtained is divided into two groups as train (80\%) and test (20\%) in order to train. The model to be used in real-time drone analysis is obtained using TensorFlow and MobileNetV2-SSD. Experiments are carried out by transferring the obtained model to the Raspberry Pi 4 development board. The accuracy of the model created as a result of experimental studies has been proven. © 2021 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Alsoliman2021166,
	author={Alsoliman, A. and Rigoni, G. and Levorato, M. and Pinotti, C. and Tippenhauer, N.O. and Conti, M.},
	title={COTS Drone Detection using Video Streaming Characteristics},
	journal={ACM International Conference Proceeding Series},
	year={2021},
	pages={166-175},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85098731548\&doi=10.1145\%2f3427796.3428480\&partnerID=40\&md5=6fa92f45d9f9e4e3b3ff9a96bc8068c3},
	abstract={Cheap commercial off-the-shelf (COTS) drones have become widely available for consumers in recent years. Unfortunately, they also provide low-cost capabilities for attackers. Therefore, effective methods to detect the presence of non-cooperating rogue drones within a restricted area are highly required. Approaches based on detection of control traffic have been proposed but were not yet shown to work against other benign traffic, such as that generated by wireless security cameras. In this work, we propose a novel drone detection framework based on a Random Forest classification model. In essence, the framework leverages specific patterns in video traffic transmitted by drones. The patterns consist of repetitive synchronization packets (denoted as pivots) which we use as features in the proposed machine learning classifier. We show that our framework can achieve up to 99\% detection accuracy over an encrypted WiFi channel using only 20 packets originated from the drone. Our system is able to identify drone transmissions even among very similar WiFi transmission (such as a security camera video stream) and in a noisy scenario with background traffic. © 2021 ACM.},
	publisher={Association for Computing Machinery},
}

@CONFERENCE{WeiXun2021,
	author={Wei Xun, D.T. and Lim, Y.L. and Srigrarom, S.},
	title={Drone detection using YOLOv3 with transfer learning on NVIDIA Jetson TX2},
	journal={2021 2nd International Symposium on Instrumentation, Control, Artificial Intelligence, and Robotics, ICA-SYMP 2021},
	year={2021},
	art_number={9358449},
	note={cited By 3},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85102488569\&doi=10.1109\%2fICA-SYMP50206.2021.9358449\&partnerID=40\&md5=ae6ad5ae58b864696f708b4e20c4432b},
	abstract={The rise of drones in the recent years largely due to the advancements of drone technology which provide drones the ability to perform many more complex tasks autonomously with the incorporation of technologies such as computer vision, object avoidance and artificial intelligence. However, the misuse of drones such as the Gatwick Airport drone incident resulted in major disruptions which affected approximately 140,000 passengers. To deter this from happening in the future, drone surveillance are extremely crucial. With this, it will be achieved firstly by detection and followed by tracking of drones. This paper presents and investigates the use of a deep learning object detector, YOLOv3 with pretrained weights and transfer learning to train YOLOv3 to specifically detect drones. We demonstrated that the detection results from YOLOv3 after machine learning had an average accuracy of 88.9\% at input image size of 416 × 416. Finally, we integrated into NVIDIA Jetson TX2 for real-time drone detection. © 2021 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Srigrarom2021,
	author={Srigrarom, S. and Sie, N.J.L. and Cheng, H. and Chew, K.H. and Lee, M. and Ratsamee, P.},
	title={Multi-camera Multi-drone Detection, Tracking and Localization with Trajectory-based Re-identification},
	journal={2021 2nd International Symposium on Instrumentation, Control, Artificial Intelligence, and Robotics, ICA-SYMP 2021},
	year={2021},
	art_number={9358454},
	note={cited By 1},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85102508687\&doi=10.1109\%2fICA-SYMP50206.2021.9358454\&partnerID=40\&md5=252f23d2f6e3c6adbfd8d8fc6b3dd48c},
	abstract={This paper presents a real-time multiple camera system for detecting, tracking and localizing multiple moving drones simultaneously in a 3 dimension space. The distinct feature of the system is in its target re-identification process, which provides for information fusion among cameras based on the targets' trajectories and relative locations. Drones are detected by the multiple camera system based on motion-based blob detection, and the 2D locations of each drone in individual camera frames are tracked by A geometry- and camera-based model. From the paths of the tracked drones, their trajectories are examined using drone track feature variable. Cross-correlated among cameras for object re-identifications will allow the individual 2D position information to be integrated into overall global 3D positions of all the tracked drones from all cameras. Preliminary outdoor flight demonstrations with 2 drones flying in formation and using 3 cameras show optimal results. The system is able to detect, track, localize and re-identifying individual drone with average positional error of 8\%. © 2021 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Trapal2021162,
	author={Trapal, D.D.C. and Leong, B.C.C. and Ng, H.W. and Zhong, J.T.G. and Srigrarom, S. and Chan, T.H.},
	title={Improvement of Vision-based Drone Detection and Tracking by Removing Cluttered Background, Shadow and Water Reflection with Super Resolution},
	journal={2021 6th International Conference on Control and Robotics Engineering, ICCRE 2021},
	year={2021},
	pages={162-168},
	art_number={9435671},
	note={cited By 1},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85107773816\&doi=10.1109\%2fICCRE51898.2021.9435671\&partnerID=40\&md5=6acf92e6bf850762c7b7e6875c5e5303},
	abstract={Detection and tracking of small and fast moving aerial targets especially drones has got attention nowadays. This paper focuses on the vision-based technique using images taken from observing cameras. In real life situations, the target drone objects maybe are hidden in the cluttered background such as trees shadow or foliage, rows of buildings, and other kind of scenery that will hinder the clear indication of the drones. The object is further confused by the presence of its shadow and reflection from the water or glass wall reflection. For vision-based objection, the clarity and the ambiguity of the target images in the video stream are the key for effective and successful target detection and tracking. Here, we present the improvement by mitigating the effect of cluttered background, shadow and water reflection to the target images. We applied the schemes to make the drone more visible and more clear. We also implemented super resolution to increase the image resolution for more precise detection and tracking. As a result, the target drone could be detected and tracked throughout the sample clips. The comparative tracking results using DCF are presented. Likewise, we applied the water removal scheme to eliminate the reflection to avoid confusion to the tracker. With this, just the correct drone targets were detected and tracked. Overall, the drones could be detected and tracked all the way, as long as they appeared in the camera scene. © 2021 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Liu2021,
	author={Liu, H. and Fan, K. and Ouyang, Q. and Li, N.},
	title={Real-time small drones detection based on pruned yolov4},
	journal={Sensors},
	year={2021},
	volume={21},
	number={10},
	art_number={3374},
	note={cited By 4},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85105444029\&doi=10.3390\%2fs21103374\&partnerID=40\&md5=b5524dee7146413d58000b027561cc5b},
	abstract={To address the threat of drones intruding into high-security areas, the real-time detection of drones is urgently required to protect these areas. There are two main difficulties in real-time detection of drones. One of them is that the drones move quickly, which leads to requiring faster detectors. Another problem is that small drones are difficult to detect. In this paper, firstly, we achieve high detection accuracy by evaluating three state-of-the-art object detection methods: RetinaNet, FCOS, YOLOv3 and YOLOv4. Then, to address the first problem, we prune the convolutional channel and shortcut layer of YOLOv4 to develop thinner and shallower models. Furthermore, to improve the accuracy of small drone detection, we implement a special augmentation for small object detection by copying and pasting small drones. Experimental results verify that compared to YOLOv4, our pruned-YOLOv4 model, with 0.8 channel prune rate and 24 layers prune, achieves 90.5\% mAP and its processing speed is increased by 60.4\%. Additionally, after small object augmentation, the precision and recall of the pruned-YOLOv4 almost increases by 22.8\% and 12.7\%, respectively. Experiment results verify that our pruned-YOLOv4 is an effective and accurate approach for drone detection. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
	publisher={MDPI AG},
}

@ARTICLE{Zhang202123723,
	author={Zhang, X. and Kusrini, K.},
	title={Autonomous long-range drone detection system for critical infrastructure safety},
	journal={Multimedia Tools and Applications},
	year={2021},
	volume={80},
	number={15},
	pages={23723-23743},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85101035500\&doi=10.1007\%2fs11042-020-10231-x\&partnerID=40\&md5=99c60df7dbad429c0b51661887d685fb},
	abstract={The development of unmanned aerial vehicles has been identified as a potential source of a weapon for causing operational disruptions against critical infrastructures. To mitigate and neutralise the threat posed by the misuse of drones against malicious and terrorist activity, this paper presents a holistic design of a long-range autonomous drone detection platform. The novelty of the proposed system lies in the confluence between the design of hardware and software components to effective and efficient localisation of the intruder objects. The research presented in the paper proposes the design and validation of a situation awareness component which is interfaced with the hardware component for controlling the focal length of the camera. The continuous stream of media data obtained from the region of vulnerability is processed using the object detection that is built on region based fully connected neural network. The novelty of the proposed system relies on the processing of multi-threaded dual-media input streams that are evaluated to mitigate the latency of the system. Upon the successful detection of malicious drones, the system logs the occurrence of intruders that consists of both event description and the associated media evidence for the deployment of the mitigation strategy. The analytics platform that controls the signalling of the low-cost sensing equipment contains the NVIDIA GeForce GTX 1080 for detecting drones. The experimental testbeds developed for the validation of the proposed system has been constructed to include environments and situations that are commonly faced by critical infrastructure operators such as the area of protection, drone flight path, tradeoff between the angle of coverage against the distance of coverage. The validation of the proposed system has resulted in yielding a range of intruder drone detection by 250m with an accuracy of 95.5\%. © 2021, The Author(s).},
	publisher={Springer},
}

@CONFERENCE{Kabir2021,
	author={Kabir, M.S. and Ndukwe, I.K. and Awan, E.Z.S.},
	title={Deep Learning Inspired Vision based Frameworks for Drone Detection},
	journal={3rd International Conference on Electrical, Communication and Computer Engineering, ICECCE 2021},
	year={2021},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85115062215\&doi=10.1109\%2fICECCE52056.2021.9514124\&partnerID=40\&md5=3cf17f66190f9c86745bfaf6f4c60e7c},
	abstract={Drone detection technology is a new frontier in defence systems. With increasing incidences of crimes and terroristic attacks using commercial drones, detection of unauthorized drones is critical for timely responses from law enforcement agencies. In this paper, the issues of unavailability of benchmark dataset and performance metrics for drone detection are addressed and three single shot detectors, based on YOLOv4, YOLOv5 and DETR architectures are presented. A maximum of 99\% average precision (AP) with an average Intersection over Union (IOU) of 84\% was achieved. The precision-recall curves corroborate the generalization and fitness of the trained detection models. © 2021 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Singha2021,
	author={Singha, S. and Aydin, B.},
	title={Automated drone detection using YOLOv4},
	journal={Drones},
	year={2021},
	volume={5},
	number={3},
	art_number={95},
	note={cited By 3},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85115638681\&doi=10.3390\%2fdrones5030095\&partnerID=40\&md5=602ae52700c39773ff1ac0752b1e828d},
	abstract={Drones are increasing in popularity and are reaching the public faster than ever before. Consequently, the chances of a drone being misused are multiplying. Automated drone detection is necessary to prevent unauthorized and unwanted drone interventions. In this research, we designed an automated drone detection system using YOLOv4. The model was trained using drone and bird datasets. We then evaluated the trained YOLOv4 model on the testing dataset, using mean average precision (mAP), frames per second (FPS), precision, recall, and F1-score as evaluation parameters. We next collected our own two types of drone videos, performed drone detections, and calculated the FPS to identify the speed of detection at three altitudes. Our methodology showed better performance than what has been found in previous similar studies, achieving a mAP of 74.36\%, precision of 0.95, recall of 0.68, and F1-score of 0.79. For video detection, we achieved an FPS of 20.5 on the DJI Phantom III and an FPS of 19.0 on the DJI Mavic Pro. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
	publisher={MDPI},
}

@CONFERENCE{Makirin2021,
	author={Makirin, M.K. and Wastupranata, L.M. and Daffa, A.},
	title={Onboard visual drone detection for drone chasing and collision avoidance},
	journal={AIP Conference Proceedings},
	year={2021},
	volume={2366},
	art_number={060013},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85115313401\&doi=10.1063\%2f5.0059987\&partnerID=40\&md5=2d14f42d526c07a40aea73af21a0c2a4},
	abstract={We proposed a method for real-time detection of flying drones and UAVs that could be run with a limited computing device like an onboard computer for a drone. This method is approached from a machine learning perspective resulting in an object detection model to detect and localize multiple drones in a given image. The constraint is that the model will have to be lightweight and performant while still maintaining good accuracy. This leads us to choose SSD Mobilenet V2 model architecture to train and test how effective it is for detecting drones. Our method gained an average precision and recall of 0.586 and 0.622 (IoU 0.50-0.95, all area) respectively. © 2021 Author(s).},
	publisher={American Institute of Physics Inc.},
}

@ARTICLE{Çetin20211871,
	author={Çetin, E. and Barrado, C. and Pastor, E.},
	title={Improving real-time drone detection for counter-drone systems},
	journal={Aeronautical Journal},
	year={2021},
	volume={125},
	number={1292},
	pages={1871-1896},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85108189175\&doi=10.1017\%2faer.2021.43\&partnerID=40\&md5=698c9eeb9733033b6a86279c6ba0848a},
	abstract={The number of unmanned aerial vehicles (UAVs, also known as drones) has increased dramatically in the airspace worldwide for tasks such as surveillance, reconnaissance, shipping and delivery. However, a small number of them, acting maliciously, can raise many security risks. Recent Artificial Intelligence (AI) capabilities for object detection can be very useful for the identification and classification of drones flying in the airspace and, in particular, are a good solution against malicious drones. A number of counter-drone solutions are being developed, but the cost of drone detection ground systems can also be very high, depending on the number of sensors deployed and powerful fusion algorithms. We propose a low-cost counter-drone solution composed uniquely by a guard-drone that should be able to detect, locate and eliminate any malicious drone. In this paper, a state-of-the-art object detection algorithm is used to train the system to detect drones. Three existing object detection models are improved by transfer learning and tested for real-time drone detection. Training is done with a new dataset of drone images, constructed automatically from a very realistic flight simulator. While flying, the guard-drone captures random images of the area, while at the same time, a malicious drone is flying too. The drone images are auto-labelled using the location and attitude information available in the simulator for both drones. The world coordinates for the malicious drone position must then be projected into image pixel coordinates. The training and test results show a minimum accuracy improvement of 22\% with respect to state-of-the-art object detection models, representing promising results that enable a step towards the construction of a fully autonomous counter-drone system. © 2021 The Author(s). Published by Cambridge University Press on behalf of Royal Aeronautical Society.},
	publisher={Cambridge University Press},
}

@ARTICLE{Lee202134237,
	author={Lee, D.-H.},
	title={CNN-based single object detection and tracking in videos and its application to drone detection},
	journal={Multimedia Tools and Applications},
	year={2021},
	volume={80},
	number={26-27},
	pages={34237-34248},
	note={cited By 4},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85092404216\&doi=10.1007\%2fs11042-020-09924-0\&partnerID=40\&md5=bbf486a15020d78496728649fd80ee40},
	abstract={This paper presents convolutional neural network (CNN)-based single object detection and tracking algorithms. CNN-based object detection methods are directly applicable to static images, but not to videos. On the other hand, model-free visual object tracking methods cannot detect an object until a ground truth bounding box of the target is provided. Moreover, many annotated video datasets of the target object are required to train both the object detectors and visual trackers. In this work, three simple yet effective object detection and tracking algorithms for videos are proposed to efficiently combine a state-of-the-art object detector and visual tracker for circumstances in which only a few static images of the target are available for training. The proposed algorithms are tested using a drone detection task and the experimental results demonstrated their effectiveness. © 2020, Springer Science+Business Media, LLC, part of Springer Nature.},
	publisher={Springer},
}

@ARTICLE{Ahmed202115,
	author={Ahmed, T. and Rahman, T. and Roy, B.B. and Uddin, J.},
	title={Drone Detection by Neural Network Using GLCM and SURF Features},
	journal={Journal of Information Systems and Telecommunication},
	year={2021},
	volume={9},
	number={33},
	pages={15-23},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85104721682\&doi=10.52547\%2fjist.9.33.15\&partnerID=40\&md5=8fede080c0ed5e7b09138f001ae4bef9},
	abstract={This paper presents a vision-based drone detection method. There are a number of researches on object detection which includes different feature extraction methods – all of those are used distinctly for the experiments. But in the proposed model, a hybrid feature extraction method using SURF and GLCM is used to detect object by Neural Network which has never been experimented before. Both are very popular ways of feature extraction. Speeded-up Robust Feature (SURF) is a blob detection algorithm which extracts the points of interest from an integral image, thus converts the image into a 2D vector. The Gray-Level Co-Occurrence Matrix (GLCM) calculates the number of occurrences of consecutive pixels in same spatial relationship and represents it in a new vector- 8 × 8 matrix of best possible attributes of an image. SURF is a popular method of feature extraction and fast matching of images, whereas, GLCM method extracts the best attributes of the images. In the proposed model, the images were processed first to fit our feature extraction methods, then the SURF method was implemented to extract the features from those images into a 2D vector. Then for our next step GLCM was implemented which extracted the best possible features out of the previous vector, into a 8 × 8 matrix. Thus, image is processed in to a 2D vector and feature extracted from the combination of both SURF and GLCM methods ensures the quality of the training dataset by not just extracting features faster (with SURF) but also extracting the best of the point of interests (with GLCM). The extracted featured related to the pattern are used in the neural network for training and testing. Pattern recognition algorithm has been used as a machine learning tool for the training and testing of the model. In the experimental evaluation, the performance of proposed model is examined by cross entropy for each instance and percentage error. For the tested drone dataset, experimental results demonstrate improved performance over the state-of-art models by exhibiting less cross entropy and percentage error. © 2021. All Rights Reserved.},
	publisher={Iranian Academic Center for Education, Culture and Research},
}

@ARTICLE{Pulido2022149,
author={Pulido, C. and Ceron, A.},@ARTICLE{Dogru2022,
title={Towards Real-Time Drone Detection Using Deep Neural Networks},	author={Dogru, S. and Marques, L.},
journal={Smart Innovation, Systems and Technologies},	title={Drone Detection Using Sparse Lidar Measurements},
year={2022},	journal={IEEE Robotics and Automation Letters},
volume={255},	year={2022},
pages={149-159},	note={cited By 0},
note={cited By 0},	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85123733442\&doi=10.1109\%2fLRA.2022.3145498\&partnerID=40\&md5=282c72dcfaf610892885e653288869b1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85119370707\&doi=10.1007\%2f978-981-16-4884-7_12\&partnerID=40\&md5=0f3c279ba0d1e9d31ec6548a795ca686},	abstract={Unmanned aerial vehicles (UAV) have been serving people, fulfilling various roles in research, industry and military, not to exclude personal entertainment. They have also been in use more often for malicious purposes, such as annoying neighbors, disrupting air-travel, attacking people or infrastructure. Therefore, motivated particularly by malicious uses, the research community has been interested in proposing solutions for detection of UAVs. In this work we present a ground based aerial target detection system using lidars, relying on sparse detections rather than dense point clouds, with the aim of not only detecting but also estimating their motion and active tracking. We lay a theoretical groundwork to analyse the performance of such a lidar based detection system and help understanding its limitations. The work is complemented with field experiments utilizing a state-of-the-art lidar and several drones of different sizes, showing effectiveness in both detection and tracking using sparse measurements. IEEE},
abstract={The growing use of drones/unmanned aerial vehicles (UAV’s) has generated in the general public as well as in institutions the awareness of the possible misuse that can be given to these devices. For this reason, the detection of drones has become a necessity that poses in the case of detection using images a great difficulty due to its small size, in addition to the background that can make detection even more difficult. Regarding this work, the aim is not only to detect drones but also to distinguish the type of detected drone. Different networks were trained whereupon an analysis was conducted in which it was found that the YOLOv4tiny network with 416 × 416 input resolution presents the best results considering both the inference performance and the processing speed. © 2022, The Author(s), under exclusive license to Springer Nature Singapore Pte Ltd.},	publisher={Institute of Electrical and Electronics Engineers Inc.},
publisher={Springer Science and Business Media Deutschland GmbH},}
}
@ARTICLE{Prayitno2014819,
	author={Prayitno, A. and Indrawati, V. and Utomo, G.},
	title={Trajectory tracking of AR.Drone quadrotor using fuzzy logic controller},
	journal={Telkomnika (Telecommunication Computing Electronics and Control)},
	year={2014},
	volume={12},
	number={4},
	pages={819-828},
	note={cited By 20},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84923129981\&doi=10.12928\%2fTELKOMNIKA.v12i4.368\&partnerID=40\&md5=d83a90e296b8f7a46d4d3c0e03fddc48},
	abstract={In this paper, Fuzzy Logic Controller (FLC) is implemented in the AR.Drone quadrotor in order to make it follow a given trajectory reference. The distance between the position and angle of the AR.Drone to the reference point is used as the input of the FLC. As for the output, pitch value and yaw rate will be the controlling signal for the AR.Drone. The navigation data of the AR.Drone are forward speed (vx), sideward speed (vy), and yaw. These navigation data are going to be used to estimate positions and orientation of the AR.Drone. To compensate for the y-position drift, the value of vy is also used as a criterion to determine the roll compensation. The FLC algorithm is implemented to AR.Drone 2.0 Elite Edition using LabVIEW software. Also, the algorithm has been tested in various trajectories such as a straight line, a straight line with a perpendicular turn, a rectangular trajectory and a curved trajectory. The results have shown that AR.Drone can follow a given trajectory with various initial positions and orientations quite well.},
	publisher={Universitas Ahmad Dahlan},
}

@ARTICLE{Pilté2017301,
	author={Pilté, M. and Bonnabel, S. and Barbaresco, F.},
	title={Drone tracking using an innovative UKF},
	journal={Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
	year={2017},
	volume={10589 LNCS},
	pages={301-309},
	note={cited By 1},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85033698230\&doi=10.1007\%2f978-3-319-68445-1_35\&partnerID=40\&md5=a7c8a22b3b81a0b0bc3564feb3c08975},
	abstract={This paper addresses the drone tracking problem, using a model based on the Frenet-Serret frame. A kinematic model in 2D, representing intrinsic coordinates of the drone is used. The tracking problem is tackled using two recent filtering methods. On the one hand, the Invariant Extended Kalman Filter (IEKF), introduced in [1] is tested, and on the other hand, the second step of the filtering algorithm, i.e. the update step of the IEKF is replaced by the update step of the Unscented Kalman Filter (UKF), introduced in [2]. These two filters are compared to the well known Extended Kalman Filter. The estimation precision of all three algorithms are computed on a real drone tracking problem. © 2017, Springer International Publishing AG.},
	publisher={Springer Verlag},
}

@CONFERENCE{Park2017696,
	author={Park, J. and Kim, D.H. and Shin, Y.S. and Lee, S.-H.},
	title={A comparison of convolutional object detectors for real-time drone tracking using a PTZ camera},
	journal={International Conference on Control, Automation and Systems},
	year={2017},
	volume={2017-October},
	pages={696-699},
	note={cited By 18},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85044476793\&doi=10.23919\%2fICCAS.2017.8204318\&partnerID=40\&md5=3c00be6c4f69925ea70b9e75d9d35cb0},
	abstract={As highly maneuverable drones are available at the low price, the threats that might be caused by the drone attacks has been increased. Recent object detectors have been dramatically improved in accuracy by using convolutional neural networks, and these can be utilized to identify hostile drones. In this paper, we examine state-of-the-arts convolutional object detectors for a real-time drone detection and tracking system using a Pan-Tilt-Zoom (PTZ) camera. In the drone detection and tracking system, an object detector is used to identify whether an image from the PTZ camera contains a drone, and our system generates PTZ actions to track the detected drone. To detect small size drones in real-time, an appropriate object detector should be selected. This paper compares six convolutional object detectors in the accuracy and speed. © 2017 Institute of Control, Robotics and Systems - ICROS.},
	publisher={IEEE Computer Society},
}

@ARTICLE{Chen2018131,
	author={Chen, P. and Dang, Y. and Liang, R. and Zhu, W. and He, X.},
	title={Real-Time Object Tracking on a Drone with Multi-Inertial Sensing Data},
	journal={IEEE Transactions on Intelligent Transportation Systems},
	year={2018},
	volume={19},
	number={1},
	pages={131-139},
	art_number={8054712},
	note={cited By 40},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85030776761\&doi=10.1109\%2fTITS.2017.2750091\&partnerID=40\&md5=c18562b34f2c84dfd3d33f78f81b2890},
	abstract={Real-time object tracking on a drone under a dynamic environment has been a challenging issue for many years, with existing approaches using off-line calculation or powerful computation units on board. This paper presents a new lightweight real-time onboard object tracking approach with multi-inertial sensing data, wherein a highly energy-efficient drone is built based on the Snapdragon flight board of Qualcomm. The flight board uses a digital signal processor core of the Snapdragon 801 processor to realize PX4 autopilot, an open-source autopilot system oriented toward inexpensive autonomous aircraft. It also uses an ARM core to realize Linux, robot operating systems, open-source computer vision library, and related algorithms. A lightweight moving object detection algorithm is proposed that extracts feature points in the video frame using the oriented FAST and rotated binary robust independent elementary features algorithm and adapts a local difference binary algorithm to construct the image binary descriptors. The K-nearest neighbor method is then used to match the image descriptors. Finally, an object tracking method is proposed that fuses inertial measurement unit data, global positioning system data, and the moving object detection results to calculate the relative position between coordinate systems of the object and the drone. All the algorithms are run on the Qualcomm platform in real time. Experimental results demonstrate the superior performance of our method over the state-of-the-art visual tracking method. © 2000-2011 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Boudjit20181013,
	author={Boudjit, K. and Larbes, C. and Ramzan, N.},
	title={ANN design and implementation for real-time object tracking using quadrotor ar.Drone 2.0},
	journal={Journal of Experimental and Theoretical Artificial Intelligence},
	year={2018},
	volume={30},
	number={6},
	pages={1013-1035},
	note={cited By 7},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85053040527\&doi=10.1080\%2f0952813X.2018.1509896\&partnerID=40\&md5=d447547cb1ec29541f703c1080a6beee},
	abstract={This paper aims to use a visual-based control mechanism to control a quadrotor, which is in pursuit of a target. The non-linear nature of a quadrotor, on onehand, and the difficulty of obtaining an exact model for it, on the other hand, constitute two serious challenges in designing a controller for this UAV. A potential solution for such problems is the use of intelligent control methods such as those that rely on ANNs. A novel technique based on ANNs is proposed in this work for the identification and tracking of targets. Multilayer perceptron is used for this purpose. Experimental results and simulations are shown to demonstrate the feasibility of the proposed method for target tracking. © 2018 Informa UK Limited, trading as Taylor \& Francis Group.},
	publisher={Taylor and Francis Ltd.},
}

@ARTICLE{Rohan201969575,
	author={Rohan, A. and Rabah, M. and Kim, S.-H.},
	title={Convolutional Neural Network-Based Real-Time Object Detection and Tracking for Parrot AR Drone 2},
	journal={IEEE Access},
	year={2019},
	volume={7},
	pages={69575-69584},
	art_number={8723347},
	note={cited By 30},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85067241645\&doi=10.1109\%2fACCESS.2019.2919332\&partnerID=40\&md5=89296d33f2f1efa959011e06c363d9c4},
	abstract={Recent advancements in the field of Artificial Intelligence (AI) have provided an opportunity to create autonomous devices, robots, and machines characterized particularly with the ability to make decisions and perform tasks without human mediation. One of these devices, Unmanned Aerial Vehicles (UAVs) or drones are widely used to perform tasks like surveillance, search and rescue, object detection and target tracking, parcel delivery (recently started by Amazon), and many more. The sensitivity in performing said tasks demands that drones must be efficient and reliable. For this, in this paper, an approach to detect and track the target object, moving or still, for a drone is presented. The Parrot AR Drone 2 is used for this application. Convolutional Neural Network (CNN) is used for object detection and target tracking. The object detection results show that CNN detects and classifies object with a high level of accuracy (98\%). For real-time tracking, the tracking algorithm responds faster than conventionally used approaches, efficiently tracking the detected object without losing it from sight. The calculations based on several iterations exhibit that the efficiency achieved for target tracking is 96.5\%. © 2013 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Unlu2019,
	author={Unlu, E. and Zenou, E. and Riviere, N. and Dupouy, P.-E.},
	title={An autonomous drone surveillance and tracking architecture},
	journal={IS and T International Symposium on Electronic Imaging Science and Technology},
	year={2019},
	volume={2019},
	number={15},
	art_number={AVM-035},
	note={cited By 4},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85078066430\&doi=10.2352\%2fISSN.2470-1173.2019.15.AVM-035\&partnerID=40\&md5=f25b40abb78f2370289a12084f6b93f2},
	abstract={In this work, we present a computer vision and machine learning backed autonomous drone surveillance system, in order to protect critical locations. The system is composed of a wide angle, high resolution daylight camera and a relatively narrow angle thermal camera mounted on a rotating turret. The wide angle daylight camera allows the detection of flying intruders, as small as 20 pixels with a very low false alarm rate. The primary detection is based on YOLO convolutional neural network (CNN) rather than conventional background subtraction algorithms due its low false alarm rate performance. At the same time, the tracked flying objects are tracked by the rotating turret and classified by the narrow angle, zoomed thermal camera, where classification algorithm is also based on CNNs. The training of the algorithms is performed by artificial and augmented datasets due to scarcity of infrared videos of drones. © 2019, Society for Imaging Science and Technology},
	publisher={Society for Imaging Science and Technology},
}

@CONFERENCE{Thai2019,
	author={Thai, V.-P. and Zhong, W. and Pham, T. and Alam, S. and Duong, V.},
	title={Detection, tracking and classification of aircraft and drones in digital towers using machine learning on motion patterns},
	journal={Integrated Communications, Navigation and Surveillance Conference, ICNS},
	year={2019},
	volume={2019-April},
	art_number={8735238},
	note={cited By 13},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85068036283\&doi=10.1109\%2fICNSURV.2019.8735238\&partnerID=40\&md5=df6734f1e61d40165a06cd041bee4710},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
	abstract={Remote digital towers using high-resolution cameras that cover a 360-degree view of airports have recently been a solution to some airports in replacing physical towers and in introducing digital technologies as tools to assist tower controllers. We propose the use of machine learning techniques to automatically detect and track small moving objects in the airfield from their motion patterns, i.e. the ways an object moves. A video dataset comprising aircraft in an airfield and drones captured from a fixed angle is constructed. To the dataset, we apply Harris Detection and Convolutional Neural Network followed by Optical Flow to locate and track very small moving objects in the wide-area scene. Motion-based features are extracted from their trajectories after which a K-Nearest Neighbor classifier is applied to classify objects into drones or aircraft. Our tests show that the accuracy and execution time are appropriate for real-time operation.}
}

@CONFERENCE{Fernandes2019,
	author={Fernandes, A. and Baptista, M. and Fernandes, L. and Chaves, P.},
	title={Drone, Aircraft and Bird Identification in Video Images Using Object Tracking and Residual Neural Networks},
	journal={Proceedings of the 11th International Conference on Electronics, Computers and Artificial Intelligence, ECAI 2019},
	year={2019},
	art_number={9042167},
	note={cited By 4},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85079516058\&doi=10.1109\%2fECAI46879.2019.9042167\&partnerID=40\&md5=bc25f7fbed5b9428e79f5664d9ed07d5},
	abstract={As maritime smuggling is being combatted more effectively, the criminal 'modus operandi' consists more frequently of using small aircraft and drones for drug transport. To address this issue, we report our efforts to develop a system capable of accurately tracking suspicious flying objects and identifying them on video streams. Our solution consists in coupling classical computer vision with deep learning to perform tracking and object detection. A discrete Kalman filter is used to predict the location of each object being tracked while the Hungarian algorithm is used to match objects between successive frames. Whenever a potential target is considered suspicious the input images are zoomed and fed into a deep learning pipeline that separates images into the classes aircraft, drones, birds or clouds. A literature survey indicates that this problem with important applications is yet to be fully explored. © 2019 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}


@CONFERENCE{Han2019414,
	author={Han, X. and Wang, C. and Li, Y. and Wu, X.},
	title={A trajectory optimization algorithm for drone target localization and tracking},
	journal={2019 IEEE International Conference on Real-Time Computing and Robotics, RCAR 2019},
	year={2019},
	volume={2019-August},
	pages={414-419},
	art_number={9043968},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85089142027\&doi=10.1109\%2fRCAR47638.2019.9043968\&partnerID=40\&md5=f5571a5a42491340df72d6c0206b8fbd},
	abstract={Accurate positioning is the premise for the drone to successfully capture the target, this paper proposes a solution to the positioning failure caused by the relatively severe jitter of the drone and the target. In this paper, the Improved Kernel Correlation Filter (KCF) is used for target tracking, and the improved Kalman filter is used to smooth the input signal in real time, which reduces the continuous jitter of the drone. The advantage of this approach is that it will not cause misjudgment from the deviation where the measured value is too large. Further, the hysteresis is also significantly improved. The experimental works are carried out on a M100 UAV to verify the improved KCF and the improved Kalman algorithm, respectively. The results showed the effectiveness of the proposed approach. © 2018 IEEE},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Kim20191627,
	author={Kim, T. and Wee, I. and Shim, D.H.},
	title={Occlusion Robust Object Detection and Tracking on a Real-time Drone},
	journal={International Conference on Control, Automation and Systems},
	year={2019},
	volume={2019-October},
	pages={1627-1631},
	art_number={8971546},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85079104572\&doi=10.23919\%2fICCAS47443.2019.8971546\&partnerID=40\&md5=842d8f202273121a35d63bb16e9d53fb},
	abstract={This paper presents a vision-based tracking algorithm for real-time drone. This method consists of cnn based object detection and object tracking using the result of detector. The detector outputs a class label and a binary mask of the object. The tracker uses this binary mask to extract object features from the background. We use this information to estimate the accurate target location and tracking the target to each frame considering the similarity between target and each detected object feature vector. We validate this method using real-time drone. © 2019 Institute of Control, Robotics and Systems - ICROS.},
	publisher={IEEE Computer Society},
}

@CONFERENCE{Respall2019477,
	author={Respall, V.M. and Sellami, S. and Afanasyev, I.},
	title={Implementation of autonomous visual detection, tracking and landing for AR.Drone 2.0 quadcopter},
	journal={Proceedings - International Conference on Developments in eSystems Engineering, DeSE},
	year={2019},
	volume={October-2019},
	pages={477-482},
	art_number={9072990},
	note={cited By 2},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85084410982\&doi=10.1109\%2fDeSE.2019.00093\&partnerID=40\&md5=a9d0b243da21855f8361e8f427516687},
	abstract={This paper presents the design and implementation of a system where an autonomous aerial vehicle (UAV) has to detect, track and land in the vicinity of a moving Unmanned Ground Vehicle (UGV). The quadcopter needs, using camerabased data, to identify and track the UGV platform. A colorbased detection algorithm is employed to detect the UGV position and Kernelized Correlation Filters (KCF) are taken for its tracking. For suppressing the false positive cases of the detection algorithm, and to double check the presence of the UGV in an image frame, the ORB (Oriented FAST and rotated BRIEF) feature detector is used. Then the UGV position detected in the image frame is used in a PD feedback control loop in the quadcopter's controller that enables the actual tracking of the moving UGV in the horizontal plane, while another PID controller stabilizes the UAV altitude. The proposed approach was initially tested in Gazebo simulator, and then in real environment with Parrot AR.Drone 2.0 and Plato robots (as UAV and UGV correspondingly). The results show that the proposed system can detect and track the UGV in online mode without artificial markers and perform robust UAV landing. © 2019 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Unlu2019,
	author={Unlu, E. and Zenou, E. and Riviere, N. and Dupouy, P.-E.},
	title={Deep learning-based strategies for the detection and tracking of drones using several cameras},
	journal={IPSJ Transactions on Computer Vision and Applications},
	year={2019},
	volume={11},
	number={1},
	art_number={7},
	note={cited By 35},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85069679620\&doi=10.1186\%2fs41074-019-0059-x\&partnerID=40\&md5=71095e7b029b06cd5032f33c1eed5497},
	abstract={Commercial Unmanned aerial vehicle (UAV) industry, which is publicly known as drone, has seen a tremendous increase in last few years, making these devices highly accessible to public. This phenomenon has immediately raised security concerns due to fact that these devices can intentionally or unintentionally cause serious hazards. In order to protect critical locations, the academia and industry have proposed several solutions in recent years. Computer vision is extensively used to detect drones autonomously compared to other proposed solutions such as RADAR, acoustics and RF signal analysis thanks to its robustness. Among these computer vision-based approaches, we see the preference of deep learning algorithms thanks to their effectiveness. In this paper, we are presenting an autonomous drone detection and tracking system which uses a static wide-angle camera and a lower-angle camera mounted on a rotating turret. In order to use memory and time efficiently, we propose a combined multi-frame deep learning detection technique, where the frame coming from the zoomed camera on the turret is overlaid on the wide-angle static camera’s frame. With this approach, we are able to build an efficient pipeline where the initial detection of small sized aerial intruders on the main image plane and their detection on the zoomed image plane is performed simultaneously, minimizing the cost of resource exhaustive detection algorithm. In addition to this, we present the integral system including tracking algorithms, deep learning classification architectures and the protocols. © 2019, The Author(s).},
	publisher={Springer Berlin Heidelberg},
}

@CONFERENCE{Fujiwara20192239,
	author={Fujiwara, N. and Jiang, M. and Takaki, T. and Ishii, I. and Shimasaki, K.},
	title={Super-telephoto drone tracking using HFR-video-based vibration source localization},
	journal={IEEE International Conference on Robotics and Biomimetics, ROBIO 2019},
	year={2019},
	pages={2239-2244},
	art_number={8961695},
	note={cited By 1},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85079069150\&doi=10.1109\%2fROBIO49542.2019.8961695\&partnerID=40\&md5=822ca0ed5b5ab04da4c58c70e3f63f09},
	abstract={In this paper, we propose a super-telephoto drone surveillance system that can search and track a flying drone at a 1 km distance or more within an area spanning hundreds of square meters. By constructing a mirror-drive high-speed pan-tilt control system with a super-telephoto camera lens, remote drone surveillance becomes possible owing to the acquisition of high spatial resolution images of target objects. We adopted a vibration-based drone localization algorithm that can simultaneously detect fast-rotating drone-propellers in an high-frame-rate video using a pixel-level short-time Fourier transform to achieve robust surveillance under various challenging conditions for super-telephoto video-shooting such as low luminance and heat haze. The effectiveness of the super-telephoto drone tracking system is demonstrated by conducting a drone searching and tracking experiment at a 1 km distance using an 800-mm focal length lens with a mirror-drive video-shooting system. © 2019 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Stadler2020604,
	author={Stadler, D. and Sommer, L.W. and Beyerer, J.},
	title={PAS Tracker: Position-, Appearance- and Size-Aware Multi-object Tracking in Drone Videos},
	journal={Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
	year={2020},
	volume={12538 LNCS},
	pages={604-620},
	note={cited By 1},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85101779406\&doi=10.1007\%2f978-3-030-66823-5_36\&partnerID=40\&md5=12e2cc955cb288ce85486e6ea2a5b580},
	abstract={While most multi-object tracking methods based on tracking-by-detection use either spatial or appearance cues for associating detections or apply one cue after another, our proposed PAS tracker employs a novel similarity measure that combines position, appearance and size information jointly to make full use of object representations. We further extend the PAS tracker by introducing a filtering technique to remove false positive detections, particularly in crowded scenarios, and apply a camera motion compensation model to align track positions across frames. To provide high quality detections as input for the proposed tracker, the performance of eight state-of-the-art object detectors is compared on the VisDrone MOT dataset, on which the PAS tracker achieves state-of-the-art performance and ranks 3rd in the VisDrone2020 MOT challenge. In an ablation study, we demonstrate the effectiveness of the introduced tracking components and the impact of the employed detections on the tracking performance is analyzed in detail. © 2020, Springer Nature Switzerland AG.},
	publisher={Springer Science and Business Media Deutschland GmbH},
}

@ARTICLE{Zhang2020638,
	author={Zhang, X. and Jiao, L. and Liu, X. and Li, X. and Zhang, W. and Zhu, H. and Zhang, J.},
	title={A Deep Learning Filter for Visual Drone Single Object Tracking},
	journal={Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
	year={2020},
	volume={12538 LNCS},
	pages={638-650},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85101785168\&doi=10.1007\%2f978-3-030-66823-5_38\&partnerID=40\&md5=7225f8989e49509aaff0db09b24a36a8},
	abstract={Object tracking is one of the most important topics in computer vision. In visual drone tracking, it is an extremely challenging due to various factors, such as camera motion, partial occlusion, and full occlusion. In this paper, we propose a deep learning filter method to relieve the above problems, which is to obtain a priori position of the object at the subsequent frame and predict its trajectory to follow up the object during occlusion. Our tracker adopts the geometric transformation of the surrounding of the object to prevent the bounding box of the object lost, and it uses context information to integrate its motion trend thereby tracking the object successfully when it reappears. Experiments on the VisDrone-SOT2018 test dataset and the VisDrone-SOT2020 val dataset illustrate the effectiveness of the proposed approach. © 2020, Springer Nature Switzerland AG.},
	publisher={Springer Science and Business Media Deutschland GmbH},
}

@CONFERENCE{Gözen202010082,
	author={Gözen, D. and Özer, S.},
	title={Visual object tracking in drone images with deep reinforcement learning},
	journal={Proceedings - International Conference on Pattern Recognition},
	year={2020},
	pages={10082-10089},
	art_number={9413316},
	note={cited By 2},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85110437567\&doi=10.1109\%2fICPR48806.2021.9413316\&partnerID=40\&md5=8d8523943d903916bb794f6e5f5fcc1b},
	abstract={There is an increasing demand on utilizing camera equipped drones and their applications in many domains varying from agriculture to entertainment and from sports events to surveillance. In such drone applications, an essential and a common task is tracking an object of interest visually. Drone (or UAV) images have different properties when compared to the ground taken (natural) images and those differences introduce additional complexities to the existing object trackers to be directly applied on drone applications. Some important differences among those complexities include (i) smaller object sizes to be tracked and (ii) different orientations and viewing angles yielding different texture and features to be observed. Therefore, new algorithms trained on drone images are needed for the drone-based applications. In this paper, we introduce a deep reinforcement learning (RL) based single object tracker that tracks an object of interest in drone images by estimating a series of actions to find the location of the object in the next frame. This is the first work introducing a single object tracker using a deep RL-based technique for drone images. Our proposed solution introduces a novel reward function that aims to reduce the total number of actions taken to estimate the object's location in the next frame and also introduces a different backbone network to be used on low resolution images. Additionally, we introduce a set of new actions into the action library to better deal with the above-mentioned complexities. We compare our proposed solutions to a state of the art tracking algorithm from the recent literature and demonstrate up to 3.87\% improvement in precision and 3.6\% improvement in IoU values on the VisDrone2019 data set. We also provide additional results on OTB-100 data set and show up to 3.15\% improvement in precision on the OTB-100 data set when compared to the same previous state of the art algorithm. Lastly, we analyze the ability to handle some of the challenges faced during tracking, including but not limited to occlusion, deformation, and scale variation for our proposed solutions. © 2020 IEEE},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Tao2020463,
	author={Tao, L. and Hong, T. and Chao, X.},
	title={Drone identification and location tracking based on YOLOv3},
	journal={Gongcheng Kexue Xuebao/Chinese Journal of Engineering},
	year={2020},
	volume={42},
	number={4},
	pages={463-468},
	note={cited By 2},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85084657549\&doi=10.13374\%2fj.issn2095-9389.2019.09.10.002\&partnerID=40\&md5=9886fcd3c298392dc440f5898d521b69},
	abstract={In recent years, increasing incidents of drone intrusion have occurred, and the drone collisions have become common. As a result, accidents may occur in densely populated areas. Therefore, drone monitoring is an important research topic in the field of security. Although many types of drone monitoring programs exist, most of them are costly and difficult to implement. To solve this problem, in the 5G context, this study proposed a method of using a city's existing monitoring network to acquire data based on a deep learning algorithm for drone target detection, constructing a recognizable drone, and tracking the unmanned aerial vehicle. The method used the improved YOLOv3 (You only look once) model to detect the presence of drones in video frames. The YOLOv3 algorithm is the third generation version of the YOLO series, belonging to the one-stage target detection algorithm. This algorithm has significant advantages over the two-stage type of algorithm in speed. YOLOv3 outputs the position information of the drone in the video frame. According to the position information, the PID (Proportion integration differentiation) algorithm was used to adjust the center of the camera to track the drone. Then, the parameters of the plurality of cameras were used to calculate the actual coordinates of the drone, thereby realizing the positioning. We built the dataset by taking photos of the drone's flight, searching and downloading drone pictures from the Internet, and labeling the drones in the image by using the labelImg tool. The dataset was classified according to the number of rotors of the drone. In the experiment, the detection model was trained by the dataset classified by the number of rotors. The trained model can achieve 83.24\% accuracy and 88.15\% recall rate on the test set, and speed of 20 frames per second on the computer equipped with NVIDIA GTX 1060 for real-time tracking. © All right reserved.},
	publisher={Science Press},
}


@CONFERENCE{Hamdi2020,
	author={Hamdi, A. and Salim, F. and Kim, D.Y.},
	title={DroTrack: High-speed drone-based object tracking under uncertainty},
	journal={IEEE International Conference on Fuzzy Systems},
	year={2020},
	volume={2020-July},
	art_number={9177571},
	note={cited By 2},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85090502234\&doi=10.1109\%2fFUZZ48607.2020.9177571\&partnerID=40\&md5=d812ed4752293897e36d11218c741fd9},
	abstract={We present DroTrack, a high-speed visual single-object tracking framework for drone-captured video sequences. Most of the existing object tracking methods are designed to tackle well-known challenges, such as occlusion and cluttered backgrounds. The complex motion of drones, i.e., multiple degrees of freedom in three-dimensional space, causes high uncertainty. The uncertainty problem leads to inaccurate location predictions and fuzziness in scale estimations. DroTrack solves such issues by discovering the dependency between object representation and motion geometry. We implement an effective object segmentation based on Fuzzy C Means (FCM). We incorporate the spatial information into the membership function to cluster the most discriminative segments. We then enhance the object segmentation by using a pre-trained Convolution Neural Network (CNN) model. DroTrack also leverages the geometrical angular motion to estimate a reliable object scale. We discuss the experimental results and performance evaluation using two datasets of 51, 462 drone-captured frames. The combination of the FCM segmentation and the angular scaling increased DroTrack precision by up to 9\% and decreased the centre location error by 162 pixels on average. DroTrack outperforms all the high-speed trackers and achieves comparable results in comparison to deep learning trackers. DroTrack offers high frame rates up to 1000 frame per second (fps) with the best location precision, more than a set of state-of-the-art real-time trackers. © 2020 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Zhou2020,
	author={Zhou, H. and Ni, B.},
	title={Tracking of drone flight by neural network Siamese-RPN},
	journal={Proceedings - 2020 6th International Conference on Engineering, Applied Sciences and Technology, ICEAST 2020},
	year={2020},
	art_number={9165441},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85091984976\&doi=10.1109\%2fICEAST50382.2020.9165441\&partnerID=40\&md5=77fe44bc4ab70154b9b3827ba896a3e1},
	abstract={Recently deep learning has made a great progress in the image classification and video object tracking. However the speed of traditional region proposal algorithms is too slow and become a bottleneck. Researchers have proposed a lot of neural networks for the improvements. With the region proposal network proposed, neural network can finish the computation enabling cost-free region proposals, which make it possible to do real-time detection and tracking. This paper will set up a system which can detect and track drone by using neural networks such as Faster R-CNN and Siamese-RPN. © 2020 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Srigrarom2020615,
	author={Srigrarom, S. and Hoe Chew, K.},
	title={Hybrid motion-based object detection for detecting and tracking of small and fast moving drones},
	journal={2020 International Conference on Unmanned Aircraft Systems, ICUAS 2020},
	year={2020},
	pages={615-621},
	art_number={9213912},
	note={cited By 3},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85094978319\&doi=10.1109\%2fICUAS48674.2020.9213912\&partnerID=40\&md5=6b3a625e05b0a0c4ad29592c29b60c95},
	abstract={A hybrid detecting and tracking system that is made especially for small and fast moving drones in which the other existing techniques cannot detect is presented. This new automatic system integrates geometry estimation, 2D object detection, 3D localization, trajectory estimation and tracking for dynamic scene interpretation. This caters to moving cameras, e.g. those mounted on a separate flying platform. The technique is built on the unified two-step real-time algorithm for detection and tracking of moving objects (DATMO) in dynamic outdoor environments. The first step is built on the motion-based detection approach for early detection of an object when the targeted object is still far away and appears very small in the scene. The second step is based on the appearance-based detection approach for continual detection, further identification and verification of the object. The camera's own position is estimated by 3D triangulation of the static landscape in the scene, doubled up as ground truth. This includes both the pan-tilt-zoom motion and the camera's vibration compensation. Therefore, the drone can be tracked, even when the camera is in motion and/or under jittery condition. As a result, the position of the tracked drone in the global inertial coordinate is further improved. Subsequently, the drone motion is tracked using the Extended Kalman Filter scheme. Initial results show that this hybrid system is able to detect a small drone from a distance away in less than a few frames after such a drone appears in the scene. The drone is always tracked as long as it is in the camera's field of view. As this technique is vision-based, this drone detection and tracking system can expand to detect multiple drones. © 2020 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Demir20201625,
	author={Demir, B. and Ergunay, S. and Nurlu, G. and Popovic, V. and Ott, B. and Wellig, P. and Thiran, J.-P. and Leblebici, Y.},
	title={Real-time high-resolution omnidirectional imaging platform for drone detection and tracking},
	journal={Journal of Real-Time Image Processing},
	year={2020},
	volume={17},
	number={5},
	pages={1625-1635},
	note={cited By 2},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85074700180\&doi=10.1007\%2fs11554-019-00921-7\&partnerID=40\&md5=ca09300a973af4909bdf83c5d8857a02},
	abstract={Drones have become steadily affordable, which raises privacy and security concerns as well as interest in drone detection systems. On the other hand, drone detection is a challenging task due to small dimensions of drones, difficulty of long-distance detection, strict real-time constraints and necessity of wide angle coverage for drones. Although different radar and audio-assisted drone detection systems have been presented, they suffer from the cost, range, or interference problems. On the contrary, a long-range detection can be obtained by a vision-based system. Aiming that, we propose a real-time moving object detection and tracking system optimized for drone detection using 16 cameras with 20 MP resolution. The proposed system detects drones from short range and long range with 360∘ surveillance coverage owing high-performance ultra-high-resolution (320 MP) video-processing capability. It is able to detect drones with 100 cm diameter from 700 m distance despite deceptive background. It is interference free, so multiple systems can properly operate in the vicinity without effecting each other. It integrates processing power of embedded systems with flexibility of software to generate a full platform for drone detection and tracking. © 2019, Springer-Verlag GmbH Germany, part of Springer Nature.},
	publisher={Springer},
}

@ARTICLE{Cajo2021528,
	author={Cajo, R. and Zhao, S. and Plaza, D. and De Keyser, R. and Ionescu, C.},
	title={A fractional order predictive control for trajectory tracking of the ar.drone quadrotor},
	journal={Lecture Notes in Electrical Engineering},
	year={2021},
	volume={695 LNEE},
	pages={528-537},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85091315012\&doi=10.1007\%2f978-3-030-58653-9_51\&partnerID=40\&md5=91b85cf3808ca75824a3408bc7d5b8c6},
	abstract={A fractional-order model predictive control with extended prediction self-adaptive control (FOMPC-EPSAC) strategy is proposed for the AR.Drone quadrotor system. The objective is to achieve an optimal trajectory tracking control for an AR.Drone quadrotor by using a fractional order integral cost function in the conventional MPC-EPSAC algorithm. In addition, a particle swarm optimization (PSO) algorithm is applied to find the optimal weighting matrices, which depend on the terms ($$\alpha $$, $$\beta $$) of the fractional order cost function. Some simulation results show the superiority of FOMPC-EPSAC over conventional MPC-EPSAC with respect to trajectory tracking and robustness under wind disturbances. © The Editor(s) (if applicable) and The Author(s), under exclusive license to Springer Nature Switzerland AG 2021.},
	publisher={Springer Science and Business Media Deutschland GmbH},
}

@CONFERENCE{Fussi20211,
	author={Fussi, M. and Corsi, E. and Rinaldi, G. and Alibani, M. and Pollini, L.},
	title={Simultaneous tracking of multiple drones using convolutional neural networks and optical flow},
	journal={AIAA Scitech 2021 Forum},
	year={2021},
	pages={1-11},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85099805074\&partnerID=40\&md5=7149ab425780d505836abceb56d30149},
	abstract={The aim of this paper is to implement a multi-object tracker for detecting, discriminating and following multiple drones on the 2D image plane. The main system consists in a neural network trained for detecting drones on the image plane. Once the drones are identified, their Region Of Interest information are sent to the Kalman filter based tracking system in order to compute position estimates. Each detected drone is given an ID using the Global Nearest Neighbor and Auction Algorithms, then the tracking system employs a set of Kalman filters and each measure is assigned to the respective estimate/filter using the unique ID. In order to reduce the effects of the neural network computation (e.g detection) time, every position estimate is corrected using Optical Flow. Results are evaluated through MOT (Multi-Object Tracking) Metrics, aiming to demonstrate the benefits of implementing Optical Flow algorithms for building a robust multi-tracking system. © 2021, American Institute of Aeronautics and Astronautics Inc, AIAA. All rights reserved.},
	publisher={American Institute of Aeronautics and Astronautics Inc, AIAA},
}

@CONFERENCE{Phung2021189,
	author={Phung, K.-P. and Lu, T.-H. and Nguyen, T.-T. and Le, N.-L. and Nguyen, H.-H. and Hoang, V.-P.},
	title={Multi-model Deep Learning Drone Detection and Tracking in Complex Background Conditions},
	journal={International Conference on Advanced Technologies for Communications},
	year={2021},
	volume={2021-October},
	pages={189-194},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85122942707\&doi=10.1109\%2fATC52653.2021.9598317\&partnerID=40\&md5=1efcc3b7b42865ce80289e93f937799d},
	abstract={The recent popularity of drones with quadcopter layouts is threatening public safety and personal privacy. With the ability to hover and perform complex maneuvers even in indoor conditions, equipped with video cameras as well as capable of carrying hazardous materials, drones can truly become a security threat, especially to vulnerable organizations. Therefore, detecting and tracking drones in secured areas poses an urgent task for the surveillance system. In this paper, we design a real-time drone detection and tracking system with the combination of multiple deep learning and computer vision techniques: 1) Yolo-v4 model for detecting drones and 2) visual models for tracking drones. Besides, we have collected and labeled a larger drone dataset by mixing the existing datasets with our collected images. We evaluated three deep learning models for drone detection on this dataset and acquired the Yolo-V4 model to be the highest detection performance with AP = 34.63\%. Combining this detection model and the existing visual tracking modules can boost the drone tracking up to more than 20fps for different backgrounds at around 700m by using an usual PC without GPU. © 2021 IEEE.},
	publisher={IEEE Computer Society},
}

@CONFERENCE{Srigrarom2021,
	author={Srigrarom, S. and Sie, N.J.L. and Cheng, H. and Chew, K.H. and Lee, M. and Ratsamee, P.},
	title={Multi-camera Multi-drone Detection, Tracking and Localization with Trajectory-based Re-identification},
	journal={2021 2nd International Symposium on Instrumentation, Control, Artificial Intelligence, and Robotics, ICA-SYMP 2021},
	year={2021},
	art_number={9358454},
	note={cited By 1},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85102508687\&doi=10.1109\%2fICA-SYMP50206.2021.9358454\&partnerID=40\&md5=252f23d2f6e3c6adbfd8d8fc6b3dd48c},
	abstract={This paper presents a real-time multiple camera system for detecting, tracking and localizing multiple moving drones simultaneously in a 3 dimension space. The distinct feature of the system is in its target re-identification process, which provides for information fusion among cameras based on the targets' trajectories and relative locations. Drones are detected by the multiple camera system based on motion-based blob detection, and the 2D locations of each drone in individual camera frames are tracked by A geometry- and camera-based model. From the paths of the tracked drones, their trajectories are examined using drone track feature variable. Cross-correlated among cameras for object re-identifications will allow the individual 2D position information to be integrated into overall global 3D positions of all the tracked drones from all cameras. Preliminary outdoor flight demonstrations with 2 drones flying in formation and using 3 cameras show optimal results. The system is able to detect, track, localize and re-identifying individual drone with average positional error of 8\%. © 2021 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Yi2021,
	author={Yi, J. and Chew, K.H. and Srigrarom, S.},
	title={Enabling Continuous Drone Tracking across Translational Scene Transitions through Frame-Stitching},
	journal={2021 2nd International Symposium on Instrumentation, Control, Artificial Intelligence, and Robotics, ICA-SYMP 2021},
	year={2021},
	art_number={9358444},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85102533218\&doi=10.1109\%2fICA-SYMP50206.2021.9358444\&partnerID=40\&md5=10d74e3d4953c9de3eb9a7f800506a91},
	abstract={This paper introduces a method for enabling the continuous tracking of drones across translational scene transitions through the introduction of a stationary global frame. The main benefit of such a method is that it allows current pan-tilt-zoom (PTZ) cameras commonly used in security applications to be used in the domain of drone tracking. The first step in the process is to correct for lens distortion with the intrinsic parameters of the camera obtained through calibration. The motion of the camera frame is then estimated using the optical flow of tracked features from frame to frame. Information obtained about the translational motion of the frame is then used to construct a global frame on which object tracking is performed. Results from the comparison of object detection and tracking performed on two clips with and without pre-processing to construct the global frame show an improvement in tracking performance when the technique was applied to the video. The method was shown to successfully compensate for the relative velocity of objects in the frame relative to the frame, with no sudden changes of velocity during the scene transition. In addition, the introduction of a global frame enabled the continuous tracking of a stationary drone that was reassigned to a new track in the original video. © 2021 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Lu2021205,
	author={Lu, P. and Ding, Y. and Wang, C.},
	title={Multi-small target detection and tracking based on improved yolo and sift for drones},
	journal={International Journal of Innovative Computing, Information and Control},
	year={2021},
	volume={17},
	number={1},
	pages={205-224},
	note={cited By 2},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85100698692\&doi=10.24507\%2fijicic.17.01.205\&partnerID=40\&md5=21fe14bdf957c4f985783a73e14cf0eb},
	abstract={Multi-target tracking algorithms applied to drones often face more detection algorithm, while achieving active tracking of small targets and fast-moving targets. In response to these problems, this paper proposes a multi-small target detection and tracking method based on improved YOLO and SIFT for drones. First, we prune the network of the YOLO algorithm. Through sparse training, channel pruning, and network adjust-ment, the drone can deploy a target detection network with a smaller model. Secondly, we propose a method of adaptive threshold and minimum distance and optimize SIFT feature extraction, achieve effective detection of small targets, and improve tracking accuracy and success rate. Finally, we consider the needs of the UAV to track fast-moving targets, we use scale and position information to complete the data association, and the UAV can effectively track fast-moving targets. The algorithm of this paper is evaluat-ed by the VisDrone 2019 MOT benchmark data set. The leading evaluation indicators MOTA and MOTP are 38.7 and 75.7. The secondary evaluation indicators IDF1, ML, and FN, etc. all perform better. The algorithm meets the complex task requirements of multi-target tracking for UAVs. © ICIC International.},
	publisher={ICIC International},
}

@ARTICLE{Pavliv20211455,
	author={Pavliv, M. and Schiano, F. and Reardon, C. and Floreano, D. and Loianno, G.},
	title={Tracking and Relative Localization of Drone Swarms with a Vision-Based Headset},
	journal={IEEE Robotics and Automation Letters},
	year={2021},
	volume={6},
	number={2},
	pages={1455-1462},
	art_number={9324934},
	note={cited By 1},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85099723615\&doi=10.1109\%2fLRA.2021.3051565\&partnerID=40\&md5=7d1eab81195955500e46f1d03c8ec2c5},
	abstract={We address the detection, tracking, and relative localization of the agents of a drone swarm from a human perspective using a headset equipped with a single camera and an Inertial Measurement Unit (IMU). We train and deploy a deep neural network detector on image data to detect the drones. A joint probabilistic data association filter resolves the detection problems and couples this information with the headset IMU data to track the agents. In order to estimate the drones' relative poses in 3D space with respect to the human, we use an additional deep neural network that processes image regions of the drones provided by the tracker. Finally, to speed up the deep neural networks' training, we introduce an automated labeling process relying on a motion capture system. Several experimental results validate the effectiveness of the proposed approach. The approach is real-time, does not rely on any communication between the human and the drones, and can scale to a large number of agents, often called swarms. It can be used to spatially task a swarm of drones and also employed without a headset for formation control and coordination of terrestrial vehicles. © 2016 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Sie2021139,
	author={Sie, N.J. and Srigrarom, S. and Huang, S.},
	title={Field Test Validations of Vision-based Multi-camera Multi-drone Tracking and 3D Localizing with Concurrent Camera Pose Estimation},
	journal={2021 6th International Conference on Control and Robotics Engineering, ICCRE 2021},
	year={2021},
	pages={139-144},
	art_number={9435654},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85107766876\&doi=10.1109\%2fICCRE51898.2021.9435654\&partnerID=40\&md5=fa3061c3d01f6d685364d3cc5f65b41e},
	abstract={This paper reports the field test validations of the recently proposed vision-based real-time multi-camera setups for detecting, tracking and 3D localizing multiple aerial targets (mainly drones). We also propose the additional concurrent camera pose estimation when the camera poses are not known beforehand. This extra step can be used alongside (in parallel) with the drone tracking and localizing process. We conducted flight tests using 2 drones flying in 2 specific scenarios, and used 3 cameras to observe, detect, track and locate the positions of both drones in global frame. The efficacy of our technique is measured by the accuracy of the temporal and spatial positions of the observed drones, against the drones' own GPS recordings. Our initial results show reasonable accuracy, i.e. ±1m at 50m, as such, the proposed vision-based methods can be used for drone detection and tracking. © 2021 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Trapal2021162,
	author={Trapal, D.D.C. and Leong, B.C.C. and Ng, H.W. and Zhong, J.T.G. and Srigrarom, S. and Chan, T.H.},
	title={Improvement of Vision-based Drone Detection and Tracking by Removing Cluttered Background, Shadow and Water Reflection with Super Resolution},
	journal={2021 6th International Conference on Control and Robotics Engineering, ICCRE 2021},
	year={2021},
	pages={162-168},
	art_number={9435671},
	note={cited By 1},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85107773816\&doi=10.1109\%2fICCRE51898.2021.9435671\&partnerID=40\&md5=6acf92e6bf850762c7b7e6875c5e5303},
	abstract={Detection and tracking of small and fast moving aerial targets especially drones has got attention nowadays. This paper focuses on the vision-based technique using images taken from observing cameras. In real life situations, the target drone objects maybe are hidden in the cluttered background such as trees shadow or foliage, rows of buildings, and other kind of scenery that will hinder the clear indication of the drones. The object is further confused by the presence of its shadow and reflection from the water or glass wall reflection. For vision-based objection, the clarity and the ambiguity of the target images in the video stream are the key for effective and successful target detection and tracking. Here, we present the improvement by mitigating the effect of cluttered background, shadow and water reflection to the target images. We applied the schemes to make the drone more visible and more clear. We also implemented super resolution to increase the image resolution for more precise detection and tracking. As a result, the target drone could be detected and tracked throughout the sample clips. The comparative tracking results using DCF are presented. Likewise, we applied the water removal scheme to eliminate the reflection to avoid confusion to the tracker. With this, just the correct drone targets were detected and tracked. Overall, the drones could be detected and tracked all the way, as long as they appeared in the camera scene. © 2021 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Sie20211085,
	author={Sie, N.J. and Xuan Seah, S. and Chan, J.J. and Yi, J. and Chew, K.H. and Hooi Chan, T. and Srigrarom, S. and Holzapfel, F. and Hesse, H.},
	title={Vision-based drones tracking using correlation filters and linear integrated multiple model},
	journal={ECTI-CON 2021 - 2021 18th International Conference on Electrical Engineering/Electronics, Computer, Telecommunications and Information Technology: Smart Electrical System and Technology, Proceedings},
	year={2021},
	pages={1085-1090},
	art_number={9454735},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85112805697\&doi=10.1109\%2fECTI-CON51831.2021.9454735\&partnerID=40\&md5=8b0bcd38e95202661430602feb767ba0},
	abstract={This paper presents the use of Correlation Filters and Integrated Multiple Model (IMM) for filtering the position measurement of fast moving drones acquired by computer vision, with probability for model selection. The maneuvering movement of the drones are often non-linear making it hard to be estimated by a simple Kalman filter. Instead of using a non-linear filter which are more complex and non-universal, this paper attempt to integrate multiple filters to estimate the drone position using low computational cost. The IMM switches between the Constant Velocity (CV), Constant Acceleration (CA) and a Constant Turn (CT) model with a Markov Chain in different flight scenario depending on the drone movement. Other filters i.e. Kernelized Correlation Filter (KCF), Particle Filter (PF) and Discriminative Correlation Filter (DCF) models are also presented for direct comparison. © 2021 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Anastasiou2021927,
	author={Anastasiou, A. and Makrigiorgis, R. and Kolios, P. and Panayiotou, C.},
	title={Hyperion: A Robust Drone-based Target Tracking System},
	journal={2021 International Conference on Unmanned Aircraft Systems, ICUAS 2021},
	year={2021},
	pages={927-933},
	art_number={9476687},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85111435049\&doi=10.1109\%2fICUAS51884.2021.9476687\&partnerID=40\&md5=fd877456b5288f9b4ce307698d6fed2e},
	abstract={Recent advances in mobile computing and embedded systems have had a transformative impact in the field of Unmanned Aircraft Systems (UASs). These advances have unlocked a great number of new capabilities ranging from realtime machine learning for detection and tracking of targets, and autonomous intelligent control for mission-critical trajectory planning. This paper introduces Hyperion, a robust detect, track and follow algorithm for UASs, leveraging and integrating various computer vision techniques and a combination of two proportional integral derivative (PID) controllers for following a moving vehicle. The proposed system is evaluated under real settings using off-the-shelf hardware and an elaborated comparison is made with a variety of state-of-the-art trackers available in the OpenCV library. © 2021 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Liang20211337,
	author={Liang, N.S.J. and Srigrarom, S.},
	title={Multi-camera multi-target drone tracking systems with trajectory-based target matching and re-identification},
	journal={2021 International Conference on Unmanned Aircraft Systems, ICUAS 2021},
	year={2021},
	pages={1337-1344},
	art_number={9476845},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85111466987\&doi=10.1109\%2fICUAS51884.2021.9476845\&partnerID=40\&md5=e7d53d6af9245dca1d0efbf1acfd4fa5},
	abstract={This paper presents the integrated use of multiple cameras to detect, track and localize multiple moving objects, especially drones, in real-time by computer vision. The algorithm of the integrated system incorporates target tracking, localizing and identifying schemes, with the ability to use multiple cameras from different viewing angles and simultaneously track moving objects in the cameras' frames. Moving objects are detected by hybrid detection (motion-based blob detection appearance-based detection), and movements are predicted with Extended Kalman Filter. For motion-based detection, the trajectories of the tracked objects are analyzed using trajectory features variable. For appearance-based detection, motion is tracked with Yolo V3 detection algorithm. The integrated target identification algorithm matches and re-identifies targets between frames (intra-camera) and among cameras (inter-camera). This algorithm subsequently cross-correlate every tracked object in the different camera frames, and pair all the tracked targets to each other so that the cameras track the same objects for subsequent 3D localization. We tested our multi-cameras system to track multiple aerial and ground targets, and were successful in the re-identification of targets in real time. © 2021 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Barbary2021277,
	author={Barbary, M. and ElAzeem, M.H.A.},
	title={Drones tracking based on robust Cubature Kalman-TBD-Multi-Bernoulli filter},
	journal={ISA Transactions},
	year={2021},
	volume={114},
	pages={277-290},
	note={cited By 2},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85098634933\&doi=10.1016\%2fj.isatra.2020.12.042\&partnerID=40\&md5=b4a00dd6a26279d94484196c3f92956d},
	abstract={The problem of nonlinear tracking and detection of small unmanned aerial vehicles and micro-drone targets is very challenging and has received great attention recently. Recently, the Cubature Kalman-multi-Bernoulli filter which employs a third-degree spherical-radical cubature rule has been presented to handle the nonlinear models. The Cubature Kalman filter is more principled and accurate in mathematical terms. In addition, a recent multi-Bernoulli filter based on variational Bayesian approximation has been presented with the estimation the fluctuation of variances of measurement. However, Cubature Kalman and variational Bayesian-Multi-Bernoulli filters are unsuitable for tracking the micro-drones because of the unknown probability of detection. As we known, the track-before-detect (TBD) schemes was an effective method for tracking the small objects. In this work, a novel robust Cubature Kalman-Multi-Bernoulli filter with variational Bayesian-TBD is proposed jointing with estimate the fluctuated variances of measurement. The improved filter is an effective method to solve the problem of detection profile estimation for micro-drones. A novel implementation with a non-linear Cubature Kalman Gaussian mixture and Inverse Gamma approximation is presented to estimate a hybrid kinematic state of micro-drones. The simulation results confirm the effectiveness and robustness of the proposed algorithm. © 2020 ISA},
	publisher={ISA - Instrumentation, Systems, and Automation Society},
}

@CONFERENCE{Koryttsev2021318,
	author={Koryttsev, I. and Sheiko, S. and Kartashov, V. and Zubkov, O. and Oleynikov, V. and Selieznov, I. and Anohin, M.},
	title={Practical Aspects of Range Determination and Tracking of Small Drones by Their Video Observation},
	journal={2020 IEEE International Conference on Problems of Infocommunications Science and Technology, PIC S and T 2020 - Proceedings},
	year={2021},
	pages={318-322},
	art_number={9468047},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85114443718\&doi=10.1109\%2fPICST51311.2020.9468047\&partnerID=40\&md5=f07e95196cc57a6d79033fd1a6491e46},
	abstract={Different methods used for drones detection and estimation of their parameters (radar, acoustical, optical etc.). Among them optical methods can perform an important role in a precise definition of drones' coordinates, their tracking and recognition. The paper is devoted to the primary signal processing in the passive optical system with two channels of video observation and photosensitive matrices. The considered configuration of the optical system allows estimate a distance from a drone and realize its angle tracking on the base of measuring linear parallaxes of drones light images projected onto matrices. Experimental results include corrections of lens distortions. © 2020 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Lee202134237,
	author={Lee, D.-H.},
	title={CNN-based single object detection and tracking in videos and its application to drone detection},
	journal={Multimedia Tools and Applications},
	year={2021},
	volume={80},
	number={26-27},
	pages={34237-34248},
	note={cited By 4},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85092404216\&doi=10.1007\%2fs11042-020-09924-0\&partnerID=40\&md5=bbf486a15020d78496728649fd80ee40},
	abstract={This paper presents convolutional neural network (CNN)-based single object detection and tracking algorithms. CNN-based object detection methods are directly applicable to static images, but not to videos. On the other hand, model-free visual object tracking methods cannot detect an object until a ground truth bounding box of the target is provided. Moreover, many annotated video datasets of the target object are required to train both the object detectors and visual trackers. In this work, three simple yet effective object detection and tracking algorithms for videos are proposed to efficiently combine a state-of-the-art object detector and visual tracker for circumstances in which only a few static images of the target are available for training. The proposed algorithms are tested using a drone detection task and the experimental results demonstrated their effectiveness. © 2020, Springer Science+Business Media, LLC, part of Springer Nature.},
	publisher={Springer},
}

@ARTICLE{Natesan2010395,
	author={Natesan, K. and Gu, D.-W. and Postlethwaite, I.},
	title={Design of linear parameter varying trajectory tracking controllers for an unmanned air vehicle},
	journal={Proceedings of the Institution of Mechanical Engineers, Part G: Journal of Aerospace Engineering},
	year={2010},
	volume={224},
	number={4},
	pages={395-402},
	note={cited By 7},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-77950606002\&doi=10.1243\%2f09544100JAERO586\&partnerID=40\&md5=71bebb9c3896774cf9454a7cc486c821},
	abstract={This article presents a trajectory tracking controller design approach for an unmanned air vehicle using the linear parameter varying (LPV) methods. The longitudinal and lateral controllers are designed using an inner-outer loop structure with the inner loop LPV controller designed first using μ-synthesis. The inner loop is then approximated with a reference model and the outer loop is designed using loop-shaping techniques. Flight trajectory is expressed in terms of earth co-ordinates, which the outer loop controller converts into reference signals for the inner loop. Full-scale non-linear simulations are used to test the efficiency of the designed controller and of the proposed design approach.},
}

@CONFERENCE{Natesan2008,
	author={Natesan, K. and Gu, D. and Postlethwaite, I.},
	title={Trajectory tracking controller design for an unmanned air vehicle},
	journal={IFAC Proceedings Volumes (IFAC-PapersOnline)},
	year={2008},
	volume={17},
	number={1 PART 1},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-79961018252\&doi=10.3182\%2f20080706-5-KR-1001.0846\&partnerID=40\&md5=12b12223c9ffa9e5726884dc271e5c70},
	abstract={This paper presents a complete trajectory tracking controller design for an Unmanned Air Vehicle using Linear Parameter Varying design methods. The longitudinal and lateral controllers are designed using an inner loop - outer loop structure with the inner loop LPV controller designed using μ -synthesis. The inner-loop is then approximated with a reference model and the outer loop is designed using loop-shaping techniques. Full scale nonlinear simulations are used to test the efficiency of the designed controller and of the proposed design approach. Copyright © 2007 International Federation of Automatic Control All Rights Reserved.},
}

@CONFERENCE{Kartashov2019,
	author={Kartashov, V. and Oleynikov, V. and Zubkov, O. and Sheiko, S.},
	title={Optical detection of unmanned air vehicles on a video stream in a real-time},
	journal={2019 International Conference on Information and Telecommunication Technologies and Radio Electronics, UkrMiCo 2019 - Proceedings},
	year={2019},
	art_number={9165362},
	note={cited By 2},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85091703254\&doi=10.1109\%2fUkrMiCo47782.2019.9165362\&partnerID=40\&md5=88aad692c12ea5d33a8e8d47dd9a1fd0},
	abstract={The paper describes the research connected with motion detection of small unmanned air vehicles on a video stream. The most comprehensive detection methods are analyzed and investigated with a real video shooting. The research shows that the differential method is more reliable in the authenticity of motion detection and may be considered as a base for practical systems. © 2019 IEEE},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Yu20189635,
	author={Yu, Q. and Yao, H. and He, F. and Qi, H.},
	title={U-Net Based Moving Target Detection for Unmanned Air Vehicles},
	journal={Chinese Control Conference, CCC},
	year={2018},
	volume={2018-July},
	pages={9635-9640},
	art_number={8483331},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85056106998\&doi=10.23919\%2fChiCC.2018.8483331\&partnerID=40\&md5=728fa39051b8dd57f7538e13f1e40164},
	abstract={In this paper, a moving target detection problem is investigated for the unmanned air vehicles with a monocular vision sensor. First, a detection algorithm based on U-Net network is proposed to obtain the position and velocity direction of a moving target. Then, a Kalman Filter is incorporated into the proposed algorithm to increase the accuracy of states acquisition of the moving targets. Then, the experimental results show the proposed algorithm has low computation and better performance. © 2018 Technical Committee on Control Theory, Chinese Association of Automation.},
	publisher={IEEE Computer Society},
}

@CONFERENCE{Yao201711459,
	author={Yao, H. and Yu, Q. and Xing, X. and He, F. and Ma, J.},
	title={Deep-learning-based moving target detection for unmanned air vehicles},
	journal={Chinese Control Conference, CCC},
	year={2017},
	pages={11459-11463},
	art_number={8029186},
	note={cited By 7},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85032226732\&doi=10.23919\%2fChiCC.2017.8029186\&partnerID=40\&md5=bf5444545afd0c019aba71ec5c4896a4},
	abstract={In this paper, a deep learning network is investigated to detect moving targets for a UAV equipped with monocular camera. An algorithm based on fully convolutional network is proposed to obtain the position and moving direction of targets. A Kalman filter is incorporated into the proposed algorithm to increase the accuracy of target position information acquisition. The experimental results show the effectiveness of the proposed algorithm with a relatively low hardware resource consumption. © 2017 Technical Committee on Control Theory, CAA.},
	publisher={IEEE Computer Society},
}



% ==============================================================================================
% ==============================================================================================
% ==============================================================================================
\section{UAV Detection and Tracking using Cameras, Acoustic, and Radar (Multiple Sensor)} % 1 Paper

@CONFERENCE{Vasquez2008,
	author={Vasquez, J.R. and Tarplee, K.M. and Case, E.E. and Zelnio, A.M. and Rigling, B.D.},
	title={Multisensor 3D tracking for counter small unmanned air vehicles (CSUAV)},
	journal={Proceedings of SPIE - The International Society for Optical Engineering},
	year={2008},
	volume={6971},
	art_number={697107},
	note={cited By 11},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-79959405651\&doi=10.1117\%2f12.785531\&partnerID=40\&md5=8ae9d421d65fafc0310fdbc92f42bbb3},
	abstract={A variety of unmanned air vehicles (UAVs) have been developed for both military and civilian use. The typical large UAV is typically state owned, whereas small UAVs (SUAVs) may be in the form of remote controlled aircraft that are widely available. The potential threat of these SUAVs to both the military and civilian populace has led to research efforts to counter these assets via track, ID, and attack. Difficulties arise from the small size and low radar cross section when attempting to detect and track these targets with a single sensor such as radar or video cameras. In addition, clutter objects make accurate ID difficult without very high resolution data, leading to the use of an acoustic array to support this function. This paper presents a multi-sensor architecture that exploits sensor modes including EO/IR cameras, an acoustic array, and future inclusion of a radar. A sensor resource management concept is presented along with preliminary results from three of the sensors.},
}

% ==============================================================================================
% ==============================================================================================
% ==============================================================================================
\section{UAV Detection and Tracking using Thermal Sensor} % 1 Paper

@ARTICLE{Beranek2021260,
	author={Beranek, C.T. and Roff, A. and Denholm, B. and Howell, L.G. and Witt, R.R.},
	title={Trialling a real-time drone detection and validation protocol for the koala (Phascolarctos cinereus)},
	journal={Australian Mammalogy},
	year={2021},
	volume={43},
	number={2},
	pages={260-264},
	note={cited By 3},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85087788781\&doi=10.1071\%2fAM20043\&partnerID=40\&md5=1030cd895d14b4daa182b277c7349103},
	abstract={Remotely piloted aircraft system (RPAS), or drone, technology has emerged as a promising survey method for the cryptic koala. We demonstrate an in-field protocol for wild koala RPAS surveys which provides real-time validation of thermal signatures. During 15 trial flights using a quadcopter drone (DJI Matrice 200 v2) we successfully detected and validated koala thermal signatures (n = 12) using two in-field approaches: Validation by on-ground observer (n = 10) and validation using 4K footage captured and reviewed directly after the survey (n = 2). We also provide detectability considerations relative to survey time, temperature, wildlife-RPAS interactions and detection of non-target species, which can be used to further inform RPAS survey protocols. © 2021 CSIRO. All rights reserved.},
	publisher={CSIRO},
}

\section{UAV Detection and Tracking using Visible, Thermal and Acoustic (Multiple Sensor)} % 2 Paper

@CONFERENCE{Svanström20207265,
	author={Svanström, F. and Englund, C. and Alonso-Fernandez, F.},
	title={Real-time drone detection and tracking with visible, thermal and acoustic sensors},
	journal={Proceedings - International Conference on Pattern Recognition},
	year={2020},
	pages={7265-7272},
	art_number={9413241},
	note={cited By 6},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85109250336\&doi=10.1109\%2fICPR48806.2021.9413241\&partnerID=40\&md5=2fca213bab1dd99da7d217f33a31f4af},
	abstract={This paper explores the process of designing an automatic multi-sensor drone detection system. Besides the common video and audio sensors, the system also includes a thermal infrared camera, which is shown to be a feasible solution to the drone detection task. Even with slightly lower resolution, the performance is just as good as a camera in visible range. The detector performance as a function of the sensor-to-target distance is also investigated. In addition, using sensor fusion, the system is made more robust than the individual sensors, helping to reduce false detections. To counteract the lack of public datasets, a novel video dataset containing 650 annotated infrared and visible videos of drones, birds, airplanes and helicopters is also presented1. The database is complemented with an audio dataset of the classes drones, helicopters and background noise. © 2020 IEEE},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Svanström20207265,
	author={Svanström, F. and Englund, C. and Alonso-Fernandez, F.},
	title={Real-time drone detection and tracking with visible, thermal and acoustic sensors},
	journal={Proceedings - International Conference on Pattern Recognition},
	year={2020},
	pages={7265-7272},
	art_number={9413241},
	note={cited By 6},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85109250336\&doi=10.1109\%2fICPR48806.2021.9413241\&partnerID=40\&md5=2fca213bab1dd99da7d217f33a31f4af},
	abstract={This paper explores the process of designing an automatic multi-sensor drone detection system. Besides the common video and audio sensors, the system also includes a thermal infrared camera, which is shown to be a feasible solution to the drone detection task. Even with slightly lower resolution, the performance is just as good as a camera in visible range. The detector performance as a function of the sensor-to-target distance is also investigated. In addition, using sensor fusion, the system is made more robust than the individual sensors, helping to reduce false detections. To counteract the lack of public datasets, a novel video dataset containing 650 annotated infrared and visible videos of drones, birds, airplanes and helicopters is also presented1. The database is complemented with an audio dataset of the classes drones, helicopters and background noise. © 2020 IEEE},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}


% ==============================================================================================
% ==============================================================================================
% ==============================================================================================
\section{UAV Detection and Tracking using RF} % 16 Paper

@ARTICLE{Solomitckii201843,
	author={Solomitckii, D. and Gapeyenko, M. and Semkin, V. and Andreev, S. and Koucheryavy, Y.},
	title={Technologies for Efficient Amateur Drone Detection in 5G Millimeter-Wave Cellular Infrastructure},
	journal={IEEE Communications Magazine},
	year={2018},
	volume={56},
	number={1},
	pages={43-50},
	art_number={8255736},
	note={cited By 65},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85040720734\&doi=10.1109\%2fMCOM.2017.1700450\&partnerID=40\&md5=78d5cd7bc30d2f75041145e26ed4b126},
	abstract={Unmanned aerial vehicles, also called drones, are recently gaining increased research attention across various fields due to their flexibility and application potential. The steady increase in the number of amateur drones demands more stringent regulations on their allowed route, mass, and load. However, these regulations may be violated accidentally or deliberately. In these cases, spying with drones, transfer of dangerous payloads, or losing reliable drone control can represent a new hazard for people, governments, and business sector. The technologies to detect, track, and disarm possible aerial threats are therefore in prompt demand. To this end, ubiquitous cellular networks, and especially 5G infrastructures based on the use of millimeter-wave radio modules, may be efficiently leveraged to offer the much needed drone detection capabilities. In this work, we propose to exploit 5G millimeter-wave deployments to detect violating amateur drones. We argue that the prospective 5G infrastructure may provide all the necessary technology elements to support efficient detection of small-sized drones. We therefore outline a novel technology and system design perspective, including such considerations as the density of base stations, their directional antennas, and the available bandwidth, among others, as well as characterize their impact with our ray-based modeling methods. © 1979-2012 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Basak20181,
	author={Basak, S. and Scheers, B.},
	title={Passive radio system for real-time drone detection and DoA estimation},
	journal={2018 International Conference on Military Communications and Information Systems, ICMCIS 2018},
	year={2018},
	pages={1-6},
	note={cited By 9},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85050262355\&doi=10.1109\%2fICMCIS.2018.8398721\&partnerID=40\&md5=91d132200c12b2b910ad9b216ac974d6},
	abstract={The principal objective behind the development of passive radio system is to detect and localize mini remotely piloted aircraft systems (RPAS) and their operators in three dimensions (3D). This paper describes the system architecture, detection procedure and intermediate test results. Goodness-of-Fit (GoF) based spectrum sensing is used to detect the frequency of the transmitted signal of mini-RPAS and its controller. The direction of arrival (DoA) is estimated with the MUSIC algorithm. The implementation of GoF-based wideband spectrum sensing and one dimensional DoA estimation including spatial smoothing and automatic source number detection are detailed in this paper. Several test results are presented to validate the real time operation of the passive radio system. © 2018 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Bello2019,
	author={Bello, A. and Biswal, B. and Shetty, S. and Kamhoua, C. and Gold, K.},
	title={Radio frequency classification toolbox for drone detection},
	journal={Proceedings of SPIE - The International Society for Optical Engineering},
	year={2019},
	volume={11006},
	art_number={110061Y},
	note={cited By 2},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85072574963\&doi=10.1117\%2f12.2514759\&partnerID=40\&md5=e14fe88cfefbab09beb3625798aa87e6},
	abstract={There is a need for Radio Frequency Signal Classification (RF-Class) toolbox which can monitor, detect, and classify wireless signals. Rapid developments in the unmanned aerial systems (UAS) have made its usage in a variety of offensive as well as defensive applications especially in military, high priority and sensitive government sites. The ability to accurately classify over-The-Air radio signals will provide insights into spectrum utilization, device fingerprinting and protocol identification. These insights can help the Warfighter to constantly be informed about adversarys transmitters capabilities without their knowledge. Recently, few researches have proposed feature-based machine learning techniques to classify RF signals. However, these researches are mostly evaluated on simulated environments, less accurate, and failed to explore advance machine learning techniques. In this research, we proposed a feature-engineering based signal classification (RF-class) toolbox which implements RF signal detection, Cyclostationary Features Extraction and Feature engineering, Automatic Modulation Recognition to automatically recognize modulation as well as sub-modulation types of the received signal. To demonstrate the feasibility and accuracy of our approach, we have evaluated the performance on a real environment with an UAS (Drone DJI Phantom 4). Our initial experimental result showed that we were able to detect presence of drone signal successfully when power on and transmitting. And further experiments are under progress. © COPYRIGHT SPIE. Downloading of the abstract is permitted for personal use only.},
	publisher={SPIE},
}

@CONFERENCE{Minz2019,
	author={Minz, L. and Kang, H.-S. and Azim, M.T. and Aziz, R.S. and Park, S.-O.},
	title={Wide-beam Choke Horn Antenna for Small Drone Detection},
	journal={ISAP 2018 - 2018 International Symposium on Antennas and Propagation},
	year={2019},
	art_number={8627548},
	note={cited By 1},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85062788915\&partnerID=40\&md5=3e2d7097a0318eb5756f5897e754b070},
	abstract={A conventional narrow beam scanning antenna radar systems are inept in detection of small RCS drones. A wide-beam choke horn antennas are proposed for the surveillance system in order to detect and track a small object like drones. The proposed choke horn antenna is derived from sector beam pattern synthesis. The designed antenna has a wide beam width of 700 and has a low field level in the horizontal plane (-40dB w.r.t. main beam), which is crucial for high isolation among Rx and between Tx and Rx as well. © 2018 KIEES.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Ryden2019,
	author={Ryden, H. and Redhwan, S.B. and Lin, X.},
	title={Rogue Drone Detection: A Machine Learning Approach},
	journal={IEEE Wireless Communications and Networking Conference, WCNC},
	year={2019},
	volume={2019-April},
	art_number={8886040},
	note={cited By 7},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85074749102\&doi=10.1109\%2fWCNC.2019.8886040\&partnerID=40\&md5=0e3d6ad15ea9cd96bbf85be2382f3680},
	abstract={The emerging, practical and observed issue of how to detect rogue drones carrying terrestrial user equipment (UE) on mobile networks is addressed in this paper. This issue has drawn much attention since the rogue drones may generate excessive interference to mobile networks and may not be allowed by regulations in some regions. In this paper, we propose a novel machine learning approach to identify the rogue drones in mobile networks based on radio measurements. We apply two classification machine learning models, Logistic Regression, and Decision Tree, using features from radio measurements to identify the rogue drones. Simulation results show that the proposed machine learning solutions can achieve high rogue drone detection rate for high altitudes while not mis-classifying regular ground based UEs as rogue drone UEs. © 2019 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Al-Sa'd201986,
	author={Al-Sa'd, M.F. and Al-Ali, A. and Mohamed, A. and Khattab, T. and Erbad, A.},
	title={RF-based drone detection and identification using deep learning approaches: An initiative towards a large open source drone database},
	journal={Future Generation Computer Systems},
	year={2019},
	volume={100},
	pages={86-97},
	note={cited By 44},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85065643831\&doi=10.1016\%2fj.future.2019.05.007\&partnerID=40\&md5=70cec981a0d638ffc1f8c6eed12edd9d},
	abstract={The omnipresence of unmanned aerial vehicles, or drones, among civilians can lead to technical, security, and public safety issues that need to be addressed, regulated and prevented. Security agencies are in continuous search for technologies and intelligent systems that are capable of detecting drones. Unfortunately, breakthroughs in relevant technologies are hindered by the lack of open source databases for drone's Radio Frequency (RF) signals, which are remotely sensed and stored to enable developing the most effective way for detecting and identifying these drones. This paper presents a stepping stone initiative towards the goal of building a database for the RF signals of various drones under different flight modes. We systematically collect, analyze, and record raw RF signals of different drones under different flight modes such as: off, on and connected, hovering, flying, and video recording. In addition, we design intelligent algorithms to detect and identify intruding drones using the developed RF database. Three deep neural networks (DNN) are used to detect the presence of a drone, the presence of a drone and its type, and lastly, the presence of a drone, its type, and flight mode. Performance of each DNN is validated through a 10-fold cross-validation process and evaluated using various metrics. Classification results show a general decline in performance when increasing the number of classes. Averaged accuracy has decreased from 99.7\% for the first DNN (2-classes), to 84.5\% for the second DNN (4-classes), and lastly, to 46.8\% for the third DNN (10-classes). Nevertheless, results of the designed methods confirm the feasibility of the developed drone RF database to be used for detection and identification. The developed drone RF database along with our implementations are made publicly available for students and researchers alike. © 2019 Elsevier B.V.},
	publisher={Elsevier B.V.},
}

@CONFERENCE{Sharma2019449,
	author={Sharma, V. and Kumari, M.},
	title={Drone Detection Mechanism using Radio communication Technology and Internet Protocol Address},
	journal={Proceedings of the 2nd International Conference on Smart Systems and Inventive Technology, ICSSIT 2019},
	year={2019},
	pages={449-453},
	art_number={8987972},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85080062789\&doi=10.1109\%2fICSSIT46314.2019.8987972\&partnerID=40\&md5=841ab7a7f0dfe415a5a6493f289254b6},
	abstract={Unmanned Aerial Vehicles (UAVs) are among the real significant advances that have various significant and advantageous applications. But recently the threats imposed by Unmanned Aerial Vehicles (UAVs), especially small drones, have increased to a greater extent. Unmanned Aerial Vehicles(UAVs) are being misused nowadays for various illegal activities including terrorism and smuggling. Recently, there have been situations where they enter private or confined property. To kill such exercises, a framework has been structured which can distinguish and detect the nearness of obscure little aerial targets, for example, Unmanned Aerial Vehicles (UAVs), specifically small drones. The system is based on the concept of Radio Communication(RC) technology and Internet Protocol(IP) address. This framework is devised such that it detects Internet Protocol(IP) addresses in certain range and using the detected Internet Protocol(IP) addresses and presence or absence of radio waves, detects the presence of Unmanned Aerial Vehicles(UAVs). This system is capable of detecting the presence of unknown Unmanned Aerial Vehicles(UAVs) in certain range. This paper reports on the prototype of the same. © 2019 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Allahham2020112,
	author={Allahham, M.S. and Khattab, T. and Mohamed, A.},
	title={Deep Learning for RF-Based Drone Detection and Identification: A Multi-Channel 1-D Convolutional Neural Networks Approach},
	journal={2020 IEEE International Conference on Informatics, IoT, and Enabling Technologies, ICIoT 2020},
	year={2020},
	pages={112-117},
	art_number={9089657},
	note={cited By 8},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85085474950\&doi=10.1109\%2fICIoT48696.2020.9089657\&partnerID=40\&md5=9bfa150bcc4868e361e8a1b11465ffa8},
	abstract={Commercial unmanned aerial vehicles, or drones, are getting increasingly popular in the last few years. The fact that these drones are highly accessible to public may bring a range of security and technical issues to sensitive areas such as airfields and military bases. Consequently, drone detection and state identification are becoming very crucial and essential for governments and security agencies. This paper proposes a deep learning based approach for drone detection, type identification and state identification using a multi-channel 1-dimensional convolutional neural network. The deep learning model is trained utilizing a publicly published database for drone's radio frequency signals. The proposed model can be used to produce new features that can represent the whole dataset in a more compact form which enables the use of classical machine learning algorithms for classification. © 2020 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Al-Emadi202029,
	author={Al-Emadi, S. and Al-Senaid, F.},
	title={Drone Detection Approach Based on Radio-Frequency Using Convolutional Neural Network},
	journal={2020 IEEE International Conference on Informatics, IoT, and Enabling Technologies, ICIoT 2020},
	year={2020},
	pages={29-34},
	art_number={9089489},
	note={cited By 12},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85085478429\&doi=10.1109\%2fICIoT48696.2020.9089489\&partnerID=40\&md5=e9652f8067c99f9d4b2398018e913222},
	abstract={Recently, Unmanned Aerial Vehicles, also known as drones, are becoming rapidly popular due to the advancement of their technology and the significant decrease in their cost. Although commercial drones have proven their effectiveness in many day to day applications such as cinematography, agriculture monitoring and search and rescue, they are also being used in malicious activities that are targeting to harm individuals and societies which raises great privacy, safety and security concerns. In this research, we propose a new drone detection solution based on the Radio Frequency (RF) emitted during the live communication session between the drone and its controller using a Deep Learning (DL) technique, namely, the Convolutional Neural Network (CNN). The results of the study have proven the effectiveness of using CNN for drone detection with accuracy and F1 score of over 99.7\% and drone identification with accuracy and F1 score of 88.4\%. Moreover, the results yielded from this experiment have outperformed those reported in the literature for RF based drone detection using Deep Neural Networks. © 2020 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{M.Alaboudi2020278,
	author={M. Alaboudi, M. and Abu Talib, M. and Nasir, Q.},
	title={Radio frequency-based techniques of drone detection and classification using machine learning},
	journal={ACM International Conference Proceeding Series},
	year={2020},
	pages={278-282},
	art_number={3449348},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85108145264\&doi=10.1145\%2f3449301.3449348\&partnerID=40\&md5=419d1472ae846696eb3660f5f791c579},
	abstract={This research paper provides a comprehensive survey review on drone detection using Radio Frequency (RF)-based techniques along with machine learning and localization algorithms. RF signals proved its effectiveness in detecting drones, however, due to the lack of a published survey, this research paper reviews the newly emerged RF-based techniques by addressing the implemented methods and discussing the results obtained in terms of the testing environment, range of detection and accuracy of the system. In this survey review, thirty conference and journal papers have been collected, however only selected papers have been discussed depending on the contribution and limited space of the paper. Finally, this survey also discusses the challenges encountered in drone detection using RF due to its great impact on the efficiency of the system. © 2020 ACM.},
	publisher={Association for Computing Machinery},
}

@CONFERENCE{Almasri2021208,
	author={Almasri, M.},
	title={Deep learning for RF-based drone detection and identification using welch's method},
	journal={Proceedings of the 10th International Conference on Data Science, Technology and Applications, DATA 2021},
	year={2021},
	pages={208-214},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85111768869\&doi=10.5220\%2f0010530302080214\&partnerID=40\&md5=486752452eaf8696da50c2b6336f4fc9},
	abstract={Radio Frequency (RF) combined with the deep learning methods promised a solution to detect the presence of the drones. Indeed, the classical techniques (i.e. radar, vision and acoustics, etc.) suffer several drawbacks such as difficult to detect the small drones, false alarm of flying birds or balloons, the influence of the wind on the performance, etc. For an effective drones's detection, two main stages should be established: Feature extraction and feature classification. The proposed approach in this paper is based on a novel feature extraction method and an optimized deep neural network (DNN). At first, we present a novel method based on Welch to extract meaningful features from the RF signal of drones. Later on, three optimized Deep Neural Network (DNN) models are considered to classify the extracted features. The first DNN model can be used to detect the presence of the drones and contains two classes. The second DNN help us to detect and recognize the type of the drone with 4 classes: A class for each drone and the last one for the RF background activities. In the third model, 10 classes have been considered: the presence of the drone, its type, and its flight mode (i.e. Stationary, Hovering, flying with or without video recording). Our proposed approach can achieve an average accuracy higher than 94\% and it significantly improves the accuracy, up to 30\%, compared to existing methods. Copyright © 2021 by SCITEPRESS - Science and Technology Publications, Lda. All rights reserved},
	publisher={SciTePress},
}

@CONFERENCE{Zhang2021425,
	author={Zhang, Y.},
	title={RF-based drone detection using machine learning},
	journal={Proceedings - 2021 2nd International Conference on Computing and Data Science, CDS 2021},
	year={2021},
	pages={425-428},
	art_number={9463220},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85112395611\&doi=10.1109\%2fCDS52072.2021.00079\&partnerID=40\&md5=856c415a7a8f9f95c14fafaa59fa790f},
	abstract={Drones or unmanned aerial vehicles have become a new option for multiple tasks including delivery, photograph, etc. However, the small size and flight ability of drones make it easier to break through any barriers and intrude important facilities. With an increasing safety concern of drone incursions, the research for an effective drone detection and identification approach has drawn a lot of attention in recent years. Among existing methods, passive radio frequency sensing is both reliable and cost-effective. However, previous studies are evaluating both machine learning and statistical methods on private datasets under different settings. To make a fair comparison, we evaluate six machine learning models on an open drone dataset for RF-based drone detection in this paper. The results demonstrate that XGBoost achieves the state-of-the-art results on this pioneering dataset. © 2021 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Basak2021,
	author={Basak, S. and Rajendran, S. and Pollin, S. and Scheers, B.},
	title={Combined RF-based drone detection and classification},
	journal={IEEE Transactions on Cognitive Communications and Networking},
	year={2021},
	note={cited By 2},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85112640839\&doi=10.1109\%2fTCCN.2021.3099114\&partnerID=40\&md5=5d3f7866c1bb0dd90849ea26a59dd5b0},
	abstract={Despite several beneficial applications, unfortunately, drones are also being used for illicit activities such as drug trafficking, firearm smuggling or to impose threats to security-sensitive places like airports and nuclear power plants. The existing drone localization and neutralization technologies work on the assumption that the drone has already been detected and classified. Although we have observed a tremendous advancement in the sensor industry in this decade, there is no robust drone detection and classification method proposed in the literature yet. This paper focuses on radio frequency (RF) based drone detection and classification using the frequency signature of the transmitted signal. We have created a novel drone RF dataset using commercial drones and presented a detailed comparison between a two-stage and combined detection and classification framework. The detection and classification performance of both frameworks are presented for a single-signal and simultaneous multi-signal scenario. With detailed analysis, we show that You Only Look Once (YOLO) framework provides better detection performance compared to the Goodness-of-Fit (GoF) spectrum sensing for a simultaneous multi-signal scenario and good classification performance comparable to Deep Residual Neural Network (DRNN) framework. IEEE},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Flak2021114574,
	author={Flak, P.},
	title={Drone Detection Sensor with Continuous 2.4 GHz ISM Band Coverage Based on Cost-Effective SDR Platform},
	journal={IEEE Access},
	year={2021},
	volume={9},
	pages={114574-114586},
	art_number={9513316},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113316401\&doi=10.1109\%2fACCESS.2021.3104738\&partnerID=40\&md5=cfd5a2b504fc46cfcdab4c7397ebc30a},
	abstract={The development of Unmanned Aerial Vehicles (UAVs), commonly referred to as drones, has introduced revolutionary changes in many areas over the past few years. However, aside from opening new possibilities, the usage of drones in an irresponsible and dangerous manner leads to many hazardous incidents. This paper presents a drone detection sensor with a continuous 2.400 GHz-2.483 GHz operational frequency range for detection methods based on passive radio frequency imaging techniques. The implementation based on Software Defined Radio (SDR) and Field Programmable Logic Array (FPGA) hardware that overcomes the 40 MHz real-time bandwidth limit of other popular SDRs is presented utilizing low-cost off-the-shelf components. Furthermore, a hardware realization of the signal processing chain for specific detection algorithms is proposed to minimize the throughput between SDR and the companion computer and offload software computations. The device validation is made in a laboratory and real-life scenario and presented in relation to the sensor used in other works. In addition to the increased real-time bandwidth, the measurements show a 9 dB reduction in detection sensitivity compared to the reference receiver, in line with the analog RF front-end specifications. The final analysis demonstrates the proposed device's relevance as a sensor for obtaining machine learning datasets and as a part of a final anti-drone system. © 2013 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Medaiyese202158,
	author={Medaiyese, O.O. and Syed, A. and Lauf, A.P.},
	title={Machine Learning Framework for RF-Based Drone Detection and Identification System},
	journal={Proceedings of 2nd 2021 International Conference on Smart Cities, Automation and Intelligent Computing Systems, ICON-SONICS 2021},
	year={2021},
	pages={58-64},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85123055247\&doi=10.1109\%2fICON-SONICS53103.2021.9617168\&partnerID=40\&md5=ef3a8626d21290ba24223510f0d64b3e},
	abstract={The emergence of drones has added a new dimension to privacy and security issues. There are little or no strict regulations on the people that can purchase or own a drone. For this reason, people can take advantage of these aircraft to intrude into restricted or private areas. A drone detection and identification (DDI) system is one of the ways of detecting and identifying the presence of a drone in an area. DDI systems can employ different sensing techniques such as radio frequency (RF) signals, video, sounds, and thermal imaging for detecting an intruding drone. In this work, we propose a machine learning RF-based DDI system that uses low band RF signals from drone-to-flight controller communication. We develop three machine learning models using the XGBoost algorithm to detect and identify the presence of a drone, the type of the drone, and the operational mode of drones. For these three XGBoost models, we evaluated the models using 10-fold cross validation and we achieve average accuracy of 99.96\%, 90.73\%, and 70.09\% respectively. © 2021 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Aledhari2021,
	author={Aledhari, M. and Razzak, R. and Parizi, R.M. and Srivastava, G.},
	title={Sensor Fusion for Drone Detection},
	journal={IEEE Vehicular Technology Conference},
	year={2021},
	volume={2021-April},
	art_number={9448699},
	note={cited By 2},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85112401473\&doi=10.1109\%2fVTC2021-Spring51267.2021.9448699\&partnerID=40\&md5=2d1ddefc7484a1fa71b3b18e8bd9500b},
	abstract={With the rapid development of commercial drones, drone detection and classification have emerged and grown recently. Drone detection works to detect unmanned aerial vehicles (UAVs). Usually, systems for drone detection utilize a combination of one or more sensors and some methodology. Many unique technologies and methods are used to detect drones. However, each type of technology offers its benefits and limitations. Most approaches use computer vision or machine learning, but one methodology that has not been given much attention is Sensor Fusion. Sensor Fusion has less uncertainty than most methods, making it suitable for drone detection. In this paper, we propose an artificial neural network-based detection system that uses a deep neural network (DNN) to process the RF data and a convolutional neural network (CNN) to process image data. The features from CNNs and DNNs are concatenated and input into another DNN, which outputs a single prediction score of drone presence. Our model achieved a validation accuracy of 75\% that shows the feasibility of a sensor fusion based technique for drone detection. © 2021 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

\section{UAV Detection and Tracking using Radar} % 54 Paper

@CONFERENCE{Häfner2018,
	author={Häfner, S. and Röding, M. and Sommerkorn, G. and Müller, R. and Thomä, R.S. and Del Galdo, G. and Goerlich, J.},
	title={Contribution to drone detection by exploiting parameter estimation for a prototype mm-wave radar system},
	journal={WSA 2018 - 22nd International ITG Workshop on Smart Antennas},
	year={2018},
	note={cited By 4},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85081589669\&partnerID=40\&md5=fa255759863f850eb84c39d254144dca},
	abstract={An estimator to infer parameters from radar measurements is presented, applicable for further detection and localisation of unmanned aircraft systems. The problem of parameter estimation is presented as an inverse problem, necessitating a model of the measurement data. Based on the data model, a maximum-likelihood based objective function is derived. The objective function is minimised by a framework similar to the RIMAX framework, including joint parameter and model order estimation. A SIMO radar system is presented and employed to test and demonstrate the estimators capability in simulations as well as test measurements with flying UASs. © 2018 VDE VERLAG GMBH ∙ Berlin ∙ Offenbach},
	publisher={VDE Verlag GmbH},
}

@CONFERENCE{Jian20181146,
	author={Jian, M. and Lu, Z. and Chen, V.C.},
	title={Drone detection and tracking based on phase-interferometric Doppler radar},
	journal={2018 IEEE Radar Conference, RadarConf 2018},
	year={2018},
	pages={1146-1149},
	note={cited By 33},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85049928482\&doi=10.1109\%2fRADAR.2018.8378723\&partnerID=40\&md5=72e95fda4ec128ff0efa9abff67b10ea},
	abstract={In this paper, drone detection and tracking based on phase-interferometry are investigated. Data collected by a simple dual-channel Doppler radar is used for implementing the joint range-Doppler-azimuth processing. Experimental results show that micro drones can be detected and tracked by applying the joint range-Doppler-azimuth processing. Features extracted from the range-Doppler-azimuth domain can be used to identify drones. © 2018 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Fang201833542,
	author={Fang, G. and Yi, J. and Wan, X. and Liu, Y. and Ke, H.},
	title={Experimental Research of Multistatic Passive Radar with a Single Antenna for Drone Detection},
	journal={IEEE Access},
	year={2018},
	volume={6},
	pages={33542-33551},
	note={cited By 29},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85048170961\&doi=10.1109\%2fACCESS.2018.2844556\&partnerID=40\&md5=878b8d68a98c82f29f207d24d04066e6},
	abstract={Digital television signals are attractive illuminations of opportunity for the passive radars in the field of low altitude and slow speed target detection. The digital television standard permits reconstruction of a reference signal using the received signal in surveillance channel, which enables a single-antenna digital television based passive radar (SDPR) processing. This paper investigates the practical feasibility of a multistatic SDPR (MSDPR) for the drone detection. First, the detection range of the SDPR is analyzed in terms of signal processing procedures involving multipath energy, extracted reference signal purity, and receiving antenna. Second, according to the characteristics of the SDPR, the reference signal extraction is analyzed. In addition, considering that the SDPR cannot locate and track the detected target, a novel MSDPR processing method is proposed. The core idea of this method is to use the optimal reference signal extracted from the receiving station with the least interference as the shared reference signal in MSDPR, which can greatly improve the system detection capability. Finally, the small drone detection experiments using the MSDPR are presented. The theoretical considerations are demonstrated using the experimental data. © 2013 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Kim2018188,
	author={Kim, B.-K. and Park, J. and Park, S.-J. and Kim, T.-W. and Jung, D.-H. and Kim, D.-H. and Kim, T. and Park, S.-O.},
	title={Drone Detection with Chirp-Pulse Radar Based on Target Fluctuation Models},
	journal={ETRI Journal},
	year={2018},
	volume={40},
	number={2},
	pages={188-196},
	note={cited By 8},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85045404841\&doi=10.4218\%2fetrij.2017-0090\&partnerID=40\&md5=0823d2152394c92c06ab01d1c8041473},
	abstract={This paper presents a pulse radar system to detect drones based on a target fluctuation model, specifically the Swerling target model. Because drones are small atypical objects and are mainly composed of non-conducting materials, their radar cross-section value is low and fluctuating. Therefore, determining the target fluctuation model and applying a proper integration method are important. The proposed system is herein experimentally verified and the results are discussed. A prototype design of the pulse radar system is based on radar equations. It adopts three different pulse modes and a coherent pulse integration to ensure a high signal-to-noise ratio. Outdoor measurements are performed with a prototype radar system to detect Doppler frequencies from both the drone frame and blades. The results indicate that the drone frame and blades are detected within an instrumental maximum range. Additionally, the results show that the drone's frame and blades are close to the Swerling 3 and 4 target models, respectively. By the analysis of the Swerling target models, proper integration methods for detecting drones are verified and can thus contribute to increasing in detectability. © 2018 ETRI},
	publisher={John Wiley and Sons Inc.},
}

@CONFERENCE{DeQuevedo2018,
	author={De Quevedo, A.D. and Urzaiz, F.I. and Menoyo, J.G. and Lopez, A.A.},
	title={Drone detection with x-band ubiquitous radar},
	journal={Proceedings International Radar Symposium},
	year={2018},
	volume={2018-June},
	art_number={8447942},
	note={cited By 8},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85053624493\&doi=10.23919\%2fIRS.2018.8447942\&partnerID=40\&md5=c6321d18df2b5cb6fe83590a82ffa7ed},
	abstract={This paper presents the design and experimental results on commercial-drone detection with a ubiquitous frequency modulated continuous wave (FMCW) radar system demonstrator, working at 8.75 GHz (X-band). The demonstrator is introduced and its main blocks are described, with particular attention to the PC-based signal processor. Subsequently, the document presents the chosen scenario for the tests, and shows the results of the offline processing, achieving a DJI-Phantom-4 detection at a range up to 2 km. The results are illustrated with range-Doppler matrices and detection figures. Range, speed and azimuth accuracies are discussed, considering the drone GPS data. Finally, the paper introduces statistical radar-cross-section (RCS) studies based on the processed data, in order to classify the drone as a Swerling target, and discusses the drone average RCS. © 2018 German Institute of Navigation - DGON.},
	publisher={IEEE Computer Society},
}

@CONFERENCE{Stasiak2018521,
	author={Stasiak, K. and Ciesielski, M. and Kurowska, A. and Przybysz, W.},
	title={A study on using different kinds of continuous-wave radars operating in C-band for drone detection},
	journal={MIKON 2018 - 22nd International Microwave and Radar Conference},
	year={2018},
	pages={521-526},
	note={cited By 8},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85050780669\&doi=10.23919\%2fMIKON.2018.8405275\&partnerID=40\&md5=ea42a9a4838c8a20e59c57296add85ea},
	abstract={The paper focuses on results of field trials for drone detection using CW (Continuous-Wave) radars operating in the C-band. The experiments have involved two different implementations of FMCW (Frequency-Modulated Continuous-Wave) radar and an implementation of CW noise radar. The theoretical comparison of the FMCW and noise radar, along with the description of their implementations is included. The obtained results are presented and discussed. For the conclusion, the limitations of each implementation are identified and recom-mendations for its usage in considered application are provided. © 2018 Warsaw University of Technology.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Zywek2018,
	author={Zywek, M. and Krawczyk, G. and Malanowski, M.},
	title={Experimental results of drone detection using noise radar},
	journal={Proceedings International Radar Symposium},
	year={2018},
	volume={2018-June},
	art_number={8447988},
	note={cited By 2},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85053631756\&doi=10.23919\%2fIRS.2018.8447988\&partnerID=40\&md5=3306d3be6891aba9322d9b08eff9a6fc},
	abstract={The paper deals with detection of drones using noise radar. The radar under consideration is a low-power, continuous-wave narrow-band noise radar. First, thethe-oretical analysis concerning power budget and velocity resolution is carried out. Next, the experimental setup is described. The results of a small drone detection are presented. It is demonstrated that in the experiment, the drone detection range was in the order of 300 m. © 2018 German Institute of Navigation - DGON.},
	publisher={IEEE Computer Society},
}

@CONFERENCE{Jarabo-Amores2018313,
	author={Jarabo-Amores, M.P. and Mata-Moya, D. and Gomez-Del-Hoyo, P.J. and Barcena-Humanes, J.L. and Rosado-Sanz, J. and Rey-Maestre, N. and Rosa-Zurera, M.},
	title={Drone detection feasibility with passive radars},
	journal={2018 15th European Radar Conference, EuRAD 2018},
	year={2018},
	pages={313-316},
	art_number={8546549},
	note={cited By 12},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85060376387\&doi=10.23919\%2fEuRAD.2018.8546549\&partnerID=40\&md5=597aed919e050c4862601668a6afe838},
	abstract={Drones are considered an important threat for critical infrastructures, and for people in crowded environments, because they can carry explosives, chemicals, or biological agents, cameras, etc. Passive radars are emerging sensor technologies that use non-cooperative illuminators instead of a dedicated transmitter. This feature makes them attractive candidates due to the absence of transmitted power. In this work, the viability of passive radars for detecting drone-like targets has been studied. Theoretical coverage studies based on bistatic radar cross section simulations and complex propagation models predict the possibility of drone detection with passive radars. Theoretical results have been validated with real experiments using the IDEPAR demonstrator, developed at the University of Alcalá. © 2018 European Microwave Association.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Choi2018,
	author={Choi, B. and Oh, D. and Kim, S. and Chong, J.-W. and Li, Y.-C.},
	title={Long-range drone detection of 24 G FMCW radar with E-plane sectoral horn array},
	journal={Sensors (Switzerland)},
	year={2018},
	volume={18},
	number={12},
	art_number={4171},
	note={cited By 5},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85057545444\&doi=10.3390\%2fs18124171\&partnerID=40\&md5=b83bad140d325edcad0be4170e537507},
	abstract={In this work, a 24-GHz frequency-modulated continuous-wave (FMCW) radar system with two sectoral horn antennas and one transmitting lens antenna for long-range drone detection is presented. The present work demonstrates the detection of a quadcopter-type drone using the implemented radar system up to a distance of 1 km. Moreover, a 3D subspace-based algorithm is proposed for the joint range-azimuth-Doppler estimation of long-range drone detection. The effectiveness of the long-range drone detection is verified with the implemented radar system through a variety of experiments in outdoor environments. This is the first such demonstration for long-range drone detection with a 24-GHz FMCW radar. © 2018 by the authors. Licensee MDPI, Basel, Switzerland.},
	publisher={MDPI AG},
}

@CONFERENCE{DeQuevedo2018,
	author={De Quevedo, A.D. and Urzaiz, F.I. and Menoyo, J.G. and López, A.A.},
	title={Drone Detection and RCS Measurements with Ubiquitous Radar},
	journal={2018 International Conference on Radar, RADAR 2018},
	year={2018},
	art_number={8557320},
	note={cited By 17},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85060138187\&doi=10.1109\%2fRADAR.2018.8557320\&partnerID=40\&md5=0d02a7bdc95b917c35b8ed5891af72cf},
	abstract={This paper presents experimental results on commercial-drone detection with a ubiquitous frequency modulated continuous wave (FMCW) radar system, working at 8.75 GHz (X-band). The system and its main blocks are briefly introduced. Subsequently, the document presents the chosen scenario for the tests, and shows the results of the offline signal processing, achieving a DJI-Phantom-4 detection at a range up to 2 km. The results are illustrated with range-Doppler matrices and detection figures. Range, speed and azimuth accuracies are discussed, considering the drone GPS data. Finally, the paper introduces a statistical radar-cross-section (RCS) study based on the processed data, in order to classify the drone as a Swerling target, and discusses the drone average RCS. © 2018 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Musa201916,
	author={Musa, S.A. and Abdullah, R.S.A.R. and Sali, A. and Ismail, A. and Rashid, N.E.A. and Ibrahim, I.P. and Salah, A.A.},
	title={A review of copter drone detection using radar systems},
	journal={Defence S and T Technical Bulletin},
	year={2019},
	volume={12},
	number={1},
	pages={16-38},
	note={cited By 3},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85072774419\&partnerID=40\&md5=021fb3184bb9977290054a6df9ec5007},
	abstract={The exponential growth of copter drone usage and the threats posed by drone users, such as unauthorised imaging and filming in restricted areas, illegal surveillance, air collisions, drug smuggling, terrorist attacks, and radio frequency (RF) jamming, have led to many efforts and research projects aimed at drone detection. The attempted methodologies include using acoustics, cameras, cascades (audio-visual) and radio frequency. In addition, there are the nontechnical methods such as shooting and netting. This paper presents radar systems as a method for copter drone detection. It presents the state of the art review of the efforts so far made towards detecting drones given preference to radar systems for micro-Doppler-based analysis. It also introduces passive forward scatter radar (PFSR) as an emerging methodology, presenting its reported achievements for both ground and airborne target detection. In an attempt to improve the detection of low-profile targets, this paper discusses the basic parameters aiding Doppler and micro-Doppler analysis of a copter drone. The paper concludes by proposing digital video broadcasting satellite (DVBS) based PFSR for drone detection due to its improved capabilities, thereby making micro- Doppler analysis for a low-profile target, a feasible endeavour. © 2019, Science and Technology Research Institute for Defence.},
	publisher={Science and Technology Research Institute for Defence},
}

@ARTICLE{Li2019101527,
	author={Li, T. and Wen, B. and Tian, Y. and Wang, S. and Yin, Y.},
	title={Optimized Radar Waveform Parameter Design for Small Drone Detection Based on Echo Modeling and Experimental Analysis},
	journal={IEEE Access},
	year={2019},
	volume={7},
	pages={101527-101538},
	art_number={8772049},
	note={cited By 2},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85079762663\&doi=10.1109\%2fACCESS.2019.2931087\&partnerID=40\&md5=06d156b608f328bf5837183b6ce8976a},
	abstract={Monitoring small drones is significant for security requirements, but it is challenging because of small drones' low radar cross section (RCS) and hovering ability. In order to analyze the effect of radar waveform on the echo spectra and optimize the waveform design, an analytical expression of the rotor's temporal RCS is desired. Integral model, a widely used radar echo model of the rotor's temporal RCS, does not involve the electromagnetic scattering, thus it cannot be applied to all frequency bands. The method of moments (MoM) is a strictly numerical method based on the Maxwell's equations, but cannot obtain the analytical expression. Hence, this paper proposes a new method combing the integral model and MoM to model the rotor's temporal RCS in very high frequency (VHF) band. The linear frequency modulation (LFM) signal which has a high Doppler tolerance and a large gain bandwidth product is adopted in optimizing waveform parameters design. Based on the new method, the analytical expression of LFM echo is also derived. Moreover, the spectral spread over range and Doppler dimension caused by the rotating rotors is analyzed in detail. A criterion for optimizing the LFM waveform parameters for small drone detection is presented. Field experiments confirm the validity of the echo model and waveform parameters optimization criterion, and the full Acrylonitrile Butadiene Styrene small drone is successfully detected in VHF band. In addition, experiments are implemented to verify the applicability of the echo model and waveform parameters optimization method to other drones with different size. © 2013 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Park20191221,
	author={Park, J. and Park, S. and Kim, D.-H. and Park, S.-O.},
	title={Leakage mitigation in heterodyne FMCW radar for small drone detection with stationary point concentration technique},
	journal={IEEE Transactions on Microwave Theory and Techniques},
	year={2019},
	volume={67},
	number={3},
	pages={1221-1232},
	art_number={8605523},
	note={cited By 27},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85062601083\&doi=10.1109\%2fTMTT.2018.2889045\&partnerID=40\&md5=11296dcb9780c8004494799ee34659a6},
	abstract={To prevent potential hazards posed by fast-evolving drones, it is of importance to develop a radar system for drone detection. Frequency modulated continuous wave (FMCW) radars are widely used for that purpose. Heterodyne architectures are preferred for them to mitigate dc offset errors. Having said that, FMCW radars suffer from permanent leakage from the transmitter into the receiver. The leakage phase noise raises the total noise floor and limits the radar sensitivity. Here, we propose a stationary point concentration (SPC) technique in order to overcome the challenges. The SPC technique concentrates the leakage phase noise on a stationary point to alleviate the impact of the noise. The technique can be realized using digital signal processing without additional hardware. The results show that the proposed technique significantly lowers the noise floor. © 2018 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Fang2019,
	author={Fang, X. and Min, R. and Cao, Z. and Pi, Y.},
	title={A coherent integration method for drone detection via PSIAF-KT-SFT},
	journal={2019 IEEE Radar Conference, RadarConf 2019},
	year={2019},
	art_number={8835565},
	note={cited By 3},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85073102081\&doi=10.1109\%2fRADAR.2019.8835565\&partnerID=40\&md5=dbc7025857149eb583e13241948da8ff},
	abstract={In this paper, the coherent integration for drone detection is considered and a method based on parametric symmetric instantaneous autocorrelation function (PSIAF), keystone transform (KT) and scaled Fourier transform (SFT), i.e., PSIAF-KT-SFT, is presented. To be specific, the PSIAF is first applied to eliminate the quadratic range migration (RM) and Doppler frequency migration (DFM) induced by the acceleration. Then, the residual linear RM can be removed by KT and SFT. After that, the motion parameters of drone can be estimated via the Fourier transform (FT) with respect to the lag time. Based on the estimated motion parameters, the coherent integration can be achieved and the target energy can be accumulated at one point, which can be used for drone detection. Finally, the simulations and real experiment are performed to demonstrate the effectiveness. © 2019 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Musa2019,
	author={Musa, S.A. and Rsa, R.A. and Sali, A. and Isma'Il, A. and Rashid, N.E.A.},
	title={DVBS based forward scattering radar for drone detection},
	journal={Proceedings International Radar Symposium},
	year={2019},
	volume={2019-June},
	art_number={8767456},
	note={cited By 3},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85069924832\&doi=10.23919\%2fIRS.2019.8767456\&partnerID=40\&md5=4cdd64c869693f2cb9e698d1e08baade},
	abstract={The drone detection challenge of implementing satellite base passive radar for air surveillance among others were low received power, short integration time, target receiver ranges etc. Following some identified benefits of forward scattering radar (FSR) geometry over conventional radars such as improved radar cross section RCS value irrespective of radar absorbing material (RAM), direct signal perturbation and high resolutions, this paper aimed at a feasibility study of implementing passive FSR by using Measat3a/3/3b Malaysian Satellite for a drone detection. This was achieved by analyzing the signal properties such as ambiguity function, power budget, target-to-receiver range profile. The paper further validated the claim with an actual signal from the Measat3 satellite. The resulted analysis of the signal ambiguity, minimum acceptable signal-to-Noise ratio (SNR) and the range profile was encouraging hence, manifesting the possibility of implementing this satellite for drone detection in FSR geometry. © 2019 German Institute of Navigation (DGON).},
	publisher={IEEE Computer Society},
}

@ARTICLE{DeQuevedo20191437,
	author={De Quevedo, A.D. and Urzaiz, F.I. and Menoyo, J.G. and López, A.A.},
	title={Drone detection and radar-cross-section measurements by RAD-DAR},
	journal={IET Radar, Sonar and Navigation},
	year={2019},
	volume={13},
	number={9},
	pages={1437-1447},
	note={cited By 10},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85071233759\&doi=10.1049\%2fiet-rsn.2018.5646\&partnerID=40\&md5=6058161749424ac745115cdb196d65fd},
	abstract={RAD-DAR is a frequency-modulated-continuous-wave radar demonstrator, working at X-band, completely designed and constructed by the authors' research group following the ubiquitous-radar concept. After introducing its main hardware and software blocks, with special emphasis to its off-line signal processing and data processing, this study presents the results of a drone detection test, where RAD-DAR achieved a DJI-Phantom 4 detection and tracking at a range up to 3 km. The system performance is discussed with different flights including an attack manoeuvre, and a free flight, which helps to highlight their advantages in surveillance tasks due to the RAD-DAR staring nature. Furthermore, range, speed and azimuth accuracies are discussed, considering the drone global positioning system data. Finally, this study shows a statistical radar cross-section study based on the processed data of the drone and attempts to classify this target by means of Swerling models. © The Institution of Engineering and Technology 2019.},
	publisher={Institution of Engineering and Technology},
}

@CONFERENCE{Aldowesh2019203,
	author={Aldowesh, A. and Binkhamis, T. and Alnuaim, T. and Alzogaiby, A.},
	title={Low Power Digital Array Radar for Drone Detection and Micro-Doppler Classification},
	journal={2019 Signal Processing Symposium, SPSympo 2019},
	year={2019},
	pages={203-206},
	art_number={8882033},
	note={cited By 4},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85074939707\&doi=10.1109\%2fSPS.2019.8882033\&partnerID=40\&md5=910444761223c597ecb6be218d7673d6},
	abstract={Due to the ever-increasing threat of micro-Unmanned Aerial Vehicles (UAVs), a necessity arises for robust detection and classification methods. Generally, radar sensor face difficulties in discriminating micro-UAVs from flying birds, as they have comparable Radar Cross Section (RCS) and velocity profiles. Exploiting the uniqueness of their respective micro-Doppler signature could alleviate the issue. In this paper, an experimental investigation is conducted to analyze different micro-Doppler signatures for different consumer drones in different frequency bands, with the aim to clearly distinguish a drone from other flying targets with similar characteristics. © 2019 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Al-Nuaim2019183,
	author={Al-Nuaim, T. and Alam, M. and Aldowesh, A.},
	title={Low-cost implementation of a multiple-input multiple-output radar prototype for drone detection},
	journal={Proceedings Elmar - International Symposium Electronics in Marine},
	year={2019},
	volume={2019-September},
	pages={183-186},
	art_number={8918664},
	note={cited By 2},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85077554671\&doi=10.1109\%2fELMAR.2019.8918664\&partnerID=40\&md5=620f14e799c5f469f55e2eb0c7638222},
	abstract={The usage of micro-Unmanned Aerial Vehicles (UAVs) has witnessed an enormous increase recently. Detection of such drones became a necessity nowadays to prevent any harmful activities. Typically, such targets have low velocity and low Radar Cross Section (RCS), making them indistinguishable from clutter and phase noise. Multiple-Input Multiple-Output (MIMO) Radars have many potentials; they increase the degrees of freedom on both transmit and receive ends. Such architecture allows for flexibility in operation, through utilizing the direct access to every element in the transmit/ receive array. MIMO systems allow for several array processing techniques, permitting the system to stare at targets for longer times, which improves the Doppler resolution. In this paper, a 2 × 2 low-cost MIMO radar prototype is developed using Software Defined Radio (SDR) technology, and its performance is evaluated against a slow-moving low radar cross section micro-UAV used by hobbyists. © 2019 IEEE.},
	publisher={Croatian Society Electronics in Marine - ELMAR},
}

@CONFERENCE{Yang2019,
	author={Yang, F. and Qu, K. and Hao, M. and Liu, Q. and Chen, X. and Xu, F.},
	title={Practical Investigation of a MIMO Radar System for Small Drones Detection},
	journal={2019 International Radar Conference, RADAR 2019},
	year={2019},
	art_number={9078960},
	note={cited By 1},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85084956125\&doi=10.1109\%2fRADAR41533.2019.171348\&partnerID=40\&md5=f60fd2cbdccc377001e787c18de7f62f},
	abstract={This study presents the latest progress of the MIMO radar system developed for small drones detection. The sparse array optimization method in practical situation is proposed and a target-based MIMO radar array calibration method is presented to improve the signal-to-noise ratio of the target. Experiment in the microwave chamber is conducted to verify the designed sparse array beam pattern and measurement campaigns for small drones are performed to test the system performance. Experimental results and analysis show that the system has good capability in small drones detection and tracking. © 2019 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Park2019,
	author={Park, J. and Bae, K.-B. and Jung, D.-H. and Park, S.-O.},
	title={Micro-Drone Detection with FMCW Radar Based on Stationary Point Concentration Technique},
	journal={2019 International Symposium on Antennas and Propagation, ISAP 2019 - Proceedings},
	year={2019},
	art_number={8963107},
	note={cited By 4},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85078965527\&partnerID=40\&md5=2267df120fbea87df0c74eae84895ed6},
	abstract={This paper shows an interesting detection performance of frequency modulated continuous wave (FMCW) radar. We challenge to detect a micro-drone whose size is about a little finger. Applying the stationary point concentration (SPC) technique, we overcome the inherent problem of leakage in the FMCW radar and set a new record for ultra-small drone detection. The SPC technique attenuates the phase noise of the leakage, and this leads to the reduction of the noise floor in the power spectrum. Therefore, we can expect to detect the beat signal of the micro-drone buried in the noise floor due to its extremely small radar cross section. Experimental results demonstrate that the noise floor is significantly reduced, and the micro-drone buried in the noise floor is detected well. © 2019 Antenna Branch of Chinese Institute of Electronics.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Bae2019,
	author={Bae, K.-B. and Park, J. and Kim, D.-H. and Park, S.-O.},
	title={Drone Detection with Linear Chirp Pulse Radar using Coherent Pulse Integration},
	journal={2019 International Symposium on Antennas and Propagation, ISAP 2019 - Proceedings},
	year={2019},
	art_number={8963414},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85079011039\&partnerID=40\&md5=749e7f61922e57c7d2824c479f10371d},
	abstract={This paper discusses the detection of small drone with linear chirp pulse radar system. The system employs 14.1GHz as RF center frequency with bandwidth 200MHz to cover Linear Chirp Pulse (LCP) whose chirp rate is 80MHz. The LCP is radiated and received through quasi-monostatic antennas with the gain of 16dBi. The system also includes digital down converter to obtain IQ signal from LCP received at RX antenna. Finally, Matched filtering of the LCP is performed to maximize the SNR of the signal reflected from the drone. In the actual performance measurement, the drone signal was detected up to 400m distance in real-time using Coherent Pulse Integration (CPI). The raw data is obtained as csv file and then later processed with MATLAB. © 2019 Antenna Branch of Chinese Institute of Electronics.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}


@CONFERENCE{Huang201913,
	author={Huang, R. and Du, X.-Y. and Hu, W.-D.},
	title={Phase Compensation Based Multi-frame Coherent Integration for Drone Detection with Radar},
	journal={Proceedings of the 2019 IEEE International Conference on Unmanned Systems, ICUS 2019},
	year={2019},
	pages={13-18},
	art_number={8995972},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85080880270\&doi=10.1109\%2fICUS48101.2019.8995972\&partnerID=40\&md5=3dfcd51cbfb0c4d235011a4a3da3839c},
	abstract={In order to improve the detection ability of small and weak targets such as drones, a multi-frame coherent integration(MFCI) method based on phase compensation is proposed. The phase information of the multi-frame radar echoes is first analyzed and the maximum likelihood estimation(MLE) model of the motion parameters is established. Due to the target motion, the phenomena of migration through range and Doppler cells will occur in the successive frames of target echoes. In order to achieve coherent integration in multiple frames, all the orientations of the multi-frame signal are searched within a certain initial radial velocity and radial acceleration range. The trajectory of each moving target and the corresponding motion parameter values are then obtained, while the phase of the multi-frame signal is located in the same range and the Doppler cell corresponding to a target, thereby improving the detection performance of the weak targets. To further reduce the amount of computation, the influence of radial acceleration on the detection performance of weak targets is studied. Simulation and measured data experiments show that the proposed algorithm can accurately detect drones with less computational complexity. © 2019 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Bouzayene2019,
	author={Bouzayene, I. and Mabrouk, K. and Gharsallah, A. and Kholodnyak, D.},
	title={Scan Radar Using an Uniform Rectangular Array for Drone Detection with Low RCS},
	journal={Mediterranean Microwave Symposium},
	year={2019},
	volume={2019-October},
	art_number={9157299},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85090321961\&doi=10.1109\%2fMMS48040.2019.9157299\&partnerID=40\&md5=ce478e30d20adf5a8011caa7059700fd},
	abstract={Drones are becoming more and more available to the general public for leisure activities and exploited in commercial applications, this boom in drone use has contributed to the emergence of new threats in security applications. Because of their great agility and small size, UAV can be used for numerous missions and are very challenging to detect. Radar technology with its all-weather capability can play an important role in detecting UAV-based threats and in protecting critical assets, but standard radar is ill-prepared for UAV detection: UAVs are low-velocity aircraft with a very weak radar. A radar simulation is discussed and preliminary results are presented. In general, an X-band radar with electronic scanning capability can contribute to a reliable and affordable solution for detecting UAV threats. Radar could be the technology of choice for detecting the drone, signature. © 2019 IEEE.},
	publisher={IEEE Computer Society},
}

@ARTICLE{Sun20193667,
	author={Sun, H. and Oh, B.-S. and Guo, X. and Lin, Z.},
	title={Improving the Doppler Resolution of Ground-Based Surveillance Radar for Drone Detection},
	journal={IEEE Transactions on Aerospace and Electronic Systems},
	year={2019},
	volume={55},
	number={6},
	pages={3667-3673},
	art_number={8631137},
	note={cited By 8},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85065534249\&doi=10.1109\%2fTAES.2019.2895585\&partnerID=40\&md5=9bdbf9b282ab8f3751282c160eaec9c2},
	abstract={In this paper, we propose to use an iterative adaptive approach to perform the Doppler processing in ground-based surveillance radar for drone detection. It overcomes the limited dwell time and improves the Doppler resolution, and therefore significantly enhances the discrimination of micro-Doppler signature and the correct classification of drones. In addition, the target detectability is also improved. This approach is validated in the field experiments conducted with a commercial portable ground-based surveillance radar. © 1965-2011 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Lee2020213,
	author={Lee, S.J. and Jung, J.H. and Yu, J.-W.},
	title={TX Leakage Canceller for Small Drone Detection Radar in 2-GHz Band},
	journal={IEEE Microwave and Wireless Components Letters},
	year={2020},
	volume={30},
	number={2},
	pages={213-215},
	art_number={8998608},
	note={cited By 1},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85079742921\&doi=10.1109\%2fLMWC.2019.2959441\&partnerID=40\&md5=9ef0b3ab2b584d31a88d0dca043140f6},
	abstract={A transmitter leakage canceller (TLC) having high isolation from a transmitter (TX) to a receiver (RX) is proposed, which is for a single antenna continuous-wave (CW) radar in the 2-GHz band. The proposed TLC is based on three points to obtain sufficient TX-to-RX isolation in a bandwidth of tens of MHz. The first is the use of a quasi-balanced structure in a leakage path and an antileakage path, which makes both signals in the two paths similar in a wide bandwidth. The second point is the adoption of active circuits in the antileakage path, which provides sufficient cancellation between the two signals. However, this adoption makes both signals in two paths with different phase slopes versus frequency; therefore, the sufficient cancellation is confined to a narrow bandwidth. The last is the application of a delay line in the leakage path, which compensates the different phase slopes. Thus, a bandwidth feature of tens of MHz is obtained. Laboratory measurements show more than 60 dB TX-to-RX isolation for an arbitrary targeted 20-MHz bandwidth from 2.3 to 2.7 GHz. © 2001-2012 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Park20201858,
	author={Park, J. and Jung, D.-H. and Bae, K.-B. and Park, S.-O.},
	title={Range-Doppler Map Improvement in FMCW Radar for Small Moving Drone Detection Using the Stationary Point Concentration Technique},
	journal={IEEE Transactions on Microwave Theory and Techniques},
	year={2020},
	volume={68},
	number={5},
	pages={1858-1871},
	art_number={8957391},
	note={cited By 6},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85084850484\&doi=10.1109\%2fTMTT.2019.2961911\&partnerID=40\&md5=bb279d0b2889e9e317e3b3ac3feb927b},
	abstract={Given the rapidly growing drone market, the development of drone detection radars has become highly important to prevent drones from damaging lives and property. Frequency-modulated continuous-wave (FMCW) radars have been frequently used for drone detection. Among the architectures of FMCW radar, a heterodyne architecture that involves different local oscillators and produces beat signals at the IF stage has often been chosen. The FMCW radar, however, has a chronic problem called leakage. In an earlier study, we proposed the stationary point concentration (SPC) technique to improve the signal-to-noise ratio (SNR) of small drones by reducing the increase in noise floor caused by leakage. We demonstrated that the proposed technique increases the SNR of small hovering drones in the 1-D power spectrum. In this article, we newly analyze the practical problems in the heterodyne FMCW radar system. One is the 2-D noise floor increase in the range-Doppler (r-D) map due to the leakage, and the other is unwanted Doppler shifts. Then, we propose an upgraded theory and realization method of the SPC technique for the detection of the small moving drone by improving the r-D map. We prove that the proposed method not only reduces the 2-D noise floor by mitigating the leakage but also removes the unwanted Doppler shifts by the phase calibration. Consequently, we show that the proposed method increases the SNR of the small moving drone and corrects its velocity information at the same time in the r-D map. © 1963-2012 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Abdullah2020,
	author={Abdullah, R.S.A.R. and Musa, S.A. and Rashid, N.E.A. and Sali, A. and Salah, A.A. and Ismail, A.},
	title={Passive forward-scattering radar using digital video broadcasting satellite signal for drone detection},
	journal={Remote Sensing},
	year={2020},
	volume={12},
	number={18},
	art_number={3075},
	note={cited By 4},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85092268648\&doi=10.3390\%2fRS12183075\&partnerID=40\&md5=cc4b708be21a21a6e3555b65a0907b31},
	abstract={This paper presents a passive radar system using a signal of opportunity from Digital Video Broadcasting Satellite (DVB-S). The ultimate purpose of the system is to be used as an air traffic monitoring and surveillance system. However, the work focuses on drone detection as a proof of the concept. Detecting a drone by using satellite-based passive radar possess inherent challenges, such as the small radar cross section and low speed. Therefore, this paper proposes a unique method by leveraging the advantage of forward-scattering radar (FSR) topology and characteristics to detect a drone, in other words, the system is known as a passive FSR (p-FSR) system. In the signal-processing algorithm, the empirical mode decomposition (EMD) is applied to the received signal to extract the unique feature vector of the micro-Doppler frequency from the drone's rotating blades. The paper highlights the p-FSR experimental setup and experiment campaign to detect drones. The experimental results show the feasibility of the p-FSR using a signal transmitted from a satellite to detect flying drone crossing the forward-scatter baseline between the satellite and ground station. © 2020 by the authors.},
	publisher={MDPI AG},
}

@CONFERENCE{Zulkifli2020,
	author={Zulkifli, S. and Balleri, A.},
	title={Design and Development of K-Band FMCW Radar for Nano-Drone Detection},
	journal={IEEE National Radar Conference - Proceedings},
	year={2020},
	volume={2020-September},
	art_number={9266538},
	note={cited By 3},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85098536006\&doi=10.1109\%2fRadarConf2043947.2020.9266538\&partnerID=40\&md5=e432c2d5a152ce0dee62c68b0b96214a},
	abstract={Nano-drones, are insect-like size drones with a capability of intrusion to provide intelligence and potentially violate secure establishments and public privacy rights. Nano-drones are already an existing technology which is becoming more and more available, portable, affordable and easily operated. As such, they may soon become a plausible defence and security threat. This paper presents the design and development of a K-Band FMCW radar prototype for nano-drone detection. The FMCW radar prototype consists of connectorised components operating at a carrier frequency of 24 GHz and offer high parameter selection flexibility. Experiments have been carried out in order to evaluate the system performance. Results show that a small Arcade PICO Drone Nano Quadcopter (smaller than 5 cm) could be detected, and that its micro-Doppler signature could be extracted from data. © 2020 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Martelli2020,
	author={Martelli, T. and Cabrera, O. and Colone, F. and Lombardo, P.},
	title={Exploitation of Long Coherent Integration Times to Improve Drone Detection in DVB-S based Passive Radar},
	journal={IEEE National Radar Conference - Proceedings},
	year={2020},
	volume={2020-September},
	art_number={9266624},
	note={cited By 5},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85098597794\&doi=10.1109\%2fRadarConf2043947.2020.9266624\&partnerID=40\&md5=c11d038bf2b948ba64ec556f60f31684},
	abstract={In this paper, we consider the exploitation of long coherent integration times for improving the detection of small drones in a DVB-S based Passive Radar (PR). In fact, since these low-flying objects are characterized by very small RCS values, their detection is challenging especially when using DVB-S signals as source of opportunity, typically received with low power levels. In this work, in order to benefit from the use of extended coherent integration times, the target range and Doppler migration effects have been properly compensated. Then, the effectiveness of the adopted detection scheme has been tested against real data collected by a multi-polarimetric DVB-S based PR receiver developed at Sapienza University of Rome. The reported results show that the coherent integration time can be increased up to a few seconds thus improving the drone detection capability of the considered system. © 2020 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Karpovich202077,
	author={Karpovich, P. and Kareneuski, S. and Zielinski, T.P.},
	title={Practical results of drone detection by passive coherent DVB-T2 radar},
	journal={Proceedings International Radar Symposium},
	year={2020},
	volume={2020-October},
	pages={77-81},
	art_number={9253800},
	note={cited By 1},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85097307558\&doi=10.23919\%2fIRS48640.2020.9253800\&partnerID=40\&md5=64193c037b00b9c377a8b2d41a53535e},
	abstract={In this paper practical results of drone detection and tracking in a DVB-T2 passive radar system are presented. DVB-T2 signal from TV tower was used to detect and measure distance and velocity of a drone. To increase SNR, adaptive filtering and re-modulation of DVB-T2 signal were applied before the detection. Since integration time of the reflected signal is large, a non-trivial range-Doppler matrix calculation algorithm was used to reduce the computational expense. Detection was done by CFAR algorithm. Finally, it was shown that peaks from drone's propellers are visible in range-Doppler matrix what can be used for its type identification, and application of multiple TV-tower signals has been suggested. © 2020 Warsaw University of Technology.},
	publisher={IEEE Computer Society},
}

@CONFERENCE{Huang2020,
	author={Huang, A. and Sevigny, P. and Balaji, B. and Rajan, S.},
	title={Radar Micro-Doppler-based Rotary Drone Detection using Parametric Spectral Estimation Methods},
	journal={Proceedings of IEEE Sensors},
	year={2020},
	volume={2020-October},
	art_number={9278678},
	note={cited By 2},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85098689652\&doi=10.1109\%2fSENSORS47125.2020.9278678\&partnerID=40\&md5=663950eb7d1ee398abbe458d850faff7},
	abstract={Micro-Doppler methods of detecting and classifying small UAVs are limited in range due to the weak radar returns from their plastic propellers. Smaller windows of data instead of longer windows are used for detection as stationarity assumptions often fail for longer windows. Traditional non-parametric methods may be inadequate as they have limited spectral resolution with smaller windows and may provide false detection when radar returns are weak. A rotary drone detector using the number of Helicopter Rotation Modulation (HERM) lines is considered in this paper. Two parametric methods for estimating the number of HERM lines, Minimum Description Length (MDL) and Akaike Information Criterion (AIC), are considered for detection purposes. Experiments using real data acquired using a micro-helicopter drone and a commercial ultra-wide band radar reveal that MDL performs significantly better than AIC and the traditional Fourier-based non-parametric estimation methods. © 2020 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Singh2021416,
	author={Singh, A.K. and Bae, K.-B. and Park, S.-O.},
	title={NLFM pulse radar for drone detection using predistortion technique},
	journal={Journal of Electromagnetic Waves and Applications},
	year={2021},
	volume={35},
	number={3},
	pages={416-429},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85096109532\&doi=10.1080\%2f09205071.2020.1844598\&partnerID=40\&md5=75ef32c6ddc72ff0aa4ab7e5f419e2be},
	abstract={The development of radar technology for the detection of small drones is getting attention of researchers. In this work, the detection of drones using Ku-band radar system has been discussed. We have utilized the advantage of nonlinear frequency modulation (NLFM) waveform for the suppression of range sidelobes. The performance and sensitivity of a radar system can be related with the linearity of system response. Here, we have made an effort to minimize non-linearity in the radar system response by using digital predistortion method. In this method, amplitude weighting coefficients have been calculated based on the received data. We have used FPGA-based transceiver for intermediate frequency (IF) signal generation and data acquisition, along with Ku-band up-down converters. The radar system was first calibrated for desired frequency band using amplitude predistortion method. In this article, experiment results for the detection of single drone and two drones using NLFM pulse signal are presented. © 2020 Informa UK Limited, trading as Taylor \& Francis Group.},
	publisher={Taylor and Francis Ltd.},
}

@ARTICLE{Chahrour2021123950,
	author={Chahrour, H. and Dansereau, R.M. and Rajan, S. and Balaji, B.},
	title={Target Detection through Riemannian Geometric Approach with Application to Drone Detection},
	journal={IEEE Access},
	year={2021},
	volume={9},
	pages={123950-123963},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85114740423\&doi=10.1109\%2fACCESS.2021.3105594\&partnerID=40\&md5=5f06f173522e8409142f0d36e032a9ed},
	abstract={Radar detection of small drones in presence of noise and clutter is considered from a differential geometry viewpoint. The drone detection problem is challenging due to low radar cross section (RCS) of drones, especially in cluttered environments and when drones fly low and slow in urban areas. This paper proposes two detection techniques, the Riemannian-Brauer matrix (RBM) and the angle-based hybrid-Brauer (ABHB), to improve the probability of drone detection under small sample size and low signal-to-clutter ratio (SCR). These techniques are based on the regularized Burg algorithm (RBA), the Brauer disc (BD) theorem, and the Riemannian mean and distance. Both techniques exploit the RBA to obtain a Toeplitz Hermitian positive definite (THPD) covariance matrix from each snapshot and apply the BD theorem to cluster the clutter-plus-noise THPD covariance matrices. The proposed Riemannian-Brauer matrix technique is based on the Riemannian distance between the Riemannian mean of clutter-plus-noise cluster and potential targets. The proposed angle-based hybrid-Brauer technique uses the Euclidean tangent space and the Riemannian geodesical distances between the Riemannian mean, the Riemannian median and the potential target point. The angle at the potential target on the manifold is computed using the law of cosines on the manifold. The proposed detection techniques show advantage over the fast Fourier transform, the Riemannian distance-based matrix and the Kullback-Leibler (KLB) divergence detectors. The validity of both proposed techniques are demonstrated with real data. © 2013 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Semkin2021223,
	author={Semkin, V. and Yin, M. and Hu, Y. and Mezzavilla, M. and Rangan, S.},
	title={Drone detection and classification based on radar cross section signatures},
	journal={2020 International Symposium on Antennas and Propagation, ISAP 2020},
	year={2021},
	pages={223-224},
	art_number={9391260},
	note={cited By 3},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85104496955\&doi=10.23919\%2fISAP47053.2021.9391260\&partnerID=40\&md5=13b4bfa36a5b409fa9fb27b354392e10},
	abstract={In this work, we show how drone detection and classification can be enabled by leveraging a database of radar cross section (RCS) signatures. First, we present a set of measurement results of the RCS of a carbon fiber drone model at 28 GHz. The measurements were performed in an anechoic chamber and provide essential information about the RCS signature of the specific drone. Then, we assess the RCS-based detection probability and the range error by running simulations in urban environments. The drones were positioned at different distances, from 30m to 90m, and the RCS signatures used for the detection and classification were obtained experimentally. © 2021 IEICE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Park2021737,
	author={Park, J. and Park, S.-O.},
	title={Improved drone detection in FMCW Radar using SPC Technique (invited talk)},
	journal={2020 International Symposium on Antennas and Propagation, ISAP 2020},
	year={2021},
	pages={737-738},
	art_number={9391464},
	note={cited By 1},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85104500313\&doi=10.23919\%2fISAP47053.2021.9391464\&partnerID=40\&md5=ad5f4c51ae22da60f40fcabd76a5111b},
	abstract={This paper introduces the stationary point concentration (SPC) technique, one of the state-of-the-art techniques for detecting small drones with frequency modulated continuous wave radars. A novel approach of the SPC technique is explained, and representative experimental results are shown. Finally, the promising potentials of the SPC technique are discussed. © 2021 IEICE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Park20211791,
	author={Park, J. and Park, J.-S. and Bae, K.-B. and Park, S.-O.},
	title={Advanced Stationary Point Concentration Technique for Leakage Mitigation and Small Drone Detection with FMCW Radar},
	journal={IEEE Transactions on Microwave Theory and Techniques},
	year={2021},
	volume={69},
	number={3},
	pages={1791-1804},
	art_number={9339993},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85100510402\&doi=10.1109\%2fTMTT.2021.3052190\&partnerID=40\&md5=8616002a9e13d4e1d87fc5836f8de3b0},
	abstract={With the increase in threats posed by small drones, the development of radars to detect such drones has become a key necessity. In earlier studies, we proposed the stationary point concentration (SPC) technique for small drone detection using frequency-modulated continuous-wave (FMCW) radar. The SPC technique is a novel approach for mitigating leakage, which is an inherent problem in FMCW radar. The SPC technique improves the signal-to-noise ratio of small drones by reducing the noise floor and provides accurate distance and velocity information of such drones. However, this technique has shortcomings in its realization. In this article, we present the drawbacks of this technique and propose an advanced SPC (A-SPC) technique. The proposed technique can overcome the drawbacks of the SPC technique while implementing the benefits of the SPC technique. The experimental results verify the proposed A-SPC technique and demonstrate its robustness and usefulness. © 1963-2012 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Geschke2021,
	author={Geschke, R.H. and Shoykhetbrod, A. and Brauns, R. and Schwabig, C. and Wickmann, S. and Leuchs, S. and Krebs, C. and Kuter, A. and Nussler, D.},
	title={Post-integration Antenna Characterisation for a V-band Drone-detection Radar},
	journal={15th European Conference on Antennas and Propagation, EuCAP 2021},
	year={2021},
	art_number={9411016},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85105435735\&doi=10.23919\%2fEuCAP51087.2021.9411016\&partnerID=40\&md5=2a66042adf9bf39ea6362b11b64d0a53},
	abstract={A drone detection FMCW radar operating from 57 to 64 GHz band has one transmit and two receiving fan-beam antennas. Due to the close integration of the system and enclosure, aspects related to board layout such as direct transmitter antenna to receiver antenna coupling and packaging effects reduce the antenna beamwidths and may reduce antenna efficiency. Post-integration diagnostic methods are presented to test the antenna system performance. The concept of a combined transmit-receive radiation pattern in combination with a large planar reflector is introduced and used to characterise radar fan-beam antenna patterns. The system is used as an uncalibrated network analyser to characterise the two fan-beam pairs with the influence of the packaging included. © 2021 EurAAP.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}
@CONFERENCE{Teo2021875,
	author={Teo, M.I. and Seow, C.K. and Wen, K.},
	title={5G Radar and Wi-Fi Based Machine Learning on Drone Detection and Localization},
	journal={2021 IEEE 6th International Conference on Computer and Communication Systems, ICCCS 2021},
	year={2021},
	pages={875-880},
	art_number={9449224},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113335396\&doi=10.1109\%2fICCCS52626.2021.9449224\&partnerID=40\&md5=290e39f9f3d074ead5638d921ba479d4},
	abstract={Drone usages have been proliferating for various government initiatives, commercial benefits and civilian leisure purposes. Drone mismanagement especially civilian usage drones can easily expose threat and vulnerability of the Government Public Key Infrastructures (PKI) that hold crucial operations, affecting the survival and economic of the country. As such, detection and location identification of these drones are crucial immediately prior to their payload action. Existing drone detection solutions are bulky, expensive and hard to setup in real time. With the advent of 5G and Internet of Things (IoT), this paper proposes a cost effective bistatic radar solution that leverages on 5G cellular spectrum to detect the presence and localize the drone. Coupled with K-Nearest Neighbours (KNN) Machine Learning (ML) algorithm, the features of Non- Line of Sight (NLOS) transmissions by 5G radar and Received Signal Strength Indicator (RSSI) emitted by drone are used to predict the location of the drone. The proposed 5G radar solution can detect the presence of a drone in both outdoor and indoor environment with accuracy of 100\%. Furthermore, it can localize the drone with an accuracy of up to 75\%. These results have shown that a cost effective radar machine learning system, operating on the 5G cellular network spectrum can be developed to successfully identify and locate a drone in real-time. © 2021 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Zhang2021,
	author={Zhang, Y.D. and Xiang, X. and Li, Y. and Chen, G.},
	title={Enhanced Micro-Doppler Feature Analysis for Drone Detection},
	journal={IEEE National Radar Conference - Proceedings},
	year={2021},
	volume={2021-May},
	art_number={9455228},
	note={cited By 2},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85112467486\&doi=10.1109\%2fRadarConf2147009.2021.9455228\&partnerID=40\&md5=eb65a4bbd8504c310b70b9a6083bc6c4},
	abstract={As low-cost drones become more accessible, they pose various safety, security, and privacy threats. As such, it becomes increasingly important to detect their presence, locate and track their positions, and classify their types in real time. In this paper, we perform time-frequency analyses of drone Doppler and micro-Doppler signatures to provide enhanced drone detection and feature extraction capabilities. The analyses are based on the combined use of spectrogram and inverse Radon transform (IRT). The paired property of propeller blades associated with a rotor is further utilized to compute the IRT product for enhanced performance. It is demonstrated that the IRT and IRT product images, when expressed in terms of the rotation frequency and blade position phase, provide flexibility and effectiveness for the presentation and estimation of these parameters. © 2021 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Blake2021,
	author={Blake, W. and Burger, I.},
	title={Small Drone Detection Using Airborne Weather Radar},
	journal={IEEE National Radar Conference - Proceedings},
	year={2021},
	volume={2021-May},
	art_number={9455224},
	note={cited By 1},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85112409525\&doi=10.1109\%2fRadarConf2147009.2021.9455224\&partnerID=40\&md5=6c477d1199d71ab2451eb461315f8b23},
	abstract={As small commercial and hobby drones increase in popularity, there is a desire to monitor and avoid these drones. This paper focuses on how small drones such as the DJI Phantom 3 and DJI Inspire could be detected using existing weather radar hardware already installed in many airplanes. Garmin's GWX 80 airborne weather radar was used to demonstrate this potential. Only software modifications were made to the aviation certified hardware for the feasibility of this approach. © 2021 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Ciesielski2021,
	author={Ciesielski, M. and Stasiak, K. and Khyzhniak, M. and Jedrzejewski, K. and Zywek, M. and Brawata, S.},
	title={Simultaneous Signal Processing with Multiple Coherent Processing Intervals in FMCW Radar for Drone Detection},
	journal={Proceedings International Radar Symposium},
	year={2021},
	volume={2021-June},
	art_number={9466232},
	note={cited By 1},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113850556\&doi=10.23919\%2fIRS51887.2021.9466232\&partnerID=40\&md5=9e780ebf8e7082c052f4df32d2a82fba},
	abstract={The paper presents research on using multiple signal processors operating simultaneously with different coherent processing intervals. The papers focuses on considerations related to drone detection. Theoretical analysis of the problems arising in FMCW radars is provided and a solution utilizing multiple signal processors is proposed. Results of field trials are also presented. © 2021 German Institute of Navigation (DGON).},
	publisher={IEEE Computer Society},
}

@CONFERENCE{Rahman2021,
	author={Rahman, S. and Robertson, D.A.},
	title={FAROS-E: A compact and low-cost millimeter wave surveillance radar for real time drone detection and classification},
	journal={Proceedings International Radar Symposium},
	year={2021},
	volume={2021-June},
	art_number={9466175},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113891659\&doi=10.23919\%2fIRS51887.2021.9466175\&partnerID=40\&md5=d58bd0d201b911b6e01cdeaa5effa6a8},
	abstract={This paper describes the system architecture and performance of the FAROS-E 77 GHz radar designed and built at the University of St Andrews for real time drone detection and classification (drone vs non-drone). The motivation behind the system is to demonstrate a highly reliable drone classification sensor for security surveillance in a compact, low-cost and potentially portable form factor. The low phase noise, coherent architecture exploits the high Doppler sensitivity available at millimeter wave frequencies, to enable robust micro-Doppler signature analysis and classification. Outdoor trials of FAROS-E have yielded high fidelity data and shown very promising results as a short-range system capable of detecting a DJI Phantom Standard 3 up to 300 m and classifying it up to 150m. The classification algorithm is capable of classifying the presence of a drone even when it is hovering stationary. © 2021 German Institute of Navigation (DGON).},
	publisher={IEEE Computer Society},
}

@CONFERENCE{Schneebeli2021,
	author={Schneebeli, M. and Leuenberger, A. and Wabeke, L. and Kloke, K. and Kitching, C. and Siegenthaler, U. and Wellig, P.},
	title={Drone detection with a multistatic C-band radar},
	journal={Proceedings International Radar Symposium},
	year={2021},
	volume={2021-June},
	art_number={9466200},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113895167\&doi=10.23919\%2fIRS51887.2021.9466200\&partnerID=40\&md5=e6cc8deb5e496d99af09971908d475bd},
	abstract={The multistatic active surveillance radar system SAMURAI (Swiss African MUltistatic RAdar Initiative) was tested on its drone detection capabilities during two field campaigns in Switzerland. The C-band system, consisting of one transmit and two receive nodes, was geometrically and radiometrically calibrated with a specific multistatic target simulator. GPS trajectories of a DJI Phantom 4 drone were compared to the radar detections. It was found that the radar system's inherent pointing angle and range biases can be corrected in a straightforward manner by using the virtually generated radar targets as a reference. After the corrections were applied to the radar data, deviations between the drone's GPS position and the radar detections on the order of 5 m were found. © 2021 German Institute of Navigation (DGON).},
	publisher={IEEE Computer Society},
}

@CONFERENCE{Mata-Moya2021,
	author={Mata-Moya, D. and Rey-Maestre, N. and Gomez-Del-Hoyo, P.-J. and Rosado-Sanz, J. and Jarabo-Amores, M.-P.},
	title={4D Passive Radar for Drone Detection and Tracking},
	journal={Proceedings International Radar Symposium},
	year={2021},
	volume={2021-June},
	art_number={9466190},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113909664\&doi=10.23919\%2fIRS51887.2021.9466190\&partnerID=40\&md5=e67a24dcd11615c34f7328241811abcc},
	abstract={An upgraded version of IDEPAR demonstrator capable of detecting and extracting parameters from targets in a 4D measurements space(range, Doppler, azimuth and elevation) is presented to allow the localization of small aerial drones in the Cartesian space (x,y,z). A two-stage spatial filtering processing scheme based on a 2D reception antenna system provides target's directions of arrival (azimuth, elevation) for targets' localization in the Cartesian space. The PR system was validated in measurement campaigns using small drones confirming the location capabilities of the proposed approach. © 2021 German Institute of Navigation (DGON).},
	publisher={IEEE Computer Society},
}

@ARTICLE{Yang2021760,
	author={Yang, F. and Xu, F. and Fioranelli, F. and Le Kernec, J. and Chang, S. and Long, T.},
	title={Practical Investigation of a MIMO radar system capabilities for small drones detection},
	journal={IET Radar, Sonar and Navigation},
	year={2021},
	volume={15},
	number={7},
	pages={760-774},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85104836532\&doi=10.1049\%2frsn2.12082\&partnerID=40\&md5=9059635bb87c5a1b766d7277672794a1},
	abstract={The latest progress of the multiple-input multiple-output (MIMO) radar system developed for small drones detection at Beijing Institute of Technology is presented herein. A low-cost S-band MIMO scanning radar system is designed for the detection of small drones. A practical design optimisation and implementation of a sparse array covering the whole airspace, and a target-based MIMO radar array calibration method to improve the signal-to-noise ratio of the target are proposed. An experiment in the microwave chamber was conducted to verify the designed sparse-array beam-pattern, and measurement campaigns for small drones were performed to test the system performance where the radar achieved detection and tracking of a small DJI-Phantom 4 drone at a range of up to 5 km. Target features, including micro-Doppler and radar cross-section signatures were extracted to assist target classification. The experimental results indicate that the system has promising capability in small drones detection and tracking, despite the challenges of low dwell time on targets due to the scanning nature of the system. © 2021 The Authors. IET Radar, Sonar \& Navigation published by John Wiley \& Sons Ltd on behalf of The Institution of Engineering and Technology.},
	publisher={John Wiley and Sons Inc},
}

@ARTICLE{Sazdić-Jotić2022,
	author={Sazdić-Jotić, B. and Pokrajac, I. and Bajčetić, J. and Bondžulić, B. and Obradović, D.},
	title={Single and multiple drones detection and identification using RF based deep learning algorithm},
	journal={Expert Systems with Applications},
	year={2022},
	volume={187},
	art_number={115928},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85115947866\&doi=10.1016\%2fj.eswa.2021.115928\&partnerID=40\&md5=c95b79c41e2dfce066bb0fc3ff0ae60b},
	abstract={Unmanned aerial systems, especially drones have gone through remarkable improvement and expansion in recent years. Drones have been widely utilized in many applications and scenarios, due to their low price and ease of use. However, in some applications drones can pose a malicious threat. To diminish risks to public security and personal privacy, it is necessary to deploy an effective and affordable anti-drone system in sensitive areas to detect, localize, identify, and defend against intruding malicious drones. This research article presents a new publicly available radio frequency drone dataset and investigates detection and identification methodologies to detect single or multiple drones and identify a single detected drone's type. Moreover, special attention in this paper has been underlined to examine the possibility of using deep learning algorithms, particularly fully connected deep neural networks as an anti-drone solution within two different radio frequency bands. We proposed a supervised deep learning algorithm with fully-connected deep neural network models that use raw drone signals rather than features. Regarding the research results, the proposed algorithm shows a lot of potentials. The probability of detecting a single drone is 99.8\%, and the probability of type identification is 96.1\%. Moreover, the results of multiple drones detection demonstrate an average accuracy of 97.3\%. There have not been such comprehensive publications, to this time, in the open literature that have presented and enlightened the problem of multiple drones detection in the radio frequency domain. © 2021 Elsevier Ltd},
	publisher={Elsevier Ltd},
}

@CONFERENCE{Jian20181146,
	author={Jian, M. and Lu, Z. and Chen, V.C.},
	title={Drone detection and tracking based on phase-interferometric Doppler radar},
	journal={2018 IEEE Radar Conference, RadarConf 2018},
	year={2018},
	pages={1146-1149},
	note={cited By 33},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85049928482\&doi=10.1109\%2fRADAR.2018.8378723\&partnerID=40\&md5=72e95fda4ec128ff0efa9abff67b10ea},
	abstract={In this paper, drone detection and tracking based on phase-interferometry are investigated. Data collected by a simple dual-channel Doppler radar is used for implementing the joint range-Doppler-azimuth processing. Experimental results show that micro drones can be detected and tracked by applying the joint range-Doppler-azimuth processing. Features extracted from the range-Doppler-azimuth domain can be used to identify drones. © 2018 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Oliveira2019,
	author={Oliveira, M.T.D. and Miranda, R.K. and Costa, J.P.C.L.D. and Almeida, A.L.F.D. and Sousa, R.T.D.},
	title={Low cost antenna array based drone tracking device for outdoor environments},
	journal={Wireless Communications and Mobile Computing},
	year={2019},
	volume={2019},
	art_number={5437908},
	note={cited By 2},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85068849795\&doi=10.1155\%2f2019\%2f5437908\&partnerID=40\&md5=6f7d7359d52a07c4b66bfcee838b6167},
	abstract={Applications of direction of arrival (DoA) techniques have dramatically increased in various areas ranging from the traditional wireless communication systems and rescue operations to GNSS systems and drone tracking. Particularly, police forces and security companies have drawn their attention to drone tracking devices, in order to provide the safeness of citizens and of clients, respectively. In this paper, we propose a low cost antenna array based drone tracking device for outdoor environments. The proposed solution is divided into hardware and software parts. The hardware part of the proposed device is based on off-the-shelf components such as an omnidirectional antenna array, a 4-channel software defined radio (SDR) platform with carrier frequency ranging from 70 MHz to 6 GHz, a FPGA motherboard, and a laptop. The software part includes algorithms for calibration, model order selection (MOS), and DoA estimation, including specific preprocessing steps and a tensor-based estimator to increase the DoA accuracy. We evaluate the performance of our proposed low cost solution in outdoor scenarios. According to our measurement campaigns, we show that when the array is in the front fire position, i.e., with a DoA ranging from-60° to 60°, the maximum and the average DoA errors are 6° and 1,9°, respectively. © 2019 Marcos T. de Oliveira et al.},
	publisher={Hindawi Limited},
}

@ARTICLE{Lu20191941,
	author={Lu, X. and Chen, Z. and Wang, L. and Li, R. and Zhai, C.},
	title={RF-Drone: Multi-tag system for RF-ID enables drone tracking in GPS-denied environments},
	journal={IEICE Transactions on Communications},
	year={2019},
	volume={E102B},
	number={10},
	pages={1941-1950},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85073237627\&doi=10.1587\%2ftranscom.2018DRP0005\&partnerID=40\&md5=31dd44ac148e4d3e35b397c4d49115f5},
	abstract={In resent years, providing location services for mobile targets in a closed environment has been a growing interest. In order to provide good localization and tracking performance for drones in GPS-denied scenarios, this paper proposes a multi-tag radio frequency identification (RFID) system that is easy to equip and does not take up the limited resources of the drone which is not susceptible to processor performance and cost constraints compared with computer vision based approaches. The passive RFID tags, no battery equipped, have an ultra-high resolution of millimeter level. We attach multiple tags to the drone and form multiple sets of virtual antenna arrays during motion, avoiding arranging redundant antennas in applications, and calibrating the speed chain to improve tracking performance. After combining the strap-down inertial navigation system (SINS) carried by the drone, we have established a coupled integration model that can suppress the drift error of SINS with time. The experiment was designed in bi-dimensional and three-dimensional scenarios, and the integrated positioning system based on SINS/RFID was evaluated. Finally, we discussed the impact of some parameters, this innovative approach is verified in real scenarios. Copyright © 2019 The Institute of Electronics, Information and Communication Engineers},
	publisher={Institute of Electronics, Information and Communication, Engineers, IEICE},
}

@CONFERENCE{Stallone2019,
	author={Stallone, R. and Massardo, M. and Montanari, G. and Buono, D. and Madia, D. and Merko, R.},
	title={Omega360 an innovative radar for detection and tracking of small drones},
	journal={2019 International Radar Conference, RADAR 2019},
	year={2019},
	art_number={9078999},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85084949640\&doi=10.1109\%2fRADAR41533.2019.171273\&partnerID=40\&md5=398ee70074fec4a4789fb4508424c41d},
	abstract={The steadily increasing number of small unmanned aerial vehicles (UAV) commonly known as drones implies the need to detect and track them in order to avoid dangerous impacts with other flying objects and to prevent threats. A promising way for detecting, tracking and recognizing drones is to employ radar systems with a long integration time. This paper describes the performance results obtained with an innovative 2D ubiquitous radar, called Omega360, in an Outdoor Test Range sited in San Benedetto del Tronto (Italy). The ubiquity characteristic of Omega360 is obtained with a circular antenna capable of simultaneous staring beams, created by means of Digital Beam Forming, that allow to cover continuously 360 degrees in azimuth. The paper shows how the prolonged time on target provided by the staring beams permits long integration time and then the ability to detect low observability targets such as small drones in a natural environment. © 2019 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Jarabo-Amores2020,
	author={Jarabo-Amores, M.-P. and Mata-Moya, D. and Gomez-Del-Hoyo, P.-J. and Del-Rey-Maestre, N. and Rosado-Sanz, J.},
	title={On the Impact of Drone Airscrews Signature on Passive Radar Detection and Tracking Stages},
	journal={IEEE National Radar Conference - Proceedings},
	year={2020},
	volume={2020-September},
	art_number={9266658},
	note={cited By 1},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85098582302\&doi=10.1109\%2fRadarConf2043947.2020.9266658\&partnerID=40\&md5=ac6f2fdb8999169787cc939f7bccdcfa},
	abstract={In this paper, the impact of the drone airscrews signature in passive radars exploiting Digital Video Broadcasting signals is tackled. Beamforming techniques optimized to minimize the variance of the interference using the statistical characterization of real clutter data followed by a CFAR detector are used to detect drones and their associated airscrews signature. An independent bi-dimensional tracker based on the Kalman filter is proposed to tackle the drone and airscrews tracking process, and to extract micro-Doppler signature features. Real radar data acquired by a technological demonstrator developed at the University of Alcalá were used to evaluate the proposed solution. Results proved the suitability of the proposed detection and tracking schemes for airscrews signature feature extraction. Ansys HFSS electromagnetic simulator validated the results. © 2020 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Zhu2021,
	author={Zhu, H. and Liu, C. and Li, M. and Shang, B. and Liu, M.},
	title={Passive detection of unmanned aerial vehicle in space-air-ground integrated networks},
	journal={Physical Communication},
	year={2021},
	volume={48},
	art_number={101439},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85112345292\&doi=10.1016\%2fj.phycom.2021.101439\&partnerID=40\&md5=0af0f44ed5fe4e3931fbd251a6549b5b},
	abstract={Passive detection of unmanned aerial vehicle (UAV) is an important part of surveillance. Satellite has the potential to play a key role in many applications of space-air-ground integrated networks (SAGIN). In this paper, we propose a novel passive detection method for UAV based on Rao detection. Two hypotheses of UAV detection features are proposed when constructing the signal model. Under this condition, the Rao detection method is extended to weak echo signal detection in a multi-satellite scene. When the noise variance is unknown, two different Rao detectors are designed according to the existence of an interfering target. Moreover, the two detectors’ detection thresholds are obtained given the false alarm probability, respectively. Then, the detection performance of the two detectors is analyzed. Finally, we evaluate the Rao detection performance in different situations with extensive simulations. © 2021 Elsevier B.V.},
	publisher={Elsevier B.V.},
}

@CONFERENCE{Mata-Moya2021,
	author={Mata-Moya, D. and Rey-Maestre, N. and Gomez-Del-Hoyo, P.-J. and Rosado-Sanz, J. and Jarabo-Amores, M.-P.},
	title={4D Passive Radar for Drone Detection and Tracking},
	journal={Proceedings International Radar Symposium},
	year={2021},
	volume={2021-June},
	art_number={9466190},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113909664\&doi=10.23919\%2fIRS51887.2021.9466190\&partnerID=40\&md5=e67a24dcd11615c34f7328241811abcc},
	abstract={An upgraded version of IDEPAR demonstrator capable of detecting and extracting parameters from targets in a 4D measurements space(range, Doppler, azimuth and elevation) is presented to allow the localization of small aerial drones in the Cartesian space (x,y,z). A two-stage spatial filtering processing scheme based on a 2D reception antenna system provides target's directions of arrival (azimuth, elevation) for targets' localization in the Cartesian space. The PR system was validated in measurement campaigns using small drones confirming the location capabilities of the proposed approach. © 2021 German Institute of Navigation (DGON).},
	publisher={IEEE Computer Society},
}

@CONFERENCE{Harman2021,
	author={Harman, S. and Ahmad, B.I.},
	title={The Need for Simultaneous Tracking and Recognition in Drone Surveillance Radar},
	journal={Proceedings International Radar Symposium},
	year={2021},
	volume={2021-June},
	art_number={9466222},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113882484\&doi=10.23919\%2fIRS51887.2021.9466222\&partnerID=40\&md5=39a6c57d14efdad945b14b4fdad9aa37},
	abstract={This paper focuses on the need for good target recognition in order to provide effective tracking and on good tracking to provide effective recognition in the application of radar to drone surveillance. The joint function, merging drone tracking and recognition, referred to as Simultaneous Tracking and Recognition (STaR) of drones is discussed and the benefits are presented through examples. This includes real measurements from Aveillant's Gamekeeper Radar. © 2021 German Institute of Navigation (DGON).},
	publisher={IEEE Computer Society},
}

\section{UAV Detection and Tracking using Radar and Imaging (Multiple Sensor)} % 1 Paper

@CONFERENCE{Dani20211538,
	author={Dani, R.R. and Kubde, R.R. and Sadhu, M.A.},
	title={A Comprehensive Study of Various Techniques for Hostile Drone Detection and Their Classification},
	journal={Proceedings of the 6th International Conference on Communication and Electronics Systems, ICCES 2021},
	year={2021},
	pages={1538-1543},
	art_number={9489236},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113736789\&doi=10.1109\%2fICCES51350.2021.9489236\&partnerID=40\&md5=5721bb2749696013d9d3f8d0b6326704},
	abstract={Today's atmosphere is being increasingly congested due to the proliferation of airborne objects such as small airplanes, helicopters, and unmanned aerial vehicles (drones) of varying forms and sizes. The UAVs can also become a major threat as they can be utilized in smuggling, industrial spy, robbery, and terrorism, besides enabling access to new technologies. Owing to its speed, agility, and altitude, it is hard to defend against a UAV incursion. Aerial defence systems are integrated with a wide range of sensors to efficiently track aircraft. There are several methods and techniques discussed in this paper that are ideal for this specific application. This paper also discusses the paradigm of drone detection using Radar and Imaging techniques and the classification of drones based on their size, features, flying height, and Unique Identification Number (UIN). © 2021 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}


% ==============================================================================================
% ==============================================================================================
% ==============================================================================================
\section{UAV Detection and Tracking using Acoustic Sensor} % 17 Paper

@CONFERENCE{Seo2019,
	author={Seo, Y. and Jang, B. and Im, S.},
	title={Drone Detection Using Convolutional Neural Networks with Acoustic STFT Features},
	journal={Proceedings of AVSS 2018 - 2018 15th IEEE International Conference on Advanced Video and Signal-Based Surveillance},
	year={2019},
	art_number={8639425},
	note={cited By 9},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85063251483\&doi=10.1109\%2fAVSS.2018.8639425\&partnerID=40\&md5=03bf052d7171a6061b73ed58200310fd},
	abstract={As the use of drones has raised in the city, the regulation of malicious usage of drones is an important issue. However, it is difficult to detect a drone due to its miniaturization and modification. In this paper, we investigate the performance of using the convolutional neural networks (CNN) for detecting drones with the acoustic signals received by a microphone. Since the harmonic characteristics of drones are different from those of the objects that produce similar noise including scooters and motorcycles, the two-dimensional feature employed in the study is made of the normalized short time Fourier transform (STFT) magnitude. The performance of the proposed approach is evaluated in terms of detection rate and false alarm rate under various environments. The dataset used in this study consists of the measurements through experiments. The experiments are carried out in the open space with a hovering drone, which is DJI Phantom 3 or Phantom 4. The dataset contains 68,931 frames of drone sound and 41,958 frames of non-drone sound. For the 100-epoch model, the detection rate is 98.97 \% and the false alarm rate is 1.28, while the 10-epoch model demonstrates the detection rate of 98.77 \% and the false alarm rate of 1.62 \%. © 2018 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Anwar20192526,
	author={Anwar, M.Z. and Kaleem, Z. and Jamalipour, A.},
	title={Machine Learning Inspired Sound-Based Amateur Drone Detection for Public Safety Applications},
	journal={IEEE Transactions on Vehicular Technology},
	year={2019},
	volume={68},
	number={3},
	pages={2526-2534},
	art_number={8616877},
	note={cited By 67},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85063268841\&doi=10.1109\%2fTVT.2019.2893615\&partnerID=40\&md5=67048e28db8737300a105a236a170928},
	abstract={In recent years, popularity of unmanned air vehicles enormously increased due to their autonomous moving capability and applications in various domains. This also results in some serious security threats, that needs proper investigation and timely detection of the amateur drones (ADr) to protect the security sensitive institutions. In this paper, we propose the novel machine learning (ML) framework for detection and classification of ADr sounds out of the various sounds like bird, airplanes, and thunderstorm in the noisy environment. To extract the necessary features from ADr sound, Mel frequency cepstral coefficients (MFCC), and linear predictive cepstral coefficients (LPCC) feature extraction techniques are implemented. After feature extraction, support vector machines (SVM) with various kernels are adopted to accurately classify these sounds. The experimental results verify that SVM cubic kernel with MFCC outperform LPCC method by achieving around 96.7\% accuracy for ADr detection. Moreover, the results verified that the proposed ML scheme has more than 17\% detection accuracy, compared with correlation-based drone sound detection scheme that ignores ML prediction. © 1967-2012 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Al-Emadi2019459,
	author={Al-Emadi, S. and Al-Ali, A. and Mohammad, A. and Al-Ali, A.},
	title={Audio based drone detection and identification using deep learning},
	journal={2019 15th International Wireless Communications and Mobile Computing Conference, IWCMC 2019},
	year={2019},
	pages={459-464},
	art_number={8766732},
	note={cited By 25},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85072648004\&doi=10.1109\%2fIWCMC.2019.8766732\&partnerID=40\&md5=a98bf02cf101498ad35beea2b45bd2d3},
	abstract={In recent years, unmanned aerial vehicles (UAVs) have become increasingly accessible to the public due to their high availability with affordable prices while being equipped with better technology. However, this raises a great concern from both the cyber and physical security perspectives since UAVs can be utilized for malicious activities in order to exploit vulnerabilities by spying on private properties, critical areas or to carry dangerous objects such as explosives which makes them a great threat to the society. Drone identification is considered the first step in a multi-procedural process in securing physical infrastructure against this threat. In this paper, we present drone detection and identification methods using deep learning techniques such as Convolutional Neural Network (CNN), Recurrent Neural Network (RNN) and Convolutional Recurrent Neural Network (CRNN). These algorithms will be utilized to exploit the unique acoustic fingerprints of the flying drones in order to detect and identify them. We propose a comparison between the performance of different neural networks based on our dataset which features audio recorded samples of drone activities. The major contribution of our work is to validate the usage of these methodologies of drone detection and identification in real life scenarios and to provide a robust comparison of the performance between different deep neural network algorithms for this application. In addition, we are releasing the dataset of drone audio clips for the research community for further analysis. © 2019 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Sedunov2019,
	author={Sedunov, A. and Haddad, D. and Salloum, H. and Sutin, A. and Sedunov, N. and Yakubovskiy, A.},
	title={Stevens Drone Detection Acoustic System and Experiments in Acoustics UAV Tracking},
	journal={2019 IEEE International Symposium on Technologies for Homeland Security, HST 2019},
	year={2019},
	art_number={9032916},
	note={cited By 6},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85078740995\&doi=10.1109\%2fHST47167.2019.9032916\&partnerID=40\&md5=f05665e8b9991d975cae8cb3f3ec9c14},
	abstract={Concerns about improper use of Unmanned Aerial Vehicles (UAVs, also unmanned aerial systems or UAS) led to the development of various methods for their detection, tracking, and classification. One of the methods is using acoustics. Advantages of passive acoustics include the low cost of acoustic systems, finding of the Direction of Arrival (DOA) and localization by simple means; and classification of UAV sounds by acoustic signature. Stevens Institute of Technology has developed and built the Drone Acoustic Detection System (DADS) that can detect, track and classify UAVs based on the propeller noise. The system consists of three or more microphone nodes. The microphones in each node are arranged in a tetrahedron with configurable size. The microphone data is transferred over WiFi in real-time to a central computer, where it is processed. The Stevens DADS system was investigated in numerous field tests together with several other directional arrays including a 16-channel two-tier cross array, the OptiNav 40-microphone phased array, and parabolic and shot gun microphones. Multirotor UAVs of different sizes were employed in testing, including DJI models Phantom 4, M600 and S1000. The test results of the different systems were compared. © 2019 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Shi20202731,
	author={Shi, Z. and Chang, X. and Yang, C. and Wu, Z. and Wu, J.},
	title={An Acoustic-Based Surveillance System for Amateur Drones Detection and Localization},
	journal={IEEE Transactions on Vehicular Technology},
	year={2020},
	volume={69},
	number={3},
	pages={2731-2739},
	art_number={8950116},
	note={cited By 10},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85082063635\&doi=10.1109\%2fTVT.2020.2964110\&partnerID=40\&md5=f9ed2b64e134858cebaf71ddcda18fac},
	abstract={Due to cost reduction and device miniaturization, amateur drones are now widely used in numerous civilian and commercial applications. However, the abuse of amateur drones has resulted in emerging threats to personal privacy and public security. To alleviate these threats, we design an acoustic-based surveillance system, which can achieve the capacity of amateur drones detection and localization with 24/7 (24 hours per day and 7 days per week under normal circumstances) availability. In the designed system, a detection fusion algorithm and a TDOA estimation algorithm based on the Bayesian filter are applied to improve the performance of drone detection and localization. Field experiments are carried out, and the results demonstrate that the designed system can detect and locate an amateur drone in real time with high accuracy and 24/7 availability. © 1967-2012 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Uddin2020236,
	author={Uddin, Z. and Altaf, M. and Bilal, M. and Nkenyereye, L. and Bashir, A.K.},
	title={Amateur Drones Detection: A machine learning approach utilizing the acoustic signals in the presence of strong interference},
	journal={Computer Communications},
	year={2020},
	volume={154},
	pages={236-245},
	note={cited By 8},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85080874387\&doi=10.1016\%2fj.comcom.2020.02.065\&partnerID=40\&md5=679d83ca6c2c966c81b2112aa181570b},
	abstract={Owing to small size, sensing capabilities and autonomous nature, the Unmanned Air Vehicles (UAVs) have enormous applications in various areas e.g., remote sensing, navigation, archaeology, journalism, environmental science, and agriculture. However, the un-monitored deployment of UAVs called the amateur drones (AmDr) can lead to serious security threats and risk to human life and infrastructure. Therefore, timely detection of the AmDr is essential for the protection and security of sensitive organizations, human life and other vital infrastructure. AmDrs can be detected using different techniques based on sound, video, thermal, and radio frequencies. However, the performance of these techniques is limited in sever atmospheric conditions. In this paper, we propose an efficient un-supervise machine learning approach of independent component analysis (ICA) to detect various acoustic signals i.e., sounds of bird, airplanes, thunderstorm, rain, wind and the UAVs in practical scenario. After unmixing the signals, the features like Mel Frequency Cepstral Coefficients (MFCC), the power spectral density (PSD) and the Root Mean Square Value (RMS) of the PSD are extracted by using ICA. The PSD and the RMS of PSD signals are extracted by first passing the signals from octave band filter banks. Based on the above features the signals are classified using Support Vector Machines (SVM)and K Nearest Neighbour (KNN)to detect the presence or absence of AmDr. Unique feature of the proposed technique is the detection of a single or multiple AmDrs at a time in the presence of multiple acoustic interfering signals. The proposed technique is verified through extensive simulations and it is observed that the RMS values of PSD with KNN performs better than the MFCC with KNN and SVM. © 2020 Elsevier B.V.},
	publisher={Elsevier B.V.},
}

@ARTICLE{Uddin202163456,
	author={Uddin, Z. and Nebhen, J. and Altaf, M. and Orakzai, F.A.},
	title={Independent Vector Analysis Inspired Amateur Drone Detection through Acoustic Signals},
	journal={IEEE Access},
	year={2021},
	volume={9},
	pages={63456-63462},
	art_number={9410561},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85104596461\&doi=10.1109\%2fACCESS.2021.3074966\&partnerID=40\&md5=e7db64f28b0681a233304cb4714efde8},
	abstract={Detection of amateur drones (AmDrs) is mandatory requirement of various defence organizations and is also required to protect human life. In literature, various researchers contributed in this regard and developed different algorithms utilizing video, thermal, radio frequencies and acoustic signals. However, inefficiency of the existing techniques is reported in different atmospheric conditions. In this paper, acoustic signal processing is performed based on independent vector analysis (IVA) to detect AmDrs in the field. This technique is capable to detect more than one AmDrs in the sensing field at a time in the presence of strong interfering sources. The IVA is a relatively new and practically applicable technique of blind source separation and is more efficient than the independent component analysis technique. In the proposed technique, recorded mixed signals through multiple microphones are first un-mixed through using the IVA technique. Then various features of the separated signals are extracted. These features include Root Mean Square (RMS) values, Power Spectral Density (PSD) and Mel Frequency Cepstral coefficients (MFCC). Finally, signals classification is performed through Support Vector Machines (SVM)and K Nearest Neighbor (KNN) to detect AmDrs in the field. Performance evaluation of the proposed technique is carried out through simulations and observed the superior performance of the proposed technique. © 2013 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Salman2021335,
	author={Salman, S. and Mir, J. and Farooq, M.T. and Malik, A.N. and Haleemdeen, R.},
	title={Machine Learning Inspired Efficient Audio Drone Detection using Acoustic Features},
	journal={Proceedings of 18th International Bhurban Conference on Applied Sciences and Technologies, IBCAST 2021},
	year={2021},
	pages={335-339},
	art_number={9393232},
	note={cited By 2},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85104663735\&doi=10.1109\%2fIBCAST51254.2021.9393232\&partnerID=40\&md5=08a2f9d93b937f5dd78569e1acd82886},
	abstract={With the recent proliferation of drones in the consumer market, drone detection has become critical to address the security and privacy issues raised by drone technology. This paper presents an efficient method for drone detection based on the drone's acoustic signature. Five different features are analyzed and compared to determine the best audio descriptor for drone detection. The selected features include Mel-frequency cepstral coefficients, Gammatone cepstral coefficients, linear prediction coefficients, spectral roll-off, and zero-crossing rate. Different support vector machine (SVM) classifier models are trained and tested on a large diverse database using 10-fold and 20\% data holdout cross-validation schemes to evaluate the individual feature performance for efficient drone detection. Experimental results indicate that Gammatone cepstral coefficients are the most efficient features for audio drone detection. Further, the medium Gaussian SVM trained on all the investigated features achieves the classification accuracy of 99.9\% with 99.8\% recall and 100\% precision, outperforming the compared existing state-of-the-art audio drone detection methods. © 2021 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Ohlenbusch20216,
	author={Ohlenbusch, M. and Ahrens, A. and Rollwage, C. and Bitzer, J.},
	title={Robust drone detection for acoustic monitoring applications},
	journal={European Signal Processing Conference},
	year={2021},
	volume={2021-January},
	pages={6-10},
	art_number={9287433},
	note={cited By 1},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85099318868\&doi=10.23919\%2fEusipco47968.2020.9287433\&partnerID=40\&md5=c3e7331f08ab67dc49eb5f292ac2e8e2},
	abstract={Commercially available light-weight unmanned aerial vehicles (UAVs) present a challenge for public safety, e.g. espionage, transporting dangerous goods or devices. Therefore, countermeasures are necessary. Usually, detection of UAVs is a first step. Along many other modalities, acoustic detection seems promising. Recent publications show interesting results by using machine and deep learning methods. The acoustic detection of UAVs appears to be particularly difficult in adverse situations, such as in heavy wind noise or in the presence of construction noise. In this contribution, the typical feature set is extended to increase separation of background noise and the UAV signature noise. The decision algorithm utilized is support vector machine (SVM) classification. The classification is based on an extended training dataset labeled to support binary classification. The proposed method is evaluated in comparison to previously published algorithms, on the basis of a dataset recorded from different acoustic environments, including unknown UAV types. The results show an improvement over existing methods, especially in terms of false-positive detection rate. For a first step into real-time embedded systems a recursive feature elimination method is applied to reduce the model dimensionality. The results indicate only a slight decreases in detection performance. © 2021 European Signal Processing Conference, EUSIPCO. All rights reserved.},
	publisher={European Signal Processing Conference, EUSIPCO},
}

@ARTICLE{Kolamunna2021,
	author={Kolamunna, H. and Dahanayaka, T. and Li, J. and Seneviratne, S. and Thilakaratne, K. and Zomaya, A.Y. and Seneviratne, A.},
	title={DronePrint: Acoustic Signatures for Open-set Drone Detection and Identification with Online Data},
	journal={Proceedings of the ACM on Interactive, Mobile, Wearable and Ubiquitous Technologies},
	year={2021},
	volume={5},
	number={1},
	art_number={3448115},
	note={cited By 1},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85103617755\&doi=10.1145\%2f3448115\&partnerID=40\&md5=17c6a7cfc90ea02b91d25045125725cc},
	abstract={With the ubiquitous availability of drones, they are adopted benignly in multiple applications such as cinematography, surveying, and legal goods delivery. Nonetheless, they are also being used for reconnaissance, invading personal or secure spaces, harming targeted individuals, smuggling drugs and contraband, or creating public disturbances. These malicious or improper use of drones can pose significant privacy and security threats in both civilian and military settings. Therefore, it is vital to identify drones in different environments to assist the decisions on whether or not to contain unknown drones. While there are several methods proposed for detecting the presence of a drone, they have limitations when it comes to low visibility, limited access, or hostile environments. In this paper, we propose DronePrint that uses drone acoustic signatures to detect the presence of a drone and identify the make and the model of the drone. We address the shortage of drone acoustic data by relying on audio components of online videos. In drone detection, we achieved 96\% accuracy in a closed-set scenario, and 86\% accuracy in a more challenging open-set scenario. Our proposed method of cascaded drone identification, where a drone is identified for its 'make' followed by the 'model' of the drone achieves 90\% overall accuracy. In this work, we cover 13 commonly used commercial and consumer drone models, which is to the best of understanding is the most comprehensive such study to date. Finally, we demonstrate the robustness of DronePrint to drone hardware modifications, Doppler effect, varying SNR conditions, and in realistic open-set acoustic scenes. © 2021 ACM.},
	publisher={Association for Computing Machinery},
}

@ARTICLE{Al-Emadi2021,
	author={Al-Emadi, S. and Al-Ali, A. and Al-Ali, A.},
	title={Audio-based drone detection and identification using deep learning techniques with dataset enhancement through generative adversarial networks†},
	journal={Sensors},
	year={2021},
	volume={21},
	number={15},
	art_number={4953},
	note={cited By 3},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85110553859\&doi=10.3390\%2fs21154953\&partnerID=40\&md5=eb11d513250c12d3519843b4337ea665},
	abstract={Drones are becoming increasingly popular not only for recreational purposes but in day-to-day applications in engineering, medicine, logistics, security and others. In addition to their useful applications, an alarming concern in regard to the physical infrastructure security, safety and privacy has arisen due to the potential of their use in malicious activities. To address this problem, we propose a novel solution that automates the drone detection and identification processes using a drone’s acoustic features with different deep learning algorithms. However, the lack of acoustic drone datasets hinders the ability to implement an effective solution. In this paper, we aim to fill this gap by introducing a hybrid drone acoustic dataset composed of recorded drone audio clips and artificially generated drone audio samples using a state-of-the-art deep learning technique known as the Generative Adversarial Network. Furthermore, we examine the effectiveness of using drone audio with different deep learning algorithms, namely, the Convolutional Neural Network, the Recurrent Neural Network and the Convolutional Recurrent Neural Network in drone detection and identification. Moreover, we investigate the impact of our proposed hybrid dataset in drone detection. Our findings prove the advantage of using deep learning techniques for drone detection and identification while confirming our hypothesis on the benefits of using the Generative Adversarial Networks to generate real-like drone audio clips with an aim of enhancing the detection of new and unfamiliar drones. © 2021 by the authors. Licensee MDPI, Basel, Switzerland.},
	publisher={MDPI AG},
}

@CONFERENCE{Chang2018573,
	author={Chang, X. and Yang, C. and Wu, J. and Shi, X. and Shi, Z.},
	title={A Surveillance System for Drone Localization and Tracking Using Acoustic Arrays},
	journal={Proceedings of the IEEE Sensor Array and Multichannel Signal Processing Workshop},
	year={2018},
	volume={2018-July},
	pages={573-577},
	art_number={8448409},
	note={cited By 27},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85053598809\&doi=10.1109\%2fSAM.2018.8448409\&partnerID=40\&md5=d4ec0d633505809085aad4f57c0c5663},
	abstract={The wide proliferation of drones has posed great threats to personal privacy and public security, which makes it urgent to monitor the drones in the sensitive areas. Drone surveillance using acoustic arrays, as a promising method, could localize and track the drones effectively. In this paper, we develop a systematic method for drone localization and tracking by using acoustic arrays. Specifically, we develop a time difference of arrival (TDOA) estimation algorithm based on Gauss priori probability density function to overcome the multipath effect and the low signal-to-noise ratio (SNR), and design a localization method by making full use of the TDOA estimation results, followed by tracking the drone by Kalman filter. Finally, field experiments are carried out to verify the effectiveness and performance of the proposed methods. The results show that they can achieve good performance in drone localization and tracking. © 2018 IEEE.},
	publisher={IEEE Computer Society},
}

@CONFERENCE{Wang20182511,
	author={Wang, L. and Sanchez-Matilla, R. and Cavallaro, A.},
	title={Tracking a moving sound source from a multi-rotor drone},
	journal={IEEE International Conference on Intelligent Robots and Systems},
	year={2018},
	pages={2511-2516},
	art_number={8594483},
	note={cited By 11},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85063013801\&doi=10.1109\%2fIROS.2018.8594483\&partnerID=40\&md5=3a2de526d0fe5e689aa14cd8774a6dc6},
	abstract={We propose a method to track from a multi-rotor drone a moving source, such as a human speaker or an emergency whistle, whose sound is mixed with the strong ego-noise generated by rotating motors and propellers. The proposed method is independent of the specific drone and does not need pre-training nor reference signals. We first employ a time-frequency spatial filter to estimate, on short audio segments, the direction of arrival of the moving source and then we track these noisy estimations with a particle filter. We quantitatively evaluate the results using a ground-truth trajectory of the sound source obtained with an on-board camera and compare the performance of the proposed method with baseline solutions. © 2018 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Jung2019,
	author={Jung, I.-J. and Ih, J.-G.},
	title={Acoustic localization and tracking of the multiple drones},
	journal={INTER-NOISE 2019 MADRID - 48th International Congress and Exhibition on Noise Control Engineering},
	year={2019},
	note={cited By 2},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85084160406\&partnerID=40\&md5=5d12463b67127706fb9eb5946c74bc9a},
	abstract={Due to the social problems in the intrusion of privacy and the collision hazard, monitoring of the drones are needed for the regulations. To enhance the identification of multiple drones flying at a specific zone simultaneously, a new localization method other than the optical or electromagnetic methods is needed. In this work, a method to use the acoustic cues of the drone is presented, and the three-dimensional acoustic intensimetry (3DAI) is employed for the localization. The 3DAI implements the compensation algorithm for the spectral bias error of the probe configured in a tetrahedron shape. The blade passing frequency and its harmonics radiated from the quadcopter drones are adopted as the acoustical cues for the detection. The test for single drone is done within an anechoic chamber to estimate the localization error in the real-time. For the multiple drones, the test is carried out for the localization by using recorded sounds of three drones having different rotor sizes. The results show that the mean azimuth and elevation angle error is less than 5° for localization of multiple drones. The localization result is fine when BPFs are distinguishable, but, for the case with spectral overlap, it bears a large error. © INTER-NOISE 2019 MADRID - 48th International Congress and Exhibition on Noise Control Engineering. All Rights Reserved.},
	publisher={SOCIEDAD ESPANOLA DE ACUSTICA - Spanish Acoustical Society, SEA},
}

@CONFERENCE{Baggenstoss2019,
	author={Baggenstoss, P.M. and Springer, M. and Oispuu, M. and Kurth, F.},
	title={Efficient phase-based acoustic tracking of drones using a microphone array},
	journal={European Signal Processing Conference},
	year={2019},
	volume={2019-September},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85075607680\&doi=10.23919\%2fEUSIPCO.2019.8902972\&partnerID=40\&md5=d4b581d8748faa1b3bd363cffe087b3c},
	abstract={An efficient phase-based acoustic detection and tracking algorithm for drones is presented. The algorithm separately tracks the time difference of arrival (TDOA) of the incoming signal with respect to microphone pairs based on the phase in the discrete Fourier transform (DFT) bins. The direction of arrival (DOA) of the drone is determined by forming a solution curve corresponding to each TDOA, then clustering the curve intersections. The algorithm avoids the computationally expensive grid-search over DOA, so is significantly more efficient than beamforming. The proposed algorithm and the maximum likelihood (ML) processor (beamformer) are compared in simulated and real data scenarios. Using simulated data, the ML estimator is shown to agree with the Cramér-Rao lower bound (CRLB) and the proposed algorithm is shown to approach the performance of ML at higher SNR. In real data scenarios, the phase-based algorithm implemented with simple alpha-beta TDOA trackers consistently tracked the target through difficult maneuvers at short and long range, showing no degradation with respect to the beamformer. Other potential advantages include robustness against interference and ability to create phase-based spectrograms for classification. © 2019 IEEE},
	publisher={European Signal Processing Conference, EUSIPCO},
}

@CONFERENCE{Sedunov2019,
	author={Sedunov, A. and Haddad, D. and Salloum, H. and Sutin, A. and Sedunov, N. and Yakubovskiy, A.},
	title={Stevens Drone Detection Acoustic System and Experiments in Acoustics UAV Tracking},
	journal={2019 IEEE International Symposium on Technologies for Homeland Security, HST 2019},
	year={2019},
	art_number={9032916},
	note={cited By 6},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85078740995\&doi=10.1109\%2fHST47167.2019.9032916\&partnerID=40\&md5=f05665e8b9991d975cae8cb3f3ec9c14},
	abstract={Concerns about improper use of Unmanned Aerial Vehicles (UAVs, also unmanned aerial systems or UAS) led to the development of various methods for their detection, tracking, and classification. One of the methods is using acoustics. Advantages of passive acoustics include the low cost of acoustic systems, finding of the Direction of Arrival (DOA) and localization by simple means; and classification of UAV sounds by acoustic signature. Stevens Institute of Technology has developed and built the Drone Acoustic Detection System (DADS) that can detect, track and classify UAVs based on the propeller noise. The system consists of three or more microphone nodes. The microphones in each node are arranged in a tetrahedron with configurable size. The microphone data is transferred over WiFi in real-time to a central computer, where it is processed. The Stevens DADS system was investigated in numerous field tests together with several other directional arrays including a 16-channel two-tier cross array, the OptiNav 40-microphone phased array, and parabolic and shot gun microphones. Multirotor UAVs of different sizes were employed in testing, including DJI models Phantom 4, M600 and S1000. The test results of the different systems were compared. © 2019 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Guo2020,
	author={Guo, J. and Ahmad, I. and Chang, K.H.},
	title={Classification, positioning, and tracking of drones by HMM using acoustic circular microphone array beamforming},
	journal={Eurasip Journal on Wireless Communications and Networking},
	year={2020},
	volume={2020},
	number={1},
	art_number={9},
	note={cited By 5},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85077507201\&doi=10.1186\%2fs13638-019-1632-9\&partnerID=40\&md5=6a5717f70f3fd8dbf78af3c10b815ced},
	abstract={This paper addresses issues with monitoring systems that identify and track illegal drones. The development of drone technologies promotes the widespread commercial application of drones. However, the ability of a drone to carry explosives and other destructive materials may pose serious threats to public safety. In order to reduce these threats, we propose an acoustic-based scheme for positioning and tracking of illegal drones. Our proposed scheme has three main focal points. First, we scan the sky with switched beamforming to find sound sources and record the sounds using a microphone array; second, we perform classification with a hidden Markov model (HMM) in order to know whether the sound is a drone or something else. Finally, if the sound source is a drone, we use its recorded sound as a reference signal for tracking based on adaptive beamforming. Simulations are conducted under both ideal conditions (without background noise and interference sounds) and non-ideal conditions (with background noise and interference sounds), and we evaluate the performance when tracking illegal drones. © 2020, The Author(s).},
	publisher={Springer},
}


\section{UAV Detection and Tracking using Infrared Imagery} % 2 Paper

@ARTICLE{Ryu20181146,
	author={Ryu, J. and Kim, S.},
	title={Data driven proposal and deep learning-based small infrared drone detection},
	journal={Journal of Institute of Control, Robotics and Systems},
	year={2018},
	volume={24},
	number={12},
	pages={1146-1151},
	note={cited By 1},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85058642831\&doi=10.5302\%2fJ.ICROS.2018\&partnerID=40\&md5=c68276af7636c1292162e4a66cc03619},
	abstract={In this paper, we propose a data-driven and deep-learning based classification scheme for small infrared target detection. Previous studies have shown feasible performance using conventional computer vision techniques, such as spatial and temporal filters. However, those handcrafted approaches are not optimized due to the nature of the application fields. Recently, deep-learning has shown excellent performance for many computer vision problems. The proposed data-driven proposal and convolutional neural network (DDP-CNN) approach can generate possible target locations through the DDP, and final targets are recognized through the CNN for classification. According to the experimental results using drone databases, the DDP-CNN shows an 0.85 average precision (AP) of target detection. © ICROS 2018.},
	publisher={Institute of Control, Robotics and Systems},
}

@CONFERENCE{Sommer2020,
	author={Sommer, L. and Schumann, A.},
	title={Deep learning-based drone detection in infrared imagery with limited training data},
	journal={Proceedings of SPIE - The International Society for Optical Engineering},
	year={2020},
	volume={11542},
	art_number={1154204},
	note={cited By 1},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85096365614\&doi=10.1117\%2f12.2574171\&partnerID=40\&md5=f105d82088e98a2cd7918679fe4e825e},
	abstract={The increased availability and capabilities of drones in the consumer market has lead to increased risk in air traffic control and other public safety concerns. Automated drone detection systems can help to generate alerts and increase reaction time by security forces. Recently proposed approaches and systems are usually based on a combination of sensors and machine learning to carry out the detection of drones. While electro-optical imagery is the most prevalent modality, infrared sensors can complement it by providing better visibility in certain situations with cluttered background or low light conditions. A key limitation when using infrared data is the limited availability of data for training machine learning methods. In this work, we specifically focus on the task of drone detection in infrared imagery. Our main focus lies on investigating how the small amount of available infrared data can be compensated for. We approach this problem through three different types of experiments. First, we compare a detector resulting from training on limited infrared data with a detector trained on more diverse optical data. We then propose and evaluate several methods for pre-processing optical data in such a way that it better resembles the characteristics of infrared data. Finally, we train detectors on a combination of infrared and pre-processed optical data and evaluate the trade-off between amount of available infrared data and achieved accuracy of the resulting detector. We evaluate all detectors on our own set of diverse infrared recordings. Our results show that suitable pre-processing of optical data can significantly improve the resulting accuracy and performs much better than training solely on limited infrared data. © 2020 SPIE},
	publisher={SPIE},
}
% ==============================================================================================
% ==============================================================================================
% ==============================================================================================

\section{UAV Detection and Tracking using Bluetooth} % 1 Paper

@ARTICLE{Shin20211,
	author={Shin, J.-M. and Kim, Y.-S. and Ban, T.-W. and Choi, S. and Kang, K.-M. and Ryu, J.-Y.},
	title={Position tracking techniques using multiple receivers for anti-drone systems},
	journal={Sensors (Switzerland)},
	year={2021},
	volume={21},
	number={1},
	pages={1-14},
	art_number={35},
	note={cited By 3},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85098670763\&doi=10.3390\%2fs21010035\&partnerID=40\&md5=c639a79645c9d19242a90f07eb961df0},
	abstract={The need for drone traffic control management has emerged as the demand for drones increased. Particularly, in order to control unauthorized drones, the systems to detect and track drones have to be developed. In this paper, we propose the drone position tracking system using multiple Bluetooth low energy (BLE) receivers. The proposed system first estimates the target’s location, which consists of the distance and angle, while using the received signal strength indication (RSSI) signals at four BLE receivers and gradually tracks the target based on the estimated distance and angle. We propose two tracking algorithms, depending on the estimation method and also apply the memory process, improving the tracking performance by using stored previous movement information. We evaluate the proposed system’s performance in terms of the average number of movements that are required to track and the tracking success rate. © 2020 by the authors. Licensee MDPI, Basel, Switzerland.},
	publisher={MDPI AG},
}


\section{Others} % 4 Paper

@ARTICLE{Sciancalepore2020,
	author={Sciancalepore, S. and Ibrahim, O.A. and Oligeri, G. and Di Pietro, R.},
	title={PiNcH: An effective, efficient, and robust solution to drone detection via network traffic analysis},
	journal={Computer Networks},
	year={2020},
	volume={168},
	art_number={107044},
	note={cited By 18},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85076546502\&doi=10.1016\%2fj.comnet.2019.107044\&partnerID=40\&md5=2338a5e886850121c1e54c7e3595bd7c},
	abstract={We propose Picking a Needle in a Haystack (PiNcH), a methodology to detect the presence of a drone, its current status, and its movements by leveraging just the communication traffic exchanged between the drone and its Remote Controller (RC). PiNcH is built applying standard classification algorithms to the eavesdropped traffic, analyzing features such as packets inter-arrival time and size. PiNcH is fully passive and it requires just cheap and general-purpose hardware. To evaluate the effectiveness of our solution, we collected real communication traces originated by a drone running the widespread ArduCopter open-source firmware, currently mounted on-board of a wide range (30+) of commercial amateur drones. Then, we tested our solution against different publicly available wireless traces. The results prove that PiNcH can efficiently and effectively: (i) identify the presence of the drone in several heterogeneous scenarios; (ii) identify the current state of a powered-on drone, i.e., flying or lying on the ground; (iii) discriminate the movements of the drone; and, finally, (iv) enjoy a reduced upper bound on the time required to identify a drone with the requested level of assurance. The effectiveness of PiNcH has been also evaluated in the presence of both heavy packet loss and evasion attacks. In this latter case, the adversary modifies on purpose the profile of the traffic of the drone-RC link to avoid the detection. In both the cited cases, PiNcH continues enjoying a remarkable performance. Further, the comparison against state of the art solution confirms the superior performance of PiNcH in several scenarios. Note that all the drone-controller generated data traces have been released as open-source, to allow replicability and foster follow-up. Finally, the quality and viability of our solution, do prove that network traffic analysis can be successfully adopted for drone identification and status discrimination, and pave the way for future research in the area. © 2019},
	publisher={Elsevier B.V.},
}

@CONFERENCE{Salhi2020,
	author={Salhi, M. and Boudriga, N.},
	title={Multi-array spherical LIDAR system for drone detection},
	journal={International Conference on Transparent Optical Networks},
	year={2020},
	volume={2020-July},
	art_number={9203381},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85092452815\&doi=10.1109\%2fICTON51198.2020.9203381\&partnerID=40\&md5=0afd0f4f5cb66f010e6e2a826a8f661a},
	abstract={The detection of unmanned aerial vehicles (UAVs) represents a necessity to protect critical areas and infrastructures against potential attacks performed by these UAVs. Different detection solutions have been proposed in the literature. They include conventional radars, radio frequency signal detection, acoustic detection, as well as light detection and ranging (Lidar). Using cameras, the latter technology is new and promising, yet controversial for its feasibility and cost effectiveness. In this paper, we propose a multi-array Lidar system that is capable of detecting potential UAVs using visible light communication. The system is composed of laser sources and laser concentrators. These transmitting/receiving elements are arranged through arrays along a spherical form including a photodiode at its centre. The reflected optical energy reaching the concentrators is transmitted to this central photodiode. The work assesses the feasibility and effectiveness of the solution through an in-depth examination of the design parameters. This includes the sensors' characteristics, the elements positioning and interspace, as well as the dimensions of the monitored cylinder. © 2020 IEEE.},
	publisher={IEEE Computer Society},
}

@CONFERENCE{Heidger2021,
	author={Heidger, R. and Lambercy, V. and Lambers, D.},
	title={Tracking Analysis of Drone Detection Systems at Airports: Methodology and Results},
	journal={Proceedings International Radar Symposium},
	year={2021},
	volume={2021-June},
	art_number={9466192},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85113871508\&doi=10.23919\%2fIRS51887.2021.9466192\&partnerID=40\&md5=c7bcded901564f2e3ebd6454725f2049},
	abstract={This paper describes the methodology that has been established in the DFS to test Drone Detection Systems (DDS) at airports, as well as the global test results of the test campaign conducted at Frankfurt and Munich airports in summer and autumn 2020 together with Fraport and FMG. The test campaign was part of a feasibility study to evaluate, what small noncooperative UAS current DDS systems today can detect and track at large infrastructures like airports, and which limitations exist. © 2021 German Institute of Navigation (DGON).},
	publisher={IEEE Computer Society},
}

@CONFERENCE{Chen20212839,
	author={Chen, G. and Wang, W. and He, Z. and Wang, L. and Yuan, Y. and Zhang, D. and Zhang, J. and Zhu, P. and Van Gool, L. and Han, J. and Hoi, S. and Hu, Q. and Liu, M. and Sciarrone, A. and Sun, C. and Garibotto, C. and Tran, D.N.-N. and Lavagetto, F. and Haleem, H. and Motorcu, H. and Ates, H.F. and Nguyen, H.-H. and Jeon, H.-J. and Bisio, I. and Jeon, J.W. and Li, J. and Pham, L.H. and Jeon, M. and Feng, Q. and Li, S. and Tran, T.H.-P. and Pan, X. and Song, Y.-M. and Yao, Y. and Du, Y. and Xu, Z. and Luo, Z.},
	title={VisDrone-MOT2021: The Vision Meets Drone Multiple Object Tracking Challenge Results},
	journal={Proceedings of the IEEE International Conference on Computer Vision},
	year={2021},
	volume={2021-October},
	pages={2839-2846},
	note={cited By 0},
	url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85122776407\&doi=10.1109\%2fICCVW54120.2021.00318\&partnerID=40\&md5=ae844c8f5ec548c634fca39509c6f9f2},
	abstract={Vision Meets Drone: Multiple Object Tracking (VisDrone-MOT2021) challenge - the forth annual activity organized by the VisDrone team - focuses on benchmarking UAV MOT algorithms in realistic challenging environments. It is held in conjunction with ICCV 2021. VisDrone-MOT2021 contains 96 video sequences in total, including 56 sequences (~24K frames) for training, 7 sequences (~3K frames) for validation and 33 sequences (~13K frames) for testing. Bounding-box annotations for novel object categories are provided every frame and temporally consistent instance IDs are also given. Additionally, occlusion ratio and truncation ratio are provided as extra useful annotations. The results of eight state-of-the-art MOT algorithms are reported and discussed. We hope that our VisDrone-MOT2021 challenge will facilitate future research and applications in the field of UAV vision. The website of our challenge can be found at http://www.aiskyeye.com/. © 2021 IEEE.},
	publisher={Institute of Electrical and Electronics Engineers Inc.},
}





==> UAVdetectionRef.tex <==
Scopus
EXPORT DATE: 7 February 2022

@ARTICLE{Zhu2021,
author={Zhu, H. and Liu, C. and Li, M. and Shang, B. and Liu, M.},
title={Passive detection of unmanned aerial vehicle in space-air-ground integrated networks},
journal={Physical Communication},
year={2021},
volume={48},
art_number={101439},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85112345292&doi=10.1016%2fj.phycom.2021.101439&partnerID=40&md5=0af0f44ed5fe4e3931fbd251a6549b5b},
abstract={Passive detection of unmanned aerial vehicle (UAV) is an important part of surveillance. Satellite has the potential to play a key role in many applications of space-air-ground integrated networks (SAGIN). In this paper, we propose a novel passive detection method for UAV based on Rao detection. Two hypotheses of UAV detection features are proposed when constructing the signal model. Under this condition, the Rao detection method is extended to weak echo signal detection in a multi-satellite scene. When the noise variance is unknown, two different Rao detectors are designed according to the existence of an interfering target. Moreover, the two detectors’ detection thresholds are obtained given the false alarm probability, respectively. Then, the detection performance of the two detectors is analyzed. Finally, we evaluate the Rao detection performance in different situations with extensive simulations. © 2021 Elsevier B.V.},
publisher={Elsevier B.V.},
}

@ARTICLE{Tony2021506,
author={Tony, L.A. and Ghose, D. and Chakravarthy, A.},
title={Unmanned aerial vehicle mid-air collision detection and resolution using avoidance maps},
journal={Journal of Aerospace Information Systems},
year={2021},
volume={18},
number={8},
pages={506-529},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85114640728&doi=10.2514%2f1.I010900&partnerID=40&md5=424a79a82b468776f59461b6d05d27fb},
abstract={Collision avoidance for fixed-wing unmanned aerial vehicles (UAVs), using a novel methodology of avoidance map, is addressed in this work. Avoidance map is defined as a mapping in the control input space of a pair of UAVs, which partitions the control space into avoidance and collision regions, respectively. The choice of maneuvers to execute successful avoidance can be effectively obtained by using the avoidance map. The duration of control application is determined by a simple method that is time optimal and computationally efficient. Different versions of the map portraying the evolution of the concept are also given. Precision control, defined as a gradual reduction in control, is discussed to reduce the control input demand for the entire duration of avoidance. The concept is extended to multiple UAVs, and the additional requirement of the UAVs to return to nominal trajectory after avoidance, using Dubins paths, is also addressed. Finally, simulation results using realistic UAV models are considered, and some needed modifications to the basic avoidance strategy, made necessary by realistic maneuver models, are discussed. Several illustrative simulation results are given to support the applicability of the proposed method. Copyright © 2021 by Lima Agnel Tony, Debasish Ghose, and Animesh Chakravarty. Published by the American Institute of Aeronautics and Astronautics, Inc., with permission.},
publisher={AIAA International},
}

@ARTICLE{Guan20211,
author={Guan, R. and Yu, J. and Li, M. and Yan, J. and Liu, Z.},
title={Preparation of electrochemical sensor assisted unmanned aerial vehicles system for SO2, O3, NO2, CO and PM2.5/PM10 detection in air},
journal={International Journal of Electrochemical Science},
year={2021},
volume={16},
pages={1-9},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85115645821&doi=10.20964%2f2021.10.28&partnerID=40&md5=ca65f8a981540b84bdf65b6067ad1352},
abstract={The spatial and especially vertical monitoring of atmospheric pollutants is of great significance to the analysis and prevention of air pollution. It is also a useful supplement to the current monitoring method which is mainly based on ground monitoring stations. Small UAVs offer a new way of vertical monitoring of air pollution. In this study, an electrochemical sensor incorporated unmanned aerial vehicles (UAV) platform was proposed, which can detect pollution at vertical heights, and has been used for PM2.5, PM10 and 4 pollutants (SO2, O3, NO2, CO) at different heights. Based on this monitoring data, the vertical distribution characteristics as well as the statistical correlation of PM2.5 and its pollutants were analyzed. The experimental results show that PM2.5 concentration increases with height in the larger integrated industrial areas, while it decreases and then increases near the small-scale industrial and residential areas. The trends of PM10 and PM2.5 are basically consistent. In the vertical direction, the maximum values of CO and SO2 always appear near the ground and then start to decrease, and NO2 increases with the height © 2021 The Authors. Published by ESG (www.electrochemsci.org). This article is an open access article distributed under the terms and conditions of the Creative Commons Attribution license (http://creativecommons.org/licenses/by/4.0/).},
publisher={Electrochemical Science Group},
}

@ARTICLE{Li2021,
author={Li, J. and Sun, T. and Huang, X. and Ma, L. and Lin, Q. and Chen, J. and Leung, V.C.M.},
title={A Memetic Path Planning Algorithm for Unmanned Air/Ground Vehicle Cooperative Detection Systems},
journal={IEEE Transactions on Automation Science and Engineering},
year={2021},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85102620971&doi=10.1109%2fTASE.2021.3061870&partnerID=40&md5=3ec47ec5691508387f8a92f51961c99b},
abstract={The studies of Unmanned Air/Ground Vehicle (UAV/UGV) cooperative detection systems have received much attention due to their wide applications in the disaster rescue, target tracking, intelligent surveillance, and automatical package delivery missions. UAVs provide a broad view and have a fast speed in the air, while UGVs have sufficient load capacity and can serve as repeater stations on the ground. The path planning of a UAV/UGV cooperative system is an important but difficult issue, which aims to plan paths for both the UAVs and the UGVs in the system to cooperatively complete a mission. In this article, we consider the path planning problem of the UAV/UGV cooperative system for illegal urban building detection, by taking the limits of UGV speed, UAV load power, and UAV/UGV communication restriction into consideration. To solve this problem, we first model the path planning problem as a constraint optimization problem which tries to minimize an overall execution time for completing the illegal urban building detection tasks, and then propose a two-level memetic algorithm (called Two-MA) to solve the path planning problems of both the UAV and the UGV. Experiments on both synthetic and real-world data sets show the superiority of the proposed Two-MA over several states-of-the-art algorithms in solving the path planning problems of the UAV and UGV for illegal urban building detection tasks. IEEE},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Ma202025,
author={Ma, L. and Huang, X. and Chen, J. and Li, J. and Sun, T.},
title={A Two-level Memetic Path Planning Algorithm for Unmanned Air/Ground Vehicle Cooperative Detection Systems},
journal={ICARM 2020 - 2020 5th IEEE International Conference on Advanced Robotics and Mechatronics},
year={2020},
pages={25-30},
art_number={9195287},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85092670599&doi=10.1109%2fICARM49381.2020.9195287&partnerID=40&md5=ed142f46626f5853b80dda5421d47ee5},
abstract={The Unmanned Air/Ground Vehicle (UAV/UGV) cooperative detection systems are widely used in terrain reconnaissance, disaster rescue and urban/rural buildings survey, in which the UAV in the air can provide a broad view and take photography, while the UGV on the ground can offer sufficient load capacity and serve as repeater stations as well. The path planning of UAV/UGV is one of the most important issues in the cooperative detection system, and its studies have attracted great attentions in recent years. In this study, a two-level memetic path planning algorithm is proposed to help the unmanned air/ground vehicle cooperative systems detect realistic urban illegal building, considering the limits of the endurance capacity of the UAV, the load capacity of the UGV, and the communication restrictions between them. Experiments on both the synthetic data and the realistic urban illegal building data show the effectiveness of the proposed algorithm on solving the path planning problem in the UAV/UGV cooperative system for urban illegal building detection tasks. © 2020 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Boyuk2020,
author={Boyuk, M. and Duvar, R. and Urhan, O.},
title={Deep Learning Based Vehicle Detection with Images Taken from Unmanned Air Vehicle [Insansiz Hava Aracindan Alinan Görüntüler ile Derin Öǧrenme Tabanli Araç Tespiti]},
journal={Proceedings - 2020 Innovations in Intelligent Systems and Applications Conference, ASYU 2020},
year={2020},
art_number={9259868},
note={cited By 3},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85097939871&doi=10.1109%2fASYU50717.2020.9259868&partnerID=40&md5=c3a437812ceb240c90284682a4027ac1},
abstract={Especially in recent years, unmanned aerial vehicles (UAV) have been used in many platforms for military, commercial and entertainment purposes. Thanks to high computational graphics cards, many computer vision applications based on deep learning can work in real time on unmanned aerial vehicles. In this study, fast and high-performance object detection algorithms Faster R-CNN, YOLOv3-Tiny and SSD algorithms are used to detect vehicles in image taken from UAVs. Thus, the positions of vehicles driving in traffic are found automatically. © 2020 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Karakiş2020151,
author={Karakiş, S. and Sefercik, U.G. and Bilir, T. and Atalay, C.},
title={Precise monitoring of temporal topographic change detection via unmanned air vehicle},
journal={Bulletin of the Mineral Research and Exploration},
year={2020},
volume={161},
pages={151-156},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85098503622&doi=10.19111%2fbulletinofmre.524179&partnerID=40&md5=7d66e88d8968367f6839f424374f5d82},
abstract={Nowadays, fast developing space-borne and airborne remote sensing technologies became indispensable for land related engineering disciplines such as mapping, geology, environment, mining and forestry. The new technologies, provide more qualified and rapid achievable outcomes, are adopted permanently. The description of the topographic surface became easier by means of very high resolution (VHR), rapid achievable and accurate point clouds acquired by digital photogrammetry and airborne laser scanning (ALS). Optical unmanned air vehicle (UAV), one of the most actual photogrammetric techniques, is much in demand for varied purposes. UAVs provide high resolution data using the advantage of lower flight altitudes. In this study, a construction activity and its environmental influences in Bulent Ecevit University Central Campus were monitored by an optical hand-made UAV. In the application, the temporal change was detected by generating contour-lines, digital terrain models (DTMs) and differential DTMs (DiffDTM) of the topography. By DiffDTMs, temporal changes on the topography were visualized in color height scale where the contour-lines presents the change of morphological structure. © 2020 General Directorate of Mineral Research and Exploration (MTA). All rights reserved.},
publisher={General Directorate of Mineral Research and Exploration (MTA)},
}

@CONFERENCE{Kartashov2019,
author={Kartashov, V. and Oleynikov, V. and Zubkov, O. and Sheiko, S.},
title={Optical detection of unmanned air vehicles on a video stream in a real-time},
journal={2019 International Conference on Information and Telecommunication Technologies and Radio Electronics, UkrMiCo 2019 - Proceedings},
year={2019},
art_number={9165362},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85091703254&doi=10.1109%2fUkrMiCo47782.2019.9165362&partnerID=40&md5=88aad692c12ea5d33a8e8d47dd9a1fd0},
abstract={The paper describes the research connected with motion detection of small unmanned air vehicles on a video stream. The most comprehensive detection methods are analyzed and investigated with a real video shooting. The research shows that the differential method is more reliable in the authenticity of motion detection and may be considered as a base for practical systems. © 2019 IEEE},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Kurdi2019194,
author={Kurdi, M.M. and Dadykin, A.K. and Elzein, I.A. and Ibrahim, A.K.},
title={Cooperative unmanned air and ground vehicles for landmine detection},
journal={International Journal of Electrical and Electronic Engineering and Telecommunications},
year={2019},
volume={8},
number={4},
pages={194-198},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85069182823&doi=10.18178%2fijeetc.8.4.194-198&partnerID=40&md5=c1318f1bd350d8e066c7f149c0c574f3},
abstract={The unmanned aerial vehicle used in this research is multi-functional quadcopter with infrared camera and Ground Penetrating Radar (GPR). The unmanned aerial vehicle detects the landmines using infrared camera and GPR; maps a pin in digital map for future use by ground vehicle. The ground vehicle used in this research is Belarus132N mobile robot. It has the following onboard sensors: stereo pair camera, GPS, and image processing system. The ground vehicle will use onboard sensors: stereo pair camera, GPS and the map provided by the quadcopter to traverse the region, and locate the mapped landmines. The base station consists of a laptop that provides a communication link between the aerial and ground vehicle systems and for saving information from any destruction. This proposed system will demonstrate how an air-ground vehicle system use to cooperatively detect, locate and traverse of landmines. © 2019 Int. J. Elec. & Elecn. Eng. & Telcomm.},
publisher={Warsaw University of Technology},
}

@ARTICLE{Zilun20193223,
author={Zilun, H. and Jianying, Y.},
title={Distributed efficiency-based circular formation for the unmanned air vehicles detection system},
journal={Proceedings of the Institution of Mechanical Engineers, Part G: Journal of Aerospace Engineering},
year={2019},
volume={233},
number={9},
pages={3223-3234},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85052562629&doi=10.1177%2f0954410018793764&partnerID=40&md5=758af5d7f124932e82b73b17a07522f8},
abstract={This paper considers on the general circumnavigation problem for a team of vertical takeoff and landing unmanned air vehicles, with the goal of achieving specific circular formations and circling centered at a target of interest. Different from the traditional circular formation problem, in this paper, not only the formation but also the detection efficiency of the formation is taken into consideration. A novel distributed optimal circular formation algorithm is proposed. According to this algorithm, the circular formation can be guaranteed with the optimal radius that can optimize the team performance function. Hereon, the performance functions can be time-varying, and thus a time-varying optimal circular formation is created. Theoretical studies indicate that the proposed algorithm can achieve the formation in a distributed manner only based on the local information and the network connection. Finally, simulation examples are presented to show the validity of the theoretical results. © IMechE 2018.},
publisher={SAGE Publications Ltd},
}

@CONFERENCE{Yu20189635,
author={Yu, Q. and Yao, H. and He, F. and Qi, H.},
title={U-Net Based Moving Target Detection for Unmanned Air Vehicles},
journal={Chinese Control Conference, CCC},
year={2018},
volume={2018-July},
pages={9635-9640},
art_number={8483331},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85056106998&doi=10.23919%2fChiCC.2018.8483331&partnerID=40&md5=728fa39051b8dd57f7538e13f1e40164},
abstract={In this paper, a moving target detection problem is investigated for the unmanned air vehicles with a monocular vision sensor. First, a detection algorithm based on U-Net network is proposed to obtain the position and velocity direction of a moving target. Then, a Kalman Filter is incorporated into the proposed algorithm to increase the accuracy of states acquisition of the moving targets. Then, the experimental results show the proposed algorithm has low computation and better performance. © 2018 Technical Committee on Control Theory, Chinese Association of Automation.},
publisher={IEEE Computer Society},
}

@CONFERENCE{Seiferth2018196,
author={Seiferth, D. and Heller, M. and Holzapfel, F.},
title={Automatic safe area detection for novel unmanned air vehicle},
journal={Proceedings - 2018 4th International Conference on Control, Automation and Robotics, ICCAR 2018},
year={2018},
pages={196-201},
art_number={8384669},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85049899395&doi=10.1109%2fICCAR.2018.8384669&partnerID=40&md5=04f2fb95b0f3efe7ab1178491fc4f5a3},
abstract={For experimental and commercial applications of Unmanned Air Vehicles within the middle and heavy weight category, a high level of safety during flights beyond visual line of sight needs to be ensured. Therefore, it is only allowed to operate the aircraft within a certain flight zone, which is defined prior to its flights. If the aircraft leaves the predefined flight area, the responsible operator would be forced to activate the aircraft's termination system, in order to avoid the aircraft from violating the flight zone in any case. This paper focuses on the development and implementation of a safe area detection algorithm for Unmanned Air Vehicles to prevent automatically the aircraft's leaving from its predefined flight zone without action of the operator on ground. It presents a mathematical approach to determine, if the aircraft stays within a certain area and underlines its functionality by appropriate model-in-the-loop simulations of a novel reference Unmanned Air Vehicle configuration. Additionally, a pre-flight verification algorithm of the flight zone is presented. Thereby, prior to flight, the flight zone specification is checked, to ensure a proper flight zone definition and to guarantee the functionality of the safe area detection algorithm. The presented approach can be generalized and applied to any other Unmanned Air Vehicles. © 2018 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Phelps2018,
author={Phelps, D. and Gamagedara, K. and Waldron, J. and Patil, K. and Snyder, M.},
title={Ship air wake detection using a small fixed wing unmanned aerial vehicle},
journal={AIAA Aerospace Sciences Meeting, 2018},
year={2018},
number={210059},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85044408657&doi=10.2514%2f6.2018-0784&partnerID=40&md5=8961debf8cbd6788eeb6f86e265c1ee3},
abstract={A ship’s air wake is dynamically detected using an airborne inertial measurement unit and global positioning system attached to a fixed wing unmanned aerial system. The instrumented aircraft is used for validation of computational fluid dynamic simulations of naval ship air wakes. A simulation was completed using Gridtool, VGrid, and Kestral to validate the experimental data collection method. Forces from the experiment were collected and compared with that of a one-way coupled CFD simulation mimicking the physical experiment. Similar trends in forces that indicate detection of the ship air wake were observed in both experimental and simulation data. © 2018, American Institute of Aeronautics and Astronautics Inc, AIAA. All rights reserved.},
publisher={American Institute of Aeronautics and Astronautics Inc, AIAA},
}

@CONFERENCE{Yao201711459,
author={Yao, H. and Yu, Q. and Xing, X. and He, F. and Ma, J.},
title={Deep-learning-based moving target detection for unmanned air vehicles},
journal={Chinese Control Conference, CCC},
year={2017},
pages={11459-11463},
art_number={8029186},
note={cited By 7},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85032226732&doi=10.23919%2fChiCC.2017.8029186&partnerID=40&md5=bf5444545afd0c019aba71ec5c4896a4},
abstract={In this paper, a deep learning network is investigated to detect moving targets for a UAV equipped with monocular camera. An algorithm based on fully convolutional network is proposed to obtain the position and moving direction of targets. A Kalman filter is incorporated into the proposed algorithm to increase the accuracy of target position information acquisition. The experimental results show the effectiveness of the proposed algorithm with a relatively low hardware resource consumption. © 2017 Technical Committee on Control Theory, CAA.},
publisher={IEEE Computer Society},
}

@ARTICLE{Mitchell2014593,
author={Mitchell, R. and Chen, I.-R.},
title={Adaptive intrusion detection of malicious unmanned air vehicles using behavior rule specifications},
journal={IEEE Transactions on Systems, Man, and Cybernetics: Systems},
year={2014},
volume={44},
number={5},
pages={593-604},
art_number={6573382},
note={cited By 120},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84899500829&doi=10.1109%2fTSMC.2013.2265083&partnerID=40&md5=d4d0fdf361ea95e3e451b555b6a8e521},
abstract={In this paper, we propose an adaptive specification-based intrusion detection system (IDS) for detecting malicious unmanned air vehicles (UAVs) in an airborne system in which continuity of operation is of the utmost importance. An IDS audits UAVs in a distributed system to determine if the UAVs are functioning normally or are operating under malicious attacks. We investigate the impact of reckless, random, and opportunistic attacker behaviors (modes which many historical cyber attacks have used) on the effectiveness of our behavior rule-based UAV IDS (BRUIDS) which bases its audit on behavior rules to quickly assess the survivability of the UAV facing malicious attacks. Through a comparative analysis with the multiagent system/ant-colony clustering model, we demonstrate a high detection accuracy of BRUIDS for compliant performance. By adjusting the detection strength, BRUIDS can effectively trade higher false positives for lower false negatives to cope with more sophisticated random and opportunistic attackers to support ultrasafe and secure UAV applications. © 2013 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@CONFERENCE{Mohammad2013,
author={Mohammad, A.},
title={Efficient video object detection for optimizing unmanned air vehicle communications},
journal={AIAA Infotech at Aerospace (I at A) Conference},
year={2013},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84883713734&partnerID=40&md5=02ab6f32cca1fdd0b96c324e4383218d},
abstract={Unmanned Air Vehicles (UAVs) used in aerial surveillance are equipped with video devices to capture real-time video and transmit it to a ground station. However, the link bandwidth available to UAVs is generally limited, and includes VHF links, satellite links, directional links, and various other forms of air-to-ground radio frequency links. Also, during the course of a mission/flight, the bandwidth available for communication between the UAV and ground crew can vary significantly and unpredictably due to the wireless nature of the links. The ground crew controlling/monitoring the UAV may be hundreds or thousands of miles away, and have to rely on the video data feed to make decisions throughout the mission. It would greatly improve the mission efficiency if only important data is streamed to the ground station and just in time information/guidance about the object detected is readily made available to the ground personnel. In this paper, we will describe the use of efficient real-time object detection methods within captured video frames to trigger video streaming to the ground station. There are two advantages to this approach. The first is that only video scenes of interest are transmitted to the ground station, and the second is relevant just in time information of the objects detected can be presented to the ground station personnel via object matching techniques and linking to a relevant knowledge database. There are several algorithms proposed in the literature for object detection in video frames. The focus of this paper is on meeting processing constraints onboard UAVs, making efficient use of the available bandwidth form air to ground, providing important just in time information relevant to the objects detected, while meeting real-time end to end delay constraints. The full paper will provide a comprehensive analysis of existing approaches, classify these approaches, and discuss approaches relevant to the UAV environment.},
}

@ARTICLE{Samy20121,
author={Samy, I. and Gu, D.-W.},
title={Fault detection and flight data measurement: Demonstrated on unmanned air vehicles using neural networks},
journal={Lecture Notes in Control and Information Sciences},
year={2012},
volume={419},
pages={1-165},
note={cited By 2},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-82155191754&doi=10.1007%2f978-3-642-24052-2_1&partnerID=40&md5=eccc057168a1ddb6f35aa08b5a3121a7},
}

@CONFERENCE{Samy2010913,
author={Samy, I. and Postlethwaite, I. and Gu, D.-W. and Fan, I.S.},
title={Detection of multiple sensor faults using neural networks-demonstrated on a unmanned air vehicle (UAV) model},
journal={IET Seminar Digest},
year={2010},
volume={2010},
number={4},
pages={913-919},
art_number={0403},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84877827915&doi=10.1049%2fic.2010.0403&partnerID=40&md5=382f2b79f79aa061a730c1ef0639cf68},
abstract={Model-based sensor fault detection, isolation and accommodation (SFDIA) is a direction of development in particular with small UAVs where sensor redundancy may not be an option due to weight, cost and space implications. SFDIA via neural networks (NNs) have been proposed over the years due to their nonlinear structures and online learning capabilities. However few applications have considered multiple sensor faults in fixed-wing UAVs where full autonomy is most needed. In this paper an Extended Minimum Resource Allocating Network (EMRAN) Radial Basis Function (RBF) NN is chosen for modelling purposes due to its ability to adapt well to nonlinear environments while maintaining high computational speeds. After 30 separate SFDIA tests implemented on a 1.6 GHz Pentium processor, the NN-SFDIA scheme detected all but 2 faults and the NN processing time was 97% lower than the flight data sampling time.},
}

@ARTICLE{Samy2010437,
author={Samy, I. and Postlethwaite, I. and Gu, D.-W.},
title={Sensor fault detection and accommodation using neural networks with application to a non-linear unmanned air vehicle model},
journal={Proceedings of the Institution of Mechanical Engineers, Part G: Journal of Aerospace Engineering},
year={2010},
volume={224},
number={4},
pages={437-447},
note={cited By 19},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-77950612949&doi=10.1243%2f09544100JAERO579&partnerID=40&md5=a0cb7c3e0b723932a79a24cedd1ac01d},
abstract={Model-based fault detection and isolation (FDI) systems have become a crucial step towards autonomy in aerospace engineering. Traditional methods such as observer-based methods have already been developed and widely applied. Novel approaches make use of online learning neural networks (NN) which have seen an increase in FDI applications over the years. However, few publications consider FDI applications to unmanned air vehicles (UAV) where high levels of autonomy are required. This article demonstrates such an application, where an extended minimum resource allocation network radial basis function (RBF) NN is used for modelling purposes. A novel residual generation approach is also presented and found to outperform a conventional approach by reducing the number of false alarms and missed faults. All tests are carried out in simulation where single sensor faults are assumed to occur in the pitch gyro of a non-linear UAV model.},
}

@CONFERENCE{King2009694,
author={King, S. and Ramos-Hernandez, D. and Moran, J. and Sundaram, S.},
title={Anomaly detection of combustor systems in support of unmanned air vehicle applications},
journal={6th International Conference on Condition Monitoring and Machinery Failure Prevention Technologies 2009},
year={2009},
volume={2},
pages={694-705},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84905678568&partnerID=40&md5=4139cfe09482d46ed809ea2b64a089fa},
abstract={The use of Unmanned Air Vehicles (UAVs) is a growing technology area and has prompted consideration of how such technology can be certified to operate in civil airspace. The DTI funded ASTRAEA I project, completed December 2008, aimed to address a range of certification and standards issues covering compliance of UAV systems for aircraft type certification/airworthiness, procedures for operation of UAVs in UK airspace, and integration of UAVs into existing/emerging traffic management infrastructure. In addition, the project considered aspects of data communications, UAV flight control, adaptive routing, collision avoidance, multi-air vehicle integration, onboard decision-making and finally prognostics and health management. The focus of this paper is with the latter work package, which aims to provide technology and systems that can enable UAVs to monitor their own operational state and perform real-time prognosis of their current and future capabilities. More specifically, our interest is in early detection of combustor anomalies in the propulsion system which could have adverse effects on the UAVs thrust capability and hence its ability to maintain its intended mission profile.},
publisher={British Institute of Non-Destructive Testing},
}

@CONFERENCE{Byrne20062830,
author={Byrne, J. and Cosgrove, M. and Mehra, R.},
title={Stereo based obstacle detection for an unmanned air vehicle},
journal={Proceedings - IEEE International Conference on Robotics and Automation},
year={2006},
volume={2006},
pages={2830-2835},
art_number={1642130},
note={cited By 47},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-33845679986&doi=10.1109%2fROBOT.2006.1642130&partnerID=40&md5=b4663b72454c93f622f9258eb740b4b8},
abstract={This paper presents the Visual Threat Awareness (VISTA) system for real time collision obstacle detection for an unmanned air vehicle (UAV). Computational stereo performance has progressed such that several commercial or open source implementations are available which operate at frame rate, but suffer from well known correspondence errors. We show that introducing a global segmentation step after commodity stereo can increase robustness and leverage existing stereo software. The global segmentation step is based on a graph structure appropriate for collision detection, human vision inspired foveation, perceptual organization and graph partitioning using the minimum s-t graph cut. This system has been prototyped using the Sarnoff Acadia I vision processor to enable processing of 640×480 resolution imagery at 5-10Hz operation on embedded avionics. We describe system theory, demonstrate segmentation results on scenes of increasing complexity, and show flight experiment results on Georgia Tech's GT-Max autonomous helicopter against real collision obstacles. © 2006 IEEE.},
}

@CONFERENCE{MacArthur2005,
author={MacArthur, E.Z. and MacArthur, D. and Crane, C.},
title={Use of cooperative unmanned air and ground vehicles for detection and disposal of mines},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2005},
volume={5999},
art_number={599909},
note={cited By 28},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-33644626763&doi=10.1117%2f12.631314&partnerID=40&md5=088d01e9c9669a8d9286d39a169ab34f},
abstract={The objective of this research is to extend the sensing capabilities of a multi-vehicle ground system by incorporating the environmental perception abilities of unmanned aerial vehicles. The aerial vehicle used in this research is a Miniature Aircraft Gas Xcell RC helicopter. It is outfitted with a sensor payload containing stereo vision cameras, GPS, and a digital compass. Geo-referenced images are gathered using the above sensors that are used in this research to create a map of the operating region. The ground vehicle used in this research is an automated Suzuki Mini-Quad ATV. It has the following onboard sensors: single-vision camera, laser range device, digital compass, GPS, and an encoder. The ground vehicle uses the above sensors and the map provided by the helicopter to traverse the region, locate, and isolate simulated land mines. The base station consists of a laptop that provides a communication link between the aerial and ground vehicle systems. It also provides the operator with system operation information and statistics. All communication between the vehicles and the base station is performed using JAUS (Joint Architecture for Unmanned Systems) messages. The JAUS architecture is employed as a means to organize inter-vehicle and intravehicle communication and system component hierarchy. The purpose of JAUS is to provide interoperability between various unmanned systems and subsystems for both military and commercial applications. JAUS seeks to achieve this through the development of functionally cohesive building blocks called components whose interface messages are clearly defined. The JAUS architecture allows for a layered control strategy which has specific message sets for each layer of control. Implementation of the JAUS architecture allows for ease of software development for a multi-vehicle system. This experiment demonstrates how an air-ground vehicle system can be used to cooperatively locate and dispose of simulated mines.},
}

@CONFERENCE{Kovacina20022782,
author={Kovacina, M.A. and Palmer, D. and Yang, G. and Vaidyanathan, R.},
title={Multi-agent control algorithms for chemical cloud detection and mapping using unmanned air vehicles},
journal={IEEE International Conference on Intelligent Robots and Systems},
year={2002},
volume={3},
pages={2782-2788},
note={cited By 67},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-0036453716&partnerID=40&md5=b6bc22f8567f497fc7436b396edf16b6},
abstract={Traditional control approaches fall well short of the necessary flexibility and efficiency needed to meet the commercial and military demands placed upon UAV swarms. Effective coordination of these swarms requires development of control strategies based on emergent behavior. We have developed a rule-based, decentralized control algorithm that relies on constrained randomized behavior and respects UAV restrictions on sensors, computation, and flight envelope. To demonstrate and evaluate the effectiveness of our approach, we have created a simulation of an air vehicle swarm searching for and mapping a chemical cloud within a patrolled region. We then consider several different detection and mapping strategies based on emergent behavior. We then establish an inverse linear relation between the size of the swarm and the time to detect the cloud, regardless of the size of the cloud. Further, we also show the size of the swarm has a linear relation with the successful detection of the cloud.},
}


==> UAVtracking.tex <==
Scopus
EXPORT DATE: 7 February 2022

@CONFERENCE{Shen20174153,
author={Shen, H. and Li, N. and Griffiths, H. and Rojas, S.},
title={Tracking control of a small unmanned air vehicle with airflow awareness},
journal={Proceedings of the American Control Conference},
year={2017},
pages={4153-4158},
art_number={7963593},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85027006044&doi=10.23919%2fACC.2017.7963593&partnerID=40&md5=27323d27317f14561c62c511be61f805},
abstract={Flying animals are so well adapted to their complex natural environment, that their aerial locomotive flight mechanisms attract much attention in the context of designing high performance flying robots. Inspired from the sensing and flight control strategies of birds and bats, a bioinspired robust tracking control method for small unmanned air vehicles using in-situ measured airflow information, is proposed. First, the relationship between the airflow measurment and aerodynamic forces is presented. Then, an aerodynamic model is derived, with the aerodynamic forces calculated from the flow measurment. To cope with the un-modeled dynamics, wind gust disturbances, and measurement noise, a robust sliding mode tracking controller is derived using the backstepping framework. Finally, a simulation system is created to test the effectiveness of the proposed tracking control method. The results demonstrate that the proposed tracking control system provides an enhanced tracking performance. © 2017 American Automatic Control Council (AACC).},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Sakamaki2017249,
author={Sakamaki, J.Y. and Beard, R.W. and Rice, M.},
title={Tracking multiple ground objects using a team of unmanned air vehicles},
journal={Lecture Notes in Control and Information Sciences},
year={2017},
volume={474},
pages={249-268},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85020377265&doi=10.1007%2f978-3-319-55372-6_12&partnerID=40&md5=91e65e76a5d18817c74f856f6dc9d1c3},
abstract={This paper proposes a system architecture for tracking multiple ground-based objects using a team of unmanned air systems (UAS). In the architecture pipeline, video data is processed by each UAS to detect motion in the image frame. The ground-based location of the detected motion is estimated using a geolocation algorithm. The subsequent data points are then process by the recently introduced Recursive RANSAC (R-RANSASC) algorithm to produce a set of tracks. These tracks are then communicated over the network and the error in the coordinate frames between vehicles must be estimated. After the tracks have been placed in the same coordinate frame, a track-to-track association algorithm is used to determine which tracks in each camera correspond to tracks in other cameras. Associated tracks are then fused using a distributed information filter. The proposed method is demonstrated on data collected from two multi-rotors tracking a person walking on the ground. © Springer International Publishing AG 2017.},
publisher={Springer Verlag},
}

@CONFERENCE{Tavakoli2016,
author={Tavakoli, S. and Heaton, A. and Ansell, D. and Poslad, S.},
title={Wildlife tracking on the wing using Unmanned Air Vehicles},
journal={AIAA Infotech @ Aerospace Conference},
year={2016},
page_count={7},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84968542458&partnerID=40&md5=9243c5baaf8c2b77964b0597b98e193e},
abstract={The miniaturisation and increasing accessibility of tracking technology is transforming the fields of animal behaviour and ecology. Studies involving animal movement are shifting from sparse observational data to high-throughput, dynamic, precision time series for individual animals and groups. However, a combination of high cost, high mass, and inflexibility currently limits deployments of state of the art devices such as Unmanned Air Vehicles (UAVs) to track more species or at greater scales. The recent uptake of low-cost logging devices has demonstrated the appeal of low-cost approaches, but these devices are necessarily limited by the need for field recovery. Here, we describe the concepts of a novel, low-cost, and wirelessly enabled UAV tracking platform that allows researchers the flexibility and power to tackle a variety of novel research questions. The novel application of the system is the following; 1) To track multiple individual animals within a free-moving group simultaneously, 2) To allow freedom from data retrieval efforts by collection of the wildlife movement data on-the-fly, 3) To allow tracking of hard-to-detect individuals by data sharing and collection from highly mobile, easily accessible endangered species. © 2016, American Institute of Aeronautics and Astronautics Inc, AIAA. All rights reserved.},
publisher={American Institute of Aeronautics and Astronautics Inc, AIAA},
}

@ARTICLE{Yu2015541,
author={Yu, H. and Meier, K. and Argyle, M. and Beard, R.W.},
title={Cooperative path planning for target tracking in urban environments using unmanned air and ground vehicles},
journal={IEEE/ASME Transactions on Mechatronics},
year={2015},
volume={20},
number={2},
pages={541-552},
art_number={6732930},
note={cited By 121},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84908399248&doi=10.1109%2fTMECH.2014.2301459&partnerID=40&md5=88bf4791fadfc36720d8ca4e87037789},
abstract={As the need for autonomous reconnaissance and surveillance missions in cluttered urban environments has been increasing, this paper describes a cooperative path planning algorithm for tracking a moving target in urban environments using both unmanned air vehicles (UAVs) and unmanned ground vehicles (UGVs). The novelty of the algorithm is that it takes into account vision occlusions due to obstacles in the environment. The algorithm uses a dynamic occupancy grid to model the target state, which is updated by sensor measurements using a Bayesian filter. Based on the current and predicted target behavior, the path planning algorithm for a single vehicle (UAV/UGV) is first designed to maximize the sum of the probability of detection over a finite look-ahead horizon. The algorithm is then extended to multiple vehicle collaboration scenarios, where a decentralized planning algorithm relying on an auction scheme is designed to plan finite look-ahead paths that maximize the sum of the joint probability of detection over all vehicles. © 2014 IEEE.},
publisher={Institute of Electrical and Electronics Engineers Inc.},
}

@ARTICLE{Su2015121,
author={Su, C. and Ma, Y. and Wang, Y. and Fang, Y. and Wang, D.},
title={Low speed stability of tracking turntable for the unmanned air vehicle landing},
journal={Lecture Notes in Electrical Engineering},
year={2015},
volume={334},
pages={121-129},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84938703843&doi=10.1007%2f978-3-319-13707-0_14&partnerID=40&md5=ff3fb00711ba239e908144f59b941631},
abstract={In the unmanned air vehicle (UAV) landing test, the rate fluctuation of tracking turntable appears in using the grounding active laser guidance system. To improve its stability, the reasons for tracking turntable rate fluctuation at low speed are analyzed. It is verified that the motor cogging torque fluctuation is the main reason at low speed by modeling and experiment. A disturbance observer based compensation control on the basis of the traditional double closed loop PID correction is proposed. Through analyzing the dynamic structure of tracking turntable, the compensation equation of disturbance torque described by the angular acceleration and torque current is derivated and then the torque disturbance observer structure is designed based on the equation. The comparative test shows that the rate fluctuation is 2.12 % after compensation when the speed is 1(°)/s, lower over 3 times than by only the traditional double closed loop PID correction. This method proposed can improve low speed stability of tracking Turntable for the UAV landing. © Springer International Publishing Switzerland 2015.},
publisher={Springer Verlag},
}

@CONFERENCE{Cook20131,
author={Cook, K. and Bryan, E. and Yu, H. and Bai, H. and Seppi, K. and Beard, R.},
title={Intelligent cooperative control for urban tracking with Unmanned Air Vehicles},
journal={2013 International Conference on Unmanned Aircraft Systems, ICUAS 2013 - Conference Proceedings},
year={2013},
pages={1-6},
art_number={6564667},
note={cited By 10},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84883088171&doi=10.1109%2fICUAS.2013.6564667&partnerID=40&md5=025a6f278c3f35ff680fe076903e9a78},
abstract={We introduce an intelligent cooperative control system for ground target tracking in a cluttered urban environment with a team of Unmanned Air Vehicles (UAVs). We extend the work of Yu et. al. [1] to add a machine learning component that uses observations of target position to learn a model of target motion. Our learner is the Sequence Memoizer [2], a Bayesian model for discrete sequence data, which we use to predict future target location identifiers, given a context of previous location identifiers. Simulated cooperative control of a team of 3 UAVs in a 100-block city filled with various sizes of buildings verifies that learning a model of target motion can improve target tracking performance. © 2013 IEEE.},
}

@ARTICLE{Bradley2011295,
author={Bradley, J.M. and Taylor, C.N.},
title={Georeferenced mosaics for tracking fires using unmanned miniature air vehicles},
journal={Journal of Aerospace Computing, Information and Communication},
year={2011},
volume={8},
number={10},
pages={295-309},
note={cited By 12},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-80055018427&doi=10.2514%2f1.45342&partnerID=40&md5=5b6f6073e43a3f05dbc80a9510cc3f78},
abstract={Fire tracking is an increasingly important area of research aiming to help firefighters more effectively fight fires. In the past, piloted aircraft have been the main source for obtaining fire characteristics from the air. In recent years unmanned air vehicles (UAVs) have become popular for the same purpose. While large UAVs are an effective means of assisting firefighters, they are expensive to purchase and operate. Mini UAVs or MAVs, on the other hand, have become cheap and reliable platforms for surveillance missions. However, due to weight and size constraints, MAVs are often equipped with error-prone sensors, in contrast to large UAVs, resultinginpoor-quality georeferencing and geolocating.Techniquestosolve this problem in the fire tracking context have focused on fusing information from on-board infrared and color cameras and using various filters to correct single geolocation estimates. However, a fire can be very large and arbitrarily shaped, thereby invalidating the single geolocation point assumption. We aim to solve this problem by producing a Georeferenced Uncertainty Mosaic (GUM) in which size, shape, and geolocation information is shown simultaneously in an easy to understand georeferenced image. The GUM is created by appropriately blurring the infrared images captured by the on-board camera, and using the blurred images as observations in a particle filter. Copyright © 2011 by the American Institute of Aeronautics and Astronautics, Inc.},
}

@ARTICLE{Natesan2010395,
author={Natesan, K. and Gu, D.-W. and Postlethwaite, I.},
title={Design of linear parameter varying trajectory tracking controllers for an unmanned air vehicle},
journal={Proceedings of the Institution of Mechanical Engineers, Part G: Journal of Aerospace Engineering},
year={2010},
volume={224},
number={4},
pages={395-402},
note={cited By 7},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-77950606002&doi=10.1243%2f09544100JAERO586&partnerID=40&md5=71bebb9c3896774cf9454a7cc486c821},
abstract={This article presents a trajectory tracking controller design approach for an unmanned air vehicle using the linear parameter varying (LPV) methods. The longitudinal and lateral controllers are designed using an inner-outer loop structure with the inner loop LPV controller designed first using μ-synthesis. The inner loop is then approximated with a reference model and the outer loop is designed using loop-shaping techniques. Flight trajectory is expressed in terms of earth co-ordinates, which the outer loop controller converts into reference signals for the inner loop. Full-scale non-linear simulations are used to test the efficiency of the designed controller and of the proposed design approach.},
}

@CONFERENCE{Bencatel2009189,
author={Bencatel, R. and Correia, J. and Sousa, J.B. and Gonçalves, G.M. and Pereira, E.},
title={Video tracking control algorithms for unmanned air vehicles},
journal={2008 Proceedings of the ASME Dynamic Systems and Control Conference, DSCC 2008},
year={2009},
number={PART A},
pages={189-196},
note={cited By 7},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-70349895751&partnerID=40&md5=346bfe4e9eab27544ec53319f01f86ba},
abstract={We present and discuss a modular flight control system suitable for video tracking natural structures with Unmanned Air Vehicles (UAVs), like rivers, roads or canals. The control system is modeled in the framework of hybrid automata, where each state corresponds to different control algorithms. We implemented four nonlinear turn-rate control algorithms and compared them in a simulation environment to assess tracking performance. Copyright © 2008 by ASME.},
}

@ARTICLE{Xin2009398,
author={Xin, Z. and Fang, Y.},
title={Modeling and control for tracking ground target using an unmanned air vehicle},
journal={Gaojishu Tongxin/Chinese High Technology Letters},
year={2009},
volume={19},
number={4},
pages={398-403},
note={cited By 9},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-65549094473&partnerID=40&md5=f7ad532aac826b1a4af94e2904fe822b},
abstract={The paper analyses the dynamic target tracking problem of an unmanned air vehicle (UAV) equipped with visual sensors, and sets up the models for each component of the tracking system. Specifically, for the two kernel technologies avoiding target lost, that is, UAV flight control and camera orientation regulation, the paper proposes a path planning and tracking algorithm for the UAV, which can keep a certain distance between the UAV and the target, and ensure the orientation of UAV facing the target at the same time. Besides, a pan-tilt control technique for the camera orientation is constructed by combining the UAV states and image error as feedback. The simulation results show that the overall target tracking system demonstrates the performance.},
}

@CONFERENCE{Natesan2008,
author={Natesan, K. and Gu, D. and Postlethwaite, I.},
title={Trajectory tracking controller design for an unmanned air vehicle},
journal={IFAC Proceedings Volumes (IFAC-PapersOnline)},
year={2008},
volume={17},
number={1 PART 1},
note={cited By 0},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-79961018252&doi=10.3182%2f20080706-5-KR-1001.0846&partnerID=40&md5=12b12223c9ffa9e5726884dc271e5c70},
abstract={This paper presents a complete trajectory tracking controller design for an Unmanned Air Vehicle using Linear Parameter Varying design methods. The longitudinal and lateral controllers are designed using an inner loop - outer loop structure with the inner loop LPV controller designed using μ -synthesis. The inner-loop is then approximated with a reference model and the outer loop is designed using loop-shaping techniques. Full scale nonlinear simulations are used to test the efficiency of the designed controller and of the proposed design approach. Copyright © 2007 International Federation of Automatic Control All Rights Reserved.},
}

@CONFERENCE{Vasquez2008,
author={Vasquez, J.R. and Tarplee, K.M. and Case, E.E. and Zelnio, A.M. and Rigling, B.D.},
title={Multisensor 3D tracking for counter small unmanned air vehicles (CSUAV)},
journal={Proceedings of SPIE - The International Society for Optical Engineering},
year={2008},
volume={6971},
art_number={697107},
note={cited By 11},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-79959405651&doi=10.1117%2f12.785531&partnerID=40&md5=8ae9d421d65fafc0310fdbc92f42bbb3},
abstract={A variety of unmanned air vehicles (UAVs) have been developed for both military and civilian use. The typical large UAV is typically state owned, whereas small UAVs (SUAVs) may be in the form of remote controlled aircraft that are widely available. The potential threat of these SUAVs to both the military and civilian populace has led to research efforts to counter these assets via track, ID, and attack. Difficulties arise from the small size and low radar cross section when attempting to detect and track these targets with a single sensor such as radar or video cameras. In addition, clutter objects make accurate ID difficult without very high resolution data, leading to the use of an acoustic array to support this function. This paper presents a multi-sensor architecture that exploits sensor modes including EO/IR cameras, an acoustic array, and future inclusion of a radar. A sensor resource management concept is presented along with preliminary results from three of the sensors.},
}

@ARTICLE{Innocenti20081125,
author={Innocenti, M. and Pollini, L. and Turra, D.},
title={A fuzzy approach to the guidance of unmanned air vehicles tracking moving targets},
journal={IEEE Transactions on Control Systems Technology},
year={2008},
volume={16},
number={6},
pages={1125-1137},
note={cited By 27},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-55349147658&doi=10.1109%2fTCST.2008.917224&partnerID=40&md5=bf69fc2a58f4ac8a7e94fb38c3c33c52},
abstract={This paper presents the development of a fuzzy guidance system for unmanned aircraft based on waypoints described in a 5-D space: position in 3-dimensions, desired crossing heading, and speed. The aircraft is assumed to be auto piloted in speed, heading, and flight path angle. The proposed system uses standard Takagi-Sugeno fuzzy controllers that provide speed, heading, and flight path angle references for the autopilots. In particular, the heading guidance law results in a pipeline of two fuzzy controllers depending on the relative distance between aircraft and waypoint. A trajectory optimization algorithm is used to yield a long-distance guidance law blended with a short-distance guidance law as the waypoint approaches. The system handles sets of not directly flyable waypoints, driving the aircraft on flyable trajectories that try to cross the waypoints at a prescribed altitude and heading. © 2008 IEEE.},
}

@ARTICLE{Dobrokhodov2008907,
author={Dobrokhodov, V.N. and Kaminer, I.I. and Jones, K.D. and Ghabcheloo, R.},
title={Vision-based tracking and motion estimation for moving targets using unmanned air vehicles},
journal={Journal of Guidance, Control, and Dynamics},
year={2008},
volume={31},
number={4},
pages={907-917},
note={cited By 69},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-48849101997&doi=10.2514%2f1.33206&partnerID=40&md5=c2df7151d9fd348737847d59b0942dd4},
abstract={The algorithm performs autonomous tracking of a moving target, while simultaneously estimating geographic coordinates, speed, and heading of the target. Tight real-time integration of unmanned air vehicle's video and telemetry data streams with georeferenced database allows for reliable target identification, increased precision, and shortened time of target motion estimation. A low-cost off-the-shelf system is used, with a modified radiocontrolled aircraft airframe, gas engine, and servos. Tracking is enabled using a low-cost, miniature pan-tilt gimbal. The control algorithm provides rapid target acquisition and tracking capability. A target motion estimator was designed and shown in multiple flight tests to provide reasonable targeting accuracy. The impact of tracking loss events on the control and estimation algorithms is analyzed in detail.},
publisher={American Institute of Aeronautics and Astronautics Inc.},
}

@ARTICLE{Ren2007361,
author={Ren, W.},
title={Trajectory tracking control for a miniature fixed-wing unmanned air vehicle},
journal={International Journal of Systems Science},
year={2007},
volume={38},
number={4},
pages={361-368},
note={cited By 29},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-34250868955&doi=10.1080%2f00207720601170586&partnerID=40&md5=5cc7ca0ab80f7b502ed50344486b9e25},
abstract={This article considers the problem of trajectory tracking control for a miniature fixed-wing unmanned air vehicle (UAV). With the UAV equipped with longitudinal and lateral autopilots, we adopt a kinematic model that takes into account the fact that the heading of the UAV is controlled by its roll motion and the autopilot responses to air speed and roll control commands are first order in nature. Backstepping techniques are applied to derive air speed and roll control commands from known air speed and heading control laws that explicitly account for air speed and heading rate constraints of the UAV. Regarding inaccurately known autopilot constants, a parameter adaptation technique is used to estimate autopilot constants. High-fidelity simulation results on a six degree-of-freedom (DOF) 12-state fixed-wing UAV model are presented to show the effectiveness of our approach.},
}

@CONFERENCE{Call20063406,
author={Call, B. and Beard, R. and Taylor, C. and Barber, B.},
title={Obstacle avoidance for unmanned air vehicles using image feature tracking},
journal={Collection of Technical Papers - AIAA Guidance, Navigation, and Control Conference 2006},
year={2006},
volume={5},
pages={3406-3414},
note={cited By 41},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-33845762353&doi=10.2514%2f6.2006-6541&partnerID=40&md5=10e85cbb20ab2e7a62b895343f4bc779},
abstract={This paper discusses a computer vision algorithm and a control law for obstacle avoidance for small unmanned air vehicles using a video camera as the primary sensor. Small UAVs are used for low altitude surveillance nights where unknown obstacles can be encountered. Small UAVs can be given the capability to navigate in uncertain environments if obstacles are identified. This paper presents an obstacle detection methodology using feature tracking in a forward looking, onboard camera. Features are found using the Harris Corner Detector and tracked through multiple video frames which provides three dimensional localization of the salient features. A sparse three dimensional map of features provides a rough estimate of obstacle locations. The features are grouped into potentially problematic areas using agglomerative clustering. The small UAV then employs a sliding mode control law in the autopilot to avoid obstacles.},
publisher={American Institute of Aeronautics and Astronautics Inc.},
}

@CONFERENCE{Ren20044663,
author={Ren, W. and Beard, R.W.},
title={Constrained nonlinear tracking control for small fixed-wing unmanned air vehicles},
journal={Proceedings of the American Control Conference},
year={2004},
volume={5},
pages={4663-4668},
note={cited By 11},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-8744316867&doi=10.1109%2fACC.2004.182688&partnerID=40&md5=0a923b753db85121e882e2d4a39208dd},
abstract={This paper considers the problem of constrained nonlinear tracking control for small fixed-wing unmanned air vehicles equipped with longitudinal and lateral autopilots. Four different controllers based on SDRE, Sontag's formula, geometric mean, and aggressive selection from the feasible control set are proposed and compared to show their strengths and weaknesses under different application scenarios. Issues of measurement noise and input uncertainties are also addressed under the input-to-state stability framework. The effectiveness of the approaches is demonstrated through detailed simulation studies.},
}

@ARTICLE{Ren2004706,
author={Ren, W. and Beard, R.W.},
title={Trajectory tracking for unmanned air vehicles with velocity and heading rate constraints},
journal={IEEE Transactions on Control Systems Technology},
year={2004},
volume={12},
number={5},
pages={706-716},
note={cited By 216},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-4444342773&doi=10.1109%2fTCST.2004.826956&partnerID=40&md5=3ad97e2e57cbe262a4ded2877c2f5751},
abstract={This paper considers the problem of constrained nonlinear trajectory tracking control for unmanned air vehicles (UAVs). We assume that the UAV is equipped with longitudinal and lateral autopilots which reduces the 12-state model to a six-state model with altitude, heading, and velocity command inputs. One of the novel features of our approach is that we explicitly account for heading rate and velocity input constraints. For a UAV, the velocity is constrained to lie between two positive constants, and therefore presents particular challenges for the control design. We propose a control Lyapunov function (CLF) approach. We first introduce a CLF for the input constrained case, and then construct the set of all constrained inputs that are feasible with respect to this CLF. The control input is then selected from this "feasible" set. The proposed approach is applied to a simulation scenario, where the UAV is assigned to transition through several targets in the presence of multiple dynamic threats. © 2004 IEEE.},
}

@CONFERENCE{Kaminer19952970,
author={Kaminer, Isaac and Hallberg, Eric N. and Pascoal, Antonio and Silvestre, Carlos},
title={On the design and implementation of a trajectory tracking controller for a fixed wing unmanned air vehicle},
journal={Proceedings of the American Control Conference},
year={1995},
volume={5},
pages={2970-2974},
note={cited By 4},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-0029179717&partnerID=40&md5=0c32378c88936058a008d44cbd0888e1},
abstract={This paper introduces a new methodology for integrated design of guidance and control systems for autonomous vehicles. An application of this methodology to the design of a guidance and control system for a a fixed wing Unmanned Air Vehicle is presented.},
}

